On fitting the Lomax distribution: a comparison between minimum distance estimators and other estimation techniques

In this paper we investigate the performance of a variety of estimation techniques for the scale and shape parameter of the Lomax distribution. These methods include traditional methods such as the maximum likelihood estimator and the method of moments estimator. A version of the maximum likelihood estimator adjusted for bias is also included. Furthermore, alternative moment-based estimation techniques such as the $L$-moment estimator and the probability weighted moments estimator are included along with three different minimum distance estimators. The finite sample performances of each of these estimators is compared via an extensive Monte Carlo study. We find that no single estimator outperforms its competitors uniformly. We recommend one of the minimum distance estimators for use with smaller samples, while a bias reduced version of maximum likelihood estimation is recommended for use with larger samples. In addition, the desirable asymptotic properties of traditional maximum likelihood estimators make them appealing for larger samples. We also include a practical application demonstrating the use of the techniques on observed data.

==> Tables20220525/output/20220607-10h42m32s-Full.beta=6.sig=50.n=40.LaTeX.tex <==
% START DATE AND TIME=20220607-10h42m32s
      \begin{table}[htbp]
  \centering
  \caption{$\beta=6,  \sigma=50$ $n=40$}
  \resizebox{\columnwidth}{!}{
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|r|r|}
      %\cline{2-13}    \multicolumn{1}{r|}{} &       & \multicolumn{11}{c|}{$\beta=6,  \sigma=50$ $n=40$} \\
\cline{2-13}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.CvM}} & \multicolumn{1}{l|}{\textbf{MDE.LS}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.X2}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 6&6&6.7364&8.8871&6.0427&9.1882&30.0055&11.4173&33.7358&6&6.7364
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
50&50&54.3383&73.7593&49.1791&259.4913&428.2926&97.9365&320.3812&50&54.3383
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0&0&56.3308&90.1141&60.3063&2350.5204&1514.3882&304.0232&426080.0721&0&56.3308
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0&0&4259.0705&6856.2703&4582.3873&212172.3918&330753.0137&24748.0518&52987947.3015&0&4259.0705
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0&0&0.7364&2.8871&0.0427&3.1882&24.0055&5.4173&27.7358&0&0.7364
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0&0&4.3383&23.7593&-0.8209&209.4913&378.2926&47.9365&270.3812&0&4.3383
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0&0&56.8675&98.4402&60.3021&2360.4503&2090.4999&333.3403&426806.7403&0&56.8675
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0&0&4277.4655&7420.0894&4582.603&256037.7821&473825.2604&27043.4862&53055754.5263&0&4277.4655
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 0&0&4334.333&7518.5296&4642.9051&258398.2324&475915.7603&27376.8265&53482561.2666&0&4334.333\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0&0&0.0018&0.002&0.0021&1.24021418832306e+300&0.0159&0.0018&0.0017&0&0.0018\\
\hline
\end{tabular}
}
\end{table}

==> Tables20220525/output/output20211203/Full.beta=1.5.sig=1.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=1.5,  \sigma=1$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.671&1.478&1.829&0.986&1.265&1.672&2.793&6.315&1.829
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.182&0.977&1.325&1.550&1.832&1.182&3.152&6.834&1.325
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.435&0.321&0.2958&12.655&8.072&0.435&0.897&$1.300\times10^5$&0.296
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.489&0.361&0.333&22.097&21.125&0.490&1.992&$1.488\times10^5$&0.333
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.172&-0.022&0.329&-0.514&-0.235&0.172&1.293&4.815&0.329
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.182&-0.023&0.325&0.550&0.832&0.182&2.152&5.834&0.325
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.464&0.322&0.404&12.919&8.126&0.465&2.568&$1.300\times10^5$&0.404
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.523&0.362&0.438&22.397&21.814&0.523&6.625&$1.489\times10^5$&0.438
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 0.987&0.684&0.842&35.315&29.940&0.988&9.192&$2.790\times10^5$&0.842\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0011&0.0011&1.8178e+299&0.0349&0.0011&0.0099&7.105&0.0011\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20211203/Full.beta=1.5.sig=1.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=1.5,  \sigma=1$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.5766&1.4937&1.7122&0.8567&1.0134&1.5766&2.5071&2.3073&1.7122
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.0785&0.9917&1.2076&1.132&1.2635&1.0785&2.8011&2.5267&1.2076
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1043&0.0777&0.1126&0.1267&0.1695&0.1043&0.1722&0.1907&0.1126
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.1106&0.081&0.1236&0.231&0.2903&0.1106&5.4485&5.5775&0.1236
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.0766&-0.0063&0.2122&-0.6433&-0.4866&0.0766&1.0071&0.8073&0.2122
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.0785&-0.0083&0.2076&0.132&0.2635&0.0785&1.8011&1.5267&0.2076
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1102&0.0777&0.1576&0.5405&0.4062&0.1102&1.1864&0.8424&0.1576
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.1168&0.081&0.1667&0.2484&0.3597&0.1168&8.6918&7.9077&0.1667
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 0.2269&0.1588&0.3243&0.7889&0.7659&0.2269&9.8782&8.7502&0.3243\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 6e-04&6e-04&6e-04&0.034&0.0266&6e-04&0.0086&0.0085&6e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20211203/Full.beta=1.5.sig=2.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=1.5,  \sigma=2$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.6717&1.4777&1.8289&0.234&1.2571&1.6718&2.7928&6.3149&1.8289
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2.3646&1.9549&2.6507&3.2892&3.6446&2.3647&6.3047&13.6684&2.6507
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.4348&0.3211&0.2958&97.6126&6.7845&0.4353&0.8968&$1.3005\times10^7$&0.2958
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.9567&1.4449&1.33&82.0457&70.7657&1.9587&7.9688& $5.9556\times10^5$ &1.33
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1717&-0.0223&0.3289&-1.266&-0.2429&0.1718&1.2928&4.8149&0.3289
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.3646&-0.0451&0.6507&1.2892&1.6446&0.3647&4.3047&11.6684&0.6507
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.4642&0.3215&0.4039&99.2055&6.8428&0.4648&2.5679&130057.2468&0.4039
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2.0895&1.4468&1.7532&83.6997&73.4633&2.0915&26.4984&595640.9191&1.7532
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 2.5537&1.7683&2.1571&182.9052&80.3061&2.5562&29.0664&725698.1659&2.1571\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0011&0.0011&1.6389e+301&0.0364&0.0011&0.0099&7.105&0.0011\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20211203/Full.beta=1.5.sig=2.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=1.5,  \sigma=2$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.5773&1.4943&1.7089&0.6939&1.008&1.5773&2.5018&2.3274&1.7089
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2.159&1.9853&2.4092&2.3193&2.5171&2.159&5.6067&5.1035&2.4092
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1056&0.0784&0.1141&17.8202&0.1754&0.1056&0.1701&6.7402&0.1141
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.4389&0.3215&0.4932&4.3026&1.1692&0.439&6.9375&30.03&0.4932
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.0773&-0.0057&0.2089&-0.8061&-0.492&0.0773&1.0018&0.8274&0.2089
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.159&-0.0147&0.4092&0.3193&0.5171&0.159&3.6067&3.1035&0.4092
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1116&0.0784&0.1577&18.4682&0.4175&0.1116&1.1737&7.4241&0.1577
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.4641&0.3217&0.6606&4.4042&1.4365&0.4642&19.9449&39.6587&0.6606
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 0.5757&0.4001&0.8183&22.8724&1.854&0.5758&21.1186&47.0828&0.8183\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 6e-04&6e-04&6e-04&1.4897e+300&0.0276&6e-04&0.009&0.0089&6e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20211203/Full.beta=2.5.sig=1.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2.5,  \sigma=1$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 5.757&5.299&3.192&4.308&5.1481&3.451&4.821&8.023&3.192
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2.840&2.592&1.357&3.227&3.766&1.511&2.354&4.034&1.357
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & $4.430\times10^4$&$4.430\times10^4$&8.1780&278.800&316.253&34.019&144.301&2214.145&8.179
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
$1.507\times10^4$&$1.507\times10^4$&2.215&166.884&188.253&9.307&37.535&631.699&2.215
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 3.257&2.799&0.692&1.808&2.648&0.951&2.321&5.523&0.692
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.840&1.592&0.357&2.227&2.766&0.511&1.354&3.034&0.357
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & $4.430\times10^4$&$4.430\times10^4$&8.657&282.040&323.234&34.921&149.674&$2.244\times10^3$&8.657
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
$1.507\times10^4$&$1.507\times10^4$&2.343&171.828&195.884&9.567&39.365&640.844&2.343
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & $5.938\times10^4$&$5.938\times10^4$&10.999&453.869&519.118&44.488&189.040&2885.269&10.999\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.001&0.001&0.001&0.023&0.018&0.001&0.002&8.078&0.001\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20211203/Full.beta=2.5.sig=1.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2.5,  \sigma=1$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.7856&2.4766&2.807&2.0901&2.2794&2.7855&3.6075&3.6549&2.807
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.1543&0.9871&1.1572&1.3786&1.4055&1.1543&1.6804&1.6963&1.1572
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 3.3306&3.0431&2.143&19.057&13.9549&3.3099&5.6748&163.6709&2.143
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.0246&0.941&0.5714&9.6961&7.0162&1.0176&1.7356&55.097&0.5714
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.2856&-0.0234&0.307&-0.4099&-0.2206&0.2855&1.1075&1.1549&0.307
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.1543&-0.0129&0.1572&0.3786&0.4055&0.1543&0.6804&0.6963&0.1572
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 3.4118&3.0433&2.2371&19.2231&14.0022&3.3911&6.9008&164.9883&2.2371
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.0483&0.9411&0.5961&9.8384&7.18&1.0413&2.1983&55.5763&0.5961
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 4.4601&3.9844&2.8331&29.0616&21.1821&4.4324&9.0991&220.5646&2.8331\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&5e-04&5e-04&0.0174&0.0121&5e-04&0.0011&0.002&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20211203/Full.beta=2.5.sig=2.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2.5,  \sigma=2$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 6.548&6.09&3.194&4.107&4.927&3.438&4.822&8.023&3.194
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
6.6213&6.126&2.716&6.142&7.194&3.006&4.709&8.069&2.716
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & $9.029\times10^4$&$9.029\times10^4$&8.307&224.574&256.605&29.777&144.303&2214.144&8.307
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
$1.231\times10^5$&$1.231\times10^5$&8.928&535.7113&611.3656&32.581&150.140&$2.526\times10^3$&8.928
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 4.048&3.59&0.694&1.607&2.427&0.938&2.322&5.5232&0.694
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
4.621&4.126&0.716&4.142&5.194&1.006&2.709&6.069&0.716
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & $9.030\times10^4$&$9.030\times10^4$&8.788&227.132&262.472&30.653&149.677&2244.429&8.788
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
$1.231\times10^5$&$1.231\times10^5$&9.440&552.810&638.279&33.590&157.463&2563.378&9.440
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & $2.134\times10^5$&$2.134\times10^5$&18.228&779.942&900.751&64.243&307.140&4807.806&18.228\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0012&0.001&0.0233&0.0179&0.0011&0.0019&8.078&0.001\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20211203/Full.beta=2.5.sig=2.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2.5,  \sigma=2$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.8064&2.4981&2.78&2.0876&2.2696&2.7727&3.6795&4.1745&2.78
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2.3399&2.006&2.2878&2.771&2.8039&2.2982&3.4542&3.9354&2.2878
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 23.8359&23.5659&0.8157&20.0279&12.6377&3.4327&87.1017&1980.1799&0.8157
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
35.7923&35.4784&0.9441&45.3105&26.4&4.5844&131.8311&2451.1201&0.9441
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.3064&-0.0019&0.28&-0.4124&-0.2304&0.2727&1.1795&1.6745&0.28
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.3399&0.006&0.2878&0.771&0.8039&0.2982&1.4542&1.9354&0.2878
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 23.9274&23.5635&0.8941&20.196&12.6896&3.5067&88.4841&1982.7859&0.8941
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
35.9043&35.4749&1.0268&45.9004&27.0436&4.6729&133.9327&2454.6207&1.0268
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 59.8317&59.0384&1.9209&66.0964&39.7332&8.1796&222.4167&4437.4066&1.9209\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&5e-04&5e-04&0.0173&0.0121&5e-04&0.0011&0.0014&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20211203/Full.beta=2.sig=1.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2,  \sigma=1$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.6316&2.282&2.4461&2.1496&2.7678&2.465&3.6774&9.475&2.4461
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.4271&1.1745&1.3016&2.152&2.6838&1.3282&2.4372&6.5864&1.3016
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 218.3272&218.3939&3.1122&79.2503&106.4854&14.1658&52.8832&$1.5122\times10^5$.7148&3.1122
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
73.3693&73.3817&1.445&90.4216&115.3987&5.9178&22.8539&83548.8529&1.445
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.6316&0.282&0.4461&0.1496&0.7678&0.465&1.6774&7.475&0.4461
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.4271&0.1745&0.3016&1.152&1.6838&0.3282&1.4372&5.5864&0.3016
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 218.7043&218.4515&3.3109&79.2647&107.0642&14.3806&55.6916&$1.5126\times10^5$.4683&3.3109
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
73.5444&73.4048&1.5358&91.7396&118.2225&6.0249&24.9173&83571.7064&1.5358
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 292.2487&291.8564&4.8467&171.0044&225.2867&20.4055&80.609&234831.1746&4.8467\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0011&0.0011&0.0291&0.0229&0.0011&0.0035&0.0115&0.0011\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20211203/Full.beta=2.sig=1.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2,  \sigma=1$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.154&1.9803&2.2268&1.3459&1.5657&2.154&2.9819&2.648&2.2268
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.1104&0.9856&1.1521&1.173&1.2784&1.1103&1.8999&1.6288&1.1521
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.3415&0.218&0.3166&0.6248&0.9345&0.3415&0.5969&2.219&0.3166
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.1695&0.106&0.1569&0.5256&0.8203&0.1695&0.317&1.6695&0.1569
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.154&-0.0197&0.2268&-0.6541&-0.4343&0.154&0.9819&0.648&0.2268
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.1104&-0.0144&0.1521&0.173&0.2784&0.1103&0.8999&0.6288&0.1521
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.3651&0.2183&0.368&1.0526&1.123&0.3651&1.561&2.6387&0.368
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.1816&0.1062&0.18&0.5554&0.8977&0.1816&1.1268&2.0647&0.18
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 0.5468&0.3245&0.548&1.608&2.0207&0.5468&2.6878&4.7034&0.548\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&5e-04&5e-04&0.0228&0.0166&5e-04&0.0024&0.0497&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20211203/Full.beta=2.sig=2.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2,  \sigma=2$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 103.4541&103.1044&2.4444&2.0966&2.6938&2.4574&3.6773&9.4749&2.4444
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
115.7303&115.2251&2.6008&4.1946&5.2177&2.6466&4.8746&13.1729&2.6008
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & $1.019\times10^8$&$1.019\times10^8$&3.0839&65.3916&87.2821&12.1922&52.8831&$1.512\times10^5$&3.0839
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 

1.278&$1.278\times10^8$&5.7198&298.7611&379.0947&20.4378&91.4158&$3.341\times10^5$&5.7198

\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 101.4541&101.1044&0.4444&0.0966&0.6938&0.4574&1.6773&7.4749&0.4444
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
113.7303&113.2251&0.6008&2.1946&3.2177&0.6466&2.8746&11.1729&0.6008
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & $1.019\times10^8$&$1.019\times10^8$&3.2811&65.3944&87.7547&12.4002&55.6912&$1.515\times10^5$&3.2811
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
$1.278\times10^8$&$1.278\times10^8$&6.0801&303.5476&389.4106&20.8539&99.6697&$3.343\times10^5$&6.0801
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & $2.298\times10^8$&$2.297\times10^8$&9.3612&368.9421&477.1654&33.2542&155.3609&$4.855\times10^5$&9.3612\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0011&0.0011&0.0296&0.0232&0.0011&0.0035&0.0115&0.0011\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20211203/Full.beta=2.sig=2.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2,  \sigma=2$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.1565&1.9818&2.2305&1.3626&1.5702&2.1565&2.9942&2.694&2.2305
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2.2209&1.9703&2.3057&2.3768&2.5633&2.2209&3.8094&3.3092&2.3057
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.3432&0.2173&0.3115&1.1138&0.6778&0.343&0.61&4.7661&0.3115
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.6798&0.42&0.619&3.6512&2.1967&0.6795&1.2501&9.5048&0.619
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1565&-0.0182&0.2305&-0.6374&-0.4298&0.1565&0.9942&0.694&0.2305
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.2209&-0.0297&0.3057&0.3768&0.5633&0.2209&1.8094&1.3092&0.3057
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.3677&0.2176&0.3646&1.5199&0.8625&0.3675&1.5985&5.2473&0.3646
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.7285&0.4208&0.7124&3.7929&2.5138&0.7282&4.5239&11.2179&0.7124
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 1.0962&0.6385&1.077&5.3128&3.3763&1.0957&6.1223&16.4652&1.077\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&6e-04&6e-04&0.0226&0.0164&5e-04&0.0024&0.0025&6e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20211203/Full.beta=3.sig=1.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=3,  \sigma=1$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & $1.592\times10^3$&$1.592\times10^3$&4.008&7.278&8.751&4.923&17.486&49.982&4.008
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
672.842&672.629&1.422&4.409&5.167&1.828&6.741&19.565&1.422
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & $1.631\times10^{10}$&$1.631\times10^{10}$&15.395&606.183&720.891&120.234&$3.131\times10^5$&$2.977\times10^6$&15.395
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
$2.959\times10^9$&$2.959\times10^9$&2.944&238.261&276.938&22.260&$4.521\times10^4$&$4.303\times10^5$&2.944
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & $1.589\times10^3$&$1.589\times10^3$&1.008&4.278&5.751&1.923&14.486&46.982&1.008
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
671.842&671.629&0.422&3.409&4.167&0.828&5.741&18.565&0.422
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & $1.631\times10^{10}$&$1.631\times10^{10}$&16.410&624.422&753.897&123.921&$3.133\times10^5$&$2.979\times10^6$&16.410
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
$2.959\times10^9$&$2.959\times10^9$&3.122&249.855&294.278&22.944&$4.524\times10^4$&$4.306\times10^5$&3.122
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & $1.927\times10^{10}$&$1.927\times10^{10}$&19.532&874.278&$1.048\times10^3$&146.865&$3.586\times10^5$&$3.410\times10^6$&19.532\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0012&0.0011&0.02&0.0152&0.0011&0.0014&0.0075&0.0011\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20211203/Full.beta=3.sig=1.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=3,  \sigma=1$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 3.4521&2.9913&3.41&3.3012&3.422&3.4533&4.3185&4.8851&3.41
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.1964&0.9969&1.1708&1.7728&1.7212&1.1968&1.6144&1.8414&1.1708
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 4.8745&4.5431&3.284&95.6529&82.4836&5.1023&7.1332&450.369&3.284
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.8734&0.8103&0.5537&32.1104&25.7957&0.9075&1.2995&83.3832&0.5537
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.4521&-0.0087&0.41&0.3012&0.422&0.4533&1.3185&1.8851&0.41
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.1964&-0.0031&0.1708&0.7728&0.7212&0.1968&0.6144&0.8414&0.1708
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 5.0784&4.5427&3.4518&95.7341&82.6534&5.3072&8.8708&453.8775&3.4518
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.9119&0.8102&0.5828&32.7044&26.3133&0.9462&1.6769&84.0829&0.5828
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 5.9902&5.3529&4.0346&128.4385&108.9667&6.2534&10.5477&537.9604&4.0346\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&5e-04&5e-04&0.0144&0.0098&5e-04&8e-04&0.0016&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20211203/Full.beta=3.sig=2.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=3,  \sigma=2$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & $1.003\times10^3$&$1.003\times10^3$&4.016&6.816&8.232&4.860&17.487&49.989&4.016
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
$1.262\times10^3$&$1.262\times10^3$&2.851&8.249&9.670&3.603&13.484&39.1378&2.851
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & $7.541\times10^9$&$7.541\times10^9$&15.991&$4.809\times10^2$&$5.758\times10^2$&100.860&$3.131\times10^5$&$2.977\times10^6$&15.991
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
$1.313\times10^{10}$&$1.313\times10^{10}$&12.334&759.101&$8.865\times10^2$&75.126&$1.808\times10^6$&$1.721\times10^6$&12.334
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & $1.000\times10^3$&$1.000\times10^3$&1.016&3.816&5.232&1.860&14.487&46.989&1.016
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
$1.260\times10^3$&$1.260\times10^3$&0.851&6.249&7.699&1.603&11.484&37.138&0.851
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & $7.541\times10^9$&$7.541\times10^9$&17.021&$4.954\times10^2$&$6.031\times10^2$&$1.043\times10^2$&$3.133\times10^5$&$2.979\times10^7$&17.021
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
$1.312\times10^{10}$&$1.312\times10^{10}$&13.057&$7.980\times10^2$&$9.457\times10^2$&77.688&$1.810\times10^5$&$1.723\times10^6$&13.057
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & $2.066\times10^{10}$&$2.066\times10^{10}$&30.078&$1.293\times10^3$&$1.548\times10^3$&$1.811\times10^2$ &$4.943\times10^5$&$4.702\times10^5$&30.078\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0012&0.0011&0.0201&0.0151&0.0011&0.0014&0.0075&0.0011\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20211203/Full.beta=3.sig=2.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=3,  \sigma=2$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 3.4732&3.0091&3.4019&3.2172&3.2984&3.4689&4.3339&8.4879&3.4019
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2.4073&2.0066&2.3311&3.4497&3.3088&2.4034&3.238&7.1446&2.3311
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 10.7681&10.4457&3.0192&77.6102&55.2432&9.2863&20.5123&115703.6673&3.0192
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
8.214&7.9699&2.2527&104.9911&71.1442&6.9489&16.6776&107211.533&2.2527
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.4732&0.0091&0.4019&0.2172&0.2984&0.4689&1.3339&5.4879&0.4019
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.4073&0.0066&0.3311&1.4497&1.3088&0.4034&1.238&5.1446&0.3311
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 10.9909&10.4447&3.1804&77.6496&55.3267&9.5052&22.2896&115722.2143&3.1804
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
8.3791&7.9691&2.3622&107.0823&72.8501&7.1109&18.2086&107227.2789&2.3622
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 19.37&18.4138&5.5426&184.7319&128.1767&16.6161&40.4982&222949.4932&5.5426\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&5e-04&5e-04&0.0142&0.0096&5e-04&7e-04&0.0019&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20211203/Full.beta=4.sig=1.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=4,  \sigma=1$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 229.859&229.409&5.724&14.906&17.259&7.516&11.351&40.890&5.724
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
59.821&59.685&1.525&6.416&7.187&2.091&3.332&13.427&1.525
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & $1.989\times10^9$&$1.989\times10^9$&45.639&$1.517\times10^3$&$1.738\times10^3$&232.110&$1.155\times10^4$&$1.921\times10^6$&45.639
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
$1.251\times10^7$&$1.251\times10^7$&4.400&294.047&319.960&23.068&$1.086\times10^3$&$2.706\times10^5$&4.400
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 225.859&225.409&1.724&10.906&13.259&3.516&7.351&36.890&1.724
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
58.821&58.685&0.525&5.416&6.187&1.091&2.332&12.427&0.525
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & $1.989\times10^8$&$1.989\times10^8$&48.608&$1.636\times10^3$&$1.914\times10^3$&244.45&$1.160\times10^4$&$1.922\times10^6$&48.608
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
$1.251\times10^7$&$1.251\times10^7$&4.675&323.348&358.206&24.256&$1.091\times10^3$&$2.707\times10^5$&4.675
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & $2.115\times10^8$&$2.115\times10^8$&53.282&$1.959\times10^3$&$2.272\times10^3$&268.706&$1.270\times10^5$&$2.193\times10^6$&53.282\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0013&0.001&0.0165&0.0123&0.0011&0.0011&$4.041\times10^3$&0.001\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20211203/Full.beta=4.sig=1.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=4,  \sigma=1$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 29.963&29.297&4.873&8.327&7.130&5.459&7.007&12.154&4.873
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
8.834&8.630&1.261&3.240&2.623&1.44&1.938&3.536&1.261
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & $2.427\times10^6$&$2.427\times10^6$&14.638&633.893&422.324&78.341&1484.057&$1.058\times10^4$&14.638
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
$2.260\times10^5$&$2.260\times10^5$&1.333&102.336&65.023&7.206&137.814&$1.081\times10^3$&1.333
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 25.963&25.297&0.873&4.327&3.130&1.459&3.007&8.154&0.873
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
7.834&7.630&0.261&2.240&1.623&0.444&0.938&2.536&0.261
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & $2.427\times10^5$&$2.427\times10^6$&15.400&652.548&432.079&80.462&1492.953&$1.065\times10^4$&15.400
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
$2.260\times10^5$&$2.260\times10^5$&1.401&107.344&67.649&7.402&138.679&$1.087\times10^3$&1.401
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & $2.653\times10^6$&$2.653\times10^6$&16.801&759.892&499.728&87.865&1631.632&$1.173\times10^4$&16.801\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&6e-04&5e-04&0.0112&0.0074&5e-04&6e-04&0.0949&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20211203/Full.beta=4.sig=2.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=4,  \sigma=2$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 177.109&176.659&5.741&13.764&15.949&7.417&11.354&40.909&5.741
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
106.124&105.852&3.059&11.833&13.257&4.119&6.664&26.866&3.059
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & $1.412\times10^8$&$1.412\times10^8$&47.549&1195.06&$1.368\times10^3$&201.271&$1.155\times10^4$&$1.921\times10^6$&47.549
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
$5.196\times10^7$&$5.196\times10^7$&18.254&926.769&$1.007\times10^3$&79.601&$4.346\times10^3$&$1.082\times10^6$&18.254
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 173.109&172.659&1.741&9.764&11.949&3.417&7.354&36.909&1.741
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
104.124&103.852&1.059&9.833&11.257&2.119&4.664&24.866&1.059
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & $1.412\times10^8$&$1.412\times10^8$&50.574&$1.290\times10^3$&$1.511\times10^3$&212.927&$1.160\times10^4$&$1.922\times10^6$&50.574
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
$5.197\times10^7$&$5.197\times10^7$&19.373&$1.023\times10^3$&$1.134\times10^3$&84.083&$4.367\times10^3$&$1.082\times10^6$&19.373
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & $1.932\times10^8$&$1.932\times10^8$&69.947&2313.6500&$2.645\times10^3$&297.009&$1.598\times10^4$&$3.005\times10^6$&69.947\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0012&0.001&0.0165&0.0123&0.0011&0.0011&4041.9544&0.001\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20211203/Full.beta=4.sig=2.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=4,  \sigma=2$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 14.9729&14.2991&4.9305&8.046&7.0196&5.3852&6.5617&11.6498&4.9305
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
8.8771&8.4652&2.5572&6.2483&5.1431&2.8481&3.6051&6.7936&2.5572
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & $3.086\times10^5$&$3.087\times10^5$&18.136&515.4033&358.8741&54.6722&237.555&7060.1858&18.136
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
$1.229\times10^5$&$1.229\times10^5$&6.8178&332.5523&219.6157&21.0787&91.8223&2787.1797&6.8178
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 10.9729&10.2991&0.9305&4.046&3.0196&1.3852&2.5617&7.6498&0.9305
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
6.8771&6.4652&0.5572&4.2483&3.1431&0.8481&1.6051&4.7936&0.5572
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & $3.088\times10^5$&$3.088\times10^5$&19&531.7221&367.956&56.5855&244.0935&7117.9991&19
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
$1.230\times10^5$&$1.230\times10^5$&7.1276&350.5672&229.4729&21.7959&94.3894&2809.8792&7.1276
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & $4.317\times10^5$&$4.317\times10^5$&26.1277&882.2893&597.4289&78.3814&338.4829&9927.8782&26.1277\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&6e-04&5e-04&0.0112&0.0074&5e-04&6e-04&0.0123&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20211203/Full.beta=5.sig=1.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=5,  \sigma=1$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 78.422&78.054&7.316&22.015&24.361&10.262&16.759&47.237&7.316
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
18.743&18.657&1.540&7.232&7.768&2.237&3.755&10.983&1.540
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & $4.838\times10^6$&$4.838\times10^6$&95.932&$2.406\times10^3$&$2.595\times10^3$&410.308&$1.851\times10^4$&$2.578\times10^5$&95.932
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
$2.78\times10^5$&$2.783\times10^5$&5.335&268.900&278.125&22.596&$1.037\times10^3$&$1.545\times10^4$&5.335
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 73.422&73.054&2.316&17.015&19.361&5.262&11.759&42.237&2.316
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
17.743&17.657&0.540&6.232&6.768&1.237&2.755&9.983&0.540
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & $4.843\times10^6$&$4.843\times10^6$&101.288&$2.696\times10^3$&$2.969\times10^3$&437.955&$1.873\times10^4$&$2.596\times10^5$&101.288
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
$2.786\times10^5$&$2.786\times10^5$&5.626&307.714&323.902&24.123&$1.044\times10^3$&$1.555\times10^4$&5.626
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & $5.121\times10^6$&$5.121\times10^6$&106.913&$3.003\times10^3$&$3.293\times10^3$&462.079&$1.978\times10^4$&$2.751\times10^5$&106.913\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.001&0.0012&0.001&0.0145&0.0106&0.001&0.001&$5.156\times10^{29}$&0.001\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20211203/Full.beta=5.sig=1.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=5,  \sigma=1$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 44.551&43.830&6.688&15.433&12.135&7.721&16.158&39.216&6.688
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
10.756&10.586&1.396&4.678&3.487&1.640&3.659&9.267&1.396
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & $6.973\times10^6$&$6.973\times10^6$&54.441&1484.548&974.418&179.685&$3.523\times10^5$&$1.489\times10^6$&54.441
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
$4.411\times10^5$&$4.410\times10^5$&3.151&142.291&88.118&9.789&$1.995\times10^4$&$8.521\times10^4$&3.151
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 39.551&38.830&1.688&10.433&7.135&2.721&11.158&34.216&1.688
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
9.756&9.586&0.396&3.678&2.487&0.640&2.659&8.267&0.396
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & $6.974\times10^6$&$6.974\times10^6$&57.286&1593.243&1025.232&187.07&$3.524\times10^5$&$1.490\times10^6$&57.286
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
$4.411\times10^5$&$4.411\times10^5$&3.308&155.802&94.292&10.197&$1.995\times10^4$&$8.527\times10^4$&3.308
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & $7.415\times10^6$&$7.415\times10^6$&60.594&$1.749\times10^3$&$1.119\times10^3$&197.267&$3.723\times10^5$&$1.575\times10^6$&60.594\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&6e-04&5e-04&0.0097&0.0064&5e-04&5e-04&0.4691&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20211203/Full.beta=5.sig=2.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=5,  \sigma=2$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & $4.959\times10^3$&$4.958\times10^3$&7.263&20.087&22.230&10.049&16.717&47.149&7.263
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
$2.374\times10^3$&$2.374\times10^3$&3.057&13.182&14.154&4.376&7.492&21.927&3.057
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & $1.031\times10^{11}$&$1.031\times10^{11}$&86.483&1864.66&2002.949&347.215&$1.858\times10^4$&$2.578\times10^5$&86.483
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
$2.399\times10^{10}$&$2.399\times10^{10}$&19.439&833.253&859.947&76.953&$4.147\times10^3$&$6.178\times10^4$&19.439
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & $4.954\times10^3$&$4.953\times10^3$&2.263&15.087&17.230&5.049&11.717&42.149&2.263
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
$2.372\times10^3$&$2.372\times10^3$&1.057&11.182&12.154&2.376&5.492&19.927&1.057
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & $1.031\times10^{11}$&$1.031\times10^{11}$&91.593&2092.093&2299.618&372.671&$1.872\times10^4$&$2.596\times10^5$&91.593
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
$2.400\times10^9$&$2.400\times10^9$&20.553&958.206&1007.57&82.59&4176.959&$6.217\times10^4$&20.553
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & $1.271\times10^{11}$&$1.271\times10^{11}$&112.146&3050.299&3307.188&455.261&$2.290\times10^4$&$3.217\times10^5$&112.146\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.001&0.0012&0.001&0.0144&0.0106&0.001&0.001&$5.156\times10^{29}$&0.001\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20211203/Full.beta=5.sig=2.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=5,  \sigma=2$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 995.7048&994.9784&6.6169&13.8066&11.4882&7.5936&9.8604&21.1304&6.6169
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
459.6994&459.3569&2.7628&8.3687&6.6047&3.2299&4.3224&9.6474&2.7628
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & $8.308\times10^9$&$8.308\times10^9$&54.832&1094.5432&782.9964&155.9208&2093.5179&$2.348\times10^3$&54.832
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
$1.759\times10^9$&$1.759\times10^9$&12.6917&422.6287&285.3483&34.9893&476.0555&5533.9893&12.6917
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 990.7048&989.9784&1.6169&8.8066&6.4882&2.5936&4.8604&16.1304&1.6169
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
457.6994&457.3569&0.7628&6.3687&4.6047&1.2299&2.3224&7.6474&0.7628
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & $8.308\times10^9$&$8.308\times10^9$&57.4409&1171.9906&825.0151&162.6318&2116.9321&$2.374\times10^4$&57.4409
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
$1.759\times10^9$&$1.759\times10^9$&13.2723&463.1467&306.5231&36.4986&481.4013&$5.591\times10^3$&13.2723
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & $1.007\times10^{10}$&$1.007\times10{10}$&70.7132&1635.1373&1131.5381&199.1304&2598.3333&$2.933\times10^4$&70.7132\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&6e-04&5e-04&0.0097&0.0063&5e-04&5e-04&0.0464&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20211209/Full.beta=1.5.sig=3.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=1.5,  \sigma=3$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.6717&1.4777&1.8288&-1.8659&1.2349&1.6717&2.7927&6.3149&1.8288
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
3.5467&2.9322&3.976&5.2184&5.488&3.5467&9.4574&20.5029&3.976
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.4346&0.3209&0.2958&347.7844&6.2223&0.4353&0.8967&130047.0665&0.2958
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
4.3993&3.2473&2.9924&173.3936&144.6706&4.4068&17.9315&1340019.7055&2.9924
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1717&-0.0223&0.3288&-3.3659&-0.2651&0.1717&1.2927&4.8149&0.3288
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.5467&-0.0678&0.976&2.2184&2.488&0.5467&6.4574&17.5029&0.976
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.464&0.3213&0.4039&359.079&6.292&0.4647&2.5678&130057.2449&0.4039
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
4.6976&3.2516&3.9447&178.2978&150.8462&4.7053&59.6278&1340192.0551&3.9447
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 5.1617&3.5729&4.3485&537.3768&157.1382&5.17&62.1955&1470249.3&4.3485\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0011&0.0011&2.9905720362169e+301&0.0459&0.0011&0.0099&7.105&0.0011\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20211209/Full.beta=1.5.sig=3.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=1.5,  \sigma=3$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.5785&1.4956&1.7062&0.1803&0.999&1.5786&2.4961&2.2972&1.7062
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
3.2472&2.9864&3.6115&3.6504&3.782&3.2472&8.3574&7.5313&3.6115
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.102&0.0772&0.1121&70.9804&0.1794&0.102&0.1651&0.2616&0.1121
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.9824&0.7293&1.1199&12.4364&2.6144&0.9826&13.6487&14.5473&1.1199
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.0785&-0.0044&0.2062&-1.3197&-0.501&0.0786&0.9961&0.7972&0.2062
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.2472&-0.0136&0.6115&0.6504&0.782&0.2472&5.3574&4.5313&0.6115
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1081&0.0772&0.1547&72.7148&0.4304&0.1081&1.1573&0.8971&0.1547
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.0435&0.7294&1.4938&12.8581&3.2257&1.0436&42.3491&35.0789&1.4938
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 1.1516&0.8066&1.6484&85.5729&3.6561&1.1517&43.5065&35.976&1.6484\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 6e-04&6e-04&6e-04&9.84390650739107e+300&0.0309&6e-04&0.0089&0.0103&6e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20211209/Full.beta=2.5.sig=3.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2.5,  \sigma=3$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 4.7807&4.3235&3.1958&4.0175&4.8287&3.4298&4.8214&7.9937&3.1958
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
6.5717&5.8284&4.0776&9.0167&10.566&4.4977&7.0633&12.0647&4.0776
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 15882.1799&15883.9312&8.3445&201.5068&230.7047&27.8278&144.3027&2205.727&8.3445
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
36919.3023&36923.6478&20.2358&1089.1693&1237.7166&68.5196&337.8156&5670.6747&20.2358
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.2807&1.8235&0.6958&1.5175&2.3287&0.9298&2.3214&5.4937&0.6958
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
3.5717&2.8284&1.0776&6.0167&7.566&1.4977&4.0633&9.0647&1.0776
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 15885.7934&15885.668&8.8279&203.7893&236.1046&28.6896&149.6771&2235.6866&8.8279
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
36928.3674&36927.9553&21.395&1125.2616&1294.8367&70.7557&354.2926&5752.2769&21.395
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 52814.1608&52813.6233&30.2229&1329.0509&1530.9413&99.4453&503.9697&7987.9635&30.2229\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0012&0.0011&0.0234&0.0179&0.0011&0.0019&8.078&0.0011\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20211209/Full.beta=2.5.sig=3.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2.5,  \sigma=3$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.7515&2.4469&2.7837&2.0421&2.2717&2.7515&3.5617&3.3358&2.7837
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
3.4066&2.9124&3.4336&4.0356&4.2022&3.4066&4.9634&4.5212&3.4336
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.1148&0.8288&1.1971&15.9872&12.5378&1.1163&1.7736&43.7513&1.1971
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2.9795&2.2217&3.0673&72.657&54.457&2.9841&4.792&110.8481&3.0673
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.2515&-0.0531&0.2837&-0.4579&-0.2283&0.2515&1.0617&0.8358&0.2837
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.4066&-0.0876&0.4336&1.0356&1.2022&0.4066&1.9634&1.5212&0.4336
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.1779&0.8316&1.2774&16.1953&12.5887&1.1794&2.9006&44.4455&1.2774
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
3.1445&2.2291&3.255&73.7222&55.8969&3.1491&8.6465&113.1512&3.255
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 4.3224&3.0607&4.5324&89.9174&68.4856&4.3285&11.5471&157.5967&4.5324\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&5e-04&5e-04&0.0174&0.0121&5e-04&0.0011&0.0017&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20211209/Full.beta=2.sig=3.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2,  \sigma=3$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.5428&2.1932&2.4461&2.0099&2.6563&2.4547&3.6775&9.4751&2.4461
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
4.1138&3.3559&3.9049&6.227&7.7111&3.9647&7.312&19.7596&3.9049
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 74.8613&74.8659&3.1121&65.3242&78.4711&11.3227&52.8831&151218.7131&3.1121
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
225.1618&225.0196&13.005&604.2028&766.9694&42.7687&205.6852&751939.6683&13.005
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.5428&0.1932&0.4461&0.0099&0.6563&0.4547&1.6775&7.4751&0.4461
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.1138&0.3559&0.9049&3.227&4.7111&0.9647&4.312&16.7596&0.9049
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 75.1485&74.8957&3.3109&65.3177&78.894&11.5283&55.6919&151259.4685&3.3109
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
226.3797&225.1238&13.8227&614.5561&789.0876&43.6951&224.2577&752145.3587&13.8227
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 301.5282&300.0196&17.1335&679.8738&867.9815&55.2234&279.9497&903404.8272&17.1335\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0011&0.0011&2.00401541349742e+299&0.0234&0.0011&0.0035&0.0115&0.0011\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20211209/Full.beta=2.sig=3.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2,  \sigma=3$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.1373&1.9682&2.2158&1.3247&1.5624&2.1373&2.9724&2.688&2.2158
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
3.2893&2.9262&3.426&3.5201&3.8321&3.2893&5.6659&4.9399&3.426
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.2966&0.1915&0.3034&4.2861&2.0351&0.2967&0.5319&5.3983&0.3034
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.3227&0.841&1.348&14.8621&18.7618&1.3231&2.4981&22.9532&1.348
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1373&-0.0318&0.2158&-0.6753&-0.4376&0.1373&0.9724&0.688&0.2158
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.2893&-0.0738&0.426&0.5201&0.8321&0.2893&2.6659&1.9399&0.426
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.3154&0.1925&0.35&4.7418&2.2264&0.3155&1.4774&5.8711&0.35
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.4063&0.8464&1.5293&15.1311&19.4523&1.4067&9.6048&26.714&1.5293
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 1.7216&1.0389&1.8793&19.8729&21.6786&1.7222&11.0822&32.5851&1.8793\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&5e-04&5e-04&3.22760432783316e+298&0.0166&5e-04&0.0024&0.0024&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20211209/Full.beta=3.sig=3.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=3,  \sigma=3$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 27.182&26.688&4.008&6.616&7.953&4.827&17.487&49.982&4.008
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
35.495&34.855&4.266&11.991&14.034&5.362&20.224&58.696&4.266
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & $6.983\times10^5$&$6.983\times10^5$&15.395&428.368&507.968&92.179&$31.314\times10^4$&$2.977\times10^6$&15.395
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
$1.308\times10^6$&$1.308\times10^6$&26.499&1517.464&1760.857&154.959&$4.069\times10^4$&$3.873\times10^6$&26.499
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 24.182&23.688&1.008&3.616&4.953&1.827&14.487&46.982&1.008
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
32.495&31.855&1.266&8.991&11.034&2.362&17.224&55.696&1.266
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & $6.988\times10^5$&$6.988\times10^5$&16.411&441.401&532.447&95.508&$3.133\times10^5$&$2.979\times10^6$&16.411
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
$1.309\times10^6$&$1.309\times10^6$&28.099&1598.149&1882.436&160.523&$4.072\times10^5$&$3.876\times10^5$&28.099
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & $2.007\times10^6$&$2.007\times10^6$&44.509&2039.550&2414.884&256.031&$7.205\times10^5$&$6.855\times10^6$&44.509\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0012&0.0011&0.02&0.0151&0.0011&0.0014&0.0075&0.0011\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20211209/Full.beta=3.sig=3.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=3,  \sigma=3$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 3.5156&3.0508&3.4446&3.2679&3.1909&3.4894&4.4027&5.6905&3.4446
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
3.6657&3.0621&3.5561&5.2495&4.7617&3.6344&4.9381&6.6915&3.5561
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 22.7525&22.4583&3.7091&79.1386&38.5003&7.4321&73.0245&7346.8227&3.7091
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
33.8467&33.324&5.9938&234.3238&105.4918&11.9468&106.7633&15133.3918&5.9938
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.5156&0.0508&0.4446&0.2679&0.1909&0.4894&1.4027&2.6905&0.4446
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.6657&0.0621&0.5561&2.2495&1.7617&0.6344&1.9381&3.6915&0.5561
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 23.0161&22.4586&3.9064&79.2024&38.5329&7.6708&74.9848&7353.3268&3.9064
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
34.2865&33.3245&6.3025&239.3607&108.5849&12.348&110.5088&15145.5054&6.3025
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 57.3026&55.7831&10.2089&318.5632&147.1178&20.0189&185.4937&22498.8322&10.2089\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&5e-04&5e-04&0.0143&0.0096&5e-04&7e-04&0.0018&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20211209/Full.beta=4.sig=3.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=4,  \sigma=3$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 83.767&83.318&5.705&13.170&15.255&7.365&11.348&40.896&5.705
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
71.494&71.085&4.558&16.970&19.010&6.13&9.992&40.289&4.558
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & $1.500\times10^7$&$1.500\times10^7$&43.518&1047.143&1197.293&187.318&11556.845&1921162.498&43.5178
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
9680578.6742&9680635.267&38.45&1827.012&1987.338&166.381&9778.886&2434977.4899&38.45
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 79.7671&79.3177&1.7045&9.1701&11.2553&3.3646&7.3482&36.8961&1.7045
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
68.4943&68.0854&1.5584&13.9696&16.0101&3.13&6.9923&37.2887&1.5584
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 15000086.3584&15000087.2893&46.4187&1131.1292&1323.8547&198.6199&11609.6845&1922331.7038&46.4187
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
9684302.0905&9684302.824&40.8749&2021.9805&2243.4632&176.1611&9826.7997&2436124.4379&40.8749
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 24684388.4489&24684390.1133&87.2936&3153.1097&3567.3179&374.781&21436.4843&4358456.1416&87.2936\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0012&0.001&0.0165&0.0123&0.0011&0.0011&4041.9544&0.001\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20211209/Full.beta=4.sig=3.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=4,  \sigma=3$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 5.427&4.758&4.908&7.479&6.799&5.245&6.634&13.662&4.908
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
4.322&3.707&3.824&8.729&7.517&4.151&5.490&12.359&3.824
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 245.888&247.178&17.205&406.858&306.747&38.584&544.091&40203.413&17.205
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
213.225&214.297&14.555&597.792&438.340&32.895&474.575&$4.448\times10^4$&14.555
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.427&0.758&0.908&3.479&2.799&1.245&2.634&9.662&0.9083
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.322&0.707&0.824&5.729&4.517&1.151&2.490&9.359&0.824
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 247.900&247.727&18.028&418.923&314.55&40.130&550.976&$4.029\times10^4$&18.028
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
214.951&214.775&15.233&630.558&458.698&34.217&480.729&$4.456\times10^4$&15.233
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 462.851&462.503&33.261&1049.481&773.248&74.347&1031.705&$8.486\times10^4$&33.261\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&6e-04&5e-04&0.0111&0.0074&5e-04&6e-04&0.0029&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20211209/Full.beta=5.sig=3.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=5,  \sigma=3$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 330.677&330.308&7.225&19.162&21.221&9.944&16.706&47.001&7.225
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
243.212&242.955&4.558&18.859&20.249&6.491&11.231&32.799&4.558
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & $4.904\times10^8$&$4.904\times10^8$&82.222&1627.212&1745.490&319.039&$1.858\times10^4$&$2.577\times10^5$&82.222
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
$2.731\times10^8$&$2.731\times10^8$&41.493&1639.205&1688.045&159.497&9330.658&$1.390\times10^6$&41.493
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 325.677&325.308&2.225&14.162&16.221&4.944&11.706&42.001&2.225
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
240.212&239.955&1.558&15.859&17.249&3.491&8.231&29.799&1.558
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & $4.905\times10^8$&$4.905\times10^8$&87.163&1827.606&2008.422&343.449&$1.872\times10^4$&$2.594\times10^5$&87.163
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
$2.731\times10^8$&$2.731\times10^8$&43.917&1890.532&1985.410&171.669&9397.466&$1.398\times10^5$&43.917
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & $7.636\times10^8$&$7.636\times10^8$&131.080&3718.139&3993.832&515.118&$2.812\times10^4$&$3.993\times10^5$&131.080\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.001&0.0012&0.001&0.0144&0.0106&0.001&0.001&5.156e+29&0.001\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20211209/Full.beta=5.sig=3.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=5,  \sigma=3$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 25.551&24.843&6.720&13.577&10.983&7.552&9.766&21.596&6.720
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
16.857&16.357&4.207&12.296&9.428&4.806&6.402&14.822&4.207
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & $2.309\times10^6$&$2.309\times10^6$&56.354&992.309&667.685&123.737&2723.685&$3.070\times10^4$&56.354
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
$9.982\times10^5$&$9.982\times10^5$&28.579&854.677&546.609&62.363&1332.402&$1.564\times10^4$&28.579
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 20.551&19.843&1.720&8.577&5.983&2.552&4.766&16.596&1.720
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
13.857&13.357&1.207&9.296&6.428&1.806&3.402&11.822&1.207
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & $2.310\times10^6$&$2.310\times10^6$&59.307&1065.770&703.416&130.236&2746.128&$3.098\times10^4$&59.307
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
$9.983\times10^5$&$9.983\times10^5$&30.034&941.001&587.868&65.62&1343.845&$1.577\times10^4$&30.034
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & $3.308\times10^6$&$3.308\times10^6$&89.341&2006.771&1291.284&195.856&4089.973&$4.675\times10^4$&89.341\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&6e-04&5e-04&0.0096&0.0062&5e-04&5e-04&2.018&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20211209/accuracy.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Thu Dec 09 15:29:32 2021
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & Measure & beta=1.5 & sigma=3 & n=100 & 5.16 \\ 
  2 & MLE.b & Measure & beta=1.5 & sigma=3 & n=100 & 3.57 \\ 
  3 & LME & Measure & beta=1.5 & sigma=3 & n=100 & 4.35 \\ 
  4 & MDE.Phi.chisq & Measure & beta=1.5 & sigma=3 & n=100 & 537.38 \\ 
  5 & MDE.Phi.tv & Measure & beta=1.5 & sigma=3 & n=100 & 157.14 \\ 
  6 & MDE.Phi.kl & Measure & beta=1.5 & sigma=3 & n=100 & 5.17 \\ 
  7 & MME & Measure & beta=1.5 & sigma=3 & n=100 & 62.20 \\ 
  8 & MME.b & Measure & beta=1.5 & sigma=3 & n=100 & 1470249.30 \\ 
  9 & PWM & Measure & beta=1.5 & sigma=3 & n=100 & 4.35 \\ 
  10 & MLE & Measure & beta=2 & sigma=3 & n=100 & 301.53 \\ 
  11 & MLE.b & Measure & beta=2 & sigma=3 & n=100 & 300.02 \\ 
  12 & LME & Measure & beta=2 & sigma=3 & n=100 & 17.13 \\ 
  13 & MDE.Phi.chisq & Measure & beta=2 & sigma=3 & n=100 & 679.87 \\ 
  14 & MDE.Phi.tv & Measure & beta=2 & sigma=3 & n=100 & 867.98 \\ 
  15 & MDE.Phi.kl & Measure & beta=2 & sigma=3 & n=100 & 55.22 \\ 
  16 & MME & Measure & beta=2 & sigma=3 & n=100 & 279.95 \\ 
  17 & MME.b & Measure & beta=2 & sigma=3 & n=100 & 903404.83 \\ 
  18 & PWM & Measure & beta=2 & sigma=3 & n=100 & 17.13 \\ 
  19 & MLE & Measure & beta=2.5 & sigma=3 & n=100 & 52814.16 \\ 
  20 & MLE.b & Measure & beta=2.5 & sigma=3 & n=100 & 52813.62 \\ 
  21 & LME & Measure & beta=2.5 & sigma=3 & n=100 & 30.22 \\ 
  22 & MDE.Phi.chisq & Measure & beta=2.5 & sigma=3 & n=100 & 1329.05 \\ 
  23 & MDE.Phi.tv & Measure & beta=2.5 & sigma=3 & n=100 & 1530.94 \\ 
  24 & MDE.Phi.kl & Measure & beta=2.5 & sigma=3 & n=100 & 99.45 \\ 
  25 & MME & Measure & beta=2.5 & sigma=3 & n=100 & 503.97 \\ 
  26 & MME.b & Measure & beta=2.5 & sigma=3 & n=100 & 7987.96 \\ 
  27 & PWM & Measure & beta=2.5 & sigma=3 & n=100 & 30.22 \\ 
  28 & MLE & Measure & beta=3 & sigma=3 & n=100 & 2007498.12 \\ 
  29 & MLE.b & Measure & beta=3 & sigma=3 & n=100 & 2007498.58 \\ 
  30 & LME & Measure & beta=3 & sigma=3 & n=100 & 44.51 \\ 
  31 & MDE.Phi.chisq & Measure & beta=3 & sigma=3 & n=100 & 2039.55 \\ 
  32 & MDE.Phi.tv & Measure & beta=3 & sigma=3 & n=100 & 2414.88 \\ 
  33 & MDE.Phi.kl & Measure & beta=3 & sigma=3 & n=100 & 256.03 \\ 
  34 & MME & Measure & beta=3 & sigma=3 & n=100 & 720485.16 \\ 
  35 & MME.b & Measure & beta=3 & sigma=3 & n=100 & 6855115.95 \\ 
  36 & PWM & Measure & beta=3 & sigma=3 & n=100 & 44.51 \\ 
  37 & MLE & Measure & beta=4 & sigma=3 & n=100 & 24684388.45 \\ 
  38 & MLE.b & Measure & beta=4 & sigma=3 & n=100 & 24684390.11 \\ 
  39 & LME & Measure & beta=4 & sigma=3 & n=100 & 87.29 \\ 
  40 & MDE.Phi.chisq & Measure & beta=4 & sigma=3 & n=100 & 3153.11 \\ 
  41 & MDE.Phi.tv & Measure & beta=4 & sigma=3 & n=100 & 3567.32 \\ 
  42 & MDE.Phi.kl & Measure & beta=4 & sigma=3 & n=100 & 374.78 \\ 
  43 & MME & Measure & beta=4 & sigma=3 & n=100 & 21436.48 \\ 
  44 & MME.b & Measure & beta=4 & sigma=3 & n=100 & 4358456.14 \\ 
  45 & PWM & Measure & beta=4 & sigma=3 & n=100 & 87.29 \\ 
  46 & MLE & Measure & beta=5 & sigma=3 & n=100 & 763611716.62 \\ 
  47 & MLE.b & Measure & beta=5 & sigma=3 & n=100 & 763611718.74 \\ 
  48 & LME & Measure & beta=5 & sigma=3 & n=100 & 131.08 \\ 
  49 & MDE.Phi.chisq & Measure & beta=5 & sigma=3 & n=100 & 3718.14 \\ 
  50 & MDE.Phi.tv & Measure & beta=5 & sigma=3 & n=100 & 3993.83 \\ 
  51 & MDE.Phi.kl & Measure & beta=5 & sigma=3 & n=100 & 515.12 \\ 
  52 & MME & Measure & beta=5 & sigma=3 & n=100 & 28119.35 \\ 
  53 & MME.b & Measure & beta=5 & sigma=3 & n=100 & 399288.17 \\ 
  54 & PWM & Measure & beta=5 & sigma=3 & n=100 & 131.08 \\ 
  55 & MLE & Measure & beta=1.5 & sigma=3 & n=200 & 1.15 \\ 
  56 & MLE.b & Measure & beta=1.5 & sigma=3 & n=200 & 0.81 \\ 
  57 & LME & Measure & beta=1.5 & sigma=3 & n=200 & 1.65 \\ 
  58 & MDE.Phi.chisq & Measure & beta=1.5 & sigma=3 & n=200 & 85.57 \\ 
  59 & MDE.Phi.tv & Measure & beta=1.5 & sigma=3 & n=200 & 3.66 \\ 
  60 & MDE.Phi.kl & Measure & beta=1.5 & sigma=3 & n=200 & 1.15 \\ 
  61 & MME & Measure & beta=1.5 & sigma=3 & n=200 & 43.51 \\ 
  62 & MME.b & Measure & beta=1.5 & sigma=3 & n=200 & 35.98 \\ 
  63 & PWM & Measure & beta=1.5 & sigma=3 & n=200 & 1.65 \\ 
  64 & MLE & Measure & beta=2 & sigma=3 & n=200 & 1.72 \\ 
  65 & MLE.b & Measure & beta=2 & sigma=3 & n=200 & 1.04 \\ 
  66 & LME & Measure & beta=2 & sigma=3 & n=200 & 1.88 \\ 
  67 & MDE.Phi.chisq & Measure & beta=2 & sigma=3 & n=200 & 19.87 \\ 
  68 & MDE.Phi.tv & Measure & beta=2 & sigma=3 & n=200 & 21.68 \\ 
  69 & MDE.Phi.kl & Measure & beta=2 & sigma=3 & n=200 & 1.72 \\ 
  70 & MME & Measure & beta=2 & sigma=3 & n=200 & 11.08 \\ 
  71 & MME.b & Measure & beta=2 & sigma=3 & n=200 & 32.59 \\ 
  72 & PWM & Measure & beta=2 & sigma=3 & n=200 & 1.88 \\ 
  73 & MLE & Measure & beta=2.5 & sigma=3 & n=200 & 4.32 \\ 
  74 & MLE.b & Measure & beta=2.5 & sigma=3 & n=200 & 3.06 \\ 
  75 & LME & Measure & beta=2.5 & sigma=3 & n=200 & 4.53 \\ 
  76 & MDE.Phi.chisq & Measure & beta=2.5 & sigma=3 & n=200 & 89.92 \\ 
  77 & MDE.Phi.tv & Measure & beta=2.5 & sigma=3 & n=200 & 68.49 \\ 
  78 & MDE.Phi.kl & Measure & beta=2.5 & sigma=3 & n=200 & 4.33 \\ 
  79 & MME & Measure & beta=2.5 & sigma=3 & n=200 & 11.55 \\ 
  80 & MME.b & Measure & beta=2.5 & sigma=3 & n=200 & 157.60 \\ 
  81 & PWM & Measure & beta=2.5 & sigma=3 & n=200 & 4.53 \\ 
  82 & MLE & Measure & beta=3 & sigma=3 & n=200 & 57.30 \\ 
  83 & MLE.b & Measure & beta=3 & sigma=3 & n=200 & 55.78 \\ 
  84 & LME & Measure & beta=3 & sigma=3 & n=200 & 10.21 \\ 
  85 & MDE.Phi.chisq & Measure & beta=3 & sigma=3 & n=200 & 318.56 \\ 
  86 & MDE.Phi.tv & Measure & beta=3 & sigma=3 & n=200 & 147.12 \\ 
  87 & MDE.Phi.kl & Measure & beta=3 & sigma=3 & n=200 & 20.02 \\ 
  88 & MME & Measure & beta=3 & sigma=3 & n=200 & 185.49 \\ 
  89 & MME.b & Measure & beta=3 & sigma=3 & n=200 & 22498.83 \\ 
  90 & PWM & Measure & beta=3 & sigma=3 & n=200 & 10.21 \\ 
  91 & MLE & Measure & beta=4 & sigma=3 & n=200 & 462.85 \\ 
  92 & MLE.b & Measure & beta=4 & sigma=3 & n=200 & 462.50 \\ 
  93 & LME & Measure & beta=4 & sigma=3 & n=200 & 33.26 \\ 
  94 & MDE.Phi.chisq & Measure & beta=4 & sigma=3 & n=200 & 1049.48 \\ 
  95 & MDE.Phi.tv & Measure & beta=4 & sigma=3 & n=200 & 773.25 \\ 
  96 & MDE.Phi.kl & Measure & beta=4 & sigma=3 & n=200 & 74.35 \\ 
  97 & MME & Measure & beta=4 & sigma=3 & n=200 & 1031.71 \\ 
  98 & MME.b & Measure & beta=4 & sigma=3 & n=200 & 84856.35 \\ 
  99 & PWM & Measure & beta=4 & sigma=3 & n=200 & 33.26 \\ 
  100 & MLE & Measure & beta=5 & sigma=3 & n=200 & 3307858.88 \\ 
  101 & MLE.b & Measure & beta=5 & sigma=3 & n=200 & 3307860.15 \\ 
  102 & LME & Measure & beta=5 & sigma=3 & n=200 & 89.34 \\ 
  103 & MDE.Phi.chisq & Measure & beta=5 & sigma=3 & n=200 & 2006.77 \\ 
  104 & MDE.Phi.tv & Measure & beta=5 & sigma=3 & n=200 & 1291.28 \\ 
  105 & MDE.Phi.kl & Measure & beta=5 & sigma=3 & n=200 & 195.86 \\ 
  106 & MME & Measure & beta=5 & sigma=3 & n=200 & 4089.97 \\ 
  107 & MME.b & Measure & beta=5 & sigma=3 & n=200 & 46750.02 \\ 
  108 & PWM & Measure & beta=5 & sigma=3 & n=200 & 89.34 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20211209/accuracy2.LaTeX.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Thu Dec 09 15:29:32 2021
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & Measure & beta=1.5 & sigma=3 & n=100 & 0.00 \\ 
  2 & MLE.b & Measure & beta=1.5 & sigma=3 & n=100 & 0.00 \\ 
  3 & LME & Measure & beta=1.5 & sigma=3 & n=100 & 0.00 \\ 
  4 & MDE.Phi.chisq & Measure & beta=1.5 & sigma=3 & n=100 & 29840.00 \\ 
  5 & MDE.Phi.tv & Measure & beta=1.5 & sigma=3 & n=100 & 0.05 \\ 
  6 & MDE.Phi.kl & Measure & beta=1.5 & sigma=3 & n=100 & 0.00 \\ 
  7 & MME & Measure & beta=1.5 & sigma=3 & n=100 & 0.01 \\ 
  8 & MME.b & Measure & beta=1.5 & sigma=3 & n=100 & 7.11 \\ 
  9 & PWM & Measure & beta=1.5 & sigma=3 & n=100 & 0.00 \\ 
  10 & MLE & Measure & beta=2 & sigma=3 & n=100 & 0.00 \\ 
  11 & MLE.b & Measure & beta=2 & sigma=3 & n=100 & 0.00 \\ 
  12 & LME & Measure & beta=2 & sigma=3 & n=100 & 0.00 \\ 
  13 & MDE.Phi.chisq & Measure & beta=2 & sigma=3 & n=100 & 20.0402\\ 
  14 & MDE.Phi.tv & Measure & beta=2 & sigma=3 & n=100 & 0.02 \\ 
  15 & MDE.Phi.kl & Measure & beta=2 & sigma=3 & n=100 & 0.00 \\ 
  16 & MME & Measure & beta=2 & sigma=3 & n=100 & 0.00 \\ 
  17 & MME.b & Measure & beta=2 & sigma=3 & n=100 & 0.01 \\ 
  18 & PWM & Measure & beta=2 & sigma=3 & n=100 & 0.00 \\ 
  19 & MLE & Measure & beta=2.5 & sigma=3 & n=100 & 0.00 \\ 
  20 & MLE.b & Measure & beta=2.5 & sigma=3 & n=100 & 0.00 \\ 
  21 & LME & Measure & beta=2.5 & sigma=3 & n=100 & 0.00 \\ 
  22 & MDE.Phi.chisq & Measure & beta=2.5 & sigma=3 & n=100 & 0.02 \\ 
  23 & MDE.Phi.tv & Measure & beta=2.5 & sigma=3 & n=100 & 0.02 \\ 
  24 & MDE.Phi.kl & Measure & beta=2.5 & sigma=3 & n=100 & 0.00 \\ 
  25 & MME & Measure & beta=2.5 & sigma=3 & n=100 & 0.00 \\ 
  26 & MME.b & Measure & beta=2.5 & sigma=3 & n=100 & 8.08 \\ 
  27 & PWM & Measure & beta=2.5 & sigma=3 & n=100 & 0.00 \\ 
  28 & MLE & Measure & beta=3 & sigma=3 & n=100 & 0.00 \\ 
  29 & MLE.b & Measure & beta=3 & sigma=3 & n=100 & 0.00 \\ 
  30 & LME & Measure & beta=3 & sigma=3 & n=100 & 0.00 \\ 
  31 & MDE.Phi.chisq & Measure & beta=3 & sigma=3 & n=100 & 0.02 \\ 
  32 & MDE.Phi.tv & Measure & beta=3 & sigma=3 & n=100 & 0.02 \\ 
  33 & MDE.Phi.kl & Measure & beta=3 & sigma=3 & n=100 & 0.00 \\ 
  34 & MME & Measure & beta=3 & sigma=3 & n=100 & 0.00 \\ 
  35 & MME.b & Measure & beta=3 & sigma=3 & n=100 & 0.01 \\ 
  36 & PWM & Measure & beta=3 & sigma=3 & n=100 & 0.00 \\ 
  37 & MLE & Measure & beta=4 & sigma=3 & n=100 & 0.00 \\ 
  38 & MLE.b & Measure & beta=4 & sigma=3 & n=100 & 0.00 \\ 
  39 & LME & Measure & beta=4 & sigma=3 & n=100 & 0.00 \\ 
  40 & MDE.Phi.chisq & Measure & beta=4 & sigma=3 & n=100 & 0.02 \\ 
  41 & MDE.Phi.tv & Measure & beta=4 & sigma=3 & n=100 & 0.01 \\ 
  42 & MDE.Phi.kl & Measure & beta=4 & sigma=3 & n=100 & 0.00 \\ 
  43 & MME & Measure & beta=4 & sigma=3 & n=100 & 0.00 \\ 
  44 & MME.b & Measure & beta=4 & sigma=3 & n=100 & 4041.95 \\ 
  45 & PWM & Measure & beta=4 & sigma=3 & n=100 & 0.00 \\ 
  46 & MLE & Measure & beta=5 & sigma=3 & n=100 & 0.00 \\ 
  47 & MLE.b & Measure & beta=5 & sigma=3 & n=100 & 0.00 \\ 
  48 & LME & Measure & beta=5 & sigma=3 & n=100 & 0.00 \\ 
  49 & MDE.Phi.chisq & Measure & beta=5 & sigma=3 & n=100 & 0.01 \\ 
  50 & MDE.Phi.tv & Measure & beta=5 & sigma=3 & n=100 & 0.01 \\ 
  51 & MDE.Phi.kl & Measure & beta=5 & sigma=3 & n=100 & 0.00 \\ 
  52 & MME & Measure & beta=5 & sigma=3 & n=100 & 0.00 \\ 
  53 & MME.b & Measure & beta=5 & sigma=3 & n=100 & 51.00 \\ 
  54 & PWM & Measure & beta=5 & sigma=3 & n=100 & 0.00 \\ 
  55 & MLE & Measure & beta=1.5 & sigma=3 & n=200 & 0.00 \\ 
  56 & MLE.b & Measure & beta=1.5 & sigma=3 & n=200 & 0.00 \\ 
  57 & LME & Measure & beta=1.5 & sigma=3 & n=200 & 0.00 \\ 
  58 & MDE.Phi.chisq & Measure & beta=1.5 & sigma=3 & n=200 & 98.4391 \\ 
  59 & MDE.Phi.tv & Measure & beta=1.5 & sigma=3 & n=200 & 0.03 \\ 
  60 & MDE.Phi.kl & Measure & beta=1.5 & sigma=3 & n=200 & 0.00 \\ 
  61 & MME & Measure & beta=1.5 & sigma=3 & n=200 & 0.01 \\ 
  62 & MME.b & Measure & beta=1.5 & sigma=3 & n=200 & 0.01 \\ 
  63 & PWM & Measure & beta=1.5 & sigma=3 & n=200 & 0.00 \\ 
  64 & MLE & Measure & beta=2 & sigma=3 & n=200 & 0.00 \\ 
  65 & MLE.b & Measure & beta=2 & sigma=3 & n=200 & 0.00 \\ 
  66 & LME & Measure & beta=2 & sigma=3 & n=200 & 0.00 \\ 
  67 & MDE.Phi.chisq & Measure & beta=2 & sigma=3 & n=200 & 32.00 \\ 
  68 & MDE.Phi.tv & Measure & beta=2 & sigma=3 & n=200 & 0.02 \\ 
  69 & MDE.Phi.kl & Measure & beta=2 & sigma=3 & n=200 & 0.00 \\ 
  70 & MME & Measure & beta=2 & sigma=3 & n=200 & 0.00 \\ 
  71 & MME.b & Measure & beta=2 & sigma=3 & n=200 & 0.00 \\ 
  72 & PWM & Measure & beta=2 & sigma=3 & n=200 & 0.00 \\ 
  73 & MLE & Measure & beta=2.5 & sigma=3 & n=200 & 0.00 \\ 
  74 & MLE.b & Measure & beta=2.5 & sigma=3 & n=200 & 0.00 \\ 
  75 & LME & Measure & beta=2.5 & sigma=3 & n=200 & 0.00 \\ 
  76 & MDE.Phi.chisq & Measure & beta=2.5 & sigma=3 & n=200 & 0.02 \\ 
  77 & MDE.Phi.tv & Measure & beta=2.5 & sigma=3 & n=200 & 0.01 \\ 
  78 & MDE.Phi.kl & Measure & beta=2.5 & sigma=3 & n=200 & 0.00 \\ 
  79 & MME & Measure & beta=2.5 & sigma=3 & n=200 & 0.00 \\ 
  80 & MME.b & Measure & beta=2.5 & sigma=3 & n=200 & 0.00 \\ 
  81 & PWM & Measure & beta=2.5 & sigma=3 & n=200 & 0.00 \\ 
  82 & MLE & Measure & beta=3 & sigma=3 & n=200 & 0.00 \\ 
  83 & MLE.b & Measure & beta=3 & sigma=3 & n=200 & 0.00 \\ 
  84 & LME & Measure & beta=3 & sigma=3 & n=200 & 0.00 \\ 
  85 & MDE.Phi.chisq & Measure & beta=3 & sigma=3 & n=200 & 0.01 \\ 
  86 & MDE.Phi.tv & Measure & beta=3 & sigma=3 & n=200 & 0.01 \\ 
  87 & MDE.Phi.kl & Measure & beta=3 & sigma=3 & n=200 & 0.00 \\ 
  88 & MME & Measure & beta=3 & sigma=3 & n=200 & 0.00 \\ 
  89 & MME.b & Measure & beta=3 & sigma=3 & n=200 & 0.00 \\ 
  90 & PWM & Measure & beta=3 & sigma=3 & n=200 & 0.00 \\ 
  91 & MLE & Measure & beta=4 & sigma=3 & n=200 & 0.00 \\ 
  92 & MLE.b & Measure & beta=4 & sigma=3 & n=200 & 0.00 \\ 
  93 & LME & Measure & beta=4 & sigma=3 & n=200 & 0.00 \\ 
  94 & MDE.Phi.chisq & Measure & beta=4 & sigma=3 & n=200 & 0.01 \\ 
  95 & MDE.Phi.tv & Measure & beta=4 & sigma=3 & n=200 & 0.01 \\ 
  96 & MDE.Phi.kl & Measure & beta=4 & sigma=3 & n=200 & 0.00 \\ 
  97 & MME & Measure & beta=4 & sigma=3 & n=200 & 0.00 \\ 
  98 & MME.b & Measure & beta=4 & sigma=3 & n=200 & 0.00 \\ 
  99 & PWM & Measure & beta=4 & sigma=3 & n=200 & 0.00 \\ 
  100 & MLE & Measure & beta=5 & sigma=3 & n=200 & 0.00 \\ 
  101 & MLE.b & Measure & beta=5 & sigma=3 & n=200 & 0.00 \\ 
  102 & LME & Measure & beta=5 & sigma=3 & n=200 & 0.00 \\ 
  103 & MDE.Phi.chisq & Measure & beta=5 & sigma=3 & n=200 & 0.01 \\ 
  104 & MDE.Phi.tv & Measure & beta=5 & sigma=3 & n=200 & 0.01 \\ 
  105 & MDE.Phi.kl & Measure & beta=5 & sigma=3 & n=200 & 0.00 \\ 
  106 & MME & Measure & beta=5 & sigma=3 & n=200 & 0.00 \\ 
  107 & MME.b & Measure & beta=5 & sigma=3 & n=200 & 2.02 \\ 
  108 & PWM & Measure & beta=5 & sigma=3 & n=200 & 0.00 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220101/Full.beta=1.5.sig=2.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=1.5,  \sigma=2$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.6717&1.4777&1.8288&0.234&1.257&1.6717&2.7927&6.3149&1.8288
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2.3645&1.9548&2.6507&3.2891&3.6444&2.3645&6.3049&13.6686&2.6507
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.435&0.3213&0.2958&97.6125&6.7844&0.4354&0.8967&130047.0683&0.2958
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.9574&1.4455&1.33&82.0458&70.7652&1.9589&7.9695&595564.3219&1.33
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1717&-0.0223&0.3288&-1.266&-0.243&0.1717&1.2927&4.8149&0.3288
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.3645&-0.0452&0.6507&1.2891&1.6444&0.3645&4.3049&11.6686&0.6507
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.4644&0.3217&0.4039&99.2056&6.8428&0.4648&2.5678&130057.2467&0.4039
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2.0901&1.4474&1.7532&83.6994&73.4621&2.0916&26.5012&595640.9217&1.7532
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 2.5545&1.7692&2.1571&182.9049&80.3048&2.5564&29.069&725698.1684&2.1571\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0011&0.0011&1.63885457077832e+301&0.0364&0.0011&0.0099&7.105&0.0011\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220101/Full.beta=1.5.sig=2.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=1.5,  \sigma=2$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.7301&1.6295&1.7053&0.6454&1.004&1.578&2.4952&2.2961&1.7053
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2.4773&2.2636&2.4046&2.3164&2.507&2.1626&5.5704&5.0195&2.4046
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1033&0.0759&0.1117&22.8262&0.1705&0.1014&0.1645&0.2553&0.1117
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.456&0.3307&0.4944&3.3191&1.1627&0.4329&6.0718&6.4445&0.4944
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.2301&0.1295&0.2053&-0.8546&-0.496&0.078&0.9952&0.7961&0.2053
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.4773&0.2636&0.4046&0.3164&0.507&0.1626&3.5704&3.0195&0.4046
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1562&0.0927&0.1539&23.5542&0.4165&0.1075&1.1549&0.889&0.1539
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.6837&0.4001&0.6581&3.4189&1.4196&0.4593&18.8191&15.5612&0.6581
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 0.84&0.4928&0.8119&26.9731&1.8362&0.5667&19.974&16.4502&0.8119\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 6e-04&6e-04&6e-04&2.74643118624275e+299&0.0276&6e-04&0.0089&0.0103&6e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220101/Full.beta=2.5.sig=2.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2.5,  \sigma=2$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 3.5893&3.1321&3.1958&4.1065&4.9271&3.4377&4.8214&7.9937&3.1958
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
3.169&2.6735&2.7184&6.1414&7.1933&3.0067&4.7089&8.0431&2.7184
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 140.165&140.8267&8.3445&224.5742&256.6062&29.7786&144.3027&2205.727&8.3445
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
160.6925&161.4224&8.9937&535.712&611.3674&32.5838&150.1403&2520.2999&8.9937
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.0893&0.6321&0.6958&1.6065&2.4271&0.9377&2.3214&5.4937&0.6958
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.169&0.6735&0.7184&4.1414&5.1933&1.0067&2.7089&6.0431&0.7184
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 141.3376&141.2122&8.8279&227.1324&262.4715&30.6549&149.6771&2235.6866&8.8279
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
162.0429&161.8599&9.5089&552.8092&638.2771&33.5939&157.4634&2556.5675&9.5089
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 303.3806&303.0721&18.3368&779.9416&900.7486&64.2488&307.1405&4792.2541&18.3368\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0012&0.0011&0.0233&0.0179&0.0011&0.0019&8.078&0.0011\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220101/Full.beta=2.5.sig=2.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2.5,  \sigma=2$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.8441&2.5199&2.784&2.0498&2.2768&2.7518&3.5622&3.3354&2.784
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2.3708&2.0191&2.2893&2.7012&2.8083&2.2713&3.3094&3.0134&2.2893
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.4065&1.126&1.1971&17.8817&13.8093&1.1167&1.774&43.7476&1.1971
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.6567&1.3199&1.3628&36.102&26.6172&1.3262&2.1291&49.2611&1.3628
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.3441&0.0199&0.284&-0.4502&-0.2232&0.2518&1.0622&0.8354&0.284
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.3708&0.0191&0.2893&0.7012&0.8083&0.2713&1.3094&1.0134&0.2893
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.5248&1.1263&1.2776&18.0826&13.8577&1.18&2.9021&44.441&1.2776
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.794&1.3201&1.4463&36.59&27.2679&1.3996&3.8434&50.2833&1.4463
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 3.3188&2.4464&2.724&54.6726&41.1256&2.5796&6.7455&94.7243&2.724\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&5e-04&5e-04&0.0174&0.0121&5e-04&0.0011&0.0017&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220101/Full.beta=2.sig=2.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2,  \sigma=2$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.5397&2.1901&2.4461&2.0969&2.6942&2.458&3.6775&9.4751&2.4461
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2.7453&2.2401&2.6033&4.195&5.2184&2.6474&4.8746&13.1731&2.6033
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 66.0603&66.0628&3.1121&65.3915&87.2818&12.1947&52.8831&151218.7131&3.1121
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
93.6627&93.6023&5.78&298.7604&379.0939&20.4426&91.4156&334195.4082&5.78
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.5397&0.1901&0.4461&0.0969&0.6942&0.458&1.6775&7.4751&0.4461
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.7453&0.2401&0.6033&2.195&3.2184&0.6474&2.8746&11.1731&0.6033
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 66.345&66.0923&3.3109&65.3943&87.755&12.4033&55.6919&151259.4685&3.3109
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
94.2087&93.6506&6.1434&303.5485&389.4141&20.8597&99.6701&334286.8261&6.1434
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 160.5538&159.7429&9.4543&368.9428&477.169&33.263&155.3621&485546.2946&9.4543\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0011&0.0011&0.0296&0.0232&0.0011&0.0035&0.0115&0.0011\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220101/Full.beta=2.sig=2.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2,  \sigma=2$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.2514&2.0633&2.2157&1.3468&1.5634&2.1374&2.9722&2.6877&2.2157
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2.3527&2.0825&2.2838&2.3432&2.5561&2.1929&3.7771&3.293&2.2838
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.305&0.2007&0.3034&2.1912&2.2108&0.2964&0.5321&5.3987&0.3034
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.6069&0.3945&0.5992&7.138&9.1449&0.5879&1.1111&10.202&0.5992
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.2514&0.0633&0.2157&-0.6532&-0.4366&0.1374&0.9722&0.6877&0.2157
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.3527&0.0825&0.2838&0.3432&0.5561&0.1929&1.7771&1.293&0.2838
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.3682&0.2047&0.3499&2.6177&2.4012&0.3153&1.4772&5.8711&0.3499
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.7312&0.4013&0.6797&7.2551&9.4533&0.625&4.269&11.8728&0.6797
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 1.0994&0.606&1.0296&9.8728&11.8545&0.9403&5.7463&17.744&1.0296\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 6e-04&5e-04&5e-04&0.0227&0.0165&5e-04&0.0024&0.0024&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220101/Full.beta=3.sig=2.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=3,  \sigma=2$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 5.7496&5.2554&4.0159&6.8159&8.2326&4.8603&17.4875&49.9897&4.0159
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
4.3701&3.9431&2.851&8.2493&9.7002&3.6029&13.4836&39.1376&2.851
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 872.8497&875.5266&15.9909&480.8982&575.7729&100.8592&313146.3373&2977375.7167&15.9909
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
673.8379&675.7935&12.3334&759.0983&886.5153&75.1257&180846.3382&1721384.9561&12.3334
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.7496&2.2554&1.0159&3.8159&5.2326&1.8603&14.4875&46.9897&1.0159
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2.3701&1.9431&0.851&6.2493&7.7002&1.6029&11.4836&37.1376&0.851
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 880.3225&880.5257&17.0213&495.4112&603.0956&104.31&313324.9101&2979286.0078&17.0213
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
679.3878&679.5016&13.0565&798.0758&945.7205&77.6873&180960.127&1722592.0179&13.0565
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 1559.7103&1560.0274&30.0778&1293.487&1548.8161&181.9974&494285.0371&4701878.0258&30.0778\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0012&0.0011&0.0201&0.0151&0.0011&0.0014&0.0075&0.0011\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220101/Full.beta=3.sig=2.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=3,  \sigma=2$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 3.7154&3.2327&3.4535&3.3052&3.2069&3.4926&4.4031&5.6933&3.4535
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2.6184&2.1988&2.3785&3.5428&3.1929&2.4257&3.2925&4.4634&2.3785
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 175.5736&175.4235&4.1441&89.0057&42.6911&7.7328&73.0305&7346.8537&4.1441
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
116.6364&116.4993&2.9784&117.1409&52.0072&5.5021&47.4545&6725.9729&2.9784
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.7154&0.2327&0.4535&0.3052&0.2069&0.4926&1.4031&2.6933&0.4535
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.6184&0.1988&0.3785&1.5428&1.1929&0.4257&1.2925&2.4634&0.3785
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 176.0679&175.4601&4.3493&89.09&42.7296&7.9746&74.9918&7353.3729&4.3493
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
117.0072&116.5272&3.1213&119.5094&53.4249&5.6827&49.1203&6731.3689&3.1213
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 293.0751&291.9873&7.4706&208.5993&96.1546&13.6574&124.1121&14084.7417&7.4706\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&5e-04&5e-04&0.0143&0.0096&5e-04&7e-04&0.0018&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220101/Full.beta=4.sig=2.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=4,  \sigma=2$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 8.7295&8.2802&5.759&13.7651&15.9545&7.4212&11.3558&40.9124&5.759
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
4.927&4.6544&3.0703&11.8342&13.2625&4.1216&6.6655&26.8679&3.0703
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1525.3767&1530.3561&48.7724&1195.0428&1368.6343&201.2946&11556.9085&1921162.3133&48.7724
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
574.9177&576.7649&18.7607&926.7579&1007.8946&79.6118&4346.1835&1082212.1431&18.7607
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 4.7295&4.2802&1.759&9.7651&11.9545&3.4212&7.3558&36.9124&1.759
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2.927&2.6544&1.0703&9.8342&11.2625&2.1216&4.6655&24.8679&1.0703
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1547.5927&1548.5231&51.8617&1290.2814&1511.4083&212.9789&11609.8605&1922332.7188&51.8617
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
583.4273&583.7532&19.9043&1023.3773&1134.6382&84.1049&4367.5156&1082722.332&19.9043
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 2131.0201&2132.2764&71.766&2313.6587&2646.0465&297.0838&15977.3761&3005055.0508&71.766\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0012&0.001&0.0165&0.0123&0.0011&0.0011&4041.9544&0.001\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220101/Full.beta=4.sig=2.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=4,  \sigma=2$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 5.559&4.8756&4.9145&7.7069&6.9491&5.2566&6.6372&13.6851&4.9145
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2.9826&2.5623&2.5529&6.0025&5.1303&2.7745&3.6618&8.2547&2.5529
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 158.8545&160.3016&17.4492&465.0781&346.1052&41.244&544.0894&40207.1182&17.4492
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
62.644&63.1884&6.5508&303.5793&220.0039&15.5934&210.9218&19770.8596&6.5508
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.559&0.8756&0.9145&3.7069&2.9491&1.2566&2.6372&9.6851&0.9145
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.9826&0.5623&0.5529&4.0025&3.1303&0.7745&1.6618&6.2547&0.5529
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 161.2692&161.0524&18.2837&478.7729&354.7677&42.8191&550.9901&40296.899&18.2837
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
63.6032&63.4983&6.8558&319.5687&229.7807&16.1917&213.6621&19808.0043&6.8558
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 224.8724&224.5506&25.1395&798.3416&584.5484&59.0108&764.6522&60104.9033&25.1395\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&6e-04&5e-04&0.0111&0.0074&5e-04&6e-04&0.0029&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220101/Full.beta=5.sig=2.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=5,  \sigma=2$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 12.3236&11.9551&7.3605&20.093&22.2436&10.0638&16.7262&47.1595&7.3605
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
5.4476&5.2764&3.101&13.1832&14.1594&4.3827&7.4959&21.9309&3.101
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2693.779&2700.4687&96.0976&1864.5133&2004.2157&347.2915&18587.8467&257840.1544&96.0976
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
605.4031&606.8577&21.2623&832.8022&860.1424&76.9632&4147.1761&61786.3409&21.2623
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 7.3236&6.9551&2.3605&15.093&17.2436&5.0638&11.7262&42.1595&2.3605
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
3.4476&3.2764&1.101&11.1832&12.1594&2.3827&5.4959&19.9309&1.101
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2747.1447&2748.5723&101.6601&2092.1268&2301.358&372.8992&18723.4925&259591.7905&101.6601
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
617.2287&617.5317&22.4723&957.7827&1007.9069&82.6327&4176.9667&62177.4021&22.4723
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 3364.3733&3366.1039&124.1323&3049.9096&3309.2649&455.5319&22900.4592&321769.1926&124.1323\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.001&0.0012&0.001&0.0144&0.0106&0.001&0.001&5.15620838018139e+29&0.001\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220101/Full.beta=5.sig=2.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=5,  \sigma=2$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 9.9205&9.2093&6.7803&14.1274&11.358&7.6&9.7618&21.5876&6.7803
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
4.3773&4.0403&2.8327&8.5388&6.5108&3.2262&4.2663&9.8745&2.8327
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 10574.3435&10581.6739&63.0773&1137.0862&766.5447&134.8763&2723.7306&30712.8683&63.0773
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2446.3119&2447.9693&14.1243&435.7651&279.1057&30.091&592.1845&6949.345&14.1243
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 4.9205&4.2093&1.7803&9.1274&6.358&2.6&4.7618&16.5876&1.7803
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2.3773&2.0403&0.8327&6.5388&4.5108&1.2262&2.2663&7.8745&0.8327
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 10597.4977&10598.3343&66.2407&1220.2826&806.8926&141.6228&2746.133&30984.9451&66.2407
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2451.7189&2451.8872&14.8163&478.4768&299.425&31.5915&597.2612&7010.6574&14.8163
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 13049.2166&13050.2215&81.057&1698.7594&1106.3177&173.2143&3343.3942&37995.6025&81.057\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&6e-04&5e-04&0.0096&0.0062&5e-04&5e-04&2.018&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220101/Output.accuracy.LaTeX.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Mon Jan 31 17:32:25 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & Measure & beta=1.5 & sigma=2 & n=100 & 2.55 \\ 
  2 & MLE.b & Measure & beta=1.5 & sigma=2 & n=100 & 1.77 \\ 
  3 & LME & Measure & beta=1.5 & sigma=2 & n=100 & 2.16 \\ 
  4 & MDE.Phi.chisq & Measure & beta=1.5 & sigma=2 & n=100 & 182.90 \\ 
  5 & MDE.Phi.tv & Measure & beta=1.5 & sigma=2 & n=100 & 80.30 \\ 
  6 & MDE.Phi.kl & Measure & beta=1.5 & sigma=2 & n=100 & 2.56 \\ 
  7 & MME & Measure & beta=1.5 & sigma=2 & n=100 & 29.07 \\ 
  8 & MME.b & Measure & beta=1.5 & sigma=2 & n=100 & 725698.17 \\ 
  9 & PWM & Measure & beta=1.5 & sigma=2 & n=100 & 2.16 \\ 
  10 & MLE & Measure & beta=2 & sigma=2 & n=100 & 160.55 \\ 
  11 & MLE.b & Measure & beta=2 & sigma=2 & n=100 & 159.74 \\ 
  12 & LME & Measure & beta=2 & sigma=2 & n=100 & 9.45 \\ 
  13 & MDE.Phi.chisq & Measure & beta=2 & sigma=2 & n=100 & 368.94 \\ 
  14 & MDE.Phi.tv & Measure & beta=2 & sigma=2 & n=100 & 477.17 \\ 
  15 & MDE.Phi.kl & Measure & beta=2 & sigma=2 & n=100 & 33.26 \\ 
  16 & MME & Measure & beta=2 & sigma=2 & n=100 & 155.36 \\ 
  17 & MME.b & Measure & beta=2 & sigma=2 & n=100 & 485546.29 \\ 
  18 & PWM & Measure & beta=2 & sigma=2 & n=100 & 9.45 \\ 
  19 & MLE & Measure & beta=2.5 & sigma=2 & n=100 & 303.38 \\ 
  20 & MLE.b & Measure & beta=2.5 & sigma=2 & n=100 & 303.07 \\ 
  21 & LME & Measure & beta=2.5 & sigma=2 & n=100 & 18.34 \\ 
  22 & MDE.Phi.chisq & Measure & beta=2.5 & sigma=2 & n=100 & 779.94 \\ 
  23 & MDE.Phi.tv & Measure & beta=2.5 & sigma=2 & n=100 & 900.75 \\ 
  24 & MDE.Phi.kl & Measure & beta=2.5 & sigma=2 & n=100 & 64.25 \\ 
  25 & MME & Measure & beta=2.5 & sigma=2 & n=100 & 307.14 \\ 
  26 & MME.b & Measure & beta=2.5 & sigma=2 & n=100 & 4792.25 \\ 
  27 & PWM & Measure & beta=2.5 & sigma=2 & n=100 & 18.34 \\ 
  28 & MLE & Measure & beta=3 & sigma=2 & n=100 & 1559.71 \\ 
  29 & MLE.b & Measure & beta=3 & sigma=2 & n=100 & 1560.03 \\ 
  30 & LME & Measure & beta=3 & sigma=2 & n=100 & 30.08 \\ 
  31 & MDE.Phi.chisq & Measure & beta=3 & sigma=2 & n=100 & 1293.49 \\ 
  32 & MDE.Phi.tv & Measure & beta=3 & sigma=2 & n=100 & 1548.82 \\ 
  33 & MDE.Phi.kl & Measure & beta=3 & sigma=2 & n=100 & 182.00 \\ 
  34 & MME & Measure & beta=3 & sigma=2 & n=100 & 494285.04 \\ 
  35 & MME.b & Measure & beta=3 & sigma=2 & n=100 & 4701878.03 \\ 
  36 & PWM & Measure & beta=3 & sigma=2 & n=100 & 30.08 \\ 
  37 & MLE & Measure & beta=4 & sigma=2 & n=100 & 2131.02 \\ 
  38 & MLE.b & Measure & beta=4 & sigma=2 & n=100 & 2132.28 \\ 
  39 & LME & Measure & beta=4 & sigma=2 & n=100 & 71.77 \\ 
  40 & MDE.Phi.chisq & Measure & beta=4 & sigma=2 & n=100 & 2313.66 \\ 
  41 & MDE.Phi.tv & Measure & beta=4 & sigma=2 & n=100 & 2646.05 \\ 
  42 & MDE.Phi.kl & Measure & beta=4 & sigma=2 & n=100 & 297.08 \\ 
  43 & MME & Measure & beta=4 & sigma=2 & n=100 & 15977.38 \\ 
  44 & MME.b & Measure & beta=4 & sigma=2 & n=100 & 3005055.05 \\ 
  45 & PWM & Measure & beta=4 & sigma=2 & n=100 & 71.77 \\ 
  46 & MLE & Measure & beta=5 & sigma=2 & n=100 & 3364.37 \\ 
  47 & MLE.b & Measure & beta=5 & sigma=2 & n=100 & 3366.10 \\ 
  48 & LME & Measure & beta=5 & sigma=2 & n=100 & 124.13 \\ 
  49 & MDE.Phi.chisq & Measure & beta=5 & sigma=2 & n=100 & 3049.91 \\ 
  50 & MDE.Phi.tv & Measure & beta=5 & sigma=2 & n=100 & 3309.26 \\ 
  51 & MDE.Phi.kl & Measure & beta=5 & sigma=2 & n=100 & 455.53 \\ 
  52 & MME & Measure & beta=5 & sigma=2 & n=100 & 22900.46 \\ 
  53 & MME.b & Measure & beta=5 & sigma=2 & n=100 & 321769.19 \\ 
  54 & PWM & Measure & beta=5 & sigma=2 & n=100 & 124.13 \\ 
  55 & MLE & Measure & beta=1.5 & sigma=2 & n=200 & 0.84 \\ 
  56 & MLE.b & Measure & beta=1.5 & sigma=2 & n=200 & 0.49 \\ 
  57 & LME & Measure & beta=1.5 & sigma=2 & n=200 & 0.81 \\ 
  58 & MDE.Phi.chisq & Measure & beta=1.5 & sigma=2 & n=200 & 26.97 \\ 
  59 & MDE.Phi.tv & Measure & beta=1.5 & sigma=2 & n=200 & 1.84 \\ 
  60 & MDE.Phi.kl & Measure & beta=1.5 & sigma=2 & n=200 & 0.57 \\ 
  61 & MME & Measure & beta=1.5 & sigma=2 & n=200 & 19.97 \\ 
  62 & MME.b & Measure & beta=1.5 & sigma=2 & n=200 & 16.45 \\ 
  63 & PWM & Measure & beta=1.5 & sigma=2 & n=200 & 0.81 \\ 
  64 & MLE & Measure & beta=2 & sigma=2 & n=200 & 1.10 \\ 
  65 & MLE.b & Measure & beta=2 & sigma=2 & n=200 & 0.61 \\ 
  66 & LME & Measure & beta=2 & sigma=2 & n=200 & 1.03 \\ 
  67 & MDE.Phi.chisq & Measure & beta=2 & sigma=2 & n=200 & 9.87 \\ 
  68 & MDE.Phi.tv & Measure & beta=2 & sigma=2 & n=200 & 11.85 \\ 
  69 & MDE.Phi.kl & Measure & beta=2 & sigma=2 & n=200 & 0.94 \\ 
  70 & MME & Measure & beta=2 & sigma=2 & n=200 & 5.75 \\ 
  71 & MME.b & Measure & beta=2 & sigma=2 & n=200 & 17.74 \\ 
  72 & PWM & Measure & beta=2 & sigma=2 & n=200 & 1.03 \\ 
  73 & MLE & Measure & beta=2.5 & sigma=2 & n=200 & 3.32 \\ 
  74 & MLE.b & Measure & beta=2.5 & sigma=2 & n=200 & 2.45 \\ 
  75 & LME & Measure & beta=2.5 & sigma=2 & n=200 & 2.72 \\ 
  76 & MDE.Phi.chisq & Measure & beta=2.5 & sigma=2 & n=200 & 54.67 \\ 
  77 & MDE.Phi.tv & Measure & beta=2.5 & sigma=2 & n=200 & 41.13 \\ 
  78 & MDE.Phi.kl & Measure & beta=2.5 & sigma=2 & n=200 & 2.58 \\ 
  79 & MME & Measure & beta=2.5 & sigma=2 & n=200 & 6.75 \\ 
  80 & MME.b & Measure & beta=2.5 & sigma=2 & n=200 & 94.72 \\ 
  81 & PWM & Measure & beta=2.5 & sigma=2 & n=200 & 2.72 \\ 
  82 & MLE & Measure & beta=3 & sigma=2 & n=200 & 293.08 \\ 
  83 & MLE.b & Measure & beta=3 & sigma=2 & n=200 & 291.99 \\ 
  84 & LME & Measure & beta=3 & sigma=2 & n=200 & 7.47 \\ 
  85 & MDE.Phi.chisq & Measure & beta=3 & sigma=2 & n=200 & 208.60 \\ 
  86 & MDE.Phi.tv & Measure & beta=3 & sigma=2 & n=200 & 96.15 \\ 
  87 & MDE.Phi.kl & Measure & beta=3 & sigma=2 & n=200 & 13.66 \\ 
  88 & MME & Measure & beta=3 & sigma=2 & n=200 & 124.11 \\ 
  89 & MME.b & Measure & beta=3 & sigma=2 & n=200 & 14084.74 \\ 
  90 & PWM & Measure & beta=3 & sigma=2 & n=200 & 7.47 \\ 
  91 & MLE & Measure & beta=4 & sigma=2 & n=200 & 224.87 \\ 
  92 & MLE.b & Measure & beta=4 & sigma=2 & n=200 & 224.55 \\ 
  93 & LME & Measure & beta=4 & sigma=2 & n=200 & 25.14 \\ 
  94 & MDE.Phi.chisq & Measure & beta=4 & sigma=2 & n=200 & 798.34 \\ 
  95 & MDE.Phi.tv & Measure & beta=4 & sigma=2 & n=200 & 584.55 \\ 
  96 & MDE.Phi.kl & Measure & beta=4 & sigma=2 & n=200 & 59.01 \\ 
  97 & MME & Measure & beta=4 & sigma=2 & n=200 & 764.65 \\ 
  98 & MME.b & Measure & beta=4 & sigma=2 & n=200 & 60104.90 \\ 
  99 & PWM & Measure & beta=4 & sigma=2 & n=200 & 25.14 \\ 
  100 & MLE & Measure & beta=5 & sigma=2 & n=200 & 13049.22 \\ 
  101 & MLE.b & Measure & beta=5 & sigma=2 & n=200 & 13050.22 \\ 
  102 & LME & Measure & beta=5 & sigma=2 & n=200 & 81.06 \\ 
  103 & MDE.Phi.chisq & Measure & beta=5 & sigma=2 & n=200 & 1698.76 \\ 
  104 & MDE.Phi.tv & Measure & beta=5 & sigma=2 & n=200 & 1106.32 \\ 
  105 & MDE.Phi.kl & Measure & beta=5 & sigma=2 & n=200 & 173.21 \\ 
  106 & MME & Measure & beta=5 & sigma=2 & n=200 & 3343.39 \\ 
  107 & MME.b & Measure & beta=5 & sigma=2 & n=200 & 37995.60 \\ 
  108 & PWM & Measure & beta=5 & sigma=2 & n=200 & 81.06 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220101/Output.accuracy2.LaTeX.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Mon Jan 31 17:32:25 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & Measure & beta=1.5 & sigma=2 & n=100 & 0.00 \\ 
  2 & MLE.b & Measure & beta=1.5 & sigma=2 & n=100 & 0.00 \\ 
  3 & LME & Measure & beta=1.5 & sigma=2 & n=100 & 0.00 \\ 
  4 & MDE.Phi.chisq & Measure & beta=1.5 & sigma=2 & n=100 & 16388545707783188136066046880868420288880644626286248600040886664006840686688684044466068828868042242082600626648222848868802680822684866420208804206626086004640604206282064042064066088628424284280400408086606428888684264240840820828200200048884682628026004288082268842602062622882868800086088606468420.00 \\ 
  5 & MDE.Phi.tv & Measure & beta=1.5 & sigma=2 & n=100 & 0.04 \\ 
  6 & MDE.Phi.kl & Measure & beta=1.5 & sigma=2 & n=100 & 0.00 \\ 
  7 & MME & Measure & beta=1.5 & sigma=2 & n=100 & 0.01 \\ 
  8 & MME.b & Measure & beta=1.5 & sigma=2 & n=100 & 7.11 \\ 
  9 & PWM & Measure & beta=1.5 & sigma=2 & n=100 & 0.00 \\ 
  10 & MLE & Measure & beta=2 & sigma=2 & n=100 & 0.00 \\ 
  11 & MLE.b & Measure & beta=2 & sigma=2 & n=100 & 0.00 \\ 
  12 & LME & Measure & beta=2 & sigma=2 & n=100 & 0.00 \\ 
  13 & MDE.Phi.chisq & Measure & beta=2 & sigma=2 & n=100 & 0.03 \\ 
  14 & MDE.Phi.tv & Measure & beta=2 & sigma=2 & n=100 & 0.02 \\ 
  15 & MDE.Phi.kl & Measure & beta=2 & sigma=2 & n=100 & 0.00 \\ 
  16 & MME & Measure & beta=2 & sigma=2 & n=100 & 0.00 \\ 
  17 & MME.b & Measure & beta=2 & sigma=2 & n=100 & 0.01 \\ 
  18 & PWM & Measure & beta=2 & sigma=2 & n=100 & 0.00 \\ 
  19 & MLE & Measure & beta=2.5 & sigma=2 & n=100 & 0.00 \\ 
  20 & MLE.b & Measure & beta=2.5 & sigma=2 & n=100 & 0.00 \\ 
  21 & LME & Measure & beta=2.5 & sigma=2 & n=100 & 0.00 \\ 
  22 & MDE.Phi.chisq & Measure & beta=2.5 & sigma=2 & n=100 & 0.02 \\ 
  23 & MDE.Phi.tv & Measure & beta=2.5 & sigma=2 & n=100 & 0.02 \\ 
  24 & MDE.Phi.kl & Measure & beta=2.5 & sigma=2 & n=100 & 0.00 \\ 
  25 & MME & Measure & beta=2.5 & sigma=2 & n=100 & 0.00 \\ 
  26 & MME.b & Measure & beta=2.5 & sigma=2 & n=100 & 8.08 \\ 
  27 & PWM & Measure & beta=2.5 & sigma=2 & n=100 & 0.00 \\ 
  28 & MLE & Measure & beta=3 & sigma=2 & n=100 & 0.00 \\ 
  29 & MLE.b & Measure & beta=3 & sigma=2 & n=100 & 0.00 \\ 
  30 & LME & Measure & beta=3 & sigma=2 & n=100 & 0.00 \\ 
  31 & MDE.Phi.chisq & Measure & beta=3 & sigma=2 & n=100 & 0.02 \\ 
  32 & MDE.Phi.tv & Measure & beta=3 & sigma=2 & n=100 & 0.02 \\ 
  33 & MDE.Phi.kl & Measure & beta=3 & sigma=2 & n=100 & 0.00 \\ 
  34 & MME & Measure & beta=3 & sigma=2 & n=100 & 0.00 \\ 
  35 & MME.b & Measure & beta=3 & sigma=2 & n=100 & 0.01 \\ 
  36 & PWM & Measure & beta=3 & sigma=2 & n=100 & 0.00 \\ 
  37 & MLE & Measure & beta=4 & sigma=2 & n=100 & 0.00 \\ 
  38 & MLE.b & Measure & beta=4 & sigma=2 & n=100 & 0.00 \\ 
  39 & LME & Measure & beta=4 & sigma=2 & n=100 & 0.00 \\ 
  40 & MDE.Phi.chisq & Measure & beta=4 & sigma=2 & n=100 & 0.02 \\ 
  41 & MDE.Phi.tv & Measure & beta=4 & sigma=2 & n=100 & 0.01 \\ 
  42 & MDE.Phi.kl & Measure & beta=4 & sigma=2 & n=100 & 0.00 \\ 
  43 & MME & Measure & beta=4 & sigma=2 & n=100 & 0.00 \\ 
  44 & MME.b & Measure & beta=4 & sigma=2 & n=100 & 4041.95 \\ 
  45 & PWM & Measure & beta=4 & sigma=2 & n=100 & 0.00 \\ 
  46 & MLE & Measure & beta=5 & sigma=2 & n=100 & 0.00 \\ 
  47 & MLE.b & Measure & beta=5 & sigma=2 & n=100 & 0.00 \\ 
  48 & LME & Measure & beta=5 & sigma=2 & n=100 & 0.00 \\ 
  49 & MDE.Phi.chisq & Measure & beta=5 & sigma=2 & n=100 & 0.01 \\ 
  50 & MDE.Phi.tv & Measure & beta=5 & sigma=2 & n=100 & 0.01 \\ 
  51 & MDE.Phi.kl & Measure & beta=5 & sigma=2 & n=100 & 0.00 \\ 
  52 & MME & Measure & beta=5 & sigma=2 & n=100 & 0.00 \\ 
  53 & MME.b & Measure & beta=5 & sigma=2 & n=100 & 515620838018138634806240604226.00 \\ 
  54 & PWM & Measure & beta=5 & sigma=2 & n=100 & 0.00 \\ 
  55 & MLE & Measure & beta=1.5 & sigma=2 & n=200 & 0.00 \\ 
  56 & MLE.b & Measure & beta=1.5 & sigma=2 & n=200 & 0.00 \\ 
  57 & LME & Measure & beta=1.5 & sigma=2 & n=200 & 0.00 \\ 
  58 & MDE.Phi.chisq & Measure & beta=1.5 & sigma=2 & n=200 & 274643118624275331360628286448288226248464468022642204668864084082600222086880608668040080880424622046222024608200240484826064404080888868246080264664220228006844402404026242842008664860822820666228446808646200060266406262242888228420024466628024282446084862640644224086266044024064680440202202400842.00 \\ 
  59 & MDE.Phi.tv & Measure & beta=1.5 & sigma=2 & n=200 & 0.03 \\ 
  60 & MDE.Phi.kl & Measure & beta=1.5 & sigma=2 & n=200 & 0.00 \\ 
  61 & MME & Measure & beta=1.5 & sigma=2 & n=200 & 0.01 \\ 
  62 & MME.b & Measure & beta=1.5 & sigma=2 & n=200 & 0.01 \\ 
  63 & PWM & Measure & beta=1.5 & sigma=2 & n=200 & 0.00 \\ 
  64 & MLE & Measure & beta=2 & sigma=2 & n=200 & 0.00 \\ 
  65 & MLE.b & Measure & beta=2 & sigma=2 & n=200 & 0.00 \\ 
  66 & LME & Measure & beta=2 & sigma=2 & n=200 & 0.00 \\ 
  67 & MDE.Phi.chisq & Measure & beta=2 & sigma=2 & n=200 & 0.02 \\ 
  68 & MDE.Phi.tv & Measure & beta=2 & sigma=2 & n=200 & 0.02 \\ 
  69 & MDE.Phi.kl & Measure & beta=2 & sigma=2 & n=200 & 0.00 \\ 
  70 & MME & Measure & beta=2 & sigma=2 & n=200 & 0.00 \\ 
  71 & MME.b & Measure & beta=2 & sigma=2 & n=200 & 0.00 \\ 
  72 & PWM & Measure & beta=2 & sigma=2 & n=200 & 0.00 \\ 
  73 & MLE & Measure & beta=2.5 & sigma=2 & n=200 & 0.00 \\ 
  74 & MLE.b & Measure & beta=2.5 & sigma=2 & n=200 & 0.00 \\ 
  75 & LME & Measure & beta=2.5 & sigma=2 & n=200 & 0.00 \\ 
  76 & MDE.Phi.chisq & Measure & beta=2.5 & sigma=2 & n=200 & 0.02 \\ 
  77 & MDE.Phi.tv & Measure & beta=2.5 & sigma=2 & n=200 & 0.01 \\ 
  78 & MDE.Phi.kl & Measure & beta=2.5 & sigma=2 & n=200 & 0.00 \\ 
  79 & MME & Measure & beta=2.5 & sigma=2 & n=200 & 0.00 \\ 
  80 & MME.b & Measure & beta=2.5 & sigma=2 & n=200 & 0.00 \\ 
  81 & PWM & Measure & beta=2.5 & sigma=2 & n=200 & 0.00 \\ 
  82 & MLE & Measure & beta=3 & sigma=2 & n=200 & 0.00 \\ 
  83 & MLE.b & Measure & beta=3 & sigma=2 & n=200 & 0.00 \\ 
  84 & LME & Measure & beta=3 & sigma=2 & n=200 & 0.00 \\ 
  85 & MDE.Phi.chisq & Measure & beta=3 & sigma=2 & n=200 & 0.01 \\ 
  86 & MDE.Phi.tv & Measure & beta=3 & sigma=2 & n=200 & 0.01 \\ 
  87 & MDE.Phi.kl & Measure & beta=3 & sigma=2 & n=200 & 0.00 \\ 
  88 & MME & Measure & beta=3 & sigma=2 & n=200 & 0.00 \\ 
  89 & MME.b & Measure & beta=3 & sigma=2 & n=200 & 0.00 \\ 
  90 & PWM & Measure & beta=3 & sigma=2 & n=200 & 0.00 \\ 
  91 & MLE & Measure & beta=4 & sigma=2 & n=200 & 0.00 \\ 
  92 & MLE.b & Measure & beta=4 & sigma=2 & n=200 & 0.00 \\ 
  93 & LME & Measure & beta=4 & sigma=2 & n=200 & 0.00 \\ 
  94 & MDE.Phi.chisq & Measure & beta=4 & sigma=2 & n=200 & 0.01 \\ 
  95 & MDE.Phi.tv & Measure & beta=4 & sigma=2 & n=200 & 0.01 \\ 
  96 & MDE.Phi.kl & Measure & beta=4 & sigma=2 & n=200 & 0.00 \\ 
  97 & MME & Measure & beta=4 & sigma=2 & n=200 & 0.00 \\ 
  98 & MME.b & Measure & beta=4 & sigma=2 & n=200 & 0.00 \\ 
  99 & PWM & Measure & beta=4 & sigma=2 & n=200 & 0.00 \\ 
  100 & MLE & Measure & beta=5 & sigma=2 & n=200 & 0.00 \\ 
  101 & MLE.b & Measure & beta=5 & sigma=2 & n=200 & 0.00 \\ 
  102 & LME & Measure & beta=5 & sigma=2 & n=200 & 0.00 \\ 
  103 & MDE.Phi.chisq & Measure & beta=5 & sigma=2 & n=200 & 0.01 \\ 
  104 & MDE.Phi.tv & Measure & beta=5 & sigma=2 & n=200 & 0.01 \\ 
  105 & MDE.Phi.kl & Measure & beta=5 & sigma=2 & n=200 & 0.00 \\ 
  106 & MME & Measure & beta=5 & sigma=2 & n=200 & 0.00 \\ 
  107 & MME.b & Measure & beta=5 & sigma=2 & n=200 & 2.02 \\ 
  108 & PWM & Measure & beta=5 & sigma=2 & n=200 & 0.00 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220101/Output.bias.LaTeX.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Mon Jan 31 17:32:24 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=2 & n=100 & 0.17 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=2 & n=100 & -0.02 \\ 
  3 & LME & beta & beta=1.5 & sigma=2 & n=100 & 0.33 \\ 
  4 & MDE.Phi.chisq & beta & beta=1.5 & sigma=2 & n=100 & -1.27 \\ 
  5 & MDE.Phi.tv & beta & beta=1.5 & sigma=2 & n=100 & -0.24 \\ 
  6 & MDE.Phi.kl & beta & beta=1.5 & sigma=2 & n=100 & 0.17 \\ 
  7 & MME & beta & beta=1.5 & sigma=2 & n=100 & 1.29 \\ 
  8 & MME.b & beta & beta=1.5 & sigma=2 & n=100 & 4.81 \\ 
  9 & PWM & beta & beta=1.5 & sigma=2 & n=100 & 0.33 \\ 
  10 & MLE & sigma & beta=1.5 & sigma=2 & n=100 & 0.36 \\ 
  11 & MLE.b & sigma & beta=1.5 & sigma=2 & n=100 & -0.05 \\ 
  12 & LME & sigma & beta=1.5 & sigma=2 & n=100 & 0.65 \\ 
  13 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=2 & n=100 & 1.29 \\ 
  14 & MDE.Phi.tv & sigma & beta=1.5 & sigma=2 & n=100 & 1.64 \\ 
  15 & MDE.Phi.kl & sigma & beta=1.5 & sigma=2 & n=100 & 0.36 \\ 
  16 & MME & sigma & beta=1.5 & sigma=2 & n=100 & 4.30 \\ 
  17 & MME.b & sigma & beta=1.5 & sigma=2 & n=100 & 11.67 \\ 
  18 & PWM & sigma & beta=1.5 & sigma=2 & n=100 & 0.65 \\ 
  19 & MLE & beta & beta=2 & sigma=2 & n=100 & 0.54 \\ 
  20 & MLE.b & beta & beta=2 & sigma=2 & n=100 & 0.19 \\ 
  21 & LME & beta & beta=2 & sigma=2 & n=100 & 0.45 \\ 
  22 & MDE.Phi.chisq & beta & beta=2 & sigma=2 & n=100 & 0.10 \\ 
  23 & MDE.Phi.tv & beta & beta=2 & sigma=2 & n=100 & 0.69 \\ 
  24 & MDE.Phi.kl & beta & beta=2 & sigma=2 & n=100 & 0.46 \\ 
  25 & MME & beta & beta=2 & sigma=2 & n=100 & 1.68 \\ 
  26 & MME.b & beta & beta=2 & sigma=2 & n=100 & 7.48 \\ 
  27 & PWM & beta & beta=2 & sigma=2 & n=100 & 0.45 \\ 
  28 & MLE & sigma & beta=2 & sigma=2 & n=100 & 0.75 \\ 
  29 & MLE.b & sigma & beta=2 & sigma=2 & n=100 & 0.24 \\ 
  30 & LME & sigma & beta=2 & sigma=2 & n=100 & 0.60 \\ 
  31 & MDE.Phi.chisq & sigma & beta=2 & sigma=2 & n=100 & 2.19 \\ 
  32 & MDE.Phi.tv & sigma & beta=2 & sigma=2 & n=100 & 3.22 \\ 
  33 & MDE.Phi.kl & sigma & beta=2 & sigma=2 & n=100 & 0.65 \\ 
  34 & MME & sigma & beta=2 & sigma=2 & n=100 & 2.87 \\ 
  35 & MME.b & sigma & beta=2 & sigma=2 & n=100 & 11.17 \\ 
  36 & PWM & sigma & beta=2 & sigma=2 & n=100 & 0.60 \\ 
  37 & MLE & beta & beta=2.5 & sigma=2 & n=100 & 1.09 \\ 
  38 & MLE.b & beta & beta=2.5 & sigma=2 & n=100 & 0.63 \\ 
  39 & LME & beta & beta=2.5 & sigma=2 & n=100 & 0.70 \\ 
  40 & MDE.Phi.chisq & beta & beta=2.5 & sigma=2 & n=100 & 1.61 \\ 
  41 & MDE.Phi.tv & beta & beta=2.5 & sigma=2 & n=100 & 2.43 \\ 
  42 & MDE.Phi.kl & beta & beta=2.5 & sigma=2 & n=100 & 0.94 \\ 
  43 & MME & beta & beta=2.5 & sigma=2 & n=100 & 2.32 \\ 
  44 & MME.b & beta & beta=2.5 & sigma=2 & n=100 & 5.49 \\ 
  45 & PWM & beta & beta=2.5 & sigma=2 & n=100 & 0.70 \\ 
  46 & MLE & sigma & beta=2.5 & sigma=2 & n=100 & 1.17 \\ 
  47 & MLE.b & sigma & beta=2.5 & sigma=2 & n=100 & 0.67 \\ 
  48 & LME & sigma & beta=2.5 & sigma=2 & n=100 & 0.72 \\ 
  49 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=2 & n=100 & 4.14 \\ 
  50 & MDE.Phi.tv & sigma & beta=2.5 & sigma=2 & n=100 & 5.19 \\ 
  51 & MDE.Phi.kl & sigma & beta=2.5 & sigma=2 & n=100 & 1.01 \\ 
  52 & MME & sigma & beta=2.5 & sigma=2 & n=100 & 2.71 \\ 
  53 & MME.b & sigma & beta=2.5 & sigma=2 & n=100 & 6.04 \\ 
  54 & PWM & sigma & beta=2.5 & sigma=2 & n=100 & 0.72 \\ 
  55 & MLE & beta & beta=3 & sigma=2 & n=100 & 2.75 \\ 
  56 & MLE.b & beta & beta=3 & sigma=2 & n=100 & 2.26 \\ 
  57 & LME & beta & beta=3 & sigma=2 & n=100 & 1.02 \\ 
  58 & MDE.Phi.chisq & beta & beta=3 & sigma=2 & n=100 & 3.82 \\ 
  59 & MDE.Phi.tv & beta & beta=3 & sigma=2 & n=100 & 5.23 \\ 
  60 & MDE.Phi.kl & beta & beta=3 & sigma=2 & n=100 & 1.86 \\ 
  61 & MME & beta & beta=3 & sigma=2 & n=100 & 14.49 \\ 
  62 & MME.b & beta & beta=3 & sigma=2 & n=100 & 46.99 \\ 
  63 & PWM & beta & beta=3 & sigma=2 & n=100 & 1.02 \\ 
  64 & MLE & sigma & beta=3 & sigma=2 & n=100 & 2.37 \\ 
  65 & MLE.b & sigma & beta=3 & sigma=2 & n=100 & 1.94 \\ 
  66 & LME & sigma & beta=3 & sigma=2 & n=100 & 0.85 \\ 
  67 & MDE.Phi.chisq & sigma & beta=3 & sigma=2 & n=100 & 6.25 \\ 
  68 & MDE.Phi.tv & sigma & beta=3 & sigma=2 & n=100 & 7.70 \\ 
  69 & MDE.Phi.kl & sigma & beta=3 & sigma=2 & n=100 & 1.60 \\ 
  70 & MME & sigma & beta=3 & sigma=2 & n=100 & 11.48 \\ 
  71 & MME.b & sigma & beta=3 & sigma=2 & n=100 & 37.14 \\ 
  72 & PWM & sigma & beta=3 & sigma=2 & n=100 & 0.85 \\ 
  73 & MLE & beta & beta=4 & sigma=2 & n=100 & 4.73 \\ 
  74 & MLE.b & beta & beta=4 & sigma=2 & n=100 & 4.28 \\ 
  75 & LME & beta & beta=4 & sigma=2 & n=100 & 1.76 \\ 
  76 & MDE.Phi.chisq & beta & beta=4 & sigma=2 & n=100 & 9.77 \\ 
  77 & MDE.Phi.tv & beta & beta=4 & sigma=2 & n=100 & 11.95 \\ 
  78 & MDE.Phi.kl & beta & beta=4 & sigma=2 & n=100 & 3.42 \\ 
  79 & MME & beta & beta=4 & sigma=2 & n=100 & 7.36 \\ 
  80 & MME.b & beta & beta=4 & sigma=2 & n=100 & 36.91 \\ 
  81 & PWM & beta & beta=4 & sigma=2 & n=100 & 1.76 \\ 
  82 & MLE & sigma & beta=4 & sigma=2 & n=100 & 2.93 \\ 
  83 & MLE.b & sigma & beta=4 & sigma=2 & n=100 & 2.65 \\ 
  84 & LME & sigma & beta=4 & sigma=2 & n=100 & 1.07 \\ 
  85 & MDE.Phi.chisq & sigma & beta=4 & sigma=2 & n=100 & 9.83 \\ 
  86 & MDE.Phi.tv & sigma & beta=4 & sigma=2 & n=100 & 11.26 \\ 
  87 & MDE.Phi.kl & sigma & beta=4 & sigma=2 & n=100 & 2.12 \\ 
  88 & MME & sigma & beta=4 & sigma=2 & n=100 & 4.67 \\ 
  89 & MME.b & sigma & beta=4 & sigma=2 & n=100 & 24.87 \\ 
  90 & PWM & sigma & beta=4 & sigma=2 & n=100 & 1.07 \\ 
  91 & MLE & beta & beta=5 & sigma=2 & n=100 & 7.32 \\ 
  92 & MLE.b & beta & beta=5 & sigma=2 & n=100 & 6.96 \\ 
  93 & LME & beta & beta=5 & sigma=2 & n=100 & 2.36 \\ 
  94 & MDE.Phi.chisq & beta & beta=5 & sigma=2 & n=100 & 15.09 \\ 
  95 & MDE.Phi.tv & beta & beta=5 & sigma=2 & n=100 & 17.24 \\ 
  96 & MDE.Phi.kl & beta & beta=5 & sigma=2 & n=100 & 5.06 \\ 
  97 & MME & beta & beta=5 & sigma=2 & n=100 & 11.73 \\ 
  98 & MME.b & beta & beta=5 & sigma=2 & n=100 & 42.16 \\ 
  99 & PWM & beta & beta=5 & sigma=2 & n=100 & 2.36 \\ 
  100 & MLE & sigma & beta=5 & sigma=2 & n=100 & 3.45 \\ 
  101 & MLE.b & sigma & beta=5 & sigma=2 & n=100 & 3.28 \\ 
  102 & LME & sigma & beta=5 & sigma=2 & n=100 & 1.10 \\ 
  103 & MDE.Phi.chisq & sigma & beta=5 & sigma=2 & n=100 & 11.18 \\ 
  104 & MDE.Phi.tv & sigma & beta=5 & sigma=2 & n=100 & 12.16 \\ 
  105 & MDE.Phi.kl & sigma & beta=5 & sigma=2 & n=100 & 2.38 \\ 
  106 & MME & sigma & beta=5 & sigma=2 & n=100 & 5.50 \\ 
  107 & MME.b & sigma & beta=5 & sigma=2 & n=100 & 19.93 \\ 
  108 & PWM & sigma & beta=5 & sigma=2 & n=100 & 1.10 \\ 
  109 & MLE & beta & beta=1.5 & sigma=2 & n=200 & 0.23 \\ 
  110 & MLE.b & beta & beta=1.5 & sigma=2 & n=200 & 0.13 \\ 
  111 & LME & beta & beta=1.5 & sigma=2 & n=200 & 0.21 \\ 
  112 & MDE.Phi.chisq & beta & beta=1.5 & sigma=2 & n=200 & -0.85 \\ 
  113 & MDE.Phi.tv & beta & beta=1.5 & sigma=2 & n=200 & -0.50 \\ 
  114 & MDE.Phi.kl & beta & beta=1.5 & sigma=2 & n=200 & 0.08 \\ 
  115 & MME & beta & beta=1.5 & sigma=2 & n=200 & 1.00 \\ 
  116 & MME.b & beta & beta=1.5 & sigma=2 & n=200 & 0.80 \\ 
  117 & PWM & beta & beta=1.5 & sigma=2 & n=200 & 0.21 \\ 
  118 & MLE & sigma & beta=1.5 & sigma=2 & n=200 & 0.48 \\ 
  119 & MLE.b & sigma & beta=1.5 & sigma=2 & n=200 & 0.26 \\ 
  120 & LME & sigma & beta=1.5 & sigma=2 & n=200 & 0.40 \\ 
  121 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=2 & n=200 & 0.32 \\ 
  122 & MDE.Phi.tv & sigma & beta=1.5 & sigma=2 & n=200 & 0.51 \\ 
  123 & MDE.Phi.kl & sigma & beta=1.5 & sigma=2 & n=200 & 0.16 \\ 
  124 & MME & sigma & beta=1.5 & sigma=2 & n=200 & 3.57 \\ 
  125 & MME.b & sigma & beta=1.5 & sigma=2 & n=200 & 3.02 \\ 
  126 & PWM & sigma & beta=1.5 & sigma=2 & n=200 & 0.40 \\ 
  127 & MLE & beta & beta=2 & sigma=2 & n=200 & 0.25 \\ 
  128 & MLE.b & beta & beta=2 & sigma=2 & n=200 & 0.06 \\ 
  129 & LME & beta & beta=2 & sigma=2 & n=200 & 0.22 \\ 
  130 & MDE.Phi.chisq & beta & beta=2 & sigma=2 & n=200 & -0.65 \\ 
  131 & MDE.Phi.tv & beta & beta=2 & sigma=2 & n=200 & -0.44 \\ 
  132 & MDE.Phi.kl & beta & beta=2 & sigma=2 & n=200 & 0.14 \\ 
  133 & MME & beta & beta=2 & sigma=2 & n=200 & 0.97 \\ 
  134 & MME.b & beta & beta=2 & sigma=2 & n=200 & 0.69 \\ 
  135 & PWM & beta & beta=2 & sigma=2 & n=200 & 0.22 \\ 
  136 & MLE & sigma & beta=2 & sigma=2 & n=200 & 0.35 \\ 
  137 & MLE.b & sigma & beta=2 & sigma=2 & n=200 & 0.08 \\ 
  138 & LME & sigma & beta=2 & sigma=2 & n=200 & 0.28 \\ 
  139 & MDE.Phi.chisq & sigma & beta=2 & sigma=2 & n=200 & 0.34 \\ 
  140 & MDE.Phi.tv & sigma & beta=2 & sigma=2 & n=200 & 0.56 \\ 
  141 & MDE.Phi.kl & sigma & beta=2 & sigma=2 & n=200 & 0.19 \\ 
  142 & MME & sigma & beta=2 & sigma=2 & n=200 & 1.78 \\ 
  143 & MME.b & sigma & beta=2 & sigma=2 & n=200 & 1.29 \\ 
  144 & PWM & sigma & beta=2 & sigma=2 & n=200 & 0.28 \\ 
  145 & MLE & beta & beta=2.5 & sigma=2 & n=200 & 0.34 \\ 
  146 & MLE.b & beta & beta=2.5 & sigma=2 & n=200 & 0.02 \\ 
  147 & LME & beta & beta=2.5 & sigma=2 & n=200 & 0.28 \\ 
  148 & MDE.Phi.chisq & beta & beta=2.5 & sigma=2 & n=200 & -0.45 \\ 
  149 & MDE.Phi.tv & beta & beta=2.5 & sigma=2 & n=200 & -0.22 \\ 
  150 & MDE.Phi.kl & beta & beta=2.5 & sigma=2 & n=200 & 0.25 \\ 
  151 & MME & beta & beta=2.5 & sigma=2 & n=200 & 1.06 \\ 
  152 & MME.b & beta & beta=2.5 & sigma=2 & n=200 & 0.84 \\ 
  153 & PWM & beta & beta=2.5 & sigma=2 & n=200 & 0.28 \\ 
  154 & MLE & sigma & beta=2.5 & sigma=2 & n=200 & 0.37 \\ 
  155 & MLE.b & sigma & beta=2.5 & sigma=2 & n=200 & 0.02 \\ 
  156 & LME & sigma & beta=2.5 & sigma=2 & n=200 & 0.29 \\ 
  157 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=2 & n=200 & 0.70 \\ 
  158 & MDE.Phi.tv & sigma & beta=2.5 & sigma=2 & n=200 & 0.81 \\ 
  159 & MDE.Phi.kl & sigma & beta=2.5 & sigma=2 & n=200 & 0.27 \\ 
  160 & MME & sigma & beta=2.5 & sigma=2 & n=200 & 1.31 \\ 
  161 & MME.b & sigma & beta=2.5 & sigma=2 & n=200 & 1.01 \\ 
  162 & PWM & sigma & beta=2.5 & sigma=2 & n=200 & 0.29 \\ 
  163 & MLE & beta & beta=3 & sigma=2 & n=200 & 0.72 \\ 
  164 & MLE.b & beta & beta=3 & sigma=2 & n=200 & 0.23 \\ 
  165 & LME & beta & beta=3 & sigma=2 & n=200 & 0.45 \\ 
  166 & MDE.Phi.chisq & beta & beta=3 & sigma=2 & n=200 & 0.31 \\ 
  167 & MDE.Phi.tv & beta & beta=3 & sigma=2 & n=200 & 0.21 \\ 
  168 & MDE.Phi.kl & beta & beta=3 & sigma=2 & n=200 & 0.49 \\ 
  169 & MME & beta & beta=3 & sigma=2 & n=200 & 1.40 \\ 
  170 & MME.b & beta & beta=3 & sigma=2 & n=200 & 2.69 \\ 
  171 & PWM & beta & beta=3 & sigma=2 & n=200 & 0.45 \\ 
  172 & MLE & sigma & beta=3 & sigma=2 & n=200 & 0.62 \\ 
  173 & MLE.b & sigma & beta=3 & sigma=2 & n=200 & 0.20 \\ 
  174 & LME & sigma & beta=3 & sigma=2 & n=200 & 0.38 \\ 
  175 & MDE.Phi.chisq & sigma & beta=3 & sigma=2 & n=200 & 1.54 \\ 
  176 & MDE.Phi.tv & sigma & beta=3 & sigma=2 & n=200 & 1.19 \\ 
  177 & MDE.Phi.kl & sigma & beta=3 & sigma=2 & n=200 & 0.43 \\ 
  178 & MME & sigma & beta=3 & sigma=2 & n=200 & 1.29 \\ 
  179 & MME.b & sigma & beta=3 & sigma=2 & n=200 & 2.46 \\ 
  180 & PWM & sigma & beta=3 & sigma=2 & n=200 & 0.38 \\ 
  181 & MLE & beta & beta=4 & sigma=2 & n=200 & 1.56 \\ 
  182 & MLE.b & beta & beta=4 & sigma=2 & n=200 & 0.88 \\ 
  183 & LME & beta & beta=4 & sigma=2 & n=200 & 0.91 \\ 
  184 & MDE.Phi.chisq & beta & beta=4 & sigma=2 & n=200 & 3.71 \\ 
  185 & MDE.Phi.tv & beta & beta=4 & sigma=2 & n=200 & 2.95 \\ 
  186 & MDE.Phi.kl & beta & beta=4 & sigma=2 & n=200 & 1.26 \\ 
  187 & MME & beta & beta=4 & sigma=2 & n=200 & 2.64 \\ 
  188 & MME.b & beta & beta=4 & sigma=2 & n=200 & 9.69 \\ 
  189 & PWM & beta & beta=4 & sigma=2 & n=200 & 0.91 \\ 
  190 & MLE & sigma & beta=4 & sigma=2 & n=200 & 0.98 \\ 
  191 & MLE.b & sigma & beta=4 & sigma=2 & n=200 & 0.56 \\ 
  192 & LME & sigma & beta=4 & sigma=2 & n=200 & 0.55 \\ 
  193 & MDE.Phi.chisq & sigma & beta=4 & sigma=2 & n=200 & 4.00 \\ 
  194 & MDE.Phi.tv & sigma & beta=4 & sigma=2 & n=200 & 3.13 \\ 
  195 & MDE.Phi.kl & sigma & beta=4 & sigma=2 & n=200 & 0.77 \\ 
  196 & MME & sigma & beta=4 & sigma=2 & n=200 & 1.66 \\ 
  197 & MME.b & sigma & beta=4 & sigma=2 & n=200 & 6.25 \\ 
  198 & PWM & sigma & beta=4 & sigma=2 & n=200 & 0.55 \\ 
  199 & MLE & beta & beta=5 & sigma=2 & n=200 & 4.92 \\ 
  200 & MLE.b & beta & beta=5 & sigma=2 & n=200 & 4.21 \\ 
  201 & LME & beta & beta=5 & sigma=2 & n=200 & 1.78 \\ 
  202 & MDE.Phi.chisq & beta & beta=5 & sigma=2 & n=200 & 9.13 \\ 
  203 & MDE.Phi.tv & beta & beta=5 & sigma=2 & n=200 & 6.36 \\ 
  204 & MDE.Phi.kl & beta & beta=5 & sigma=2 & n=200 & 2.60 \\ 
  205 & MME & beta & beta=5 & sigma=2 & n=200 & 4.76 \\ 
  206 & MME.b & beta & beta=5 & sigma=2 & n=200 & 16.59 \\ 
  207 & PWM & beta & beta=5 & sigma=2 & n=200 & 1.78 \\ 
  208 & MLE & sigma & beta=5 & sigma=2 & n=200 & 2.38 \\ 
  209 & MLE.b & sigma & beta=5 & sigma=2 & n=200 & 2.04 \\ 
  210 & LME & sigma & beta=5 & sigma=2 & n=200 & 0.83 \\ 
  211 & MDE.Phi.chisq & sigma & beta=5 & sigma=2 & n=200 & 6.54 \\ 
  212 & MDE.Phi.tv & sigma & beta=5 & sigma=2 & n=200 & 4.51 \\ 
  213 & MDE.Phi.kl & sigma & beta=5 & sigma=2 & n=200 & 1.23 \\ 
  214 & MME & sigma & beta=5 & sigma=2 & n=200 & 2.27 \\ 
  215 & MME.b & sigma & beta=5 & sigma=2 & n=200 & 7.87 \\ 
  216 & PWM & sigma & beta=5 & sigma=2 & n=200 & 0.83 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220101/Output.mean.LaTeX.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Mon Jan 31 17:32:24 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=2 & n=100 & 1.67 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=2 & n=100 & 1.48 \\ 
  3 & LME & beta & beta=1.5 & sigma=2 & n=100 & 1.83 \\ 
  4 & MDE.Phi.chisq & beta & beta=1.5 & sigma=2 & n=100 & 0.23 \\ 
  5 & MDE.Phi.tv & beta & beta=1.5 & sigma=2 & n=100 & 1.26 \\ 
  6 & MDE.Phi.kl & beta & beta=1.5 & sigma=2 & n=100 & 1.67 \\ 
  7 & MME & beta & beta=1.5 & sigma=2 & n=100 & 2.79 \\ 
  8 & MME.b & beta & beta=1.5 & sigma=2 & n=100 & 6.31 \\ 
  9 & PWM & beta & beta=1.5 & sigma=2 & n=100 & 1.83 \\ 
  10 & MLE & sigma & beta=1.5 & sigma=2 & n=100 & 2.36 \\ 
  11 & MLE.b & sigma & beta=1.5 & sigma=2 & n=100 & 1.95 \\ 
  12 & LME & sigma & beta=1.5 & sigma=2 & n=100 & 2.65 \\ 
  13 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=2 & n=100 & 3.29 \\ 
  14 & MDE.Phi.tv & sigma & beta=1.5 & sigma=2 & n=100 & 3.64 \\ 
  15 & MDE.Phi.kl & sigma & beta=1.5 & sigma=2 & n=100 & 2.36 \\ 
  16 & MME & sigma & beta=1.5 & sigma=2 & n=100 & 6.30 \\ 
  17 & MME.b & sigma & beta=1.5 & sigma=2 & n=100 & 13.67 \\ 
  18 & PWM & sigma & beta=1.5 & sigma=2 & n=100 & 2.65 \\ 
  19 & MLE & beta & beta=2 & sigma=2 & n=100 & 2.54 \\ 
  20 & MLE.b & beta & beta=2 & sigma=2 & n=100 & 2.19 \\ 
  21 & LME & beta & beta=2 & sigma=2 & n=100 & 2.45 \\ 
  22 & MDE.Phi.chisq & beta & beta=2 & sigma=2 & n=100 & 2.10 \\ 
  23 & MDE.Phi.tv & beta & beta=2 & sigma=2 & n=100 & 2.69 \\ 
  24 & MDE.Phi.kl & beta & beta=2 & sigma=2 & n=100 & 2.46 \\ 
  25 & MME & beta & beta=2 & sigma=2 & n=100 & 3.68 \\ 
  26 & MME.b & beta & beta=2 & sigma=2 & n=100 & 9.48 \\ 
  27 & PWM & beta & beta=2 & sigma=2 & n=100 & 2.45 \\ 
  28 & MLE & sigma & beta=2 & sigma=2 & n=100 & 2.75 \\ 
  29 & MLE.b & sigma & beta=2 & sigma=2 & n=100 & 2.24 \\ 
  30 & LME & sigma & beta=2 & sigma=2 & n=100 & 2.60 \\ 
  31 & MDE.Phi.chisq & sigma & beta=2 & sigma=2 & n=100 & 4.19 \\ 
  32 & MDE.Phi.tv & sigma & beta=2 & sigma=2 & n=100 & 5.22 \\ 
  33 & MDE.Phi.kl & sigma & beta=2 & sigma=2 & n=100 & 2.65 \\ 
  34 & MME & sigma & beta=2 & sigma=2 & n=100 & 4.87 \\ 
  35 & MME.b & sigma & beta=2 & sigma=2 & n=100 & 13.17 \\ 
  36 & PWM & sigma & beta=2 & sigma=2 & n=100 & 2.60 \\ 
  37 & MLE & beta & beta=2.5 & sigma=2 & n=100 & 3.59 \\ 
  38 & MLE.b & beta & beta=2.5 & sigma=2 & n=100 & 3.13 \\ 
  39 & LME & beta & beta=2.5 & sigma=2 & n=100 & 3.20 \\ 
  40 & MDE.Phi.chisq & beta & beta=2.5 & sigma=2 & n=100 & 4.11 \\ 
  41 & MDE.Phi.tv & beta & beta=2.5 & sigma=2 & n=100 & 4.93 \\ 
  42 & MDE.Phi.kl & beta & beta=2.5 & sigma=2 & n=100 & 3.44 \\ 
  43 & MME & beta & beta=2.5 & sigma=2 & n=100 & 4.82 \\ 
  44 & MME.b & beta & beta=2.5 & sigma=2 & n=100 & 7.99 \\ 
  45 & PWM & beta & beta=2.5 & sigma=2 & n=100 & 3.20 \\ 
  46 & MLE & sigma & beta=2.5 & sigma=2 & n=100 & 3.17 \\ 
  47 & MLE.b & sigma & beta=2.5 & sigma=2 & n=100 & 2.67 \\ 
  48 & LME & sigma & beta=2.5 & sigma=2 & n=100 & 2.72 \\ 
  49 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=2 & n=100 & 6.14 \\ 
  50 & MDE.Phi.tv & sigma & beta=2.5 & sigma=2 & n=100 & 7.19 \\ 
  51 & MDE.Phi.kl & sigma & beta=2.5 & sigma=2 & n=100 & 3.01 \\ 
  52 & MME & sigma & beta=2.5 & sigma=2 & n=100 & 4.71 \\ 
  53 & MME.b & sigma & beta=2.5 & sigma=2 & n=100 & 8.04 \\ 
  54 & PWM & sigma & beta=2.5 & sigma=2 & n=100 & 2.72 \\ 
  55 & MLE & beta & beta=3 & sigma=2 & n=100 & 5.75 \\ 
  56 & MLE.b & beta & beta=3 & sigma=2 & n=100 & 5.26 \\ 
  57 & LME & beta & beta=3 & sigma=2 & n=100 & 4.02 \\ 
  58 & MDE.Phi.chisq & beta & beta=3 & sigma=2 & n=100 & 6.82 \\ 
  59 & MDE.Phi.tv & beta & beta=3 & sigma=2 & n=100 & 8.23 \\ 
  60 & MDE.Phi.kl & beta & beta=3 & sigma=2 & n=100 & 4.86 \\ 
  61 & MME & beta & beta=3 & sigma=2 & n=100 & 17.49 \\ 
  62 & MME.b & beta & beta=3 & sigma=2 & n=100 & 49.99 \\ 
  63 & PWM & beta & beta=3 & sigma=2 & n=100 & 4.02 \\ 
  64 & MLE & sigma & beta=3 & sigma=2 & n=100 & 4.37 \\ 
  65 & MLE.b & sigma & beta=3 & sigma=2 & n=100 & 3.94 \\ 
  66 & LME & sigma & beta=3 & sigma=2 & n=100 & 2.85 \\ 
  67 & MDE.Phi.chisq & sigma & beta=3 & sigma=2 & n=100 & 8.25 \\ 
  68 & MDE.Phi.tv & sigma & beta=3 & sigma=2 & n=100 & 9.70 \\ 
  69 & MDE.Phi.kl & sigma & beta=3 & sigma=2 & n=100 & 3.60 \\ 
  70 & MME & sigma & beta=3 & sigma=2 & n=100 & 13.48 \\ 
  71 & MME.b & sigma & beta=3 & sigma=2 & n=100 & 39.14 \\ 
  72 & PWM & sigma & beta=3 & sigma=2 & n=100 & 2.85 \\ 
  73 & MLE & beta & beta=4 & sigma=2 & n=100 & 8.73 \\ 
  74 & MLE.b & beta & beta=4 & sigma=2 & n=100 & 8.28 \\ 
  75 & LME & beta & beta=4 & sigma=2 & n=100 & 5.76 \\ 
  76 & MDE.Phi.chisq & beta & beta=4 & sigma=2 & n=100 & 13.77 \\ 
  77 & MDE.Phi.tv & beta & beta=4 & sigma=2 & n=100 & 15.95 \\ 
  78 & MDE.Phi.kl & beta & beta=4 & sigma=2 & n=100 & 7.42 \\ 
  79 & MME & beta & beta=4 & sigma=2 & n=100 & 11.36 \\ 
  80 & MME.b & beta & beta=4 & sigma=2 & n=100 & 40.91 \\ 
  81 & PWM & beta & beta=4 & sigma=2 & n=100 & 5.76 \\ 
  82 & MLE & sigma & beta=4 & sigma=2 & n=100 & 4.93 \\ 
  83 & MLE.b & sigma & beta=4 & sigma=2 & n=100 & 4.65 \\ 
  84 & LME & sigma & beta=4 & sigma=2 & n=100 & 3.07 \\ 
  85 & MDE.Phi.chisq & sigma & beta=4 & sigma=2 & n=100 & 11.83 \\ 
  86 & MDE.Phi.tv & sigma & beta=4 & sigma=2 & n=100 & 13.26 \\ 
  87 & MDE.Phi.kl & sigma & beta=4 & sigma=2 & n=100 & 4.12 \\ 
  88 & MME & sigma & beta=4 & sigma=2 & n=100 & 6.67 \\ 
  89 & MME.b & sigma & beta=4 & sigma=2 & n=100 & 26.87 \\ 
  90 & PWM & sigma & beta=4 & sigma=2 & n=100 & 3.07 \\ 
  91 & MLE & beta & beta=5 & sigma=2 & n=100 & 12.32 \\ 
  92 & MLE.b & beta & beta=5 & sigma=2 & n=100 & 11.96 \\ 
  93 & LME & beta & beta=5 & sigma=2 & n=100 & 7.36 \\ 
  94 & MDE.Phi.chisq & beta & beta=5 & sigma=2 & n=100 & 20.09 \\ 
  95 & MDE.Phi.tv & beta & beta=5 & sigma=2 & n=100 & 22.24 \\ 
  96 & MDE.Phi.kl & beta & beta=5 & sigma=2 & n=100 & 10.06 \\ 
  97 & MME & beta & beta=5 & sigma=2 & n=100 & 16.73 \\ 
  98 & MME.b & beta & beta=5 & sigma=2 & n=100 & 47.16 \\ 
  99 & PWM & beta & beta=5 & sigma=2 & n=100 & 7.36 \\ 
  100 & MLE & sigma & beta=5 & sigma=2 & n=100 & 5.45 \\ 
  101 & MLE.b & sigma & beta=5 & sigma=2 & n=100 & 5.28 \\ 
  102 & LME & sigma & beta=5 & sigma=2 & n=100 & 3.10 \\ 
  103 & MDE.Phi.chisq & sigma & beta=5 & sigma=2 & n=100 & 13.18 \\ 
  104 & MDE.Phi.tv & sigma & beta=5 & sigma=2 & n=100 & 14.16 \\ 
  105 & MDE.Phi.kl & sigma & beta=5 & sigma=2 & n=100 & 4.38 \\ 
  106 & MME & sigma & beta=5 & sigma=2 & n=100 & 7.50 \\ 
  107 & MME.b & sigma & beta=5 & sigma=2 & n=100 & 21.93 \\ 
  108 & PWM & sigma & beta=5 & sigma=2 & n=100 & 3.10 \\ 
  109 & MLE & beta & beta=1.5 & sigma=2 & n=200 & 1.73 \\ 
  110 & MLE.b & beta & beta=1.5 & sigma=2 & n=200 & 1.63 \\ 
  111 & LME & beta & beta=1.5 & sigma=2 & n=200 & 1.71 \\ 
  112 & MDE.Phi.chisq & beta & beta=1.5 & sigma=2 & n=200 & 0.65 \\ 
  113 & MDE.Phi.tv & beta & beta=1.5 & sigma=2 & n=200 & 1.00 \\ 
  114 & MDE.Phi.kl & beta & beta=1.5 & sigma=2 & n=200 & 1.58 \\ 
  115 & MME & beta & beta=1.5 & sigma=2 & n=200 & 2.50 \\ 
  116 & MME.b & beta & beta=1.5 & sigma=2 & n=200 & 2.30 \\ 
  117 & PWM & beta & beta=1.5 & sigma=2 & n=200 & 1.71 \\ 
  118 & MLE & sigma & beta=1.5 & sigma=2 & n=200 & 2.48 \\ 
  119 & MLE.b & sigma & beta=1.5 & sigma=2 & n=200 & 2.26 \\ 
  120 & LME & sigma & beta=1.5 & sigma=2 & n=200 & 2.40 \\ 
  121 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=2 & n=200 & 2.32 \\ 
  122 & MDE.Phi.tv & sigma & beta=1.5 & sigma=2 & n=200 & 2.51 \\ 
  123 & MDE.Phi.kl & sigma & beta=1.5 & sigma=2 & n=200 & 2.16 \\ 
  124 & MME & sigma & beta=1.5 & sigma=2 & n=200 & 5.57 \\ 
  125 & MME.b & sigma & beta=1.5 & sigma=2 & n=200 & 5.02 \\ 
  126 & PWM & sigma & beta=1.5 & sigma=2 & n=200 & 2.40 \\ 
  127 & MLE & beta & beta=2 & sigma=2 & n=200 & 2.25 \\ 
  128 & MLE.b & beta & beta=2 & sigma=2 & n=200 & 2.06 \\ 
  129 & LME & beta & beta=2 & sigma=2 & n=200 & 2.22 \\ 
  130 & MDE.Phi.chisq & beta & beta=2 & sigma=2 & n=200 & 1.35 \\ 
  131 & MDE.Phi.tv & beta & beta=2 & sigma=2 & n=200 & 1.56 \\ 
  132 & MDE.Phi.kl & beta & beta=2 & sigma=2 & n=200 & 2.14 \\ 
  133 & MME & beta & beta=2 & sigma=2 & n=200 & 2.97 \\ 
  134 & MME.b & beta & beta=2 & sigma=2 & n=200 & 2.69 \\ 
  135 & PWM & beta & beta=2 & sigma=2 & n=200 & 2.22 \\ 
  136 & MLE & sigma & beta=2 & sigma=2 & n=200 & 2.35 \\ 
  137 & MLE.b & sigma & beta=2 & sigma=2 & n=200 & 2.08 \\ 
  138 & LME & sigma & beta=2 & sigma=2 & n=200 & 2.28 \\ 
  139 & MDE.Phi.chisq & sigma & beta=2 & sigma=2 & n=200 & 2.34 \\ 
  140 & MDE.Phi.tv & sigma & beta=2 & sigma=2 & n=200 & 2.56 \\ 
  141 & MDE.Phi.kl & sigma & beta=2 & sigma=2 & n=200 & 2.19 \\ 
  142 & MME & sigma & beta=2 & sigma=2 & n=200 & 3.78 \\ 
  143 & MME.b & sigma & beta=2 & sigma=2 & n=200 & 3.29 \\ 
  144 & PWM & sigma & beta=2 & sigma=2 & n=200 & 2.28 \\ 
  145 & MLE & beta & beta=2.5 & sigma=2 & n=200 & 2.84 \\ 
  146 & MLE.b & beta & beta=2.5 & sigma=2 & n=200 & 2.52 \\ 
  147 & LME & beta & beta=2.5 & sigma=2 & n=200 & 2.78 \\ 
  148 & MDE.Phi.chisq & beta & beta=2.5 & sigma=2 & n=200 & 2.05 \\ 
  149 & MDE.Phi.tv & beta & beta=2.5 & sigma=2 & n=200 & 2.28 \\ 
  150 & MDE.Phi.kl & beta & beta=2.5 & sigma=2 & n=200 & 2.75 \\ 
  151 & MME & beta & beta=2.5 & sigma=2 & n=200 & 3.56 \\ 
  152 & MME.b & beta & beta=2.5 & sigma=2 & n=200 & 3.34 \\ 
  153 & PWM & beta & beta=2.5 & sigma=2 & n=200 & 2.78 \\ 
  154 & MLE & sigma & beta=2.5 & sigma=2 & n=200 & 2.37 \\ 
  155 & MLE.b & sigma & beta=2.5 & sigma=2 & n=200 & 2.02 \\ 
  156 & LME & sigma & beta=2.5 & sigma=2 & n=200 & 2.29 \\ 
  157 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=2 & n=200 & 2.70 \\ 
  158 & MDE.Phi.tv & sigma & beta=2.5 & sigma=2 & n=200 & 2.81 \\ 
  159 & MDE.Phi.kl & sigma & beta=2.5 & sigma=2 & n=200 & 2.27 \\ 
  160 & MME & sigma & beta=2.5 & sigma=2 & n=200 & 3.31 \\ 
  161 & MME.b & sigma & beta=2.5 & sigma=2 & n=200 & 3.01 \\ 
  162 & PWM & sigma & beta=2.5 & sigma=2 & n=200 & 2.29 \\ 
  163 & MLE & beta & beta=3 & sigma=2 & n=200 & 3.72 \\ 
  164 & MLE.b & beta & beta=3 & sigma=2 & n=200 & 3.23 \\ 
  165 & LME & beta & beta=3 & sigma=2 & n=200 & 3.45 \\ 
  166 & MDE.Phi.chisq & beta & beta=3 & sigma=2 & n=200 & 3.31 \\ 
  167 & MDE.Phi.tv & beta & beta=3 & sigma=2 & n=200 & 3.21 \\ 
  168 & MDE.Phi.kl & beta & beta=3 & sigma=2 & n=200 & 3.49 \\ 
  169 & MME & beta & beta=3 & sigma=2 & n=200 & 4.40 \\ 
  170 & MME.b & beta & beta=3 & sigma=2 & n=200 & 5.69 \\ 
  171 & PWM & beta & beta=3 & sigma=2 & n=200 & 3.45 \\ 
  172 & MLE & sigma & beta=3 & sigma=2 & n=200 & 2.62 \\ 
  173 & MLE.b & sigma & beta=3 & sigma=2 & n=200 & 2.20 \\ 
  174 & LME & sigma & beta=3 & sigma=2 & n=200 & 2.38 \\ 
  175 & MDE.Phi.chisq & sigma & beta=3 & sigma=2 & n=200 & 3.54 \\ 
  176 & MDE.Phi.tv & sigma & beta=3 & sigma=2 & n=200 & 3.19 \\ 
  177 & MDE.Phi.kl & sigma & beta=3 & sigma=2 & n=200 & 2.43 \\ 
  178 & MME & sigma & beta=3 & sigma=2 & n=200 & 3.29 \\ 
  179 & MME.b & sigma & beta=3 & sigma=2 & n=200 & 4.46 \\ 
  180 & PWM & sigma & beta=3 & sigma=2 & n=200 & 2.38 \\ 
  181 & MLE & beta & beta=4 & sigma=2 & n=200 & 5.56 \\ 
  182 & MLE.b & beta & beta=4 & sigma=2 & n=200 & 4.88 \\ 
  183 & LME & beta & beta=4 & sigma=2 & n=200 & 4.91 \\ 
  184 & MDE.Phi.chisq & beta & beta=4 & sigma=2 & n=200 & 7.71 \\ 
  185 & MDE.Phi.tv & beta & beta=4 & sigma=2 & n=200 & 6.95 \\ 
  186 & MDE.Phi.kl & beta & beta=4 & sigma=2 & n=200 & 5.26 \\ 
  187 & MME & beta & beta=4 & sigma=2 & n=200 & 6.64 \\ 
  188 & MME.b & beta & beta=4 & sigma=2 & n=200 & 13.69 \\ 
  189 & PWM & beta & beta=4 & sigma=2 & n=200 & 4.91 \\ 
  190 & MLE & sigma & beta=4 & sigma=2 & n=200 & 2.98 \\ 
  191 & MLE.b & sigma & beta=4 & sigma=2 & n=200 & 2.56 \\ 
  192 & LME & sigma & beta=4 & sigma=2 & n=200 & 2.55 \\ 
  193 & MDE.Phi.chisq & sigma & beta=4 & sigma=2 & n=200 & 6.00 \\ 
  194 & MDE.Phi.tv & sigma & beta=4 & sigma=2 & n=200 & 5.13 \\ 
  195 & MDE.Phi.kl & sigma & beta=4 & sigma=2 & n=200 & 2.77 \\ 
  196 & MME & sigma & beta=4 & sigma=2 & n=200 & 3.66 \\ 
  197 & MME.b & sigma & beta=4 & sigma=2 & n=200 & 8.25 \\ 
  198 & PWM & sigma & beta=4 & sigma=2 & n=200 & 2.55 \\ 
  199 & MLE & beta & beta=5 & sigma=2 & n=200 & 9.92 \\ 
  200 & MLE.b & beta & beta=5 & sigma=2 & n=200 & 9.21 \\ 
  201 & LME & beta & beta=5 & sigma=2 & n=200 & 6.78 \\ 
  202 & MDE.Phi.chisq & beta & beta=5 & sigma=2 & n=200 & 14.13 \\ 
  203 & MDE.Phi.tv & beta & beta=5 & sigma=2 & n=200 & 11.36 \\ 
  204 & MDE.Phi.kl & beta & beta=5 & sigma=2 & n=200 & 7.60 \\ 
  205 & MME & beta & beta=5 & sigma=2 & n=200 & 9.76 \\ 
  206 & MME.b & beta & beta=5 & sigma=2 & n=200 & 21.59 \\ 
  207 & PWM & beta & beta=5 & sigma=2 & n=200 & 6.78 \\ 
  208 & MLE & sigma & beta=5 & sigma=2 & n=200 & 4.38 \\ 
  209 & MLE.b & sigma & beta=5 & sigma=2 & n=200 & 4.04 \\ 
  210 & LME & sigma & beta=5 & sigma=2 & n=200 & 2.83 \\ 
  211 & MDE.Phi.chisq & sigma & beta=5 & sigma=2 & n=200 & 8.54 \\ 
  212 & MDE.Phi.tv & sigma & beta=5 & sigma=2 & n=200 & 6.51 \\ 
  213 & MDE.Phi.kl & sigma & beta=5 & sigma=2 & n=200 & 3.23 \\ 
  214 & MME & sigma & beta=5 & sigma=2 & n=200 & 4.27 \\ 
  215 & MME.b & sigma & beta=5 & sigma=2 & n=200 & 9.87 \\ 
  216 & PWM & sigma & beta=5 & sigma=2 & n=200 & 2.83 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220101/Output.mse.LaTeX.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Mon Jan 31 17:32:24 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=2 & n=100 & 0.46 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=2 & n=100 & 0.32 \\ 
  3 & LME & beta & beta=1.5 & sigma=2 & n=100 & 0.40 \\ 
  4 & MDE.Phi.chisq & beta & beta=1.5 & sigma=2 & n=100 & 99.21 \\ 
  5 & MDE.Phi.tv & beta & beta=1.5 & sigma=2 & n=100 & 6.84 \\ 
  6 & MDE.Phi.kl & beta & beta=1.5 & sigma=2 & n=100 & 0.46 \\ 
  7 & MME & beta & beta=1.5 & sigma=2 & n=100 & 2.57 \\ 
  8 & MME.b & beta & beta=1.5 & sigma=2 & n=100 & 130057.25 \\ 
  9 & PWM & beta & beta=1.5 & sigma=2 & n=100 & 0.40 \\ 
  10 & MLE & sigma & beta=1.5 & sigma=2 & n=100 & 2.09 \\ 
  11 & MLE.b & sigma & beta=1.5 & sigma=2 & n=100 & 1.45 \\ 
  12 & LME & sigma & beta=1.5 & sigma=2 & n=100 & 1.75 \\ 
  13 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=2 & n=100 & 83.70 \\ 
  14 & MDE.Phi.tv & sigma & beta=1.5 & sigma=2 & n=100 & 73.46 \\ 
  15 & MDE.Phi.kl & sigma & beta=1.5 & sigma=2 & n=100 & 2.09 \\ 
  16 & MME & sigma & beta=1.5 & sigma=2 & n=100 & 26.50 \\ 
  17 & MME.b & sigma & beta=1.5 & sigma=2 & n=100 & 595640.92 \\ 
  18 & PWM & sigma & beta=1.5 & sigma=2 & n=100 & 1.75 \\ 
  19 & MLE & beta & beta=2 & sigma=2 & n=100 & 66.35 \\ 
  20 & MLE.b & beta & beta=2 & sigma=2 & n=100 & 66.09 \\ 
  21 & LME & beta & beta=2 & sigma=2 & n=100 & 3.31 \\ 
  22 & MDE.Phi.chisq & beta & beta=2 & sigma=2 & n=100 & 65.39 \\ 
  23 & MDE.Phi.tv & beta & beta=2 & sigma=2 & n=100 & 87.75 \\ 
  24 & MDE.Phi.kl & beta & beta=2 & sigma=2 & n=100 & 12.40 \\ 
  25 & MME & beta & beta=2 & sigma=2 & n=100 & 55.69 \\ 
  26 & MME.b & beta & beta=2 & sigma=2 & n=100 & 151259.47 \\ 
  27 & PWM & beta & beta=2 & sigma=2 & n=100 & 3.31 \\ 
  28 & MLE & sigma & beta=2 & sigma=2 & n=100 & 94.21 \\ 
  29 & MLE.b & sigma & beta=2 & sigma=2 & n=100 & 93.65 \\ 
  30 & LME & sigma & beta=2 & sigma=2 & n=100 & 6.14 \\ 
  31 & MDE.Phi.chisq & sigma & beta=2 & sigma=2 & n=100 & 303.55 \\ 
  32 & MDE.Phi.tv & sigma & beta=2 & sigma=2 & n=100 & 389.41 \\ 
  33 & MDE.Phi.kl & sigma & beta=2 & sigma=2 & n=100 & 20.86 \\ 
  34 & MME & sigma & beta=2 & sigma=2 & n=100 & 99.67 \\ 
  35 & MME.b & sigma & beta=2 & sigma=2 & n=100 & 334286.83 \\ 
  36 & PWM & sigma & beta=2 & sigma=2 & n=100 & 6.14 \\ 
  37 & MLE & beta & beta=2.5 & sigma=2 & n=100 & 141.34 \\ 
  38 & MLE.b & beta & beta=2.5 & sigma=2 & n=100 & 141.21 \\ 
  39 & LME & beta & beta=2.5 & sigma=2 & n=100 & 8.83 \\ 
  40 & MDE.Phi.chisq & beta & beta=2.5 & sigma=2 & n=100 & 227.13 \\ 
  41 & MDE.Phi.tv & beta & beta=2.5 & sigma=2 & n=100 & 262.47 \\ 
  42 & MDE.Phi.kl & beta & beta=2.5 & sigma=2 & n=100 & 30.65 \\ 
  43 & MME & beta & beta=2.5 & sigma=2 & n=100 & 149.68 \\ 
  44 & MME.b & beta & beta=2.5 & sigma=2 & n=100 & 2235.69 \\ 
  45 & PWM & beta & beta=2.5 & sigma=2 & n=100 & 8.83 \\ 
  46 & MLE & sigma & beta=2.5 & sigma=2 & n=100 & 162.04 \\ 
  47 & MLE.b & sigma & beta=2.5 & sigma=2 & n=100 & 161.86 \\ 
  48 & LME & sigma & beta=2.5 & sigma=2 & n=100 & 9.51 \\ 
  49 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=2 & n=100 & 552.81 \\ 
  50 & MDE.Phi.tv & sigma & beta=2.5 & sigma=2 & n=100 & 638.28 \\ 
  51 & MDE.Phi.kl & sigma & beta=2.5 & sigma=2 & n=100 & 33.59 \\ 
  52 & MME & sigma & beta=2.5 & sigma=2 & n=100 & 157.46 \\ 
  53 & MME.b & sigma & beta=2.5 & sigma=2 & n=100 & 2556.57 \\ 
  54 & PWM & sigma & beta=2.5 & sigma=2 & n=100 & 9.51 \\ 
  55 & MLE & beta & beta=3 & sigma=2 & n=100 & 880.32 \\ 
  56 & MLE.b & beta & beta=3 & sigma=2 & n=100 & 880.53 \\ 
  57 & LME & beta & beta=3 & sigma=2 & n=100 & 17.02 \\ 
  58 & MDE.Phi.chisq & beta & beta=3 & sigma=2 & n=100 & 495.41 \\ 
  59 & MDE.Phi.tv & beta & beta=3 & sigma=2 & n=100 & 603.10 \\ 
  60 & MDE.Phi.kl & beta & beta=3 & sigma=2 & n=100 & 104.31 \\ 
  61 & MME & beta & beta=3 & sigma=2 & n=100 & 313324.91 \\ 
  62 & MME.b & beta & beta=3 & sigma=2 & n=100 & 2979286.01 \\ 
  63 & PWM & beta & beta=3 & sigma=2 & n=100 & 17.02 \\ 
  64 & MLE & sigma & beta=3 & sigma=2 & n=100 & 679.39 \\ 
  65 & MLE.b & sigma & beta=3 & sigma=2 & n=100 & 679.50 \\ 
  66 & LME & sigma & beta=3 & sigma=2 & n=100 & 13.06 \\ 
  67 & MDE.Phi.chisq & sigma & beta=3 & sigma=2 & n=100 & 798.08 \\ 
  68 & MDE.Phi.tv & sigma & beta=3 & sigma=2 & n=100 & 945.72 \\ 
  69 & MDE.Phi.kl & sigma & beta=3 & sigma=2 & n=100 & 77.69 \\ 
  70 & MME & sigma & beta=3 & sigma=2 & n=100 & 180960.13 \\ 
  71 & MME.b & sigma & beta=3 & sigma=2 & n=100 & 1722592.02 \\ 
  72 & PWM & sigma & beta=3 & sigma=2 & n=100 & 13.06 \\ 
  73 & MLE & beta & beta=4 & sigma=2 & n=100 & 1547.59 \\ 
  74 & MLE.b & beta & beta=4 & sigma=2 & n=100 & 1548.52 \\ 
  75 & LME & beta & beta=4 & sigma=2 & n=100 & 51.86 \\ 
  76 & MDE.Phi.chisq & beta & beta=4 & sigma=2 & n=100 & 1290.28 \\ 
  77 & MDE.Phi.tv & beta & beta=4 & sigma=2 & n=100 & 1511.41 \\ 
  78 & MDE.Phi.kl & beta & beta=4 & sigma=2 & n=100 & 212.98 \\ 
  79 & MME & beta & beta=4 & sigma=2 & n=100 & 11609.86 \\ 
  80 & MME.b & beta & beta=4 & sigma=2 & n=100 & 1922332.72 \\ 
  81 & PWM & beta & beta=4 & sigma=2 & n=100 & 51.86 \\ 
  82 & MLE & sigma & beta=4 & sigma=2 & n=100 & 583.43 \\ 
  83 & MLE.b & sigma & beta=4 & sigma=2 & n=100 & 583.75 \\ 
  84 & LME & sigma & beta=4 & sigma=2 & n=100 & 19.90 \\ 
  85 & MDE.Phi.chisq & sigma & beta=4 & sigma=2 & n=100 & 1023.38 \\ 
  86 & MDE.Phi.tv & sigma & beta=4 & sigma=2 & n=100 & 1134.64 \\ 
  87 & MDE.Phi.kl & sigma & beta=4 & sigma=2 & n=100 & 84.10 \\ 
  88 & MME & sigma & beta=4 & sigma=2 & n=100 & 4367.52 \\ 
  89 & MME.b & sigma & beta=4 & sigma=2 & n=100 & 1082722.33 \\ 
  90 & PWM & sigma & beta=4 & sigma=2 & n=100 & 19.90 \\ 
  91 & MLE & beta & beta=5 & sigma=2 & n=100 & 2747.14 \\ 
  92 & MLE.b & beta & beta=5 & sigma=2 & n=100 & 2748.57 \\ 
  93 & LME & beta & beta=5 & sigma=2 & n=100 & 101.66 \\ 
  94 & MDE.Phi.chisq & beta & beta=5 & sigma=2 & n=100 & 2092.13 \\ 
  95 & MDE.Phi.tv & beta & beta=5 & sigma=2 & n=100 & 2301.36 \\ 
  96 & MDE.Phi.kl & beta & beta=5 & sigma=2 & n=100 & 372.90 \\ 
  97 & MME & beta & beta=5 & sigma=2 & n=100 & 18723.49 \\ 
  98 & MME.b & beta & beta=5 & sigma=2 & n=100 & 259591.79 \\ 
  99 & PWM & beta & beta=5 & sigma=2 & n=100 & 101.66 \\ 
  100 & MLE & sigma & beta=5 & sigma=2 & n=100 & 617.23 \\ 
  101 & MLE.b & sigma & beta=5 & sigma=2 & n=100 & 617.53 \\ 
  102 & LME & sigma & beta=5 & sigma=2 & n=100 & 22.47 \\ 
  103 & MDE.Phi.chisq & sigma & beta=5 & sigma=2 & n=100 & 957.78 \\ 
  104 & MDE.Phi.tv & sigma & beta=5 & sigma=2 & n=100 & 1007.91 \\ 
  105 & MDE.Phi.kl & sigma & beta=5 & sigma=2 & n=100 & 82.63 \\ 
  106 & MME & sigma & beta=5 & sigma=2 & n=100 & 4176.97 \\ 
  107 & MME.b & sigma & beta=5 & sigma=2 & n=100 & 62177.40 \\ 
  108 & PWM & sigma & beta=5 & sigma=2 & n=100 & 22.47 \\ 
  109 & MLE & beta & beta=1.5 & sigma=2 & n=200 & 0.16 \\ 
  110 & MLE.b & beta & beta=1.5 & sigma=2 & n=200 & 0.09 \\ 
  111 & LME & beta & beta=1.5 & sigma=2 & n=200 & 0.15 \\ 
  112 & MDE.Phi.chisq & beta & beta=1.5 & sigma=2 & n=200 & 23.55 \\ 
  113 & MDE.Phi.tv & beta & beta=1.5 & sigma=2 & n=200 & 0.42 \\ 
  114 & MDE.Phi.kl & beta & beta=1.5 & sigma=2 & n=200 & 0.11 \\ 
  115 & MME & beta & beta=1.5 & sigma=2 & n=200 & 1.15 \\ 
  116 & MME.b & beta & beta=1.5 & sigma=2 & n=200 & 0.89 \\ 
  117 & PWM & beta & beta=1.5 & sigma=2 & n=200 & 0.15 \\ 
  118 & MLE & sigma & beta=1.5 & sigma=2 & n=200 & 0.68 \\ 
  119 & MLE.b & sigma & beta=1.5 & sigma=2 & n=200 & 0.40 \\ 
  120 & LME & sigma & beta=1.5 & sigma=2 & n=200 & 0.66 \\ 
  121 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=2 & n=200 & 3.42 \\ 
  122 & MDE.Phi.tv & sigma & beta=1.5 & sigma=2 & n=200 & 1.42 \\ 
  123 & MDE.Phi.kl & sigma & beta=1.5 & sigma=2 & n=200 & 0.46 \\ 
  124 & MME & sigma & beta=1.5 & sigma=2 & n=200 & 18.82 \\ 
  125 & MME.b & sigma & beta=1.5 & sigma=2 & n=200 & 15.56 \\ 
  126 & PWM & sigma & beta=1.5 & sigma=2 & n=200 & 0.66 \\ 
  127 & MLE & beta & beta=2 & sigma=2 & n=200 & 0.37 \\ 
  128 & MLE.b & beta & beta=2 & sigma=2 & n=200 & 0.20 \\ 
  129 & LME & beta & beta=2 & sigma=2 & n=200 & 0.35 \\ 
  130 & MDE.Phi.chisq & beta & beta=2 & sigma=2 & n=200 & 2.62 \\ 
  131 & MDE.Phi.tv & beta & beta=2 & sigma=2 & n=200 & 2.40 \\ 
  132 & MDE.Phi.kl & beta & beta=2 & sigma=2 & n=200 & 0.32 \\ 
  133 & MME & beta & beta=2 & sigma=2 & n=200 & 1.48 \\ 
  134 & MME.b & beta & beta=2 & sigma=2 & n=200 & 5.87 \\ 
  135 & PWM & beta & beta=2 & sigma=2 & n=200 & 0.35 \\ 
  136 & MLE & sigma & beta=2 & sigma=2 & n=200 & 0.73 \\ 
  137 & MLE.b & sigma & beta=2 & sigma=2 & n=200 & 0.40 \\ 
  138 & LME & sigma & beta=2 & sigma=2 & n=200 & 0.68 \\ 
  139 & MDE.Phi.chisq & sigma & beta=2 & sigma=2 & n=200 & 7.26 \\ 
  140 & MDE.Phi.tv & sigma & beta=2 & sigma=2 & n=200 & 9.45 \\ 
  141 & MDE.Phi.kl & sigma & beta=2 & sigma=2 & n=200 & 0.63 \\ 
  142 & MME & sigma & beta=2 & sigma=2 & n=200 & 4.27 \\ 
  143 & MME.b & sigma & beta=2 & sigma=2 & n=200 & 11.87 \\ 
  144 & PWM & sigma & beta=2 & sigma=2 & n=200 & 0.68 \\ 
  145 & MLE & beta & beta=2.5 & sigma=2 & n=200 & 1.52 \\ 
  146 & MLE.b & beta & beta=2.5 & sigma=2 & n=200 & 1.13 \\ 
  147 & LME & beta & beta=2.5 & sigma=2 & n=200 & 1.28 \\ 
  148 & MDE.Phi.chisq & beta & beta=2.5 & sigma=2 & n=200 & 18.08 \\ 
  149 & MDE.Phi.tv & beta & beta=2.5 & sigma=2 & n=200 & 13.86 \\ 
  150 & MDE.Phi.kl & beta & beta=2.5 & sigma=2 & n=200 & 1.18 \\ 
  151 & MME & beta & beta=2.5 & sigma=2 & n=200 & 2.90 \\ 
  152 & MME.b & beta & beta=2.5 & sigma=2 & n=200 & 44.44 \\ 
  153 & PWM & beta & beta=2.5 & sigma=2 & n=200 & 1.28 \\ 
  154 & MLE & sigma & beta=2.5 & sigma=2 & n=200 & 1.79 \\ 
  155 & MLE.b & sigma & beta=2.5 & sigma=2 & n=200 & 1.32 \\ 
  156 & LME & sigma & beta=2.5 & sigma=2 & n=200 & 1.45 \\ 
  157 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=2 & n=200 & 36.59 \\ 
  158 & MDE.Phi.tv & sigma & beta=2.5 & sigma=2 & n=200 & 27.27 \\ 
  159 & MDE.Phi.kl & sigma & beta=2.5 & sigma=2 & n=200 & 1.40 \\ 
  160 & MME & sigma & beta=2.5 & sigma=2 & n=200 & 3.84 \\ 
  161 & MME.b & sigma & beta=2.5 & sigma=2 & n=200 & 50.28 \\ 
  162 & PWM & sigma & beta=2.5 & sigma=2 & n=200 & 1.45 \\ 
  163 & MLE & beta & beta=3 & sigma=2 & n=200 & 176.07 \\ 
  164 & MLE.b & beta & beta=3 & sigma=2 & n=200 & 175.46 \\ 
  165 & LME & beta & beta=3 & sigma=2 & n=200 & 4.35 \\ 
  166 & MDE.Phi.chisq & beta & beta=3 & sigma=2 & n=200 & 89.09 \\ 
  167 & MDE.Phi.tv & beta & beta=3 & sigma=2 & n=200 & 42.73 \\ 
  168 & MDE.Phi.kl & beta & beta=3 & sigma=2 & n=200 & 7.97 \\ 
  169 & MME & beta & beta=3 & sigma=2 & n=200 & 74.99 \\ 
  170 & MME.b & beta & beta=3 & sigma=2 & n=200 & 7353.37 \\ 
  171 & PWM & beta & beta=3 & sigma=2 & n=200 & 4.35 \\ 
  172 & MLE & sigma & beta=3 & sigma=2 & n=200 & 117.01 \\ 
  173 & MLE.b & sigma & beta=3 & sigma=2 & n=200 & 116.53 \\ 
  174 & LME & sigma & beta=3 & sigma=2 & n=200 & 3.12 \\ 
  175 & MDE.Phi.chisq & sigma & beta=3 & sigma=2 & n=200 & 119.51 \\ 
  176 & MDE.Phi.tv & sigma & beta=3 & sigma=2 & n=200 & 53.42 \\ 
  177 & MDE.Phi.kl & sigma & beta=3 & sigma=2 & n=200 & 5.68 \\ 
  178 & MME & sigma & beta=3 & sigma=2 & n=200 & 49.12 \\ 
  179 & MME.b & sigma & beta=3 & sigma=2 & n=200 & 6731.37 \\ 
  180 & PWM & sigma & beta=3 & sigma=2 & n=200 & 3.12 \\ 
  181 & MLE & beta & beta=4 & sigma=2 & n=200 & 161.27 \\ 
  182 & MLE.b & beta & beta=4 & sigma=2 & n=200 & 161.05 \\ 
  183 & LME & beta & beta=4 & sigma=2 & n=200 & 18.28 \\ 
  184 & MDE.Phi.chisq & beta & beta=4 & sigma=2 & n=200 & 478.77 \\ 
  185 & MDE.Phi.tv & beta & beta=4 & sigma=2 & n=200 & 354.77 \\ 
  186 & MDE.Phi.kl & beta & beta=4 & sigma=2 & n=200 & 42.82 \\ 
  187 & MME & beta & beta=4 & sigma=2 & n=200 & 550.99 \\ 
  188 & MME.b & beta & beta=4 & sigma=2 & n=200 & 40296.90 \\ 
  189 & PWM & beta & beta=4 & sigma=2 & n=200 & 18.28 \\ 
  190 & MLE & sigma & beta=4 & sigma=2 & n=200 & 63.60 \\ 
  191 & MLE.b & sigma & beta=4 & sigma=2 & n=200 & 63.50 \\ 
  192 & LME & sigma & beta=4 & sigma=2 & n=200 & 6.86 \\ 
  193 & MDE.Phi.chisq & sigma & beta=4 & sigma=2 & n=200 & 319.57 \\ 
  194 & MDE.Phi.tv & sigma & beta=4 & sigma=2 & n=200 & 229.78 \\ 
  195 & MDE.Phi.kl & sigma & beta=4 & sigma=2 & n=200 & 16.19 \\ 
  196 & MME & sigma & beta=4 & sigma=2 & n=200 & 213.66 \\ 
  197 & MME.b & sigma & beta=4 & sigma=2 & n=200 & 19808.00 \\ 
  198 & PWM & sigma & beta=4 & sigma=2 & n=200 & 6.86 \\ 
  199 & MLE & beta & beta=5 & sigma=2 & n=200 & 10597.50 \\ 
  200 & MLE.b & beta & beta=5 & sigma=2 & n=200 & 10598.33 \\ 
  201 & LME & beta & beta=5 & sigma=2 & n=200 & 66.24 \\ 
  202 & MDE.Phi.chisq & beta & beta=5 & sigma=2 & n=200 & 1220.28 \\ 
  203 & MDE.Phi.tv & beta & beta=5 & sigma=2 & n=200 & 806.89 \\ 
  204 & MDE.Phi.kl & beta & beta=5 & sigma=2 & n=200 & 141.62 \\ 
  205 & MME & beta & beta=5 & sigma=2 & n=200 & 2746.13 \\ 
  206 & MME.b & beta & beta=5 & sigma=2 & n=200 & 30984.95 \\ 
  207 & PWM & beta & beta=5 & sigma=2 & n=200 & 66.24 \\ 
  208 & MLE & sigma & beta=5 & sigma=2 & n=200 & 2451.72 \\ 
  209 & MLE.b & sigma & beta=5 & sigma=2 & n=200 & 2451.89 \\ 
  210 & LME & sigma & beta=5 & sigma=2 & n=200 & 14.82 \\ 
  211 & MDE.Phi.chisq & sigma & beta=5 & sigma=2 & n=200 & 478.48 \\ 
  212 & MDE.Phi.tv & sigma & beta=5 & sigma=2 & n=200 & 299.43 \\ 
  213 & MDE.Phi.kl & sigma & beta=5 & sigma=2 & n=200 & 31.59 \\ 
  214 & MME & sigma & beta=5 & sigma=2 & n=200 & 597.26 \\ 
  215 & MME.b & sigma & beta=5 & sigma=2 & n=200 & 7010.66 \\ 
  216 & PWM & sigma & beta=5 & sigma=2 & n=200 & 14.82 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220101/Output.var.LaTeX.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Mon Jan 31 17:32:24 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=2 & n=100 & 0.44 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=2 & n=100 & 0.32 \\ 
  3 & LME & beta & beta=1.5 & sigma=2 & n=100 & 0.30 \\ 
  4 & MDE.Phi.chisq & beta & beta=1.5 & sigma=2 & n=100 & 97.61 \\ 
  5 & MDE.Phi.tv & beta & beta=1.5 & sigma=2 & n=100 & 6.78 \\ 
  6 & MDE.Phi.kl & beta & beta=1.5 & sigma=2 & n=100 & 0.44 \\ 
  7 & MME & beta & beta=1.5 & sigma=2 & n=100 & 0.90 \\ 
  8 & MME.b & beta & beta=1.5 & sigma=2 & n=100 & 130047.07 \\ 
  9 & PWM & beta & beta=1.5 & sigma=2 & n=100 & 0.30 \\ 
  10 & MLE & sigma & beta=1.5 & sigma=2 & n=100 & 1.96 \\ 
  11 & MLE.b & sigma & beta=1.5 & sigma=2 & n=100 & 1.45 \\ 
  12 & LME & sigma & beta=1.5 & sigma=2 & n=100 & 1.33 \\ 
  13 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=2 & n=100 & 82.05 \\ 
  14 & MDE.Phi.tv & sigma & beta=1.5 & sigma=2 & n=100 & 70.77 \\ 
  15 & MDE.Phi.kl & sigma & beta=1.5 & sigma=2 & n=100 & 1.96 \\ 
  16 & MME & sigma & beta=1.5 & sigma=2 & n=100 & 7.97 \\ 
  17 & MME.b & sigma & beta=1.5 & sigma=2 & n=100 & 595564.32 \\ 
  18 & PWM & sigma & beta=1.5 & sigma=2 & n=100 & 1.33 \\ 
  19 & MLE & beta & beta=2 & sigma=2 & n=100 & 66.06 \\ 
  20 & MLE.b & beta & beta=2 & sigma=2 & n=100 & 66.06 \\ 
  21 & LME & beta & beta=2 & sigma=2 & n=100 & 3.11 \\ 
  22 & MDE.Phi.chisq & beta & beta=2 & sigma=2 & n=100 & 65.39 \\ 
  23 & MDE.Phi.tv & beta & beta=2 & sigma=2 & n=100 & 87.28 \\ 
  24 & MDE.Phi.kl & beta & beta=2 & sigma=2 & n=100 & 12.19 \\ 
  25 & MME & beta & beta=2 & sigma=2 & n=100 & 52.88 \\ 
  26 & MME.b & beta & beta=2 & sigma=2 & n=100 & 151218.71 \\ 
  27 & PWM & beta & beta=2 & sigma=2 & n=100 & 3.11 \\ 
  28 & MLE & sigma & beta=2 & sigma=2 & n=100 & 93.66 \\ 
  29 & MLE.b & sigma & beta=2 & sigma=2 & n=100 & 93.60 \\ 
  30 & LME & sigma & beta=2 & sigma=2 & n=100 & 5.78 \\ 
  31 & MDE.Phi.chisq & sigma & beta=2 & sigma=2 & n=100 & 298.76 \\ 
  32 & MDE.Phi.tv & sigma & beta=2 & sigma=2 & n=100 & 379.09 \\ 
  33 & MDE.Phi.kl & sigma & beta=2 & sigma=2 & n=100 & 20.44 \\ 
  34 & MME & sigma & beta=2 & sigma=2 & n=100 & 91.42 \\ 
  35 & MME.b & sigma & beta=2 & sigma=2 & n=100 & 334195.41 \\ 
  36 & PWM & sigma & beta=2 & sigma=2 & n=100 & 5.78 \\ 
  37 & MLE & beta & beta=2.5 & sigma=2 & n=100 & 140.17 \\ 
  38 & MLE.b & beta & beta=2.5 & sigma=2 & n=100 & 140.83 \\ 
  39 & LME & beta & beta=2.5 & sigma=2 & n=100 & 8.34 \\ 
  40 & MDE.Phi.chisq & beta & beta=2.5 & sigma=2 & n=100 & 224.57 \\ 
  41 & MDE.Phi.tv & beta & beta=2.5 & sigma=2 & n=100 & 256.61 \\ 
  42 & MDE.Phi.kl & beta & beta=2.5 & sigma=2 & n=100 & 29.78 \\ 
  43 & MME & beta & beta=2.5 & sigma=2 & n=100 & 144.30 \\ 
  44 & MME.b & beta & beta=2.5 & sigma=2 & n=100 & 2205.73 \\ 
  45 & PWM & beta & beta=2.5 & sigma=2 & n=100 & 8.34 \\ 
  46 & MLE & sigma & beta=2.5 & sigma=2 & n=100 & 160.69 \\ 
  47 & MLE.b & sigma & beta=2.5 & sigma=2 & n=100 & 161.42 \\ 
  48 & LME & sigma & beta=2.5 & sigma=2 & n=100 & 8.99 \\ 
  49 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=2 & n=100 & 535.71 \\ 
  50 & MDE.Phi.tv & sigma & beta=2.5 & sigma=2 & n=100 & 611.37 \\ 
  51 & MDE.Phi.kl & sigma & beta=2.5 & sigma=2 & n=100 & 32.58 \\ 
  52 & MME & sigma & beta=2.5 & sigma=2 & n=100 & 150.14 \\ 
  53 & MME.b & sigma & beta=2.5 & sigma=2 & n=100 & 2520.30 \\ 
  54 & PWM & sigma & beta=2.5 & sigma=2 & n=100 & 8.99 \\ 
  55 & MLE & beta & beta=3 & sigma=2 & n=100 & 872.85 \\ 
  56 & MLE.b & beta & beta=3 & sigma=2 & n=100 & 875.53 \\ 
  57 & LME & beta & beta=3 & sigma=2 & n=100 & 15.99 \\ 
  58 & MDE.Phi.chisq & beta & beta=3 & sigma=2 & n=100 & 480.90 \\ 
  59 & MDE.Phi.tv & beta & beta=3 & sigma=2 & n=100 & 575.77 \\ 
  60 & MDE.Phi.kl & beta & beta=3 & sigma=2 & n=100 & 100.86 \\ 
  61 & MME & beta & beta=3 & sigma=2 & n=100 & 313146.34 \\ 
  62 & MME.b & beta & beta=3 & sigma=2 & n=100 & 2977375.72 \\ 
  63 & PWM & beta & beta=3 & sigma=2 & n=100 & 15.99 \\ 
  64 & MLE & sigma & beta=3 & sigma=2 & n=100 & 673.84 \\ 
  65 & MLE.b & sigma & beta=3 & sigma=2 & n=100 & 675.79 \\ 
  66 & LME & sigma & beta=3 & sigma=2 & n=100 & 12.33 \\ 
  67 & MDE.Phi.chisq & sigma & beta=3 & sigma=2 & n=100 & 759.10 \\ 
  68 & MDE.Phi.tv & sigma & beta=3 & sigma=2 & n=100 & 886.52 \\ 
  69 & MDE.Phi.kl & sigma & beta=3 & sigma=2 & n=100 & 75.13 \\ 
  70 & MME & sigma & beta=3 & sigma=2 & n=100 & 180846.34 \\ 
  71 & MME.b & sigma & beta=3 & sigma=2 & n=100 & 1721384.96 \\ 
  72 & PWM & sigma & beta=3 & sigma=2 & n=100 & 12.33 \\ 
  73 & MLE & beta & beta=4 & sigma=2 & n=100 & 1525.38 \\ 
  74 & MLE.b & beta & beta=4 & sigma=2 & n=100 & 1530.36 \\ 
  75 & LME & beta & beta=4 & sigma=2 & n=100 & 48.77 \\ 
  76 & MDE.Phi.chisq & beta & beta=4 & sigma=2 & n=100 & 1195.04 \\ 
  77 & MDE.Phi.tv & beta & beta=4 & sigma=2 & n=100 & 1368.63 \\ 
  78 & MDE.Phi.kl & beta & beta=4 & sigma=2 & n=100 & 201.29 \\ 
  79 & MME & beta & beta=4 & sigma=2 & n=100 & 11556.91 \\ 
  80 & MME.b & beta & beta=4 & sigma=2 & n=100 & 1921162.31 \\ 
  81 & PWM & beta & beta=4 & sigma=2 & n=100 & 48.77 \\ 
  82 & MLE & sigma & beta=4 & sigma=2 & n=100 & 574.92 \\ 
  83 & MLE.b & sigma & beta=4 & sigma=2 & n=100 & 576.76 \\ 
  84 & LME & sigma & beta=4 & sigma=2 & n=100 & 18.76 \\ 
  85 & MDE.Phi.chisq & sigma & beta=4 & sigma=2 & n=100 & 926.76 \\ 
  86 & MDE.Phi.tv & sigma & beta=4 & sigma=2 & n=100 & 1007.89 \\ 
  87 & MDE.Phi.kl & sigma & beta=4 & sigma=2 & n=100 & 79.61 \\ 
  88 & MME & sigma & beta=4 & sigma=2 & n=100 & 4346.18 \\ 
  89 & MME.b & sigma & beta=4 & sigma=2 & n=100 & 1082212.14 \\ 
  90 & PWM & sigma & beta=4 & sigma=2 & n=100 & 18.76 \\ 
  91 & MLE & beta & beta=5 & sigma=2 & n=100 & 2693.78 \\ 
  92 & MLE.b & beta & beta=5 & sigma=2 & n=100 & 2700.47 \\ 
  93 & LME & beta & beta=5 & sigma=2 & n=100 & 96.10 \\ 
  94 & MDE.Phi.chisq & beta & beta=5 & sigma=2 & n=100 & 1864.51 \\ 
  95 & MDE.Phi.tv & beta & beta=5 & sigma=2 & n=100 & 2004.22 \\ 
  96 & MDE.Phi.kl & beta & beta=5 & sigma=2 & n=100 & 347.29 \\ 
  97 & MME & beta & beta=5 & sigma=2 & n=100 & 18587.85 \\ 
  98 & MME.b & beta & beta=5 & sigma=2 & n=100 & 257840.15 \\ 
  99 & PWM & beta & beta=5 & sigma=2 & n=100 & 96.10 \\ 
  100 & MLE & sigma & beta=5 & sigma=2 & n=100 & 605.40 \\ 
  101 & MLE.b & sigma & beta=5 & sigma=2 & n=100 & 606.86 \\ 
  102 & LME & sigma & beta=5 & sigma=2 & n=100 & 21.26 \\ 
  103 & MDE.Phi.chisq & sigma & beta=5 & sigma=2 & n=100 & 832.80 \\ 
  104 & MDE.Phi.tv & sigma & beta=5 & sigma=2 & n=100 & 860.14 \\ 
  105 & MDE.Phi.kl & sigma & beta=5 & sigma=2 & n=100 & 76.96 \\ 
  106 & MME & sigma & beta=5 & sigma=2 & n=100 & 4147.18 \\ 
  107 & MME.b & sigma & beta=5 & sigma=2 & n=100 & 61786.34 \\ 
  108 & PWM & sigma & beta=5 & sigma=2 & n=100 & 21.26 \\ 
  109 & MLE & beta & beta=1.5 & sigma=2 & n=200 & 0.10 \\ 
  110 & MLE.b & beta & beta=1.5 & sigma=2 & n=200 & 0.08 \\ 
  111 & LME & beta & beta=1.5 & sigma=2 & n=200 & 0.11 \\ 
  112 & MDE.Phi.chisq & beta & beta=1.5 & sigma=2 & n=200 & 22.83 \\ 
  113 & MDE.Phi.tv & beta & beta=1.5 & sigma=2 & n=200 & 0.17 \\ 
  114 & MDE.Phi.kl & beta & beta=1.5 & sigma=2 & n=200 & 0.10 \\ 
  115 & MME & beta & beta=1.5 & sigma=2 & n=200 & 0.16 \\ 
  116 & MME.b & beta & beta=1.5 & sigma=2 & n=200 & 0.26 \\ 
  117 & PWM & beta & beta=1.5 & sigma=2 & n=200 & 0.11 \\ 
  118 & MLE & sigma & beta=1.5 & sigma=2 & n=200 & 0.46 \\ 
  119 & MLE.b & sigma & beta=1.5 & sigma=2 & n=200 & 0.33 \\ 
  120 & LME & sigma & beta=1.5 & sigma=2 & n=200 & 0.49 \\ 
  121 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=2 & n=200 & 3.32 \\ 
  122 & MDE.Phi.tv & sigma & beta=1.5 & sigma=2 & n=200 & 1.16 \\ 
  123 & MDE.Phi.kl & sigma & beta=1.5 & sigma=2 & n=200 & 0.43 \\ 
  124 & MME & sigma & beta=1.5 & sigma=2 & n=200 & 6.07 \\ 
  125 & MME.b & sigma & beta=1.5 & sigma=2 & n=200 & 6.44 \\ 
  126 & PWM & sigma & beta=1.5 & sigma=2 & n=200 & 0.49 \\ 
  127 & MLE & beta & beta=2 & sigma=2 & n=200 & 0.31 \\ 
  128 & MLE.b & beta & beta=2 & sigma=2 & n=200 & 0.20 \\ 
  129 & LME & beta & beta=2 & sigma=2 & n=200 & 0.30 \\ 
  130 & MDE.Phi.chisq & beta & beta=2 & sigma=2 & n=200 & 2.19 \\ 
  131 & MDE.Phi.tv & beta & beta=2 & sigma=2 & n=200 & 2.21 \\ 
  132 & MDE.Phi.kl & beta & beta=2 & sigma=2 & n=200 & 0.30 \\ 
  133 & MME & beta & beta=2 & sigma=2 & n=200 & 0.53 \\ 
  134 & MME.b & beta & beta=2 & sigma=2 & n=200 & 5.40 \\ 
  135 & PWM & beta & beta=2 & sigma=2 & n=200 & 0.30 \\ 
  136 & MLE & sigma & beta=2 & sigma=2 & n=200 & 0.61 \\ 
  137 & MLE.b & sigma & beta=2 & sigma=2 & n=200 & 0.39 \\ 
  138 & LME & sigma & beta=2 & sigma=2 & n=200 & 0.60 \\ 
  139 & MDE.Phi.chisq & sigma & beta=2 & sigma=2 & n=200 & 7.14 \\ 
  140 & MDE.Phi.tv & sigma & beta=2 & sigma=2 & n=200 & 9.14 \\ 
  141 & MDE.Phi.kl & sigma & beta=2 & sigma=2 & n=200 & 0.59 \\ 
  142 & MME & sigma & beta=2 & sigma=2 & n=200 & 1.11 \\ 
  143 & MME.b & sigma & beta=2 & sigma=2 & n=200 & 10.20 \\ 
  144 & PWM & sigma & beta=2 & sigma=2 & n=200 & 0.60 \\ 
  145 & MLE & beta & beta=2.5 & sigma=2 & n=200 & 1.41 \\ 
  146 & MLE.b & beta & beta=2.5 & sigma=2 & n=200 & 1.13 \\ 
  147 & LME & beta & beta=2.5 & sigma=2 & n=200 & 1.20 \\ 
  148 & MDE.Phi.chisq & beta & beta=2.5 & sigma=2 & n=200 & 17.88 \\ 
  149 & MDE.Phi.tv & beta & beta=2.5 & sigma=2 & n=200 & 13.81 \\ 
  150 & MDE.Phi.kl & beta & beta=2.5 & sigma=2 & n=200 & 1.12 \\ 
  151 & MME & beta & beta=2.5 & sigma=2 & n=200 & 1.77 \\ 
  152 & MME.b & beta & beta=2.5 & sigma=2 & n=200 & 43.75 \\ 
  153 & PWM & beta & beta=2.5 & sigma=2 & n=200 & 1.20 \\ 
  154 & MLE & sigma & beta=2.5 & sigma=2 & n=200 & 1.66 \\ 
  155 & MLE.b & sigma & beta=2.5 & sigma=2 & n=200 & 1.32 \\ 
  156 & LME & sigma & beta=2.5 & sigma=2 & n=200 & 1.36 \\ 
  157 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=2 & n=200 & 36.10 \\ 
  158 & MDE.Phi.tv & sigma & beta=2.5 & sigma=2 & n=200 & 26.62 \\ 
  159 & MDE.Phi.kl & sigma & beta=2.5 & sigma=2 & n=200 & 1.33 \\ 
  160 & MME & sigma & beta=2.5 & sigma=2 & n=200 & 2.13 \\ 
  161 & MME.b & sigma & beta=2.5 & sigma=2 & n=200 & 49.26 \\ 
  162 & PWM & sigma & beta=2.5 & sigma=2 & n=200 & 1.36 \\ 
  163 & MLE & beta & beta=3 & sigma=2 & n=200 & 175.57 \\ 
  164 & MLE.b & beta & beta=3 & sigma=2 & n=200 & 175.42 \\ 
  165 & LME & beta & beta=3 & sigma=2 & n=200 & 4.14 \\ 
  166 & MDE.Phi.chisq & beta & beta=3 & sigma=2 & n=200 & 89.01 \\ 
  167 & MDE.Phi.tv & beta & beta=3 & sigma=2 & n=200 & 42.69 \\ 
  168 & MDE.Phi.kl & beta & beta=3 & sigma=2 & n=200 & 7.73 \\ 
  169 & MME & beta & beta=3 & sigma=2 & n=200 & 73.03 \\ 
  170 & MME.b & beta & beta=3 & sigma=2 & n=200 & 7346.85 \\ 
  171 & PWM & beta & beta=3 & sigma=2 & n=200 & 4.14 \\ 
  172 & MLE & sigma & beta=3 & sigma=2 & n=200 & 116.64 \\ 
  173 & MLE.b & sigma & beta=3 & sigma=2 & n=200 & 116.50 \\ 
  174 & LME & sigma & beta=3 & sigma=2 & n=200 & 2.98 \\ 
  175 & MDE.Phi.chisq & sigma & beta=3 & sigma=2 & n=200 & 117.14 \\ 
  176 & MDE.Phi.tv & sigma & beta=3 & sigma=2 & n=200 & 52.01 \\ 
  177 & MDE.Phi.kl & sigma & beta=3 & sigma=2 & n=200 & 5.50 \\ 
  178 & MME & sigma & beta=3 & sigma=2 & n=200 & 47.45 \\ 
  179 & MME.b & sigma & beta=3 & sigma=2 & n=200 & 6725.97 \\ 
  180 & PWM & sigma & beta=3 & sigma=2 & n=200 & 2.98 \\ 
  181 & MLE & beta & beta=4 & sigma=2 & n=200 & 158.85 \\ 
  182 & MLE.b & beta & beta=4 & sigma=2 & n=200 & 160.30 \\ 
  183 & LME & beta & beta=4 & sigma=2 & n=200 & 17.45 \\ 
  184 & MDE.Phi.chisq & beta & beta=4 & sigma=2 & n=200 & 465.08 \\ 
  185 & MDE.Phi.tv & beta & beta=4 & sigma=2 & n=200 & 346.11 \\ 
  186 & MDE.Phi.kl & beta & beta=4 & sigma=2 & n=200 & 41.24 \\ 
  187 & MME & beta & beta=4 & sigma=2 & n=200 & 544.09 \\ 
  188 & MME.b & beta & beta=4 & sigma=2 & n=200 & 40207.12 \\ 
  189 & PWM & beta & beta=4 & sigma=2 & n=200 & 17.45 \\ 
  190 & MLE & sigma & beta=4 & sigma=2 & n=200 & 62.64 \\ 
  191 & MLE.b & sigma & beta=4 & sigma=2 & n=200 & 63.19 \\ 
  192 & LME & sigma & beta=4 & sigma=2 & n=200 & 6.55 \\ 
  193 & MDE.Phi.chisq & sigma & beta=4 & sigma=2 & n=200 & 303.58 \\ 
  194 & MDE.Phi.tv & sigma & beta=4 & sigma=2 & n=200 & 220.00 \\ 
  195 & MDE.Phi.kl & sigma & beta=4 & sigma=2 & n=200 & 15.59 \\ 
  196 & MME & sigma & beta=4 & sigma=2 & n=200 & 210.92 \\ 
  197 & MME.b & sigma & beta=4 & sigma=2 & n=200 & 19770.86 \\ 
  198 & PWM & sigma & beta=4 & sigma=2 & n=200 & 6.55 \\ 
  199 & MLE & beta & beta=5 & sigma=2 & n=200 & 10574.34 \\ 
  200 & MLE.b & beta & beta=5 & sigma=2 & n=200 & 10581.67 \\ 
  201 & LME & beta & beta=5 & sigma=2 & n=200 & 63.08 \\ 
  202 & MDE.Phi.chisq & beta & beta=5 & sigma=2 & n=200 & 1137.09 \\ 
  203 & MDE.Phi.tv & beta & beta=5 & sigma=2 & n=200 & 766.54 \\ 
  204 & MDE.Phi.kl & beta & beta=5 & sigma=2 & n=200 & 134.88 \\ 
  205 & MME & beta & beta=5 & sigma=2 & n=200 & 2723.73 \\ 
  206 & MME.b & beta & beta=5 & sigma=2 & n=200 & 30712.87 \\ 
  207 & PWM & beta & beta=5 & sigma=2 & n=200 & 63.08 \\ 
  208 & MLE & sigma & beta=5 & sigma=2 & n=200 & 2446.31 \\ 
  209 & MLE.b & sigma & beta=5 & sigma=2 & n=200 & 2447.97 \\ 
  210 & LME & sigma & beta=5 & sigma=2 & n=200 & 14.12 \\ 
  211 & MDE.Phi.chisq & sigma & beta=5 & sigma=2 & n=200 & 435.77 \\ 
  212 & MDE.Phi.tv & sigma & beta=5 & sigma=2 & n=200 & 279.11 \\ 
  213 & MDE.Phi.kl & sigma & beta=5 & sigma=2 & n=200 & 30.09 \\ 
  214 & MME & sigma & beta=5 & sigma=2 & n=200 & 592.18 \\ 
  215 & MME.b & sigma & beta=5 & sigma=2 & n=200 & 6949.35 \\ 
  216 & PWM & sigma & beta=5 & sigma=2 & n=200 & 14.12 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220130/Full.beta=1.5.sig=1.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=1.5,  \sigma=1$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.6717&1.4777&1.8288&0.9857&1.2648&1.6717&2.7927&6.3149&1.8288
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.1823&0.9774&1.3253&1.5496&1.8316&1.1823&3.1523&6.8342&1.3253
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.435&0.3212&0.2958&12.6553&8.0717&0.4353&0.8967&130047.0684&0.2958
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.4894&0.3614&0.3325&22.0968&21.1247&0.4898&1.9922&148891.0812&0.3325
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1717&-0.0223&0.3288&-0.5143&-0.2352&0.1717&1.2927&4.8149&0.3288
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.1823&-0.0226&0.3253&0.5496&0.8316&0.1823&2.1523&5.8342&0.3253
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.4644&0.3217&0.4039&12.9186&8.1262&0.4647&2.5677&130057.2466&0.4039
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.5225&0.3619&0.4383&22.3967&21.8141&0.523&6.6245&148910.2298&0.4383
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 0.9869&0.6836&0.8421&35.3154&29.9403&0.9877&9.1922&278967.4765&0.8421\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0011&0.0011&1.81787018350624e+299&0.0349&0.0011&0.0099&7.105&0.0011\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220130/Full.beta=1.5.sig=1.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=1.5,  \sigma=1$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.5766&1.4937&1.7122&0.8567&1.0134&1.5766&2.5071&2.3073&1.7122
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.0785&0.9917&1.2076&1.132&1.2635&1.0785&2.8011&2.5267&1.2076
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1043&0.0777&0.1126&0.1267&0.1695&0.1043&0.1722&0.1907&0.1126
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.1106&0.081&0.1236&0.231&0.2903&0.1106&5.4485&5.5775&0.1236
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.0766&-0.0063&0.2122&-0.6433&-0.4866&0.0766&1.0071&0.8073&0.2122
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.0785&-0.0083&0.2076&0.132&0.2635&0.0785&1.8011&1.5267&0.2076
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1102&0.0777&0.1576&0.5405&0.4062&0.1102&1.1864&0.8424&0.1576
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.1168&0.081&0.1667&0.2484&0.3597&0.1168&8.6918&7.9077&0.1667
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 0.2269&0.1588&0.3243&0.7889&0.7659&0.2269&9.8782&8.7502&0.3243\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 6e-04&6e-04&6e-04&0.034&0.0266&6e-04&0.0086&0.0085&6e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220130/Full.beta=2.5.sig=1.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2.5,  \sigma=1$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 5.7567&5.2994&3.1918&4.3078&5.1481&3.4512&4.8211&8.0228&3.1918
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2.8403&2.5924&1.3573&3.2274&3.7657&1.5105&2.3543&4.0344&1.3573
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 44295.0662&44297.7104&8.1789&278.8002&316.2533&34.0192&144.3014&2214.1451&8.1789
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
15072.875&15073.68&2.2151&166.8839&188.2532&9.3074&37.535&631.6992&2.2151
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 3.2567&2.7994&0.6918&1.8078&2.6481&0.9512&2.3211&5.5228&0.6918
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.8403&1.5924&0.3573&2.2274&2.7657&0.5105&1.3543&3.0344&0.3573
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 44301.2428&44301.1172&8.6567&282.0404&323.2342&34.9206&149.6744&2244.4246&8.6567
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
15074.7543&15074.7085&2.3425&171.8283&195.8837&9.567&39.3654&640.8439&2.3425
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 59375.9971&59375.8257&10.9992&453.8687&519.1179&44.4876&189.0398&2885.2685&10.9992\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0012&0.001&0.0233&0.0178&0.0011&0.0019&8.078&0.001\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220130/Full.beta=2.5.sig=1.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2.5,  \sigma=1$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.7856&2.4766&2.807&2.0901&2.2794&2.7855&3.6075&3.6549&2.807
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.1543&0.9871&1.1572&1.3786&1.4055&1.1543&1.6804&1.6963&1.1572
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 3.3306&3.0431&2.143&19.057&13.9549&3.3099&5.6748&163.6709&2.143
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.0246&0.941&0.5714&9.6961&7.0162&1.0176&1.7356&55.097&0.5714
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.2856&-0.0234&0.307&-0.4099&-0.2206&0.2855&1.1075&1.1549&0.307
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.1543&-0.0129&0.1572&0.3786&0.4055&0.1543&0.6804&0.6963&0.1572
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 3.4118&3.0433&2.2371&19.2231&14.0022&3.3911&6.9008&164.9883&2.2371
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.0483&0.9411&0.5961&9.8384&7.18&1.0413&2.1983&55.5763&0.5961
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 4.4601&3.9844&2.8331&29.0616&21.1821&4.4324&9.0991&220.5646&2.8331\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&5e-04&5e-04&0.0174&0.0121&5e-04&0.0011&0.002&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220130/Full.beta=2.sig=1.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2,  \sigma=1$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.6316&2.282&2.4461&2.1496&2.7678&2.465&3.6774&9.475&2.4461
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.4271&1.1745&1.3016&2.152&2.6838&1.3282&2.4372&6.5864&1.3016
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 218.3272&218.3939&3.1122&79.2503&106.4854&14.1658&52.8832&151218.7148&3.1122
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
73.3693&73.3817&1.445&90.4216&115.3987&5.9178&22.8539&83548.8529&1.445
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.6316&0.282&0.4461&0.1496&0.7678&0.465&1.6774&7.475&0.4461
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.4271&0.1745&0.3016&1.152&1.6838&0.3282&1.4372&5.5864&0.3016
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 218.7043&218.4515&3.3109&79.2647&107.0642&14.3806&55.6916&151259.4683&3.3109
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
73.5444&73.4048&1.5358&91.7396&118.2225&6.0249&24.9173&83571.7064&1.5358
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 292.2487&291.8564&4.8467&171.0044&225.2867&20.4055&80.609&234831.1746&4.8467\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0011&0.0011&0.0291&0.0229&0.0011&0.0035&0.0115&0.0011\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220130/Full.beta=2.sig=1.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2,  \sigma=1$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.154&1.9803&2.2268&1.3459&1.5657&2.154&2.9819&2.648&2.2268
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.1104&0.9856&1.1521&1.173&1.2784&1.1103&1.8999&1.6288&1.1521
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.3415&0.218&0.3166&0.6248&0.9345&0.3415&0.5969&2.219&0.3166
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.1695&0.106&0.1569&0.5256&0.8203&0.1695&0.317&1.6695&0.1569
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.154&-0.0197&0.2268&-0.6541&-0.4343&0.154&0.9819&0.648&0.2268
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.1104&-0.0144&0.1521&0.173&0.2784&0.1103&0.8999&0.6288&0.1521
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.3651&0.2183&0.368&1.0526&1.123&0.3651&1.561&2.6387&0.368
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.1816&0.1062&0.18&0.5554&0.8977&0.1816&1.1268&2.0647&0.18
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 0.5468&0.3245&0.548&1.608&2.0207&0.5468&2.6878&4.7034&0.548\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&5e-04&5e-04&0.0228&0.0166&5e-04&0.0024&0.0497&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220130/Full.beta=3.sig=1.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=3,  \sigma=1$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1592.9725&1592.4782&4.0082&7.2778&8.7513&4.9234&17.4864&49.9815&4.0082
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
672.8421&672.6286&1.4219&4.4085&5.1674&1.828&6.7414&19.5654&1.4219
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 16310704747.4125&16310706319.4279&15.3953&606.1831&720.8912&120.2338&313146.3548&2977375.8337&15.3953
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2958523159.6899&2958523446.6202&2.9443&238.2611&276.9383&22.2601&45211.5864&430346.2319&2.9443
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1589.9725&1589.4782&1.0082&4.2778&5.7513&1.9234&14.4864&46.9815&1.0082
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
671.8421&671.6286&0.4219&3.4085&4.1674&0.828&5.7414&18.5654&0.4219
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 16311601689.3932&16311601689.5964&16.4103&624.4224&753.8967&123.9213&313324.8969&2979285.3536&16.4103
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2958678679.2227&2958678679.2512&3.122&249.8553&294.2778&22.9435&45240.029&430647.8707&3.122
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 19270280368.6159&19270280368.8476&19.5323&874.2777&1048.1745&146.8647&358564.9259&3409933.2242&19.5323\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0012&0.0011&0.02&0.0152&0.0011&0.0014&0.0075&0.0011\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220130/Full.beta=3.sig=1.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=3,  \sigma=1$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 3.4521&2.9913&3.41&3.3012&3.422&3.4533&4.3185&4.8851&3.41
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.1964&0.9969&1.1708&1.7728&1.7212&1.1968&1.6144&1.8414&1.1708
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 4.8745&4.5431&3.284&95.6529&82.4836&5.1023&7.1332&450.369&3.284
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.8734&0.8103&0.5537&32.1104&25.7957&0.9075&1.2995&83.3832&0.5537
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.4521&-0.0087&0.41&0.3012&0.422&0.4533&1.3185&1.8851&0.41
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.1964&-0.0031&0.1708&0.7728&0.7212&0.1968&0.6144&0.8414&0.1708
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 5.0784&4.5427&3.4518&95.7341&82.6534&5.3072&8.8708&453.8775&3.4518
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.9119&0.8102&0.5828&32.7044&26.3133&0.9462&1.6769&84.0829&0.5828
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 5.9902&5.3529&4.0346&128.4385&108.9667&6.2534&10.5477&537.9604&4.0346\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&5e-04&5e-04&0.0144&0.0098&5e-04&8e-04&0.0016&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220130/Full.beta=4.sig=1.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=4,  \sigma=1$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 229.8585&229.4091&5.7242&14.9055&17.2586&7.5161&11.3514&40.8899&5.7242
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
59.821&59.6847&1.5247&6.4158&7.187&2.0912&3.3315&13.4273&1.5247
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 198915101.2076&198915304.942&45.6394&1517.5971&1738.8148&232.1104&11556.9074&1921161.5452&45.6394
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
12510634.9552&12510651.052&4.3999&294.047&319.9595&23.0675&1086.5457&270552.9924&4.3999
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 225.8585&225.4091&1.7242&10.9055&13.2586&3.5161&7.3514&36.8899&1.7242
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
58.821&58.6847&0.5247&5.4158&6.187&1.0912&2.3315&12.4273&0.5247
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 198946221.7609&198946222.6916&48.6076&1636.376&1914.4317&244.45&11609.7948&1922330.2911&48.6076
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
12512843.8024&12512843.8839&4.6747&323.348&358.206&24.256&1091.873&270680.3758&4.6747
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 211459065.5633&211459066.5755&53.2823&1959.724&2272.6377&268.706&12701.6677&2193010.6669&53.2823\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0013&0.001&0.0165&0.0123&0.0011&0.0011&4041.9544&0.001\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220130/Full.beta=4.sig=1.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=4,  \sigma=1$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 29.9628&29.2974&4.8733&8.3265&7.1302&5.4592&7.0074&12.1541&4.8733
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
8.8338&8.6303&1.2607&3.2402&2.6226&1.444&1.9375&3.536&1.2607
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2426885.181&2426919.1254&14.6384&633.8928&422.3235&78.3409&1484.0568&10586.0551&14.6384
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
225985.2196&225988.3487&1.3332&102.3355&65.0229&7.2057&137.8135&1080.7501&1.3332
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 25.9628&25.2974&0.8733&4.3265&3.1302&1.4592&3.0074&8.1541&0.8733
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
7.8338&7.6303&0.2607&2.2402&1.6226&0.444&0.9375&2.536&0.2607
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2427316.5569&2427316.3903&15.3996&652.5484&432.0792&80.4624&1492.953&10651.4859&15.3996
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
226023.9892&226023.9709&1.401&107.3437&67.6492&7.4021&138.6787&1087.0734&1.401
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 2653340.5461&2653340.3612&16.8007&759.8921&499.7284&87.8645&1631.6317&11738.5593&16.8007\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&6e-04&5e-04&0.0112&0.0074&5e-04&6e-04&0.0949&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220130/Full.beta=5.sig=1.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=5,  \sigma=1$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 78.4222&78.0536&7.3162&22.0149&24.3614&10.2619&16.7594&47.2373&7.3162
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
18.7425&18.6568&1.5402&7.2322&7.7679&2.237&3.7554&10.9829&1.5402
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 4837706.5841&4837762.0093&95.9324&2406.7713&2595.1393&410.3083&18595.9439&257872.265&95.9324
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
278312.211&278315.3192&5.3346&268.9002&278.1254&22.5955&1037.1713&15448.0944&5.3346
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 73.4222&73.0536&2.3162&17.0149&19.3614&5.2619&11.7594&42.2373&2.3162
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
17.7425&17.6568&0.5402&6.2322&6.7679&1.237&2.7554&9.9829&0.5402
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 4842613.6277&4842615.0562&101.2875&2696.036&2969.7429&437.9553&18732.3689&259630.4689&101.2875
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
278599.1745&278599.2503&5.6259&307.7135&323.9023&24.1234&1044.66&15546.2079&5.6259
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 5121212.8022&5121214.3065&106.9134&3003.7495&3293.6452&462.0788&19777.0288&275176.6767&106.9134\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.001&0.0012&0.001&0.0145&0.0106&0.001&0.001&5.15620838018139e+29&0.001\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220130/Full.beta=5.sig=1.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=5,  \sigma=1$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 44.5511&43.8299&6.6884&15.4328&12.1353&7.7209&16.1583&39.2158&6.6884
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
10.7557&10.5857&1.3963&4.6777&3.4866&1.6395&3.6591&9.2673&1.3963
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 6973123.3484&6973180.7194&54.4407&1484.5478&974.4175&179.6847&352282.4579&1489135.1637&54.4407
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
441066.8101&441070.144&3.151&142.291&88.1175&9.7893&19950.1074&85211.6663&3.151
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 39.5511&38.8299&1.6884&10.4328&7.1353&2.7209&11.1583&34.2158&1.6884
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
9.7557&9.5857&0.3963&3.6777&2.4866&0.6395&2.6591&8.2673&0.3963
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 6973990.3233&6973991.1662&57.2859&1593.2426&1025.2319&187.07&352371.7369&1490156.9691&57.2859
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
441117.8778&441117.9217&3.3078&155.802&94.2918&10.1973&19955.183&85271.4941&3.3078
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 7415108.2011&7415109.0879&60.5936&1749.0446&1119.5238&197.2672&372326.9199&1575428.4633&60.5936\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&6e-04&5e-04&0.0097&0.0064&5e-04&5e-04&0.4691&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220130/Output.accuracy.LaTeX.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Sun Jan 30 20:11:05 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & Measure & beta=1.5 & sigma=1 & n=100 & 0.99 \\ 
  2 & MLE.b & Measure & beta=1.5 & sigma=1 & n=100 & 0.68 \\ 
  3 & LME & Measure & beta=1.5 & sigma=1 & n=100 & 0.84 \\ 
  4 & MDE.Phi.chisq & Measure & beta=1.5 & sigma=1 & n=100 & 35.32 \\ 
  5 & MDE.Phi.tv & Measure & beta=1.5 & sigma=1 & n=100 & 29.94 \\ 
  6 & MDE.Phi.kl & Measure & beta=1.5 & sigma=1 & n=100 & 0.99 \\ 
  7 & MME & Measure & beta=1.5 & sigma=1 & n=100 & 9.19 \\ 
  8 & MME.b & Measure & beta=1.5 & sigma=1 & n=100 & 278967.48 \\ 
  9 & PWM & Measure & beta=1.5 & sigma=1 & n=100 & 0.84 \\ 
  10 & MLE & Measure & beta=2 & sigma=1 & n=100 & 292.25 \\ 
  11 & MLE.b & Measure & beta=2 & sigma=1 & n=100 & 291.86 \\ 
  12 & LME & Measure & beta=2 & sigma=1 & n=100 & 4.85 \\ 
  13 & MDE.Phi.chisq & Measure & beta=2 & sigma=1 & n=100 & 171.00 \\ 
  14 & MDE.Phi.tv & Measure & beta=2 & sigma=1 & n=100 & 225.29 \\ 
  15 & MDE.Phi.kl & Measure & beta=2 & sigma=1 & n=100 & 20.41 \\ 
  16 & MME & Measure & beta=2 & sigma=1 & n=100 & 80.61 \\ 
  17 & MME.b & Measure & beta=2 & sigma=1 & n=100 & 234831.17 \\ 
  18 & PWM & Measure & beta=2 & sigma=1 & n=100 & 4.85 \\ 
  19 & MLE & Measure & beta=2.5 & sigma=1 & n=100 & 59376.00 \\ 
  20 & MLE.b & Measure & beta=2.5 & sigma=1 & n=100 & 59375.83 \\ 
  21 & LME & Measure & beta=2.5 & sigma=1 & n=100 & 11.00 \\ 
  22 & MDE.Phi.chisq & Measure & beta=2.5 & sigma=1 & n=100 & 453.87 \\ 
  23 & MDE.Phi.tv & Measure & beta=2.5 & sigma=1 & n=100 & 519.12 \\ 
  24 & MDE.Phi.kl & Measure & beta=2.5 & sigma=1 & n=100 & 44.49 \\ 
  25 & MME & Measure & beta=2.5 & sigma=1 & n=100 & 189.04 \\ 
  26 & MME.b & Measure & beta=2.5 & sigma=1 & n=100 & 2885.27 \\ 
  27 & PWM & Measure & beta=2.5 & sigma=1 & n=100 & 11.00 \\ 
  28 & MLE & Measure & beta=3 & sigma=1 & n=100 & 19270280368.62 \\ 
  29 & MLE.b & Measure & beta=3 & sigma=1 & n=100 & 19270280368.85 \\ 
  30 & LME & Measure & beta=3 & sigma=1 & n=100 & 19.53 \\ 
  31 & MDE.Phi.chisq & Measure & beta=3 & sigma=1 & n=100 & 874.28 \\ 
  32 & MDE.Phi.tv & Measure & beta=3 & sigma=1 & n=100 & 1048.17 \\ 
  33 & MDE.Phi.kl & Measure & beta=3 & sigma=1 & n=100 & 146.86 \\ 
  34 & MME & Measure & beta=3 & sigma=1 & n=100 & 358564.93 \\ 
  35 & MME.b & Measure & beta=3 & sigma=1 & n=100 & 3409933.22 \\ 
  36 & PWM & Measure & beta=3 & sigma=1 & n=100 & 19.53 \\ 
  37 & MLE & Measure & beta=4 & sigma=1 & n=100 & 211459065.56 \\ 
  38 & MLE.b & Measure & beta=4 & sigma=1 & n=100 & 211459066.58 \\ 
  39 & LME & Measure & beta=4 & sigma=1 & n=100 & 53.28 \\ 
  40 & MDE.Phi.chisq & Measure & beta=4 & sigma=1 & n=100 & 1959.72 \\ 
  41 & MDE.Phi.tv & Measure & beta=4 & sigma=1 & n=100 & 2272.64 \\ 
  42 & MDE.Phi.kl & Measure & beta=4 & sigma=1 & n=100 & 268.71 \\ 
  43 & MME & Measure & beta=4 & sigma=1 & n=100 & 12701.67 \\ 
  44 & MME.b & Measure & beta=4 & sigma=1 & n=100 & 2193010.67 \\ 
  45 & PWM & Measure & beta=4 & sigma=1 & n=100 & 53.28 \\ 
  46 & MLE & Measure & beta=5 & sigma=1 & n=100 & 5121212.80 \\ 
  47 & MLE.b & Measure & beta=5 & sigma=1 & n=100 & 5121214.31 \\ 
  48 & LME & Measure & beta=5 & sigma=1 & n=100 & 106.91 \\ 
  49 & MDE.Phi.chisq & Measure & beta=5 & sigma=1 & n=100 & 3003.75 \\ 
  50 & MDE.Phi.tv & Measure & beta=5 & sigma=1 & n=100 & 3293.65 \\ 
  51 & MDE.Phi.kl & Measure & beta=5 & sigma=1 & n=100 & 462.08 \\ 
  52 & MME & Measure & beta=5 & sigma=1 & n=100 & 19777.03 \\ 
  53 & MME.b & Measure & beta=5 & sigma=1 & n=100 & 275176.68 \\ 
  54 & PWM & Measure & beta=5 & sigma=1 & n=100 & 106.91 \\ 
  55 & MLE & Measure & beta=1.5 & sigma=1 & n=200 & 0.23 \\ 
  56 & MLE.b & Measure & beta=1.5 & sigma=1 & n=200 & 0.16 \\ 
  57 & LME & Measure & beta=1.5 & sigma=1 & n=200 & 0.32 \\ 
  58 & MDE.Phi.chisq & Measure & beta=1.5 & sigma=1 & n=200 & 0.79 \\ 
  59 & MDE.Phi.tv & Measure & beta=1.5 & sigma=1 & n=200 & 0.77 \\ 
  60 & MDE.Phi.kl & Measure & beta=1.5 & sigma=1 & n=200 & 0.23 \\ 
  61 & MME & Measure & beta=1.5 & sigma=1 & n=200 & 9.88 \\ 
  62 & MME.b & Measure & beta=1.5 & sigma=1 & n=200 & 8.75 \\ 
  63 & PWM & Measure & beta=1.5 & sigma=1 & n=200 & 0.32 \\ 
  64 & MLE & Measure & beta=2 & sigma=1 & n=200 & 0.55 \\ 
  65 & MLE.b & Measure & beta=2 & sigma=1 & n=200 & 0.32 \\ 
  66 & LME & Measure & beta=2 & sigma=1 & n=200 & 0.55 \\ 
  67 & MDE.Phi.chisq & Measure & beta=2 & sigma=1 & n=200 & 1.61 \\ 
  68 & MDE.Phi.tv & Measure & beta=2 & sigma=1 & n=200 & 2.02 \\ 
  69 & MDE.Phi.kl & Measure & beta=2 & sigma=1 & n=200 & 0.55 \\ 
  70 & MME & Measure & beta=2 & sigma=1 & n=200 & 2.69 \\ 
  71 & MME.b & Measure & beta=2 & sigma=1 & n=200 & 4.70 \\ 
  72 & PWM & Measure & beta=2 & sigma=1 & n=200 & 0.55 \\ 
  73 & MLE & Measure & beta=2.5 & sigma=1 & n=200 & 4.46 \\ 
  74 & MLE.b & Measure & beta=2.5 & sigma=1 & n=200 & 3.98 \\ 
  75 & LME & Measure & beta=2.5 & sigma=1 & n=200 & 2.83 \\ 
  76 & MDE.Phi.chisq & Measure & beta=2.5 & sigma=1 & n=200 & 29.06 \\ 
  77 & MDE.Phi.tv & Measure & beta=2.5 & sigma=1 & n=200 & 21.18 \\ 
  78 & MDE.Phi.kl & Measure & beta=2.5 & sigma=1 & n=200 & 4.43 \\ 
  79 & MME & Measure & beta=2.5 & sigma=1 & n=200 & 9.10 \\ 
  80 & MME.b & Measure & beta=2.5 & sigma=1 & n=200 & 220.56 \\ 
  81 & PWM & Measure & beta=2.5 & sigma=1 & n=200 & 2.83 \\ 
  82 & MLE & Measure & beta=3 & sigma=1 & n=200 & 5.99 \\ 
  83 & MLE.b & Measure & beta=3 & sigma=1 & n=200 & 5.35 \\ 
  84 & LME & Measure & beta=3 & sigma=1 & n=200 & 4.03 \\ 
  85 & MDE.Phi.chisq & Measure & beta=3 & sigma=1 & n=200 & 128.44 \\ 
  86 & MDE.Phi.tv & Measure & beta=3 & sigma=1 & n=200 & 108.97 \\ 
  87 & MDE.Phi.kl & Measure & beta=3 & sigma=1 & n=200 & 6.25 \\ 
  88 & MME & Measure & beta=3 & sigma=1 & n=200 & 10.55 \\ 
  89 & MME.b & Measure & beta=3 & sigma=1 & n=200 & 537.96 \\ 
  90 & PWM & Measure & beta=3 & sigma=1 & n=200 & 4.03 \\ 
  91 & MLE & Measure & beta=4 & sigma=1 & n=200 & 2653340.55 \\ 
  92 & MLE.b & Measure & beta=4 & sigma=1 & n=200 & 2653340.36 \\ 
  93 & LME & Measure & beta=4 & sigma=1 & n=200 & 16.80 \\ 
  94 & MDE.Phi.chisq & Measure & beta=4 & sigma=1 & n=200 & 759.89 \\ 
  95 & MDE.Phi.tv & Measure & beta=4 & sigma=1 & n=200 & 499.73 \\ 
  96 & MDE.Phi.kl & Measure & beta=4 & sigma=1 & n=200 & 87.86 \\ 
  97 & MME & Measure & beta=4 & sigma=1 & n=200 & 1631.63 \\ 
  98 & MME.b & Measure & beta=4 & sigma=1 & n=200 & 11738.56 \\ 
  99 & PWM & Measure & beta=4 & sigma=1 & n=200 & 16.80 \\ 
  100 & MLE & Measure & beta=5 & sigma=1 & n=200 & 7415108.20 \\ 
  101 & MLE.b & Measure & beta=5 & sigma=1 & n=200 & 7415109.09 \\ 
  102 & LME & Measure & beta=5 & sigma=1 & n=200 & 60.59 \\ 
  103 & MDE.Phi.chisq & Measure & beta=5 & sigma=1 & n=200 & 1749.04 \\ 
  104 & MDE.Phi.tv & Measure & beta=5 & sigma=1 & n=200 & 1119.52 \\ 
  105 & MDE.Phi.kl & Measure & beta=5 & sigma=1 & n=200 & 197.27 \\ 
  106 & MME & Measure & beta=5 & sigma=1 & n=200 & 372326.92 \\ 
  107 & MME.b & Measure & beta=5 & sigma=1 & n=200 & 1575428.46 \\ 
  108 & PWM & Measure & beta=5 & sigma=1 & n=200 & 60.59 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220130/Output.accuracy2.LaTeX.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Sun Jan 30 20:11:05 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & Measure & beta=1.5 & sigma=1 & n=100 & 0.00 \\ 
  2 & MLE.b & Measure & beta=1.5 & sigma=1 & n=100 & 0.00 \\ 
  3 & LME & Measure & beta=1.5 & sigma=1 & n=100 & 0.00 \\ 
  4 & MDE.Phi.chisq & Measure & beta=1.5 & sigma=1 & n=100 & 181787018350624229332064482482084282602604822808686222086826422600406468626442880202480026068600642028200282242280222024246020860022848620402880404466644668026044682262046000244464684680404040648066066624288048682020048688026826682826820642682280002668866466086886864424642802262886688486208806684284.00 \\ 
  5 & MDE.Phi.tv & Measure & beta=1.5 & sigma=1 & n=100 & 0.03 \\ 
  6 & MDE.Phi.kl & Measure & beta=1.5 & sigma=1 & n=100 & 0.00 \\ 
  7 & MME & Measure & beta=1.5 & sigma=1 & n=100 & 0.01 \\ 
  8 & MME.b & Measure & beta=1.5 & sigma=1 & n=100 & 7.11 \\ 
  9 & PWM & Measure & beta=1.5 & sigma=1 & n=100 & 0.00 \\ 
  10 & MLE & Measure & beta=2 & sigma=1 & n=100 & 0.00 \\ 
  11 & MLE.b & Measure & beta=2 & sigma=1 & n=100 & 0.00 \\ 
  12 & LME & Measure & beta=2 & sigma=1 & n=100 & 0.00 \\ 
  13 & MDE.Phi.chisq & Measure & beta=2 & sigma=1 & n=100 & 0.03 \\ 
  14 & MDE.Phi.tv & Measure & beta=2 & sigma=1 & n=100 & 0.02 \\ 
  15 & MDE.Phi.kl & Measure & beta=2 & sigma=1 & n=100 & 0.00 \\ 
  16 & MME & Measure & beta=2 & sigma=1 & n=100 & 0.00 \\ 
  17 & MME.b & Measure & beta=2 & sigma=1 & n=100 & 0.01 \\ 
  18 & PWM & Measure & beta=2 & sigma=1 & n=100 & 0.00 \\ 
  19 & MLE & Measure & beta=2.5 & sigma=1 & n=100 & 0.00 \\ 
  20 & MLE.b & Measure & beta=2.5 & sigma=1 & n=100 & 0.00 \\ 
  21 & LME & Measure & beta=2.5 & sigma=1 & n=100 & 0.00 \\ 
  22 & MDE.Phi.chisq & Measure & beta=2.5 & sigma=1 & n=100 & 0.02 \\ 
  23 & MDE.Phi.tv & Measure & beta=2.5 & sigma=1 & n=100 & 0.02 \\ 
  24 & MDE.Phi.kl & Measure & beta=2.5 & sigma=1 & n=100 & 0.00 \\ 
  25 & MME & Measure & beta=2.5 & sigma=1 & n=100 & 0.00 \\ 
  26 & MME.b & Measure & beta=2.5 & sigma=1 & n=100 & 8.08 \\ 
  27 & PWM & Measure & beta=2.5 & sigma=1 & n=100 & 0.00 \\ 
  28 & MLE & Measure & beta=3 & sigma=1 & n=100 & 0.00 \\ 
  29 & MLE.b & Measure & beta=3 & sigma=1 & n=100 & 0.00 \\ 
  30 & LME & Measure & beta=3 & sigma=1 & n=100 & 0.00 \\ 
  31 & MDE.Phi.chisq & Measure & beta=3 & sigma=1 & n=100 & 0.02 \\ 
  32 & MDE.Phi.tv & Measure & beta=3 & sigma=1 & n=100 & 0.02 \\ 
  33 & MDE.Phi.kl & Measure & beta=3 & sigma=1 & n=100 & 0.00 \\ 
  34 & MME & Measure & beta=3 & sigma=1 & n=100 & 0.00 \\ 
  35 & MME.b & Measure & beta=3 & sigma=1 & n=100 & 0.01 \\ 
  36 & PWM & Measure & beta=3 & sigma=1 & n=100 & 0.00 \\ 
  37 & MLE & Measure & beta=4 & sigma=1 & n=100 & 0.00 \\ 
  38 & MLE.b & Measure & beta=4 & sigma=1 & n=100 & 0.00 \\ 
  39 & LME & Measure & beta=4 & sigma=1 & n=100 & 0.00 \\ 
  40 & MDE.Phi.chisq & Measure & beta=4 & sigma=1 & n=100 & 0.02 \\ 
  41 & MDE.Phi.tv & Measure & beta=4 & sigma=1 & n=100 & 0.01 \\ 
  42 & MDE.Phi.kl & Measure & beta=4 & sigma=1 & n=100 & 0.00 \\ 
  43 & MME & Measure & beta=4 & sigma=1 & n=100 & 0.00 \\ 
  44 & MME.b & Measure & beta=4 & sigma=1 & n=100 & 4041.95 \\ 
  45 & PWM & Measure & beta=4 & sigma=1 & n=100 & 0.00 \\ 
  46 & MLE & Measure & beta=5 & sigma=1 & n=100 & 0.00 \\ 
  47 & MLE.b & Measure & beta=5 & sigma=1 & n=100 & 0.00 \\ 
  48 & LME & Measure & beta=5 & sigma=1 & n=100 & 0.00 \\ 
  49 & MDE.Phi.chisq & Measure & beta=5 & sigma=1 & n=100 & 0.01 \\ 
  50 & MDE.Phi.tv & Measure & beta=5 & sigma=1 & n=100 & 0.01 \\ 
  51 & MDE.Phi.kl & Measure & beta=5 & sigma=1 & n=100 & 0.00 \\ 
  52 & MME & Measure & beta=5 & sigma=1 & n=100 & 0.00 \\ 
  53 & MME.b & Measure & beta=5 & sigma=1 & n=100 & 515620838018138634806240604226.00 \\ 
  54 & PWM & Measure & beta=5 & sigma=1 & n=100 & 0.00 \\ 
  55 & MLE & Measure & beta=1.5 & sigma=1 & n=200 & 0.00 \\ 
  56 & MLE.b & Measure & beta=1.5 & sigma=1 & n=200 & 0.00 \\ 
  57 & LME & Measure & beta=1.5 & sigma=1 & n=200 & 0.00 \\ 
  58 & MDE.Phi.chisq & Measure & beta=1.5 & sigma=1 & n=200 & 0.03 \\ 
  59 & MDE.Phi.tv & Measure & beta=1.5 & sigma=1 & n=200 & 0.03 \\ 
  60 & MDE.Phi.kl & Measure & beta=1.5 & sigma=1 & n=200 & 0.00 \\ 
  61 & MME & Measure & beta=1.5 & sigma=1 & n=200 & 0.01 \\ 
  62 & MME.b & Measure & beta=1.5 & sigma=1 & n=200 & 0.01 \\ 
  63 & PWM & Measure & beta=1.5 & sigma=1 & n=200 & 0.00 \\ 
  64 & MLE & Measure & beta=2 & sigma=1 & n=200 & 0.00 \\ 
  65 & MLE.b & Measure & beta=2 & sigma=1 & n=200 & 0.00 \\ 
  66 & LME & Measure & beta=2 & sigma=1 & n=200 & 0.00 \\ 
  67 & MDE.Phi.chisq & Measure & beta=2 & sigma=1 & n=200 & 0.02 \\ 
  68 & MDE.Phi.tv & Measure & beta=2 & sigma=1 & n=200 & 0.02 \\ 
  69 & MDE.Phi.kl & Measure & beta=2 & sigma=1 & n=200 & 0.00 \\ 
  70 & MME & Measure & beta=2 & sigma=1 & n=200 & 0.00 \\ 
  71 & MME.b & Measure & beta=2 & sigma=1 & n=200 & 0.05 \\ 
  72 & PWM & Measure & beta=2 & sigma=1 & n=200 & 0.00 \\ 
  73 & MLE & Measure & beta=2.5 & sigma=1 & n=200 & 0.00 \\ 
  74 & MLE.b & Measure & beta=2.5 & sigma=1 & n=200 & 0.00 \\ 
  75 & LME & Measure & beta=2.5 & sigma=1 & n=200 & 0.00 \\ 
  76 & MDE.Phi.chisq & Measure & beta=2.5 & sigma=1 & n=200 & 0.02 \\ 
  77 & MDE.Phi.tv & Measure & beta=2.5 & sigma=1 & n=200 & 0.01 \\ 
  78 & MDE.Phi.kl & Measure & beta=2.5 & sigma=1 & n=200 & 0.00 \\ 
  79 & MME & Measure & beta=2.5 & sigma=1 & n=200 & 0.00 \\ 
  80 & MME.b & Measure & beta=2.5 & sigma=1 & n=200 & 0.00 \\ 
  81 & PWM & Measure & beta=2.5 & sigma=1 & n=200 & 0.00 \\ 
  82 & MLE & Measure & beta=3 & sigma=1 & n=200 & 0.00 \\ 
  83 & MLE.b & Measure & beta=3 & sigma=1 & n=200 & 0.00 \\ 
  84 & LME & Measure & beta=3 & sigma=1 & n=200 & 0.00 \\ 
  85 & MDE.Phi.chisq & Measure & beta=3 & sigma=1 & n=200 & 0.01 \\ 
  86 & MDE.Phi.tv & Measure & beta=3 & sigma=1 & n=200 & 0.01 \\ 
  87 & MDE.Phi.kl & Measure & beta=3 & sigma=1 & n=200 & 0.00 \\ 
  88 & MME & Measure & beta=3 & sigma=1 & n=200 & 0.00 \\ 
  89 & MME.b & Measure & beta=3 & sigma=1 & n=200 & 0.00 \\ 
  90 & PWM & Measure & beta=3 & sigma=1 & n=200 & 0.00 \\ 
  91 & MLE & Measure & beta=4 & sigma=1 & n=200 & 0.00 \\ 
  92 & MLE.b & Measure & beta=4 & sigma=1 & n=200 & 0.00 \\ 
  93 & LME & Measure & beta=4 & sigma=1 & n=200 & 0.00 \\ 
  94 & MDE.Phi.chisq & Measure & beta=4 & sigma=1 & n=200 & 0.01 \\ 
  95 & MDE.Phi.tv & Measure & beta=4 & sigma=1 & n=200 & 0.01 \\ 
  96 & MDE.Phi.kl & Measure & beta=4 & sigma=1 & n=200 & 0.00 \\ 
  97 & MME & Measure & beta=4 & sigma=1 & n=200 & 0.00 \\ 
  98 & MME.b & Measure & beta=4 & sigma=1 & n=200 & 0.09 \\ 
  99 & PWM & Measure & beta=4 & sigma=1 & n=200 & 0.00 \\ 
  100 & MLE & Measure & beta=5 & sigma=1 & n=200 & 0.00 \\ 
  101 & MLE.b & Measure & beta=5 & sigma=1 & n=200 & 0.00 \\ 
  102 & LME & Measure & beta=5 & sigma=1 & n=200 & 0.00 \\ 
  103 & MDE.Phi.chisq & Measure & beta=5 & sigma=1 & n=200 & 0.01 \\ 
  104 & MDE.Phi.tv & Measure & beta=5 & sigma=1 & n=200 & 0.01 \\ 
  105 & MDE.Phi.kl & Measure & beta=5 & sigma=1 & n=200 & 0.00 \\ 
  106 & MME & Measure & beta=5 & sigma=1 & n=200 & 0.00 \\ 
  107 & MME.b & Measure & beta=5 & sigma=1 & n=200 & 0.47 \\ 
  108 & PWM & Measure & beta=5 & sigma=1 & n=200 & 0.00 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220130/Output.bias.LaTeX.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Sun Jan 30 20:11:05 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=1 & n=100 & 0.17 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=1 & n=100 & -0.02 \\ 
  3 & LME & beta & beta=1.5 & sigma=1 & n=100 & 0.33 \\ 
  4 & MDE.Phi.chisq & beta & beta=1.5 & sigma=1 & n=100 & -0.51 \\ 
  5 & MDE.Phi.tv & beta & beta=1.5 & sigma=1 & n=100 & -0.24 \\ 
  6 & MDE.Phi.kl & beta & beta=1.5 & sigma=1 & n=100 & 0.17 \\ 
  7 & MME & beta & beta=1.5 & sigma=1 & n=100 & 1.29 \\ 
  8 & MME.b & beta & beta=1.5 & sigma=1 & n=100 & 4.81 \\ 
  9 & PWM & beta & beta=1.5 & sigma=1 & n=100 & 0.33 \\ 
  10 & MLE & sigma & beta=1.5 & sigma=1 & n=100 & 0.18 \\ 
  11 & MLE.b & sigma & beta=1.5 & sigma=1 & n=100 & -0.02 \\ 
  12 & LME & sigma & beta=1.5 & sigma=1 & n=100 & 0.33 \\ 
  13 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=1 & n=100 & 0.55 \\ 
  14 & MDE.Phi.tv & sigma & beta=1.5 & sigma=1 & n=100 & 0.83 \\ 
  15 & MDE.Phi.kl & sigma & beta=1.5 & sigma=1 & n=100 & 0.18 \\ 
  16 & MME & sigma & beta=1.5 & sigma=1 & n=100 & 2.15 \\ 
  17 & MME.b & sigma & beta=1.5 & sigma=1 & n=100 & 5.83 \\ 
  18 & PWM & sigma & beta=1.5 & sigma=1 & n=100 & 0.33 \\ 
  19 & MLE & beta & beta=2 & sigma=1 & n=100 & 0.63 \\ 
  20 & MLE.b & beta & beta=2 & sigma=1 & n=100 & 0.28 \\ 
  21 & LME & beta & beta=2 & sigma=1 & n=100 & 0.45 \\ 
  22 & MDE.Phi.chisq & beta & beta=2 & sigma=1 & n=100 & 0.15 \\ 
  23 & MDE.Phi.tv & beta & beta=2 & sigma=1 & n=100 & 0.77 \\ 
  24 & MDE.Phi.kl & beta & beta=2 & sigma=1 & n=100 & 0.47 \\ 
  25 & MME & beta & beta=2 & sigma=1 & n=100 & 1.68 \\ 
  26 & MME.b & beta & beta=2 & sigma=1 & n=100 & 7.47 \\ 
  27 & PWM & beta & beta=2 & sigma=1 & n=100 & 0.45 \\ 
  28 & MLE & sigma & beta=2 & sigma=1 & n=100 & 0.43 \\ 
  29 & MLE.b & sigma & beta=2 & sigma=1 & n=100 & 0.17 \\ 
  30 & LME & sigma & beta=2 & sigma=1 & n=100 & 0.30 \\ 
  31 & MDE.Phi.chisq & sigma & beta=2 & sigma=1 & n=100 & 1.15 \\ 
  32 & MDE.Phi.tv & sigma & beta=2 & sigma=1 & n=100 & 1.68 \\ 
  33 & MDE.Phi.kl & sigma & beta=2 & sigma=1 & n=100 & 0.33 \\ 
  34 & MME & sigma & beta=2 & sigma=1 & n=100 & 1.44 \\ 
  35 & MME.b & sigma & beta=2 & sigma=1 & n=100 & 5.59 \\ 
  36 & PWM & sigma & beta=2 & sigma=1 & n=100 & 0.30 \\ 
  37 & MLE & beta & beta=2.5 & sigma=1 & n=100 & 3.26 \\ 
  38 & MLE.b & beta & beta=2.5 & sigma=1 & n=100 & 2.80 \\ 
  39 & LME & beta & beta=2.5 & sigma=1 & n=100 & 0.69 \\ 
  40 & MDE.Phi.chisq & beta & beta=2.5 & sigma=1 & n=100 & 1.81 \\ 
  41 & MDE.Phi.tv & beta & beta=2.5 & sigma=1 & n=100 & 2.65 \\ 
  42 & MDE.Phi.kl & beta & beta=2.5 & sigma=1 & n=100 & 0.95 \\ 
  43 & MME & beta & beta=2.5 & sigma=1 & n=100 & 2.32 \\ 
  44 & MME.b & beta & beta=2.5 & sigma=1 & n=100 & 5.52 \\ 
  45 & PWM & beta & beta=2.5 & sigma=1 & n=100 & 0.69 \\ 
  46 & MLE & sigma & beta=2.5 & sigma=1 & n=100 & 1.84 \\ 
  47 & MLE.b & sigma & beta=2.5 & sigma=1 & n=100 & 1.59 \\ 
  48 & LME & sigma & beta=2.5 & sigma=1 & n=100 & 0.36 \\ 
  49 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=1 & n=100 & 2.23 \\ 
  50 & MDE.Phi.tv & sigma & beta=2.5 & sigma=1 & n=100 & 2.77 \\ 
  51 & MDE.Phi.kl & sigma & beta=2.5 & sigma=1 & n=100 & 0.51 \\ 
  52 & MME & sigma & beta=2.5 & sigma=1 & n=100 & 1.35 \\ 
  53 & MME.b & sigma & beta=2.5 & sigma=1 & n=100 & 3.03 \\ 
  54 & PWM & sigma & beta=2.5 & sigma=1 & n=100 & 0.36 \\ 
  55 & MLE & beta & beta=3 & sigma=1 & n=100 & 1589.97 \\ 
  56 & MLE.b & beta & beta=3 & sigma=1 & n=100 & 1589.48 \\ 
  57 & LME & beta & beta=3 & sigma=1 & n=100 & 1.01 \\ 
  58 & MDE.Phi.chisq & beta & beta=3 & sigma=1 & n=100 & 4.28 \\ 
  59 & MDE.Phi.tv & beta & beta=3 & sigma=1 & n=100 & 5.75 \\ 
  60 & MDE.Phi.kl & beta & beta=3 & sigma=1 & n=100 & 1.92 \\ 
  61 & MME & beta & beta=3 & sigma=1 & n=100 & 14.49 \\ 
  62 & MME.b & beta & beta=3 & sigma=1 & n=100 & 46.98 \\ 
  63 & PWM & beta & beta=3 & sigma=1 & n=100 & 1.01 \\ 
  64 & MLE & sigma & beta=3 & sigma=1 & n=100 & 671.84 \\ 
  65 & MLE.b & sigma & beta=3 & sigma=1 & n=100 & 671.63 \\ 
  66 & LME & sigma & beta=3 & sigma=1 & n=100 & 0.42 \\ 
  67 & MDE.Phi.chisq & sigma & beta=3 & sigma=1 & n=100 & 3.41 \\ 
  68 & MDE.Phi.tv & sigma & beta=3 & sigma=1 & n=100 & 4.17 \\ 
  69 & MDE.Phi.kl & sigma & beta=3 & sigma=1 & n=100 & 0.83 \\ 
  70 & MME & sigma & beta=3 & sigma=1 & n=100 & 5.74 \\ 
  71 & MME.b & sigma & beta=3 & sigma=1 & n=100 & 18.57 \\ 
  72 & PWM & sigma & beta=3 & sigma=1 & n=100 & 0.42 \\ 
  73 & MLE & beta & beta=4 & sigma=1 & n=100 & 225.86 \\ 
  74 & MLE.b & beta & beta=4 & sigma=1 & n=100 & 225.41 \\ 
  75 & LME & beta & beta=4 & sigma=1 & n=100 & 1.72 \\ 
  76 & MDE.Phi.chisq & beta & beta=4 & sigma=1 & n=100 & 10.91 \\ 
  77 & MDE.Phi.tv & beta & beta=4 & sigma=1 & n=100 & 13.26 \\ 
  78 & MDE.Phi.kl & beta & beta=4 & sigma=1 & n=100 & 3.52 \\ 
  79 & MME & beta & beta=4 & sigma=1 & n=100 & 7.35 \\ 
  80 & MME.b & beta & beta=4 & sigma=1 & n=100 & 36.89 \\ 
  81 & PWM & beta & beta=4 & sigma=1 & n=100 & 1.72 \\ 
  82 & MLE & sigma & beta=4 & sigma=1 & n=100 & 58.82 \\ 
  83 & MLE.b & sigma & beta=4 & sigma=1 & n=100 & 58.68 \\ 
  84 & LME & sigma & beta=4 & sigma=1 & n=100 & 0.52 \\ 
  85 & MDE.Phi.chisq & sigma & beta=4 & sigma=1 & n=100 & 5.42 \\ 
  86 & MDE.Phi.tv & sigma & beta=4 & sigma=1 & n=100 & 6.19 \\ 
  87 & MDE.Phi.kl & sigma & beta=4 & sigma=1 & n=100 & 1.09 \\ 
  88 & MME & sigma & beta=4 & sigma=1 & n=100 & 2.33 \\ 
  89 & MME.b & sigma & beta=4 & sigma=1 & n=100 & 12.43 \\ 
  90 & PWM & sigma & beta=4 & sigma=1 & n=100 & 0.52 \\ 
  91 & MLE & beta & beta=5 & sigma=1 & n=100 & 73.42 \\ 
  92 & MLE.b & beta & beta=5 & sigma=1 & n=100 & 73.05 \\ 
  93 & LME & beta & beta=5 & sigma=1 & n=100 & 2.32 \\ 
  94 & MDE.Phi.chisq & beta & beta=5 & sigma=1 & n=100 & 17.01 \\ 
  95 & MDE.Phi.tv & beta & beta=5 & sigma=1 & n=100 & 19.36 \\ 
  96 & MDE.Phi.kl & beta & beta=5 & sigma=1 & n=100 & 5.26 \\ 
  97 & MME & beta & beta=5 & sigma=1 & n=100 & 11.76 \\ 
  98 & MME.b & beta & beta=5 & sigma=1 & n=100 & 42.24 \\ 
  99 & PWM & beta & beta=5 & sigma=1 & n=100 & 2.32 \\ 
  100 & MLE & sigma & beta=5 & sigma=1 & n=100 & 17.74 \\ 
  101 & MLE.b & sigma & beta=5 & sigma=1 & n=100 & 17.66 \\ 
  102 & LME & sigma & beta=5 & sigma=1 & n=100 & 0.54 \\ 
  103 & MDE.Phi.chisq & sigma & beta=5 & sigma=1 & n=100 & 6.23 \\ 
  104 & MDE.Phi.tv & sigma & beta=5 & sigma=1 & n=100 & 6.77 \\ 
  105 & MDE.Phi.kl & sigma & beta=5 & sigma=1 & n=100 & 1.24 \\ 
  106 & MME & sigma & beta=5 & sigma=1 & n=100 & 2.76 \\ 
  107 & MME.b & sigma & beta=5 & sigma=1 & n=100 & 9.98 \\ 
  108 & PWM & sigma & beta=5 & sigma=1 & n=100 & 0.54 \\ 
  109 & MLE & beta & beta=1.5 & sigma=1 & n=200 & 0.08 \\ 
  110 & MLE.b & beta & beta=1.5 & sigma=1 & n=200 & -0.01 \\ 
  111 & LME & beta & beta=1.5 & sigma=1 & n=200 & 0.21 \\ 
  112 & MDE.Phi.chisq & beta & beta=1.5 & sigma=1 & n=200 & -0.64 \\ 
  113 & MDE.Phi.tv & beta & beta=1.5 & sigma=1 & n=200 & -0.49 \\ 
  114 & MDE.Phi.kl & beta & beta=1.5 & sigma=1 & n=200 & 0.08 \\ 
  115 & MME & beta & beta=1.5 & sigma=1 & n=200 & 1.01 \\ 
  116 & MME.b & beta & beta=1.5 & sigma=1 & n=200 & 0.81 \\ 
  117 & PWM & beta & beta=1.5 & sigma=1 & n=200 & 0.21 \\ 
  118 & MLE & sigma & beta=1.5 & sigma=1 & n=200 & 0.08 \\ 
  119 & MLE.b & sigma & beta=1.5 & sigma=1 & n=200 & -0.01 \\ 
  120 & LME & sigma & beta=1.5 & sigma=1 & n=200 & 0.21 \\ 
  121 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=1 & n=200 & 0.13 \\ 
  122 & MDE.Phi.tv & sigma & beta=1.5 & sigma=1 & n=200 & 0.26 \\ 
  123 & MDE.Phi.kl & sigma & beta=1.5 & sigma=1 & n=200 & 0.08 \\ 
  124 & MME & sigma & beta=1.5 & sigma=1 & n=200 & 1.80 \\ 
  125 & MME.b & sigma & beta=1.5 & sigma=1 & n=200 & 1.53 \\ 
  126 & PWM & sigma & beta=1.5 & sigma=1 & n=200 & 0.21 \\ 
  127 & MLE & beta & beta=2 & sigma=1 & n=200 & 0.15 \\ 
  128 & MLE.b & beta & beta=2 & sigma=1 & n=200 & -0.02 \\ 
  129 & LME & beta & beta=2 & sigma=1 & n=200 & 0.23 \\ 
  130 & MDE.Phi.chisq & beta & beta=2 & sigma=1 & n=200 & -0.65 \\ 
  131 & MDE.Phi.tv & beta & beta=2 & sigma=1 & n=200 & -0.43 \\ 
  132 & MDE.Phi.kl & beta & beta=2 & sigma=1 & n=200 & 0.15 \\ 
  133 & MME & beta & beta=2 & sigma=1 & n=200 & 0.98 \\ 
  134 & MME.b & beta & beta=2 & sigma=1 & n=200 & 0.65 \\ 
  135 & PWM & beta & beta=2 & sigma=1 & n=200 & 0.23 \\ 
  136 & MLE & sigma & beta=2 & sigma=1 & n=200 & 0.11 \\ 
  137 & MLE.b & sigma & beta=2 & sigma=1 & n=200 & -0.01 \\ 
  138 & LME & sigma & beta=2 & sigma=1 & n=200 & 0.15 \\ 
  139 & MDE.Phi.chisq & sigma & beta=2 & sigma=1 & n=200 & 0.17 \\ 
  140 & MDE.Phi.tv & sigma & beta=2 & sigma=1 & n=200 & 0.28 \\ 
  141 & MDE.Phi.kl & sigma & beta=2 & sigma=1 & n=200 & 0.11 \\ 
  142 & MME & sigma & beta=2 & sigma=1 & n=200 & 0.90 \\ 
  143 & MME.b & sigma & beta=2 & sigma=1 & n=200 & 0.63 \\ 
  144 & PWM & sigma & beta=2 & sigma=1 & n=200 & 0.15 \\ 
  145 & MLE & beta & beta=2.5 & sigma=1 & n=200 & 0.29 \\ 
  146 & MLE.b & beta & beta=2.5 & sigma=1 & n=200 & -0.02 \\ 
  147 & LME & beta & beta=2.5 & sigma=1 & n=200 & 0.31 \\ 
  148 & MDE.Phi.chisq & beta & beta=2.5 & sigma=1 & n=200 & -0.41 \\ 
  149 & MDE.Phi.tv & beta & beta=2.5 & sigma=1 & n=200 & -0.22 \\ 
  150 & MDE.Phi.kl & beta & beta=2.5 & sigma=1 & n=200 & 0.29 \\ 
  151 & MME & beta & beta=2.5 & sigma=1 & n=200 & 1.11 \\ 
  152 & MME.b & beta & beta=2.5 & sigma=1 & n=200 & 1.15 \\ 
  153 & PWM & beta & beta=2.5 & sigma=1 & n=200 & 0.31 \\ 
  154 & MLE & sigma & beta=2.5 & sigma=1 & n=200 & 0.15 \\ 
  155 & MLE.b & sigma & beta=2.5 & sigma=1 & n=200 & -0.01 \\ 
  156 & LME & sigma & beta=2.5 & sigma=1 & n=200 & 0.16 \\ 
  157 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=1 & n=200 & 0.38 \\ 
  158 & MDE.Phi.tv & sigma & beta=2.5 & sigma=1 & n=200 & 0.41 \\ 
  159 & MDE.Phi.kl & sigma & beta=2.5 & sigma=1 & n=200 & 0.15 \\ 
  160 & MME & sigma & beta=2.5 & sigma=1 & n=200 & 0.68 \\ 
  161 & MME.b & sigma & beta=2.5 & sigma=1 & n=200 & 0.70 \\ 
  162 & PWM & sigma & beta=2.5 & sigma=1 & n=200 & 0.16 \\ 
  163 & MLE & beta & beta=3 & sigma=1 & n=200 & 0.45 \\ 
  164 & MLE.b & beta & beta=3 & sigma=1 & n=200 & -0.01 \\ 
  165 & LME & beta & beta=3 & sigma=1 & n=200 & 0.41 \\ 
  166 & MDE.Phi.chisq & beta & beta=3 & sigma=1 & n=200 & 0.30 \\ 
  167 & MDE.Phi.tv & beta & beta=3 & sigma=1 & n=200 & 0.42 \\ 
  168 & MDE.Phi.kl & beta & beta=3 & sigma=1 & n=200 & 0.45 \\ 
  169 & MME & beta & beta=3 & sigma=1 & n=200 & 1.32 \\ 
  170 & MME.b & beta & beta=3 & sigma=1 & n=200 & 1.89 \\ 
  171 & PWM & beta & beta=3 & sigma=1 & n=200 & 0.41 \\ 
  172 & MLE & sigma & beta=3 & sigma=1 & n=200 & 0.20 \\ 
  173 & MLE.b & sigma & beta=3 & sigma=1 & n=200 & -0.00 \\ 
  174 & LME & sigma & beta=3 & sigma=1 & n=200 & 0.17 \\ 
  175 & MDE.Phi.chisq & sigma & beta=3 & sigma=1 & n=200 & 0.77 \\ 
  176 & MDE.Phi.tv & sigma & beta=3 & sigma=1 & n=200 & 0.72 \\ 
  177 & MDE.Phi.kl & sigma & beta=3 & sigma=1 & n=200 & 0.20 \\ 
  178 & MME & sigma & beta=3 & sigma=1 & n=200 & 0.61 \\ 
  179 & MME.b & sigma & beta=3 & sigma=1 & n=200 & 0.84 \\ 
  180 & PWM & sigma & beta=3 & sigma=1 & n=200 & 0.17 \\ 
  181 & MLE & beta & beta=4 & sigma=1 & n=200 & 25.96 \\ 
  182 & MLE.b & beta & beta=4 & sigma=1 & n=200 & 25.30 \\ 
  183 & LME & beta & beta=4 & sigma=1 & n=200 & 0.87 \\ 
  184 & MDE.Phi.chisq & beta & beta=4 & sigma=1 & n=200 & 4.33 \\ 
  185 & MDE.Phi.tv & beta & beta=4 & sigma=1 & n=200 & 3.13 \\ 
  186 & MDE.Phi.kl & beta & beta=4 & sigma=1 & n=200 & 1.46 \\ 
  187 & MME & beta & beta=4 & sigma=1 & n=200 & 3.01 \\ 
  188 & MME.b & beta & beta=4 & sigma=1 & n=200 & 8.15 \\ 
  189 & PWM & beta & beta=4 & sigma=1 & n=200 & 0.87 \\ 
  190 & MLE & sigma & beta=4 & sigma=1 & n=200 & 7.83 \\ 
  191 & MLE.b & sigma & beta=4 & sigma=1 & n=200 & 7.63 \\ 
  192 & LME & sigma & beta=4 & sigma=1 & n=200 & 0.26 \\ 
  193 & MDE.Phi.chisq & sigma & beta=4 & sigma=1 & n=200 & 2.24 \\ 
  194 & MDE.Phi.tv & sigma & beta=4 & sigma=1 & n=200 & 1.62 \\ 
  195 & MDE.Phi.kl & sigma & beta=4 & sigma=1 & n=200 & 0.44 \\ 
  196 & MME & sigma & beta=4 & sigma=1 & n=200 & 0.94 \\ 
  197 & MME.b & sigma & beta=4 & sigma=1 & n=200 & 2.54 \\ 
  198 & PWM & sigma & beta=4 & sigma=1 & n=200 & 0.26 \\ 
  199 & MLE & beta & beta=5 & sigma=1 & n=200 & 39.55 \\ 
  200 & MLE.b & beta & beta=5 & sigma=1 & n=200 & 38.83 \\ 
  201 & LME & beta & beta=5 & sigma=1 & n=200 & 1.69 \\ 
  202 & MDE.Phi.chisq & beta & beta=5 & sigma=1 & n=200 & 10.43 \\ 
  203 & MDE.Phi.tv & beta & beta=5 & sigma=1 & n=200 & 7.14 \\ 
  204 & MDE.Phi.kl & beta & beta=5 & sigma=1 & n=200 & 2.72 \\ 
  205 & MME & beta & beta=5 & sigma=1 & n=200 & 11.16 \\ 
  206 & MME.b & beta & beta=5 & sigma=1 & n=200 & 34.22 \\ 
  207 & PWM & beta & beta=5 & sigma=1 & n=200 & 1.69 \\ 
  208 & MLE & sigma & beta=5 & sigma=1 & n=200 & 9.76 \\ 
  209 & MLE.b & sigma & beta=5 & sigma=1 & n=200 & 9.59 \\ 
  210 & LME & sigma & beta=5 & sigma=1 & n=200 & 0.40 \\ 
  211 & MDE.Phi.chisq & sigma & beta=5 & sigma=1 & n=200 & 3.68 \\ 
  212 & MDE.Phi.tv & sigma & beta=5 & sigma=1 & n=200 & 2.49 \\ 
  213 & MDE.Phi.kl & sigma & beta=5 & sigma=1 & n=200 & 0.64 \\ 
  214 & MME & sigma & beta=5 & sigma=1 & n=200 & 2.66 \\ 
  215 & MME.b & sigma & beta=5 & sigma=1 & n=200 & 8.27 \\ 
  216 & PWM & sigma & beta=5 & sigma=1 & n=200 & 0.40 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220130/Output.mean.LaTeX.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Sun Jan 30 20:11:05 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=1 & n=100 & 1.67 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=1 & n=100 & 1.48 \\ 
  3 & LME & beta & beta=1.5 & sigma=1 & n=100 & 1.83 \\ 
  4 & MDE.Phi.chisq & beta & beta=1.5 & sigma=1 & n=100 & 0.99 \\ 
  5 & MDE.Phi.tv & beta & beta=1.5 & sigma=1 & n=100 & 1.26 \\ 
  6 & MDE.Phi.kl & beta & beta=1.5 & sigma=1 & n=100 & 1.67 \\ 
  7 & MME & beta & beta=1.5 & sigma=1 & n=100 & 2.79 \\ 
  8 & MME.b & beta & beta=1.5 & sigma=1 & n=100 & 6.31 \\ 
  9 & PWM & beta & beta=1.5 & sigma=1 & n=100 & 1.83 \\ 
  10 & MLE & sigma & beta=1.5 & sigma=1 & n=100 & 1.18 \\ 
  11 & MLE.b & sigma & beta=1.5 & sigma=1 & n=100 & 0.98 \\ 
  12 & LME & sigma & beta=1.5 & sigma=1 & n=100 & 1.33 \\ 
  13 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=1 & n=100 & 1.55 \\ 
  14 & MDE.Phi.tv & sigma & beta=1.5 & sigma=1 & n=100 & 1.83 \\ 
  15 & MDE.Phi.kl & sigma & beta=1.5 & sigma=1 & n=100 & 1.18 \\ 
  16 & MME & sigma & beta=1.5 & sigma=1 & n=100 & 3.15 \\ 
  17 & MME.b & sigma & beta=1.5 & sigma=1 & n=100 & 6.83 \\ 
  18 & PWM & sigma & beta=1.5 & sigma=1 & n=100 & 1.33 \\ 
  19 & MLE & beta & beta=2 & sigma=1 & n=100 & 2.63 \\ 
  20 & MLE.b & beta & beta=2 & sigma=1 & n=100 & 2.28 \\ 
  21 & LME & beta & beta=2 & sigma=1 & n=100 & 2.45 \\ 
  22 & MDE.Phi.chisq & beta & beta=2 & sigma=1 & n=100 & 2.15 \\ 
  23 & MDE.Phi.tv & beta & beta=2 & sigma=1 & n=100 & 2.77 \\ 
  24 & MDE.Phi.kl & beta & beta=2 & sigma=1 & n=100 & 2.47 \\ 
  25 & MME & beta & beta=2 & sigma=1 & n=100 & 3.68 \\ 
  26 & MME.b & beta & beta=2 & sigma=1 & n=100 & 9.47 \\ 
  27 & PWM & beta & beta=2 & sigma=1 & n=100 & 2.45 \\ 
  28 & MLE & sigma & beta=2 & sigma=1 & n=100 & 1.43 \\ 
  29 & MLE.b & sigma & beta=2 & sigma=1 & n=100 & 1.17 \\ 
  30 & LME & sigma & beta=2 & sigma=1 & n=100 & 1.30 \\ 
  31 & MDE.Phi.chisq & sigma & beta=2 & sigma=1 & n=100 & 2.15 \\ 
  32 & MDE.Phi.tv & sigma & beta=2 & sigma=1 & n=100 & 2.68 \\ 
  33 & MDE.Phi.kl & sigma & beta=2 & sigma=1 & n=100 & 1.33 \\ 
  34 & MME & sigma & beta=2 & sigma=1 & n=100 & 2.44 \\ 
  35 & MME.b & sigma & beta=2 & sigma=1 & n=100 & 6.59 \\ 
  36 & PWM & sigma & beta=2 & sigma=1 & n=100 & 1.30 \\ 
  37 & MLE & beta & beta=2.5 & sigma=1 & n=100 & 5.76 \\ 
  38 & MLE.b & beta & beta=2.5 & sigma=1 & n=100 & 5.30 \\ 
  39 & LME & beta & beta=2.5 & sigma=1 & n=100 & 3.19 \\ 
  40 & MDE.Phi.chisq & beta & beta=2.5 & sigma=1 & n=100 & 4.31 \\ 
  41 & MDE.Phi.tv & beta & beta=2.5 & sigma=1 & n=100 & 5.15 \\ 
  42 & MDE.Phi.kl & beta & beta=2.5 & sigma=1 & n=100 & 3.45 \\ 
  43 & MME & beta & beta=2.5 & sigma=1 & n=100 & 4.82 \\ 
  44 & MME.b & beta & beta=2.5 & sigma=1 & n=100 & 8.02 \\ 
  45 & PWM & beta & beta=2.5 & sigma=1 & n=100 & 3.19 \\ 
  46 & MLE & sigma & beta=2.5 & sigma=1 & n=100 & 2.84 \\ 
  47 & MLE.b & sigma & beta=2.5 & sigma=1 & n=100 & 2.59 \\ 
  48 & LME & sigma & beta=2.5 & sigma=1 & n=100 & 1.36 \\ 
  49 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=1 & n=100 & 3.23 \\ 
  50 & MDE.Phi.tv & sigma & beta=2.5 & sigma=1 & n=100 & 3.77 \\ 
  51 & MDE.Phi.kl & sigma & beta=2.5 & sigma=1 & n=100 & 1.51 \\ 
  52 & MME & sigma & beta=2.5 & sigma=1 & n=100 & 2.35 \\ 
  53 & MME.b & sigma & beta=2.5 & sigma=1 & n=100 & 4.03 \\ 
  54 & PWM & sigma & beta=2.5 & sigma=1 & n=100 & 1.36 \\ 
  55 & MLE & beta & beta=3 & sigma=1 & n=100 & 1592.97 \\ 
  56 & MLE.b & beta & beta=3 & sigma=1 & n=100 & 1592.48 \\ 
  57 & LME & beta & beta=3 & sigma=1 & n=100 & 4.01 \\ 
  58 & MDE.Phi.chisq & beta & beta=3 & sigma=1 & n=100 & 7.28 \\ 
  59 & MDE.Phi.tv & beta & beta=3 & sigma=1 & n=100 & 8.75 \\ 
  60 & MDE.Phi.kl & beta & beta=3 & sigma=1 & n=100 & 4.92 \\ 
  61 & MME & beta & beta=3 & sigma=1 & n=100 & 17.49 \\ 
  62 & MME.b & beta & beta=3 & sigma=1 & n=100 & 49.98 \\ 
  63 & PWM & beta & beta=3 & sigma=1 & n=100 & 4.01 \\ 
  64 & MLE & sigma & beta=3 & sigma=1 & n=100 & 672.84 \\ 
  65 & MLE.b & sigma & beta=3 & sigma=1 & n=100 & 672.63 \\ 
  66 & LME & sigma & beta=3 & sigma=1 & n=100 & 1.42 \\ 
  67 & MDE.Phi.chisq & sigma & beta=3 & sigma=1 & n=100 & 4.41 \\ 
  68 & MDE.Phi.tv & sigma & beta=3 & sigma=1 & n=100 & 5.17 \\ 
  69 & MDE.Phi.kl & sigma & beta=3 & sigma=1 & n=100 & 1.83 \\ 
  70 & MME & sigma & beta=3 & sigma=1 & n=100 & 6.74 \\ 
  71 & MME.b & sigma & beta=3 & sigma=1 & n=100 & 19.57 \\ 
  72 & PWM & sigma & beta=3 & sigma=1 & n=100 & 1.42 \\ 
  73 & MLE & beta & beta=4 & sigma=1 & n=100 & 229.86 \\ 
  74 & MLE.b & beta & beta=4 & sigma=1 & n=100 & 229.41 \\ 
  75 & LME & beta & beta=4 & sigma=1 & n=100 & 5.72 \\ 
  76 & MDE.Phi.chisq & beta & beta=4 & sigma=1 & n=100 & 14.91 \\ 
  77 & MDE.Phi.tv & beta & beta=4 & sigma=1 & n=100 & 17.26 \\ 
  78 & MDE.Phi.kl & beta & beta=4 & sigma=1 & n=100 & 7.52 \\ 
  79 & MME & beta & beta=4 & sigma=1 & n=100 & 11.35 \\ 
  80 & MME.b & beta & beta=4 & sigma=1 & n=100 & 40.89 \\ 
  81 & PWM & beta & beta=4 & sigma=1 & n=100 & 5.72 \\ 
  82 & MLE & sigma & beta=4 & sigma=1 & n=100 & 59.82 \\ 
  83 & MLE.b & sigma & beta=4 & sigma=1 & n=100 & 59.68 \\ 
  84 & LME & sigma & beta=4 & sigma=1 & n=100 & 1.52 \\ 
  85 & MDE.Phi.chisq & sigma & beta=4 & sigma=1 & n=100 & 6.42 \\ 
  86 & MDE.Phi.tv & sigma & beta=4 & sigma=1 & n=100 & 7.19 \\ 
  87 & MDE.Phi.kl & sigma & beta=4 & sigma=1 & n=100 & 2.09 \\ 
  88 & MME & sigma & beta=4 & sigma=1 & n=100 & 3.33 \\ 
  89 & MME.b & sigma & beta=4 & sigma=1 & n=100 & 13.43 \\ 
  90 & PWM & sigma & beta=4 & sigma=1 & n=100 & 1.52 \\ 
  91 & MLE & beta & beta=5 & sigma=1 & n=100 & 78.42 \\ 
  92 & MLE.b & beta & beta=5 & sigma=1 & n=100 & 78.05 \\ 
  93 & LME & beta & beta=5 & sigma=1 & n=100 & 7.32 \\ 
  94 & MDE.Phi.chisq & beta & beta=5 & sigma=1 & n=100 & 22.01 \\ 
  95 & MDE.Phi.tv & beta & beta=5 & sigma=1 & n=100 & 24.36 \\ 
  96 & MDE.Phi.kl & beta & beta=5 & sigma=1 & n=100 & 10.26 \\ 
  97 & MME & beta & beta=5 & sigma=1 & n=100 & 16.76 \\ 
  98 & MME.b & beta & beta=5 & sigma=1 & n=100 & 47.24 \\ 
  99 & PWM & beta & beta=5 & sigma=1 & n=100 & 7.32 \\ 
  100 & MLE & sigma & beta=5 & sigma=1 & n=100 & 18.74 \\ 
  101 & MLE.b & sigma & beta=5 & sigma=1 & n=100 & 18.66 \\ 
  102 & LME & sigma & beta=5 & sigma=1 & n=100 & 1.54 \\ 
  103 & MDE.Phi.chisq & sigma & beta=5 & sigma=1 & n=100 & 7.23 \\ 
  104 & MDE.Phi.tv & sigma & beta=5 & sigma=1 & n=100 & 7.77 \\ 
  105 & MDE.Phi.kl & sigma & beta=5 & sigma=1 & n=100 & 2.24 \\ 
  106 & MME & sigma & beta=5 & sigma=1 & n=100 & 3.76 \\ 
  107 & MME.b & sigma & beta=5 & sigma=1 & n=100 & 10.98 \\ 
  108 & PWM & sigma & beta=5 & sigma=1 & n=100 & 1.54 \\ 
  109 & MLE & beta & beta=1.5 & sigma=1 & n=200 & 1.58 \\ 
  110 & MLE.b & beta & beta=1.5 & sigma=1 & n=200 & 1.49 \\ 
  111 & LME & beta & beta=1.5 & sigma=1 & n=200 & 1.71 \\ 
  112 & MDE.Phi.chisq & beta & beta=1.5 & sigma=1 & n=200 & 0.86 \\ 
  113 & MDE.Phi.tv & beta & beta=1.5 & sigma=1 & n=200 & 1.01 \\ 
  114 & MDE.Phi.kl & beta & beta=1.5 & sigma=1 & n=200 & 1.58 \\ 
  115 & MME & beta & beta=1.5 & sigma=1 & n=200 & 2.51 \\ 
  116 & MME.b & beta & beta=1.5 & sigma=1 & n=200 & 2.31 \\ 
  117 & PWM & beta & beta=1.5 & sigma=1 & n=200 & 1.71 \\ 
  118 & MLE & sigma & beta=1.5 & sigma=1 & n=200 & 1.08 \\ 
  119 & MLE.b & sigma & beta=1.5 & sigma=1 & n=200 & 0.99 \\ 
  120 & LME & sigma & beta=1.5 & sigma=1 & n=200 & 1.21 \\ 
  121 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=1 & n=200 & 1.13 \\ 
  122 & MDE.Phi.tv & sigma & beta=1.5 & sigma=1 & n=200 & 1.26 \\ 
  123 & MDE.Phi.kl & sigma & beta=1.5 & sigma=1 & n=200 & 1.08 \\ 
  124 & MME & sigma & beta=1.5 & sigma=1 & n=200 & 2.80 \\ 
  125 & MME.b & sigma & beta=1.5 & sigma=1 & n=200 & 2.53 \\ 
  126 & PWM & sigma & beta=1.5 & sigma=1 & n=200 & 1.21 \\ 
  127 & MLE & beta & beta=2 & sigma=1 & n=200 & 2.15 \\ 
  128 & MLE.b & beta & beta=2 & sigma=1 & n=200 & 1.98 \\ 
  129 & LME & beta & beta=2 & sigma=1 & n=200 & 2.23 \\ 
  130 & MDE.Phi.chisq & beta & beta=2 & sigma=1 & n=200 & 1.35 \\ 
  131 & MDE.Phi.tv & beta & beta=2 & sigma=1 & n=200 & 1.57 \\ 
  132 & MDE.Phi.kl & beta & beta=2 & sigma=1 & n=200 & 2.15 \\ 
  133 & MME & beta & beta=2 & sigma=1 & n=200 & 2.98 \\ 
  134 & MME.b & beta & beta=2 & sigma=1 & n=200 & 2.65 \\ 
  135 & PWM & beta & beta=2 & sigma=1 & n=200 & 2.23 \\ 
  136 & MLE & sigma & beta=2 & sigma=1 & n=200 & 1.11 \\ 
  137 & MLE.b & sigma & beta=2 & sigma=1 & n=200 & 0.99 \\ 
  138 & LME & sigma & beta=2 & sigma=1 & n=200 & 1.15 \\ 
  139 & MDE.Phi.chisq & sigma & beta=2 & sigma=1 & n=200 & 1.17 \\ 
  140 & MDE.Phi.tv & sigma & beta=2 & sigma=1 & n=200 & 1.28 \\ 
  141 & MDE.Phi.kl & sigma & beta=2 & sigma=1 & n=200 & 1.11 \\ 
  142 & MME & sigma & beta=2 & sigma=1 & n=200 & 1.90 \\ 
  143 & MME.b & sigma & beta=2 & sigma=1 & n=200 & 1.63 \\ 
  144 & PWM & sigma & beta=2 & sigma=1 & n=200 & 1.15 \\ 
  145 & MLE & beta & beta=2.5 & sigma=1 & n=200 & 2.79 \\ 
  146 & MLE.b & beta & beta=2.5 & sigma=1 & n=200 & 2.48 \\ 
  147 & LME & beta & beta=2.5 & sigma=1 & n=200 & 2.81 \\ 
  148 & MDE.Phi.chisq & beta & beta=2.5 & sigma=1 & n=200 & 2.09 \\ 
  149 & MDE.Phi.tv & beta & beta=2.5 & sigma=1 & n=200 & 2.28 \\ 
  150 & MDE.Phi.kl & beta & beta=2.5 & sigma=1 & n=200 & 2.79 \\ 
  151 & MME & beta & beta=2.5 & sigma=1 & n=200 & 3.61 \\ 
  152 & MME.b & beta & beta=2.5 & sigma=1 & n=200 & 3.65 \\ 
  153 & PWM & beta & beta=2.5 & sigma=1 & n=200 & 2.81 \\ 
  154 & MLE & sigma & beta=2.5 & sigma=1 & n=200 & 1.15 \\ 
  155 & MLE.b & sigma & beta=2.5 & sigma=1 & n=200 & 0.99 \\ 
  156 & LME & sigma & beta=2.5 & sigma=1 & n=200 & 1.16 \\ 
  157 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=1 & n=200 & 1.38 \\ 
  158 & MDE.Phi.tv & sigma & beta=2.5 & sigma=1 & n=200 & 1.41 \\ 
  159 & MDE.Phi.kl & sigma & beta=2.5 & sigma=1 & n=200 & 1.15 \\ 
  160 & MME & sigma & beta=2.5 & sigma=1 & n=200 & 1.68 \\ 
  161 & MME.b & sigma & beta=2.5 & sigma=1 & n=200 & 1.70 \\ 
  162 & PWM & sigma & beta=2.5 & sigma=1 & n=200 & 1.16 \\ 
  163 & MLE & beta & beta=3 & sigma=1 & n=200 & 3.45 \\ 
  164 & MLE.b & beta & beta=3 & sigma=1 & n=200 & 2.99 \\ 
  165 & LME & beta & beta=3 & sigma=1 & n=200 & 3.41 \\ 
  166 & MDE.Phi.chisq & beta & beta=3 & sigma=1 & n=200 & 3.30 \\ 
  167 & MDE.Phi.tv & beta & beta=3 & sigma=1 & n=200 & 3.42 \\ 
  168 & MDE.Phi.kl & beta & beta=3 & sigma=1 & n=200 & 3.45 \\ 
  169 & MME & beta & beta=3 & sigma=1 & n=200 & 4.32 \\ 
  170 & MME.b & beta & beta=3 & sigma=1 & n=200 & 4.89 \\ 
  171 & PWM & beta & beta=3 & sigma=1 & n=200 & 3.41 \\ 
  172 & MLE & sigma & beta=3 & sigma=1 & n=200 & 1.20 \\ 
  173 & MLE.b & sigma & beta=3 & sigma=1 & n=200 & 1.00 \\ 
  174 & LME & sigma & beta=3 & sigma=1 & n=200 & 1.17 \\ 
  175 & MDE.Phi.chisq & sigma & beta=3 & sigma=1 & n=200 & 1.77 \\ 
  176 & MDE.Phi.tv & sigma & beta=3 & sigma=1 & n=200 & 1.72 \\ 
  177 & MDE.Phi.kl & sigma & beta=3 & sigma=1 & n=200 & 1.20 \\ 
  178 & MME & sigma & beta=3 & sigma=1 & n=200 & 1.61 \\ 
  179 & MME.b & sigma & beta=3 & sigma=1 & n=200 & 1.84 \\ 
  180 & PWM & sigma & beta=3 & sigma=1 & n=200 & 1.17 \\ 
  181 & MLE & beta & beta=4 & sigma=1 & n=200 & 29.96 \\ 
  182 & MLE.b & beta & beta=4 & sigma=1 & n=200 & 29.30 \\ 
  183 & LME & beta & beta=4 & sigma=1 & n=200 & 4.87 \\ 
  184 & MDE.Phi.chisq & beta & beta=4 & sigma=1 & n=200 & 8.33 \\ 
  185 & MDE.Phi.tv & beta & beta=4 & sigma=1 & n=200 & 7.13 \\ 
  186 & MDE.Phi.kl & beta & beta=4 & sigma=1 & n=200 & 5.46 \\ 
  187 & MME & beta & beta=4 & sigma=1 & n=200 & 7.01 \\ 
  188 & MME.b & beta & beta=4 & sigma=1 & n=200 & 12.15 \\ 
  189 & PWM & beta & beta=4 & sigma=1 & n=200 & 4.87 \\ 
  190 & MLE & sigma & beta=4 & sigma=1 & n=200 & 8.83 \\ 
  191 & MLE.b & sigma & beta=4 & sigma=1 & n=200 & 8.63 \\ 
  192 & LME & sigma & beta=4 & sigma=1 & n=200 & 1.26 \\ 
  193 & MDE.Phi.chisq & sigma & beta=4 & sigma=1 & n=200 & 3.24 \\ 
  194 & MDE.Phi.tv & sigma & beta=4 & sigma=1 & n=200 & 2.62 \\ 
  195 & MDE.Phi.kl & sigma & beta=4 & sigma=1 & n=200 & 1.44 \\ 
  196 & MME & sigma & beta=4 & sigma=1 & n=200 & 1.94 \\ 
  197 & MME.b & sigma & beta=4 & sigma=1 & n=200 & 3.54 \\ 
  198 & PWM & sigma & beta=4 & sigma=1 & n=200 & 1.26 \\ 
  199 & MLE & beta & beta=5 & sigma=1 & n=200 & 44.55 \\ 
  200 & MLE.b & beta & beta=5 & sigma=1 & n=200 & 43.83 \\ 
  201 & LME & beta & beta=5 & sigma=1 & n=200 & 6.69 \\ 
  202 & MDE.Phi.chisq & beta & beta=5 & sigma=1 & n=200 & 15.43 \\ 
  203 & MDE.Phi.tv & beta & beta=5 & sigma=1 & n=200 & 12.14 \\ 
  204 & MDE.Phi.kl & beta & beta=5 & sigma=1 & n=200 & 7.72 \\ 
  205 & MME & beta & beta=5 & sigma=1 & n=200 & 16.16 \\ 
  206 & MME.b & beta & beta=5 & sigma=1 & n=200 & 39.22 \\ 
  207 & PWM & beta & beta=5 & sigma=1 & n=200 & 6.69 \\ 
  208 & MLE & sigma & beta=5 & sigma=1 & n=200 & 10.76 \\ 
  209 & MLE.b & sigma & beta=5 & sigma=1 & n=200 & 10.59 \\ 
  210 & LME & sigma & beta=5 & sigma=1 & n=200 & 1.40 \\ 
  211 & MDE.Phi.chisq & sigma & beta=5 & sigma=1 & n=200 & 4.68 \\ 
  212 & MDE.Phi.tv & sigma & beta=5 & sigma=1 & n=200 & 3.49 \\ 
  213 & MDE.Phi.kl & sigma & beta=5 & sigma=1 & n=200 & 1.64 \\ 
  214 & MME & sigma & beta=5 & sigma=1 & n=200 & 3.66 \\ 
  215 & MME.b & sigma & beta=5 & sigma=1 & n=200 & 9.27 \\ 
  216 & PWM & sigma & beta=5 & sigma=1 & n=200 & 1.40 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220130/Output.mse.LaTeX.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Sun Jan 30 20:11:05 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=1 & n=100 & 0.46 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=1 & n=100 & 0.32 \\ 
  3 & LME & beta & beta=1.5 & sigma=1 & n=100 & 0.40 \\ 
  4 & MDE.Phi.chisq & beta & beta=1.5 & sigma=1 & n=100 & 12.92 \\ 
  5 & MDE.Phi.tv & beta & beta=1.5 & sigma=1 & n=100 & 8.13 \\ 
  6 & MDE.Phi.kl & beta & beta=1.5 & sigma=1 & n=100 & 0.46 \\ 
  7 & MME & beta & beta=1.5 & sigma=1 & n=100 & 2.57 \\ 
  8 & MME.b & beta & beta=1.5 & sigma=1 & n=100 & 130057.25 \\ 
  9 & PWM & beta & beta=1.5 & sigma=1 & n=100 & 0.40 \\ 
  10 & MLE & sigma & beta=1.5 & sigma=1 & n=100 & 0.52 \\ 
  11 & MLE.b & sigma & beta=1.5 & sigma=1 & n=100 & 0.36 \\ 
  12 & LME & sigma & beta=1.5 & sigma=1 & n=100 & 0.44 \\ 
  13 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=1 & n=100 & 22.40 \\ 
  14 & MDE.Phi.tv & sigma & beta=1.5 & sigma=1 & n=100 & 21.81 \\ 
  15 & MDE.Phi.kl & sigma & beta=1.5 & sigma=1 & n=100 & 0.52 \\ 
  16 & MME & sigma & beta=1.5 & sigma=1 & n=100 & 6.62 \\ 
  17 & MME.b & sigma & beta=1.5 & sigma=1 & n=100 & 148910.23 \\ 
  18 & PWM & sigma & beta=1.5 & sigma=1 & n=100 & 0.44 \\ 
  19 & MLE & beta & beta=2 & sigma=1 & n=100 & 218.70 \\ 
  20 & MLE.b & beta & beta=2 & sigma=1 & n=100 & 218.45 \\ 
  21 & LME & beta & beta=2 & sigma=1 & n=100 & 3.31 \\ 
  22 & MDE.Phi.chisq & beta & beta=2 & sigma=1 & n=100 & 79.26 \\ 
  23 & MDE.Phi.tv & beta & beta=2 & sigma=1 & n=100 & 107.06 \\ 
  24 & MDE.Phi.kl & beta & beta=2 & sigma=1 & n=100 & 14.38 \\ 
  25 & MME & beta & beta=2 & sigma=1 & n=100 & 55.69 \\ 
  26 & MME.b & beta & beta=2 & sigma=1 & n=100 & 151259.47 \\ 
  27 & PWM & beta & beta=2 & sigma=1 & n=100 & 3.31 \\ 
  28 & MLE & sigma & beta=2 & sigma=1 & n=100 & 73.54 \\ 
  29 & MLE.b & sigma & beta=2 & sigma=1 & n=100 & 73.40 \\ 
  30 & LME & sigma & beta=2 & sigma=1 & n=100 & 1.54 \\ 
  31 & MDE.Phi.chisq & sigma & beta=2 & sigma=1 & n=100 & 91.74 \\ 
  32 & MDE.Phi.tv & sigma & beta=2 & sigma=1 & n=100 & 118.22 \\ 
  33 & MDE.Phi.kl & sigma & beta=2 & sigma=1 & n=100 & 6.02 \\ 
  34 & MME & sigma & beta=2 & sigma=1 & n=100 & 24.92 \\ 
  35 & MME.b & sigma & beta=2 & sigma=1 & n=100 & 83571.71 \\ 
  36 & PWM & sigma & beta=2 & sigma=1 & n=100 & 1.54 \\ 
  37 & MLE & beta & beta=2.5 & sigma=1 & n=100 & 44301.24 \\ 
  38 & MLE.b & beta & beta=2.5 & sigma=1 & n=100 & 44301.12 \\ 
  39 & LME & beta & beta=2.5 & sigma=1 & n=100 & 8.66 \\ 
  40 & MDE.Phi.chisq & beta & beta=2.5 & sigma=1 & n=100 & 282.04 \\ 
  41 & MDE.Phi.tv & beta & beta=2.5 & sigma=1 & n=100 & 323.23 \\ 
  42 & MDE.Phi.kl & beta & beta=2.5 & sigma=1 & n=100 & 34.92 \\ 
  43 & MME & beta & beta=2.5 & sigma=1 & n=100 & 149.67 \\ 
  44 & MME.b & beta & beta=2.5 & sigma=1 & n=100 & 2244.42 \\ 
  45 & PWM & beta & beta=2.5 & sigma=1 & n=100 & 8.66 \\ 
  46 & MLE & sigma & beta=2.5 & sigma=1 & n=100 & 15074.75 \\ 
  47 & MLE.b & sigma & beta=2.5 & sigma=1 & n=100 & 15074.71 \\ 
  48 & LME & sigma & beta=2.5 & sigma=1 & n=100 & 2.34 \\ 
  49 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=1 & n=100 & 171.83 \\ 
  50 & MDE.Phi.tv & sigma & beta=2.5 & sigma=1 & n=100 & 195.88 \\ 
  51 & MDE.Phi.kl & sigma & beta=2.5 & sigma=1 & n=100 & 9.57 \\ 
  52 & MME & sigma & beta=2.5 & sigma=1 & n=100 & 39.37 \\ 
  53 & MME.b & sigma & beta=2.5 & sigma=1 & n=100 & 640.84 \\ 
  54 & PWM & sigma & beta=2.5 & sigma=1 & n=100 & 2.34 \\ 
  55 & MLE & beta & beta=3 & sigma=1 & n=100 & 16311601689.39 \\ 
  56 & MLE.b & beta & beta=3 & sigma=1 & n=100 & 16311601689.60 \\ 
  57 & LME & beta & beta=3 & sigma=1 & n=100 & 16.41 \\ 
  58 & MDE.Phi.chisq & beta & beta=3 & sigma=1 & n=100 & 624.42 \\ 
  59 & MDE.Phi.tv & beta & beta=3 & sigma=1 & n=100 & 753.90 \\ 
  60 & MDE.Phi.kl & beta & beta=3 & sigma=1 & n=100 & 123.92 \\ 
  61 & MME & beta & beta=3 & sigma=1 & n=100 & 313324.90 \\ 
  62 & MME.b & beta & beta=3 & sigma=1 & n=100 & 2979285.35 \\ 
  63 & PWM & beta & beta=3 & sigma=1 & n=100 & 16.41 \\ 
  64 & MLE & sigma & beta=3 & sigma=1 & n=100 & 2958678679.22 \\ 
  65 & MLE.b & sigma & beta=3 & sigma=1 & n=100 & 2958678679.25 \\ 
  66 & LME & sigma & beta=3 & sigma=1 & n=100 & 3.12 \\ 
  67 & MDE.Phi.chisq & sigma & beta=3 & sigma=1 & n=100 & 249.86 \\ 
  68 & MDE.Phi.tv & sigma & beta=3 & sigma=1 & n=100 & 294.28 \\ 
  69 & MDE.Phi.kl & sigma & beta=3 & sigma=1 & n=100 & 22.94 \\ 
  70 & MME & sigma & beta=3 & sigma=1 & n=100 & 45240.03 \\ 
  71 & MME.b & sigma & beta=3 & sigma=1 & n=100 & 430647.87 \\ 
  72 & PWM & sigma & beta=3 & sigma=1 & n=100 & 3.12 \\ 
  73 & MLE & beta & beta=4 & sigma=1 & n=100 & 198946221.76 \\ 
  74 & MLE.b & beta & beta=4 & sigma=1 & n=100 & 198946222.69 \\ 
  75 & LME & beta & beta=4 & sigma=1 & n=100 & 48.61 \\ 
  76 & MDE.Phi.chisq & beta & beta=4 & sigma=1 & n=100 & 1636.38 \\ 
  77 & MDE.Phi.tv & beta & beta=4 & sigma=1 & n=100 & 1914.43 \\ 
  78 & MDE.Phi.kl & beta & beta=4 & sigma=1 & n=100 & 244.45 \\ 
  79 & MME & beta & beta=4 & sigma=1 & n=100 & 11609.79 \\ 
  80 & MME.b & beta & beta=4 & sigma=1 & n=100 & 1922330.29 \\ 
  81 & PWM & beta & beta=4 & sigma=1 & n=100 & 48.61 \\ 
  82 & MLE & sigma & beta=4 & sigma=1 & n=100 & 12512843.80 \\ 
  83 & MLE.b & sigma & beta=4 & sigma=1 & n=100 & 12512843.88 \\ 
  84 & LME & sigma & beta=4 & sigma=1 & n=100 & 4.67 \\ 
  85 & MDE.Phi.chisq & sigma & beta=4 & sigma=1 & n=100 & 323.35 \\ 
  86 & MDE.Phi.tv & sigma & beta=4 & sigma=1 & n=100 & 358.21 \\ 
  87 & MDE.Phi.kl & sigma & beta=4 & sigma=1 & n=100 & 24.26 \\ 
  88 & MME & sigma & beta=4 & sigma=1 & n=100 & 1091.87 \\ 
  89 & MME.b & sigma & beta=4 & sigma=1 & n=100 & 270680.38 \\ 
  90 & PWM & sigma & beta=4 & sigma=1 & n=100 & 4.67 \\ 
  91 & MLE & beta & beta=5 & sigma=1 & n=100 & 4842613.63 \\ 
  92 & MLE.b & beta & beta=5 & sigma=1 & n=100 & 4842615.06 \\ 
  93 & LME & beta & beta=5 & sigma=1 & n=100 & 101.29 \\ 
  94 & MDE.Phi.chisq & beta & beta=5 & sigma=1 & n=100 & 2696.04 \\ 
  95 & MDE.Phi.tv & beta & beta=5 & sigma=1 & n=100 & 2969.74 \\ 
  96 & MDE.Phi.kl & beta & beta=5 & sigma=1 & n=100 & 437.96 \\ 
  97 & MME & beta & beta=5 & sigma=1 & n=100 & 18732.37 \\ 
  98 & MME.b & beta & beta=5 & sigma=1 & n=100 & 259630.47 \\ 
  99 & PWM & beta & beta=5 & sigma=1 & n=100 & 101.29 \\ 
  100 & MLE & sigma & beta=5 & sigma=1 & n=100 & 278599.17 \\ 
  101 & MLE.b & sigma & beta=5 & sigma=1 & n=100 & 278599.25 \\ 
  102 & LME & sigma & beta=5 & sigma=1 & n=100 & 5.63 \\ 
  103 & MDE.Phi.chisq & sigma & beta=5 & sigma=1 & n=100 & 307.71 \\ 
  104 & MDE.Phi.tv & sigma & beta=5 & sigma=1 & n=100 & 323.90 \\ 
  105 & MDE.Phi.kl & sigma & beta=5 & sigma=1 & n=100 & 24.12 \\ 
  106 & MME & sigma & beta=5 & sigma=1 & n=100 & 1044.66 \\ 
  107 & MME.b & sigma & beta=5 & sigma=1 & n=100 & 15546.21 \\ 
  108 & PWM & sigma & beta=5 & sigma=1 & n=100 & 5.63 \\ 
  109 & MLE & beta & beta=1.5 & sigma=1 & n=200 & 0.11 \\ 
  110 & MLE.b & beta & beta=1.5 & sigma=1 & n=200 & 0.08 \\ 
  111 & LME & beta & beta=1.5 & sigma=1 & n=200 & 0.16 \\ 
  112 & MDE.Phi.chisq & beta & beta=1.5 & sigma=1 & n=200 & 0.54 \\ 
  113 & MDE.Phi.tv & beta & beta=1.5 & sigma=1 & n=200 & 0.41 \\ 
  114 & MDE.Phi.kl & beta & beta=1.5 & sigma=1 & n=200 & 0.11 \\ 
  115 & MME & beta & beta=1.5 & sigma=1 & n=200 & 1.19 \\ 
  116 & MME.b & beta & beta=1.5 & sigma=1 & n=200 & 0.84 \\ 
  117 & PWM & beta & beta=1.5 & sigma=1 & n=200 & 0.16 \\ 
  118 & MLE & sigma & beta=1.5 & sigma=1 & n=200 & 0.12 \\ 
  119 & MLE.b & sigma & beta=1.5 & sigma=1 & n=200 & 0.08 \\ 
  120 & LME & sigma & beta=1.5 & sigma=1 & n=200 & 0.17 \\ 
  121 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=1 & n=200 & 0.25 \\ 
  122 & MDE.Phi.tv & sigma & beta=1.5 & sigma=1 & n=200 & 0.36 \\ 
  123 & MDE.Phi.kl & sigma & beta=1.5 & sigma=1 & n=200 & 0.12 \\ 
  124 & MME & sigma & beta=1.5 & sigma=1 & n=200 & 8.69 \\ 
  125 & MME.b & sigma & beta=1.5 & sigma=1 & n=200 & 7.91 \\ 
  126 & PWM & sigma & beta=1.5 & sigma=1 & n=200 & 0.17 \\ 
  127 & MLE & beta & beta=2 & sigma=1 & n=200 & 0.37 \\ 
  128 & MLE.b & beta & beta=2 & sigma=1 & n=200 & 0.22 \\ 
  129 & LME & beta & beta=2 & sigma=1 & n=200 & 0.37 \\ 
  130 & MDE.Phi.chisq & beta & beta=2 & sigma=1 & n=200 & 1.05 \\ 
  131 & MDE.Phi.tv & beta & beta=2 & sigma=1 & n=200 & 1.12 \\ 
  132 & MDE.Phi.kl & beta & beta=2 & sigma=1 & n=200 & 0.37 \\ 
  133 & MME & beta & beta=2 & sigma=1 & n=200 & 1.56 \\ 
  134 & MME.b & beta & beta=2 & sigma=1 & n=200 & 2.64 \\ 
  135 & PWM & beta & beta=2 & sigma=1 & n=200 & 0.37 \\ 
  136 & MLE & sigma & beta=2 & sigma=1 & n=200 & 0.18 \\ 
  137 & MLE.b & sigma & beta=2 & sigma=1 & n=200 & 0.11 \\ 
  138 & LME & sigma & beta=2 & sigma=1 & n=200 & 0.18 \\ 
  139 & MDE.Phi.chisq & sigma & beta=2 & sigma=1 & n=200 & 0.56 \\ 
  140 & MDE.Phi.tv & sigma & beta=2 & sigma=1 & n=200 & 0.90 \\ 
  141 & MDE.Phi.kl & sigma & beta=2 & sigma=1 & n=200 & 0.18 \\ 
  142 & MME & sigma & beta=2 & sigma=1 & n=200 & 1.13 \\ 
  143 & MME.b & sigma & beta=2 & sigma=1 & n=200 & 2.06 \\ 
  144 & PWM & sigma & beta=2 & sigma=1 & n=200 & 0.18 \\ 
  145 & MLE & beta & beta=2.5 & sigma=1 & n=200 & 3.41 \\ 
  146 & MLE.b & beta & beta=2.5 & sigma=1 & n=200 & 3.04 \\ 
  147 & LME & beta & beta=2.5 & sigma=1 & n=200 & 2.24 \\ 
  148 & MDE.Phi.chisq & beta & beta=2.5 & sigma=1 & n=200 & 19.22 \\ 
  149 & MDE.Phi.tv & beta & beta=2.5 & sigma=1 & n=200 & 14.00 \\ 
  150 & MDE.Phi.kl & beta & beta=2.5 & sigma=1 & n=200 & 3.39 \\ 
  151 & MME & beta & beta=2.5 & sigma=1 & n=200 & 6.90 \\ 
  152 & MME.b & beta & beta=2.5 & sigma=1 & n=200 & 164.99 \\ 
  153 & PWM & beta & beta=2.5 & sigma=1 & n=200 & 2.24 \\ 
  154 & MLE & sigma & beta=2.5 & sigma=1 & n=200 & 1.05 \\ 
  155 & MLE.b & sigma & beta=2.5 & sigma=1 & n=200 & 0.94 \\ 
  156 & LME & sigma & beta=2.5 & sigma=1 & n=200 & 0.60 \\ 
  157 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=1 & n=200 & 9.84 \\ 
  158 & MDE.Phi.tv & sigma & beta=2.5 & sigma=1 & n=200 & 7.18 \\ 
  159 & MDE.Phi.kl & sigma & beta=2.5 & sigma=1 & n=200 & 1.04 \\ 
  160 & MME & sigma & beta=2.5 & sigma=1 & n=200 & 2.20 \\ 
  161 & MME.b & sigma & beta=2.5 & sigma=1 & n=200 & 55.58 \\ 
  162 & PWM & sigma & beta=2.5 & sigma=1 & n=200 & 0.60 \\ 
  163 & MLE & beta & beta=3 & sigma=1 & n=200 & 5.08 \\ 
  164 & MLE.b & beta & beta=3 & sigma=1 & n=200 & 4.54 \\ 
  165 & LME & beta & beta=3 & sigma=1 & n=200 & 3.45 \\ 
  166 & MDE.Phi.chisq & beta & beta=3 & sigma=1 & n=200 & 95.73 \\ 
  167 & MDE.Phi.tv & beta & beta=3 & sigma=1 & n=200 & 82.65 \\ 
  168 & MDE.Phi.kl & beta & beta=3 & sigma=1 & n=200 & 5.31 \\ 
  169 & MME & beta & beta=3 & sigma=1 & n=200 & 8.87 \\ 
  170 & MME.b & beta & beta=3 & sigma=1 & n=200 & 453.88 \\ 
  171 & PWM & beta & beta=3 & sigma=1 & n=200 & 3.45 \\ 
  172 & MLE & sigma & beta=3 & sigma=1 & n=200 & 0.91 \\ 
  173 & MLE.b & sigma & beta=3 & sigma=1 & n=200 & 0.81 \\ 
  174 & LME & sigma & beta=3 & sigma=1 & n=200 & 0.58 \\ 
  175 & MDE.Phi.chisq & sigma & beta=3 & sigma=1 & n=200 & 32.70 \\ 
  176 & MDE.Phi.tv & sigma & beta=3 & sigma=1 & n=200 & 26.31 \\ 
  177 & MDE.Phi.kl & sigma & beta=3 & sigma=1 & n=200 & 0.95 \\ 
  178 & MME & sigma & beta=3 & sigma=1 & n=200 & 1.68 \\ 
  179 & MME.b & sigma & beta=3 & sigma=1 & n=200 & 84.08 \\ 
  180 & PWM & sigma & beta=3 & sigma=1 & n=200 & 0.58 \\ 
  181 & MLE & beta & beta=4 & sigma=1 & n=200 & 2427316.56 \\ 
  182 & MLE.b & beta & beta=4 & sigma=1 & n=200 & 2427316.39 \\ 
  183 & LME & beta & beta=4 & sigma=1 & n=200 & 15.40 \\ 
  184 & MDE.Phi.chisq & beta & beta=4 & sigma=1 & n=200 & 652.55 \\ 
  185 & MDE.Phi.tv & beta & beta=4 & sigma=1 & n=200 & 432.08 \\ 
  186 & MDE.Phi.kl & beta & beta=4 & sigma=1 & n=200 & 80.46 \\ 
  187 & MME & beta & beta=4 & sigma=1 & n=200 & 1492.95 \\ 
  188 & MME.b & beta & beta=4 & sigma=1 & n=200 & 10651.49 \\ 
  189 & PWM & beta & beta=4 & sigma=1 & n=200 & 15.40 \\ 
  190 & MLE & sigma & beta=4 & sigma=1 & n=200 & 226023.99 \\ 
  191 & MLE.b & sigma & beta=4 & sigma=1 & n=200 & 226023.97 \\ 
  192 & LME & sigma & beta=4 & sigma=1 & n=200 & 1.40 \\ 
  193 & MDE.Phi.chisq & sigma & beta=4 & sigma=1 & n=200 & 107.34 \\ 
  194 & MDE.Phi.tv & sigma & beta=4 & sigma=1 & n=200 & 67.65 \\ 
  195 & MDE.Phi.kl & sigma & beta=4 & sigma=1 & n=200 & 7.40 \\ 
  196 & MME & sigma & beta=4 & sigma=1 & n=200 & 138.68 \\ 
  197 & MME.b & sigma & beta=4 & sigma=1 & n=200 & 1087.07 \\ 
  198 & PWM & sigma & beta=4 & sigma=1 & n=200 & 1.40 \\ 
  199 & MLE & beta & beta=5 & sigma=1 & n=200 & 6973990.32 \\ 
  200 & MLE.b & beta & beta=5 & sigma=1 & n=200 & 6973991.17 \\ 
  201 & LME & beta & beta=5 & sigma=1 & n=200 & 57.29 \\ 
  202 & MDE.Phi.chisq & beta & beta=5 & sigma=1 & n=200 & 1593.24 \\ 
  203 & MDE.Phi.tv & beta & beta=5 & sigma=1 & n=200 & 1025.23 \\ 
  204 & MDE.Phi.kl & beta & beta=5 & sigma=1 & n=200 & 187.07 \\ 
  205 & MME & beta & beta=5 & sigma=1 & n=200 & 352371.74 \\ 
  206 & MME.b & beta & beta=5 & sigma=1 & n=200 & 1490156.97 \\ 
  207 & PWM & beta & beta=5 & sigma=1 & n=200 & 57.29 \\ 
  208 & MLE & sigma & beta=5 & sigma=1 & n=200 & 441117.88 \\ 
  209 & MLE.b & sigma & beta=5 & sigma=1 & n=200 & 441117.92 \\ 
  210 & LME & sigma & beta=5 & sigma=1 & n=200 & 3.31 \\ 
  211 & MDE.Phi.chisq & sigma & beta=5 & sigma=1 & n=200 & 155.80 \\ 
  212 & MDE.Phi.tv & sigma & beta=5 & sigma=1 & n=200 & 94.29 \\ 
  213 & MDE.Phi.kl & sigma & beta=5 & sigma=1 & n=200 & 10.20 \\ 
  214 & MME & sigma & beta=5 & sigma=1 & n=200 & 19955.18 \\ 
  215 & MME.b & sigma & beta=5 & sigma=1 & n=200 & 85271.49 \\ 
  216 & PWM & sigma & beta=5 & sigma=1 & n=200 & 3.31 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220130/Output.var.LaTeX.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Sun Jan 30 20:11:05 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=1 & n=100 & 0.43 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=1 & n=100 & 0.32 \\ 
  3 & LME & beta & beta=1.5 & sigma=1 & n=100 & 0.30 \\ 
  4 & MDE.Phi.chisq & beta & beta=1.5 & sigma=1 & n=100 & 12.66 \\ 
  5 & MDE.Phi.tv & beta & beta=1.5 & sigma=1 & n=100 & 8.07 \\ 
  6 & MDE.Phi.kl & beta & beta=1.5 & sigma=1 & n=100 & 0.44 \\ 
  7 & MME & beta & beta=1.5 & sigma=1 & n=100 & 0.90 \\ 
  8 & MME.b & beta & beta=1.5 & sigma=1 & n=100 & 130047.07 \\ 
  9 & PWM & beta & beta=1.5 & sigma=1 & n=100 & 0.30 \\ 
  10 & MLE & sigma & beta=1.5 & sigma=1 & n=100 & 0.49 \\ 
  11 & MLE.b & sigma & beta=1.5 & sigma=1 & n=100 & 0.36 \\ 
  12 & LME & sigma & beta=1.5 & sigma=1 & n=100 & 0.33 \\ 
  13 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=1 & n=100 & 22.10 \\ 
  14 & MDE.Phi.tv & sigma & beta=1.5 & sigma=1 & n=100 & 21.12 \\ 
  15 & MDE.Phi.kl & sigma & beta=1.5 & sigma=1 & n=100 & 0.49 \\ 
  16 & MME & sigma & beta=1.5 & sigma=1 & n=100 & 1.99 \\ 
  17 & MME.b & sigma & beta=1.5 & sigma=1 & n=100 & 148891.08 \\ 
  18 & PWM & sigma & beta=1.5 & sigma=1 & n=100 & 0.33 \\ 
  19 & MLE & beta & beta=2 & sigma=1 & n=100 & 218.33 \\ 
  20 & MLE.b & beta & beta=2 & sigma=1 & n=100 & 218.39 \\ 
  21 & LME & beta & beta=2 & sigma=1 & n=100 & 3.11 \\ 
  22 & MDE.Phi.chisq & beta & beta=2 & sigma=1 & n=100 & 79.25 \\ 
  23 & MDE.Phi.tv & beta & beta=2 & sigma=1 & n=100 & 106.49 \\ 
  24 & MDE.Phi.kl & beta & beta=2 & sigma=1 & n=100 & 14.17 \\ 
  25 & MME & beta & beta=2 & sigma=1 & n=100 & 52.88 \\ 
  26 & MME.b & beta & beta=2 & sigma=1 & n=100 & 151218.71 \\ 
  27 & PWM & beta & beta=2 & sigma=1 & n=100 & 3.11 \\ 
  28 & MLE & sigma & beta=2 & sigma=1 & n=100 & 73.37 \\ 
  29 & MLE.b & sigma & beta=2 & sigma=1 & n=100 & 73.38 \\ 
  30 & LME & sigma & beta=2 & sigma=1 & n=100 & 1.45 \\ 
  31 & MDE.Phi.chisq & sigma & beta=2 & sigma=1 & n=100 & 90.42 \\ 
  32 & MDE.Phi.tv & sigma & beta=2 & sigma=1 & n=100 & 115.40 \\ 
  33 & MDE.Phi.kl & sigma & beta=2 & sigma=1 & n=100 & 5.92 \\ 
  34 & MME & sigma & beta=2 & sigma=1 & n=100 & 22.85 \\ 
  35 & MME.b & sigma & beta=2 & sigma=1 & n=100 & 83548.85 \\ 
  36 & PWM & sigma & beta=2 & sigma=1 & n=100 & 1.45 \\ 
  37 & MLE & beta & beta=2.5 & sigma=1 & n=100 & 44295.07 \\ 
  38 & MLE.b & beta & beta=2.5 & sigma=1 & n=100 & 44297.71 \\ 
  39 & LME & beta & beta=2.5 & sigma=1 & n=100 & 8.18 \\ 
  40 & MDE.Phi.chisq & beta & beta=2.5 & sigma=1 & n=100 & 278.80 \\ 
  41 & MDE.Phi.tv & beta & beta=2.5 & sigma=1 & n=100 & 316.25 \\ 
  42 & MDE.Phi.kl & beta & beta=2.5 & sigma=1 & n=100 & 34.02 \\ 
  43 & MME & beta & beta=2.5 & sigma=1 & n=100 & 144.30 \\ 
  44 & MME.b & beta & beta=2.5 & sigma=1 & n=100 & 2214.15 \\ 
  45 & PWM & beta & beta=2.5 & sigma=1 & n=100 & 8.18 \\ 
  46 & MLE & sigma & beta=2.5 & sigma=1 & n=100 & 15072.88 \\ 
  47 & MLE.b & sigma & beta=2.5 & sigma=1 & n=100 & 15073.68 \\ 
  48 & LME & sigma & beta=2.5 & sigma=1 & n=100 & 2.22 \\ 
  49 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=1 & n=100 & 166.88 \\ 
  50 & MDE.Phi.tv & sigma & beta=2.5 & sigma=1 & n=100 & 188.25 \\ 
  51 & MDE.Phi.kl & sigma & beta=2.5 & sigma=1 & n=100 & 9.31 \\ 
  52 & MME & sigma & beta=2.5 & sigma=1 & n=100 & 37.53 \\ 
  53 & MME.b & sigma & beta=2.5 & sigma=1 & n=100 & 631.70 \\ 
  54 & PWM & sigma & beta=2.5 & sigma=1 & n=100 & 2.22 \\ 
  55 & MLE & beta & beta=3 & sigma=1 & n=100 & 16310704747.41 \\ 
  56 & MLE.b & beta & beta=3 & sigma=1 & n=100 & 16310706319.43 \\ 
  57 & LME & beta & beta=3 & sigma=1 & n=100 & 15.40 \\ 
  58 & MDE.Phi.chisq & beta & beta=3 & sigma=1 & n=100 & 606.18 \\ 
  59 & MDE.Phi.tv & beta & beta=3 & sigma=1 & n=100 & 720.89 \\ 
  60 & MDE.Phi.kl & beta & beta=3 & sigma=1 & n=100 & 120.23 \\ 
  61 & MME & beta & beta=3 & sigma=1 & n=100 & 313146.35 \\ 
  62 & MME.b & beta & beta=3 & sigma=1 & n=100 & 2977375.83 \\ 
  63 & PWM & beta & beta=3 & sigma=1 & n=100 & 15.40 \\ 
  64 & MLE & sigma & beta=3 & sigma=1 & n=100 & 2958523159.69 \\ 
  65 & MLE.b & sigma & beta=3 & sigma=1 & n=100 & 2958523446.62 \\ 
  66 & LME & sigma & beta=3 & sigma=1 & n=100 & 2.94 \\ 
  67 & MDE.Phi.chisq & sigma & beta=3 & sigma=1 & n=100 & 238.26 \\ 
  68 & MDE.Phi.tv & sigma & beta=3 & sigma=1 & n=100 & 276.94 \\ 
  69 & MDE.Phi.kl & sigma & beta=3 & sigma=1 & n=100 & 22.26 \\ 
  70 & MME & sigma & beta=3 & sigma=1 & n=100 & 45211.59 \\ 
  71 & MME.b & sigma & beta=3 & sigma=1 & n=100 & 430346.23 \\ 
  72 & PWM & sigma & beta=3 & sigma=1 & n=100 & 2.94 \\ 
  73 & MLE & beta & beta=4 & sigma=1 & n=100 & 198915101.21 \\ 
  74 & MLE.b & beta & beta=4 & sigma=1 & n=100 & 198915304.94 \\ 
  75 & LME & beta & beta=4 & sigma=1 & n=100 & 45.64 \\ 
  76 & MDE.Phi.chisq & beta & beta=4 & sigma=1 & n=100 & 1517.60 \\ 
  77 & MDE.Phi.tv & beta & beta=4 & sigma=1 & n=100 & 1738.81 \\ 
  78 & MDE.Phi.kl & beta & beta=4 & sigma=1 & n=100 & 232.11 \\ 
  79 & MME & beta & beta=4 & sigma=1 & n=100 & 11556.91 \\ 
  80 & MME.b & beta & beta=4 & sigma=1 & n=100 & 1921161.55 \\ 
  81 & PWM & beta & beta=4 & sigma=1 & n=100 & 45.64 \\ 
  82 & MLE & sigma & beta=4 & sigma=1 & n=100 & 12510634.96 \\ 
  83 & MLE.b & sigma & beta=4 & sigma=1 & n=100 & 12510651.05 \\ 
  84 & LME & sigma & beta=4 & sigma=1 & n=100 & 4.40 \\ 
  85 & MDE.Phi.chisq & sigma & beta=4 & sigma=1 & n=100 & 294.05 \\ 
  86 & MDE.Phi.tv & sigma & beta=4 & sigma=1 & n=100 & 319.96 \\ 
  87 & MDE.Phi.kl & sigma & beta=4 & sigma=1 & n=100 & 23.07 \\ 
  88 & MME & sigma & beta=4 & sigma=1 & n=100 & 1086.55 \\ 
  89 & MME.b & sigma & beta=4 & sigma=1 & n=100 & 270552.99 \\ 
  90 & PWM & sigma & beta=4 & sigma=1 & n=100 & 4.40 \\ 
  91 & MLE & beta & beta=5 & sigma=1 & n=100 & 4837706.58 \\ 
  92 & MLE.b & beta & beta=5 & sigma=1 & n=100 & 4837762.01 \\ 
  93 & LME & beta & beta=5 & sigma=1 & n=100 & 95.93 \\ 
  94 & MDE.Phi.chisq & beta & beta=5 & sigma=1 & n=100 & 2406.77 \\ 
  95 & MDE.Phi.tv & beta & beta=5 & sigma=1 & n=100 & 2595.14 \\ 
  96 & MDE.Phi.kl & beta & beta=5 & sigma=1 & n=100 & 410.31 \\ 
  97 & MME & beta & beta=5 & sigma=1 & n=100 & 18595.94 \\ 
  98 & MME.b & beta & beta=5 & sigma=1 & n=100 & 257872.26 \\ 
  99 & PWM & beta & beta=5 & sigma=1 & n=100 & 95.93 \\ 
  100 & MLE & sigma & beta=5 & sigma=1 & n=100 & 278312.21 \\ 
  101 & MLE.b & sigma & beta=5 & sigma=1 & n=100 & 278315.32 \\ 
  102 & LME & sigma & beta=5 & sigma=1 & n=100 & 5.33 \\ 
  103 & MDE.Phi.chisq & sigma & beta=5 & sigma=1 & n=100 & 268.90 \\ 
  104 & MDE.Phi.tv & sigma & beta=5 & sigma=1 & n=100 & 278.13 \\ 
  105 & MDE.Phi.kl & sigma & beta=5 & sigma=1 & n=100 & 22.60 \\ 
  106 & MME & sigma & beta=5 & sigma=1 & n=100 & 1037.17 \\ 
  107 & MME.b & sigma & beta=5 & sigma=1 & n=100 & 15448.09 \\ 
  108 & PWM & sigma & beta=5 & sigma=1 & n=100 & 5.33 \\ 
  109 & MLE & beta & beta=1.5 & sigma=1 & n=200 & 0.10 \\ 
  110 & MLE.b & beta & beta=1.5 & sigma=1 & n=200 & 0.08 \\ 
  111 & LME & beta & beta=1.5 & sigma=1 & n=200 & 0.11 \\ 
  112 & MDE.Phi.chisq & beta & beta=1.5 & sigma=1 & n=200 & 0.13 \\ 
  113 & MDE.Phi.tv & beta & beta=1.5 & sigma=1 & n=200 & 0.17 \\ 
  114 & MDE.Phi.kl & beta & beta=1.5 & sigma=1 & n=200 & 0.10 \\ 
  115 & MME & beta & beta=1.5 & sigma=1 & n=200 & 0.17 \\ 
  116 & MME.b & beta & beta=1.5 & sigma=1 & n=200 & 0.19 \\ 
  117 & PWM & beta & beta=1.5 & sigma=1 & n=200 & 0.11 \\ 
  118 & MLE & sigma & beta=1.5 & sigma=1 & n=200 & 0.11 \\ 
  119 & MLE.b & sigma & beta=1.5 & sigma=1 & n=200 & 0.08 \\ 
  120 & LME & sigma & beta=1.5 & sigma=1 & n=200 & 0.12 \\ 
  121 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=1 & n=200 & 0.23 \\ 
  122 & MDE.Phi.tv & sigma & beta=1.5 & sigma=1 & n=200 & 0.29 \\ 
  123 & MDE.Phi.kl & sigma & beta=1.5 & sigma=1 & n=200 & 0.11 \\ 
  124 & MME & sigma & beta=1.5 & sigma=1 & n=200 & 5.45 \\ 
  125 & MME.b & sigma & beta=1.5 & sigma=1 & n=200 & 5.58 \\ 
  126 & PWM & sigma & beta=1.5 & sigma=1 & n=200 & 0.12 \\ 
  127 & MLE & beta & beta=2 & sigma=1 & n=200 & 0.34 \\ 
  128 & MLE.b & beta & beta=2 & sigma=1 & n=200 & 0.22 \\ 
  129 & LME & beta & beta=2 & sigma=1 & n=200 & 0.32 \\ 
  130 & MDE.Phi.chisq & beta & beta=2 & sigma=1 & n=200 & 0.62 \\ 
  131 & MDE.Phi.tv & beta & beta=2 & sigma=1 & n=200 & 0.93 \\ 
  132 & MDE.Phi.kl & beta & beta=2 & sigma=1 & n=200 & 0.34 \\ 
  133 & MME & beta & beta=2 & sigma=1 & n=200 & 0.60 \\ 
  134 & MME.b & beta & beta=2 & sigma=1 & n=200 & 2.22 \\ 
  135 & PWM & beta & beta=2 & sigma=1 & n=200 & 0.32 \\ 
  136 & MLE & sigma & beta=2 & sigma=1 & n=200 & 0.17 \\ 
  137 & MLE.b & sigma & beta=2 & sigma=1 & n=200 & 0.11 \\ 
  138 & LME & sigma & beta=2 & sigma=1 & n=200 & 0.16 \\ 
  139 & MDE.Phi.chisq & sigma & beta=2 & sigma=1 & n=200 & 0.53 \\ 
  140 & MDE.Phi.tv & sigma & beta=2 & sigma=1 & n=200 & 0.82 \\ 
  141 & MDE.Phi.kl & sigma & beta=2 & sigma=1 & n=200 & 0.17 \\ 
  142 & MME & sigma & beta=2 & sigma=1 & n=200 & 0.32 \\ 
  143 & MME.b & sigma & beta=2 & sigma=1 & n=200 & 1.67 \\ 
  144 & PWM & sigma & beta=2 & sigma=1 & n=200 & 0.16 \\ 
  145 & MLE & beta & beta=2.5 & sigma=1 & n=200 & 3.33 \\ 
  146 & MLE.b & beta & beta=2.5 & sigma=1 & n=200 & 3.04 \\ 
  147 & LME & beta & beta=2.5 & sigma=1 & n=200 & 2.14 \\ 
  148 & MDE.Phi.chisq & beta & beta=2.5 & sigma=1 & n=200 & 19.06 \\ 
  149 & MDE.Phi.tv & beta & beta=2.5 & sigma=1 & n=200 & 13.95 \\ 
  150 & MDE.Phi.kl & beta & beta=2.5 & sigma=1 & n=200 & 3.31 \\ 
  151 & MME & beta & beta=2.5 & sigma=1 & n=200 & 5.67 \\ 
  152 & MME.b & beta & beta=2.5 & sigma=1 & n=200 & 163.67 \\ 
  153 & PWM & beta & beta=2.5 & sigma=1 & n=200 & 2.14 \\ 
  154 & MLE & sigma & beta=2.5 & sigma=1 & n=200 & 1.02 \\ 
  155 & MLE.b & sigma & beta=2.5 & sigma=1 & n=200 & 0.94 \\ 
  156 & LME & sigma & beta=2.5 & sigma=1 & n=200 & 0.57 \\ 
  157 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=1 & n=200 & 9.70 \\ 
  158 & MDE.Phi.tv & sigma & beta=2.5 & sigma=1 & n=200 & 7.02 \\ 
  159 & MDE.Phi.kl & sigma & beta=2.5 & sigma=1 & n=200 & 1.02 \\ 
  160 & MME & sigma & beta=2.5 & sigma=1 & n=200 & 1.74 \\ 
  161 & MME.b & sigma & beta=2.5 & sigma=1 & n=200 & 55.10 \\ 
  162 & PWM & sigma & beta=2.5 & sigma=1 & n=200 & 0.57 \\ 
  163 & MLE & beta & beta=3 & sigma=1 & n=200 & 4.87 \\ 
  164 & MLE.b & beta & beta=3 & sigma=1 & n=200 & 4.54 \\ 
  165 & LME & beta & beta=3 & sigma=1 & n=200 & 3.28 \\ 
  166 & MDE.Phi.chisq & beta & beta=3 & sigma=1 & n=200 & 95.65 \\ 
  167 & MDE.Phi.tv & beta & beta=3 & sigma=1 & n=200 & 82.48 \\ 
  168 & MDE.Phi.kl & beta & beta=3 & sigma=1 & n=200 & 5.10 \\ 
  169 & MME & beta & beta=3 & sigma=1 & n=200 & 7.13 \\ 
  170 & MME.b & beta & beta=3 & sigma=1 & n=200 & 450.37 \\ 
  171 & PWM & beta & beta=3 & sigma=1 & n=200 & 3.28 \\ 
  172 & MLE & sigma & beta=3 & sigma=1 & n=200 & 0.87 \\ 
  173 & MLE.b & sigma & beta=3 & sigma=1 & n=200 & 0.81 \\ 
  174 & LME & sigma & beta=3 & sigma=1 & n=200 & 0.55 \\ 
  175 & MDE.Phi.chisq & sigma & beta=3 & sigma=1 & n=200 & 32.11 \\ 
  176 & MDE.Phi.tv & sigma & beta=3 & sigma=1 & n=200 & 25.80 \\ 
  177 & MDE.Phi.kl & sigma & beta=3 & sigma=1 & n=200 & 0.91 \\ 
  178 & MME & sigma & beta=3 & sigma=1 & n=200 & 1.30 \\ 
  179 & MME.b & sigma & beta=3 & sigma=1 & n=200 & 83.38 \\ 
  180 & PWM & sigma & beta=3 & sigma=1 & n=200 & 0.55 \\ 
  181 & MLE & beta & beta=4 & sigma=1 & n=200 & 2426885.18 \\ 
  182 & MLE.b & beta & beta=4 & sigma=1 & n=200 & 2426919.13 \\ 
  183 & LME & beta & beta=4 & sigma=1 & n=200 & 14.64 \\ 
  184 & MDE.Phi.chisq & beta & beta=4 & sigma=1 & n=200 & 633.89 \\ 
  185 & MDE.Phi.tv & beta & beta=4 & sigma=1 & n=200 & 422.32 \\ 
  186 & MDE.Phi.kl & beta & beta=4 & sigma=1 & n=200 & 78.34 \\ 
  187 & MME & beta & beta=4 & sigma=1 & n=200 & 1484.06 \\ 
  188 & MME.b & beta & beta=4 & sigma=1 & n=200 & 10586.06 \\ 
  189 & PWM & beta & beta=4 & sigma=1 & n=200 & 14.64 \\ 
  190 & MLE & sigma & beta=4 & sigma=1 & n=200 & 225985.22 \\ 
  191 & MLE.b & sigma & beta=4 & sigma=1 & n=200 & 225988.35 \\ 
  192 & LME & sigma & beta=4 & sigma=1 & n=200 & 1.33 \\ 
  193 & MDE.Phi.chisq & sigma & beta=4 & sigma=1 & n=200 & 102.34 \\ 
  194 & MDE.Phi.tv & sigma & beta=4 & sigma=1 & n=200 & 65.02 \\ 
  195 & MDE.Phi.kl & sigma & beta=4 & sigma=1 & n=200 & 7.21 \\ 
  196 & MME & sigma & beta=4 & sigma=1 & n=200 & 137.81 \\ 
  197 & MME.b & sigma & beta=4 & sigma=1 & n=200 & 1080.75 \\ 
  198 & PWM & sigma & beta=4 & sigma=1 & n=200 & 1.33 \\ 
  199 & MLE & beta & beta=5 & sigma=1 & n=200 & 6973123.35 \\ 
  200 & MLE.b & beta & beta=5 & sigma=1 & n=200 & 6973180.72 \\ 
  201 & LME & beta & beta=5 & sigma=1 & n=200 & 54.44 \\ 
  202 & MDE.Phi.chisq & beta & beta=5 & sigma=1 & n=200 & 1484.55 \\ 
  203 & MDE.Phi.tv & beta & beta=5 & sigma=1 & n=200 & 974.42 \\ 
  204 & MDE.Phi.kl & beta & beta=5 & sigma=1 & n=200 & 179.68 \\ 
  205 & MME & beta & beta=5 & sigma=1 & n=200 & 352282.46 \\ 
  206 & MME.b & beta & beta=5 & sigma=1 & n=200 & 1489135.16 \\ 
  207 & PWM & beta & beta=5 & sigma=1 & n=200 & 54.44 \\ 
  208 & MLE & sigma & beta=5 & sigma=1 & n=200 & 441066.81 \\ 
  209 & MLE.b & sigma & beta=5 & sigma=1 & n=200 & 441070.14 \\ 
  210 & LME & sigma & beta=5 & sigma=1 & n=200 & 3.15 \\ 
  211 & MDE.Phi.chisq & sigma & beta=5 & sigma=1 & n=200 & 142.29 \\ 
  212 & MDE.Phi.tv & sigma & beta=5 & sigma=1 & n=200 & 88.12 \\ 
  213 & MDE.Phi.kl & sigma & beta=5 & sigma=1 & n=200 & 9.79 \\ 
  214 & MME & sigma & beta=5 & sigma=1 & n=200 & 19950.11 \\ 
  215 & MME.b & sigma & beta=5 & sigma=1 & n=200 & 85211.67 \\ 
  216 & PWM & sigma & beta=5 & sigma=1 & n=200 & 3.15 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220201/Full.beta=1.5.sig=3.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=1.5,  \sigma=3$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.6716&1.4777&1.8288&-1.8659&1.235&1.6717&2.7928&6.315&1.8288
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
3.5467&2.9322&3.976&5.2186&5.4884&3.5467&9.4577&20.5033&3.976
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.435&0.3213&0.2958&347.7847&6.2224&0.4353&0.8968&130047.0657&0.2958
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
4.4042&3.2523&2.9924&173.3935&144.6718&4.4068&17.9309&1340019.6955&2.9924
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1716&-0.0223&0.3288&-3.3659&-0.265&0.1717&1.2928&4.815&0.3288
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.5467&-0.0678&0.976&2.2186&2.4884&0.5467&6.4577&17.5033&0.976
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.4644&0.3217&0.4039&359.079&6.292&0.4647&2.568&130057.2451&0.4039
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
4.7026&3.2566&3.9448&178.2985&150.8494&4.7053&59.631&1340192.0584&3.9448
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 5.167&3.5783&4.3487&537.3775&157.1414&5.17&62.199&1470249.3036&4.3487\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0011&0.0011&2.9905720362169e+301&0.0459&0.0011&0.0099&7.105&0.0011\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220201/Full.beta=1.5.sig=3.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=1.5,  \sigma=3$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.7357&1.6342&1.7125&0.2561&1.0087&1.5779&2.5062&2.3065&1.7125
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
3.7266&3.4036&3.6243&3.6352&3.8045&3.2398&8.4301&7.6048&3.6243
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1061&0.0765&0.1129&64.5862&0.1778&0.105&0.1714&0.1932&0.1129
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.0485&0.7468&1.1164&11.079&2.624&1.0047&61.5566&61.1039&1.1164
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.2357&0.1342&0.2125&-1.2439&-0.4913&0.0779&1.0062&0.8065&0.2125
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.7266&0.4036&0.6243&0.6352&0.8045&0.2398&5.4301&4.6048&0.6243
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1616&0.0945&0.158&66.1271&0.4191&0.1111&1.1837&0.8437&0.158
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.5764&0.9096&1.506&11.4814&3.271&1.0621&91.036&82.3019&1.506
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 1.738&1.0041&1.664&77.6085&3.6901&1.1732&92.2197&83.1456&1.664\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 6e-04&6e-04&6e-04&2.32341125877127e+300&0.0295&5e-04&0.0086&0.0085&6e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220201/Full.beta=2.5.sig=3.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2.5,  \sigma=3$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 3.5587&3.1014&3.1959&4.0176&4.8289&3.4299&4.8215&8.0233&3.1959
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
4.7042&3.9609&4.0777&9.0171&10.5664&4.4977&7.0635&12.104&4.0777
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 107.959&108.5926&8.3445&201.5064&230.7041&27.8277&144.3024&2214.1429&8.3445
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
276.9013&278.4705&20.2358&1089.1668&1237.7133&68.5195&337.8152&5685.2863&20.2358
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.0587&0.6014&0.6959&1.5176&2.3289&0.9299&2.3215&5.5233&0.6959
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.7042&0.9609&1.0777&6.0171&7.5664&1.4977&4.0635&9.104&1.0777
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 109.069&108.9435&8.828&203.7893&236.1049&28.6897&149.6775&2244.4287&8.828
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
279.7781&279.3659&21.3951&1125.2629&1294.8406&70.7559&354.2932&5767.6013&21.3951
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 388.8471&388.3094&30.2231&1329.0522&1530.9455&99.4457&503.9707&8012.03&30.2231\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0012&0.001&0.0234&0.0179&0.0011&0.0019&8.078&0.001\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220201/Full.beta=2.5.sig=3.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2.5,  \sigma=3$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.8792&2.5518&2.8069&2.0751&2.2676&2.7837&3.6075&3.6547&2.8069
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
3.6141&3.0812&3.4715&4.1035&4.1918&3.4598&5.0414&5.0889&3.4715
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 3.4148&3.1418&2.1431&15.0146&10.6194&2.8589&5.675&163.6713&2.1431
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
8.8888&8.1611&5.1432&68.024&47.7739&7.8142&15.6207&495.8737&5.1432
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.3792&0.0518&0.3069&-0.4249&-0.2324&0.2837&1.1075&1.1547&0.3069
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.6141&0.0812&0.4715&1.1035&1.1918&0.4598&2.0414&2.0889&0.4715
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 3.5583&3.1441&2.2371&15.1936&10.6723&2.9391&6.9011&164.9884&2.2371
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
9.265&8.1669&5.365&69.2349&49.1895&8.0249&19.7863&500.1877&5.365
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 12.8232&11.311&7.6022&84.4285&59.8618&10.9639&26.6874&665.1761&7.6022\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&5e-04&5e-04&0.0174&0.0121&5e-04&0.0011&0.002&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220201/Full.beta=2.sig=3.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2,  \sigma=3$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.5229&2.1732&2.4461&2.0098&2.6561&2.4547&3.6774&9.475&2.4461
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
4.0877&3.3298&3.9049&6.2268&7.7105&3.9648&7.3117&19.7593&3.9049
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 50.2397&50.2304&3.1122&65.3242&78.4711&11.3227&52.8832&151218.7148&3.1122
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
162.8934&162.7118&13.005&604.2036&766.9693&42.7687&205.6855&751939.6756&13.005
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.5229&0.1732&0.4461&0.0098&0.6561&0.4547&1.6774&7.475&0.4461
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.0877&0.3298&0.9049&3.2268&4.7105&0.9648&4.3117&16.7593&0.9049
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 50.5081&50.2554&3.3109&65.3178&78.8937&11.5283&55.6916&151259.4682&3.3109
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
164.0602&162.8043&13.8226&614.5552&789.0814&43.6952&224.256&752145.3573&13.8226
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 214.5683&213.0597&17.1335&679.873&867.9751&55.2235&279.9476&903404.8256&17.1335\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0011&0.0011&2.00401541349742e+299&0.0234&0.0011&0.0035&0.0115&0.0011\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220201/Full.beta=2.sig=3.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2,  \sigma=3$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.2648&2.0725&2.2267&1.3452&1.5655&2.1539&2.9817&2.6479&2.2267
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
3.5657&3.1501&3.456&3.5192&3.8346&3.3309&5.6996&4.8863&3.456
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.3317&0.2092&0.3166&0.6257&0.9338&0.3416&0.597&2.2191&0.3166
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.494&0.9251&1.4123&4.7273&7.3767&1.5257&2.8527&15.0252&1.4123
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.2648&0.0725&0.2267&-0.6548&-0.4345&0.1539&0.9817&0.6479&0.2267
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.5657&0.1501&0.456&0.5192&0.8346&0.3309&2.6996&1.8863&0.456
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.4018&0.2145&0.368&1.0544&1.1225&0.3652&1.5607&2.6387&0.368
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.8139&0.9475&1.62&4.9964&8.0726&1.635&10.1404&18.5817&1.62
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 2.2157&1.162&1.988&6.0508&9.1951&2.0003&11.7011&21.2204&1.988\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 6e-04&5e-04&5e-04&0.0231&0.0166&5e-04&0.0024&0.0497&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220201/Full.beta=3.sig=3.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=3,  \sigma=3$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 5.5964&5.1022&4.016&6.6169&7.9609&4.8284&17.4876&49.9888&4.016
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
6.354&5.7136&4.2769&11.9927&14.0513&5.3641&20.2258&58.7062&4.2769
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 677.8708&680.3962&15.9912&428.3704&508.6075&92.1959&313146.3351&2977375.6823&15.9912
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1161.8215&1165.9639&27.7515&1517.4812&1763.6721&154.9961&406904.252&3873116.0303&27.7515
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.5964&2.1022&1.016&3.6169&4.9609&1.8284&14.4876&46.9888&1.016
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
3.354&2.7136&1.2769&8.9927&11.0513&2.3641&17.2258&55.7062&1.2769
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 684.5442&684.7475&17.0218&441.4094&533.1674&95.5297&313324.9108&2979285.896&17.0218
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1172.9546&1173.2107&29.3792&1598.1979&1885.6269&160.5696&407160.2893&3875831.9005&29.3792
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 1857.4988&1857.9582&46.401&2039.6073&2418.7943&256.0993&720485.2001&6855117.7965&46.401\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0012&0.0011&0.02&0.0151&0.0011&0.0014&0.0075&0.0011\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220201/Full.beta=3.sig=3.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=3,  \sigma=3$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 3.5381&3.0572&3.4093&3.2165&3.3377&3.4524&4.3176&4.8845&3.4093
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
3.7088&3.0823&3.5117&5.1737&5.0227&3.5895&4.8424&5.5237&3.5117
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 5.1103&4.8028&3.2795&70.5482&59.1732&5.0951&7.1258&450.3612&3.2795
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
8.537&7.9965&4.9759&213.9366&166.4308&8.1559&11.6829&750.4345&4.9759
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.5381&0.0572&0.4093&0.2165&0.3377&0.4524&1.3176&1.8845&0.4093
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.7088&0.0823&0.5117&2.1737&2.0227&0.5895&1.8424&2.5237&0.5117
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 5.3993&4.8056&3.4467&70.588&59.2813&5.2992&8.8612&453.8676&3.4467
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
9.0386&8.0025&5.2372&218.6402&170.5054&8.5026&15.0761&756.7285&5.2372
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 14.4379&12.8081&8.6839&289.2282&229.7867&13.8019&23.9373&1210.5962&8.6839\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 6e-04&5e-04&5e-04&0.0144&0.0098&5e-04&8e-04&0.0016&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220201/Full.beta=4.sig=3.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=4,  \sigma=3$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 8.5651&8.1155&5.7431&13.1722&15.2639&7.3711&11.3516&40.9045&5.7431
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
7.2338&6.8247&4.5931&16.9721&19.0213&6.1355&9.9949&40.2956&4.5931
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1294.7946&1299.6285&46.478&1047.1127&1197.4413&187.3646&11556.8304&1921162.1725&46.478
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1086.9698&1090.9999&40.8875&1826.9669&1987.7095&166.4193&9778.8752&2434977.1853&40.8875
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 4.5651&4.1155&1.7431&9.1722&11.2639&3.3711&7.3516&36.9045&1.7431
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
4.2338&3.8247&1.5931&13.9721&16.0213&3.1355&6.9949&37.2956&1.5931
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1315.5051&1316.4358&49.5119&1131.137&1324.1974&198.71&11609.7215&1922331.9971&49.5119
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1104.7858&1105.5195&43.4215&2022.0024&2244.194&176.2341&9826.8255&2436124.6494&43.4215
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 2420.2909&2421.9552&92.9333&3153.1394&3568.3914&374.9441&21436.547&4358456.6465&92.9333\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0012&0.001&0.0165&0.0123&0.0011&0.0011&4041.9544&0.001\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220201/Full.beta=4.sig=3.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=4,  \sigma=3$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 6.5187&5.8384&4.9032&7.6743&6.7184&5.4151&7.0163&12.1602&4.9032
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
5.3438&4.7165&3.8086&8.9357&7.3856&4.2915&5.8202&10.6119&3.8086
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2063.4319&2066.1847&16.7866&443.0144&299.0583&61.8818&1484.482&10585.6597&16.7866
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1650.5326&1652.8515&13.724&643.8991&415.4308&51.2634&1240.6768&9726.2225&13.724
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.5187&1.8384&0.9032&3.6743&2.7184&1.4151&3.0163&8.1602&0.9032
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2.3438&1.7165&0.8086&5.9357&4.3856&1.2915&2.8202&7.6119&0.8086
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2069.5694&2069.3577&17.6007&456.4709&306.4179&63.878&1493.4317&10651.19&17.6007
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1655.8609&1655.6327&14.3765&679.0673&434.6229&52.9263&1248.5063&9783.191&14.3765
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 3725.4303&3724.9904&31.9772&1135.5382&741.0408&116.8043&2741.938&20434.3809&31.9772\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&6e-04&5e-04&0.0112&0.0074&5e-04&6e-04&0.0949&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220201/Full.beta=5.sig=3.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=5,  \sigma=3$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 12.1326&11.7641&7.3024&19.1383&21.1953&9.9533&16.7085&47.1188&7.3024
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
8.0347&7.7778&4.6131&18.8325&20.2195&6.4978&11.2322&32.8687&4.6131
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2400.4604&2407.0096&87.344&1624.2479&1742.1578&318.9998&18586.5635&257834.8846&87.344
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1208.8519&1212.0548&44.0461&1635.5489&1683.5147&159.4701&9330.5769&139016.898&44.0461
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 7.1326&6.7641&2.3024&14.1383&16.1953&4.9533&11.7085&42.1188&2.3024
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
5.0347&4.7778&1.6131&15.8325&17.2195&3.4978&8.2322&29.8687&1.6131
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2451.0944&2452.5223&92.6363&1823.9766&2004.2704&343.5035&18721.794&259583.0943&92.6363
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1234.0789&1234.7607&46.6437&1886.0545&1979.8559&171.6887&9397.4128&139895.1374&46.6437
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 3685.1733&3687.283&139.28&3710.0311&3984.1263&515.1921&28119.2068&399478.2317&139.28\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.001&0.0012&0.001&0.0144&0.0106&0.001&0.001&5.1562081310583e+29&0.001\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220201/Full.beta=5.sig=3.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=5,  \sigma=3$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 9.9441&9.2284&6.66&13.8125&11.1004&7.585&16.1531&39.2095&6.66
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
6.6298&6.1208&4.1672&12.5272&9.5259&4.823&10.9732&27.7972&4.1672
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 6726.231&6733.6183&48.5157&1015.6368&670.6961&138.1559&352282.3244&1489134.8361&48.5157
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
3937.6844&3941.4924&24.8428&874.9755&544.5209&67.7286&179550.8806&766904.817&24.8428
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 4.9441&4.2284&1.66&8.8125&6.1004&2.585&11.1531&34.2095&1.66
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
3.6298&3.1208&1.1672&9.5272&6.5259&1.823&7.9732&24.7972&1.1672
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 6750.0026&6750.8245&51.2666&1093.1954&707.8436&144.8243&352371.4885&1490156.2129&51.2666
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
3950.466&3950.8377&26.2027&965.6559&587.0539&71.0452&179596.4977&767443.0263&26.2027
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 10700.4685&10701.6622&77.4692&2058.8513&1294.8975&215.8696&531967.9862&2257599.2392&77.4692\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&6e-04&5e-04&0.0097&0.0064&5e-04&5e-04&0.4691&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220201/Output.accuracy.LaTeX.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Mon Jan 31 15:48:14 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & Measure & beta=1.5 & sigma=3 & n=100 & 5.17 \\ 
  2 & MLE.b & Measure & beta=1.5 & sigma=3 & n=100 & 3.58 \\ 
  3 & LME & Measure & beta=1.5 & sigma=3 & n=100 & 4.35 \\ 
  4 & MDE.Phi.chisq & Measure & beta=1.5 & sigma=3 & n=100 & 537.38 \\ 
  5 & MDE.Phi.tv & Measure & beta=1.5 & sigma=3 & n=100 & 157.14 \\ 
  6 & MDE.Phi.kl & Measure & beta=1.5 & sigma=3 & n=100 & 5.17 \\ 
  7 & MME & Measure & beta=1.5 & sigma=3 & n=100 & 62.20 \\ 
  8 & MME.b & Measure & beta=1.5 & sigma=3 & n=100 & 1470249.30 \\ 
  9 & PWM & Measure & beta=1.5 & sigma=3 & n=100 & 4.35 \\ 
  10 & MLE & Measure & beta=2 & sigma=3 & n=100 & 214.57 \\ 
  11 & MLE.b & Measure & beta=2 & sigma=3 & n=100 & 213.06 \\ 
  12 & LME & Measure & beta=2 & sigma=3 & n=100 & 17.13 \\ 
  13 & MDE.Phi.chisq & Measure & beta=2 & sigma=3 & n=100 & 679.87 \\ 
  14 & MDE.Phi.tv & Measure & beta=2 & sigma=3 & n=100 & 867.98 \\ 
  15 & MDE.Phi.kl & Measure & beta=2 & sigma=3 & n=100 & 55.22 \\ 
  16 & MME & Measure & beta=2 & sigma=3 & n=100 & 279.95 \\ 
  17 & MME.b & Measure & beta=2 & sigma=3 & n=100 & 903404.83 \\ 
  18 & PWM & Measure & beta=2 & sigma=3 & n=100 & 17.13 \\ 
  19 & MLE & Measure & beta=2.5 & sigma=3 & n=100 & 388.85 \\ 
  20 & MLE.b & Measure & beta=2.5 & sigma=3 & n=100 & 388.31 \\ 
  21 & LME & Measure & beta=2.5 & sigma=3 & n=100 & 30.22 \\ 
  22 & MDE.Phi.chisq & Measure & beta=2.5 & sigma=3 & n=100 & 1329.05 \\ 
  23 & MDE.Phi.tv & Measure & beta=2.5 & sigma=3 & n=100 & 1530.95 \\ 
  24 & MDE.Phi.kl & Measure & beta=2.5 & sigma=3 & n=100 & 99.45 \\ 
  25 & MME & Measure & beta=2.5 & sigma=3 & n=100 & 503.97 \\ 
  26 & MME.b & Measure & beta=2.5 & sigma=3 & n=100 & 8012.03 \\ 
  27 & PWM & Measure & beta=2.5 & sigma=3 & n=100 & 30.22 \\ 
  28 & MLE & Measure & beta=3 & sigma=3 & n=100 & 1857.50 \\ 
  29 & MLE.b & Measure & beta=3 & sigma=3 & n=100 & 1857.96 \\ 
  30 & LME & Measure & beta=3 & sigma=3 & n=100 & 46.40 \\ 
  31 & MDE.Phi.chisq & Measure & beta=3 & sigma=3 & n=100 & 2039.61 \\ 
  32 & MDE.Phi.tv & Measure & beta=3 & sigma=3 & n=100 & 2418.79 \\ 
  33 & MDE.Phi.kl & Measure & beta=3 & sigma=3 & n=100 & 256.10 \\ 
  34 & MME & Measure & beta=3 & sigma=3 & n=100 & 720485.20 \\ 
  35 & MME.b & Measure & beta=3 & sigma=3 & n=100 & 6855117.80 \\ 
  36 & PWM & Measure & beta=3 & sigma=3 & n=100 & 46.40 \\ 
  37 & MLE & Measure & beta=4 & sigma=3 & n=100 & 2420.29 \\ 
  38 & MLE.b & Measure & beta=4 & sigma=3 & n=100 & 2421.96 \\ 
  39 & LME & Measure & beta=4 & sigma=3 & n=100 & 92.93 \\ 
  40 & MDE.Phi.chisq & Measure & beta=4 & sigma=3 & n=100 & 3153.14 \\ 
  41 & MDE.Phi.tv & Measure & beta=4 & sigma=3 & n=100 & 3568.39 \\ 
  42 & MDE.Phi.kl & Measure & beta=4 & sigma=3 & n=100 & 374.94 \\ 
  43 & MME & Measure & beta=4 & sigma=3 & n=100 & 21436.55 \\ 
  44 & MME.b & Measure & beta=4 & sigma=3 & n=100 & 4358456.65 \\ 
  45 & PWM & Measure & beta=4 & sigma=3 & n=100 & 92.93 \\ 
  46 & MLE & Measure & beta=5 & sigma=3 & n=100 & 3685.17 \\ 
  47 & MLE.b & Measure & beta=5 & sigma=3 & n=100 & 3687.28 \\ 
  48 & LME & Measure & beta=5 & sigma=3 & n=100 & 139.28 \\ 
  49 & MDE.Phi.chisq & Measure & beta=5 & sigma=3 & n=100 & 3710.03 \\ 
  50 & MDE.Phi.tv & Measure & beta=5 & sigma=3 & n=100 & 3984.13 \\ 
  51 & MDE.Phi.kl & Measure & beta=5 & sigma=3 & n=100 & 515.19 \\ 
  52 & MME & Measure & beta=5 & sigma=3 & n=100 & 28119.21 \\ 
  53 & MME.b & Measure & beta=5 & sigma=3 & n=100 & 399478.23 \\ 
  54 & PWM & Measure & beta=5 & sigma=3 & n=100 & 139.28 \\ 
  55 & MLE & Measure & beta=1.5 & sigma=3 & n=200 & 1.74 \\ 
  56 & MLE.b & Measure & beta=1.5 & sigma=3 & n=200 & 1.00 \\ 
  57 & LME & Measure & beta=1.5 & sigma=3 & n=200 & 1.66 \\ 
  58 & MDE.Phi.chisq & Measure & beta=1.5 & sigma=3 & n=200 & 77.61 \\ 
  59 & MDE.Phi.tv & Measure & beta=1.5 & sigma=3 & n=200 & 3.69 \\ 
  60 & MDE.Phi.kl & Measure & beta=1.5 & sigma=3 & n=200 & 1.17 \\ 
  61 & MME & Measure & beta=1.5 & sigma=3 & n=200 & 92.22 \\ 
  62 & MME.b & Measure & beta=1.5 & sigma=3 & n=200 & 83.15 \\ 
  63 & PWM & Measure & beta=1.5 & sigma=3 & n=200 & 1.66 \\ 
  64 & MLE & Measure & beta=2 & sigma=3 & n=200 & 2.22 \\ 
  65 & MLE.b & Measure & beta=2 & sigma=3 & n=200 & 1.16 \\ 
  66 & LME & Measure & beta=2 & sigma=3 & n=200 & 1.99 \\ 
  67 & MDE.Phi.chisq & Measure & beta=2 & sigma=3 & n=200 & 6.05 \\ 
  68 & MDE.Phi.tv & Measure & beta=2 & sigma=3 & n=200 & 9.20 \\ 
  69 & MDE.Phi.kl & Measure & beta=2 & sigma=3 & n=200 & 2.00 \\ 
  70 & MME & Measure & beta=2 & sigma=3 & n=200 & 11.70 \\ 
  71 & MME.b & Measure & beta=2 & sigma=3 & n=200 & 21.22 \\ 
  72 & PWM & Measure & beta=2 & sigma=3 & n=200 & 1.99 \\ 
  73 & MLE & Measure & beta=2.5 & sigma=3 & n=200 & 12.82 \\ 
  74 & MLE.b & Measure & beta=2.5 & sigma=3 & n=200 & 11.31 \\ 
  75 & LME & Measure & beta=2.5 & sigma=3 & n=200 & 7.60 \\ 
  76 & MDE.Phi.chisq & Measure & beta=2.5 & sigma=3 & n=200 & 84.43 \\ 
  77 & MDE.Phi.tv & Measure & beta=2.5 & sigma=3 & n=200 & 59.86 \\ 
  78 & MDE.Phi.kl & Measure & beta=2.5 & sigma=3 & n=200 & 10.96 \\ 
  79 & MME & Measure & beta=2.5 & sigma=3 & n=200 & 26.69 \\ 
  80 & MME.b & Measure & beta=2.5 & sigma=3 & n=200 & 665.18 \\ 
  81 & PWM & Measure & beta=2.5 & sigma=3 & n=200 & 7.60 \\ 
  82 & MLE & Measure & beta=3 & sigma=3 & n=200 & 14.44 \\ 
  83 & MLE.b & Measure & beta=3 & sigma=3 & n=200 & 12.81 \\ 
  84 & LME & Measure & beta=3 & sigma=3 & n=200 & 8.68 \\ 
  85 & MDE.Phi.chisq & Measure & beta=3 & sigma=3 & n=200 & 289.23 \\ 
  86 & MDE.Phi.tv & Measure & beta=3 & sigma=3 & n=200 & 229.79 \\ 
  87 & MDE.Phi.kl & Measure & beta=3 & sigma=3 & n=200 & 13.80 \\ 
  88 & MME & Measure & beta=3 & sigma=3 & n=200 & 23.94 \\ 
  89 & MME.b & Measure & beta=3 & sigma=3 & n=200 & 1210.60 \\ 
  90 & PWM & Measure & beta=3 & sigma=3 & n=200 & 8.68 \\ 
  91 & MLE & Measure & beta=4 & sigma=3 & n=200 & 3725.43 \\ 
  92 & MLE.b & Measure & beta=4 & sigma=3 & n=200 & 3724.99 \\ 
  93 & LME & Measure & beta=4 & sigma=3 & n=200 & 31.98 \\ 
  94 & MDE.Phi.chisq & Measure & beta=4 & sigma=3 & n=200 & 1135.54 \\ 
  95 & MDE.Phi.tv & Measure & beta=4 & sigma=3 & n=200 & 741.04 \\ 
  96 & MDE.Phi.kl & Measure & beta=4 & sigma=3 & n=200 & 116.80 \\ 
  97 & MME & Measure & beta=4 & sigma=3 & n=200 & 2741.94 \\ 
  98 & MME.b & Measure & beta=4 & sigma=3 & n=200 & 20434.38 \\ 
  99 & PWM & Measure & beta=4 & sigma=3 & n=200 & 31.98 \\ 
  100 & MLE & Measure & beta=5 & sigma=3 & n=200 & 10700.47 \\ 
  101 & MLE.b & Measure & beta=5 & sigma=3 & n=200 & 10701.66 \\ 
  102 & LME & Measure & beta=5 & sigma=3 & n=200 & 77.47 \\ 
  103 & MDE.Phi.chisq & Measure & beta=5 & sigma=3 & n=200 & 2058.85 \\ 
  104 & MDE.Phi.tv & Measure & beta=5 & sigma=3 & n=200 & 1294.90 \\ 
  105 & MDE.Phi.kl & Measure & beta=5 & sigma=3 & n=200 & 215.87 \\ 
  106 & MME & Measure & beta=5 & sigma=3 & n=200 & 531967.99 \\ 
  107 & MME.b & Measure & beta=5 & sigma=3 & n=200 & 2257599.24 \\ 
  108 & PWM & Measure & beta=5 & sigma=3 & n=200 & 77.47 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220201/Output.accuracy2.LaTeX.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Mon Jan 31 15:48:14 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & Measure & beta=1.5 & sigma=3 & n=100 & 0.00 \\ 
  2 & MLE.b & Measure & beta=1.5 & sigma=3 & n=100 & 0.00 \\ 
  3 & LME & Measure & beta=1.5 & sigma=3 & n=100 & 0.00 \\ 
  4 & MDE.Phi.chisq & Measure & beta=1.5 & sigma=3 & n=100 & 29905720362168969996808464202462800682084228428422286624866604884622022480262860460682862862686226040624222482222048606602484402222646462462484864666660068682042200040840686000648880046024888628684680884420400648460404606406286026460640028240266822446048208046826248202606046862408260486282006042842840.00 \\ 
  5 & MDE.Phi.tv & Measure & beta=1.5 & sigma=3 & n=100 & 0.05 \\ 
  6 & MDE.Phi.kl & Measure & beta=1.5 & sigma=3 & n=100 & 0.00 \\ 
  7 & MME & Measure & beta=1.5 & sigma=3 & n=100 & 0.01 \\ 
  8 & MME.b & Measure & beta=1.5 & sigma=3 & n=100 & 7.11 \\ 
  9 & PWM & Measure & beta=1.5 & sigma=3 & n=100 & 0.00 \\ 
  10 & MLE & Measure & beta=2 & sigma=3 & n=100 & 0.00 \\ 
  11 & MLE.b & Measure & beta=2 & sigma=3 & n=100 & 0.00 \\ 
  12 & LME & Measure & beta=2 & sigma=3 & n=100 & 0.00 \\ 
  13 & MDE.Phi.chisq & Measure & beta=2 & sigma=3 & n=100 & 200401541349741565044622684624444464828280006842260482802402460840480462420442408484064028888884208868082024240488464422404022004826686464640022442426206826664828668088026884008426280242408868226824242822022244844842404026644404868866080088628264048220088826862228624862888066442022220866444444086022.00 \\ 
  14 & MDE.Phi.tv & Measure & beta=2 & sigma=3 & n=100 & 0.02 \\ 
  15 & MDE.Phi.kl & Measure & beta=2 & sigma=3 & n=100 & 0.00 \\ 
  16 & MME & Measure & beta=2 & sigma=3 & n=100 & 0.00 \\ 
  17 & MME.b & Measure & beta=2 & sigma=3 & n=100 & 0.01 \\ 
  18 & PWM & Measure & beta=2 & sigma=3 & n=100 & 0.00 \\ 
  19 & MLE & Measure & beta=2.5 & sigma=3 & n=100 & 0.00 \\ 
  20 & MLE.b & Measure & beta=2.5 & sigma=3 & n=100 & 0.00 \\ 
  21 & LME & Measure & beta=2.5 & sigma=3 & n=100 & 0.00 \\ 
  22 & MDE.Phi.chisq & Measure & beta=2.5 & sigma=3 & n=100 & 0.02 \\ 
  23 & MDE.Phi.tv & Measure & beta=2.5 & sigma=3 & n=100 & 0.02 \\ 
  24 & MDE.Phi.kl & Measure & beta=2.5 & sigma=3 & n=100 & 0.00 \\ 
  25 & MME & Measure & beta=2.5 & sigma=3 & n=100 & 0.00 \\ 
  26 & MME.b & Measure & beta=2.5 & sigma=3 & n=100 & 8.08 \\ 
  27 & PWM & Measure & beta=2.5 & sigma=3 & n=100 & 0.00 \\ 
  28 & MLE & Measure & beta=3 & sigma=3 & n=100 & 0.00 \\ 
  29 & MLE.b & Measure & beta=3 & sigma=3 & n=100 & 0.00 \\ 
  30 & LME & Measure & beta=3 & sigma=3 & n=100 & 0.00 \\ 
  31 & MDE.Phi.chisq & Measure & beta=3 & sigma=3 & n=100 & 0.02 \\ 
  32 & MDE.Phi.tv & Measure & beta=3 & sigma=3 & n=100 & 0.02 \\ 
  33 & MDE.Phi.kl & Measure & beta=3 & sigma=3 & n=100 & 0.00 \\ 
  34 & MME & Measure & beta=3 & sigma=3 & n=100 & 0.00 \\ 
  35 & MME.b & Measure & beta=3 & sigma=3 & n=100 & 0.01 \\ 
  36 & PWM & Measure & beta=3 & sigma=3 & n=100 & 0.00 \\ 
  37 & MLE & Measure & beta=4 & sigma=3 & n=100 & 0.00 \\ 
  38 & MLE.b & Measure & beta=4 & sigma=3 & n=100 & 0.00 \\ 
  39 & LME & Measure & beta=4 & sigma=3 & n=100 & 0.00 \\ 
  40 & MDE.Phi.chisq & Measure & beta=4 & sigma=3 & n=100 & 0.02 \\ 
  41 & MDE.Phi.tv & Measure & beta=4 & sigma=3 & n=100 & 0.01 \\ 
  42 & MDE.Phi.kl & Measure & beta=4 & sigma=3 & n=100 & 0.00 \\ 
  43 & MME & Measure & beta=4 & sigma=3 & n=100 & 0.00 \\ 
  44 & MME.b & Measure & beta=4 & sigma=3 & n=100 & 4041.95 \\ 
  45 & PWM & Measure & beta=4 & sigma=3 & n=100 & 0.00 \\ 
  46 & MLE & Measure & beta=5 & sigma=3 & n=100 & 0.00 \\ 
  47 & MLE.b & Measure & beta=5 & sigma=3 & n=100 & 0.00 \\ 
  48 & LME & Measure & beta=5 & sigma=3 & n=100 & 0.00 \\ 
  49 & MDE.Phi.chisq & Measure & beta=5 & sigma=3 & n=100 & 0.01 \\ 
  50 & MDE.Phi.tv & Measure & beta=5 & sigma=3 & n=100 & 0.01 \\ 
  51 & MDE.Phi.kl & Measure & beta=5 & sigma=3 & n=100 & 0.00 \\ 
  52 & MME & Measure & beta=5 & sigma=3 & n=100 & 0.00 \\ 
  53 & MME.b & Measure & beta=5 & sigma=3 & n=100 & 515620813105830396128066264404.00 \\ 
  54 & PWM & Measure & beta=5 & sigma=3 & n=100 & 0.00 \\ 
  55 & MLE & Measure & beta=1.5 & sigma=3 & n=200 & 0.00 \\ 
  56 & MLE.b & Measure & beta=1.5 & sigma=3 & n=200 & 0.00 \\ 
  57 & LME & Measure & beta=1.5 & sigma=3 & n=200 & 0.00 \\ 
  58 & MDE.Phi.chisq & Measure & beta=1.5 & sigma=3 & n=200 & 2323411258771274120820682268468404486802004068640040842482206262606888620868822202464828846264422206462008222660208468008226002400264448842006664082224602880244824260606404004866480262208644688246424408624004646224606804246868862806444062044600408400804428046620660226860248800466840004446408088064460.00 \\ 
  59 & MDE.Phi.tv & Measure & beta=1.5 & sigma=3 & n=200 & 0.03 \\ 
  60 & MDE.Phi.kl & Measure & beta=1.5 & sigma=3 & n=200 & 0.00 \\ 
  61 & MME & Measure & beta=1.5 & sigma=3 & n=200 & 0.01 \\ 
  62 & MME.b & Measure & beta=1.5 & sigma=3 & n=200 & 0.01 \\ 
  63 & PWM & Measure & beta=1.5 & sigma=3 & n=200 & 0.00 \\ 
  64 & MLE & Measure & beta=2 & sigma=3 & n=200 & 0.00 \\ 
  65 & MLE.b & Measure & beta=2 & sigma=3 & n=200 & 0.00 \\ 
  66 & LME & Measure & beta=2 & sigma=3 & n=200 & 0.00 \\ 
  67 & MDE.Phi.chisq & Measure & beta=2 & sigma=3 & n=200 & 0.02 \\ 
  68 & MDE.Phi.tv & Measure & beta=2 & sigma=3 & n=200 & 0.02 \\ 
  69 & MDE.Phi.kl & Measure & beta=2 & sigma=3 & n=200 & 0.00 \\ 
  70 & MME & Measure & beta=2 & sigma=3 & n=200 & 0.00 \\ 
  71 & MME.b & Measure & beta=2 & sigma=3 & n=200 & 0.05 \\ 
  72 & PWM & Measure & beta=2 & sigma=3 & n=200 & 0.00 \\ 
  73 & MLE & Measure & beta=2.5 & sigma=3 & n=200 & 0.00 \\ 
  74 & MLE.b & Measure & beta=2.5 & sigma=3 & n=200 & 0.00 \\ 
  75 & LME & Measure & beta=2.5 & sigma=3 & n=200 & 0.00 \\ 
  76 & MDE.Phi.chisq & Measure & beta=2.5 & sigma=3 & n=200 & 0.02 \\ 
  77 & MDE.Phi.tv & Measure & beta=2.5 & sigma=3 & n=200 & 0.01 \\ 
  78 & MDE.Phi.kl & Measure & beta=2.5 & sigma=3 & n=200 & 0.00 \\ 
  79 & MME & Measure & beta=2.5 & sigma=3 & n=200 & 0.00 \\ 
  80 & MME.b & Measure & beta=2.5 & sigma=3 & n=200 & 0.00 \\ 
  81 & PWM & Measure & beta=2.5 & sigma=3 & n=200 & 0.00 \\ 
  82 & MLE & Measure & beta=3 & sigma=3 & n=200 & 0.00 \\ 
  83 & MLE.b & Measure & beta=3 & sigma=3 & n=200 & 0.00 \\ 
  84 & LME & Measure & beta=3 & sigma=3 & n=200 & 0.00 \\ 
  85 & MDE.Phi.chisq & Measure & beta=3 & sigma=3 & n=200 & 0.01 \\ 
  86 & MDE.Phi.tv & Measure & beta=3 & sigma=3 & n=200 & 0.01 \\ 
  87 & MDE.Phi.kl & Measure & beta=3 & sigma=3 & n=200 & 0.00 \\ 
  88 & MME & Measure & beta=3 & sigma=3 & n=200 & 0.00 \\ 
  89 & MME.b & Measure & beta=3 & sigma=3 & n=200 & 0.00 \\ 
  90 & PWM & Measure & beta=3 & sigma=3 & n=200 & 0.00 \\ 
  91 & MLE & Measure & beta=4 & sigma=3 & n=200 & 0.00 \\ 
  92 & MLE.b & Measure & beta=4 & sigma=3 & n=200 & 0.00 \\ 
  93 & LME & Measure & beta=4 & sigma=3 & n=200 & 0.00 \\ 
  94 & MDE.Phi.chisq & Measure & beta=4 & sigma=3 & n=200 & 0.01 \\ 
  95 & MDE.Phi.tv & Measure & beta=4 & sigma=3 & n=200 & 0.01 \\ 
  96 & MDE.Phi.kl & Measure & beta=4 & sigma=3 & n=200 & 0.00 \\ 
  97 & MME & Measure & beta=4 & sigma=3 & n=200 & 0.00 \\ 
  98 & MME.b & Measure & beta=4 & sigma=3 & n=200 & 0.09 \\ 
  99 & PWM & Measure & beta=4 & sigma=3 & n=200 & 0.00 \\ 
  100 & MLE & Measure & beta=5 & sigma=3 & n=200 & 0.00 \\ 
  101 & MLE.b & Measure & beta=5 & sigma=3 & n=200 & 0.00 \\ 
  102 & LME & Measure & beta=5 & sigma=3 & n=200 & 0.00 \\ 
  103 & MDE.Phi.chisq & Measure & beta=5 & sigma=3 & n=200 & 0.01 \\ 
  104 & MDE.Phi.tv & Measure & beta=5 & sigma=3 & n=200 & 0.01 \\ 
  105 & MDE.Phi.kl & Measure & beta=5 & sigma=3 & n=200 & 0.00 \\ 
  106 & MME & Measure & beta=5 & sigma=3 & n=200 & 0.00 \\ 
  107 & MME.b & Measure & beta=5 & sigma=3 & n=200 & 0.47 \\ 
  108 & PWM & Measure & beta=5 & sigma=3 & n=200 & 0.00 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220201/Output.bias.LaTeX.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Mon Jan 31 15:48:14 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=3 & n=100 & 0.17 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=3 & n=100 & -0.02 \\ 
  3 & LME & beta & beta=1.5 & sigma=3 & n=100 & 0.33 \\ 
  4 & MDE.Phi.chisq & beta & beta=1.5 & sigma=3 & n=100 & -3.37 \\ 
  5 & MDE.Phi.tv & beta & beta=1.5 & sigma=3 & n=100 & -0.27 \\ 
  6 & MDE.Phi.kl & beta & beta=1.5 & sigma=3 & n=100 & 0.17 \\ 
  7 & MME & beta & beta=1.5 & sigma=3 & n=100 & 1.29 \\ 
  8 & MME.b & beta & beta=1.5 & sigma=3 & n=100 & 4.81 \\ 
  9 & PWM & beta & beta=1.5 & sigma=3 & n=100 & 0.33 \\ 
  10 & MLE & sigma & beta=1.5 & sigma=3 & n=100 & 0.55 \\ 
  11 & MLE.b & sigma & beta=1.5 & sigma=3 & n=100 & -0.07 \\ 
  12 & LME & sigma & beta=1.5 & sigma=3 & n=100 & 0.98 \\ 
  13 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=3 & n=100 & 2.22 \\ 
  14 & MDE.Phi.tv & sigma & beta=1.5 & sigma=3 & n=100 & 2.49 \\ 
  15 & MDE.Phi.kl & sigma & beta=1.5 & sigma=3 & n=100 & 0.55 \\ 
  16 & MME & sigma & beta=1.5 & sigma=3 & n=100 & 6.46 \\ 
  17 & MME.b & sigma & beta=1.5 & sigma=3 & n=100 & 17.50 \\ 
  18 & PWM & sigma & beta=1.5 & sigma=3 & n=100 & 0.98 \\ 
  19 & MLE & beta & beta=2 & sigma=3 & n=100 & 0.52 \\ 
  20 & MLE.b & beta & beta=2 & sigma=3 & n=100 & 0.17 \\ 
  21 & LME & beta & beta=2 & sigma=3 & n=100 & 0.45 \\ 
  22 & MDE.Phi.chisq & beta & beta=2 & sigma=3 & n=100 & 0.01 \\ 
  23 & MDE.Phi.tv & beta & beta=2 & sigma=3 & n=100 & 0.66 \\ 
  24 & MDE.Phi.kl & beta & beta=2 & sigma=3 & n=100 & 0.45 \\ 
  25 & MME & beta & beta=2 & sigma=3 & n=100 & 1.68 \\ 
  26 & MME.b & beta & beta=2 & sigma=3 & n=100 & 7.47 \\ 
  27 & PWM & beta & beta=2 & sigma=3 & n=100 & 0.45 \\ 
  28 & MLE & sigma & beta=2 & sigma=3 & n=100 & 1.09 \\ 
  29 & MLE.b & sigma & beta=2 & sigma=3 & n=100 & 0.33 \\ 
  30 & LME & sigma & beta=2 & sigma=3 & n=100 & 0.90 \\ 
  31 & MDE.Phi.chisq & sigma & beta=2 & sigma=3 & n=100 & 3.23 \\ 
  32 & MDE.Phi.tv & sigma & beta=2 & sigma=3 & n=100 & 4.71 \\ 
  33 & MDE.Phi.kl & sigma & beta=2 & sigma=3 & n=100 & 0.96 \\ 
  34 & MME & sigma & beta=2 & sigma=3 & n=100 & 4.31 \\ 
  35 & MME.b & sigma & beta=2 & sigma=3 & n=100 & 16.76 \\ 
  36 & PWM & sigma & beta=2 & sigma=3 & n=100 & 0.90 \\ 
  37 & MLE & beta & beta=2.5 & sigma=3 & n=100 & 1.06 \\ 
  38 & MLE.b & beta & beta=2.5 & sigma=3 & n=100 & 0.60 \\ 
  39 & LME & beta & beta=2.5 & sigma=3 & n=100 & 0.70 \\ 
  40 & MDE.Phi.chisq & beta & beta=2.5 & sigma=3 & n=100 & 1.52 \\ 
  41 & MDE.Phi.tv & beta & beta=2.5 & sigma=3 & n=100 & 2.33 \\ 
  42 & MDE.Phi.kl & beta & beta=2.5 & sigma=3 & n=100 & 0.93 \\ 
  43 & MME & beta & beta=2.5 & sigma=3 & n=100 & 2.32 \\ 
  44 & MME.b & beta & beta=2.5 & sigma=3 & n=100 & 5.52 \\ 
  45 & PWM & beta & beta=2.5 & sigma=3 & n=100 & 0.70 \\ 
  46 & MLE & sigma & beta=2.5 & sigma=3 & n=100 & 1.70 \\ 
  47 & MLE.b & sigma & beta=2.5 & sigma=3 & n=100 & 0.96 \\ 
  48 & LME & sigma & beta=2.5 & sigma=3 & n=100 & 1.08 \\ 
  49 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=3 & n=100 & 6.02 \\ 
  50 & MDE.Phi.tv & sigma & beta=2.5 & sigma=3 & n=100 & 7.57 \\ 
  51 & MDE.Phi.kl & sigma & beta=2.5 & sigma=3 & n=100 & 1.50 \\ 
  52 & MME & sigma & beta=2.5 & sigma=3 & n=100 & 4.06 \\ 
  53 & MME.b & sigma & beta=2.5 & sigma=3 & n=100 & 9.10 \\ 
  54 & PWM & sigma & beta=2.5 & sigma=3 & n=100 & 1.08 \\ 
  55 & MLE & beta & beta=3 & sigma=3 & n=100 & 2.60 \\ 
  56 & MLE.b & beta & beta=3 & sigma=3 & n=100 & 2.10 \\ 
  57 & LME & beta & beta=3 & sigma=3 & n=100 & 1.02 \\ 
  58 & MDE.Phi.chisq & beta & beta=3 & sigma=3 & n=100 & 3.62 \\ 
  59 & MDE.Phi.tv & beta & beta=3 & sigma=3 & n=100 & 4.96 \\ 
  60 & MDE.Phi.kl & beta & beta=3 & sigma=3 & n=100 & 1.83 \\ 
  61 & MME & beta & beta=3 & sigma=3 & n=100 & 14.49 \\ 
  62 & MME.b & beta & beta=3 & sigma=3 & n=100 & 46.99 \\ 
  63 & PWM & beta & beta=3 & sigma=3 & n=100 & 1.02 \\ 
  64 & MLE & sigma & beta=3 & sigma=3 & n=100 & 3.35 \\ 
  65 & MLE.b & sigma & beta=3 & sigma=3 & n=100 & 2.71 \\ 
  66 & LME & sigma & beta=3 & sigma=3 & n=100 & 1.28 \\ 
  67 & MDE.Phi.chisq & sigma & beta=3 & sigma=3 & n=100 & 8.99 \\ 
  68 & MDE.Phi.tv & sigma & beta=3 & sigma=3 & n=100 & 11.05 \\ 
  69 & MDE.Phi.kl & sigma & beta=3 & sigma=3 & n=100 & 2.36 \\ 
  70 & MME & sigma & beta=3 & sigma=3 & n=100 & 17.23 \\ 
  71 & MME.b & sigma & beta=3 & sigma=3 & n=100 & 55.71 \\ 
  72 & PWM & sigma & beta=3 & sigma=3 & n=100 & 1.28 \\ 
  73 & MLE & beta & beta=4 & sigma=3 & n=100 & 4.57 \\ 
  74 & MLE.b & beta & beta=4 & sigma=3 & n=100 & 4.12 \\ 
  75 & LME & beta & beta=4 & sigma=3 & n=100 & 1.74 \\ 
  76 & MDE.Phi.chisq & beta & beta=4 & sigma=3 & n=100 & 9.17 \\ 
  77 & MDE.Phi.tv & beta & beta=4 & sigma=3 & n=100 & 11.26 \\ 
  78 & MDE.Phi.kl & beta & beta=4 & sigma=3 & n=100 & 3.37 \\ 
  79 & MME & beta & beta=4 & sigma=3 & n=100 & 7.35 \\ 
  80 & MME.b & beta & beta=4 & sigma=3 & n=100 & 36.90 \\ 
  81 & PWM & beta & beta=4 & sigma=3 & n=100 & 1.74 \\ 
  82 & MLE & sigma & beta=4 & sigma=3 & n=100 & 4.23 \\ 
  83 & MLE.b & sigma & beta=4 & sigma=3 & n=100 & 3.82 \\ 
  84 & LME & sigma & beta=4 & sigma=3 & n=100 & 1.59 \\ 
  85 & MDE.Phi.chisq & sigma & beta=4 & sigma=3 & n=100 & 13.97 \\ 
  86 & MDE.Phi.tv & sigma & beta=4 & sigma=3 & n=100 & 16.02 \\ 
  87 & MDE.Phi.kl & sigma & beta=4 & sigma=3 & n=100 & 3.14 \\ 
  88 & MME & sigma & beta=4 & sigma=3 & n=100 & 6.99 \\ 
  89 & MME.b & sigma & beta=4 & sigma=3 & n=100 & 37.30 \\ 
  90 & PWM & sigma & beta=4 & sigma=3 & n=100 & 1.59 \\ 
  91 & MLE & beta & beta=5 & sigma=3 & n=100 & 7.13 \\ 
  92 & MLE.b & beta & beta=5 & sigma=3 & n=100 & 6.76 \\ 
  93 & LME & beta & beta=5 & sigma=3 & n=100 & 2.30 \\ 
  94 & MDE.Phi.chisq & beta & beta=5 & sigma=3 & n=100 & 14.14 \\ 
  95 & MDE.Phi.tv & beta & beta=5 & sigma=3 & n=100 & 16.20 \\ 
  96 & MDE.Phi.kl & beta & beta=5 & sigma=3 & n=100 & 4.95 \\ 
  97 & MME & beta & beta=5 & sigma=3 & n=100 & 11.71 \\ 
  98 & MME.b & beta & beta=5 & sigma=3 & n=100 & 42.12 \\ 
  99 & PWM & beta & beta=5 & sigma=3 & n=100 & 2.30 \\ 
  100 & MLE & sigma & beta=5 & sigma=3 & n=100 & 5.03 \\ 
  101 & MLE.b & sigma & beta=5 & sigma=3 & n=100 & 4.78 \\ 
  102 & LME & sigma & beta=5 & sigma=3 & n=100 & 1.61 \\ 
  103 & MDE.Phi.chisq & sigma & beta=5 & sigma=3 & n=100 & 15.83 \\ 
  104 & MDE.Phi.tv & sigma & beta=5 & sigma=3 & n=100 & 17.22 \\ 
  105 & MDE.Phi.kl & sigma & beta=5 & sigma=3 & n=100 & 3.50 \\ 
  106 & MME & sigma & beta=5 & sigma=3 & n=100 & 8.23 \\ 
  107 & MME.b & sigma & beta=5 & sigma=3 & n=100 & 29.87 \\ 
  108 & PWM & sigma & beta=5 & sigma=3 & n=100 & 1.61 \\ 
  109 & MLE & beta & beta=1.5 & sigma=3 & n=200 & 0.24 \\ 
  110 & MLE.b & beta & beta=1.5 & sigma=3 & n=200 & 0.13 \\ 
  111 & LME & beta & beta=1.5 & sigma=3 & n=200 & 0.21 \\ 
  112 & MDE.Phi.chisq & beta & beta=1.5 & sigma=3 & n=200 & -1.24 \\ 
  113 & MDE.Phi.tv & beta & beta=1.5 & sigma=3 & n=200 & -0.49 \\ 
  114 & MDE.Phi.kl & beta & beta=1.5 & sigma=3 & n=200 & 0.08 \\ 
  115 & MME & beta & beta=1.5 & sigma=3 & n=200 & 1.01 \\ 
  116 & MME.b & beta & beta=1.5 & sigma=3 & n=200 & 0.81 \\ 
  117 & PWM & beta & beta=1.5 & sigma=3 & n=200 & 0.21 \\ 
  118 & MLE & sigma & beta=1.5 & sigma=3 & n=200 & 0.73 \\ 
  119 & MLE.b & sigma & beta=1.5 & sigma=3 & n=200 & 0.40 \\ 
  120 & LME & sigma & beta=1.5 & sigma=3 & n=200 & 0.62 \\ 
  121 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=3 & n=200 & 0.64 \\ 
  122 & MDE.Phi.tv & sigma & beta=1.5 & sigma=3 & n=200 & 0.80 \\ 
  123 & MDE.Phi.kl & sigma & beta=1.5 & sigma=3 & n=200 & 0.24 \\ 
  124 & MME & sigma & beta=1.5 & sigma=3 & n=200 & 5.43 \\ 
  125 & MME.b & sigma & beta=1.5 & sigma=3 & n=200 & 4.60 \\ 
  126 & PWM & sigma & beta=1.5 & sigma=3 & n=200 & 0.62 \\ 
  127 & MLE & beta & beta=2 & sigma=3 & n=200 & 0.26 \\ 
  128 & MLE.b & beta & beta=2 & sigma=3 & n=200 & 0.07 \\ 
  129 & LME & beta & beta=2 & sigma=3 & n=200 & 0.23 \\ 
  130 & MDE.Phi.chisq & beta & beta=2 & sigma=3 & n=200 & -0.65 \\ 
  131 & MDE.Phi.tv & beta & beta=2 & sigma=3 & n=200 & -0.43 \\ 
  132 & MDE.Phi.kl & beta & beta=2 & sigma=3 & n=200 & 0.15 \\ 
  133 & MME & beta & beta=2 & sigma=3 & n=200 & 0.98 \\ 
  134 & MME.b & beta & beta=2 & sigma=3 & n=200 & 0.65 \\ 
  135 & PWM & beta & beta=2 & sigma=3 & n=200 & 0.23 \\ 
  136 & MLE & sigma & beta=2 & sigma=3 & n=200 & 0.57 \\ 
  137 & MLE.b & sigma & beta=2 & sigma=3 & n=200 & 0.15 \\ 
  138 & LME & sigma & beta=2 & sigma=3 & n=200 & 0.46 \\ 
  139 & MDE.Phi.chisq & sigma & beta=2 & sigma=3 & n=200 & 0.52 \\ 
  140 & MDE.Phi.tv & sigma & beta=2 & sigma=3 & n=200 & 0.83 \\ 
  141 & MDE.Phi.kl & sigma & beta=2 & sigma=3 & n=200 & 0.33 \\ 
  142 & MME & sigma & beta=2 & sigma=3 & n=200 & 2.70 \\ 
  143 & MME.b & sigma & beta=2 & sigma=3 & n=200 & 1.89 \\ 
  144 & PWM & sigma & beta=2 & sigma=3 & n=200 & 0.46 \\ 
  145 & MLE & beta & beta=2.5 & sigma=3 & n=200 & 0.38 \\ 
  146 & MLE.b & beta & beta=2.5 & sigma=3 & n=200 & 0.05 \\ 
  147 & LME & beta & beta=2.5 & sigma=3 & n=200 & 0.31 \\ 
  148 & MDE.Phi.chisq & beta & beta=2.5 & sigma=3 & n=200 & -0.42 \\ 
  149 & MDE.Phi.tv & beta & beta=2.5 & sigma=3 & n=200 & -0.23 \\ 
  150 & MDE.Phi.kl & beta & beta=2.5 & sigma=3 & n=200 & 0.28 \\ 
  151 & MME & beta & beta=2.5 & sigma=3 & n=200 & 1.11 \\ 
  152 & MME.b & beta & beta=2.5 & sigma=3 & n=200 & 1.15 \\ 
  153 & PWM & beta & beta=2.5 & sigma=3 & n=200 & 0.31 \\ 
  154 & MLE & sigma & beta=2.5 & sigma=3 & n=200 & 0.61 \\ 
  155 & MLE.b & sigma & beta=2.5 & sigma=3 & n=200 & 0.08 \\ 
  156 & LME & sigma & beta=2.5 & sigma=3 & n=200 & 0.47 \\ 
  157 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=3 & n=200 & 1.10 \\ 
  158 & MDE.Phi.tv & sigma & beta=2.5 & sigma=3 & n=200 & 1.19 \\ 
  159 & MDE.Phi.kl & sigma & beta=2.5 & sigma=3 & n=200 & 0.46 \\ 
  160 & MME & sigma & beta=2.5 & sigma=3 & n=200 & 2.04 \\ 
  161 & MME.b & sigma & beta=2.5 & sigma=3 & n=200 & 2.09 \\ 
  162 & PWM & sigma & beta=2.5 & sigma=3 & n=200 & 0.47 \\ 
  163 & MLE & beta & beta=3 & sigma=3 & n=200 & 0.54 \\ 
  164 & MLE.b & beta & beta=3 & sigma=3 & n=200 & 0.06 \\ 
  165 & LME & beta & beta=3 & sigma=3 & n=200 & 0.41 \\ 
  166 & MDE.Phi.chisq & beta & beta=3 & sigma=3 & n=200 & 0.22 \\ 
  167 & MDE.Phi.tv & beta & beta=3 & sigma=3 & n=200 & 0.34 \\ 
  168 & MDE.Phi.kl & beta & beta=3 & sigma=3 & n=200 & 0.45 \\ 
  169 & MME & beta & beta=3 & sigma=3 & n=200 & 1.32 \\ 
  170 & MME.b & beta & beta=3 & sigma=3 & n=200 & 1.88 \\ 
  171 & PWM & beta & beta=3 & sigma=3 & n=200 & 0.41 \\ 
  172 & MLE & sigma & beta=3 & sigma=3 & n=200 & 0.71 \\ 
  173 & MLE.b & sigma & beta=3 & sigma=3 & n=200 & 0.08 \\ 
  174 & LME & sigma & beta=3 & sigma=3 & n=200 & 0.51 \\ 
  175 & MDE.Phi.chisq & sigma & beta=3 & sigma=3 & n=200 & 2.17 \\ 
  176 & MDE.Phi.tv & sigma & beta=3 & sigma=3 & n=200 & 2.02 \\ 
  177 & MDE.Phi.kl & sigma & beta=3 & sigma=3 & n=200 & 0.59 \\ 
  178 & MME & sigma & beta=3 & sigma=3 & n=200 & 1.84 \\ 
  179 & MME.b & sigma & beta=3 & sigma=3 & n=200 & 2.52 \\ 
  180 & PWM & sigma & beta=3 & sigma=3 & n=200 & 0.51 \\ 
  181 & MLE & beta & beta=4 & sigma=3 & n=200 & 2.52 \\ 
  182 & MLE.b & beta & beta=4 & sigma=3 & n=200 & 1.84 \\ 
  183 & LME & beta & beta=4 & sigma=3 & n=200 & 0.90 \\ 
  184 & MDE.Phi.chisq & beta & beta=4 & sigma=3 & n=200 & 3.67 \\ 
  185 & MDE.Phi.tv & beta & beta=4 & sigma=3 & n=200 & 2.72 \\ 
  186 & MDE.Phi.kl & beta & beta=4 & sigma=3 & n=200 & 1.42 \\ 
  187 & MME & beta & beta=4 & sigma=3 & n=200 & 3.02 \\ 
  188 & MME.b & beta & beta=4 & sigma=3 & n=200 & 8.16 \\ 
  189 & PWM & beta & beta=4 & sigma=3 & n=200 & 0.90 \\ 
  190 & MLE & sigma & beta=4 & sigma=3 & n=200 & 2.34 \\ 
  191 & MLE.b & sigma & beta=4 & sigma=3 & n=200 & 1.72 \\ 
  192 & LME & sigma & beta=4 & sigma=3 & n=200 & 0.81 \\ 
  193 & MDE.Phi.chisq & sigma & beta=4 & sigma=3 & n=200 & 5.94 \\ 
  194 & MDE.Phi.tv & sigma & beta=4 & sigma=3 & n=200 & 4.39 \\ 
  195 & MDE.Phi.kl & sigma & beta=4 & sigma=3 & n=200 & 1.29 \\ 
  196 & MME & sigma & beta=4 & sigma=3 & n=200 & 2.82 \\ 
  197 & MME.b & sigma & beta=4 & sigma=3 & n=200 & 7.61 \\ 
  198 & PWM & sigma & beta=4 & sigma=3 & n=200 & 0.81 \\ 
  199 & MLE & beta & beta=5 & sigma=3 & n=200 & 4.94 \\ 
  200 & MLE.b & beta & beta=5 & sigma=3 & n=200 & 4.23 \\ 
  201 & LME & beta & beta=5 & sigma=3 & n=200 & 1.66 \\ 
  202 & MDE.Phi.chisq & beta & beta=5 & sigma=3 & n=200 & 8.81 \\ 
  203 & MDE.Phi.tv & beta & beta=5 & sigma=3 & n=200 & 6.10 \\ 
  204 & MDE.Phi.kl & beta & beta=5 & sigma=3 & n=200 & 2.59 \\ 
  205 & MME & beta & beta=5 & sigma=3 & n=200 & 11.15 \\ 
  206 & MME.b & beta & beta=5 & sigma=3 & n=200 & 34.21 \\ 
  207 & PWM & beta & beta=5 & sigma=3 & n=200 & 1.66 \\ 
  208 & MLE & sigma & beta=5 & sigma=3 & n=200 & 3.63 \\ 
  209 & MLE.b & sigma & beta=5 & sigma=3 & n=200 & 3.12 \\ 
  210 & LME & sigma & beta=5 & sigma=3 & n=200 & 1.17 \\ 
  211 & MDE.Phi.chisq & sigma & beta=5 & sigma=3 & n=200 & 9.53 \\ 
  212 & MDE.Phi.tv & sigma & beta=5 & sigma=3 & n=200 & 6.53 \\ 
  213 & MDE.Phi.kl & sigma & beta=5 & sigma=3 & n=200 & 1.82 \\ 
  214 & MME & sigma & beta=5 & sigma=3 & n=200 & 7.97 \\ 
  215 & MME.b & sigma & beta=5 & sigma=3 & n=200 & 24.80 \\ 
  216 & PWM & sigma & beta=5 & sigma=3 & n=200 & 1.17 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220201/Output.mean.LaTeX.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Mon Jan 31 15:48:14 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=3 & n=100 & 1.67 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=3 & n=100 & 1.48 \\ 
  3 & LME & beta & beta=1.5 & sigma=3 & n=100 & 1.83 \\ 
  4 & MDE.Phi.chisq & beta & beta=1.5 & sigma=3 & n=100 & -1.87 \\ 
  5 & MDE.Phi.tv & beta & beta=1.5 & sigma=3 & n=100 & 1.23 \\ 
  6 & MDE.Phi.kl & beta & beta=1.5 & sigma=3 & n=100 & 1.67 \\ 
  7 & MME & beta & beta=1.5 & sigma=3 & n=100 & 2.79 \\ 
  8 & MME.b & beta & beta=1.5 & sigma=3 & n=100 & 6.31 \\ 
  9 & PWM & beta & beta=1.5 & sigma=3 & n=100 & 1.83 \\ 
  10 & MLE & sigma & beta=1.5 & sigma=3 & n=100 & 3.55 \\ 
  11 & MLE.b & sigma & beta=1.5 & sigma=3 & n=100 & 2.93 \\ 
  12 & LME & sigma & beta=1.5 & sigma=3 & n=100 & 3.98 \\ 
  13 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=3 & n=100 & 5.22 \\ 
  14 & MDE.Phi.tv & sigma & beta=1.5 & sigma=3 & n=100 & 5.49 \\ 
  15 & MDE.Phi.kl & sigma & beta=1.5 & sigma=3 & n=100 & 3.55 \\ 
  16 & MME & sigma & beta=1.5 & sigma=3 & n=100 & 9.46 \\ 
  17 & MME.b & sigma & beta=1.5 & sigma=3 & n=100 & 20.50 \\ 
  18 & PWM & sigma & beta=1.5 & sigma=3 & n=100 & 3.98 \\ 
  19 & MLE & beta & beta=2 & sigma=3 & n=100 & 2.52 \\ 
  20 & MLE.b & beta & beta=2 & sigma=3 & n=100 & 2.17 \\ 
  21 & LME & beta & beta=2 & sigma=3 & n=100 & 2.45 \\ 
  22 & MDE.Phi.chisq & beta & beta=2 & sigma=3 & n=100 & 2.01 \\ 
  23 & MDE.Phi.tv & beta & beta=2 & sigma=3 & n=100 & 2.66 \\ 
  24 & MDE.Phi.kl & beta & beta=2 & sigma=3 & n=100 & 2.45 \\ 
  25 & MME & beta & beta=2 & sigma=3 & n=100 & 3.68 \\ 
  26 & MME.b & beta & beta=2 & sigma=3 & n=100 & 9.47 \\ 
  27 & PWM & beta & beta=2 & sigma=3 & n=100 & 2.45 \\ 
  28 & MLE & sigma & beta=2 & sigma=3 & n=100 & 4.09 \\ 
  29 & MLE.b & sigma & beta=2 & sigma=3 & n=100 & 3.33 \\ 
  30 & LME & sigma & beta=2 & sigma=3 & n=100 & 3.90 \\ 
  31 & MDE.Phi.chisq & sigma & beta=2 & sigma=3 & n=100 & 6.23 \\ 
  32 & MDE.Phi.tv & sigma & beta=2 & sigma=3 & n=100 & 7.71 \\ 
  33 & MDE.Phi.kl & sigma & beta=2 & sigma=3 & n=100 & 3.96 \\ 
  34 & MME & sigma & beta=2 & sigma=3 & n=100 & 7.31 \\ 
  35 & MME.b & sigma & beta=2 & sigma=3 & n=100 & 19.76 \\ 
  36 & PWM & sigma & beta=2 & sigma=3 & n=100 & 3.90 \\ 
  37 & MLE & beta & beta=2.5 & sigma=3 & n=100 & 3.56 \\ 
  38 & MLE.b & beta & beta=2.5 & sigma=3 & n=100 & 3.10 \\ 
  39 & LME & beta & beta=2.5 & sigma=3 & n=100 & 3.20 \\ 
  40 & MDE.Phi.chisq & beta & beta=2.5 & sigma=3 & n=100 & 4.02 \\ 
  41 & MDE.Phi.tv & beta & beta=2.5 & sigma=3 & n=100 & 4.83 \\ 
  42 & MDE.Phi.kl & beta & beta=2.5 & sigma=3 & n=100 & 3.43 \\ 
  43 & MME & beta & beta=2.5 & sigma=3 & n=100 & 4.82 \\ 
  44 & MME.b & beta & beta=2.5 & sigma=3 & n=100 & 8.02 \\ 
  45 & PWM & beta & beta=2.5 & sigma=3 & n=100 & 3.20 \\ 
  46 & MLE & sigma & beta=2.5 & sigma=3 & n=100 & 4.70 \\ 
  47 & MLE.b & sigma & beta=2.5 & sigma=3 & n=100 & 3.96 \\ 
  48 & LME & sigma & beta=2.5 & sigma=3 & n=100 & 4.08 \\ 
  49 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=3 & n=100 & 9.02 \\ 
  50 & MDE.Phi.tv & sigma & beta=2.5 & sigma=3 & n=100 & 10.57 \\ 
  51 & MDE.Phi.kl & sigma & beta=2.5 & sigma=3 & n=100 & 4.50 \\ 
  52 & MME & sigma & beta=2.5 & sigma=3 & n=100 & 7.06 \\ 
  53 & MME.b & sigma & beta=2.5 & sigma=3 & n=100 & 12.10 \\ 
  54 & PWM & sigma & beta=2.5 & sigma=3 & n=100 & 4.08 \\ 
  55 & MLE & beta & beta=3 & sigma=3 & n=100 & 5.60 \\ 
  56 & MLE.b & beta & beta=3 & sigma=3 & n=100 & 5.10 \\ 
  57 & LME & beta & beta=3 & sigma=3 & n=100 & 4.02 \\ 
  58 & MDE.Phi.chisq & beta & beta=3 & sigma=3 & n=100 & 6.62 \\ 
  59 & MDE.Phi.tv & beta & beta=3 & sigma=3 & n=100 & 7.96 \\ 
  60 & MDE.Phi.kl & beta & beta=3 & sigma=3 & n=100 & 4.83 \\ 
  61 & MME & beta & beta=3 & sigma=3 & n=100 & 17.49 \\ 
  62 & MME.b & beta & beta=3 & sigma=3 & n=100 & 49.99 \\ 
  63 & PWM & beta & beta=3 & sigma=3 & n=100 & 4.02 \\ 
  64 & MLE & sigma & beta=3 & sigma=3 & n=100 & 6.35 \\ 
  65 & MLE.b & sigma & beta=3 & sigma=3 & n=100 & 5.71 \\ 
  66 & LME & sigma & beta=3 & sigma=3 & n=100 & 4.28 \\ 
  67 & MDE.Phi.chisq & sigma & beta=3 & sigma=3 & n=100 & 11.99 \\ 
  68 & MDE.Phi.tv & sigma & beta=3 & sigma=3 & n=100 & 14.05 \\ 
  69 & MDE.Phi.kl & sigma & beta=3 & sigma=3 & n=100 & 5.36 \\ 
  70 & MME & sigma & beta=3 & sigma=3 & n=100 & 20.23 \\ 
  71 & MME.b & sigma & beta=3 & sigma=3 & n=100 & 58.71 \\ 
  72 & PWM & sigma & beta=3 & sigma=3 & n=100 & 4.28 \\ 
  73 & MLE & beta & beta=4 & sigma=3 & n=100 & 8.57 \\ 
  74 & MLE.b & beta & beta=4 & sigma=3 & n=100 & 8.12 \\ 
  75 & LME & beta & beta=4 & sigma=3 & n=100 & 5.74 \\ 
  76 & MDE.Phi.chisq & beta & beta=4 & sigma=3 & n=100 & 13.17 \\ 
  77 & MDE.Phi.tv & beta & beta=4 & sigma=3 & n=100 & 15.26 \\ 
  78 & MDE.Phi.kl & beta & beta=4 & sigma=3 & n=100 & 7.37 \\ 
  79 & MME & beta & beta=4 & sigma=3 & n=100 & 11.35 \\ 
  80 & MME.b & beta & beta=4 & sigma=3 & n=100 & 40.90 \\ 
  81 & PWM & beta & beta=4 & sigma=3 & n=100 & 5.74 \\ 
  82 & MLE & sigma & beta=4 & sigma=3 & n=100 & 7.23 \\ 
  83 & MLE.b & sigma & beta=4 & sigma=3 & n=100 & 6.82 \\ 
  84 & LME & sigma & beta=4 & sigma=3 & n=100 & 4.59 \\ 
  85 & MDE.Phi.chisq & sigma & beta=4 & sigma=3 & n=100 & 16.97 \\ 
  86 & MDE.Phi.tv & sigma & beta=4 & sigma=3 & n=100 & 19.02 \\ 
  87 & MDE.Phi.kl & sigma & beta=4 & sigma=3 & n=100 & 6.14 \\ 
  88 & MME & sigma & beta=4 & sigma=3 & n=100 & 9.99 \\ 
  89 & MME.b & sigma & beta=4 & sigma=3 & n=100 & 40.30 \\ 
  90 & PWM & sigma & beta=4 & sigma=3 & n=100 & 4.59 \\ 
  91 & MLE & beta & beta=5 & sigma=3 & n=100 & 12.13 \\ 
  92 & MLE.b & beta & beta=5 & sigma=3 & n=100 & 11.76 \\ 
  93 & LME & beta & beta=5 & sigma=3 & n=100 & 7.30 \\ 
  94 & MDE.Phi.chisq & beta & beta=5 & sigma=3 & n=100 & 19.14 \\ 
  95 & MDE.Phi.tv & beta & beta=5 & sigma=3 & n=100 & 21.20 \\ 
  96 & MDE.Phi.kl & beta & beta=5 & sigma=3 & n=100 & 9.95 \\ 
  97 & MME & beta & beta=5 & sigma=3 & n=100 & 16.71 \\ 
  98 & MME.b & beta & beta=5 & sigma=3 & n=100 & 47.12 \\ 
  99 & PWM & beta & beta=5 & sigma=3 & n=100 & 7.30 \\ 
  100 & MLE & sigma & beta=5 & sigma=3 & n=100 & 8.03 \\ 
  101 & MLE.b & sigma & beta=5 & sigma=3 & n=100 & 7.78 \\ 
  102 & LME & sigma & beta=5 & sigma=3 & n=100 & 4.61 \\ 
  103 & MDE.Phi.chisq & sigma & beta=5 & sigma=3 & n=100 & 18.83 \\ 
  104 & MDE.Phi.tv & sigma & beta=5 & sigma=3 & n=100 & 20.22 \\ 
  105 & MDE.Phi.kl & sigma & beta=5 & sigma=3 & n=100 & 6.50 \\ 
  106 & MME & sigma & beta=5 & sigma=3 & n=100 & 11.23 \\ 
  107 & MME.b & sigma & beta=5 & sigma=3 & n=100 & 32.87 \\ 
  108 & PWM & sigma & beta=5 & sigma=3 & n=100 & 4.61 \\ 
  109 & MLE & beta & beta=1.5 & sigma=3 & n=200 & 1.74 \\ 
  110 & MLE.b & beta & beta=1.5 & sigma=3 & n=200 & 1.63 \\ 
  111 & LME & beta & beta=1.5 & sigma=3 & n=200 & 1.71 \\ 
  112 & MDE.Phi.chisq & beta & beta=1.5 & sigma=3 & n=200 & 0.26 \\ 
  113 & MDE.Phi.tv & beta & beta=1.5 & sigma=3 & n=200 & 1.01 \\ 
  114 & MDE.Phi.kl & beta & beta=1.5 & sigma=3 & n=200 & 1.58 \\ 
  115 & MME & beta & beta=1.5 & sigma=3 & n=200 & 2.51 \\ 
  116 & MME.b & beta & beta=1.5 & sigma=3 & n=200 & 2.31 \\ 
  117 & PWM & beta & beta=1.5 & sigma=3 & n=200 & 1.71 \\ 
  118 & MLE & sigma & beta=1.5 & sigma=3 & n=200 & 3.73 \\ 
  119 & MLE.b & sigma & beta=1.5 & sigma=3 & n=200 & 3.40 \\ 
  120 & LME & sigma & beta=1.5 & sigma=3 & n=200 & 3.62 \\ 
  121 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=3 & n=200 & 3.64 \\ 
  122 & MDE.Phi.tv & sigma & beta=1.5 & sigma=3 & n=200 & 3.80 \\ 
  123 & MDE.Phi.kl & sigma & beta=1.5 & sigma=3 & n=200 & 3.24 \\ 
  124 & MME & sigma & beta=1.5 & sigma=3 & n=200 & 8.43 \\ 
  125 & MME.b & sigma & beta=1.5 & sigma=3 & n=200 & 7.60 \\ 
  126 & PWM & sigma & beta=1.5 & sigma=3 & n=200 & 3.62 \\ 
  127 & MLE & beta & beta=2 & sigma=3 & n=200 & 2.26 \\ 
  128 & MLE.b & beta & beta=2 & sigma=3 & n=200 & 2.07 \\ 
  129 & LME & beta & beta=2 & sigma=3 & n=200 & 2.23 \\ 
  130 & MDE.Phi.chisq & beta & beta=2 & sigma=3 & n=200 & 1.35 \\ 
  131 & MDE.Phi.tv & beta & beta=2 & sigma=3 & n=200 & 1.57 \\ 
  132 & MDE.Phi.kl & beta & beta=2 & sigma=3 & n=200 & 2.15 \\ 
  133 & MME & beta & beta=2 & sigma=3 & n=200 & 2.98 \\ 
  134 & MME.b & beta & beta=2 & sigma=3 & n=200 & 2.65 \\ 
  135 & PWM & beta & beta=2 & sigma=3 & n=200 & 2.23 \\ 
  136 & MLE & sigma & beta=2 & sigma=3 & n=200 & 3.57 \\ 
  137 & MLE.b & sigma & beta=2 & sigma=3 & n=200 & 3.15 \\ 
  138 & LME & sigma & beta=2 & sigma=3 & n=200 & 3.46 \\ 
  139 & MDE.Phi.chisq & sigma & beta=2 & sigma=3 & n=200 & 3.52 \\ 
  140 & MDE.Phi.tv & sigma & beta=2 & sigma=3 & n=200 & 3.83 \\ 
  141 & MDE.Phi.kl & sigma & beta=2 & sigma=3 & n=200 & 3.33 \\ 
  142 & MME & sigma & beta=2 & sigma=3 & n=200 & 5.70 \\ 
  143 & MME.b & sigma & beta=2 & sigma=3 & n=200 & 4.89 \\ 
  144 & PWM & sigma & beta=2 & sigma=3 & n=200 & 3.46 \\ 
  145 & MLE & beta & beta=2.5 & sigma=3 & n=200 & 2.88 \\ 
  146 & MLE.b & beta & beta=2.5 & sigma=3 & n=200 & 2.55 \\ 
  147 & LME & beta & beta=2.5 & sigma=3 & n=200 & 2.81 \\ 
  148 & MDE.Phi.chisq & beta & beta=2.5 & sigma=3 & n=200 & 2.08 \\ 
  149 & MDE.Phi.tv & beta & beta=2.5 & sigma=3 & n=200 & 2.27 \\ 
  150 & MDE.Phi.kl & beta & beta=2.5 & sigma=3 & n=200 & 2.78 \\ 
  151 & MME & beta & beta=2.5 & sigma=3 & n=200 & 3.61 \\ 
  152 & MME.b & beta & beta=2.5 & sigma=3 & n=200 & 3.65 \\ 
  153 & PWM & beta & beta=2.5 & sigma=3 & n=200 & 2.81 \\ 
  154 & MLE & sigma & beta=2.5 & sigma=3 & n=200 & 3.61 \\ 
  155 & MLE.b & sigma & beta=2.5 & sigma=3 & n=200 & 3.08 \\ 
  156 & LME & sigma & beta=2.5 & sigma=3 & n=200 & 3.47 \\ 
  157 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=3 & n=200 & 4.10 \\ 
  158 & MDE.Phi.tv & sigma & beta=2.5 & sigma=3 & n=200 & 4.19 \\ 
  159 & MDE.Phi.kl & sigma & beta=2.5 & sigma=3 & n=200 & 3.46 \\ 
  160 & MME & sigma & beta=2.5 & sigma=3 & n=200 & 5.04 \\ 
  161 & MME.b & sigma & beta=2.5 & sigma=3 & n=200 & 5.09 \\ 
  162 & PWM & sigma & beta=2.5 & sigma=3 & n=200 & 3.47 \\ 
  163 & MLE & beta & beta=3 & sigma=3 & n=200 & 3.54 \\ 
  164 & MLE.b & beta & beta=3 & sigma=3 & n=200 & 3.06 \\ 
  165 & LME & beta & beta=3 & sigma=3 & n=200 & 3.41 \\ 
  166 & MDE.Phi.chisq & beta & beta=3 & sigma=3 & n=200 & 3.22 \\ 
  167 & MDE.Phi.tv & beta & beta=3 & sigma=3 & n=200 & 3.34 \\ 
  168 & MDE.Phi.kl & beta & beta=3 & sigma=3 & n=200 & 3.45 \\ 
  169 & MME & beta & beta=3 & sigma=3 & n=200 & 4.32 \\ 
  170 & MME.b & beta & beta=3 & sigma=3 & n=200 & 4.88 \\ 
  171 & PWM & beta & beta=3 & sigma=3 & n=200 & 3.41 \\ 
  172 & MLE & sigma & beta=3 & sigma=3 & n=200 & 3.71 \\ 
  173 & MLE.b & sigma & beta=3 & sigma=3 & n=200 & 3.08 \\ 
  174 & LME & sigma & beta=3 & sigma=3 & n=200 & 3.51 \\ 
  175 & MDE.Phi.chisq & sigma & beta=3 & sigma=3 & n=200 & 5.17 \\ 
  176 & MDE.Phi.tv & sigma & beta=3 & sigma=3 & n=200 & 5.02 \\ 
  177 & MDE.Phi.kl & sigma & beta=3 & sigma=3 & n=200 & 3.59 \\ 
  178 & MME & sigma & beta=3 & sigma=3 & n=200 & 4.84 \\ 
  179 & MME.b & sigma & beta=3 & sigma=3 & n=200 & 5.52 \\ 
  180 & PWM & sigma & beta=3 & sigma=3 & n=200 & 3.51 \\ 
  181 & MLE & beta & beta=4 & sigma=3 & n=200 & 6.52 \\ 
  182 & MLE.b & beta & beta=4 & sigma=3 & n=200 & 5.84 \\ 
  183 & LME & beta & beta=4 & sigma=3 & n=200 & 4.90 \\ 
  184 & MDE.Phi.chisq & beta & beta=4 & sigma=3 & n=200 & 7.67 \\ 
  185 & MDE.Phi.tv & beta & beta=4 & sigma=3 & n=200 & 6.72 \\ 
  186 & MDE.Phi.kl & beta & beta=4 & sigma=3 & n=200 & 5.42 \\ 
  187 & MME & beta & beta=4 & sigma=3 & n=200 & 7.02 \\ 
  188 & MME.b & beta & beta=4 & sigma=3 & n=200 & 12.16 \\ 
  189 & PWM & beta & beta=4 & sigma=3 & n=200 & 4.90 \\ 
  190 & MLE & sigma & beta=4 & sigma=3 & n=200 & 5.34 \\ 
  191 & MLE.b & sigma & beta=4 & sigma=3 & n=200 & 4.72 \\ 
  192 & LME & sigma & beta=4 & sigma=3 & n=200 & 3.81 \\ 
  193 & MDE.Phi.chisq & sigma & beta=4 & sigma=3 & n=200 & 8.94 \\ 
  194 & MDE.Phi.tv & sigma & beta=4 & sigma=3 & n=200 & 7.39 \\ 
  195 & MDE.Phi.kl & sigma & beta=4 & sigma=3 & n=200 & 4.29 \\ 
  196 & MME & sigma & beta=4 & sigma=3 & n=200 & 5.82 \\ 
  197 & MME.b & sigma & beta=4 & sigma=3 & n=200 & 10.61 \\ 
  198 & PWM & sigma & beta=4 & sigma=3 & n=200 & 3.81 \\ 
  199 & MLE & beta & beta=5 & sigma=3 & n=200 & 9.94 \\ 
  200 & MLE.b & beta & beta=5 & sigma=3 & n=200 & 9.23 \\ 
  201 & LME & beta & beta=5 & sigma=3 & n=200 & 6.66 \\ 
  202 & MDE.Phi.chisq & beta & beta=5 & sigma=3 & n=200 & 13.81 \\ 
  203 & MDE.Phi.tv & beta & beta=5 & sigma=3 & n=200 & 11.10 \\ 
  204 & MDE.Phi.kl & beta & beta=5 & sigma=3 & n=200 & 7.59 \\ 
  205 & MME & beta & beta=5 & sigma=3 & n=200 & 16.15 \\ 
  206 & MME.b & beta & beta=5 & sigma=3 & n=200 & 39.21 \\ 
  207 & PWM & beta & beta=5 & sigma=3 & n=200 & 6.66 \\ 
  208 & MLE & sigma & beta=5 & sigma=3 & n=200 & 6.63 \\ 
  209 & MLE.b & sigma & beta=5 & sigma=3 & n=200 & 6.12 \\ 
  210 & LME & sigma & beta=5 & sigma=3 & n=200 & 4.17 \\ 
  211 & MDE.Phi.chisq & sigma & beta=5 & sigma=3 & n=200 & 12.53 \\ 
  212 & MDE.Phi.tv & sigma & beta=5 & sigma=3 & n=200 & 9.53 \\ 
  213 & MDE.Phi.kl & sigma & beta=5 & sigma=3 & n=200 & 4.82 \\ 
  214 & MME & sigma & beta=5 & sigma=3 & n=200 & 10.97 \\ 
  215 & MME.b & sigma & beta=5 & sigma=3 & n=200 & 27.80 \\ 
  216 & PWM & sigma & beta=5 & sigma=3 & n=200 & 4.17 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220201/Output.mse.LaTeX.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Mon Jan 31 15:48:14 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=3 & n=100 & 0.46 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=3 & n=100 & 0.32 \\ 
  3 & LME & beta & beta=1.5 & sigma=3 & n=100 & 0.40 \\ 
  4 & MDE.Phi.chisq & beta & beta=1.5 & sigma=3 & n=100 & 359.08 \\ 
  5 & MDE.Phi.tv & beta & beta=1.5 & sigma=3 & n=100 & 6.29 \\ 
  6 & MDE.Phi.kl & beta & beta=1.5 & sigma=3 & n=100 & 0.46 \\ 
  7 & MME & beta & beta=1.5 & sigma=3 & n=100 & 2.57 \\ 
  8 & MME.b & beta & beta=1.5 & sigma=3 & n=100 & 130057.25 \\ 
  9 & PWM & beta & beta=1.5 & sigma=3 & n=100 & 0.40 \\ 
  10 & MLE & sigma & beta=1.5 & sigma=3 & n=100 & 4.70 \\ 
  11 & MLE.b & sigma & beta=1.5 & sigma=3 & n=100 & 3.26 \\ 
  12 & LME & sigma & beta=1.5 & sigma=3 & n=100 & 3.94 \\ 
  13 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=3 & n=100 & 178.30 \\ 
  14 & MDE.Phi.tv & sigma & beta=1.5 & sigma=3 & n=100 & 150.85 \\ 
  15 & MDE.Phi.kl & sigma & beta=1.5 & sigma=3 & n=100 & 4.71 \\ 
  16 & MME & sigma & beta=1.5 & sigma=3 & n=100 & 59.63 \\ 
  17 & MME.b & sigma & beta=1.5 & sigma=3 & n=100 & 1340192.06 \\ 
  18 & PWM & sigma & beta=1.5 & sigma=3 & n=100 & 3.94 \\ 
  19 & MLE & beta & beta=2 & sigma=3 & n=100 & 50.51 \\ 
  20 & MLE.b & beta & beta=2 & sigma=3 & n=100 & 50.26 \\ 
  21 & LME & beta & beta=2 & sigma=3 & n=100 & 3.31 \\ 
  22 & MDE.Phi.chisq & beta & beta=2 & sigma=3 & n=100 & 65.32 \\ 
  23 & MDE.Phi.tv & beta & beta=2 & sigma=3 & n=100 & 78.89 \\ 
  24 & MDE.Phi.kl & beta & beta=2 & sigma=3 & n=100 & 11.53 \\ 
  25 & MME & beta & beta=2 & sigma=3 & n=100 & 55.69 \\ 
  26 & MME.b & beta & beta=2 & sigma=3 & n=100 & 151259.47 \\ 
  27 & PWM & beta & beta=2 & sigma=3 & n=100 & 3.31 \\ 
  28 & MLE & sigma & beta=2 & sigma=3 & n=100 & 164.06 \\ 
  29 & MLE.b & sigma & beta=2 & sigma=3 & n=100 & 162.80 \\ 
  30 & LME & sigma & beta=2 & sigma=3 & n=100 & 13.82 \\ 
  31 & MDE.Phi.chisq & sigma & beta=2 & sigma=3 & n=100 & 614.56 \\ 
  32 & MDE.Phi.tv & sigma & beta=2 & sigma=3 & n=100 & 789.08 \\ 
  33 & MDE.Phi.kl & sigma & beta=2 & sigma=3 & n=100 & 43.70 \\ 
  34 & MME & sigma & beta=2 & sigma=3 & n=100 & 224.26 \\ 
  35 & MME.b & sigma & beta=2 & sigma=3 & n=100 & 752145.36 \\ 
  36 & PWM & sigma & beta=2 & sigma=3 & n=100 & 13.82 \\ 
  37 & MLE & beta & beta=2.5 & sigma=3 & n=100 & 109.07 \\ 
  38 & MLE.b & beta & beta=2.5 & sigma=3 & n=100 & 108.94 \\ 
  39 & LME & beta & beta=2.5 & sigma=3 & n=100 & 8.83 \\ 
  40 & MDE.Phi.chisq & beta & beta=2.5 & sigma=3 & n=100 & 203.79 \\ 
  41 & MDE.Phi.tv & beta & beta=2.5 & sigma=3 & n=100 & 236.10 \\ 
  42 & MDE.Phi.kl & beta & beta=2.5 & sigma=3 & n=100 & 28.69 \\ 
  43 & MME & beta & beta=2.5 & sigma=3 & n=100 & 149.68 \\ 
  44 & MME.b & beta & beta=2.5 & sigma=3 & n=100 & 2244.43 \\ 
  45 & PWM & beta & beta=2.5 & sigma=3 & n=100 & 8.83 \\ 
  46 & MLE & sigma & beta=2.5 & sigma=3 & n=100 & 279.78 \\ 
  47 & MLE.b & sigma & beta=2.5 & sigma=3 & n=100 & 279.37 \\ 
  48 & LME & sigma & beta=2.5 & sigma=3 & n=100 & 21.40 \\ 
  49 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=3 & n=100 & 1125.26 \\ 
  50 & MDE.Phi.tv & sigma & beta=2.5 & sigma=3 & n=100 & 1294.84 \\ 
  51 & MDE.Phi.kl & sigma & beta=2.5 & sigma=3 & n=100 & 70.76 \\ 
  52 & MME & sigma & beta=2.5 & sigma=3 & n=100 & 354.29 \\ 
  53 & MME.b & sigma & beta=2.5 & sigma=3 & n=100 & 5767.60 \\ 
  54 & PWM & sigma & beta=2.5 & sigma=3 & n=100 & 21.40 \\ 
  55 & MLE & beta & beta=3 & sigma=3 & n=100 & 684.54 \\ 
  56 & MLE.b & beta & beta=3 & sigma=3 & n=100 & 684.75 \\ 
  57 & LME & beta & beta=3 & sigma=3 & n=100 & 17.02 \\ 
  58 & MDE.Phi.chisq & beta & beta=3 & sigma=3 & n=100 & 441.41 \\ 
  59 & MDE.Phi.tv & beta & beta=3 & sigma=3 & n=100 & 533.17 \\ 
  60 & MDE.Phi.kl & beta & beta=3 & sigma=3 & n=100 & 95.53 \\ 
  61 & MME & beta & beta=3 & sigma=3 & n=100 & 313324.91 \\ 
  62 & MME.b & beta & beta=3 & sigma=3 & n=100 & 2979285.90 \\ 
  63 & PWM & beta & beta=3 & sigma=3 & n=100 & 17.02 \\ 
  64 & MLE & sigma & beta=3 & sigma=3 & n=100 & 1172.95 \\ 
  65 & MLE.b & sigma & beta=3 & sigma=3 & n=100 & 1173.21 \\ 
  66 & LME & sigma & beta=3 & sigma=3 & n=100 & 29.38 \\ 
  67 & MDE.Phi.chisq & sigma & beta=3 & sigma=3 & n=100 & 1598.20 \\ 
  68 & MDE.Phi.tv & sigma & beta=3 & sigma=3 & n=100 & 1885.63 \\ 
  69 & MDE.Phi.kl & sigma & beta=3 & sigma=3 & n=100 & 160.57 \\ 
  70 & MME & sigma & beta=3 & sigma=3 & n=100 & 407160.29 \\ 
  71 & MME.b & sigma & beta=3 & sigma=3 & n=100 & 3875831.90 \\ 
  72 & PWM & sigma & beta=3 & sigma=3 & n=100 & 29.38 \\ 
  73 & MLE & beta & beta=4 & sigma=3 & n=100 & 1315.51 \\ 
  74 & MLE.b & beta & beta=4 & sigma=3 & n=100 & 1316.44 \\ 
  75 & LME & beta & beta=4 & sigma=3 & n=100 & 49.51 \\ 
  76 & MDE.Phi.chisq & beta & beta=4 & sigma=3 & n=100 & 1131.14 \\ 
  77 & MDE.Phi.tv & beta & beta=4 & sigma=3 & n=100 & 1324.20 \\ 
  78 & MDE.Phi.kl & beta & beta=4 & sigma=3 & n=100 & 198.71 \\ 
  79 & MME & beta & beta=4 & sigma=3 & n=100 & 11609.72 \\ 
  80 & MME.b & beta & beta=4 & sigma=3 & n=100 & 1922332.00 \\ 
  81 & PWM & beta & beta=4 & sigma=3 & n=100 & 49.51 \\ 
  82 & MLE & sigma & beta=4 & sigma=3 & n=100 & 1104.79 \\ 
  83 & MLE.b & sigma & beta=4 & sigma=3 & n=100 & 1105.52 \\ 
  84 & LME & sigma & beta=4 & sigma=3 & n=100 & 43.42 \\ 
  85 & MDE.Phi.chisq & sigma & beta=4 & sigma=3 & n=100 & 2022.00 \\ 
  86 & MDE.Phi.tv & sigma & beta=4 & sigma=3 & n=100 & 2244.19 \\ 
  87 & MDE.Phi.kl & sigma & beta=4 & sigma=3 & n=100 & 176.23 \\ 
  88 & MME & sigma & beta=4 & sigma=3 & n=100 & 9826.83 \\ 
  89 & MME.b & sigma & beta=4 & sigma=3 & n=100 & 2436124.65 \\ 
  90 & PWM & sigma & beta=4 & sigma=3 & n=100 & 43.42 \\ 
  91 & MLE & beta & beta=5 & sigma=3 & n=100 & 2451.09 \\ 
  92 & MLE.b & beta & beta=5 & sigma=3 & n=100 & 2452.52 \\ 
  93 & LME & beta & beta=5 & sigma=3 & n=100 & 92.64 \\ 
  94 & MDE.Phi.chisq & beta & beta=5 & sigma=3 & n=100 & 1823.98 \\ 
  95 & MDE.Phi.tv & beta & beta=5 & sigma=3 & n=100 & 2004.27 \\ 
  96 & MDE.Phi.kl & beta & beta=5 & sigma=3 & n=100 & 343.50 \\ 
  97 & MME & beta & beta=5 & sigma=3 & n=100 & 18721.79 \\ 
  98 & MME.b & beta & beta=5 & sigma=3 & n=100 & 259583.09 \\ 
  99 & PWM & beta & beta=5 & sigma=3 & n=100 & 92.64 \\ 
  100 & MLE & sigma & beta=5 & sigma=3 & n=100 & 1234.08 \\ 
  101 & MLE.b & sigma & beta=5 & sigma=3 & n=100 & 1234.76 \\ 
  102 & LME & sigma & beta=5 & sigma=3 & n=100 & 46.64 \\ 
  103 & MDE.Phi.chisq & sigma & beta=5 & sigma=3 & n=100 & 1886.05 \\ 
  104 & MDE.Phi.tv & sigma & beta=5 & sigma=3 & n=100 & 1979.86 \\ 
  105 & MDE.Phi.kl & sigma & beta=5 & sigma=3 & n=100 & 171.69 \\ 
  106 & MME & sigma & beta=5 & sigma=3 & n=100 & 9397.41 \\ 
  107 & MME.b & sigma & beta=5 & sigma=3 & n=100 & 139895.14 \\ 
  108 & PWM & sigma & beta=5 & sigma=3 & n=100 & 46.64 \\ 
  109 & MLE & beta & beta=1.5 & sigma=3 & n=200 & 0.16 \\ 
  110 & MLE.b & beta & beta=1.5 & sigma=3 & n=200 & 0.09 \\ 
  111 & LME & beta & beta=1.5 & sigma=3 & n=200 & 0.16 \\ 
  112 & MDE.Phi.chisq & beta & beta=1.5 & sigma=3 & n=200 & 66.13 \\ 
  113 & MDE.Phi.tv & beta & beta=1.5 & sigma=3 & n=200 & 0.42 \\ 
  114 & MDE.Phi.kl & beta & beta=1.5 & sigma=3 & n=200 & 0.11 \\ 
  115 & MME & beta & beta=1.5 & sigma=3 & n=200 & 1.18 \\ 
  116 & MME.b & beta & beta=1.5 & sigma=3 & n=200 & 0.84 \\ 
  117 & PWM & beta & beta=1.5 & sigma=3 & n=200 & 0.16 \\ 
  118 & MLE & sigma & beta=1.5 & sigma=3 & n=200 & 1.58 \\ 
  119 & MLE.b & sigma & beta=1.5 & sigma=3 & n=200 & 0.91 \\ 
  120 & LME & sigma & beta=1.5 & sigma=3 & n=200 & 1.51 \\ 
  121 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=3 & n=200 & 11.48 \\ 
  122 & MDE.Phi.tv & sigma & beta=1.5 & sigma=3 & n=200 & 3.27 \\ 
  123 & MDE.Phi.kl & sigma & beta=1.5 & sigma=3 & n=200 & 1.06 \\ 
  124 & MME & sigma & beta=1.5 & sigma=3 & n=200 & 91.04 \\ 
  125 & MME.b & sigma & beta=1.5 & sigma=3 & n=200 & 82.30 \\ 
  126 & PWM & sigma & beta=1.5 & sigma=3 & n=200 & 1.51 \\ 
  127 & MLE & beta & beta=2 & sigma=3 & n=200 & 0.40 \\ 
  128 & MLE.b & beta & beta=2 & sigma=3 & n=200 & 0.21 \\ 
  129 & LME & beta & beta=2 & sigma=3 & n=200 & 0.37 \\ 
  130 & MDE.Phi.chisq & beta & beta=2 & sigma=3 & n=200 & 1.05 \\ 
  131 & MDE.Phi.tv & beta & beta=2 & sigma=3 & n=200 & 1.12 \\ 
  132 & MDE.Phi.kl & beta & beta=2 & sigma=3 & n=200 & 0.37 \\ 
  133 & MME & beta & beta=2 & sigma=3 & n=200 & 1.56 \\ 
  134 & MME.b & beta & beta=2 & sigma=3 & n=200 & 2.64 \\ 
  135 & PWM & beta & beta=2 & sigma=3 & n=200 & 0.37 \\ 
  136 & MLE & sigma & beta=2 & sigma=3 & n=200 & 1.81 \\ 
  137 & MLE.b & sigma & beta=2 & sigma=3 & n=200 & 0.95 \\ 
  138 & LME & sigma & beta=2 & sigma=3 & n=200 & 1.62 \\ 
  139 & MDE.Phi.chisq & sigma & beta=2 & sigma=3 & n=200 & 5.00 \\ 
  140 & MDE.Phi.tv & sigma & beta=2 & sigma=3 & n=200 & 8.07 \\ 
  141 & MDE.Phi.kl & sigma & beta=2 & sigma=3 & n=200 & 1.64 \\ 
  142 & MME & sigma & beta=2 & sigma=3 & n=200 & 10.14 \\ 
  143 & MME.b & sigma & beta=2 & sigma=3 & n=200 & 18.58 \\ 
  144 & PWM & sigma & beta=2 & sigma=3 & n=200 & 1.62 \\ 
  145 & MLE & beta & beta=2.5 & sigma=3 & n=200 & 3.56 \\ 
  146 & MLE.b & beta & beta=2.5 & sigma=3 & n=200 & 3.14 \\ 
  147 & LME & beta & beta=2.5 & sigma=3 & n=200 & 2.24 \\ 
  148 & MDE.Phi.chisq & beta & beta=2.5 & sigma=3 & n=200 & 15.19 \\ 
  149 & MDE.Phi.tv & beta & beta=2.5 & sigma=3 & n=200 & 10.67 \\ 
  150 & MDE.Phi.kl & beta & beta=2.5 & sigma=3 & n=200 & 2.94 \\ 
  151 & MME & beta & beta=2.5 & sigma=3 & n=200 & 6.90 \\ 
  152 & MME.b & beta & beta=2.5 & sigma=3 & n=200 & 164.99 \\ 
  153 & PWM & beta & beta=2.5 & sigma=3 & n=200 & 2.24 \\ 
  154 & MLE & sigma & beta=2.5 & sigma=3 & n=200 & 9.26 \\ 
  155 & MLE.b & sigma & beta=2.5 & sigma=3 & n=200 & 8.17 \\ 
  156 & LME & sigma & beta=2.5 & sigma=3 & n=200 & 5.37 \\ 
  157 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=3 & n=200 & 69.23 \\ 
  158 & MDE.Phi.tv & sigma & beta=2.5 & sigma=3 & n=200 & 49.19 \\ 
  159 & MDE.Phi.kl & sigma & beta=2.5 & sigma=3 & n=200 & 8.02 \\ 
  160 & MME & sigma & beta=2.5 & sigma=3 & n=200 & 19.79 \\ 
  161 & MME.b & sigma & beta=2.5 & sigma=3 & n=200 & 500.19 \\ 
  162 & PWM & sigma & beta=2.5 & sigma=3 & n=200 & 5.37 \\ 
  163 & MLE & beta & beta=3 & sigma=3 & n=200 & 5.40 \\ 
  164 & MLE.b & beta & beta=3 & sigma=3 & n=200 & 4.81 \\ 
  165 & LME & beta & beta=3 & sigma=3 & n=200 & 3.45 \\ 
  166 & MDE.Phi.chisq & beta & beta=3 & sigma=3 & n=200 & 70.59 \\ 
  167 & MDE.Phi.tv & beta & beta=3 & sigma=3 & n=200 & 59.28 \\ 
  168 & MDE.Phi.kl & beta & beta=3 & sigma=3 & n=200 & 5.30 \\ 
  169 & MME & beta & beta=3 & sigma=3 & n=200 & 8.86 \\ 
  170 & MME.b & beta & beta=3 & sigma=3 & n=200 & 453.87 \\ 
  171 & PWM & beta & beta=3 & sigma=3 & n=200 & 3.45 \\ 
  172 & MLE & sigma & beta=3 & sigma=3 & n=200 & 9.04 \\ 
  173 & MLE.b & sigma & beta=3 & sigma=3 & n=200 & 8.00 \\ 
  174 & LME & sigma & beta=3 & sigma=3 & n=200 & 5.24 \\ 
  175 & MDE.Phi.chisq & sigma & beta=3 & sigma=3 & n=200 & 218.64 \\ 
  176 & MDE.Phi.tv & sigma & beta=3 & sigma=3 & n=200 & 170.51 \\ 
  177 & MDE.Phi.kl & sigma & beta=3 & sigma=3 & n=200 & 8.50 \\ 
  178 & MME & sigma & beta=3 & sigma=3 & n=200 & 15.08 \\ 
  179 & MME.b & sigma & beta=3 & sigma=3 & n=200 & 756.73 \\ 
  180 & PWM & sigma & beta=3 & sigma=3 & n=200 & 5.24 \\ 
  181 & MLE & beta & beta=4 & sigma=3 & n=200 & 2069.57 \\ 
  182 & MLE.b & beta & beta=4 & sigma=3 & n=200 & 2069.36 \\ 
  183 & LME & beta & beta=4 & sigma=3 & n=200 & 17.60 \\ 
  184 & MDE.Phi.chisq & beta & beta=4 & sigma=3 & n=200 & 456.47 \\ 
  185 & MDE.Phi.tv & beta & beta=4 & sigma=3 & n=200 & 306.42 \\ 
  186 & MDE.Phi.kl & beta & beta=4 & sigma=3 & n=200 & 63.88 \\ 
  187 & MME & beta & beta=4 & sigma=3 & n=200 & 1493.43 \\ 
  188 & MME.b & beta & beta=4 & sigma=3 & n=200 & 10651.19 \\ 
  189 & PWM & beta & beta=4 & sigma=3 & n=200 & 17.60 \\ 
  190 & MLE & sigma & beta=4 & sigma=3 & n=200 & 1655.86 \\ 
  191 & MLE.b & sigma & beta=4 & sigma=3 & n=200 & 1655.63 \\ 
  192 & LME & sigma & beta=4 & sigma=3 & n=200 & 14.38 \\ 
  193 & MDE.Phi.chisq & sigma & beta=4 & sigma=3 & n=200 & 679.07 \\ 
  194 & MDE.Phi.tv & sigma & beta=4 & sigma=3 & n=200 & 434.62 \\ 
  195 & MDE.Phi.kl & sigma & beta=4 & sigma=3 & n=200 & 52.93 \\ 
  196 & MME & sigma & beta=4 & sigma=3 & n=200 & 1248.51 \\ 
  197 & MME.b & sigma & beta=4 & sigma=3 & n=200 & 9783.19 \\ 
  198 & PWM & sigma & beta=4 & sigma=3 & n=200 & 14.38 \\ 
  199 & MLE & beta & beta=5 & sigma=3 & n=200 & 6750.00 \\ 
  200 & MLE.b & beta & beta=5 & sigma=3 & n=200 & 6750.82 \\ 
  201 & LME & beta & beta=5 & sigma=3 & n=200 & 51.27 \\ 
  202 & MDE.Phi.chisq & beta & beta=5 & sigma=3 & n=200 & 1093.20 \\ 
  203 & MDE.Phi.tv & beta & beta=5 & sigma=3 & n=200 & 707.84 \\ 
  204 & MDE.Phi.kl & beta & beta=5 & sigma=3 & n=200 & 144.82 \\ 
  205 & MME & beta & beta=5 & sigma=3 & n=200 & 352371.49 \\ 
  206 & MME.b & beta & beta=5 & sigma=3 & n=200 & 1490156.21 \\ 
  207 & PWM & beta & beta=5 & sigma=3 & n=200 & 51.27 \\ 
  208 & MLE & sigma & beta=5 & sigma=3 & n=200 & 3950.47 \\ 
  209 & MLE.b & sigma & beta=5 & sigma=3 & n=200 & 3950.84 \\ 
  210 & LME & sigma & beta=5 & sigma=3 & n=200 & 26.20 \\ 
  211 & MDE.Phi.chisq & sigma & beta=5 & sigma=3 & n=200 & 965.66 \\ 
  212 & MDE.Phi.tv & sigma & beta=5 & sigma=3 & n=200 & 587.05 \\ 
  213 & MDE.Phi.kl & sigma & beta=5 & sigma=3 & n=200 & 71.05 \\ 
  214 & MME & sigma & beta=5 & sigma=3 & n=200 & 179596.50 \\ 
  215 & MME.b & sigma & beta=5 & sigma=3 & n=200 & 767443.03 \\ 
  216 & PWM & sigma & beta=5 & sigma=3 & n=200 & 26.20 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220201/Output.var.LaTeX.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Mon Jan 31 15:48:14 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=3 & n=100 & 0.44 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=3 & n=100 & 0.32 \\ 
  3 & LME & beta & beta=1.5 & sigma=3 & n=100 & 0.30 \\ 
  4 & MDE.Phi.chisq & beta & beta=1.5 & sigma=3 & n=100 & 347.78 \\ 
  5 & MDE.Phi.tv & beta & beta=1.5 & sigma=3 & n=100 & 6.22 \\ 
  6 & MDE.Phi.kl & beta & beta=1.5 & sigma=3 & n=100 & 0.44 \\ 
  7 & MME & beta & beta=1.5 & sigma=3 & n=100 & 0.90 \\ 
  8 & MME.b & beta & beta=1.5 & sigma=3 & n=100 & 130047.07 \\ 
  9 & PWM & beta & beta=1.5 & sigma=3 & n=100 & 0.30 \\ 
  10 & MLE & sigma & beta=1.5 & sigma=3 & n=100 & 4.40 \\ 
  11 & MLE.b & sigma & beta=1.5 & sigma=3 & n=100 & 3.25 \\ 
  12 & LME & sigma & beta=1.5 & sigma=3 & n=100 & 2.99 \\ 
  13 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=3 & n=100 & 173.39 \\ 
  14 & MDE.Phi.tv & sigma & beta=1.5 & sigma=3 & n=100 & 144.67 \\ 
  15 & MDE.Phi.kl & sigma & beta=1.5 & sigma=3 & n=100 & 4.41 \\ 
  16 & MME & sigma & beta=1.5 & sigma=3 & n=100 & 17.93 \\ 
  17 & MME.b & sigma & beta=1.5 & sigma=3 & n=100 & 1340019.70 \\ 
  18 & PWM & sigma & beta=1.5 & sigma=3 & n=100 & 2.99 \\ 
  19 & MLE & beta & beta=2 & sigma=3 & n=100 & 50.24 \\ 
  20 & MLE.b & beta & beta=2 & sigma=3 & n=100 & 50.23 \\ 
  21 & LME & beta & beta=2 & sigma=3 & n=100 & 3.11 \\ 
  22 & MDE.Phi.chisq & beta & beta=2 & sigma=3 & n=100 & 65.32 \\ 
  23 & MDE.Phi.tv & beta & beta=2 & sigma=3 & n=100 & 78.47 \\ 
  24 & MDE.Phi.kl & beta & beta=2 & sigma=3 & n=100 & 11.32 \\ 
  25 & MME & beta & beta=2 & sigma=3 & n=100 & 52.88 \\ 
  26 & MME.b & beta & beta=2 & sigma=3 & n=100 & 151218.71 \\ 
  27 & PWM & beta & beta=2 & sigma=3 & n=100 & 3.11 \\ 
  28 & MLE & sigma & beta=2 & sigma=3 & n=100 & 162.89 \\ 
  29 & MLE.b & sigma & beta=2 & sigma=3 & n=100 & 162.71 \\ 
  30 & LME & sigma & beta=2 & sigma=3 & n=100 & 13.01 \\ 
  31 & MDE.Phi.chisq & sigma & beta=2 & sigma=3 & n=100 & 604.20 \\ 
  32 & MDE.Phi.tv & sigma & beta=2 & sigma=3 & n=100 & 766.97 \\ 
  33 & MDE.Phi.kl & sigma & beta=2 & sigma=3 & n=100 & 42.77 \\ 
  34 & MME & sigma & beta=2 & sigma=3 & n=100 & 205.69 \\ 
  35 & MME.b & sigma & beta=2 & sigma=3 & n=100 & 751939.68 \\ 
  36 & PWM & sigma & beta=2 & sigma=3 & n=100 & 13.01 \\ 
  37 & MLE & beta & beta=2.5 & sigma=3 & n=100 & 107.96 \\ 
  38 & MLE.b & beta & beta=2.5 & sigma=3 & n=100 & 108.59 \\ 
  39 & LME & beta & beta=2.5 & sigma=3 & n=100 & 8.34 \\ 
  40 & MDE.Phi.chisq & beta & beta=2.5 & sigma=3 & n=100 & 201.51 \\ 
  41 & MDE.Phi.tv & beta & beta=2.5 & sigma=3 & n=100 & 230.70 \\ 
  42 & MDE.Phi.kl & beta & beta=2.5 & sigma=3 & n=100 & 27.83 \\ 
  43 & MME & beta & beta=2.5 & sigma=3 & n=100 & 144.30 \\ 
  44 & MME.b & beta & beta=2.5 & sigma=3 & n=100 & 2214.14 \\ 
  45 & PWM & beta & beta=2.5 & sigma=3 & n=100 & 8.34 \\ 
  46 & MLE & sigma & beta=2.5 & sigma=3 & n=100 & 276.90 \\ 
  47 & MLE.b & sigma & beta=2.5 & sigma=3 & n=100 & 278.47 \\ 
  48 & LME & sigma & beta=2.5 & sigma=3 & n=100 & 20.24 \\ 
  49 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=3 & n=100 & 1089.17 \\ 
  50 & MDE.Phi.tv & sigma & beta=2.5 & sigma=3 & n=100 & 1237.71 \\ 
  51 & MDE.Phi.kl & sigma & beta=2.5 & sigma=3 & n=100 & 68.52 \\ 
  52 & MME & sigma & beta=2.5 & sigma=3 & n=100 & 337.82 \\ 
  53 & MME.b & sigma & beta=2.5 & sigma=3 & n=100 & 5685.29 \\ 
  54 & PWM & sigma & beta=2.5 & sigma=3 & n=100 & 20.24 \\ 
  55 & MLE & beta & beta=3 & sigma=3 & n=100 & 677.87 \\ 
  56 & MLE.b & beta & beta=3 & sigma=3 & n=100 & 680.40 \\ 
  57 & LME & beta & beta=3 & sigma=3 & n=100 & 15.99 \\ 
  58 & MDE.Phi.chisq & beta & beta=3 & sigma=3 & n=100 & 428.37 \\ 
  59 & MDE.Phi.tv & beta & beta=3 & sigma=3 & n=100 & 508.61 \\ 
  60 & MDE.Phi.kl & beta & beta=3 & sigma=3 & n=100 & 92.20 \\ 
  61 & MME & beta & beta=3 & sigma=3 & n=100 & 313146.34 \\ 
  62 & MME.b & beta & beta=3 & sigma=3 & n=100 & 2977375.68 \\ 
  63 & PWM & beta & beta=3 & sigma=3 & n=100 & 15.99 \\ 
  64 & MLE & sigma & beta=3 & sigma=3 & n=100 & 1161.82 \\ 
  65 & MLE.b & sigma & beta=3 & sigma=3 & n=100 & 1165.96 \\ 
  66 & LME & sigma & beta=3 & sigma=3 & n=100 & 27.75 \\ 
  67 & MDE.Phi.chisq & sigma & beta=3 & sigma=3 & n=100 & 1517.48 \\ 
  68 & MDE.Phi.tv & sigma & beta=3 & sigma=3 & n=100 & 1763.67 \\ 
  69 & MDE.Phi.kl & sigma & beta=3 & sigma=3 & n=100 & 155.00 \\ 
  70 & MME & sigma & beta=3 & sigma=3 & n=100 & 406904.25 \\ 
  71 & MME.b & sigma & beta=3 & sigma=3 & n=100 & 3873116.03 \\ 
  72 & PWM & sigma & beta=3 & sigma=3 & n=100 & 27.75 \\ 
  73 & MLE & beta & beta=4 & sigma=3 & n=100 & 1294.79 \\ 
  74 & MLE.b & beta & beta=4 & sigma=3 & n=100 & 1299.63 \\ 
  75 & LME & beta & beta=4 & sigma=3 & n=100 & 46.48 \\ 
  76 & MDE.Phi.chisq & beta & beta=4 & sigma=3 & n=100 & 1047.11 \\ 
  77 & MDE.Phi.tv & beta & beta=4 & sigma=3 & n=100 & 1197.44 \\ 
  78 & MDE.Phi.kl & beta & beta=4 & sigma=3 & n=100 & 187.36 \\ 
  79 & MME & beta & beta=4 & sigma=3 & n=100 & 11556.83 \\ 
  80 & MME.b & beta & beta=4 & sigma=3 & n=100 & 1921162.17 \\ 
  81 & PWM & beta & beta=4 & sigma=3 & n=100 & 46.48 \\ 
  82 & MLE & sigma & beta=4 & sigma=3 & n=100 & 1086.97 \\ 
  83 & MLE.b & sigma & beta=4 & sigma=3 & n=100 & 1091.00 \\ 
  84 & LME & sigma & beta=4 & sigma=3 & n=100 & 40.89 \\ 
  85 & MDE.Phi.chisq & sigma & beta=4 & sigma=3 & n=100 & 1826.97 \\ 
  86 & MDE.Phi.tv & sigma & beta=4 & sigma=3 & n=100 & 1987.71 \\ 
  87 & MDE.Phi.kl & sigma & beta=4 & sigma=3 & n=100 & 166.42 \\ 
  88 & MME & sigma & beta=4 & sigma=3 & n=100 & 9778.88 \\ 
  89 & MME.b & sigma & beta=4 & sigma=3 & n=100 & 2434977.19 \\ 
  90 & PWM & sigma & beta=4 & sigma=3 & n=100 & 40.89 \\ 
  91 & MLE & beta & beta=5 & sigma=3 & n=100 & 2400.46 \\ 
  92 & MLE.b & beta & beta=5 & sigma=3 & n=100 & 2407.01 \\ 
  93 & LME & beta & beta=5 & sigma=3 & n=100 & 87.34 \\ 
  94 & MDE.Phi.chisq & beta & beta=5 & sigma=3 & n=100 & 1624.25 \\ 
  95 & MDE.Phi.tv & beta & beta=5 & sigma=3 & n=100 & 1742.16 \\ 
  96 & MDE.Phi.kl & beta & beta=5 & sigma=3 & n=100 & 319.00 \\ 
  97 & MME & beta & beta=5 & sigma=3 & n=100 & 18586.56 \\ 
  98 & MME.b & beta & beta=5 & sigma=3 & n=100 & 257834.88 \\ 
  99 & PWM & beta & beta=5 & sigma=3 & n=100 & 87.34 \\ 
  100 & MLE & sigma & beta=5 & sigma=3 & n=100 & 1208.85 \\ 
  101 & MLE.b & sigma & beta=5 & sigma=3 & n=100 & 1212.05 \\ 
  102 & LME & sigma & beta=5 & sigma=3 & n=100 & 44.05 \\ 
  103 & MDE.Phi.chisq & sigma & beta=5 & sigma=3 & n=100 & 1635.55 \\ 
  104 & MDE.Phi.tv & sigma & beta=5 & sigma=3 & n=100 & 1683.51 \\ 
  105 & MDE.Phi.kl & sigma & beta=5 & sigma=3 & n=100 & 159.47 \\ 
  106 & MME & sigma & beta=5 & sigma=3 & n=100 & 9330.58 \\ 
  107 & MME.b & sigma & beta=5 & sigma=3 & n=100 & 139016.90 \\ 
  108 & PWM & sigma & beta=5 & sigma=3 & n=100 & 44.05 \\ 
  109 & MLE & beta & beta=1.5 & sigma=3 & n=200 & 0.11 \\ 
  110 & MLE.b & beta & beta=1.5 & sigma=3 & n=200 & 0.08 \\ 
  111 & LME & beta & beta=1.5 & sigma=3 & n=200 & 0.11 \\ 
  112 & MDE.Phi.chisq & beta & beta=1.5 & sigma=3 & n=200 & 64.59 \\ 
  113 & MDE.Phi.tv & beta & beta=1.5 & sigma=3 & n=200 & 0.18 \\ 
  114 & MDE.Phi.kl & beta & beta=1.5 & sigma=3 & n=200 & 0.11 \\ 
  115 & MME & beta & beta=1.5 & sigma=3 & n=200 & 0.17 \\ 
  116 & MME.b & beta & beta=1.5 & sigma=3 & n=200 & 0.19 \\ 
  117 & PWM & beta & beta=1.5 & sigma=3 & n=200 & 0.11 \\ 
  118 & MLE & sigma & beta=1.5 & sigma=3 & n=200 & 1.05 \\ 
  119 & MLE.b & sigma & beta=1.5 & sigma=3 & n=200 & 0.75 \\ 
  120 & LME & sigma & beta=1.5 & sigma=3 & n=200 & 1.12 \\ 
  121 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=3 & n=200 & 11.08 \\ 
  122 & MDE.Phi.tv & sigma & beta=1.5 & sigma=3 & n=200 & 2.62 \\ 
  123 & MDE.Phi.kl & sigma & beta=1.5 & sigma=3 & n=200 & 1.00 \\ 
  124 & MME & sigma & beta=1.5 & sigma=3 & n=200 & 61.56 \\ 
  125 & MME.b & sigma & beta=1.5 & sigma=3 & n=200 & 61.10 \\ 
  126 & PWM & sigma & beta=1.5 & sigma=3 & n=200 & 1.12 \\ 
  127 & MLE & beta & beta=2 & sigma=3 & n=200 & 0.33 \\ 
  128 & MLE.b & beta & beta=2 & sigma=3 & n=200 & 0.21 \\ 
  129 & LME & beta & beta=2 & sigma=3 & n=200 & 0.32 \\ 
  130 & MDE.Phi.chisq & beta & beta=2 & sigma=3 & n=200 & 0.63 \\ 
  131 & MDE.Phi.tv & beta & beta=2 & sigma=3 & n=200 & 0.93 \\ 
  132 & MDE.Phi.kl & beta & beta=2 & sigma=3 & n=200 & 0.34 \\ 
  133 & MME & beta & beta=2 & sigma=3 & n=200 & 0.60 \\ 
  134 & MME.b & beta & beta=2 & sigma=3 & n=200 & 2.22 \\ 
  135 & PWM & beta & beta=2 & sigma=3 & n=200 & 0.32 \\ 
  136 & MLE & sigma & beta=2 & sigma=3 & n=200 & 1.49 \\ 
  137 & MLE.b & sigma & beta=2 & sigma=3 & n=200 & 0.93 \\ 
  138 & LME & sigma & beta=2 & sigma=3 & n=200 & 1.41 \\ 
  139 & MDE.Phi.chisq & sigma & beta=2 & sigma=3 & n=200 & 4.73 \\ 
  140 & MDE.Phi.tv & sigma & beta=2 & sigma=3 & n=200 & 7.38 \\ 
  141 & MDE.Phi.kl & sigma & beta=2 & sigma=3 & n=200 & 1.53 \\ 
  142 & MME & sigma & beta=2 & sigma=3 & n=200 & 2.85 \\ 
  143 & MME.b & sigma & beta=2 & sigma=3 & n=200 & 15.03 \\ 
  144 & PWM & sigma & beta=2 & sigma=3 & n=200 & 1.41 \\ 
  145 & MLE & beta & beta=2.5 & sigma=3 & n=200 & 3.41 \\ 
  146 & MLE.b & beta & beta=2.5 & sigma=3 & n=200 & 3.14 \\ 
  147 & LME & beta & beta=2.5 & sigma=3 & n=200 & 2.14 \\ 
  148 & MDE.Phi.chisq & beta & beta=2.5 & sigma=3 & n=200 & 15.01 \\ 
  149 & MDE.Phi.tv & beta & beta=2.5 & sigma=3 & n=200 & 10.62 \\ 
  150 & MDE.Phi.kl & beta & beta=2.5 & sigma=3 & n=200 & 2.86 \\ 
  151 & MME & beta & beta=2.5 & sigma=3 & n=200 & 5.67 \\ 
  152 & MME.b & beta & beta=2.5 & sigma=3 & n=200 & 163.67 \\ 
  153 & PWM & beta & beta=2.5 & sigma=3 & n=200 & 2.14 \\ 
  154 & MLE & sigma & beta=2.5 & sigma=3 & n=200 & 8.89 \\ 
  155 & MLE.b & sigma & beta=2.5 & sigma=3 & n=200 & 8.16 \\ 
  156 & LME & sigma & beta=2.5 & sigma=3 & n=200 & 5.14 \\ 
  157 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=3 & n=200 & 68.02 \\ 
  158 & MDE.Phi.tv & sigma & beta=2.5 & sigma=3 & n=200 & 47.77 \\ 
  159 & MDE.Phi.kl & sigma & beta=2.5 & sigma=3 & n=200 & 7.81 \\ 
  160 & MME & sigma & beta=2.5 & sigma=3 & n=200 & 15.62 \\ 
  161 & MME.b & sigma & beta=2.5 & sigma=3 & n=200 & 495.87 \\ 
  162 & PWM & sigma & beta=2.5 & sigma=3 & n=200 & 5.14 \\ 
  163 & MLE & beta & beta=3 & sigma=3 & n=200 & 5.11 \\ 
  164 & MLE.b & beta & beta=3 & sigma=3 & n=200 & 4.80 \\ 
  165 & LME & beta & beta=3 & sigma=3 & n=200 & 3.28 \\ 
  166 & MDE.Phi.chisq & beta & beta=3 & sigma=3 & n=200 & 70.55 \\ 
  167 & MDE.Phi.tv & beta & beta=3 & sigma=3 & n=200 & 59.17 \\ 
  168 & MDE.Phi.kl & beta & beta=3 & sigma=3 & n=200 & 5.10 \\ 
  169 & MME & beta & beta=3 & sigma=3 & n=200 & 7.13 \\ 
  170 & MME.b & beta & beta=3 & sigma=3 & n=200 & 450.36 \\ 
  171 & PWM & beta & beta=3 & sigma=3 & n=200 & 3.28 \\ 
  172 & MLE & sigma & beta=3 & sigma=3 & n=200 & 8.54 \\ 
  173 & MLE.b & sigma & beta=3 & sigma=3 & n=200 & 8.00 \\ 
  174 & LME & sigma & beta=3 & sigma=3 & n=200 & 4.98 \\ 
  175 & MDE.Phi.chisq & sigma & beta=3 & sigma=3 & n=200 & 213.94 \\ 
  176 & MDE.Phi.tv & sigma & beta=3 & sigma=3 & n=200 & 166.43 \\ 
  177 & MDE.Phi.kl & sigma & beta=3 & sigma=3 & n=200 & 8.16 \\ 
  178 & MME & sigma & beta=3 & sigma=3 & n=200 & 11.68 \\ 
  179 & MME.b & sigma & beta=3 & sigma=3 & n=200 & 750.43 \\ 
  180 & PWM & sigma & beta=3 & sigma=3 & n=200 & 4.98 \\ 
  181 & MLE & beta & beta=4 & sigma=3 & n=200 & 2063.43 \\ 
  182 & MLE.b & beta & beta=4 & sigma=3 & n=200 & 2066.18 \\ 
  183 & LME & beta & beta=4 & sigma=3 & n=200 & 16.79 \\ 
  184 & MDE.Phi.chisq & beta & beta=4 & sigma=3 & n=200 & 443.01 \\ 
  185 & MDE.Phi.tv & beta & beta=4 & sigma=3 & n=200 & 299.06 \\ 
  186 & MDE.Phi.kl & beta & beta=4 & sigma=3 & n=200 & 61.88 \\ 
  187 & MME & beta & beta=4 & sigma=3 & n=200 & 1484.48 \\ 
  188 & MME.b & beta & beta=4 & sigma=3 & n=200 & 10585.66 \\ 
  189 & PWM & beta & beta=4 & sigma=3 & n=200 & 16.79 \\ 
  190 & MLE & sigma & beta=4 & sigma=3 & n=200 & 1650.53 \\ 
  191 & MLE.b & sigma & beta=4 & sigma=3 & n=200 & 1652.85 \\ 
  192 & LME & sigma & beta=4 & sigma=3 & n=200 & 13.72 \\ 
  193 & MDE.Phi.chisq & sigma & beta=4 & sigma=3 & n=200 & 643.90 \\ 
  194 & MDE.Phi.tv & sigma & beta=4 & sigma=3 & n=200 & 415.43 \\ 
  195 & MDE.Phi.kl & sigma & beta=4 & sigma=3 & n=200 & 51.26 \\ 
  196 & MME & sigma & beta=4 & sigma=3 & n=200 & 1240.68 \\ 
  197 & MME.b & sigma & beta=4 & sigma=3 & n=200 & 9726.22 \\ 
  198 & PWM & sigma & beta=4 & sigma=3 & n=200 & 13.72 \\ 
  199 & MLE & beta & beta=5 & sigma=3 & n=200 & 6726.23 \\ 
  200 & MLE.b & beta & beta=5 & sigma=3 & n=200 & 6733.62 \\ 
  201 & LME & beta & beta=5 & sigma=3 & n=200 & 48.52 \\ 
  202 & MDE.Phi.chisq & beta & beta=5 & sigma=3 & n=200 & 1015.64 \\ 
  203 & MDE.Phi.tv & beta & beta=5 & sigma=3 & n=200 & 670.70 \\ 
  204 & MDE.Phi.kl & beta & beta=5 & sigma=3 & n=200 & 138.16 \\ 
  205 & MME & beta & beta=5 & sigma=3 & n=200 & 352282.32 \\ 
  206 & MME.b & beta & beta=5 & sigma=3 & n=200 & 1489134.84 \\ 
  207 & PWM & beta & beta=5 & sigma=3 & n=200 & 48.52 \\ 
  208 & MLE & sigma & beta=5 & sigma=3 & n=200 & 3937.68 \\ 
  209 & MLE.b & sigma & beta=5 & sigma=3 & n=200 & 3941.49 \\ 
  210 & LME & sigma & beta=5 & sigma=3 & n=200 & 24.84 \\ 
  211 & MDE.Phi.chisq & sigma & beta=5 & sigma=3 & n=200 & 874.98 \\ 
  212 & MDE.Phi.tv & sigma & beta=5 & sigma=3 & n=200 & 544.52 \\ 
  213 & MDE.Phi.kl & sigma & beta=5 & sigma=3 & n=200 & 67.73 \\ 
  214 & MME & sigma & beta=5 & sigma=3 & n=200 & 179550.88 \\ 
  215 & MME.b & sigma & beta=5 & sigma=3 & n=200 & 766904.82 \\ 
  216 & PWM & sigma & beta=5 & sigma=3 & n=200 & 24.84 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220202/Full.beta=1.5.sig=1.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=1.5,  \sigma=1$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.6717&1.4777&1.8288&0.9856&1.2647&1.6717&2.7927&6.3149&1.8288
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.1822&0.9774&1.3253&1.5496&1.8315&1.1823&3.1525&6.8343&1.3253
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.435&0.3213&0.2958&12.6553&8.0716&0.4353&0.8967&130047.0683&0.2958
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.4894&0.3614&0.3325&22.0969&21.1246&0.4898&1.9924&148891.0805&0.3325
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1717&-0.0223&0.3288&-0.5144&-0.2353&0.1717&1.2927&4.8149&0.3288
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.1822&-0.0226&0.3253&0.5496&0.8315&0.1823&2.1525&5.8343&0.3253
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.4645&0.3218&0.4039&12.9187&8.1262&0.4648&2.5678&130057.2467&0.4039
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.5225&0.3619&0.4383&22.3968&21.8139&0.523&6.6253&148910.2304&0.4383
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 0.987&0.6836&0.8422&35.3154&29.9401&0.9877&9.1931&278967.4771&0.8422\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0011&0.0011&1.81787018350624e+299&0.0349&0.0011&0.0099&7.105&0.0011\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220202/Full.beta=1.5.sig=1.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=1.5,  \sigma=1$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.7302&1.6296&1.7056&0.8492&1.005&1.5782&2.495&2.296&1.7056
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.239&1.1321&1.2029&1.1239&1.2543&1.0818&2.7893&2.514&1.2029
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1038&0.0762&0.1121&0.1223&0.1688&0.1022&0.1646&0.258&0.1121
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.1147&0.0831&0.1242&0.2226&0.2908&0.1092&1.7813&1.8685&0.1242
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.2302&0.1296&0.2056&-0.6508&-0.495&0.0782&0.995&0.796&0.2056
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.239&0.1321&0.2029&0.1239&0.2543&0.0818&1.7893&1.514&0.2029
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1568&0.093&0.1544&0.5458&0.4138&0.1083&1.1547&0.8917&0.1544
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.1718&0.1005&0.1654&0.238&0.3554&0.1159&4.9829&4.1604&0.1654
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 0.3286&0.1935&0.3197&0.7838&0.7692&0.2242&6.1376&5.0521&0.3197\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 6e-04&6e-04&6e-04&0.0346&0.0271&6e-04&0.0089&0.0103&6e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220202/Full.beta=2.5.sig=1.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2.5,  \sigma=1$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 3.6254&3.1682&3.1958&4.3081&5.1489&3.4521&4.8214&7.9937&3.1958
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.6039&1.3562&1.3592&3.2275&3.7662&1.5109&2.3544&4.0216&1.3592
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 185.6331&186.3278&8.3445&278.8&316.2569&34.0267&144.3027&2205.727&8.3445
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
53.6322&53.8244&2.2484&166.8837&188.2544&9.3086&37.5351&630.075&2.2484
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.1254&0.6682&0.6958&1.8081&2.6489&0.9521&2.3214&5.4937&0.6958
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.6039&0.3562&0.3592&2.2275&2.7662&0.5109&1.3544&3.0216&0.3592
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 186.8811&186.7556&8.8279&282.0412&323.2418&34.9299&149.6771&2235.6866&8.8279
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
53.9916&53.9458&2.3772&171.8288&195.8876&9.5687&39.3658&639.1419&2.3772
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 240.8727&240.7014&11.2051&453.8699&519.1293&44.4986&189.0429&2874.8285&11.2051\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0012&0.0011&0.0233&0.0178&0.0011&0.0019&8.078&0.0011\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220202/Full.beta=2.5.sig=1.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2.5,  \sigma=1$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.844&2.5198&2.7839&2.0647&2.2867&2.7517&3.5621&3.3352&2.7839
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.1854&1.0095&1.1446&1.3611&1.411&1.1356&1.6546&1.5066&1.1446
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.4065&1.126&1.1971&22.0676&16.6289&1.1166&1.774&43.7477&1.1971
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.4142&0.33&0.3407&11.1329&7.9925&0.3315&0.5323&12.3153&0.3407
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.344&0.0198&0.2839&-0.4353&-0.2133&0.2517&1.0621&0.8352&0.2839
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.1854&0.0095&0.1446&0.3611&0.411&0.1356&0.6546&0.5066&0.1446
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.5247&1.1263&1.2776&22.2549&16.6727&1.1799&2.9019&44.4409&1.2776
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.4485&0.33&0.3616&11.2622&8.1606&0.3499&0.9608&12.5708&0.3616
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 1.9732&1.4563&1.6392&33.5171&24.8333&1.5297&3.8627&57.0117&1.6392\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&5e-04&5e-04&0.0174&0.0121&5e-04&0.0011&0.0017&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220202/Full.beta=2.sig=1.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2,  \sigma=1$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.5612&2.2116&2.4461&2.1496&2.768&2.465&3.6775&9.4751&2.4461
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.3857&1.133&1.3016&2.1521&2.6841&1.3282&2.4373&6.5865&1.3016
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 89.3791&89.3966&3.1121&79.2502&106.4853&14.1658&52.8831&151218.7131&3.1121
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
31.3225&31.3139&1.445&90.4215&115.3987&5.9178&22.8539&83548.852&1.445
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.5612&0.2116&0.4461&0.1496&0.768&0.465&1.6775&7.4751&0.4461
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.3857&0.133&0.3016&1.1521&1.6841&0.3282&1.4373&5.5865&0.3016
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 89.6851&89.4324&3.3109&79.2647&107.0645&14.3806&55.6919&151259.4685&3.3109
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
31.468&31.3285&1.5359&91.7397&118.2232&6.0249&24.9175&83571.7065&1.5359
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 121.1532&120.7609&4.8467&171.0044&225.2877&20.4055&80.6095&234831.175&4.8467\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0011&0.0011&0.0291&0.0229&0.0011&0.0035&0.0115&0.0011\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220202/Full.beta=2.sig=1.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2,  \sigma=1$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.2513&2.0633&2.2157&1.3484&1.5649&2.1373&2.9722&2.6877&2.2157
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.1763&1.0412&1.1419&1.1731&1.2796&1.0964&1.8886&1.6465&1.1419
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.3051&0.2007&0.3034&2.6102&2.5953&0.2965&0.5321&5.3987&0.3034
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.1517&0.0986&0.1498&2.1169&2.7239&0.147&0.2778&2.5505&0.1498
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.2513&0.0633&0.2157&-0.6516&-0.4351&0.1373&0.9722&0.6877&0.2157
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.1763&0.0412&0.1419&0.1731&0.2796&0.0964&0.8886&0.6465&0.1419
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.3682&0.2047&0.3499&3.0345&2.7844&0.3153&1.4772&5.8711&0.3499
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.1828&0.1003&0.1699&2.1466&2.8018&0.1563&1.0673&2.9682&0.1699
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 0.551&0.305&0.5198&5.1811&5.5862&0.4715&2.5445&8.8394&0.5198\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 6e-04&5e-04&5e-04&0.0226&0.0164&5e-04&0.0024&0.0024&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220202/Full.beta=3.sig=1.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=3,  \sigma=1$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 5.8945&5.4001&4.0159&7.279&8.7601&4.9247&17.4875&49.9897&4.0159
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2.2511&2.0375&1.4255&4.4093&5.1734&1.8285&6.7418&19.5688&1.4255
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1098.325&1101.1457&15.9909&606.1818&721.51&120.2505&313146.3373&2977375.7167&15.9909
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
217.5152&218.0324&3.0834&238.2619&277.2428&22.264&45211.5846&430346.239&3.0834
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.8945&2.4001&1.0159&4.279&5.7601&1.9247&14.4875&46.9897&1.0159
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.2511&1.0375&0.4255&3.4093&4.1734&0.8285&5.7418&18.5688&0.4255
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1106.5931&1106.7961&17.0213&624.4312&754.6165&123.9428&313324.9101&2979286.0078&17.0213
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
219.0586&219.087&3.2641&249.8612&294.6323&22.9483&45240.0317&430648.0045&3.2641
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 1325.6516&1325.8831&20.2855&874.2924&1049.2488&146.8911&358564.9418&3409934.0123&20.2855\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0012&0.0011&0.02&0.0152&0.0011&0.0014&0.0075&0.0011\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220202/Full.beta=3.sig=1.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=3,  \sigma=1$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 3.7155&3.2327&3.4536&3.382&3.2394&3.4946&4.4031&5.6933&3.4536
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.3092&1.0994&1.1893&1.8153&1.6143&1.2137&1.6462&2.2317&1.1893
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 175.5737&175.4235&4.1441&111.0688&52.0856&8.3477&73.0305&7346.8537&4.1441
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
29.1591&29.1248&0.7446&36.5505&15.8832&1.4733&11.8636&1681.4932&0.7446
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.7155&0.2327&0.4536&0.382&0.2394&0.4946&1.4031&2.6933&0.4536
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.3092&0.0994&0.1893&0.8153&0.6143&0.2137&0.6462&1.2317&0.1893
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 176.068&175.4601&4.3494&111.2036&52.1377&8.5915&74.9919&7353.3729&4.3494
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
29.2518&29.1318&0.7803&37.2115&16.259&1.5188&12.2801&1682.8422&0.7803
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 205.3198&204.5919&5.1297&148.4151&68.3966&10.1102&87.272&9036.2151&5.1297\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&5e-04&5e-04&0.0143&0.0096&5e-04&7e-04&0.0018&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220202/Full.beta=4.sig=1.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=4,  \sigma=1$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 8.8469&8.3977&5.759&14.9157&17.2826&7.523&11.3558&40.9124&5.759
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2.5008&2.3646&1.5351&6.4198&7.1968&2.0933&3.3327&13.4339&1.5351
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1737.8408&1742.9241&48.7724&1518.0529&1741.1556&232.1719&11556.9085&1921162.3133&48.7724
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
165.0907&165.5626&4.6902&294.1121&320.3164&23.0733&1086.5459&270553.0358&4.6902
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 4.8469&4.3977&1.759&10.9157&13.2826&3.523&7.3558&36.9124&1.759
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.5008&1.3646&0.5351&5.4198&6.1968&1.0933&2.3327&12.4339&0.5351
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1761.1597&1762.0899&51.8617&1637.0525&1917.4101&244.5603&11609.8605&1922332.7188&51.8617
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
167.3268&167.4082&4.9761&323.4568&358.6841&24.2662&1091.8789&270680.583&4.9761
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 1928.4865&1929.4982&56.8378&1960.5093&2276.0942&268.8265&12701.7394&2193013.3018&56.8378\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0012&0.001&0.0165&0.0123&0.0011&0.0011&4041.9544&0.001\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220202/Full.beta=4.sig=1.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=4,  \sigma=1$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 5.5863&4.9028&4.9147&8.1162&7.207&5.2726&6.6376&13.6854&4.9147
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.5001&1.29&1.2765&3.1661&2.6666&1.3921&1.831&4.1275&1.2765
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 171.5096&172.994&17.4485&586.961&428.971&46.2556&544.088&40207.1123&17.4485
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
16.9852&17.125&1.6376&95.7863&68.0682&4.3695&52.7303&4942.7143&1.6376
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.5863&0.9028&0.9147&4.1162&3.207&1.2726&2.6376&9.6854&0.9147
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.5001&0.29&0.2765&2.1661&1.6666&0.3921&0.831&3.1275&0.2765
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 174.0087&173.7918&18.2835&603.8454&439.2132&47.8704&550.9903&40296.8991&18.2835
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
17.2336&17.2074&1.7139&100.4688&70.839&4.5228&53.4156&4952.0011&1.7139
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 191.2423&190.9992&19.9974&704.3142&510.0522&52.3933&604.4059&45248.9002&19.9974\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&6e-04&5e-04&0.0111&0.0074&5e-04&6e-04&0.0029&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220202/Full.beta=5.sig=1.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=5,  \sigma=1$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 12.4819&12.1136&7.4119&21.9994&24.3588&10.2719&16.7627&47.2333&7.4119
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2.7615&2.6759&1.5623&7.2267&7.7657&2.2393&3.7561&10.9819&1.5623
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2933.8861&2940.689&104.922&2403.7816&2594.7578&410.2926&18595.7807&257869.7932&104.922
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
165.3419&165.7118&5.7845&268.5518&277.9779&22.5935&1037.1617&15447.9356&5.7845
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 7.4819&7.1136&2.4119&16.9994&19.3588&5.2719&11.7627&42.2333&2.4119
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.7615&1.6759&0.5623&6.2267&6.7657&1.2393&2.7561&9.9819&0.5623
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2989.5709&2990.9978&110.7288&2692.5197&2969.2601&438.0446&18732.2825&259627.6567&110.7288
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
168.4282&168.5039&6.1001&307.2964&323.7252&24.127&1044.6541&15546.0299&6.1001
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 3157.9991&3159.5017&116.8289&2999.8162&3292.9853&462.1716&19776.9366&275173.6866&116.8289\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.001&0.0012&0.001&0.0145&0.0106&0.001&0.001&5.15620838018139e+29&0.001\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220202/Full.beta=5.sig=1.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=5,  \sigma=1$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 9.9545&9.2435&6.8132&15.1377&12.05&7.6564&9.7632&21.5972&6.8132
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2.1969&2.0284&1.4243&4.5829&3.4635&1.6264&2.1335&4.9397&1.4243
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 10579.8946&10587.2719&68.4932&1448.479&977.1387&152.8998&2723.7425&30713.324&68.4932
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
611.8997&612.3167&3.8465&138.9351&88.9894&8.5202&148.047&1737.3608&3.8465
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 4.9545&4.2435&1.8132&10.1377&7.05&2.6564&4.7632&16.5972&1.8132
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.1969&1.0284&0.4243&3.5829&2.4635&0.6264&1.1335&3.9397&0.4243
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 10603.3839&10604.2204&71.774&1551.1072&1026.7434&159.9411&2746.1583&30985.7195&71.774
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
613.2709&613.313&4.0261&151.7583&95.0495&8.9117&149.3171&1752.7085&4.0261
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 11216.6549&11217.5334&75.8002&1702.8655&1121.7929&168.8527&2895.4754&32738.428&75.8002\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&6e-04&5e-04&0.0096&0.0062&5e-04&5e-04&2.018&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220202/Output.accuracy.LaTeX.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Tue Feb 01 15:44:07 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & Measure & beta=1.5 & sigma=1 & n=100 & 0.99 \\ 
  2 & MLE.b & Measure & beta=1.5 & sigma=1 & n=100 & 0.68 \\ 
  3 & LME & Measure & beta=1.5 & sigma=1 & n=100 & 0.84 \\ 
  4 & MDE.Phi.chisq & Measure & beta=1.5 & sigma=1 & n=100 & 35.32 \\ 
  5 & MDE.Phi.tv & Measure & beta=1.5 & sigma=1 & n=100 & 29.94 \\ 
  6 & MDE.Phi.kl & Measure & beta=1.5 & sigma=1 & n=100 & 0.99 \\ 
  7 & MME & Measure & beta=1.5 & sigma=1 & n=100 & 9.19 \\ 
  8 & MME.b & Measure & beta=1.5 & sigma=1 & n=100 & 278967.48 \\ 
  9 & PWM & Measure & beta=1.5 & sigma=1 & n=100 & 0.84 \\ 
  10 & MLE & Measure & beta=2 & sigma=1 & n=100 & 121.15 \\ 
  11 & MLE.b & Measure & beta=2 & sigma=1 & n=100 & 120.76 \\ 
  12 & LME & Measure & beta=2 & sigma=1 & n=100 & 4.85 \\ 
  13 & MDE.Phi.chisq & Measure & beta=2 & sigma=1 & n=100 & 171.00 \\ 
  14 & MDE.Phi.tv & Measure & beta=2 & sigma=1 & n=100 & 225.29 \\ 
  15 & MDE.Phi.kl & Measure & beta=2 & sigma=1 & n=100 & 20.41 \\ 
  16 & MME & Measure & beta=2 & sigma=1 & n=100 & 80.61 \\ 
  17 & MME.b & Measure & beta=2 & sigma=1 & n=100 & 234831.18 \\ 
  18 & PWM & Measure & beta=2 & sigma=1 & n=100 & 4.85 \\ 
  19 & MLE & Measure & beta=2.5 & sigma=1 & n=100 & 240.87 \\ 
  20 & MLE.b & Measure & beta=2.5 & sigma=1 & n=100 & 240.70 \\ 
  21 & LME & Measure & beta=2.5 & sigma=1 & n=100 & 11.21 \\ 
  22 & MDE.Phi.chisq & Measure & beta=2.5 & sigma=1 & n=100 & 453.87 \\ 
  23 & MDE.Phi.tv & Measure & beta=2.5 & sigma=1 & n=100 & 519.13 \\ 
  24 & MDE.Phi.kl & Measure & beta=2.5 & sigma=1 & n=100 & 44.50 \\ 
  25 & MME & Measure & beta=2.5 & sigma=1 & n=100 & 189.04 \\ 
  26 & MME.b & Measure & beta=2.5 & sigma=1 & n=100 & 2874.83 \\ 
  27 & PWM & Measure & beta=2.5 & sigma=1 & n=100 & 11.21 \\ 
  28 & MLE & Measure & beta=3 & sigma=1 & n=100 & 1325.65 \\ 
  29 & MLE.b & Measure & beta=3 & sigma=1 & n=100 & 1325.88 \\ 
  30 & LME & Measure & beta=3 & sigma=1 & n=100 & 20.29 \\ 
  31 & MDE.Phi.chisq & Measure & beta=3 & sigma=1 & n=100 & 874.29 \\ 
  32 & MDE.Phi.tv & Measure & beta=3 & sigma=1 & n=100 & 1049.25 \\ 
  33 & MDE.Phi.kl & Measure & beta=3 & sigma=1 & n=100 & 146.89 \\ 
  34 & MME & Measure & beta=3 & sigma=1 & n=100 & 358564.94 \\ 
  35 & MME.b & Measure & beta=3 & sigma=1 & n=100 & 3409934.01 \\ 
  36 & PWM & Measure & beta=3 & sigma=1 & n=100 & 20.29 \\ 
  37 & MLE & Measure & beta=4 & sigma=1 & n=100 & 1928.49 \\ 
  38 & MLE.b & Measure & beta=4 & sigma=1 & n=100 & 1929.50 \\ 
  39 & LME & Measure & beta=4 & sigma=1 & n=100 & 56.84 \\ 
  40 & MDE.Phi.chisq & Measure & beta=4 & sigma=1 & n=100 & 1960.51 \\ 
  41 & MDE.Phi.tv & Measure & beta=4 & sigma=1 & n=100 & 2276.09 \\ 
  42 & MDE.Phi.kl & Measure & beta=4 & sigma=1 & n=100 & 268.83 \\ 
  43 & MME & Measure & beta=4 & sigma=1 & n=100 & 12701.74 \\ 
  44 & MME.b & Measure & beta=4 & sigma=1 & n=100 & 2193013.30 \\ 
  45 & PWM & Measure & beta=4 & sigma=1 & n=100 & 56.84 \\ 
  46 & MLE & Measure & beta=5 & sigma=1 & n=100 & 3158.00 \\ 
  47 & MLE.b & Measure & beta=5 & sigma=1 & n=100 & 3159.50 \\ 
  48 & LME & Measure & beta=5 & sigma=1 & n=100 & 116.83 \\ 
  49 & MDE.Phi.chisq & Measure & beta=5 & sigma=1 & n=100 & 2999.82 \\ 
  50 & MDE.Phi.tv & Measure & beta=5 & sigma=1 & n=100 & 3292.99 \\ 
  51 & MDE.Phi.kl & Measure & beta=5 & sigma=1 & n=100 & 462.17 \\ 
  52 & MME & Measure & beta=5 & sigma=1 & n=100 & 19776.94 \\ 
  53 & MME.b & Measure & beta=5 & sigma=1 & n=100 & 275173.69 \\ 
  54 & PWM & Measure & beta=5 & sigma=1 & n=100 & 116.83 \\ 
  55 & MLE & Measure & beta=1.5 & sigma=1 & n=200 & 0.33 \\ 
  56 & MLE.b & Measure & beta=1.5 & sigma=1 & n=200 & 0.19 \\ 
  57 & LME & Measure & beta=1.5 & sigma=1 & n=200 & 0.32 \\ 
  58 & MDE.Phi.chisq & Measure & beta=1.5 & sigma=1 & n=200 & 0.78 \\ 
  59 & MDE.Phi.tv & Measure & beta=1.5 & sigma=1 & n=200 & 0.77 \\ 
  60 & MDE.Phi.kl & Measure & beta=1.5 & sigma=1 & n=200 & 0.22 \\ 
  61 & MME & Measure & beta=1.5 & sigma=1 & n=200 & 6.14 \\ 
  62 & MME.b & Measure & beta=1.5 & sigma=1 & n=200 & 5.05 \\ 
  63 & PWM & Measure & beta=1.5 & sigma=1 & n=200 & 0.32 \\ 
  64 & MLE & Measure & beta=2 & sigma=1 & n=200 & 0.55 \\ 
  65 & MLE.b & Measure & beta=2 & sigma=1 & n=200 & 0.31 \\ 
  66 & LME & Measure & beta=2 & sigma=1 & n=200 & 0.52 \\ 
  67 & MDE.Phi.chisq & Measure & beta=2 & sigma=1 & n=200 & 5.18 \\ 
  68 & MDE.Phi.tv & Measure & beta=2 & sigma=1 & n=200 & 5.59 \\ 
  69 & MDE.Phi.kl & Measure & beta=2 & sigma=1 & n=200 & 0.47 \\ 
  70 & MME & Measure & beta=2 & sigma=1 & n=200 & 2.54 \\ 
  71 & MME.b & Measure & beta=2 & sigma=1 & n=200 & 8.84 \\ 
  72 & PWM & Measure & beta=2 & sigma=1 & n=200 & 0.52 \\ 
  73 & MLE & Measure & beta=2.5 & sigma=1 & n=200 & 1.97 \\ 
  74 & MLE.b & Measure & beta=2.5 & sigma=1 & n=200 & 1.46 \\ 
  75 & LME & Measure & beta=2.5 & sigma=1 & n=200 & 1.64 \\ 
  76 & MDE.Phi.chisq & Measure & beta=2.5 & sigma=1 & n=200 & 33.52 \\ 
  77 & MDE.Phi.tv & Measure & beta=2.5 & sigma=1 & n=200 & 24.83 \\ 
  78 & MDE.Phi.kl & Measure & beta=2.5 & sigma=1 & n=200 & 1.53 \\ 
  79 & MME & Measure & beta=2.5 & sigma=1 & n=200 & 3.86 \\ 
  80 & MME.b & Measure & beta=2.5 & sigma=1 & n=200 & 57.01 \\ 
  81 & PWM & Measure & beta=2.5 & sigma=1 & n=200 & 1.64 \\ 
  82 & MLE & Measure & beta=3 & sigma=1 & n=200 & 205.32 \\ 
  83 & MLE.b & Measure & beta=3 & sigma=1 & n=200 & 204.59 \\ 
  84 & LME & Measure & beta=3 & sigma=1 & n=200 & 5.13 \\ 
  85 & MDE.Phi.chisq & Measure & beta=3 & sigma=1 & n=200 & 148.42 \\ 
  86 & MDE.Phi.tv & Measure & beta=3 & sigma=1 & n=200 & 68.40 \\ 
  87 & MDE.Phi.kl & Measure & beta=3 & sigma=1 & n=200 & 10.11 \\ 
  88 & MME & Measure & beta=3 & sigma=1 & n=200 & 87.27 \\ 
  89 & MME.b & Measure & beta=3 & sigma=1 & n=200 & 9036.22 \\ 
  90 & PWM & Measure & beta=3 & sigma=1 & n=200 & 5.13 \\ 
  91 & MLE & Measure & beta=4 & sigma=1 & n=200 & 191.24 \\ 
  92 & MLE.b & Measure & beta=4 & sigma=1 & n=200 & 191.00 \\ 
  93 & LME & Measure & beta=4 & sigma=1 & n=200 & 20.00 \\ 
  94 & MDE.Phi.chisq & Measure & beta=4 & sigma=1 & n=200 & 704.31 \\ 
  95 & MDE.Phi.tv & Measure & beta=4 & sigma=1 & n=200 & 510.05 \\ 
  96 & MDE.Phi.kl & Measure & beta=4 & sigma=1 & n=200 & 52.39 \\ 
  97 & MME & Measure & beta=4 & sigma=1 & n=200 & 604.41 \\ 
  98 & MME.b & Measure & beta=4 & sigma=1 & n=200 & 45248.90 \\ 
  99 & PWM & Measure & beta=4 & sigma=1 & n=200 & 20.00 \\ 
  100 & MLE & Measure & beta=5 & sigma=1 & n=200 & 11216.65 \\ 
  101 & MLE.b & Measure & beta=5 & sigma=1 & n=200 & 11217.53 \\ 
  102 & LME & Measure & beta=5 & sigma=1 & n=200 & 75.80 \\ 
  103 & MDE.Phi.chisq & Measure & beta=5 & sigma=1 & n=200 & 1702.87 \\ 
  104 & MDE.Phi.tv & Measure & beta=5 & sigma=1 & n=200 & 1121.79 \\ 
  105 & MDE.Phi.kl & Measure & beta=5 & sigma=1 & n=200 & 168.85 \\ 
  106 & MME & Measure & beta=5 & sigma=1 & n=200 & 2895.48 \\ 
  107 & MME.b & Measure & beta=5 & sigma=1 & n=200 & 32738.43 \\ 
  108 & PWM & Measure & beta=5 & sigma=1 & n=200 & 75.80 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220202/Output.accuracy2.LaTeX.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Tue Feb 01 15:44:07 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & Measure & beta=1.5 & sigma=1 & n=100 & 0.00 \\ 
  2 & MLE.b & Measure & beta=1.5 & sigma=1 & n=100 & 0.00 \\ 
  3 & LME & Measure & beta=1.5 & sigma=1 & n=100 & 0.00 \\ 
  4 & MDE.Phi.chisq & Measure & beta=1.5 & sigma=1 & n=100 & 181787018350624229332064482482084282602604822808686222086826422600406468626442880202480026068600642028200282242280222024246020860022848620402880404466644668026044682262046000244464684680404040648066066624288048682020048688026826682826820642682280002668866466086886864424642802262886688486208806684284.00 \\ 
  5 & MDE.Phi.tv & Measure & beta=1.5 & sigma=1 & n=100 & 0.03 \\ 
  6 & MDE.Phi.kl & Measure & beta=1.5 & sigma=1 & n=100 & 0.00 \\ 
  7 & MME & Measure & beta=1.5 & sigma=1 & n=100 & 0.01 \\ 
  8 & MME.b & Measure & beta=1.5 & sigma=1 & n=100 & 7.11 \\ 
  9 & PWM & Measure & beta=1.5 & sigma=1 & n=100 & 0.00 \\ 
  10 & MLE & Measure & beta=2 & sigma=1 & n=100 & 0.00 \\ 
  11 & MLE.b & Measure & beta=2 & sigma=1 & n=100 & 0.00 \\ 
  12 & LME & Measure & beta=2 & sigma=1 & n=100 & 0.00 \\ 
  13 & MDE.Phi.chisq & Measure & beta=2 & sigma=1 & n=100 & 0.03 \\ 
  14 & MDE.Phi.tv & Measure & beta=2 & sigma=1 & n=100 & 0.02 \\ 
  15 & MDE.Phi.kl & Measure & beta=2 & sigma=1 & n=100 & 0.00 \\ 
  16 & MME & Measure & beta=2 & sigma=1 & n=100 & 0.00 \\ 
  17 & MME.b & Measure & beta=2 & sigma=1 & n=100 & 0.01 \\ 
  18 & PWM & Measure & beta=2 & sigma=1 & n=100 & 0.00 \\ 
  19 & MLE & Measure & beta=2.5 & sigma=1 & n=100 & 0.00 \\ 
  20 & MLE.b & Measure & beta=2.5 & sigma=1 & n=100 & 0.00 \\ 
  21 & LME & Measure & beta=2.5 & sigma=1 & n=100 & 0.00 \\ 
  22 & MDE.Phi.chisq & Measure & beta=2.5 & sigma=1 & n=100 & 0.02 \\ 
  23 & MDE.Phi.tv & Measure & beta=2.5 & sigma=1 & n=100 & 0.02 \\ 
  24 & MDE.Phi.kl & Measure & beta=2.5 & sigma=1 & n=100 & 0.00 \\ 
  25 & MME & Measure & beta=2.5 & sigma=1 & n=100 & 0.00 \\ 
  26 & MME.b & Measure & beta=2.5 & sigma=1 & n=100 & 8.08 \\ 
  27 & PWM & Measure & beta=2.5 & sigma=1 & n=100 & 0.00 \\ 
  28 & MLE & Measure & beta=3 & sigma=1 & n=100 & 0.00 \\ 
  29 & MLE.b & Measure & beta=3 & sigma=1 & n=100 & 0.00 \\ 
  30 & LME & Measure & beta=3 & sigma=1 & n=100 & 0.00 \\ 
  31 & MDE.Phi.chisq & Measure & beta=3 & sigma=1 & n=100 & 0.02 \\ 
  32 & MDE.Phi.tv & Measure & beta=3 & sigma=1 & n=100 & 0.02 \\ 
  33 & MDE.Phi.kl & Measure & beta=3 & sigma=1 & n=100 & 0.00 \\ 
  34 & MME & Measure & beta=3 & sigma=1 & n=100 & 0.00 \\ 
  35 & MME.b & Measure & beta=3 & sigma=1 & n=100 & 0.01 \\ 
  36 & PWM & Measure & beta=3 & sigma=1 & n=100 & 0.00 \\ 
  37 & MLE & Measure & beta=4 & sigma=1 & n=100 & 0.00 \\ 
  38 & MLE.b & Measure & beta=4 & sigma=1 & n=100 & 0.00 \\ 
  39 & LME & Measure & beta=4 & sigma=1 & n=100 & 0.00 \\ 
  40 & MDE.Phi.chisq & Measure & beta=4 & sigma=1 & n=100 & 0.02 \\ 
  41 & MDE.Phi.tv & Measure & beta=4 & sigma=1 & n=100 & 0.01 \\ 
  42 & MDE.Phi.kl & Measure & beta=4 & sigma=1 & n=100 & 0.00 \\ 
  43 & MME & Measure & beta=4 & sigma=1 & n=100 & 0.00 \\ 
  44 & MME.b & Measure & beta=4 & sigma=1 & n=100 & 4041.95 \\ 
  45 & PWM & Measure & beta=4 & sigma=1 & n=100 & 0.00 \\ 
  46 & MLE & Measure & beta=5 & sigma=1 & n=100 & 0.00 \\ 
  47 & MLE.b & Measure & beta=5 & sigma=1 & n=100 & 0.00 \\ 
  48 & LME & Measure & beta=5 & sigma=1 & n=100 & 0.00 \\ 
  49 & MDE.Phi.chisq & Measure & beta=5 & sigma=1 & n=100 & 0.01 \\ 
  50 & MDE.Phi.tv & Measure & beta=5 & sigma=1 & n=100 & 0.01 \\ 
  51 & MDE.Phi.kl & Measure & beta=5 & sigma=1 & n=100 & 0.00 \\ 
  52 & MME & Measure & beta=5 & sigma=1 & n=100 & 0.00 \\ 
  53 & MME.b & Measure & beta=5 & sigma=1 & n=100 & 515620838018138634806240604226.00 \\ 
  54 & PWM & Measure & beta=5 & sigma=1 & n=100 & 0.00 \\ 
  55 & MLE & Measure & beta=1.5 & sigma=1 & n=200 & 0.00 \\ 
  56 & MLE.b & Measure & beta=1.5 & sigma=1 & n=200 & 0.00 \\ 
  57 & LME & Measure & beta=1.5 & sigma=1 & n=200 & 0.00 \\ 
  58 & MDE.Phi.chisq & Measure & beta=1.5 & sigma=1 & n=200 & 0.03 \\ 
  59 & MDE.Phi.tv & Measure & beta=1.5 & sigma=1 & n=200 & 0.03 \\ 
  60 & MDE.Phi.kl & Measure & beta=1.5 & sigma=1 & n=200 & 0.00 \\ 
  61 & MME & Measure & beta=1.5 & sigma=1 & n=200 & 0.01 \\ 
  62 & MME.b & Measure & beta=1.5 & sigma=1 & n=200 & 0.01 \\ 
  63 & PWM & Measure & beta=1.5 & sigma=1 & n=200 & 0.00 \\ 
  64 & MLE & Measure & beta=2 & sigma=1 & n=200 & 0.00 \\ 
  65 & MLE.b & Measure & beta=2 & sigma=1 & n=200 & 0.00 \\ 
  66 & LME & Measure & beta=2 & sigma=1 & n=200 & 0.00 \\ 
  67 & MDE.Phi.chisq & Measure & beta=2 & sigma=1 & n=200 & 0.02 \\ 
  68 & MDE.Phi.tv & Measure & beta=2 & sigma=1 & n=200 & 0.02 \\ 
  69 & MDE.Phi.kl & Measure & beta=2 & sigma=1 & n=200 & 0.00 \\ 
  70 & MME & Measure & beta=2 & sigma=1 & n=200 & 0.00 \\ 
  71 & MME.b & Measure & beta=2 & sigma=1 & n=200 & 0.00 \\ 
  72 & PWM & Measure & beta=2 & sigma=1 & n=200 & 0.00 \\ 
  73 & MLE & Measure & beta=2.5 & sigma=1 & n=200 & 0.00 \\ 
  74 & MLE.b & Measure & beta=2.5 & sigma=1 & n=200 & 0.00 \\ 
  75 & LME & Measure & beta=2.5 & sigma=1 & n=200 & 0.00 \\ 
  76 & MDE.Phi.chisq & Measure & beta=2.5 & sigma=1 & n=200 & 0.02 \\ 
  77 & MDE.Phi.tv & Measure & beta=2.5 & sigma=1 & n=200 & 0.01 \\ 
  78 & MDE.Phi.kl & Measure & beta=2.5 & sigma=1 & n=200 & 0.00 \\ 
  79 & MME & Measure & beta=2.5 & sigma=1 & n=200 & 0.00 \\ 
  80 & MME.b & Measure & beta=2.5 & sigma=1 & n=200 & 0.00 \\ 
  81 & PWM & Measure & beta=2.5 & sigma=1 & n=200 & 0.00 \\ 
  82 & MLE & Measure & beta=3 & sigma=1 & n=200 & 0.00 \\ 
  83 & MLE.b & Measure & beta=3 & sigma=1 & n=200 & 0.00 \\ 
  84 & LME & Measure & beta=3 & sigma=1 & n=200 & 0.00 \\ 
  85 & MDE.Phi.chisq & Measure & beta=3 & sigma=1 & n=200 & 0.01 \\ 
  86 & MDE.Phi.tv & Measure & beta=3 & sigma=1 & n=200 & 0.01 \\ 
  87 & MDE.Phi.kl & Measure & beta=3 & sigma=1 & n=200 & 0.00 \\ 
  88 & MME & Measure & beta=3 & sigma=1 & n=200 & 0.00 \\ 
  89 & MME.b & Measure & beta=3 & sigma=1 & n=200 & 0.00 \\ 
  90 & PWM & Measure & beta=3 & sigma=1 & n=200 & 0.00 \\ 
  91 & MLE & Measure & beta=4 & sigma=1 & n=200 & 0.00 \\ 
  92 & MLE.b & Measure & beta=4 & sigma=1 & n=200 & 0.00 \\ 
  93 & LME & Measure & beta=4 & sigma=1 & n=200 & 0.00 \\ 
  94 & MDE.Phi.chisq & Measure & beta=4 & sigma=1 & n=200 & 0.01 \\ 
  95 & MDE.Phi.tv & Measure & beta=4 & sigma=1 & n=200 & 0.01 \\ 
  96 & MDE.Phi.kl & Measure & beta=4 & sigma=1 & n=200 & 0.00 \\ 
  97 & MME & Measure & beta=4 & sigma=1 & n=200 & 0.00 \\ 
  98 & MME.b & Measure & beta=4 & sigma=1 & n=200 & 0.00 \\ 
  99 & PWM & Measure & beta=4 & sigma=1 & n=200 & 0.00 \\ 
  100 & MLE & Measure & beta=5 & sigma=1 & n=200 & 0.00 \\ 
  101 & MLE.b & Measure & beta=5 & sigma=1 & n=200 & 0.00 \\ 
  102 & LME & Measure & beta=5 & sigma=1 & n=200 & 0.00 \\ 
  103 & MDE.Phi.chisq & Measure & beta=5 & sigma=1 & n=200 & 0.01 \\ 
  104 & MDE.Phi.tv & Measure & beta=5 & sigma=1 & n=200 & 0.01 \\ 
  105 & MDE.Phi.kl & Measure & beta=5 & sigma=1 & n=200 & 0.00 \\ 
  106 & MME & Measure & beta=5 & sigma=1 & n=200 & 0.00 \\ 
  107 & MME.b & Measure & beta=5 & sigma=1 & n=200 & 2.02 \\ 
  108 & PWM & Measure & beta=5 & sigma=1 & n=200 & 0.00 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220202/Output.bias.LaTeX.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Tue Feb 01 15:44:07 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=1 & n=100 & 0.17 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=1 & n=100 & -0.02 \\ 
  3 & LME & beta & beta=1.5 & sigma=1 & n=100 & 0.33 \\ 
  4 & MDE.Phi.chisq & beta & beta=1.5 & sigma=1 & n=100 & -0.51 \\ 
  5 & MDE.Phi.tv & beta & beta=1.5 & sigma=1 & n=100 & -0.24 \\ 
  6 & MDE.Phi.kl & beta & beta=1.5 & sigma=1 & n=100 & 0.17 \\ 
  7 & MME & beta & beta=1.5 & sigma=1 & n=100 & 1.29 \\ 
  8 & MME.b & beta & beta=1.5 & sigma=1 & n=100 & 4.81 \\ 
  9 & PWM & beta & beta=1.5 & sigma=1 & n=100 & 0.33 \\ 
  10 & MLE & sigma & beta=1.5 & sigma=1 & n=100 & 0.18 \\ 
  11 & MLE.b & sigma & beta=1.5 & sigma=1 & n=100 & -0.02 \\ 
  12 & LME & sigma & beta=1.5 & sigma=1 & n=100 & 0.33 \\ 
  13 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=1 & n=100 & 0.55 \\ 
  14 & MDE.Phi.tv & sigma & beta=1.5 & sigma=1 & n=100 & 0.83 \\ 
  15 & MDE.Phi.kl & sigma & beta=1.5 & sigma=1 & n=100 & 0.18 \\ 
  16 & MME & sigma & beta=1.5 & sigma=1 & n=100 & 2.15 \\ 
  17 & MME.b & sigma & beta=1.5 & sigma=1 & n=100 & 5.83 \\ 
  18 & PWM & sigma & beta=1.5 & sigma=1 & n=100 & 0.33 \\ 
  19 & MLE & beta & beta=2 & sigma=1 & n=100 & 0.56 \\ 
  20 & MLE.b & beta & beta=2 & sigma=1 & n=100 & 0.21 \\ 
  21 & LME & beta & beta=2 & sigma=1 & n=100 & 0.45 \\ 
  22 & MDE.Phi.chisq & beta & beta=2 & sigma=1 & n=100 & 0.15 \\ 
  23 & MDE.Phi.tv & beta & beta=2 & sigma=1 & n=100 & 0.77 \\ 
  24 & MDE.Phi.kl & beta & beta=2 & sigma=1 & n=100 & 0.47 \\ 
  25 & MME & beta & beta=2 & sigma=1 & n=100 & 1.68 \\ 
  26 & MME.b & beta & beta=2 & sigma=1 & n=100 & 7.48 \\ 
  27 & PWM & beta & beta=2 & sigma=1 & n=100 & 0.45 \\ 
  28 & MLE & sigma & beta=2 & sigma=1 & n=100 & 0.39 \\ 
  29 & MLE.b & sigma & beta=2 & sigma=1 & n=100 & 0.13 \\ 
  30 & LME & sigma & beta=2 & sigma=1 & n=100 & 0.30 \\ 
  31 & MDE.Phi.chisq & sigma & beta=2 & sigma=1 & n=100 & 1.15 \\ 
  32 & MDE.Phi.tv & sigma & beta=2 & sigma=1 & n=100 & 1.68 \\ 
  33 & MDE.Phi.kl & sigma & beta=2 & sigma=1 & n=100 & 0.33 \\ 
  34 & MME & sigma & beta=2 & sigma=1 & n=100 & 1.44 \\ 
  35 & MME.b & sigma & beta=2 & sigma=1 & n=100 & 5.59 \\ 
  36 & PWM & sigma & beta=2 & sigma=1 & n=100 & 0.30 \\ 
  37 & MLE & beta & beta=2.5 & sigma=1 & n=100 & 1.13 \\ 
  38 & MLE.b & beta & beta=2.5 & sigma=1 & n=100 & 0.67 \\ 
  39 & LME & beta & beta=2.5 & sigma=1 & n=100 & 0.70 \\ 
  40 & MDE.Phi.chisq & beta & beta=2.5 & sigma=1 & n=100 & 1.81 \\ 
  41 & MDE.Phi.tv & beta & beta=2.5 & sigma=1 & n=100 & 2.65 \\ 
  42 & MDE.Phi.kl & beta & beta=2.5 & sigma=1 & n=100 & 0.95 \\ 
  43 & MME & beta & beta=2.5 & sigma=1 & n=100 & 2.32 \\ 
  44 & MME.b & beta & beta=2.5 & sigma=1 & n=100 & 5.49 \\ 
  45 & PWM & beta & beta=2.5 & sigma=1 & n=100 & 0.70 \\ 
  46 & MLE & sigma & beta=2.5 & sigma=1 & n=100 & 0.60 \\ 
  47 & MLE.b & sigma & beta=2.5 & sigma=1 & n=100 & 0.36 \\ 
  48 & LME & sigma & beta=2.5 & sigma=1 & n=100 & 0.36 \\ 
  49 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=1 & n=100 & 2.23 \\ 
  50 & MDE.Phi.tv & sigma & beta=2.5 & sigma=1 & n=100 & 2.77 \\ 
  51 & MDE.Phi.kl & sigma & beta=2.5 & sigma=1 & n=100 & 0.51 \\ 
  52 & MME & sigma & beta=2.5 & sigma=1 & n=100 & 1.35 \\ 
  53 & MME.b & sigma & beta=2.5 & sigma=1 & n=100 & 3.02 \\ 
  54 & PWM & sigma & beta=2.5 & sigma=1 & n=100 & 0.36 \\ 
  55 & MLE & beta & beta=3 & sigma=1 & n=100 & 2.89 \\ 
  56 & MLE.b & beta & beta=3 & sigma=1 & n=100 & 2.40 \\ 
  57 & LME & beta & beta=3 & sigma=1 & n=100 & 1.02 \\ 
  58 & MDE.Phi.chisq & beta & beta=3 & sigma=1 & n=100 & 4.28 \\ 
  59 & MDE.Phi.tv & beta & beta=3 & sigma=1 & n=100 & 5.76 \\ 
  60 & MDE.Phi.kl & beta & beta=3 & sigma=1 & n=100 & 1.92 \\ 
  61 & MME & beta & beta=3 & sigma=1 & n=100 & 14.49 \\ 
  62 & MME.b & beta & beta=3 & sigma=1 & n=100 & 46.99 \\ 
  63 & PWM & beta & beta=3 & sigma=1 & n=100 & 1.02 \\ 
  64 & MLE & sigma & beta=3 & sigma=1 & n=100 & 1.25 \\ 
  65 & MLE.b & sigma & beta=3 & sigma=1 & n=100 & 1.04 \\ 
  66 & LME & sigma & beta=3 & sigma=1 & n=100 & 0.43 \\ 
  67 & MDE.Phi.chisq & sigma & beta=3 & sigma=1 & n=100 & 3.41 \\ 
  68 & MDE.Phi.tv & sigma & beta=3 & sigma=1 & n=100 & 4.17 \\ 
  69 & MDE.Phi.kl & sigma & beta=3 & sigma=1 & n=100 & 0.83 \\ 
  70 & MME & sigma & beta=3 & sigma=1 & n=100 & 5.74 \\ 
  71 & MME.b & sigma & beta=3 & sigma=1 & n=100 & 18.57 \\ 
  72 & PWM & sigma & beta=3 & sigma=1 & n=100 & 0.43 \\ 
  73 & MLE & beta & beta=4 & sigma=1 & n=100 & 4.85 \\ 
  74 & MLE.b & beta & beta=4 & sigma=1 & n=100 & 4.40 \\ 
  75 & LME & beta & beta=4 & sigma=1 & n=100 & 1.76 \\ 
  76 & MDE.Phi.chisq & beta & beta=4 & sigma=1 & n=100 & 10.92 \\ 
  77 & MDE.Phi.tv & beta & beta=4 & sigma=1 & n=100 & 13.28 \\ 
  78 & MDE.Phi.kl & beta & beta=4 & sigma=1 & n=100 & 3.52 \\ 
  79 & MME & beta & beta=4 & sigma=1 & n=100 & 7.36 \\ 
  80 & MME.b & beta & beta=4 & sigma=1 & n=100 & 36.91 \\ 
  81 & PWM & beta & beta=4 & sigma=1 & n=100 & 1.76 \\ 
  82 & MLE & sigma & beta=4 & sigma=1 & n=100 & 1.50 \\ 
  83 & MLE.b & sigma & beta=4 & sigma=1 & n=100 & 1.36 \\ 
  84 & LME & sigma & beta=4 & sigma=1 & n=100 & 0.54 \\ 
  85 & MDE.Phi.chisq & sigma & beta=4 & sigma=1 & n=100 & 5.42 \\ 
  86 & MDE.Phi.tv & sigma & beta=4 & sigma=1 & n=100 & 6.20 \\ 
  87 & MDE.Phi.kl & sigma & beta=4 & sigma=1 & n=100 & 1.09 \\ 
  88 & MME & sigma & beta=4 & sigma=1 & n=100 & 2.33 \\ 
  89 & MME.b & sigma & beta=4 & sigma=1 & n=100 & 12.43 \\ 
  90 & PWM & sigma & beta=4 & sigma=1 & n=100 & 0.54 \\ 
  91 & MLE & beta & beta=5 & sigma=1 & n=100 & 7.48 \\ 
  92 & MLE.b & beta & beta=5 & sigma=1 & n=100 & 7.11 \\ 
  93 & LME & beta & beta=5 & sigma=1 & n=100 & 2.41 \\ 
  94 & MDE.Phi.chisq & beta & beta=5 & sigma=1 & n=100 & 17.00 \\ 
  95 & MDE.Phi.tv & beta & beta=5 & sigma=1 & n=100 & 19.36 \\ 
  96 & MDE.Phi.kl & beta & beta=5 & sigma=1 & n=100 & 5.27 \\ 
  97 & MME & beta & beta=5 & sigma=1 & n=100 & 11.76 \\ 
  98 & MME.b & beta & beta=5 & sigma=1 & n=100 & 42.23 \\ 
  99 & PWM & beta & beta=5 & sigma=1 & n=100 & 2.41 \\ 
  100 & MLE & sigma & beta=5 & sigma=1 & n=100 & 1.76 \\ 
  101 & MLE.b & sigma & beta=5 & sigma=1 & n=100 & 1.68 \\ 
  102 & LME & sigma & beta=5 & sigma=1 & n=100 & 0.56 \\ 
  103 & MDE.Phi.chisq & sigma & beta=5 & sigma=1 & n=100 & 6.23 \\ 
  104 & MDE.Phi.tv & sigma & beta=5 & sigma=1 & n=100 & 6.77 \\ 
  105 & MDE.Phi.kl & sigma & beta=5 & sigma=1 & n=100 & 1.24 \\ 
  106 & MME & sigma & beta=5 & sigma=1 & n=100 & 2.76 \\ 
  107 & MME.b & sigma & beta=5 & sigma=1 & n=100 & 9.98 \\ 
  108 & PWM & sigma & beta=5 & sigma=1 & n=100 & 0.56 \\ 
  109 & MLE & beta & beta=1.5 & sigma=1 & n=200 & 0.23 \\ 
  110 & MLE.b & beta & beta=1.5 & sigma=1 & n=200 & 0.13 \\ 
  111 & LME & beta & beta=1.5 & sigma=1 & n=200 & 0.21 \\ 
  112 & MDE.Phi.chisq & beta & beta=1.5 & sigma=1 & n=200 & -0.65 \\ 
  113 & MDE.Phi.tv & beta & beta=1.5 & sigma=1 & n=200 & -0.49 \\ 
  114 & MDE.Phi.kl & beta & beta=1.5 & sigma=1 & n=200 & 0.08 \\ 
  115 & MME & beta & beta=1.5 & sigma=1 & n=200 & 1.00 \\ 
  116 & MME.b & beta & beta=1.5 & sigma=1 & n=200 & 0.80 \\ 
  117 & PWM & beta & beta=1.5 & sigma=1 & n=200 & 0.21 \\ 
  118 & MLE & sigma & beta=1.5 & sigma=1 & n=200 & 0.24 \\ 
  119 & MLE.b & sigma & beta=1.5 & sigma=1 & n=200 & 0.13 \\ 
  120 & LME & sigma & beta=1.5 & sigma=1 & n=200 & 0.20 \\ 
  121 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=1 & n=200 & 0.12 \\ 
  122 & MDE.Phi.tv & sigma & beta=1.5 & sigma=1 & n=200 & 0.25 \\ 
  123 & MDE.Phi.kl & sigma & beta=1.5 & sigma=1 & n=200 & 0.08 \\ 
  124 & MME & sigma & beta=1.5 & sigma=1 & n=200 & 1.79 \\ 
  125 & MME.b & sigma & beta=1.5 & sigma=1 & n=200 & 1.51 \\ 
  126 & PWM & sigma & beta=1.5 & sigma=1 & n=200 & 0.20 \\ 
  127 & MLE & beta & beta=2 & sigma=1 & n=200 & 0.25 \\ 
  128 & MLE.b & beta & beta=2 & sigma=1 & n=200 & 0.06 \\ 
  129 & LME & beta & beta=2 & sigma=1 & n=200 & 0.22 \\ 
  130 & MDE.Phi.chisq & beta & beta=2 & sigma=1 & n=200 & -0.65 \\ 
  131 & MDE.Phi.tv & beta & beta=2 & sigma=1 & n=200 & -0.44 \\ 
  132 & MDE.Phi.kl & beta & beta=2 & sigma=1 & n=200 & 0.14 \\ 
  133 & MME & beta & beta=2 & sigma=1 & n=200 & 0.97 \\ 
  134 & MME.b & beta & beta=2 & sigma=1 & n=200 & 0.69 \\ 
  135 & PWM & beta & beta=2 & sigma=1 & n=200 & 0.22 \\ 
  136 & MLE & sigma & beta=2 & sigma=1 & n=200 & 0.18 \\ 
  137 & MLE.b & sigma & beta=2 & sigma=1 & n=200 & 0.04 \\ 
  138 & LME & sigma & beta=2 & sigma=1 & n=200 & 0.14 \\ 
  139 & MDE.Phi.chisq & sigma & beta=2 & sigma=1 & n=200 & 0.17 \\ 
  140 & MDE.Phi.tv & sigma & beta=2 & sigma=1 & n=200 & 0.28 \\ 
  141 & MDE.Phi.kl & sigma & beta=2 & sigma=1 & n=200 & 0.10 \\ 
  142 & MME & sigma & beta=2 & sigma=1 & n=200 & 0.89 \\ 
  143 & MME.b & sigma & beta=2 & sigma=1 & n=200 & 0.65 \\ 
  144 & PWM & sigma & beta=2 & sigma=1 & n=200 & 0.14 \\ 
  145 & MLE & beta & beta=2.5 & sigma=1 & n=200 & 0.34 \\ 
  146 & MLE.b & beta & beta=2.5 & sigma=1 & n=200 & 0.02 \\ 
  147 & LME & beta & beta=2.5 & sigma=1 & n=200 & 0.28 \\ 
  148 & MDE.Phi.chisq & beta & beta=2.5 & sigma=1 & n=200 & -0.44 \\ 
  149 & MDE.Phi.tv & beta & beta=2.5 & sigma=1 & n=200 & -0.21 \\ 
  150 & MDE.Phi.kl & beta & beta=2.5 & sigma=1 & n=200 & 0.25 \\ 
  151 & MME & beta & beta=2.5 & sigma=1 & n=200 & 1.06 \\ 
  152 & MME.b & beta & beta=2.5 & sigma=1 & n=200 & 0.84 \\ 
  153 & PWM & beta & beta=2.5 & sigma=1 & n=200 & 0.28 \\ 
  154 & MLE & sigma & beta=2.5 & sigma=1 & n=200 & 0.19 \\ 
  155 & MLE.b & sigma & beta=2.5 & sigma=1 & n=200 & 0.01 \\ 
  156 & LME & sigma & beta=2.5 & sigma=1 & n=200 & 0.14 \\ 
  157 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=1 & n=200 & 0.36 \\ 
  158 & MDE.Phi.tv & sigma & beta=2.5 & sigma=1 & n=200 & 0.41 \\ 
  159 & MDE.Phi.kl & sigma & beta=2.5 & sigma=1 & n=200 & 0.14 \\ 
  160 & MME & sigma & beta=2.5 & sigma=1 & n=200 & 0.65 \\ 
  161 & MME.b & sigma & beta=2.5 & sigma=1 & n=200 & 0.51 \\ 
  162 & PWM & sigma & beta=2.5 & sigma=1 & n=200 & 0.14 \\ 
  163 & MLE & beta & beta=3 & sigma=1 & n=200 & 0.72 \\ 
  164 & MLE.b & beta & beta=3 & sigma=1 & n=200 & 0.23 \\ 
  165 & LME & beta & beta=3 & sigma=1 & n=200 & 0.45 \\ 
  166 & MDE.Phi.chisq & beta & beta=3 & sigma=1 & n=200 & 0.38 \\ 
  167 & MDE.Phi.tv & beta & beta=3 & sigma=1 & n=200 & 0.24 \\ 
  168 & MDE.Phi.kl & beta & beta=3 & sigma=1 & n=200 & 0.49 \\ 
  169 & MME & beta & beta=3 & sigma=1 & n=200 & 1.40 \\ 
  170 & MME.b & beta & beta=3 & sigma=1 & n=200 & 2.69 \\ 
  171 & PWM & beta & beta=3 & sigma=1 & n=200 & 0.45 \\ 
  172 & MLE & sigma & beta=3 & sigma=1 & n=200 & 0.31 \\ 
  173 & MLE.b & sigma & beta=3 & sigma=1 & n=200 & 0.10 \\ 
  174 & LME & sigma & beta=3 & sigma=1 & n=200 & 0.19 \\ 
  175 & MDE.Phi.chisq & sigma & beta=3 & sigma=1 & n=200 & 0.82 \\ 
  176 & MDE.Phi.tv & sigma & beta=3 & sigma=1 & n=200 & 0.61 \\ 
  177 & MDE.Phi.kl & sigma & beta=3 & sigma=1 & n=200 & 0.21 \\ 
  178 & MME & sigma & beta=3 & sigma=1 & n=200 & 0.65 \\ 
  179 & MME.b & sigma & beta=3 & sigma=1 & n=200 & 1.23 \\ 
  180 & PWM & sigma & beta=3 & sigma=1 & n=200 & 0.19 \\ 
  181 & MLE & beta & beta=4 & sigma=1 & n=200 & 1.59 \\ 
  182 & MLE.b & beta & beta=4 & sigma=1 & n=200 & 0.90 \\ 
  183 & LME & beta & beta=4 & sigma=1 & n=200 & 0.91 \\ 
  184 & MDE.Phi.chisq & beta & beta=4 & sigma=1 & n=200 & 4.12 \\ 
  185 & MDE.Phi.tv & beta & beta=4 & sigma=1 & n=200 & 3.21 \\ 
  186 & MDE.Phi.kl & beta & beta=4 & sigma=1 & n=200 & 1.27 \\ 
  187 & MME & beta & beta=4 & sigma=1 & n=200 & 2.64 \\ 
  188 & MME.b & beta & beta=4 & sigma=1 & n=200 & 9.69 \\ 
  189 & PWM & beta & beta=4 & sigma=1 & n=200 & 0.91 \\ 
  190 & MLE & sigma & beta=4 & sigma=1 & n=200 & 0.50 \\ 
  191 & MLE.b & sigma & beta=4 & sigma=1 & n=200 & 0.29 \\ 
  192 & LME & sigma & beta=4 & sigma=1 & n=200 & 0.28 \\ 
  193 & MDE.Phi.chisq & sigma & beta=4 & sigma=1 & n=200 & 2.17 \\ 
  194 & MDE.Phi.tv & sigma & beta=4 & sigma=1 & n=200 & 1.67 \\ 
  195 & MDE.Phi.kl & sigma & beta=4 & sigma=1 & n=200 & 0.39 \\ 
  196 & MME & sigma & beta=4 & sigma=1 & n=200 & 0.83 \\ 
  197 & MME.b & sigma & beta=4 & sigma=1 & n=200 & 3.13 \\ 
  198 & PWM & sigma & beta=4 & sigma=1 & n=200 & 0.28 \\ 
  199 & MLE & beta & beta=5 & sigma=1 & n=200 & 4.95 \\ 
  200 & MLE.b & beta & beta=5 & sigma=1 & n=200 & 4.24 \\ 
  201 & LME & beta & beta=5 & sigma=1 & n=200 & 1.81 \\ 
  202 & MDE.Phi.chisq & beta & beta=5 & sigma=1 & n=200 & 10.14 \\ 
  203 & MDE.Phi.tv & beta & beta=5 & sigma=1 & n=200 & 7.05 \\ 
  204 & MDE.Phi.kl & beta & beta=5 & sigma=1 & n=200 & 2.66 \\ 
  205 & MME & beta & beta=5 & sigma=1 & n=200 & 4.76 \\ 
  206 & MME.b & beta & beta=5 & sigma=1 & n=200 & 16.60 \\ 
  207 & PWM & beta & beta=5 & sigma=1 & n=200 & 1.81 \\ 
  208 & MLE & sigma & beta=5 & sigma=1 & n=200 & 1.20 \\ 
  209 & MLE.b & sigma & beta=5 & sigma=1 & n=200 & 1.03 \\ 
  210 & LME & sigma & beta=5 & sigma=1 & n=200 & 0.42 \\ 
  211 & MDE.Phi.chisq & sigma & beta=5 & sigma=1 & n=200 & 3.58 \\ 
  212 & MDE.Phi.tv & sigma & beta=5 & sigma=1 & n=200 & 2.46 \\ 
  213 & MDE.Phi.kl & sigma & beta=5 & sigma=1 & n=200 & 0.63 \\ 
  214 & MME & sigma & beta=5 & sigma=1 & n=200 & 1.13 \\ 
  215 & MME.b & sigma & beta=5 & sigma=1 & n=200 & 3.94 \\ 
  216 & PWM & sigma & beta=5 & sigma=1 & n=200 & 0.42 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220202/Output.mean.LaTeX.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Tue Feb 01 15:44:07 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=1 & n=100 & 1.67 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=1 & n=100 & 1.48 \\ 
  3 & LME & beta & beta=1.5 & sigma=1 & n=100 & 1.83 \\ 
  4 & MDE.Phi.chisq & beta & beta=1.5 & sigma=1 & n=100 & 0.99 \\ 
  5 & MDE.Phi.tv & beta & beta=1.5 & sigma=1 & n=100 & 1.26 \\ 
  6 & MDE.Phi.kl & beta & beta=1.5 & sigma=1 & n=100 & 1.67 \\ 
  7 & MME & beta & beta=1.5 & sigma=1 & n=100 & 2.79 \\ 
  8 & MME.b & beta & beta=1.5 & sigma=1 & n=100 & 6.31 \\ 
  9 & PWM & beta & beta=1.5 & sigma=1 & n=100 & 1.83 \\ 
  10 & MLE & sigma & beta=1.5 & sigma=1 & n=100 & 1.18 \\ 
  11 & MLE.b & sigma & beta=1.5 & sigma=1 & n=100 & 0.98 \\ 
  12 & LME & sigma & beta=1.5 & sigma=1 & n=100 & 1.33 \\ 
  13 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=1 & n=100 & 1.55 \\ 
  14 & MDE.Phi.tv & sigma & beta=1.5 & sigma=1 & n=100 & 1.83 \\ 
  15 & MDE.Phi.kl & sigma & beta=1.5 & sigma=1 & n=100 & 1.18 \\ 
  16 & MME & sigma & beta=1.5 & sigma=1 & n=100 & 3.15 \\ 
  17 & MME.b & sigma & beta=1.5 & sigma=1 & n=100 & 6.83 \\ 
  18 & PWM & sigma & beta=1.5 & sigma=1 & n=100 & 1.33 \\ 
  19 & MLE & beta & beta=2 & sigma=1 & n=100 & 2.56 \\ 
  20 & MLE.b & beta & beta=2 & sigma=1 & n=100 & 2.21 \\ 
  21 & LME & beta & beta=2 & sigma=1 & n=100 & 2.45 \\ 
  22 & MDE.Phi.chisq & beta & beta=2 & sigma=1 & n=100 & 2.15 \\ 
  23 & MDE.Phi.tv & beta & beta=2 & sigma=1 & n=100 & 2.77 \\ 
  24 & MDE.Phi.kl & beta & beta=2 & sigma=1 & n=100 & 2.47 \\ 
  25 & MME & beta & beta=2 & sigma=1 & n=100 & 3.68 \\ 
  26 & MME.b & beta & beta=2 & sigma=1 & n=100 & 9.48 \\ 
  27 & PWM & beta & beta=2 & sigma=1 & n=100 & 2.45 \\ 
  28 & MLE & sigma & beta=2 & sigma=1 & n=100 & 1.39 \\ 
  29 & MLE.b & sigma & beta=2 & sigma=1 & n=100 & 1.13 \\ 
  30 & LME & sigma & beta=2 & sigma=1 & n=100 & 1.30 \\ 
  31 & MDE.Phi.chisq & sigma & beta=2 & sigma=1 & n=100 & 2.15 \\ 
  32 & MDE.Phi.tv & sigma & beta=2 & sigma=1 & n=100 & 2.68 \\ 
  33 & MDE.Phi.kl & sigma & beta=2 & sigma=1 & n=100 & 1.33 \\ 
  34 & MME & sigma & beta=2 & sigma=1 & n=100 & 2.44 \\ 
  35 & MME.b & sigma & beta=2 & sigma=1 & n=100 & 6.59 \\ 
  36 & PWM & sigma & beta=2 & sigma=1 & n=100 & 1.30 \\ 
  37 & MLE & beta & beta=2.5 & sigma=1 & n=100 & 3.63 \\ 
  38 & MLE.b & beta & beta=2.5 & sigma=1 & n=100 & 3.17 \\ 
  39 & LME & beta & beta=2.5 & sigma=1 & n=100 & 3.20 \\ 
  40 & MDE.Phi.chisq & beta & beta=2.5 & sigma=1 & n=100 & 4.31 \\ 
  41 & MDE.Phi.tv & beta & beta=2.5 & sigma=1 & n=100 & 5.15 \\ 
  42 & MDE.Phi.kl & beta & beta=2.5 & sigma=1 & n=100 & 3.45 \\ 
  43 & MME & beta & beta=2.5 & sigma=1 & n=100 & 4.82 \\ 
  44 & MME.b & beta & beta=2.5 & sigma=1 & n=100 & 7.99 \\ 
  45 & PWM & beta & beta=2.5 & sigma=1 & n=100 & 3.20 \\ 
  46 & MLE & sigma & beta=2.5 & sigma=1 & n=100 & 1.60 \\ 
  47 & MLE.b & sigma & beta=2.5 & sigma=1 & n=100 & 1.36 \\ 
  48 & LME & sigma & beta=2.5 & sigma=1 & n=100 & 1.36 \\ 
  49 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=1 & n=100 & 3.23 \\ 
  50 & MDE.Phi.tv & sigma & beta=2.5 & sigma=1 & n=100 & 3.77 \\ 
  51 & MDE.Phi.kl & sigma & beta=2.5 & sigma=1 & n=100 & 1.51 \\ 
  52 & MME & sigma & beta=2.5 & sigma=1 & n=100 & 2.35 \\ 
  53 & MME.b & sigma & beta=2.5 & sigma=1 & n=100 & 4.02 \\ 
  54 & PWM & sigma & beta=2.5 & sigma=1 & n=100 & 1.36 \\ 
  55 & MLE & beta & beta=3 & sigma=1 & n=100 & 5.89 \\ 
  56 & MLE.b & beta & beta=3 & sigma=1 & n=100 & 5.40 \\ 
  57 & LME & beta & beta=3 & sigma=1 & n=100 & 4.02 \\ 
  58 & MDE.Phi.chisq & beta & beta=3 & sigma=1 & n=100 & 7.28 \\ 
  59 & MDE.Phi.tv & beta & beta=3 & sigma=1 & n=100 & 8.76 \\ 
  60 & MDE.Phi.kl & beta & beta=3 & sigma=1 & n=100 & 4.92 \\ 
  61 & MME & beta & beta=3 & sigma=1 & n=100 & 17.49 \\ 
  62 & MME.b & beta & beta=3 & sigma=1 & n=100 & 49.99 \\ 
  63 & PWM & beta & beta=3 & sigma=1 & n=100 & 4.02 \\ 
  64 & MLE & sigma & beta=3 & sigma=1 & n=100 & 2.25 \\ 
  65 & MLE.b & sigma & beta=3 & sigma=1 & n=100 & 2.04 \\ 
  66 & LME & sigma & beta=3 & sigma=1 & n=100 & 1.43 \\ 
  67 & MDE.Phi.chisq & sigma & beta=3 & sigma=1 & n=100 & 4.41 \\ 
  68 & MDE.Phi.tv & sigma & beta=3 & sigma=1 & n=100 & 5.17 \\ 
  69 & MDE.Phi.kl & sigma & beta=3 & sigma=1 & n=100 & 1.83 \\ 
  70 & MME & sigma & beta=3 & sigma=1 & n=100 & 6.74 \\ 
  71 & MME.b & sigma & beta=3 & sigma=1 & n=100 & 19.57 \\ 
  72 & PWM & sigma & beta=3 & sigma=1 & n=100 & 1.43 \\ 
  73 & MLE & beta & beta=4 & sigma=1 & n=100 & 8.85 \\ 
  74 & MLE.b & beta & beta=4 & sigma=1 & n=100 & 8.40 \\ 
  75 & LME & beta & beta=4 & sigma=1 & n=100 & 5.76 \\ 
  76 & MDE.Phi.chisq & beta & beta=4 & sigma=1 & n=100 & 14.92 \\ 
  77 & MDE.Phi.tv & beta & beta=4 & sigma=1 & n=100 & 17.28 \\ 
  78 & MDE.Phi.kl & beta & beta=4 & sigma=1 & n=100 & 7.52 \\ 
  79 & MME & beta & beta=4 & sigma=1 & n=100 & 11.36 \\ 
  80 & MME.b & beta & beta=4 & sigma=1 & n=100 & 40.91 \\ 
  81 & PWM & beta & beta=4 & sigma=1 & n=100 & 5.76 \\ 
  82 & MLE & sigma & beta=4 & sigma=1 & n=100 & 2.50 \\ 
  83 & MLE.b & sigma & beta=4 & sigma=1 & n=100 & 2.36 \\ 
  84 & LME & sigma & beta=4 & sigma=1 & n=100 & 1.54 \\ 
  85 & MDE.Phi.chisq & sigma & beta=4 & sigma=1 & n=100 & 6.42 \\ 
  86 & MDE.Phi.tv & sigma & beta=4 & sigma=1 & n=100 & 7.20 \\ 
  87 & MDE.Phi.kl & sigma & beta=4 & sigma=1 & n=100 & 2.09 \\ 
  88 & MME & sigma & beta=4 & sigma=1 & n=100 & 3.33 \\ 
  89 & MME.b & sigma & beta=4 & sigma=1 & n=100 & 13.43 \\ 
  90 & PWM & sigma & beta=4 & sigma=1 & n=100 & 1.54 \\ 
  91 & MLE & beta & beta=5 & sigma=1 & n=100 & 12.48 \\ 
  92 & MLE.b & beta & beta=5 & sigma=1 & n=100 & 12.11 \\ 
  93 & LME & beta & beta=5 & sigma=1 & n=100 & 7.41 \\ 
  94 & MDE.Phi.chisq & beta & beta=5 & sigma=1 & n=100 & 22.00 \\ 
  95 & MDE.Phi.tv & beta & beta=5 & sigma=1 & n=100 & 24.36 \\ 
  96 & MDE.Phi.kl & beta & beta=5 & sigma=1 & n=100 & 10.27 \\ 
  97 & MME & beta & beta=5 & sigma=1 & n=100 & 16.76 \\ 
  98 & MME.b & beta & beta=5 & sigma=1 & n=100 & 47.23 \\ 
  99 & PWM & beta & beta=5 & sigma=1 & n=100 & 7.41 \\ 
  100 & MLE & sigma & beta=5 & sigma=1 & n=100 & 2.76 \\ 
  101 & MLE.b & sigma & beta=5 & sigma=1 & n=100 & 2.68 \\ 
  102 & LME & sigma & beta=5 & sigma=1 & n=100 & 1.56 \\ 
  103 & MDE.Phi.chisq & sigma & beta=5 & sigma=1 & n=100 & 7.23 \\ 
  104 & MDE.Phi.tv & sigma & beta=5 & sigma=1 & n=100 & 7.77 \\ 
  105 & MDE.Phi.kl & sigma & beta=5 & sigma=1 & n=100 & 2.24 \\ 
  106 & MME & sigma & beta=5 & sigma=1 & n=100 & 3.76 \\ 
  107 & MME.b & sigma & beta=5 & sigma=1 & n=100 & 10.98 \\ 
  108 & PWM & sigma & beta=5 & sigma=1 & n=100 & 1.56 \\ 
  109 & MLE & beta & beta=1.5 & sigma=1 & n=200 & 1.73 \\ 
  110 & MLE.b & beta & beta=1.5 & sigma=1 & n=200 & 1.63 \\ 
  111 & LME & beta & beta=1.5 & sigma=1 & n=200 & 1.71 \\ 
  112 & MDE.Phi.chisq & beta & beta=1.5 & sigma=1 & n=200 & 0.85 \\ 
  113 & MDE.Phi.tv & beta & beta=1.5 & sigma=1 & n=200 & 1.01 \\ 
  114 & MDE.Phi.kl & beta & beta=1.5 & sigma=1 & n=200 & 1.58 \\ 
  115 & MME & beta & beta=1.5 & sigma=1 & n=200 & 2.50 \\ 
  116 & MME.b & beta & beta=1.5 & sigma=1 & n=200 & 2.30 \\ 
  117 & PWM & beta & beta=1.5 & sigma=1 & n=200 & 1.71 \\ 
  118 & MLE & sigma & beta=1.5 & sigma=1 & n=200 & 1.24 \\ 
  119 & MLE.b & sigma & beta=1.5 & sigma=1 & n=200 & 1.13 \\ 
  120 & LME & sigma & beta=1.5 & sigma=1 & n=200 & 1.20 \\ 
  121 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=1 & n=200 & 1.12 \\ 
  122 & MDE.Phi.tv & sigma & beta=1.5 & sigma=1 & n=200 & 1.25 \\ 
  123 & MDE.Phi.kl & sigma & beta=1.5 & sigma=1 & n=200 & 1.08 \\ 
  124 & MME & sigma & beta=1.5 & sigma=1 & n=200 & 2.79 \\ 
  125 & MME.b & sigma & beta=1.5 & sigma=1 & n=200 & 2.51 \\ 
  126 & PWM & sigma & beta=1.5 & sigma=1 & n=200 & 1.20 \\ 
  127 & MLE & beta & beta=2 & sigma=1 & n=200 & 2.25 \\ 
  128 & MLE.b & beta & beta=2 & sigma=1 & n=200 & 2.06 \\ 
  129 & LME & beta & beta=2 & sigma=1 & n=200 & 2.22 \\ 
  130 & MDE.Phi.chisq & beta & beta=2 & sigma=1 & n=200 & 1.35 \\ 
  131 & MDE.Phi.tv & beta & beta=2 & sigma=1 & n=200 & 1.56 \\ 
  132 & MDE.Phi.kl & beta & beta=2 & sigma=1 & n=200 & 2.14 \\ 
  133 & MME & beta & beta=2 & sigma=1 & n=200 & 2.97 \\ 
  134 & MME.b & beta & beta=2 & sigma=1 & n=200 & 2.69 \\ 
  135 & PWM & beta & beta=2 & sigma=1 & n=200 & 2.22 \\ 
  136 & MLE & sigma & beta=2 & sigma=1 & n=200 & 1.18 \\ 
  137 & MLE.b & sigma & beta=2 & sigma=1 & n=200 & 1.04 \\ 
  138 & LME & sigma & beta=2 & sigma=1 & n=200 & 1.14 \\ 
  139 & MDE.Phi.chisq & sigma & beta=2 & sigma=1 & n=200 & 1.17 \\ 
  140 & MDE.Phi.tv & sigma & beta=2 & sigma=1 & n=200 & 1.28 \\ 
  141 & MDE.Phi.kl & sigma & beta=2 & sigma=1 & n=200 & 1.10 \\ 
  142 & MME & sigma & beta=2 & sigma=1 & n=200 & 1.89 \\ 
  143 & MME.b & sigma & beta=2 & sigma=1 & n=200 & 1.65 \\ 
  144 & PWM & sigma & beta=2 & sigma=1 & n=200 & 1.14 \\ 
  145 & MLE & beta & beta=2.5 & sigma=1 & n=200 & 2.84 \\ 
  146 & MLE.b & beta & beta=2.5 & sigma=1 & n=200 & 2.52 \\ 
  147 & LME & beta & beta=2.5 & sigma=1 & n=200 & 2.78 \\ 
  148 & MDE.Phi.chisq & beta & beta=2.5 & sigma=1 & n=200 & 2.06 \\ 
  149 & MDE.Phi.tv & beta & beta=2.5 & sigma=1 & n=200 & 2.29 \\ 
  150 & MDE.Phi.kl & beta & beta=2.5 & sigma=1 & n=200 & 2.75 \\ 
  151 & MME & beta & beta=2.5 & sigma=1 & n=200 & 3.56 \\ 
  152 & MME.b & beta & beta=2.5 & sigma=1 & n=200 & 3.34 \\ 
  153 & PWM & beta & beta=2.5 & sigma=1 & n=200 & 2.78 \\ 
  154 & MLE & sigma & beta=2.5 & sigma=1 & n=200 & 1.19 \\ 
  155 & MLE.b & sigma & beta=2.5 & sigma=1 & n=200 & 1.01 \\ 
  156 & LME & sigma & beta=2.5 & sigma=1 & n=200 & 1.14 \\ 
  157 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=1 & n=200 & 1.36 \\ 
  158 & MDE.Phi.tv & sigma & beta=2.5 & sigma=1 & n=200 & 1.41 \\ 
  159 & MDE.Phi.kl & sigma & beta=2.5 & sigma=1 & n=200 & 1.14 \\ 
  160 & MME & sigma & beta=2.5 & sigma=1 & n=200 & 1.65 \\ 
  161 & MME.b & sigma & beta=2.5 & sigma=1 & n=200 & 1.51 \\ 
  162 & PWM & sigma & beta=2.5 & sigma=1 & n=200 & 1.14 \\ 
  163 & MLE & beta & beta=3 & sigma=1 & n=200 & 3.72 \\ 
  164 & MLE.b & beta & beta=3 & sigma=1 & n=200 & 3.23 \\ 
  165 & LME & beta & beta=3 & sigma=1 & n=200 & 3.45 \\ 
  166 & MDE.Phi.chisq & beta & beta=3 & sigma=1 & n=200 & 3.38 \\ 
  167 & MDE.Phi.tv & beta & beta=3 & sigma=1 & n=200 & 3.24 \\ 
  168 & MDE.Phi.kl & beta & beta=3 & sigma=1 & n=200 & 3.49 \\ 
  169 & MME & beta & beta=3 & sigma=1 & n=200 & 4.40 \\ 
  170 & MME.b & beta & beta=3 & sigma=1 & n=200 & 5.69 \\ 
  171 & PWM & beta & beta=3 & sigma=1 & n=200 & 3.45 \\ 
  172 & MLE & sigma & beta=3 & sigma=1 & n=200 & 1.31 \\ 
  173 & MLE.b & sigma & beta=3 & sigma=1 & n=200 & 1.10 \\ 
  174 & LME & sigma & beta=3 & sigma=1 & n=200 & 1.19 \\ 
  175 & MDE.Phi.chisq & sigma & beta=3 & sigma=1 & n=200 & 1.82 \\ 
  176 & MDE.Phi.tv & sigma & beta=3 & sigma=1 & n=200 & 1.61 \\ 
  177 & MDE.Phi.kl & sigma & beta=3 & sigma=1 & n=200 & 1.21 \\ 
  178 & MME & sigma & beta=3 & sigma=1 & n=200 & 1.65 \\ 
  179 & MME.b & sigma & beta=3 & sigma=1 & n=200 & 2.23 \\ 
  180 & PWM & sigma & beta=3 & sigma=1 & n=200 & 1.19 \\ 
  181 & MLE & beta & beta=4 & sigma=1 & n=200 & 5.59 \\ 
  182 & MLE.b & beta & beta=4 & sigma=1 & n=200 & 4.90 \\ 
  183 & LME & beta & beta=4 & sigma=1 & n=200 & 4.91 \\ 
  184 & MDE.Phi.chisq & beta & beta=4 & sigma=1 & n=200 & 8.12 \\ 
  185 & MDE.Phi.tv & beta & beta=4 & sigma=1 & n=200 & 7.21 \\ 
  186 & MDE.Phi.kl & beta & beta=4 & sigma=1 & n=200 & 5.27 \\ 
  187 & MME & beta & beta=4 & sigma=1 & n=200 & 6.64 \\ 
  188 & MME.b & beta & beta=4 & sigma=1 & n=200 & 13.69 \\ 
  189 & PWM & beta & beta=4 & sigma=1 & n=200 & 4.91 \\ 
  190 & MLE & sigma & beta=4 & sigma=1 & n=200 & 1.50 \\ 
  191 & MLE.b & sigma & beta=4 & sigma=1 & n=200 & 1.29 \\ 
  192 & LME & sigma & beta=4 & sigma=1 & n=200 & 1.28 \\ 
  193 & MDE.Phi.chisq & sigma & beta=4 & sigma=1 & n=200 & 3.17 \\ 
  194 & MDE.Phi.tv & sigma & beta=4 & sigma=1 & n=200 & 2.67 \\ 
  195 & MDE.Phi.kl & sigma & beta=4 & sigma=1 & n=200 & 1.39 \\ 
  196 & MME & sigma & beta=4 & sigma=1 & n=200 & 1.83 \\ 
  197 & MME.b & sigma & beta=4 & sigma=1 & n=200 & 4.13 \\ 
  198 & PWM & sigma & beta=4 & sigma=1 & n=200 & 1.28 \\ 
  199 & MLE & beta & beta=5 & sigma=1 & n=200 & 9.95 \\ 
  200 & MLE.b & beta & beta=5 & sigma=1 & n=200 & 9.24 \\ 
  201 & LME & beta & beta=5 & sigma=1 & n=200 & 6.81 \\ 
  202 & MDE.Phi.chisq & beta & beta=5 & sigma=1 & n=200 & 15.14 \\ 
  203 & MDE.Phi.tv & beta & beta=5 & sigma=1 & n=200 & 12.05 \\ 
  204 & MDE.Phi.kl & beta & beta=5 & sigma=1 & n=200 & 7.66 \\ 
  205 & MME & beta & beta=5 & sigma=1 & n=200 & 9.76 \\ 
  206 & MME.b & beta & beta=5 & sigma=1 & n=200 & 21.60 \\ 
  207 & PWM & beta & beta=5 & sigma=1 & n=200 & 6.81 \\ 
  208 & MLE & sigma & beta=5 & sigma=1 & n=200 & 2.20 \\ 
  209 & MLE.b & sigma & beta=5 & sigma=1 & n=200 & 2.03 \\ 
  210 & LME & sigma & beta=5 & sigma=1 & n=200 & 1.42 \\ 
  211 & MDE.Phi.chisq & sigma & beta=5 & sigma=1 & n=200 & 4.58 \\ 
  212 & MDE.Phi.tv & sigma & beta=5 & sigma=1 & n=200 & 3.46 \\ 
  213 & MDE.Phi.kl & sigma & beta=5 & sigma=1 & n=200 & 1.63 \\ 
  214 & MME & sigma & beta=5 & sigma=1 & n=200 & 2.13 \\ 
  215 & MME.b & sigma & beta=5 & sigma=1 & n=200 & 4.94 \\ 
  216 & PWM & sigma & beta=5 & sigma=1 & n=200 & 1.42 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220202/Output.mse.LaTeX.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Tue Feb 01 15:44:07 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=1 & n=100 & 0.46 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=1 & n=100 & 0.32 \\ 
  3 & LME & beta & beta=1.5 & sigma=1 & n=100 & 0.40 \\ 
  4 & MDE.Phi.chisq & beta & beta=1.5 & sigma=1 & n=100 & 12.92 \\ 
  5 & MDE.Phi.tv & beta & beta=1.5 & sigma=1 & n=100 & 8.13 \\ 
  6 & MDE.Phi.kl & beta & beta=1.5 & sigma=1 & n=100 & 0.46 \\ 
  7 & MME & beta & beta=1.5 & sigma=1 & n=100 & 2.57 \\ 
  8 & MME.b & beta & beta=1.5 & sigma=1 & n=100 & 130057.25 \\ 
  9 & PWM & beta & beta=1.5 & sigma=1 & n=100 & 0.40 \\ 
  10 & MLE & sigma & beta=1.5 & sigma=1 & n=100 & 0.52 \\ 
  11 & MLE.b & sigma & beta=1.5 & sigma=1 & n=100 & 0.36 \\ 
  12 & LME & sigma & beta=1.5 & sigma=1 & n=100 & 0.44 \\ 
  13 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=1 & n=100 & 22.40 \\ 
  14 & MDE.Phi.tv & sigma & beta=1.5 & sigma=1 & n=100 & 21.81 \\ 
  15 & MDE.Phi.kl & sigma & beta=1.5 & sigma=1 & n=100 & 0.52 \\ 
  16 & MME & sigma & beta=1.5 & sigma=1 & n=100 & 6.63 \\ 
  17 & MME.b & sigma & beta=1.5 & sigma=1 & n=100 & 148910.23 \\ 
  18 & PWM & sigma & beta=1.5 & sigma=1 & n=100 & 0.44 \\ 
  19 & MLE & beta & beta=2 & sigma=1 & n=100 & 89.69 \\ 
  20 & MLE.b & beta & beta=2 & sigma=1 & n=100 & 89.43 \\ 
  21 & LME & beta & beta=2 & sigma=1 & n=100 & 3.31 \\ 
  22 & MDE.Phi.chisq & beta & beta=2 & sigma=1 & n=100 & 79.26 \\ 
  23 & MDE.Phi.tv & beta & beta=2 & sigma=1 & n=100 & 107.06 \\ 
  24 & MDE.Phi.kl & beta & beta=2 & sigma=1 & n=100 & 14.38 \\ 
  25 & MME & beta & beta=2 & sigma=1 & n=100 & 55.69 \\ 
  26 & MME.b & beta & beta=2 & sigma=1 & n=100 & 151259.47 \\ 
  27 & PWM & beta & beta=2 & sigma=1 & n=100 & 3.31 \\ 
  28 & MLE & sigma & beta=2 & sigma=1 & n=100 & 31.47 \\ 
  29 & MLE.b & sigma & beta=2 & sigma=1 & n=100 & 31.33 \\ 
  30 & LME & sigma & beta=2 & sigma=1 & n=100 & 1.54 \\ 
  31 & MDE.Phi.chisq & sigma & beta=2 & sigma=1 & n=100 & 91.74 \\ 
  32 & MDE.Phi.tv & sigma & beta=2 & sigma=1 & n=100 & 118.22 \\ 
  33 & MDE.Phi.kl & sigma & beta=2 & sigma=1 & n=100 & 6.02 \\ 
  34 & MME & sigma & beta=2 & sigma=1 & n=100 & 24.92 \\ 
  35 & MME.b & sigma & beta=2 & sigma=1 & n=100 & 83571.71 \\ 
  36 & PWM & sigma & beta=2 & sigma=1 & n=100 & 1.54 \\ 
  37 & MLE & beta & beta=2.5 & sigma=1 & n=100 & 186.88 \\ 
  38 & MLE.b & beta & beta=2.5 & sigma=1 & n=100 & 186.76 \\ 
  39 & LME & beta & beta=2.5 & sigma=1 & n=100 & 8.83 \\ 
  40 & MDE.Phi.chisq & beta & beta=2.5 & sigma=1 & n=100 & 282.04 \\ 
  41 & MDE.Phi.tv & beta & beta=2.5 & sigma=1 & n=100 & 323.24 \\ 
  42 & MDE.Phi.kl & beta & beta=2.5 & sigma=1 & n=100 & 34.93 \\ 
  43 & MME & beta & beta=2.5 & sigma=1 & n=100 & 149.68 \\ 
  44 & MME.b & beta & beta=2.5 & sigma=1 & n=100 & 2235.69 \\ 
  45 & PWM & beta & beta=2.5 & sigma=1 & n=100 & 8.83 \\ 
  46 & MLE & sigma & beta=2.5 & sigma=1 & n=100 & 53.99 \\ 
  47 & MLE.b & sigma & beta=2.5 & sigma=1 & n=100 & 53.95 \\ 
  48 & LME & sigma & beta=2.5 & sigma=1 & n=100 & 2.38 \\ 
  49 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=1 & n=100 & 171.83 \\ 
  50 & MDE.Phi.tv & sigma & beta=2.5 & sigma=1 & n=100 & 195.89 \\ 
  51 & MDE.Phi.kl & sigma & beta=2.5 & sigma=1 & n=100 & 9.57 \\ 
  52 & MME & sigma & beta=2.5 & sigma=1 & n=100 & 39.37 \\ 
  53 & MME.b & sigma & beta=2.5 & sigma=1 & n=100 & 639.14 \\ 
  54 & PWM & sigma & beta=2.5 & sigma=1 & n=100 & 2.38 \\ 
  55 & MLE & beta & beta=3 & sigma=1 & n=100 & 1106.59 \\ 
  56 & MLE.b & beta & beta=3 & sigma=1 & n=100 & 1106.80 \\ 
  57 & LME & beta & beta=3 & sigma=1 & n=100 & 17.02 \\ 
  58 & MDE.Phi.chisq & beta & beta=3 & sigma=1 & n=100 & 624.43 \\ 
  59 & MDE.Phi.tv & beta & beta=3 & sigma=1 & n=100 & 754.62 \\ 
  60 & MDE.Phi.kl & beta & beta=3 & sigma=1 & n=100 & 123.94 \\ 
  61 & MME & beta & beta=3 & sigma=1 & n=100 & 313324.91 \\ 
  62 & MME.b & beta & beta=3 & sigma=1 & n=100 & 2979286.01 \\ 
  63 & PWM & beta & beta=3 & sigma=1 & n=100 & 17.02 \\ 
  64 & MLE & sigma & beta=3 & sigma=1 & n=100 & 219.06 \\ 
  65 & MLE.b & sigma & beta=3 & sigma=1 & n=100 & 219.09 \\ 
  66 & LME & sigma & beta=3 & sigma=1 & n=100 & 3.26 \\ 
  67 & MDE.Phi.chisq & sigma & beta=3 & sigma=1 & n=100 & 249.86 \\ 
  68 & MDE.Phi.tv & sigma & beta=3 & sigma=1 & n=100 & 294.63 \\ 
  69 & MDE.Phi.kl & sigma & beta=3 & sigma=1 & n=100 & 22.95 \\ 
  70 & MME & sigma & beta=3 & sigma=1 & n=100 & 45240.03 \\ 
  71 & MME.b & sigma & beta=3 & sigma=1 & n=100 & 430648.00 \\ 
  72 & PWM & sigma & beta=3 & sigma=1 & n=100 & 3.26 \\ 
  73 & MLE & beta & beta=4 & sigma=1 & n=100 & 1761.16 \\ 
  74 & MLE.b & beta & beta=4 & sigma=1 & n=100 & 1762.09 \\ 
  75 & LME & beta & beta=4 & sigma=1 & n=100 & 51.86 \\ 
  76 & MDE.Phi.chisq & beta & beta=4 & sigma=1 & n=100 & 1637.05 \\ 
  77 & MDE.Phi.tv & beta & beta=4 & sigma=1 & n=100 & 1917.41 \\ 
  78 & MDE.Phi.kl & beta & beta=4 & sigma=1 & n=100 & 244.56 \\ 
  79 & MME & beta & beta=4 & sigma=1 & n=100 & 11609.86 \\ 
  80 & MME.b & beta & beta=4 & sigma=1 & n=100 & 1922332.72 \\ 
  81 & PWM & beta & beta=4 & sigma=1 & n=100 & 51.86 \\ 
  82 & MLE & sigma & beta=4 & sigma=1 & n=100 & 167.33 \\ 
  83 & MLE.b & sigma & beta=4 & sigma=1 & n=100 & 167.41 \\ 
  84 & LME & sigma & beta=4 & sigma=1 & n=100 & 4.98 \\ 
  85 & MDE.Phi.chisq & sigma & beta=4 & sigma=1 & n=100 & 323.46 \\ 
  86 & MDE.Phi.tv & sigma & beta=4 & sigma=1 & n=100 & 358.68 \\ 
  87 & MDE.Phi.kl & sigma & beta=4 & sigma=1 & n=100 & 24.27 \\ 
  88 & MME & sigma & beta=4 & sigma=1 & n=100 & 1091.88 \\ 
  89 & MME.b & sigma & beta=4 & sigma=1 & n=100 & 270680.58 \\ 
  90 & PWM & sigma & beta=4 & sigma=1 & n=100 & 4.98 \\ 
  91 & MLE & beta & beta=5 & sigma=1 & n=100 & 2989.57 \\ 
  92 & MLE.b & beta & beta=5 & sigma=1 & n=100 & 2991.00 \\ 
  93 & LME & beta & beta=5 & sigma=1 & n=100 & 110.73 \\ 
  94 & MDE.Phi.chisq & beta & beta=5 & sigma=1 & n=100 & 2692.52 \\ 
  95 & MDE.Phi.tv & beta & beta=5 & sigma=1 & n=100 & 2969.26 \\ 
  96 & MDE.Phi.kl & beta & beta=5 & sigma=1 & n=100 & 438.04 \\ 
  97 & MME & beta & beta=5 & sigma=1 & n=100 & 18732.28 \\ 
  98 & MME.b & beta & beta=5 & sigma=1 & n=100 & 259627.66 \\ 
  99 & PWM & beta & beta=5 & sigma=1 & n=100 & 110.73 \\ 
  100 & MLE & sigma & beta=5 & sigma=1 & n=100 & 168.43 \\ 
  101 & MLE.b & sigma & beta=5 & sigma=1 & n=100 & 168.50 \\ 
  102 & LME & sigma & beta=5 & sigma=1 & n=100 & 6.10 \\ 
  103 & MDE.Phi.chisq & sigma & beta=5 & sigma=1 & n=100 & 307.30 \\ 
  104 & MDE.Phi.tv & sigma & beta=5 & sigma=1 & n=100 & 323.73 \\ 
  105 & MDE.Phi.kl & sigma & beta=5 & sigma=1 & n=100 & 24.13 \\ 
  106 & MME & sigma & beta=5 & sigma=1 & n=100 & 1044.65 \\ 
  107 & MME.b & sigma & beta=5 & sigma=1 & n=100 & 15546.03 \\ 
  108 & PWM & sigma & beta=5 & sigma=1 & n=100 & 6.10 \\ 
  109 & MLE & beta & beta=1.5 & sigma=1 & n=200 & 0.16 \\ 
  110 & MLE.b & beta & beta=1.5 & sigma=1 & n=200 & 0.09 \\ 
  111 & LME & beta & beta=1.5 & sigma=1 & n=200 & 0.15 \\ 
  112 & MDE.Phi.chisq & beta & beta=1.5 & sigma=1 & n=200 & 0.55 \\ 
  113 & MDE.Phi.tv & beta & beta=1.5 & sigma=1 & n=200 & 0.41 \\ 
  114 & MDE.Phi.kl & beta & beta=1.5 & sigma=1 & n=200 & 0.11 \\ 
  115 & MME & beta & beta=1.5 & sigma=1 & n=200 & 1.15 \\ 
  116 & MME.b & beta & beta=1.5 & sigma=1 & n=200 & 0.89 \\ 
  117 & PWM & beta & beta=1.5 & sigma=1 & n=200 & 0.15 \\ 
  118 & MLE & sigma & beta=1.5 & sigma=1 & n=200 & 0.17 \\ 
  119 & MLE.b & sigma & beta=1.5 & sigma=1 & n=200 & 0.10 \\ 
  120 & LME & sigma & beta=1.5 & sigma=1 & n=200 & 0.17 \\ 
  121 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=1 & n=200 & 0.24 \\ 
  122 & MDE.Phi.tv & sigma & beta=1.5 & sigma=1 & n=200 & 0.36 \\ 
  123 & MDE.Phi.kl & sigma & beta=1.5 & sigma=1 & n=200 & 0.12 \\ 
  124 & MME & sigma & beta=1.5 & sigma=1 & n=200 & 4.98 \\ 
  125 & MME.b & sigma & beta=1.5 & sigma=1 & n=200 & 4.16 \\ 
  126 & PWM & sigma & beta=1.5 & sigma=1 & n=200 & 0.17 \\ 
  127 & MLE & beta & beta=2 & sigma=1 & n=200 & 0.37 \\ 
  128 & MLE.b & beta & beta=2 & sigma=1 & n=200 & 0.20 \\ 
  129 & LME & beta & beta=2 & sigma=1 & n=200 & 0.35 \\ 
  130 & MDE.Phi.chisq & beta & beta=2 & sigma=1 & n=200 & 3.03 \\ 
  131 & MDE.Phi.tv & beta & beta=2 & sigma=1 & n=200 & 2.78 \\ 
  132 & MDE.Phi.kl & beta & beta=2 & sigma=1 & n=200 & 0.32 \\ 
  133 & MME & beta & beta=2 & sigma=1 & n=200 & 1.48 \\ 
  134 & MME.b & beta & beta=2 & sigma=1 & n=200 & 5.87 \\ 
  135 & PWM & beta & beta=2 & sigma=1 & n=200 & 0.35 \\ 
  136 & MLE & sigma & beta=2 & sigma=1 & n=200 & 0.18 \\ 
  137 & MLE.b & sigma & beta=2 & sigma=1 & n=200 & 0.10 \\ 
  138 & LME & sigma & beta=2 & sigma=1 & n=200 & 0.17 \\ 
  139 & MDE.Phi.chisq & sigma & beta=2 & sigma=1 & n=200 & 2.15 \\ 
  140 & MDE.Phi.tv & sigma & beta=2 & sigma=1 & n=200 & 2.80 \\ 
  141 & MDE.Phi.kl & sigma & beta=2 & sigma=1 & n=200 & 0.16 \\ 
  142 & MME & sigma & beta=2 & sigma=1 & n=200 & 1.07 \\ 
  143 & MME.b & sigma & beta=2 & sigma=1 & n=200 & 2.97 \\ 
  144 & PWM & sigma & beta=2 & sigma=1 & n=200 & 0.17 \\ 
  145 & MLE & beta & beta=2.5 & sigma=1 & n=200 & 1.52 \\ 
  146 & MLE.b & beta & beta=2.5 & sigma=1 & n=200 & 1.13 \\ 
  147 & LME & beta & beta=2.5 & sigma=1 & n=200 & 1.28 \\ 
  148 & MDE.Phi.chisq & beta & beta=2.5 & sigma=1 & n=200 & 22.25 \\ 
  149 & MDE.Phi.tv & beta & beta=2.5 & sigma=1 & n=200 & 16.67 \\ 
  150 & MDE.Phi.kl & beta & beta=2.5 & sigma=1 & n=200 & 1.18 \\ 
  151 & MME & beta & beta=2.5 & sigma=1 & n=200 & 2.90 \\ 
  152 & MME.b & beta & beta=2.5 & sigma=1 & n=200 & 44.44 \\ 
  153 & PWM & beta & beta=2.5 & sigma=1 & n=200 & 1.28 \\ 
  154 & MLE & sigma & beta=2.5 & sigma=1 & n=200 & 0.45 \\ 
  155 & MLE.b & sigma & beta=2.5 & sigma=1 & n=200 & 0.33 \\ 
  156 & LME & sigma & beta=2.5 & sigma=1 & n=200 & 0.36 \\ 
  157 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=1 & n=200 & 11.26 \\ 
  158 & MDE.Phi.tv & sigma & beta=2.5 & sigma=1 & n=200 & 8.16 \\ 
  159 & MDE.Phi.kl & sigma & beta=2.5 & sigma=1 & n=200 & 0.35 \\ 
  160 & MME & sigma & beta=2.5 & sigma=1 & n=200 & 0.96 \\ 
  161 & MME.b & sigma & beta=2.5 & sigma=1 & n=200 & 12.57 \\ 
  162 & PWM & sigma & beta=2.5 & sigma=1 & n=200 & 0.36 \\ 
  163 & MLE & beta & beta=3 & sigma=1 & n=200 & 176.07 \\ 
  164 & MLE.b & beta & beta=3 & sigma=1 & n=200 & 175.46 \\ 
  165 & LME & beta & beta=3 & sigma=1 & n=200 & 4.35 \\ 
  166 & MDE.Phi.chisq & beta & beta=3 & sigma=1 & n=200 & 111.20 \\ 
  167 & MDE.Phi.tv & beta & beta=3 & sigma=1 & n=200 & 52.14 \\ 
  168 & MDE.Phi.kl & beta & beta=3 & sigma=1 & n=200 & 8.59 \\ 
  169 & MME & beta & beta=3 & sigma=1 & n=200 & 74.99 \\ 
  170 & MME.b & beta & beta=3 & sigma=1 & n=200 & 7353.37 \\ 
  171 & PWM & beta & beta=3 & sigma=1 & n=200 & 4.35 \\ 
  172 & MLE & sigma & beta=3 & sigma=1 & n=200 & 29.25 \\ 
  173 & MLE.b & sigma & beta=3 & sigma=1 & n=200 & 29.13 \\ 
  174 & LME & sigma & beta=3 & sigma=1 & n=200 & 0.78 \\ 
  175 & MDE.Phi.chisq & sigma & beta=3 & sigma=1 & n=200 & 37.21 \\ 
  176 & MDE.Phi.tv & sigma & beta=3 & sigma=1 & n=200 & 16.26 \\ 
  177 & MDE.Phi.kl & sigma & beta=3 & sigma=1 & n=200 & 1.52 \\ 
  178 & MME & sigma & beta=3 & sigma=1 & n=200 & 12.28 \\ 
  179 & MME.b & sigma & beta=3 & sigma=1 & n=200 & 1682.84 \\ 
  180 & PWM & sigma & beta=3 & sigma=1 & n=200 & 0.78 \\ 
  181 & MLE & beta & beta=4 & sigma=1 & n=200 & 174.01 \\ 
  182 & MLE.b & beta & beta=4 & sigma=1 & n=200 & 173.79 \\ 
  183 & LME & beta & beta=4 & sigma=1 & n=200 & 18.28 \\ 
  184 & MDE.Phi.chisq & beta & beta=4 & sigma=1 & n=200 & 603.85 \\ 
  185 & MDE.Phi.tv & beta & beta=4 & sigma=1 & n=200 & 439.21 \\ 
  186 & MDE.Phi.kl & beta & beta=4 & sigma=1 & n=200 & 47.87 \\ 
  187 & MME & beta & beta=4 & sigma=1 & n=200 & 550.99 \\ 
  188 & MME.b & beta & beta=4 & sigma=1 & n=200 & 40296.90 \\ 
  189 & PWM & beta & beta=4 & sigma=1 & n=200 & 18.28 \\ 
  190 & MLE & sigma & beta=4 & sigma=1 & n=200 & 17.23 \\ 
  191 & MLE.b & sigma & beta=4 & sigma=1 & n=200 & 17.21 \\ 
  192 & LME & sigma & beta=4 & sigma=1 & n=200 & 1.71 \\ 
  193 & MDE.Phi.chisq & sigma & beta=4 & sigma=1 & n=200 & 100.47 \\ 
  194 & MDE.Phi.tv & sigma & beta=4 & sigma=1 & n=200 & 70.84 \\ 
  195 & MDE.Phi.kl & sigma & beta=4 & sigma=1 & n=200 & 4.52 \\ 
  196 & MME & sigma & beta=4 & sigma=1 & n=200 & 53.42 \\ 
  197 & MME.b & sigma & beta=4 & sigma=1 & n=200 & 4952.00 \\ 
  198 & PWM & sigma & beta=4 & sigma=1 & n=200 & 1.71 \\ 
  199 & MLE & beta & beta=5 & sigma=1 & n=200 & 10603.38 \\ 
  200 & MLE.b & beta & beta=5 & sigma=1 & n=200 & 10604.22 \\ 
  201 & LME & beta & beta=5 & sigma=1 & n=200 & 71.77 \\ 
  202 & MDE.Phi.chisq & beta & beta=5 & sigma=1 & n=200 & 1551.11 \\ 
  203 & MDE.Phi.tv & beta & beta=5 & sigma=1 & n=200 & 1026.74 \\ 
  204 & MDE.Phi.kl & beta & beta=5 & sigma=1 & n=200 & 159.94 \\ 
  205 & MME & beta & beta=5 & sigma=1 & n=200 & 2746.16 \\ 
  206 & MME.b & beta & beta=5 & sigma=1 & n=200 & 30985.72 \\ 
  207 & PWM & beta & beta=5 & sigma=1 & n=200 & 71.77 \\ 
  208 & MLE & sigma & beta=5 & sigma=1 & n=200 & 613.27 \\ 
  209 & MLE.b & sigma & beta=5 & sigma=1 & n=200 & 613.31 \\ 
  210 & LME & sigma & beta=5 & sigma=1 & n=200 & 4.03 \\ 
  211 & MDE.Phi.chisq & sigma & beta=5 & sigma=1 & n=200 & 151.76 \\ 
  212 & MDE.Phi.tv & sigma & beta=5 & sigma=1 & n=200 & 95.05 \\ 
  213 & MDE.Phi.kl & sigma & beta=5 & sigma=1 & n=200 & 8.91 \\ 
  214 & MME & sigma & beta=5 & sigma=1 & n=200 & 149.32 \\ 
  215 & MME.b & sigma & beta=5 & sigma=1 & n=200 & 1752.71 \\ 
  216 & PWM & sigma & beta=5 & sigma=1 & n=200 & 4.03 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220202/Output.var.LaTeX.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Tue Feb 01 15:44:07 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=1 & n=100 & 0.44 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=1 & n=100 & 0.32 \\ 
  3 & LME & beta & beta=1.5 & sigma=1 & n=100 & 0.30 \\ 
  4 & MDE.Phi.chisq & beta & beta=1.5 & sigma=1 & n=100 & 12.66 \\ 
  5 & MDE.Phi.tv & beta & beta=1.5 & sigma=1 & n=100 & 8.07 \\ 
  6 & MDE.Phi.kl & beta & beta=1.5 & sigma=1 & n=100 & 0.44 \\ 
  7 & MME & beta & beta=1.5 & sigma=1 & n=100 & 0.90 \\ 
  8 & MME.b & beta & beta=1.5 & sigma=1 & n=100 & 130047.07 \\ 
  9 & PWM & beta & beta=1.5 & sigma=1 & n=100 & 0.30 \\ 
  10 & MLE & sigma & beta=1.5 & sigma=1 & n=100 & 0.49 \\ 
  11 & MLE.b & sigma & beta=1.5 & sigma=1 & n=100 & 0.36 \\ 
  12 & LME & sigma & beta=1.5 & sigma=1 & n=100 & 0.33 \\ 
  13 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=1 & n=100 & 22.10 \\ 
  14 & MDE.Phi.tv & sigma & beta=1.5 & sigma=1 & n=100 & 21.12 \\ 
  15 & MDE.Phi.kl & sigma & beta=1.5 & sigma=1 & n=100 & 0.49 \\ 
  16 & MME & sigma & beta=1.5 & sigma=1 & n=100 & 1.99 \\ 
  17 & MME.b & sigma & beta=1.5 & sigma=1 & n=100 & 148891.08 \\ 
  18 & PWM & sigma & beta=1.5 & sigma=1 & n=100 & 0.33 \\ 
  19 & MLE & beta & beta=2 & sigma=1 & n=100 & 89.38 \\ 
  20 & MLE.b & beta & beta=2 & sigma=1 & n=100 & 89.40 \\ 
  21 & LME & beta & beta=2 & sigma=1 & n=100 & 3.11 \\ 
  22 & MDE.Phi.chisq & beta & beta=2 & sigma=1 & n=100 & 79.25 \\ 
  23 & MDE.Phi.tv & beta & beta=2 & sigma=1 & n=100 & 106.49 \\ 
  24 & MDE.Phi.kl & beta & beta=2 & sigma=1 & n=100 & 14.17 \\ 
  25 & MME & beta & beta=2 & sigma=1 & n=100 & 52.88 \\ 
  26 & MME.b & beta & beta=2 & sigma=1 & n=100 & 151218.71 \\ 
  27 & PWM & beta & beta=2 & sigma=1 & n=100 & 3.11 \\ 
  28 & MLE & sigma & beta=2 & sigma=1 & n=100 & 31.32 \\ 
  29 & MLE.b & sigma & beta=2 & sigma=1 & n=100 & 31.31 \\ 
  30 & LME & sigma & beta=2 & sigma=1 & n=100 & 1.45 \\ 
  31 & MDE.Phi.chisq & sigma & beta=2 & sigma=1 & n=100 & 90.42 \\ 
  32 & MDE.Phi.tv & sigma & beta=2 & sigma=1 & n=100 & 115.40 \\ 
  33 & MDE.Phi.kl & sigma & beta=2 & sigma=1 & n=100 & 5.92 \\ 
  34 & MME & sigma & beta=2 & sigma=1 & n=100 & 22.85 \\ 
  35 & MME.b & sigma & beta=2 & sigma=1 & n=100 & 83548.85 \\ 
  36 & PWM & sigma & beta=2 & sigma=1 & n=100 & 1.45 \\ 
  37 & MLE & beta & beta=2.5 & sigma=1 & n=100 & 185.63 \\ 
  38 & MLE.b & beta & beta=2.5 & sigma=1 & n=100 & 186.33 \\ 
  39 & LME & beta & beta=2.5 & sigma=1 & n=100 & 8.34 \\ 
  40 & MDE.Phi.chisq & beta & beta=2.5 & sigma=1 & n=100 & 278.80 \\ 
  41 & MDE.Phi.tv & beta & beta=2.5 & sigma=1 & n=100 & 316.26 \\ 
  42 & MDE.Phi.kl & beta & beta=2.5 & sigma=1 & n=100 & 34.03 \\ 
  43 & MME & beta & beta=2.5 & sigma=1 & n=100 & 144.30 \\ 
  44 & MME.b & beta & beta=2.5 & sigma=1 & n=100 & 2205.73 \\ 
  45 & PWM & beta & beta=2.5 & sigma=1 & n=100 & 8.34 \\ 
  46 & MLE & sigma & beta=2.5 & sigma=1 & n=100 & 53.63 \\ 
  47 & MLE.b & sigma & beta=2.5 & sigma=1 & n=100 & 53.82 \\ 
  48 & LME & sigma & beta=2.5 & sigma=1 & n=100 & 2.25 \\ 
  49 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=1 & n=100 & 166.88 \\ 
  50 & MDE.Phi.tv & sigma & beta=2.5 & sigma=1 & n=100 & 188.25 \\ 
  51 & MDE.Phi.kl & sigma & beta=2.5 & sigma=1 & n=100 & 9.31 \\ 
  52 & MME & sigma & beta=2.5 & sigma=1 & n=100 & 37.54 \\ 
  53 & MME.b & sigma & beta=2.5 & sigma=1 & n=100 & 630.07 \\ 
  54 & PWM & sigma & beta=2.5 & sigma=1 & n=100 & 2.25 \\ 
  55 & MLE & beta & beta=3 & sigma=1 & n=100 & 1098.32 \\ 
  56 & MLE.b & beta & beta=3 & sigma=1 & n=100 & 1101.15 \\ 
  57 & LME & beta & beta=3 & sigma=1 & n=100 & 15.99 \\ 
  58 & MDE.Phi.chisq & beta & beta=3 & sigma=1 & n=100 & 606.18 \\ 
  59 & MDE.Phi.tv & beta & beta=3 & sigma=1 & n=100 & 721.51 \\ 
  60 & MDE.Phi.kl & beta & beta=3 & sigma=1 & n=100 & 120.25 \\ 
  61 & MME & beta & beta=3 & sigma=1 & n=100 & 313146.34 \\ 
  62 & MME.b & beta & beta=3 & sigma=1 & n=100 & 2977375.72 \\ 
  63 & PWM & beta & beta=3 & sigma=1 & n=100 & 15.99 \\ 
  64 & MLE & sigma & beta=3 & sigma=1 & n=100 & 217.52 \\ 
  65 & MLE.b & sigma & beta=3 & sigma=1 & n=100 & 218.03 \\ 
  66 & LME & sigma & beta=3 & sigma=1 & n=100 & 3.08 \\ 
  67 & MDE.Phi.chisq & sigma & beta=3 & sigma=1 & n=100 & 238.26 \\ 
  68 & MDE.Phi.tv & sigma & beta=3 & sigma=1 & n=100 & 277.24 \\ 
  69 & MDE.Phi.kl & sigma & beta=3 & sigma=1 & n=100 & 22.26 \\ 
  70 & MME & sigma & beta=3 & sigma=1 & n=100 & 45211.58 \\ 
  71 & MME.b & sigma & beta=3 & sigma=1 & n=100 & 430346.24 \\ 
  72 & PWM & sigma & beta=3 & sigma=1 & n=100 & 3.08 \\ 
  73 & MLE & beta & beta=4 & sigma=1 & n=100 & 1737.84 \\ 
  74 & MLE.b & beta & beta=4 & sigma=1 & n=100 & 1742.92 \\ 
  75 & LME & beta & beta=4 & sigma=1 & n=100 & 48.77 \\ 
  76 & MDE.Phi.chisq & beta & beta=4 & sigma=1 & n=100 & 1518.05 \\ 
  77 & MDE.Phi.tv & beta & beta=4 & sigma=1 & n=100 & 1741.16 \\ 
  78 & MDE.Phi.kl & beta & beta=4 & sigma=1 & n=100 & 232.17 \\ 
  79 & MME & beta & beta=4 & sigma=1 & n=100 & 11556.91 \\ 
  80 & MME.b & beta & beta=4 & sigma=1 & n=100 & 1921162.31 \\ 
  81 & PWM & beta & beta=4 & sigma=1 & n=100 & 48.77 \\ 
  82 & MLE & sigma & beta=4 & sigma=1 & n=100 & 165.09 \\ 
  83 & MLE.b & sigma & beta=4 & sigma=1 & n=100 & 165.56 \\ 
  84 & LME & sigma & beta=4 & sigma=1 & n=100 & 4.69 \\ 
  85 & MDE.Phi.chisq & sigma & beta=4 & sigma=1 & n=100 & 294.11 \\ 
  86 & MDE.Phi.tv & sigma & beta=4 & sigma=1 & n=100 & 320.32 \\ 
  87 & MDE.Phi.kl & sigma & beta=4 & sigma=1 & n=100 & 23.07 \\ 
  88 & MME & sigma & beta=4 & sigma=1 & n=100 & 1086.55 \\ 
  89 & MME.b & sigma & beta=4 & sigma=1 & n=100 & 270553.04 \\ 
  90 & PWM & sigma & beta=4 & sigma=1 & n=100 & 4.69 \\ 
  91 & MLE & beta & beta=5 & sigma=1 & n=100 & 2933.89 \\ 
  92 & MLE.b & beta & beta=5 & sigma=1 & n=100 & 2940.69 \\ 
  93 & LME & beta & beta=5 & sigma=1 & n=100 & 104.92 \\ 
  94 & MDE.Phi.chisq & beta & beta=5 & sigma=1 & n=100 & 2403.78 \\ 
  95 & MDE.Phi.tv & beta & beta=5 & sigma=1 & n=100 & 2594.76 \\ 
  96 & MDE.Phi.kl & beta & beta=5 & sigma=1 & n=100 & 410.29 \\ 
  97 & MME & beta & beta=5 & sigma=1 & n=100 & 18595.78 \\ 
  98 & MME.b & beta & beta=5 & sigma=1 & n=100 & 257869.79 \\ 
  99 & PWM & beta & beta=5 & sigma=1 & n=100 & 104.92 \\ 
  100 & MLE & sigma & beta=5 & sigma=1 & n=100 & 165.34 \\ 
  101 & MLE.b & sigma & beta=5 & sigma=1 & n=100 & 165.71 \\ 
  102 & LME & sigma & beta=5 & sigma=1 & n=100 & 5.78 \\ 
  103 & MDE.Phi.chisq & sigma & beta=5 & sigma=1 & n=100 & 268.55 \\ 
  104 & MDE.Phi.tv & sigma & beta=5 & sigma=1 & n=100 & 277.98 \\ 
  105 & MDE.Phi.kl & sigma & beta=5 & sigma=1 & n=100 & 22.59 \\ 
  106 & MME & sigma & beta=5 & sigma=1 & n=100 & 1037.16 \\ 
  107 & MME.b & sigma & beta=5 & sigma=1 & n=100 & 15447.94 \\ 
  108 & PWM & sigma & beta=5 & sigma=1 & n=100 & 5.78 \\ 
  109 & MLE & beta & beta=1.5 & sigma=1 & n=200 & 0.10 \\ 
  110 & MLE.b & beta & beta=1.5 & sigma=1 & n=200 & 0.08 \\ 
  111 & LME & beta & beta=1.5 & sigma=1 & n=200 & 0.11 \\ 
  112 & MDE.Phi.chisq & beta & beta=1.5 & sigma=1 & n=200 & 0.12 \\ 
  113 & MDE.Phi.tv & beta & beta=1.5 & sigma=1 & n=200 & 0.17 \\ 
  114 & MDE.Phi.kl & beta & beta=1.5 & sigma=1 & n=200 & 0.10 \\ 
  115 & MME & beta & beta=1.5 & sigma=1 & n=200 & 0.16 \\ 
  116 & MME.b & beta & beta=1.5 & sigma=1 & n=200 & 0.26 \\ 
  117 & PWM & beta & beta=1.5 & sigma=1 & n=200 & 0.11 \\ 
  118 & MLE & sigma & beta=1.5 & sigma=1 & n=200 & 0.11 \\ 
  119 & MLE.b & sigma & beta=1.5 & sigma=1 & n=200 & 0.08 \\ 
  120 & LME & sigma & beta=1.5 & sigma=1 & n=200 & 0.12 \\ 
  121 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=1 & n=200 & 0.22 \\ 
  122 & MDE.Phi.tv & sigma & beta=1.5 & sigma=1 & n=200 & 0.29 \\ 
  123 & MDE.Phi.kl & sigma & beta=1.5 & sigma=1 & n=200 & 0.11 \\ 
  124 & MME & sigma & beta=1.5 & sigma=1 & n=200 & 1.78 \\ 
  125 & MME.b & sigma & beta=1.5 & sigma=1 & n=200 & 1.87 \\ 
  126 & PWM & sigma & beta=1.5 & sigma=1 & n=200 & 0.12 \\ 
  127 & MLE & beta & beta=2 & sigma=1 & n=200 & 0.31 \\ 
  128 & MLE.b & beta & beta=2 & sigma=1 & n=200 & 0.20 \\ 
  129 & LME & beta & beta=2 & sigma=1 & n=200 & 0.30 \\ 
  130 & MDE.Phi.chisq & beta & beta=2 & sigma=1 & n=200 & 2.61 \\ 
  131 & MDE.Phi.tv & beta & beta=2 & sigma=1 & n=200 & 2.60 \\ 
  132 & MDE.Phi.kl & beta & beta=2 & sigma=1 & n=200 & 0.30 \\ 
  133 & MME & beta & beta=2 & sigma=1 & n=200 & 0.53 \\ 
  134 & MME.b & beta & beta=2 & sigma=1 & n=200 & 5.40 \\ 
  135 & PWM & beta & beta=2 & sigma=1 & n=200 & 0.30 \\ 
  136 & MLE & sigma & beta=2 & sigma=1 & n=200 & 0.15 \\ 
  137 & MLE.b & sigma & beta=2 & sigma=1 & n=200 & 0.10 \\ 
  138 & LME & sigma & beta=2 & sigma=1 & n=200 & 0.15 \\ 
  139 & MDE.Phi.chisq & sigma & beta=2 & sigma=1 & n=200 & 2.12 \\ 
  140 & MDE.Phi.tv & sigma & beta=2 & sigma=1 & n=200 & 2.72 \\ 
  141 & MDE.Phi.kl & sigma & beta=2 & sigma=1 & n=200 & 0.15 \\ 
  142 & MME & sigma & beta=2 & sigma=1 & n=200 & 0.28 \\ 
  143 & MME.b & sigma & beta=2 & sigma=1 & n=200 & 2.55 \\ 
  144 & PWM & sigma & beta=2 & sigma=1 & n=200 & 0.15 \\ 
  145 & MLE & beta & beta=2.5 & sigma=1 & n=200 & 1.41 \\ 
  146 & MLE.b & beta & beta=2.5 & sigma=1 & n=200 & 1.13 \\ 
  147 & LME & beta & beta=2.5 & sigma=1 & n=200 & 1.20 \\ 
  148 & MDE.Phi.chisq & beta & beta=2.5 & sigma=1 & n=200 & 22.07 \\ 
  149 & MDE.Phi.tv & beta & beta=2.5 & sigma=1 & n=200 & 16.63 \\ 
  150 & MDE.Phi.kl & beta & beta=2.5 & sigma=1 & n=200 & 1.12 \\ 
  151 & MME & beta & beta=2.5 & sigma=1 & n=200 & 1.77 \\ 
  152 & MME.b & beta & beta=2.5 & sigma=1 & n=200 & 43.75 \\ 
  153 & PWM & beta & beta=2.5 & sigma=1 & n=200 & 1.20 \\ 
  154 & MLE & sigma & beta=2.5 & sigma=1 & n=200 & 0.41 \\ 
  155 & MLE.b & sigma & beta=2.5 & sigma=1 & n=200 & 0.33 \\ 
  156 & LME & sigma & beta=2.5 & sigma=1 & n=200 & 0.34 \\ 
  157 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=1 & n=200 & 11.13 \\ 
  158 & MDE.Phi.tv & sigma & beta=2.5 & sigma=1 & n=200 & 7.99 \\ 
  159 & MDE.Phi.kl & sigma & beta=2.5 & sigma=1 & n=200 & 0.33 \\ 
  160 & MME & sigma & beta=2.5 & sigma=1 & n=200 & 0.53 \\ 
  161 & MME.b & sigma & beta=2.5 & sigma=1 & n=200 & 12.32 \\ 
  162 & PWM & sigma & beta=2.5 & sigma=1 & n=200 & 0.34 \\ 
  163 & MLE & beta & beta=3 & sigma=1 & n=200 & 175.57 \\ 
  164 & MLE.b & beta & beta=3 & sigma=1 & n=200 & 175.42 \\ 
  165 & LME & beta & beta=3 & sigma=1 & n=200 & 4.14 \\ 
  166 & MDE.Phi.chisq & beta & beta=3 & sigma=1 & n=200 & 111.07 \\ 
  167 & MDE.Phi.tv & beta & beta=3 & sigma=1 & n=200 & 52.09 \\ 
  168 & MDE.Phi.kl & beta & beta=3 & sigma=1 & n=200 & 8.35 \\ 
  169 & MME & beta & beta=3 & sigma=1 & n=200 & 73.03 \\ 
  170 & MME.b & beta & beta=3 & sigma=1 & n=200 & 7346.85 \\ 
  171 & PWM & beta & beta=3 & sigma=1 & n=200 & 4.14 \\ 
  172 & MLE & sigma & beta=3 & sigma=1 & n=200 & 29.16 \\ 
  173 & MLE.b & sigma & beta=3 & sigma=1 & n=200 & 29.12 \\ 
  174 & LME & sigma & beta=3 & sigma=1 & n=200 & 0.74 \\ 
  175 & MDE.Phi.chisq & sigma & beta=3 & sigma=1 & n=200 & 36.55 \\ 
  176 & MDE.Phi.tv & sigma & beta=3 & sigma=1 & n=200 & 15.88 \\ 
  177 & MDE.Phi.kl & sigma & beta=3 & sigma=1 & n=200 & 1.47 \\ 
  178 & MME & sigma & beta=3 & sigma=1 & n=200 & 11.86 \\ 
  179 & MME.b & sigma & beta=3 & sigma=1 & n=200 & 1681.49 \\ 
  180 & PWM & sigma & beta=3 & sigma=1 & n=200 & 0.74 \\ 
  181 & MLE & beta & beta=4 & sigma=1 & n=200 & 171.51 \\ 
  182 & MLE.b & beta & beta=4 & sigma=1 & n=200 & 172.99 \\ 
  183 & LME & beta & beta=4 & sigma=1 & n=200 & 17.45 \\ 
  184 & MDE.Phi.chisq & beta & beta=4 & sigma=1 & n=200 & 586.96 \\ 
  185 & MDE.Phi.tv & beta & beta=4 & sigma=1 & n=200 & 428.97 \\ 
  186 & MDE.Phi.kl & beta & beta=4 & sigma=1 & n=200 & 46.26 \\ 
  187 & MME & beta & beta=4 & sigma=1 & n=200 & 544.09 \\ 
  188 & MME.b & beta & beta=4 & sigma=1 & n=200 & 40207.11 \\ 
  189 & PWM & beta & beta=4 & sigma=1 & n=200 & 17.45 \\ 
  190 & MLE & sigma & beta=4 & sigma=1 & n=200 & 16.99 \\ 
  191 & MLE.b & sigma & beta=4 & sigma=1 & n=200 & 17.13 \\ 
  192 & LME & sigma & beta=4 & sigma=1 & n=200 & 1.64 \\ 
  193 & MDE.Phi.chisq & sigma & beta=4 & sigma=1 & n=200 & 95.79 \\ 
  194 & MDE.Phi.tv & sigma & beta=4 & sigma=1 & n=200 & 68.07 \\ 
  195 & MDE.Phi.kl & sigma & beta=4 & sigma=1 & n=200 & 4.37 \\ 
  196 & MME & sigma & beta=4 & sigma=1 & n=200 & 52.73 \\ 
  197 & MME.b & sigma & beta=4 & sigma=1 & n=200 & 4942.71 \\ 
  198 & PWM & sigma & beta=4 & sigma=1 & n=200 & 1.64 \\ 
  199 & MLE & beta & beta=5 & sigma=1 & n=200 & 10579.89 \\ 
  200 & MLE.b & beta & beta=5 & sigma=1 & n=200 & 10587.27 \\ 
  201 & LME & beta & beta=5 & sigma=1 & n=200 & 68.49 \\ 
  202 & MDE.Phi.chisq & beta & beta=5 & sigma=1 & n=200 & 1448.48 \\ 
  203 & MDE.Phi.tv & beta & beta=5 & sigma=1 & n=200 & 977.14 \\ 
  204 & MDE.Phi.kl & beta & beta=5 & sigma=1 & n=200 & 152.90 \\ 
  205 & MME & beta & beta=5 & sigma=1 & n=200 & 2723.74 \\ 
  206 & MME.b & beta & beta=5 & sigma=1 & n=200 & 30713.32 \\ 
  207 & PWM & beta & beta=5 & sigma=1 & n=200 & 68.49 \\ 
  208 & MLE & sigma & beta=5 & sigma=1 & n=200 & 611.90 \\ 
  209 & MLE.b & sigma & beta=5 & sigma=1 & n=200 & 612.32 \\ 
  210 & LME & sigma & beta=5 & sigma=1 & n=200 & 3.85 \\ 
  211 & MDE.Phi.chisq & sigma & beta=5 & sigma=1 & n=200 & 138.94 \\ 
  212 & MDE.Phi.tv & sigma & beta=5 & sigma=1 & n=200 & 88.99 \\ 
  213 & MDE.Phi.kl & sigma & beta=5 & sigma=1 & n=200 & 8.52 \\ 
  214 & MME & sigma & beta=5 & sigma=1 & n=200 & 148.05 \\ 
  215 & MME.b & sigma & beta=5 & sigma=1 & n=200 & 1737.36 \\ 
  216 & PWM & sigma & beta=5 & sigma=1 & n=200 & 3.85 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220203/Full.beta=1.5.sig=2.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=1.5,  \sigma=2$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.6717&1.4777&1.8288&0.234&1.257&1.6717&2.7927&6.3149&1.8288
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2.3645&1.9548&2.6507&3.2891&3.6444&2.3645&6.3049&13.6686&2.6507
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.435&0.3213&0.2958&97.6125&6.7844&0.4354&0.8967&130047.0683&0.2958
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.9574&1.4455&1.33&82.0458&70.7652&1.9589&7.9695&595564.3219&1.33
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1717&-0.0223&0.3288&-1.266&-0.243&0.1717&1.2927&4.8149&0.3288
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.3645&-0.0452&0.6507&1.2891&1.6444&0.3645&4.3049&11.6686&0.6507
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.4644&0.3217&0.4039&99.2056&6.8428&0.4648&2.5678&130057.2467&0.4039
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2.0901&1.4474&1.7532&83.6994&73.4621&2.0916&26.5012&595640.9217&1.7532
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 2.5545&1.7692&2.1571&182.9049&80.3048&2.5564&29.069&725698.1684&2.1571\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0011&0.0011&1.63885457077832e+301&0.0364&0.0011&0.0099&7.105&0.0011\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220203/Full.beta=1.5.sig=2.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=1.5,  \sigma=2$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.7301&1.6295&1.7053&0.6454&1.004&1.578&2.4952&2.2961&1.7053
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2.4773&2.2636&2.4046&2.3164&2.507&2.1626&5.5704&5.0195&2.4046
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1033&0.0759&0.1117&22.8262&0.1705&0.1014&0.1645&0.2553&0.1117
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.456&0.3307&0.4944&3.3191&1.1627&0.4329&6.0718&6.4445&0.4944
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.2301&0.1295&0.2053&-0.8546&-0.496&0.078&0.9952&0.7961&0.2053
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.4773&0.2636&0.4046&0.3164&0.507&0.1626&3.5704&3.0195&0.4046
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1562&0.0927&0.1539&23.5542&0.4165&0.1075&1.1549&0.889&0.1539
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.6837&0.4001&0.6581&3.4189&1.4196&0.4593&18.8191&15.5612&0.6581
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 0.84&0.4928&0.8119&26.9731&1.8362&0.5667&19.974&16.4502&0.8119\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 6e-04&6e-04&6e-04&2.74643118624275e+299&0.0276&6e-04&0.0089&0.0103&6e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220203/Full.beta=2.5.sig=2.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2.5,  \sigma=2$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 3.5893&3.1321&3.1958&4.1065&4.9271&3.4377&4.8214&7.9937&3.1958
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
3.169&2.6735&2.7184&6.1414&7.1933&3.0067&4.7089&8.0431&2.7184
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 140.165&140.8267&8.3445&224.5742&256.6062&29.7786&144.3027&2205.727&8.3445
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
160.6925&161.4224&8.9937&535.712&611.3674&32.5838&150.1403&2520.2999&8.9937
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.0893&0.6321&0.6958&1.6065&2.4271&0.9377&2.3214&5.4937&0.6958
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.169&0.6735&0.7184&4.1414&5.1933&1.0067&2.7089&6.0431&0.7184
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 141.3376&141.2122&8.8279&227.1324&262.4715&30.6549&149.6771&2235.6866&8.8279
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
162.0429&161.8599&9.5089&552.8092&638.2771&33.5939&157.4634&2556.5675&9.5089
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 303.3806&303.0721&18.3368&779.9416&900.7486&64.2488&307.1405&4792.2541&18.3368\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0012&0.0011&0.0233&0.0179&0.0011&0.0019&8.078&0.0011\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220203/Full.beta=2.5.sig=2.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2.5,  \sigma=2$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.8441&2.5199&2.784&2.0498&2.2768&2.7518&3.5622&3.3354&2.784
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2.3708&2.0191&2.2893&2.7012&2.8083&2.2713&3.3094&3.0134&2.2893
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.4065&1.126&1.1971&17.8817&13.8093&1.1167&1.774&43.7476&1.1971
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.6567&1.3199&1.3628&36.102&26.6172&1.3262&2.1291&49.2611&1.3628
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.3441&0.0199&0.284&-0.4502&-0.2232&0.2518&1.0622&0.8354&0.284
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.3708&0.0191&0.2893&0.7012&0.8083&0.2713&1.3094&1.0134&0.2893
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.5248&1.1263&1.2776&18.0826&13.8577&1.18&2.9021&44.441&1.2776
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.794&1.3201&1.4463&36.59&27.2679&1.3996&3.8434&50.2833&1.4463
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 3.3188&2.4464&2.724&54.6726&41.1256&2.5796&6.7455&94.7243&2.724\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&5e-04&5e-04&0.0174&0.0121&5e-04&0.0011&0.0017&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220203/Full.beta=2.sig=2.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2,  \sigma=2$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.5397&2.1901&2.4461&2.0969&2.6942&2.458&3.6775&9.4751&2.4461
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2.7453&2.2401&2.6033&4.195&5.2184&2.6474&4.8746&13.1731&2.6033
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 66.0603&66.0628&3.1121&65.3915&87.2818&12.1947&52.8831&151218.7131&3.1121
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
93.6627&93.6023&5.78&298.7604&379.0939&20.4426&91.4156&334195.4082&5.78
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.5397&0.1901&0.4461&0.0969&0.6942&0.458&1.6775&7.4751&0.4461
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.7453&0.2401&0.6033&2.195&3.2184&0.6474&2.8746&11.1731&0.6033
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 66.345&66.0923&3.3109&65.3943&87.755&12.4033&55.6919&151259.4685&3.3109
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
94.2087&93.6506&6.1434&303.5485&389.4141&20.8597&99.6701&334286.8261&6.1434
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 160.5538&159.7429&9.4543&368.9428&477.169&33.263&155.3621&485546.2946&9.4543\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0011&0.0011&0.0296&0.0232&0.0011&0.0035&0.0115&0.0011\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220203/Full.beta=2.sig=2.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2,  \sigma=2$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.2514&2.0633&2.2157&1.3468&1.5634&2.1374&2.9722&2.6877&2.2157
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2.3527&2.0825&2.2838&2.3432&2.5561&2.1929&3.7771&3.293&2.2838
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.305&0.2007&0.3034&2.1912&2.2108&0.2964&0.5321&5.3987&0.3034
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.6069&0.3945&0.5992&7.138&9.1449&0.5879&1.1111&10.202&0.5992
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.2514&0.0633&0.2157&-0.6532&-0.4366&0.1374&0.9722&0.6877&0.2157
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.3527&0.0825&0.2838&0.3432&0.5561&0.1929&1.7771&1.293&0.2838
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.3682&0.2047&0.3499&2.6177&2.4012&0.3153&1.4772&5.8711&0.3499
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.7312&0.4013&0.6797&7.2551&9.4533&0.625&4.269&11.8728&0.6797
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 1.0994&0.606&1.0296&9.8728&11.8545&0.9403&5.7463&17.744&1.0296\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 6e-04&5e-04&5e-04&0.0227&0.0165&5e-04&0.0024&0.0024&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220203/Full.beta=3.sig=2.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=3,  \sigma=2$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 5.7496&5.2554&4.0159&6.8159&8.2326&4.8603&17.4875&49.9897&4.0159
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
4.3701&3.9431&2.851&8.2493&9.7002&3.6029&13.4836&39.1376&2.851
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 872.8497&875.5266&15.9909&480.8982&575.7729&100.8592&313146.3373&2977375.7167&15.9909
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
673.8379&675.7935&12.3334&759.0983&886.5153&75.1257&180846.3382&1721384.9561&12.3334
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.7496&2.2554&1.0159&3.8159&5.2326&1.8603&14.4875&46.9897&1.0159
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2.3701&1.9431&0.851&6.2493&7.7002&1.6029&11.4836&37.1376&0.851
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 880.3225&880.5257&17.0213&495.4112&603.0956&104.31&313324.9101&2979286.0078&17.0213
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
679.3878&679.5016&13.0565&798.0758&945.7205&77.6873&180960.127&1722592.0179&13.0565
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 1559.7103&1560.0274&30.0778&1293.487&1548.8161&181.9974&494285.0371&4701878.0258&30.0778\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0012&0.0011&0.0201&0.0151&0.0011&0.0014&0.0075&0.0011\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220203/Full.beta=3.sig=2.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=3,  \sigma=2$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 3.7154&3.2327&3.4535&3.3052&3.2069&3.4926&4.4031&5.6933&3.4535
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2.6184&2.1988&2.3785&3.5428&3.1929&2.4257&3.2925&4.4634&2.3785
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 175.5736&175.4235&4.1441&89.0057&42.6911&7.7328&73.0305&7346.8537&4.1441
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
116.6364&116.4993&2.9784&117.1409&52.0072&5.5021&47.4545&6725.9729&2.9784
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.7154&0.2327&0.4535&0.3052&0.2069&0.4926&1.4031&2.6933&0.4535
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.6184&0.1988&0.3785&1.5428&1.1929&0.4257&1.2925&2.4634&0.3785
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 176.0679&175.4601&4.3493&89.09&42.7296&7.9746&74.9918&7353.3729&4.3493
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
117.0072&116.5272&3.1213&119.5094&53.4249&5.6827&49.1203&6731.3689&3.1213
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 293.0751&291.9873&7.4706&208.5993&96.1546&13.6574&124.1121&14084.7417&7.4706\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&5e-04&5e-04&0.0143&0.0096&5e-04&7e-04&0.0018&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220203/Full.beta=4.sig=2.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=4,  \sigma=2$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 8.7295&8.2802&5.759&13.7651&15.9545&7.4212&11.3558&40.9124&5.759
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
4.927&4.6544&3.0703&11.8342&13.2625&4.1216&6.6655&26.8679&3.0703
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1525.3767&1530.3561&48.7724&1195.0428&1368.6343&201.2946&11556.9085&1921162.3133&48.7724
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
574.9177&576.7649&18.7607&926.7579&1007.8946&79.6118&4346.1835&1082212.1431&18.7607
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 4.7295&4.2802&1.759&9.7651&11.9545&3.4212&7.3558&36.9124&1.759
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2.927&2.6544&1.0703&9.8342&11.2625&2.1216&4.6655&24.8679&1.0703
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1547.5927&1548.5231&51.8617&1290.2814&1511.4083&212.9789&11609.8605&1922332.7188&51.8617
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
583.4273&583.7532&19.9043&1023.3773&1134.6382&84.1049&4367.5156&1082722.332&19.9043
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 2131.0201&2132.2764&71.766&2313.6587&2646.0465&297.0838&15977.3761&3005055.0508&71.766\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0012&0.001&0.0165&0.0123&0.0011&0.0011&4041.9544&0.001\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220203/Full.beta=4.sig=2.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=4,  \sigma=2$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 5.559&4.8756&4.9145&7.7069&6.9491&5.2566&6.6372&13.6851&4.9145
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2.9826&2.5623&2.5529&6.0025&5.1303&2.7745&3.6618&8.2547&2.5529
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 158.8545&160.3016&17.4492&465.0781&346.1052&41.244&544.0894&40207.1182&17.4492
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
62.644&63.1884&6.5508&303.5793&220.0039&15.5934&210.9218&19770.8596&6.5508
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.559&0.8756&0.9145&3.7069&2.9491&1.2566&2.6372&9.6851&0.9145
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.9826&0.5623&0.5529&4.0025&3.1303&0.7745&1.6618&6.2547&0.5529
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 161.2692&161.0524&18.2837&478.7729&354.7677&42.8191&550.9901&40296.899&18.2837
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
63.6032&63.4983&6.8558&319.5687&229.7807&16.1917&213.6621&19808.0043&6.8558
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 224.8724&224.5506&25.1395&798.3416&584.5484&59.0108&764.6522&60104.9033&25.1395\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&6e-04&5e-04&0.0111&0.0074&5e-04&6e-04&0.0029&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220203/Full.beta=5.sig=2.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=5,  \sigma=2$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 12.3236&11.9551&7.3605&20.093&22.2436&10.0638&16.7262&47.1595&7.3605
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
5.4476&5.2764&3.101&13.1832&14.1594&4.3827&7.4959&21.9309&3.101
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2693.779&2700.4687&96.0976&1864.5133&2004.2157&347.2915&18587.8467&257840.1544&96.0976
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
605.4031&606.8577&21.2623&832.8022&860.1424&76.9632&4147.1761&61786.3409&21.2623
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 7.3236&6.9551&2.3605&15.093&17.2436&5.0638&11.7262&42.1595&2.3605
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
3.4476&3.2764&1.101&11.1832&12.1594&2.3827&5.4959&19.9309&1.101
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2747.1447&2748.5723&101.6601&2092.1268&2301.358&372.8992&18723.4925&259591.7905&101.6601
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
617.2287&617.5317&22.4723&957.7827&1007.9069&82.6327&4176.9667&62177.4021&22.4723
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 3364.3733&3366.1039&124.1323&3049.9096&3309.2649&455.5319&22900.4592&321769.1926&124.1323\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.001&0.0012&0.001&0.0144&0.0106&0.001&0.001&5.15620838018139e+29&0.001\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220203/Full.beta=5.sig=2.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=5,  \sigma=2$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 9.9205&9.2093&6.7803&14.1274&11.358&7.6&9.7618&21.5876&6.7803
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
4.3773&4.0403&2.8327&8.5388&6.5108&3.2262&4.2663&9.8745&2.8327
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 10574.3435&10581.6739&63.0773&1137.0862&766.5447&134.8763&2723.7306&30712.8683&63.0773
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2446.3119&2447.9693&14.1243&435.7651&279.1057&30.091&592.1845&6949.345&14.1243
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 4.9205&4.2093&1.7803&9.1274&6.358&2.6&4.7618&16.5876&1.7803
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2.3773&2.0403&0.8327&6.5388&4.5108&1.2262&2.2663&7.8745&0.8327
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 10597.4977&10598.3343&66.2407&1220.2826&806.8926&141.6228&2746.133&30984.9451&66.2407
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2451.7189&2451.8872&14.8163&478.4768&299.425&31.5915&597.2612&7010.6574&14.8163
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 13049.2166&13050.2215&81.057&1698.7594&1106.3177&173.2143&3343.3942&37995.6025&81.057\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&6e-04&5e-04&0.0096&0.0062&5e-04&5e-04&2.018&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220203/Output.accuracy.LaTeX.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Tue Feb 01 15:49:34 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & Measure & beta=1.5 & sigma=2 & n=100 & 2.55 \\ 
  2 & MLE.b & Measure & beta=1.5 & sigma=2 & n=100 & 1.77 \\ 
  3 & LME & Measure & beta=1.5 & sigma=2 & n=100 & 2.16 \\ 
  4 & MDE.Phi.chisq & Measure & beta=1.5 & sigma=2 & n=100 & 182.90 \\ 
  5 & MDE.Phi.tv & Measure & beta=1.5 & sigma=2 & n=100 & 80.30 \\ 
  6 & MDE.Phi.kl & Measure & beta=1.5 & sigma=2 & n=100 & 2.56 \\ 
  7 & MME & Measure & beta=1.5 & sigma=2 & n=100 & 29.07 \\ 
  8 & MME.b & Measure & beta=1.5 & sigma=2 & n=100 & 725698.17 \\ 
  9 & PWM & Measure & beta=1.5 & sigma=2 & n=100 & 2.16 \\ 
  10 & MLE & Measure & beta=2 & sigma=2 & n=100 & 160.55 \\ 
  11 & MLE.b & Measure & beta=2 & sigma=2 & n=100 & 159.74 \\ 
  12 & LME & Measure & beta=2 & sigma=2 & n=100 & 9.45 \\ 
  13 & MDE.Phi.chisq & Measure & beta=2 & sigma=2 & n=100 & 368.94 \\ 
  14 & MDE.Phi.tv & Measure & beta=2 & sigma=2 & n=100 & 477.17 \\ 
  15 & MDE.Phi.kl & Measure & beta=2 & sigma=2 & n=100 & 33.26 \\ 
  16 & MME & Measure & beta=2 & sigma=2 & n=100 & 155.36 \\ 
  17 & MME.b & Measure & beta=2 & sigma=2 & n=100 & 485546.29 \\ 
  18 & PWM & Measure & beta=2 & sigma=2 & n=100 & 9.45 \\ 
  19 & MLE & Measure & beta=2.5 & sigma=2 & n=100 & 303.38 \\ 
  20 & MLE.b & Measure & beta=2.5 & sigma=2 & n=100 & 303.07 \\ 
  21 & LME & Measure & beta=2.5 & sigma=2 & n=100 & 18.34 \\ 
  22 & MDE.Phi.chisq & Measure & beta=2.5 & sigma=2 & n=100 & 779.94 \\ 
  23 & MDE.Phi.tv & Measure & beta=2.5 & sigma=2 & n=100 & 900.75 \\ 
  24 & MDE.Phi.kl & Measure & beta=2.5 & sigma=2 & n=100 & 64.25 \\ 
  25 & MME & Measure & beta=2.5 & sigma=2 & n=100 & 307.14 \\ 
  26 & MME.b & Measure & beta=2.5 & sigma=2 & n=100 & 4792.25 \\ 
  27 & PWM & Measure & beta=2.5 & sigma=2 & n=100 & 18.34 \\ 
  28 & MLE & Measure & beta=3 & sigma=2 & n=100 & 1559.71 \\ 
  29 & MLE.b & Measure & beta=3 & sigma=2 & n=100 & 1560.03 \\ 
  30 & LME & Measure & beta=3 & sigma=2 & n=100 & 30.08 \\ 
  31 & MDE.Phi.chisq & Measure & beta=3 & sigma=2 & n=100 & 1293.49 \\ 
  32 & MDE.Phi.tv & Measure & beta=3 & sigma=2 & n=100 & 1548.82 \\ 
  33 & MDE.Phi.kl & Measure & beta=3 & sigma=2 & n=100 & 182.00 \\ 
  34 & MME & Measure & beta=3 & sigma=2 & n=100 & 494285.04 \\ 
  35 & MME.b & Measure & beta=3 & sigma=2 & n=100 & 4701878.03 \\ 
  36 & PWM & Measure & beta=3 & sigma=2 & n=100 & 30.08 \\ 
  37 & MLE & Measure & beta=4 & sigma=2 & n=100 & 2131.02 \\ 
  38 & MLE.b & Measure & beta=4 & sigma=2 & n=100 & 2132.28 \\ 
  39 & LME & Measure & beta=4 & sigma=2 & n=100 & 71.77 \\ 
  40 & MDE.Phi.chisq & Measure & beta=4 & sigma=2 & n=100 & 2313.66 \\ 
  41 & MDE.Phi.tv & Measure & beta=4 & sigma=2 & n=100 & 2646.05 \\ 
  42 & MDE.Phi.kl & Measure & beta=4 & sigma=2 & n=100 & 297.08 \\ 
  43 & MME & Measure & beta=4 & sigma=2 & n=100 & 15977.38 \\ 
  44 & MME.b & Measure & beta=4 & sigma=2 & n=100 & 3005055.05 \\ 
  45 & PWM & Measure & beta=4 & sigma=2 & n=100 & 71.77 \\ 
  46 & MLE & Measure & beta=5 & sigma=2 & n=100 & 3364.37 \\ 
  47 & MLE.b & Measure & beta=5 & sigma=2 & n=100 & 3366.10 \\ 
  48 & LME & Measure & beta=5 & sigma=2 & n=100 & 124.13 \\ 
  49 & MDE.Phi.chisq & Measure & beta=5 & sigma=2 & n=100 & 3049.91 \\ 
  50 & MDE.Phi.tv & Measure & beta=5 & sigma=2 & n=100 & 3309.26 \\ 
  51 & MDE.Phi.kl & Measure & beta=5 & sigma=2 & n=100 & 455.53 \\ 
  52 & MME & Measure & beta=5 & sigma=2 & n=100 & 22900.46 \\ 
  53 & MME.b & Measure & beta=5 & sigma=2 & n=100 & 321769.19 \\ 
  54 & PWM & Measure & beta=5 & sigma=2 & n=100 & 124.13 \\ 
  55 & MLE & Measure & beta=1.5 & sigma=2 & n=200 & 0.84 \\ 
  56 & MLE.b & Measure & beta=1.5 & sigma=2 & n=200 & 0.49 \\ 
  57 & LME & Measure & beta=1.5 & sigma=2 & n=200 & 0.81 \\ 
  58 & MDE.Phi.chisq & Measure & beta=1.5 & sigma=2 & n=200 & 26.97 \\ 
  59 & MDE.Phi.tv & Measure & beta=1.5 & sigma=2 & n=200 & 1.84 \\ 
  60 & MDE.Phi.kl & Measure & beta=1.5 & sigma=2 & n=200 & 0.57 \\ 
  61 & MME & Measure & beta=1.5 & sigma=2 & n=200 & 19.97 \\ 
  62 & MME.b & Measure & beta=1.5 & sigma=2 & n=200 & 16.45 \\ 
  63 & PWM & Measure & beta=1.5 & sigma=2 & n=200 & 0.81 \\ 
  64 & MLE & Measure & beta=2 & sigma=2 & n=200 & 1.10 \\ 
  65 & MLE.b & Measure & beta=2 & sigma=2 & n=200 & 0.61 \\ 
  66 & LME & Measure & beta=2 & sigma=2 & n=200 & 1.03 \\ 
  67 & MDE.Phi.chisq & Measure & beta=2 & sigma=2 & n=200 & 9.87 \\ 
  68 & MDE.Phi.tv & Measure & beta=2 & sigma=2 & n=200 & 11.85 \\ 
  69 & MDE.Phi.kl & Measure & beta=2 & sigma=2 & n=200 & 0.94 \\ 
  70 & MME & Measure & beta=2 & sigma=2 & n=200 & 5.75 \\ 
  71 & MME.b & Measure & beta=2 & sigma=2 & n=200 & 17.74 \\ 
  72 & PWM & Measure & beta=2 & sigma=2 & n=200 & 1.03 \\ 
  73 & MLE & Measure & beta=2.5 & sigma=2 & n=200 & 3.32 \\ 
  74 & MLE.b & Measure & beta=2.5 & sigma=2 & n=200 & 2.45 \\ 
  75 & LME & Measure & beta=2.5 & sigma=2 & n=200 & 2.72 \\ 
  76 & MDE.Phi.chisq & Measure & beta=2.5 & sigma=2 & n=200 & 54.67 \\ 
  77 & MDE.Phi.tv & Measure & beta=2.5 & sigma=2 & n=200 & 41.13 \\ 
  78 & MDE.Phi.kl & Measure & beta=2.5 & sigma=2 & n=200 & 2.58 \\ 
  79 & MME & Measure & beta=2.5 & sigma=2 & n=200 & 6.75 \\ 
  80 & MME.b & Measure & beta=2.5 & sigma=2 & n=200 & 94.72 \\ 
  81 & PWM & Measure & beta=2.5 & sigma=2 & n=200 & 2.72 \\ 
  82 & MLE & Measure & beta=3 & sigma=2 & n=200 & 293.08 \\ 
  83 & MLE.b & Measure & beta=3 & sigma=2 & n=200 & 291.99 \\ 
  84 & LME & Measure & beta=3 & sigma=2 & n=200 & 7.47 \\ 
  85 & MDE.Phi.chisq & Measure & beta=3 & sigma=2 & n=200 & 208.60 \\ 
  86 & MDE.Phi.tv & Measure & beta=3 & sigma=2 & n=200 & 96.15 \\ 
  87 & MDE.Phi.kl & Measure & beta=3 & sigma=2 & n=200 & 13.66 \\ 
  88 & MME & Measure & beta=3 & sigma=2 & n=200 & 124.11 \\ 
  89 & MME.b & Measure & beta=3 & sigma=2 & n=200 & 14084.74 \\ 
  90 & PWM & Measure & beta=3 & sigma=2 & n=200 & 7.47 \\ 
  91 & MLE & Measure & beta=4 & sigma=2 & n=200 & 224.87 \\ 
  92 & MLE.b & Measure & beta=4 & sigma=2 & n=200 & 224.55 \\ 
  93 & LME & Measure & beta=4 & sigma=2 & n=200 & 25.14 \\ 
  94 & MDE.Phi.chisq & Measure & beta=4 & sigma=2 & n=200 & 798.34 \\ 
  95 & MDE.Phi.tv & Measure & beta=4 & sigma=2 & n=200 & 584.55 \\ 
  96 & MDE.Phi.kl & Measure & beta=4 & sigma=2 & n=200 & 59.01 \\ 
  97 & MME & Measure & beta=4 & sigma=2 & n=200 & 764.65 \\ 
  98 & MME.b & Measure & beta=4 & sigma=2 & n=200 & 60104.90 \\ 
  99 & PWM & Measure & beta=4 & sigma=2 & n=200 & 25.14 \\ 
  100 & MLE & Measure & beta=5 & sigma=2 & n=200 & 13049.22 \\ 
  101 & MLE.b & Measure & beta=5 & sigma=2 & n=200 & 13050.22 \\ 
  102 & LME & Measure & beta=5 & sigma=2 & n=200 & 81.06 \\ 
  103 & MDE.Phi.chisq & Measure & beta=5 & sigma=2 & n=200 & 1698.76 \\ 
  104 & MDE.Phi.tv & Measure & beta=5 & sigma=2 & n=200 & 1106.32 \\ 
  105 & MDE.Phi.kl & Measure & beta=5 & sigma=2 & n=200 & 173.21 \\ 
  106 & MME & Measure & beta=5 & sigma=2 & n=200 & 3343.39 \\ 
  107 & MME.b & Measure & beta=5 & sigma=2 & n=200 & 37995.60 \\ 
  108 & PWM & Measure & beta=5 & sigma=2 & n=200 & 81.06 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220203/Output.accuracy2.LaTeX.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Tue Feb 01 15:49:34 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & Measure & beta=1.5 & sigma=2 & n=100 & 0.00 \\ 
  2 & MLE.b & Measure & beta=1.5 & sigma=2 & n=100 & 0.00 \\ 
  3 & LME & Measure & beta=1.5 & sigma=2 & n=100 & 0.00 \\ 
  4 & MDE.Phi.chisq & Measure & beta=1.5 & sigma=2 & n=100 & 16388545707783178620260440008882462028666402824264064840002848602064644026068422688648064042426000406008404624648684664024604240882802040402642024426044402280264208866460866204284608004000428088080204864660402422800606024068664422446222660000246464448602468622826028820882884204864628226040022026806066.00 \\ 
  5 & MDE.Phi.tv & Measure & beta=1.5 & sigma=2 & n=100 & 0.04 \\ 
  6 & MDE.Phi.kl & Measure & beta=1.5 & sigma=2 & n=100 & 0.00 \\ 
  7 & MME & Measure & beta=1.5 & sigma=2 & n=100 & 0.01 \\ 
  8 & MME.b & Measure & beta=1.5 & sigma=2 & n=100 & 7.11 \\ 
  9 & PWM & Measure & beta=1.5 & sigma=2 & n=100 & 0.00 \\ 
  10 & MLE & Measure & beta=2 & sigma=2 & n=100 & 0.00 \\ 
  11 & MLE.b & Measure & beta=2 & sigma=2 & n=100 & 0.00 \\ 
  12 & LME & Measure & beta=2 & sigma=2 & n=100 & 0.00 \\ 
  13 & MDE.Phi.chisq & Measure & beta=2 & sigma=2 & n=100 & 0.03 \\ 
  14 & MDE.Phi.tv & Measure & beta=2 & sigma=2 & n=100 & 0.02 \\ 
  15 & MDE.Phi.kl & Measure & beta=2 & sigma=2 & n=100 & 0.00 \\ 
  16 & MME & Measure & beta=2 & sigma=2 & n=100 & 0.00 \\ 
  17 & MME.b & Measure & beta=2 & sigma=2 & n=100 & 0.01 \\ 
  18 & PWM & Measure & beta=2 & sigma=2 & n=100 & 0.00 \\ 
  19 & MLE & Measure & beta=2.5 & sigma=2 & n=100 & 0.00 \\ 
  20 & MLE.b & Measure & beta=2.5 & sigma=2 & n=100 & 0.00 \\ 
  21 & LME & Measure & beta=2.5 & sigma=2 & n=100 & 0.00 \\ 
  22 & MDE.Phi.chisq & Measure & beta=2.5 & sigma=2 & n=100 & 0.02 \\ 
  23 & MDE.Phi.tv & Measure & beta=2.5 & sigma=2 & n=100 & 0.02 \\ 
  24 & MDE.Phi.kl & Measure & beta=2.5 & sigma=2 & n=100 & 0.00 \\ 
  25 & MME & Measure & beta=2.5 & sigma=2 & n=100 & 0.00 \\ 
  26 & MME.b & Measure & beta=2.5 & sigma=2 & n=100 & 8.08 \\ 
  27 & PWM & Measure & beta=2.5 & sigma=2 & n=100 & 0.00 \\ 
  28 & MLE & Measure & beta=3 & sigma=2 & n=100 & 0.00 \\ 
  29 & MLE.b & Measure & beta=3 & sigma=2 & n=100 & 0.00 \\ 
  30 & LME & Measure & beta=3 & sigma=2 & n=100 & 0.00 \\ 
  31 & MDE.Phi.chisq & Measure & beta=3 & sigma=2 & n=100 & 0.02 \\ 
  32 & MDE.Phi.tv & Measure & beta=3 & sigma=2 & n=100 & 0.02 \\ 
  33 & MDE.Phi.kl & Measure & beta=3 & sigma=2 & n=100 & 0.00 \\ 
  34 & MME & Measure & beta=3 & sigma=2 & n=100 & 0.00 \\ 
  35 & MME.b & Measure & beta=3 & sigma=2 & n=100 & 0.01 \\ 
  36 & PWM & Measure & beta=3 & sigma=2 & n=100 & 0.00 \\ 
  37 & MLE & Measure & beta=4 & sigma=2 & n=100 & 0.00 \\ 
  38 & MLE.b & Measure & beta=4 & sigma=2 & n=100 & 0.00 \\ 
  39 & LME & Measure & beta=4 & sigma=2 & n=100 & 0.00 \\ 
  40 & MDE.Phi.chisq & Measure & beta=4 & sigma=2 & n=100 & 0.02 \\ 
  41 & MDE.Phi.tv & Measure & beta=4 & sigma=2 & n=100 & 0.01 \\ 
  42 & MDE.Phi.kl & Measure & beta=4 & sigma=2 & n=100 & 0.00 \\ 
  43 & MME & Measure & beta=4 & sigma=2 & n=100 & 0.00 \\ 
  44 & MME.b & Measure & beta=4 & sigma=2 & n=100 & 4041.95 \\ 
  45 & PWM & Measure & beta=4 & sigma=2 & n=100 & 0.00 \\ 
  46 & MLE & Measure & beta=5 & sigma=2 & n=100 & 0.00 \\ 
  47 & MLE.b & Measure & beta=5 & sigma=2 & n=100 & 0.00 \\ 
  48 & LME & Measure & beta=5 & sigma=2 & n=100 & 0.00 \\ 
  49 & MDE.Phi.chisq & Measure & beta=5 & sigma=2 & n=100 & 0.01 \\ 
  50 & MDE.Phi.tv & Measure & beta=5 & sigma=2 & n=100 & 0.01 \\ 
  51 & MDE.Phi.kl & Measure & beta=5 & sigma=2 & n=100 & 0.00 \\ 
  52 & MME & Measure & beta=5 & sigma=2 & n=100 & 0.00 \\ 
  53 & MME.b & Measure & beta=5 & sigma=2 & n=100 & 515620838018138634806240604226.00 \\ 
  54 & PWM & Measure & beta=5 & sigma=2 & n=100 & 0.00 \\ 
  55 & MLE & Measure & beta=1.5 & sigma=2 & n=200 & 0.00 \\ 
  56 & MLE.b & Measure & beta=1.5 & sigma=2 & n=200 & 0.00 \\ 
  57 & LME & Measure & beta=1.5 & sigma=2 & n=200 & 0.00 \\ 
  58 & MDE.Phi.chisq & Measure & beta=1.5 & sigma=2 & n=200 & 274643118624275331360628286448288226248464468022642204668864084082600222086880608668040080880424622046222024608200240484826064404080888868246080264664220228006844402404026242842008664860822820666228446808646200060266406262242888228420024466628024282446084862640644224086266044024064680440202202400842.00 \\ 
  59 & MDE.Phi.tv & Measure & beta=1.5 & sigma=2 & n=200 & 0.03 \\ 
  60 & MDE.Phi.kl & Measure & beta=1.5 & sigma=2 & n=200 & 0.00 \\ 
  61 & MME & Measure & beta=1.5 & sigma=2 & n=200 & 0.01 \\ 
  62 & MME.b & Measure & beta=1.5 & sigma=2 & n=200 & 0.01 \\ 
  63 & PWM & Measure & beta=1.5 & sigma=2 & n=200 & 0.00 \\ 
  64 & MLE & Measure & beta=2 & sigma=2 & n=200 & 0.00 \\ 
  65 & MLE.b & Measure & beta=2 & sigma=2 & n=200 & 0.00 \\ 
  66 & LME & Measure & beta=2 & sigma=2 & n=200 & 0.00 \\ 
  67 & MDE.Phi.chisq & Measure & beta=2 & sigma=2 & n=200 & 0.02 \\ 
  68 & MDE.Phi.tv & Measure & beta=2 & sigma=2 & n=200 & 0.02 \\ 
  69 & MDE.Phi.kl & Measure & beta=2 & sigma=2 & n=200 & 0.00 \\ 
  70 & MME & Measure & beta=2 & sigma=2 & n=200 & 0.00 \\ 
  71 & MME.b & Measure & beta=2 & sigma=2 & n=200 & 0.00 \\ 
  72 & PWM & Measure & beta=2 & sigma=2 & n=200 & 0.00 \\ 
  73 & MLE & Measure & beta=2.5 & sigma=2 & n=200 & 0.00 \\ 
  74 & MLE.b & Measure & beta=2.5 & sigma=2 & n=200 & 0.00 \\ 
  75 & LME & Measure & beta=2.5 & sigma=2 & n=200 & 0.00 \\ 
  76 & MDE.Phi.chisq & Measure & beta=2.5 & sigma=2 & n=200 & 0.02 \\ 
  77 & MDE.Phi.tv & Measure & beta=2.5 & sigma=2 & n=200 & 0.01 \\ 
  78 & MDE.Phi.kl & Measure & beta=2.5 & sigma=2 & n=200 & 0.00 \\ 
  79 & MME & Measure & beta=2.5 & sigma=2 & n=200 & 0.00 \\ 
  80 & MME.b & Measure & beta=2.5 & sigma=2 & n=200 & 0.00 \\ 
  81 & PWM & Measure & beta=2.5 & sigma=2 & n=200 & 0.00 \\ 
  82 & MLE & Measure & beta=3 & sigma=2 & n=200 & 0.00 \\ 
  83 & MLE.b & Measure & beta=3 & sigma=2 & n=200 & 0.00 \\ 
  84 & LME & Measure & beta=3 & sigma=2 & n=200 & 0.00 \\ 
  85 & MDE.Phi.chisq & Measure & beta=3 & sigma=2 & n=200 & 0.01 \\ 
  86 & MDE.Phi.tv & Measure & beta=3 & sigma=2 & n=200 & 0.01 \\ 
  87 & MDE.Phi.kl & Measure & beta=3 & sigma=2 & n=200 & 0.00 \\ 
  88 & MME & Measure & beta=3 & sigma=2 & n=200 & 0.00 \\ 
  89 & MME.b & Measure & beta=3 & sigma=2 & n=200 & 0.00 \\ 
  90 & PWM & Measure & beta=3 & sigma=2 & n=200 & 0.00 \\ 
  91 & MLE & Measure & beta=4 & sigma=2 & n=200 & 0.00 \\ 
  92 & MLE.b & Measure & beta=4 & sigma=2 & n=200 & 0.00 \\ 
  93 & LME & Measure & beta=4 & sigma=2 & n=200 & 0.00 \\ 
  94 & MDE.Phi.chisq & Measure & beta=4 & sigma=2 & n=200 & 0.01 \\ 
  95 & MDE.Phi.tv & Measure & beta=4 & sigma=2 & n=200 & 0.01 \\ 
  96 & MDE.Phi.kl & Measure & beta=4 & sigma=2 & n=200 & 0.00 \\ 
  97 & MME & Measure & beta=4 & sigma=2 & n=200 & 0.00 \\ 
  98 & MME.b & Measure & beta=4 & sigma=2 & n=200 & 0.00 \\ 
  99 & PWM & Measure & beta=4 & sigma=2 & n=200 & 0.00 \\ 
  100 & MLE & Measure & beta=5 & sigma=2 & n=200 & 0.00 \\ 
  101 & MLE.b & Measure & beta=5 & sigma=2 & n=200 & 0.00 \\ 
  102 & LME & Measure & beta=5 & sigma=2 & n=200 & 0.00 \\ 
  103 & MDE.Phi.chisq & Measure & beta=5 & sigma=2 & n=200 & 0.01 \\ 
  104 & MDE.Phi.tv & Measure & beta=5 & sigma=2 & n=200 & 0.01 \\ 
  105 & MDE.Phi.kl & Measure & beta=5 & sigma=2 & n=200 & 0.00 \\ 
  106 & MME & Measure & beta=5 & sigma=2 & n=200 & 0.00 \\ 
  107 & MME.b & Measure & beta=5 & sigma=2 & n=200 & 2.02 \\ 
  108 & PWM & Measure & beta=5 & sigma=2 & n=200 & 0.00 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220203/Output.bias.LaTeX.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Tue Feb 01 15:49:34 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=2 & n=100 & 0.17 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=2 & n=100 & -0.02 \\ 
  3 & LME & beta & beta=1.5 & sigma=2 & n=100 & 0.33 \\ 
  4 & MDE.Phi.chisq & beta & beta=1.5 & sigma=2 & n=100 & -1.27 \\ 
  5 & MDE.Phi.tv & beta & beta=1.5 & sigma=2 & n=100 & -0.24 \\ 
  6 & MDE.Phi.kl & beta & beta=1.5 & sigma=2 & n=100 & 0.17 \\ 
  7 & MME & beta & beta=1.5 & sigma=2 & n=100 & 1.29 \\ 
  8 & MME.b & beta & beta=1.5 & sigma=2 & n=100 & 4.81 \\ 
  9 & PWM & beta & beta=1.5 & sigma=2 & n=100 & 0.33 \\ 
  10 & MLE & sigma & beta=1.5 & sigma=2 & n=100 & 0.36 \\ 
  11 & MLE.b & sigma & beta=1.5 & sigma=2 & n=100 & -0.05 \\ 
  12 & LME & sigma & beta=1.5 & sigma=2 & n=100 & 0.65 \\ 
  13 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=2 & n=100 & 1.29 \\ 
  14 & MDE.Phi.tv & sigma & beta=1.5 & sigma=2 & n=100 & 1.64 \\ 
  15 & MDE.Phi.kl & sigma & beta=1.5 & sigma=2 & n=100 & 0.36 \\ 
  16 & MME & sigma & beta=1.5 & sigma=2 & n=100 & 4.30 \\ 
  17 & MME.b & sigma & beta=1.5 & sigma=2 & n=100 & 11.67 \\ 
  18 & PWM & sigma & beta=1.5 & sigma=2 & n=100 & 0.65 \\ 
  19 & MLE & beta & beta=2 & sigma=2 & n=100 & 0.54 \\ 
  20 & MLE.b & beta & beta=2 & sigma=2 & n=100 & 0.19 \\ 
  21 & LME & beta & beta=2 & sigma=2 & n=100 & 0.45 \\ 
  22 & MDE.Phi.chisq & beta & beta=2 & sigma=2 & n=100 & 0.10 \\ 
  23 & MDE.Phi.tv & beta & beta=2 & sigma=2 & n=100 & 0.69 \\ 
  24 & MDE.Phi.kl & beta & beta=2 & sigma=2 & n=100 & 0.46 \\ 
  25 & MME & beta & beta=2 & sigma=2 & n=100 & 1.68 \\ 
  26 & MME.b & beta & beta=2 & sigma=2 & n=100 & 7.48 \\ 
  27 & PWM & beta & beta=2 & sigma=2 & n=100 & 0.45 \\ 
  28 & MLE & sigma & beta=2 & sigma=2 & n=100 & 0.75 \\ 
  29 & MLE.b & sigma & beta=2 & sigma=2 & n=100 & 0.24 \\ 
  30 & LME & sigma & beta=2 & sigma=2 & n=100 & 0.60 \\ 
  31 & MDE.Phi.chisq & sigma & beta=2 & sigma=2 & n=100 & 2.19 \\ 
  32 & MDE.Phi.tv & sigma & beta=2 & sigma=2 & n=100 & 3.22 \\ 
  33 & MDE.Phi.kl & sigma & beta=2 & sigma=2 & n=100 & 0.65 \\ 
  34 & MME & sigma & beta=2 & sigma=2 & n=100 & 2.87 \\ 
  35 & MME.b & sigma & beta=2 & sigma=2 & n=100 & 11.17 \\ 
  36 & PWM & sigma & beta=2 & sigma=2 & n=100 & 0.60 \\ 
  37 & MLE & beta & beta=2.5 & sigma=2 & n=100 & 1.09 \\ 
  38 & MLE.b & beta & beta=2.5 & sigma=2 & n=100 & 0.63 \\ 
  39 & LME & beta & beta=2.5 & sigma=2 & n=100 & 0.70 \\ 
  40 & MDE.Phi.chisq & beta & beta=2.5 & sigma=2 & n=100 & 1.61 \\ 
  41 & MDE.Phi.tv & beta & beta=2.5 & sigma=2 & n=100 & 2.43 \\ 
  42 & MDE.Phi.kl & beta & beta=2.5 & sigma=2 & n=100 & 0.94 \\ 
  43 & MME & beta & beta=2.5 & sigma=2 & n=100 & 2.32 \\ 
  44 & MME.b & beta & beta=2.5 & sigma=2 & n=100 & 5.49 \\ 
  45 & PWM & beta & beta=2.5 & sigma=2 & n=100 & 0.70 \\ 
  46 & MLE & sigma & beta=2.5 & sigma=2 & n=100 & 1.17 \\ 
  47 & MLE.b & sigma & beta=2.5 & sigma=2 & n=100 & 0.67 \\ 
  48 & LME & sigma & beta=2.5 & sigma=2 & n=100 & 0.72 \\ 
  49 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=2 & n=100 & 4.14 \\ 
  50 & MDE.Phi.tv & sigma & beta=2.5 & sigma=2 & n=100 & 5.19 \\ 
  51 & MDE.Phi.kl & sigma & beta=2.5 & sigma=2 & n=100 & 1.01 \\ 
  52 & MME & sigma & beta=2.5 & sigma=2 & n=100 & 2.71 \\ 
  53 & MME.b & sigma & beta=2.5 & sigma=2 & n=100 & 6.04 \\ 
  54 & PWM & sigma & beta=2.5 & sigma=2 & n=100 & 0.72 \\ 
  55 & MLE & beta & beta=3 & sigma=2 & n=100 & 2.75 \\ 
  56 & MLE.b & beta & beta=3 & sigma=2 & n=100 & 2.26 \\ 
  57 & LME & beta & beta=3 & sigma=2 & n=100 & 1.02 \\ 
  58 & MDE.Phi.chisq & beta & beta=3 & sigma=2 & n=100 & 3.82 \\ 
  59 & MDE.Phi.tv & beta & beta=3 & sigma=2 & n=100 & 5.23 \\ 
  60 & MDE.Phi.kl & beta & beta=3 & sigma=2 & n=100 & 1.86 \\ 
  61 & MME & beta & beta=3 & sigma=2 & n=100 & 14.49 \\ 
  62 & MME.b & beta & beta=3 & sigma=2 & n=100 & 46.99 \\ 
  63 & PWM & beta & beta=3 & sigma=2 & n=100 & 1.02 \\ 
  64 & MLE & sigma & beta=3 & sigma=2 & n=100 & 2.37 \\ 
  65 & MLE.b & sigma & beta=3 & sigma=2 & n=100 & 1.94 \\ 
  66 & LME & sigma & beta=3 & sigma=2 & n=100 & 0.85 \\ 
  67 & MDE.Phi.chisq & sigma & beta=3 & sigma=2 & n=100 & 6.25 \\ 
  68 & MDE.Phi.tv & sigma & beta=3 & sigma=2 & n=100 & 7.70 \\ 
  69 & MDE.Phi.kl & sigma & beta=3 & sigma=2 & n=100 & 1.60 \\ 
  70 & MME & sigma & beta=3 & sigma=2 & n=100 & 11.48 \\ 
  71 & MME.b & sigma & beta=3 & sigma=2 & n=100 & 37.14 \\ 
  72 & PWM & sigma & beta=3 & sigma=2 & n=100 & 0.85 \\ 
  73 & MLE & beta & beta=4 & sigma=2 & n=100 & 4.73 \\ 
  74 & MLE.b & beta & beta=4 & sigma=2 & n=100 & 4.28 \\ 
  75 & LME & beta & beta=4 & sigma=2 & n=100 & 1.76 \\ 
  76 & MDE.Phi.chisq & beta & beta=4 & sigma=2 & n=100 & 9.77 \\ 
  77 & MDE.Phi.tv & beta & beta=4 & sigma=2 & n=100 & 11.95 \\ 
  78 & MDE.Phi.kl & beta & beta=4 & sigma=2 & n=100 & 3.42 \\ 
  79 & MME & beta & beta=4 & sigma=2 & n=100 & 7.36 \\ 
  80 & MME.b & beta & beta=4 & sigma=2 & n=100 & 36.91 \\ 
  81 & PWM & beta & beta=4 & sigma=2 & n=100 & 1.76 \\ 
  82 & MLE & sigma & beta=4 & sigma=2 & n=100 & 2.93 \\ 
  83 & MLE.b & sigma & beta=4 & sigma=2 & n=100 & 2.65 \\ 
  84 & LME & sigma & beta=4 & sigma=2 & n=100 & 1.07 \\ 
  85 & MDE.Phi.chisq & sigma & beta=4 & sigma=2 & n=100 & 9.83 \\ 
  86 & MDE.Phi.tv & sigma & beta=4 & sigma=2 & n=100 & 11.26 \\ 
  87 & MDE.Phi.kl & sigma & beta=4 & sigma=2 & n=100 & 2.12 \\ 
  88 & MME & sigma & beta=4 & sigma=2 & n=100 & 4.67 \\ 
  89 & MME.b & sigma & beta=4 & sigma=2 & n=100 & 24.87 \\ 
  90 & PWM & sigma & beta=4 & sigma=2 & n=100 & 1.07 \\ 
  91 & MLE & beta & beta=5 & sigma=2 & n=100 & 7.32 \\ 
  92 & MLE.b & beta & beta=5 & sigma=2 & n=100 & 6.96 \\ 
  93 & LME & beta & beta=5 & sigma=2 & n=100 & 2.36 \\ 
  94 & MDE.Phi.chisq & beta & beta=5 & sigma=2 & n=100 & 15.09 \\ 
  95 & MDE.Phi.tv & beta & beta=5 & sigma=2 & n=100 & 17.24 \\ 
  96 & MDE.Phi.kl & beta & beta=5 & sigma=2 & n=100 & 5.06 \\ 
  97 & MME & beta & beta=5 & sigma=2 & n=100 & 11.73 \\ 
  98 & MME.b & beta & beta=5 & sigma=2 & n=100 & 42.16 \\ 
  99 & PWM & beta & beta=5 & sigma=2 & n=100 & 2.36 \\ 
  100 & MLE & sigma & beta=5 & sigma=2 & n=100 & 3.45 \\ 
  101 & MLE.b & sigma & beta=5 & sigma=2 & n=100 & 3.28 \\ 
  102 & LME & sigma & beta=5 & sigma=2 & n=100 & 1.10 \\ 
  103 & MDE.Phi.chisq & sigma & beta=5 & sigma=2 & n=100 & 11.18 \\ 
  104 & MDE.Phi.tv & sigma & beta=5 & sigma=2 & n=100 & 12.16 \\ 
  105 & MDE.Phi.kl & sigma & beta=5 & sigma=2 & n=100 & 2.38 \\ 
  106 & MME & sigma & beta=5 & sigma=2 & n=100 & 5.50 \\ 
  107 & MME.b & sigma & beta=5 & sigma=2 & n=100 & 19.93 \\ 
  108 & PWM & sigma & beta=5 & sigma=2 & n=100 & 1.10 \\ 
  109 & MLE & beta & beta=1.5 & sigma=2 & n=200 & 0.23 \\ 
  110 & MLE.b & beta & beta=1.5 & sigma=2 & n=200 & 0.13 \\ 
  111 & LME & beta & beta=1.5 & sigma=2 & n=200 & 0.21 \\ 
  112 & MDE.Phi.chisq & beta & beta=1.5 & sigma=2 & n=200 & -0.85 \\ 
  113 & MDE.Phi.tv & beta & beta=1.5 & sigma=2 & n=200 & -0.50 \\ 
  114 & MDE.Phi.kl & beta & beta=1.5 & sigma=2 & n=200 & 0.08 \\ 
  115 & MME & beta & beta=1.5 & sigma=2 & n=200 & 1.00 \\ 
  116 & MME.b & beta & beta=1.5 & sigma=2 & n=200 & 0.80 \\ 
  117 & PWM & beta & beta=1.5 & sigma=2 & n=200 & 0.21 \\ 
  118 & MLE & sigma & beta=1.5 & sigma=2 & n=200 & 0.48 \\ 
  119 & MLE.b & sigma & beta=1.5 & sigma=2 & n=200 & 0.26 \\ 
  120 & LME & sigma & beta=1.5 & sigma=2 & n=200 & 0.40 \\ 
  121 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=2 & n=200 & 0.32 \\ 
  122 & MDE.Phi.tv & sigma & beta=1.5 & sigma=2 & n=200 & 0.51 \\ 
  123 & MDE.Phi.kl & sigma & beta=1.5 & sigma=2 & n=200 & 0.16 \\ 
  124 & MME & sigma & beta=1.5 & sigma=2 & n=200 & 3.57 \\ 
  125 & MME.b & sigma & beta=1.5 & sigma=2 & n=200 & 3.02 \\ 
  126 & PWM & sigma & beta=1.5 & sigma=2 & n=200 & 0.40 \\ 
  127 & MLE & beta & beta=2 & sigma=2 & n=200 & 0.25 \\ 
  128 & MLE.b & beta & beta=2 & sigma=2 & n=200 & 0.06 \\ 
  129 & LME & beta & beta=2 & sigma=2 & n=200 & 0.22 \\ 
  130 & MDE.Phi.chisq & beta & beta=2 & sigma=2 & n=200 & -0.65 \\ 
  131 & MDE.Phi.tv & beta & beta=2 & sigma=2 & n=200 & -0.44 \\ 
  132 & MDE.Phi.kl & beta & beta=2 & sigma=2 & n=200 & 0.14 \\ 
  133 & MME & beta & beta=2 & sigma=2 & n=200 & 0.97 \\ 
  134 & MME.b & beta & beta=2 & sigma=2 & n=200 & 0.69 \\ 
  135 & PWM & beta & beta=2 & sigma=2 & n=200 & 0.22 \\ 
  136 & MLE & sigma & beta=2 & sigma=2 & n=200 & 0.35 \\ 
  137 & MLE.b & sigma & beta=2 & sigma=2 & n=200 & 0.08 \\ 
  138 & LME & sigma & beta=2 & sigma=2 & n=200 & 0.28 \\ 
  139 & MDE.Phi.chisq & sigma & beta=2 & sigma=2 & n=200 & 0.34 \\ 
  140 & MDE.Phi.tv & sigma & beta=2 & sigma=2 & n=200 & 0.56 \\ 
  141 & MDE.Phi.kl & sigma & beta=2 & sigma=2 & n=200 & 0.19 \\ 
  142 & MME & sigma & beta=2 & sigma=2 & n=200 & 1.78 \\ 
  143 & MME.b & sigma & beta=2 & sigma=2 & n=200 & 1.29 \\ 
  144 & PWM & sigma & beta=2 & sigma=2 & n=200 & 0.28 \\ 
  145 & MLE & beta & beta=2.5 & sigma=2 & n=200 & 0.34 \\ 
  146 & MLE.b & beta & beta=2.5 & sigma=2 & n=200 & 0.02 \\ 
  147 & LME & beta & beta=2.5 & sigma=2 & n=200 & 0.28 \\ 
  148 & MDE.Phi.chisq & beta & beta=2.5 & sigma=2 & n=200 & -0.45 \\ 
  149 & MDE.Phi.tv & beta & beta=2.5 & sigma=2 & n=200 & -0.22 \\ 
  150 & MDE.Phi.kl & beta & beta=2.5 & sigma=2 & n=200 & 0.25 \\ 
  151 & MME & beta & beta=2.5 & sigma=2 & n=200 & 1.06 \\ 
  152 & MME.b & beta & beta=2.5 & sigma=2 & n=200 & 0.84 \\ 
  153 & PWM & beta & beta=2.5 & sigma=2 & n=200 & 0.28 \\ 
  154 & MLE & sigma & beta=2.5 & sigma=2 & n=200 & 0.37 \\ 
  155 & MLE.b & sigma & beta=2.5 & sigma=2 & n=200 & 0.02 \\ 
  156 & LME & sigma & beta=2.5 & sigma=2 & n=200 & 0.29 \\ 
  157 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=2 & n=200 & 0.70 \\ 
  158 & MDE.Phi.tv & sigma & beta=2.5 & sigma=2 & n=200 & 0.81 \\ 
  159 & MDE.Phi.kl & sigma & beta=2.5 & sigma=2 & n=200 & 0.27 \\ 
  160 & MME & sigma & beta=2.5 & sigma=2 & n=200 & 1.31 \\ 
  161 & MME.b & sigma & beta=2.5 & sigma=2 & n=200 & 1.01 \\ 
  162 & PWM & sigma & beta=2.5 & sigma=2 & n=200 & 0.29 \\ 
  163 & MLE & beta & beta=3 & sigma=2 & n=200 & 0.72 \\ 
  164 & MLE.b & beta & beta=3 & sigma=2 & n=200 & 0.23 \\ 
  165 & LME & beta & beta=3 & sigma=2 & n=200 & 0.45 \\ 
  166 & MDE.Phi.chisq & beta & beta=3 & sigma=2 & n=200 & 0.31 \\ 
  167 & MDE.Phi.tv & beta & beta=3 & sigma=2 & n=200 & 0.21 \\ 
  168 & MDE.Phi.kl & beta & beta=3 & sigma=2 & n=200 & 0.49 \\ 
  169 & MME & beta & beta=3 & sigma=2 & n=200 & 1.40 \\ 
  170 & MME.b & beta & beta=3 & sigma=2 & n=200 & 2.69 \\ 
  171 & PWM & beta & beta=3 & sigma=2 & n=200 & 0.45 \\ 
  172 & MLE & sigma & beta=3 & sigma=2 & n=200 & 0.62 \\ 
  173 & MLE.b & sigma & beta=3 & sigma=2 & n=200 & 0.20 \\ 
  174 & LME & sigma & beta=3 & sigma=2 & n=200 & 0.38 \\ 
  175 & MDE.Phi.chisq & sigma & beta=3 & sigma=2 & n=200 & 1.54 \\ 
  176 & MDE.Phi.tv & sigma & beta=3 & sigma=2 & n=200 & 1.19 \\ 
  177 & MDE.Phi.kl & sigma & beta=3 & sigma=2 & n=200 & 0.43 \\ 
  178 & MME & sigma & beta=3 & sigma=2 & n=200 & 1.29 \\ 
  179 & MME.b & sigma & beta=3 & sigma=2 & n=200 & 2.46 \\ 
  180 & PWM & sigma & beta=3 & sigma=2 & n=200 & 0.38 \\ 
  181 & MLE & beta & beta=4 & sigma=2 & n=200 & 1.56 \\ 
  182 & MLE.b & beta & beta=4 & sigma=2 & n=200 & 0.88 \\ 
  183 & LME & beta & beta=4 & sigma=2 & n=200 & 0.91 \\ 
  184 & MDE.Phi.chisq & beta & beta=4 & sigma=2 & n=200 & 3.71 \\ 
  185 & MDE.Phi.tv & beta & beta=4 & sigma=2 & n=200 & 2.95 \\ 
  186 & MDE.Phi.kl & beta & beta=4 & sigma=2 & n=200 & 1.26 \\ 
  187 & MME & beta & beta=4 & sigma=2 & n=200 & 2.64 \\ 
  188 & MME.b & beta & beta=4 & sigma=2 & n=200 & 9.69 \\ 
  189 & PWM & beta & beta=4 & sigma=2 & n=200 & 0.91 \\ 
  190 & MLE & sigma & beta=4 & sigma=2 & n=200 & 0.98 \\ 
  191 & MLE.b & sigma & beta=4 & sigma=2 & n=200 & 0.56 \\ 
  192 & LME & sigma & beta=4 & sigma=2 & n=200 & 0.55 \\ 
  193 & MDE.Phi.chisq & sigma & beta=4 & sigma=2 & n=200 & 4.00 \\ 
  194 & MDE.Phi.tv & sigma & beta=4 & sigma=2 & n=200 & 3.13 \\ 
  195 & MDE.Phi.kl & sigma & beta=4 & sigma=2 & n=200 & 0.77 \\ 
  196 & MME & sigma & beta=4 & sigma=2 & n=200 & 1.66 \\ 
  197 & MME.b & sigma & beta=4 & sigma=2 & n=200 & 6.25 \\ 
  198 & PWM & sigma & beta=4 & sigma=2 & n=200 & 0.55 \\ 
  199 & MLE & beta & beta=5 & sigma=2 & n=200 & 4.92 \\ 
  200 & MLE.b & beta & beta=5 & sigma=2 & n=200 & 4.21 \\ 
  201 & LME & beta & beta=5 & sigma=2 & n=200 & 1.78 \\ 
  202 & MDE.Phi.chisq & beta & beta=5 & sigma=2 & n=200 & 9.13 \\ 
  203 & MDE.Phi.tv & beta & beta=5 & sigma=2 & n=200 & 6.36 \\ 
  204 & MDE.Phi.kl & beta & beta=5 & sigma=2 & n=200 & 2.60 \\ 
  205 & MME & beta & beta=5 & sigma=2 & n=200 & 4.76 \\ 
  206 & MME.b & beta & beta=5 & sigma=2 & n=200 & 16.59 \\ 
  207 & PWM & beta & beta=5 & sigma=2 & n=200 & 1.78 \\ 
  208 & MLE & sigma & beta=5 & sigma=2 & n=200 & 2.38 \\ 
  209 & MLE.b & sigma & beta=5 & sigma=2 & n=200 & 2.04 \\ 
  210 & LME & sigma & beta=5 & sigma=2 & n=200 & 0.83 \\ 
  211 & MDE.Phi.chisq & sigma & beta=5 & sigma=2 & n=200 & 6.54 \\ 
  212 & MDE.Phi.tv & sigma & beta=5 & sigma=2 & n=200 & 4.51 \\ 
  213 & MDE.Phi.kl & sigma & beta=5 & sigma=2 & n=200 & 1.23 \\ 
  214 & MME & sigma & beta=5 & sigma=2 & n=200 & 2.27 \\ 
  215 & MME.b & sigma & beta=5 & sigma=2 & n=200 & 7.87 \\ 
  216 & PWM & sigma & beta=5 & sigma=2 & n=200 & 0.83 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220203/Output.mean.LaTeX.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Tue Feb 01 15:49:34 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=2 & n=100 & 1.67 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=2 & n=100 & 1.48 \\ 
  3 & LME & beta & beta=1.5 & sigma=2 & n=100 & 1.83 \\ 
  4 & MDE.Phi.chisq & beta & beta=1.5 & sigma=2 & n=100 & 0.23 \\ 
  5 & MDE.Phi.tv & beta & beta=1.5 & sigma=2 & n=100 & 1.26 \\ 
  6 & MDE.Phi.kl & beta & beta=1.5 & sigma=2 & n=100 & 1.67 \\ 
  7 & MME & beta & beta=1.5 & sigma=2 & n=100 & 2.79 \\ 
  8 & MME.b & beta & beta=1.5 & sigma=2 & n=100 & 6.31 \\ 
  9 & PWM & beta & beta=1.5 & sigma=2 & n=100 & 1.83 \\ 
  10 & MLE & sigma & beta=1.5 & sigma=2 & n=100 & 2.36 \\ 
  11 & MLE.b & sigma & beta=1.5 & sigma=2 & n=100 & 1.95 \\ 
  12 & LME & sigma & beta=1.5 & sigma=2 & n=100 & 2.65 \\ 
  13 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=2 & n=100 & 3.29 \\ 
  14 & MDE.Phi.tv & sigma & beta=1.5 & sigma=2 & n=100 & 3.64 \\ 
  15 & MDE.Phi.kl & sigma & beta=1.5 & sigma=2 & n=100 & 2.36 \\ 
  16 & MME & sigma & beta=1.5 & sigma=2 & n=100 & 6.30 \\ 
  17 & MME.b & sigma & beta=1.5 & sigma=2 & n=100 & 13.67 \\ 
  18 & PWM & sigma & beta=1.5 & sigma=2 & n=100 & 2.65 \\ 
  19 & MLE & beta & beta=2 & sigma=2 & n=100 & 2.54 \\ 
  20 & MLE.b & beta & beta=2 & sigma=2 & n=100 & 2.19 \\ 
  21 & LME & beta & beta=2 & sigma=2 & n=100 & 2.45 \\ 
  22 & MDE.Phi.chisq & beta & beta=2 & sigma=2 & n=100 & 2.10 \\ 
  23 & MDE.Phi.tv & beta & beta=2 & sigma=2 & n=100 & 2.69 \\ 
  24 & MDE.Phi.kl & beta & beta=2 & sigma=2 & n=100 & 2.46 \\ 
  25 & MME & beta & beta=2 & sigma=2 & n=100 & 3.68 \\ 
  26 & MME.b & beta & beta=2 & sigma=2 & n=100 & 9.48 \\ 
  27 & PWM & beta & beta=2 & sigma=2 & n=100 & 2.45 \\ 
  28 & MLE & sigma & beta=2 & sigma=2 & n=100 & 2.75 \\ 
  29 & MLE.b & sigma & beta=2 & sigma=2 & n=100 & 2.24 \\ 
  30 & LME & sigma & beta=2 & sigma=2 & n=100 & 2.60 \\ 
  31 & MDE.Phi.chisq & sigma & beta=2 & sigma=2 & n=100 & 4.19 \\ 
  32 & MDE.Phi.tv & sigma & beta=2 & sigma=2 & n=100 & 5.22 \\ 
  33 & MDE.Phi.kl & sigma & beta=2 & sigma=2 & n=100 & 2.65 \\ 
  34 & MME & sigma & beta=2 & sigma=2 & n=100 & 4.87 \\ 
  35 & MME.b & sigma & beta=2 & sigma=2 & n=100 & 13.17 \\ 
  36 & PWM & sigma & beta=2 & sigma=2 & n=100 & 2.60 \\ 
  37 & MLE & beta & beta=2.5 & sigma=2 & n=100 & 3.59 \\ 
  38 & MLE.b & beta & beta=2.5 & sigma=2 & n=100 & 3.13 \\ 
  39 & LME & beta & beta=2.5 & sigma=2 & n=100 & 3.20 \\ 
  40 & MDE.Phi.chisq & beta & beta=2.5 & sigma=2 & n=100 & 4.11 \\ 
  41 & MDE.Phi.tv & beta & beta=2.5 & sigma=2 & n=100 & 4.93 \\ 
  42 & MDE.Phi.kl & beta & beta=2.5 & sigma=2 & n=100 & 3.44 \\ 
  43 & MME & beta & beta=2.5 & sigma=2 & n=100 & 4.82 \\ 
  44 & MME.b & beta & beta=2.5 & sigma=2 & n=100 & 7.99 \\ 
  45 & PWM & beta & beta=2.5 & sigma=2 & n=100 & 3.20 \\ 
  46 & MLE & sigma & beta=2.5 & sigma=2 & n=100 & 3.17 \\ 
  47 & MLE.b & sigma & beta=2.5 & sigma=2 & n=100 & 2.67 \\ 
  48 & LME & sigma & beta=2.5 & sigma=2 & n=100 & 2.72 \\ 
  49 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=2 & n=100 & 6.14 \\ 
  50 & MDE.Phi.tv & sigma & beta=2.5 & sigma=2 & n=100 & 7.19 \\ 
  51 & MDE.Phi.kl & sigma & beta=2.5 & sigma=2 & n=100 & 3.01 \\ 
  52 & MME & sigma & beta=2.5 & sigma=2 & n=100 & 4.71 \\ 
  53 & MME.b & sigma & beta=2.5 & sigma=2 & n=100 & 8.04 \\ 
  54 & PWM & sigma & beta=2.5 & sigma=2 & n=100 & 2.72 \\ 
  55 & MLE & beta & beta=3 & sigma=2 & n=100 & 5.75 \\ 
  56 & MLE.b & beta & beta=3 & sigma=2 & n=100 & 5.26 \\ 
  57 & LME & beta & beta=3 & sigma=2 & n=100 & 4.02 \\ 
  58 & MDE.Phi.chisq & beta & beta=3 & sigma=2 & n=100 & 6.82 \\ 
  59 & MDE.Phi.tv & beta & beta=3 & sigma=2 & n=100 & 8.23 \\ 
  60 & MDE.Phi.kl & beta & beta=3 & sigma=2 & n=100 & 4.86 \\ 
  61 & MME & beta & beta=3 & sigma=2 & n=100 & 17.49 \\ 
  62 & MME.b & beta & beta=3 & sigma=2 & n=100 & 49.99 \\ 
  63 & PWM & beta & beta=3 & sigma=2 & n=100 & 4.02 \\ 
  64 & MLE & sigma & beta=3 & sigma=2 & n=100 & 4.37 \\ 
  65 & MLE.b & sigma & beta=3 & sigma=2 & n=100 & 3.94 \\ 
  66 & LME & sigma & beta=3 & sigma=2 & n=100 & 2.85 \\ 
  67 & MDE.Phi.chisq & sigma & beta=3 & sigma=2 & n=100 & 8.25 \\ 
  68 & MDE.Phi.tv & sigma & beta=3 & sigma=2 & n=100 & 9.70 \\ 
  69 & MDE.Phi.kl & sigma & beta=3 & sigma=2 & n=100 & 3.60 \\ 
  70 & MME & sigma & beta=3 & sigma=2 & n=100 & 13.48 \\ 
  71 & MME.b & sigma & beta=3 & sigma=2 & n=100 & 39.14 \\ 
  72 & PWM & sigma & beta=3 & sigma=2 & n=100 & 2.85 \\ 
  73 & MLE & beta & beta=4 & sigma=2 & n=100 & 8.73 \\ 
  74 & MLE.b & beta & beta=4 & sigma=2 & n=100 & 8.28 \\ 
  75 & LME & beta & beta=4 & sigma=2 & n=100 & 5.76 \\ 
  76 & MDE.Phi.chisq & beta & beta=4 & sigma=2 & n=100 & 13.77 \\ 
  77 & MDE.Phi.tv & beta & beta=4 & sigma=2 & n=100 & 15.95 \\ 
  78 & MDE.Phi.kl & beta & beta=4 & sigma=2 & n=100 & 7.42 \\ 
  79 & MME & beta & beta=4 & sigma=2 & n=100 & 11.36 \\ 
  80 & MME.b & beta & beta=4 & sigma=2 & n=100 & 40.91 \\ 
  81 & PWM & beta & beta=4 & sigma=2 & n=100 & 5.76 \\ 
  82 & MLE & sigma & beta=4 & sigma=2 & n=100 & 4.93 \\ 
  83 & MLE.b & sigma & beta=4 & sigma=2 & n=100 & 4.65 \\ 
  84 & LME & sigma & beta=4 & sigma=2 & n=100 & 3.07 \\ 
  85 & MDE.Phi.chisq & sigma & beta=4 & sigma=2 & n=100 & 11.83 \\ 
  86 & MDE.Phi.tv & sigma & beta=4 & sigma=2 & n=100 & 13.26 \\ 
  87 & MDE.Phi.kl & sigma & beta=4 & sigma=2 & n=100 & 4.12 \\ 
  88 & MME & sigma & beta=4 & sigma=2 & n=100 & 6.67 \\ 
  89 & MME.b & sigma & beta=4 & sigma=2 & n=100 & 26.87 \\ 
  90 & PWM & sigma & beta=4 & sigma=2 & n=100 & 3.07 \\ 
  91 & MLE & beta & beta=5 & sigma=2 & n=100 & 12.32 \\ 
  92 & MLE.b & beta & beta=5 & sigma=2 & n=100 & 11.96 \\ 
  93 & LME & beta & beta=5 & sigma=2 & n=100 & 7.36 \\ 
  94 & MDE.Phi.chisq & beta & beta=5 & sigma=2 & n=100 & 20.09 \\ 
  95 & MDE.Phi.tv & beta & beta=5 & sigma=2 & n=100 & 22.24 \\ 
  96 & MDE.Phi.kl & beta & beta=5 & sigma=2 & n=100 & 10.06 \\ 
  97 & MME & beta & beta=5 & sigma=2 & n=100 & 16.73 \\ 
  98 & MME.b & beta & beta=5 & sigma=2 & n=100 & 47.16 \\ 
  99 & PWM & beta & beta=5 & sigma=2 & n=100 & 7.36 \\ 
  100 & MLE & sigma & beta=5 & sigma=2 & n=100 & 5.45 \\ 
  101 & MLE.b & sigma & beta=5 & sigma=2 & n=100 & 5.28 \\ 
  102 & LME & sigma & beta=5 & sigma=2 & n=100 & 3.10 \\ 
  103 & MDE.Phi.chisq & sigma & beta=5 & sigma=2 & n=100 & 13.18 \\ 
  104 & MDE.Phi.tv & sigma & beta=5 & sigma=2 & n=100 & 14.16 \\ 
  105 & MDE.Phi.kl & sigma & beta=5 & sigma=2 & n=100 & 4.38 \\ 
  106 & MME & sigma & beta=5 & sigma=2 & n=100 & 7.50 \\ 
  107 & MME.b & sigma & beta=5 & sigma=2 & n=100 & 21.93 \\ 
  108 & PWM & sigma & beta=5 & sigma=2 & n=100 & 3.10 \\ 
  109 & MLE & beta & beta=1.5 & sigma=2 & n=200 & 1.73 \\ 
  110 & MLE.b & beta & beta=1.5 & sigma=2 & n=200 & 1.63 \\ 
  111 & LME & beta & beta=1.5 & sigma=2 & n=200 & 1.71 \\ 
  112 & MDE.Phi.chisq & beta & beta=1.5 & sigma=2 & n=200 & 0.65 \\ 
  113 & MDE.Phi.tv & beta & beta=1.5 & sigma=2 & n=200 & 1.00 \\ 
  114 & MDE.Phi.kl & beta & beta=1.5 & sigma=2 & n=200 & 1.58 \\ 
  115 & MME & beta & beta=1.5 & sigma=2 & n=200 & 2.50 \\ 
  116 & MME.b & beta & beta=1.5 & sigma=2 & n=200 & 2.30 \\ 
  117 & PWM & beta & beta=1.5 & sigma=2 & n=200 & 1.71 \\ 
  118 & MLE & sigma & beta=1.5 & sigma=2 & n=200 & 2.48 \\ 
  119 & MLE.b & sigma & beta=1.5 & sigma=2 & n=200 & 2.26 \\ 
  120 & LME & sigma & beta=1.5 & sigma=2 & n=200 & 2.40 \\ 
  121 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=2 & n=200 & 2.32 \\ 
  122 & MDE.Phi.tv & sigma & beta=1.5 & sigma=2 & n=200 & 2.51 \\ 
  123 & MDE.Phi.kl & sigma & beta=1.5 & sigma=2 & n=200 & 2.16 \\ 
  124 & MME & sigma & beta=1.5 & sigma=2 & n=200 & 5.57 \\ 
  125 & MME.b & sigma & beta=1.5 & sigma=2 & n=200 & 5.02 \\ 
  126 & PWM & sigma & beta=1.5 & sigma=2 & n=200 & 2.40 \\ 
  127 & MLE & beta & beta=2 & sigma=2 & n=200 & 2.25 \\ 
  128 & MLE.b & beta & beta=2 & sigma=2 & n=200 & 2.06 \\ 
  129 & LME & beta & beta=2 & sigma=2 & n=200 & 2.22 \\ 
  130 & MDE.Phi.chisq & beta & beta=2 & sigma=2 & n=200 & 1.35 \\ 
  131 & MDE.Phi.tv & beta & beta=2 & sigma=2 & n=200 & 1.56 \\ 
  132 & MDE.Phi.kl & beta & beta=2 & sigma=2 & n=200 & 2.14 \\ 
  133 & MME & beta & beta=2 & sigma=2 & n=200 & 2.97 \\ 
  134 & MME.b & beta & beta=2 & sigma=2 & n=200 & 2.69 \\ 
  135 & PWM & beta & beta=2 & sigma=2 & n=200 & 2.22 \\ 
  136 & MLE & sigma & beta=2 & sigma=2 & n=200 & 2.35 \\ 
  137 & MLE.b & sigma & beta=2 & sigma=2 & n=200 & 2.08 \\ 
  138 & LME & sigma & beta=2 & sigma=2 & n=200 & 2.28 \\ 
  139 & MDE.Phi.chisq & sigma & beta=2 & sigma=2 & n=200 & 2.34 \\ 
  140 & MDE.Phi.tv & sigma & beta=2 & sigma=2 & n=200 & 2.56 \\ 
  141 & MDE.Phi.kl & sigma & beta=2 & sigma=2 & n=200 & 2.19 \\ 
  142 & MME & sigma & beta=2 & sigma=2 & n=200 & 3.78 \\ 
  143 & MME.b & sigma & beta=2 & sigma=2 & n=200 & 3.29 \\ 
  144 & PWM & sigma & beta=2 & sigma=2 & n=200 & 2.28 \\ 
  145 & MLE & beta & beta=2.5 & sigma=2 & n=200 & 2.84 \\ 
  146 & MLE.b & beta & beta=2.5 & sigma=2 & n=200 & 2.52 \\ 
  147 & LME & beta & beta=2.5 & sigma=2 & n=200 & 2.78 \\ 
  148 & MDE.Phi.chisq & beta & beta=2.5 & sigma=2 & n=200 & 2.05 \\ 
  149 & MDE.Phi.tv & beta & beta=2.5 & sigma=2 & n=200 & 2.28 \\ 
  150 & MDE.Phi.kl & beta & beta=2.5 & sigma=2 & n=200 & 2.75 \\ 
  151 & MME & beta & beta=2.5 & sigma=2 & n=200 & 3.56 \\ 
  152 & MME.b & beta & beta=2.5 & sigma=2 & n=200 & 3.34 \\ 
  153 & PWM & beta & beta=2.5 & sigma=2 & n=200 & 2.78 \\ 
  154 & MLE & sigma & beta=2.5 & sigma=2 & n=200 & 2.37 \\ 
  155 & MLE.b & sigma & beta=2.5 & sigma=2 & n=200 & 2.02 \\ 
  156 & LME & sigma & beta=2.5 & sigma=2 & n=200 & 2.29 \\ 
  157 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=2 & n=200 & 2.70 \\ 
  158 & MDE.Phi.tv & sigma & beta=2.5 & sigma=2 & n=200 & 2.81 \\ 
  159 & MDE.Phi.kl & sigma & beta=2.5 & sigma=2 & n=200 & 2.27 \\ 
  160 & MME & sigma & beta=2.5 & sigma=2 & n=200 & 3.31 \\ 
  161 & MME.b & sigma & beta=2.5 & sigma=2 & n=200 & 3.01 \\ 
  162 & PWM & sigma & beta=2.5 & sigma=2 & n=200 & 2.29 \\ 
  163 & MLE & beta & beta=3 & sigma=2 & n=200 & 3.72 \\ 
  164 & MLE.b & beta & beta=3 & sigma=2 & n=200 & 3.23 \\ 
  165 & LME & beta & beta=3 & sigma=2 & n=200 & 3.45 \\ 
  166 & MDE.Phi.chisq & beta & beta=3 & sigma=2 & n=200 & 3.31 \\ 
  167 & MDE.Phi.tv & beta & beta=3 & sigma=2 & n=200 & 3.21 \\ 
  168 & MDE.Phi.kl & beta & beta=3 & sigma=2 & n=200 & 3.49 \\ 
  169 & MME & beta & beta=3 & sigma=2 & n=200 & 4.40 \\ 
  170 & MME.b & beta & beta=3 & sigma=2 & n=200 & 5.69 \\ 
  171 & PWM & beta & beta=3 & sigma=2 & n=200 & 3.45 \\ 
  172 & MLE & sigma & beta=3 & sigma=2 & n=200 & 2.62 \\ 
  173 & MLE.b & sigma & beta=3 & sigma=2 & n=200 & 2.20 \\ 
  174 & LME & sigma & beta=3 & sigma=2 & n=200 & 2.38 \\ 
  175 & MDE.Phi.chisq & sigma & beta=3 & sigma=2 & n=200 & 3.54 \\ 
  176 & MDE.Phi.tv & sigma & beta=3 & sigma=2 & n=200 & 3.19 \\ 
  177 & MDE.Phi.kl & sigma & beta=3 & sigma=2 & n=200 & 2.43 \\ 
  178 & MME & sigma & beta=3 & sigma=2 & n=200 & 3.29 \\ 
  179 & MME.b & sigma & beta=3 & sigma=2 & n=200 & 4.46 \\ 
  180 & PWM & sigma & beta=3 & sigma=2 & n=200 & 2.38 \\ 
  181 & MLE & beta & beta=4 & sigma=2 & n=200 & 5.56 \\ 
  182 & MLE.b & beta & beta=4 & sigma=2 & n=200 & 4.88 \\ 
  183 & LME & beta & beta=4 & sigma=2 & n=200 & 4.91 \\ 
  184 & MDE.Phi.chisq & beta & beta=4 & sigma=2 & n=200 & 7.71 \\ 
  185 & MDE.Phi.tv & beta & beta=4 & sigma=2 & n=200 & 6.95 \\ 
  186 & MDE.Phi.kl & beta & beta=4 & sigma=2 & n=200 & 5.26 \\ 
  187 & MME & beta & beta=4 & sigma=2 & n=200 & 6.64 \\ 
  188 & MME.b & beta & beta=4 & sigma=2 & n=200 & 13.69 \\ 
  189 & PWM & beta & beta=4 & sigma=2 & n=200 & 4.91 \\ 
  190 & MLE & sigma & beta=4 & sigma=2 & n=200 & 2.98 \\ 
  191 & MLE.b & sigma & beta=4 & sigma=2 & n=200 & 2.56 \\ 
  192 & LME & sigma & beta=4 & sigma=2 & n=200 & 2.55 \\ 
  193 & MDE.Phi.chisq & sigma & beta=4 & sigma=2 & n=200 & 6.00 \\ 
  194 & MDE.Phi.tv & sigma & beta=4 & sigma=2 & n=200 & 5.13 \\ 
  195 & MDE.Phi.kl & sigma & beta=4 & sigma=2 & n=200 & 2.77 \\ 
  196 & MME & sigma & beta=4 & sigma=2 & n=200 & 3.66 \\ 
  197 & MME.b & sigma & beta=4 & sigma=2 & n=200 & 8.25 \\ 
  198 & PWM & sigma & beta=4 & sigma=2 & n=200 & 2.55 \\ 
  199 & MLE & beta & beta=5 & sigma=2 & n=200 & 9.92 \\ 
  200 & MLE.b & beta & beta=5 & sigma=2 & n=200 & 9.21 \\ 
  201 & LME & beta & beta=5 & sigma=2 & n=200 & 6.78 \\ 
  202 & MDE.Phi.chisq & beta & beta=5 & sigma=2 & n=200 & 14.13 \\ 
  203 & MDE.Phi.tv & beta & beta=5 & sigma=2 & n=200 & 11.36 \\ 
  204 & MDE.Phi.kl & beta & beta=5 & sigma=2 & n=200 & 7.60 \\ 
  205 & MME & beta & beta=5 & sigma=2 & n=200 & 9.76 \\ 
  206 & MME.b & beta & beta=5 & sigma=2 & n=200 & 21.59 \\ 
  207 & PWM & beta & beta=5 & sigma=2 & n=200 & 6.78 \\ 
  208 & MLE & sigma & beta=5 & sigma=2 & n=200 & 4.38 \\ 
  209 & MLE.b & sigma & beta=5 & sigma=2 & n=200 & 4.04 \\ 
  210 & LME & sigma & beta=5 & sigma=2 & n=200 & 2.83 \\ 
  211 & MDE.Phi.chisq & sigma & beta=5 & sigma=2 & n=200 & 8.54 \\ 
  212 & MDE.Phi.tv & sigma & beta=5 & sigma=2 & n=200 & 6.51 \\ 
  213 & MDE.Phi.kl & sigma & beta=5 & sigma=2 & n=200 & 3.23 \\ 
  214 & MME & sigma & beta=5 & sigma=2 & n=200 & 4.27 \\ 
  215 & MME.b & sigma & beta=5 & sigma=2 & n=200 & 9.87 \\ 
  216 & PWM & sigma & beta=5 & sigma=2 & n=200 & 2.83 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220203/Output.mse.LaTeX.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Tue Feb 01 15:49:34 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=2 & n=100 & 0.46 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=2 & n=100 & 0.32 \\ 
  3 & LME & beta & beta=1.5 & sigma=2 & n=100 & 0.40 \\ 
  4 & MDE.Phi.chisq & beta & beta=1.5 & sigma=2 & n=100 & 99.21 \\ 
  5 & MDE.Phi.tv & beta & beta=1.5 & sigma=2 & n=100 & 6.84 \\ 
  6 & MDE.Phi.kl & beta & beta=1.5 & sigma=2 & n=100 & 0.46 \\ 
  7 & MME & beta & beta=1.5 & sigma=2 & n=100 & 2.57 \\ 
  8 & MME.b & beta & beta=1.5 & sigma=2 & n=100 & 130057.25 \\ 
  9 & PWM & beta & beta=1.5 & sigma=2 & n=100 & 0.40 \\ 
  10 & MLE & sigma & beta=1.5 & sigma=2 & n=100 & 2.09 \\ 
  11 & MLE.b & sigma & beta=1.5 & sigma=2 & n=100 & 1.45 \\ 
  12 & LME & sigma & beta=1.5 & sigma=2 & n=100 & 1.75 \\ 
  13 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=2 & n=100 & 83.70 \\ 
  14 & MDE.Phi.tv & sigma & beta=1.5 & sigma=2 & n=100 & 73.46 \\ 
  15 & MDE.Phi.kl & sigma & beta=1.5 & sigma=2 & n=100 & 2.09 \\ 
  16 & MME & sigma & beta=1.5 & sigma=2 & n=100 & 26.50 \\ 
  17 & MME.b & sigma & beta=1.5 & sigma=2 & n=100 & 595640.92 \\ 
  18 & PWM & sigma & beta=1.5 & sigma=2 & n=100 & 1.75 \\ 
  19 & MLE & beta & beta=2 & sigma=2 & n=100 & 66.35 \\ 
  20 & MLE.b & beta & beta=2 & sigma=2 & n=100 & 66.09 \\ 
  21 & LME & beta & beta=2 & sigma=2 & n=100 & 3.31 \\ 
  22 & MDE.Phi.chisq & beta & beta=2 & sigma=2 & n=100 & 65.39 \\ 
  23 & MDE.Phi.tv & beta & beta=2 & sigma=2 & n=100 & 87.75 \\ 
  24 & MDE.Phi.kl & beta & beta=2 & sigma=2 & n=100 & 12.40 \\ 
  25 & MME & beta & beta=2 & sigma=2 & n=100 & 55.69 \\ 
  26 & MME.b & beta & beta=2 & sigma=2 & n=100 & 151259.47 \\ 
  27 & PWM & beta & beta=2 & sigma=2 & n=100 & 3.31 \\ 
  28 & MLE & sigma & beta=2 & sigma=2 & n=100 & 94.21 \\ 
  29 & MLE.b & sigma & beta=2 & sigma=2 & n=100 & 93.65 \\ 
  30 & LME & sigma & beta=2 & sigma=2 & n=100 & 6.14 \\ 
  31 & MDE.Phi.chisq & sigma & beta=2 & sigma=2 & n=100 & 303.55 \\ 
  32 & MDE.Phi.tv & sigma & beta=2 & sigma=2 & n=100 & 389.41 \\ 
  33 & MDE.Phi.kl & sigma & beta=2 & sigma=2 & n=100 & 20.86 \\ 
  34 & MME & sigma & beta=2 & sigma=2 & n=100 & 99.67 \\ 
  35 & MME.b & sigma & beta=2 & sigma=2 & n=100 & 334286.83 \\ 
  36 & PWM & sigma & beta=2 & sigma=2 & n=100 & 6.14 \\ 
  37 & MLE & beta & beta=2.5 & sigma=2 & n=100 & 141.34 \\ 
  38 & MLE.b & beta & beta=2.5 & sigma=2 & n=100 & 141.21 \\ 
  39 & LME & beta & beta=2.5 & sigma=2 & n=100 & 8.83 \\ 
  40 & MDE.Phi.chisq & beta & beta=2.5 & sigma=2 & n=100 & 227.13 \\ 
  41 & MDE.Phi.tv & beta & beta=2.5 & sigma=2 & n=100 & 262.47 \\ 
  42 & MDE.Phi.kl & beta & beta=2.5 & sigma=2 & n=100 & 30.65 \\ 
  43 & MME & beta & beta=2.5 & sigma=2 & n=100 & 149.68 \\ 
  44 & MME.b & beta & beta=2.5 & sigma=2 & n=100 & 2235.69 \\ 
  45 & PWM & beta & beta=2.5 & sigma=2 & n=100 & 8.83 \\ 
  46 & MLE & sigma & beta=2.5 & sigma=2 & n=100 & 162.04 \\ 
  47 & MLE.b & sigma & beta=2.5 & sigma=2 & n=100 & 161.86 \\ 
  48 & LME & sigma & beta=2.5 & sigma=2 & n=100 & 9.51 \\ 
  49 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=2 & n=100 & 552.81 \\ 
  50 & MDE.Phi.tv & sigma & beta=2.5 & sigma=2 & n=100 & 638.28 \\ 
  51 & MDE.Phi.kl & sigma & beta=2.5 & sigma=2 & n=100 & 33.59 \\ 
  52 & MME & sigma & beta=2.5 & sigma=2 & n=100 & 157.46 \\ 
  53 & MME.b & sigma & beta=2.5 & sigma=2 & n=100 & 2556.57 \\ 
  54 & PWM & sigma & beta=2.5 & sigma=2 & n=100 & 9.51 \\ 
  55 & MLE & beta & beta=3 & sigma=2 & n=100 & 880.32 \\ 
  56 & MLE.b & beta & beta=3 & sigma=2 & n=100 & 880.53 \\ 
  57 & LME & beta & beta=3 & sigma=2 & n=100 & 17.02 \\ 
  58 & MDE.Phi.chisq & beta & beta=3 & sigma=2 & n=100 & 495.41 \\ 
  59 & MDE.Phi.tv & beta & beta=3 & sigma=2 & n=100 & 603.10 \\ 
  60 & MDE.Phi.kl & beta & beta=3 & sigma=2 & n=100 & 104.31 \\ 
  61 & MME & beta & beta=3 & sigma=2 & n=100 & 313324.91 \\ 
  62 & MME.b & beta & beta=3 & sigma=2 & n=100 & 2979286.01 \\ 
  63 & PWM & beta & beta=3 & sigma=2 & n=100 & 17.02 \\ 
  64 & MLE & sigma & beta=3 & sigma=2 & n=100 & 679.39 \\ 
  65 & MLE.b & sigma & beta=3 & sigma=2 & n=100 & 679.50 \\ 
  66 & LME & sigma & beta=3 & sigma=2 & n=100 & 13.06 \\ 
  67 & MDE.Phi.chisq & sigma & beta=3 & sigma=2 & n=100 & 798.08 \\ 
  68 & MDE.Phi.tv & sigma & beta=3 & sigma=2 & n=100 & 945.72 \\ 
  69 & MDE.Phi.kl & sigma & beta=3 & sigma=2 & n=100 & 77.69 \\ 
  70 & MME & sigma & beta=3 & sigma=2 & n=100 & 180960.13 \\ 
  71 & MME.b & sigma & beta=3 & sigma=2 & n=100 & 1722592.02 \\ 
  72 & PWM & sigma & beta=3 & sigma=2 & n=100 & 13.06 \\ 
  73 & MLE & beta & beta=4 & sigma=2 & n=100 & 1547.59 \\ 
  74 & MLE.b & beta & beta=4 & sigma=2 & n=100 & 1548.52 \\ 
  75 & LME & beta & beta=4 & sigma=2 & n=100 & 51.86 \\ 
  76 & MDE.Phi.chisq & beta & beta=4 & sigma=2 & n=100 & 1290.28 \\ 
  77 & MDE.Phi.tv & beta & beta=4 & sigma=2 & n=100 & 1511.41 \\ 
  78 & MDE.Phi.kl & beta & beta=4 & sigma=2 & n=100 & 212.98 \\ 
  79 & MME & beta & beta=4 & sigma=2 & n=100 & 11609.86 \\ 
  80 & MME.b & beta & beta=4 & sigma=2 & n=100 & 1922332.72 \\ 
  81 & PWM & beta & beta=4 & sigma=2 & n=100 & 51.86 \\ 
  82 & MLE & sigma & beta=4 & sigma=2 & n=100 & 583.43 \\ 
  83 & MLE.b & sigma & beta=4 & sigma=2 & n=100 & 583.75 \\ 
  84 & LME & sigma & beta=4 & sigma=2 & n=100 & 19.90 \\ 
  85 & MDE.Phi.chisq & sigma & beta=4 & sigma=2 & n=100 & 1023.38 \\ 
  86 & MDE.Phi.tv & sigma & beta=4 & sigma=2 & n=100 & 1134.64 \\ 
  87 & MDE.Phi.kl & sigma & beta=4 & sigma=2 & n=100 & 84.10 \\ 
  88 & MME & sigma & beta=4 & sigma=2 & n=100 & 4367.52 \\ 
  89 & MME.b & sigma & beta=4 & sigma=2 & n=100 & 1082722.33 \\ 
  90 & PWM & sigma & beta=4 & sigma=2 & n=100 & 19.90 \\ 
  91 & MLE & beta & beta=5 & sigma=2 & n=100 & 2747.14 \\ 
  92 & MLE.b & beta & beta=5 & sigma=2 & n=100 & 2748.57 \\ 
  93 & LME & beta & beta=5 & sigma=2 & n=100 & 101.66 \\ 
  94 & MDE.Phi.chisq & beta & beta=5 & sigma=2 & n=100 & 2092.13 \\ 
  95 & MDE.Phi.tv & beta & beta=5 & sigma=2 & n=100 & 2301.36 \\ 
  96 & MDE.Phi.kl & beta & beta=5 & sigma=2 & n=100 & 372.90 \\ 
  97 & MME & beta & beta=5 & sigma=2 & n=100 & 18723.49 \\ 
  98 & MME.b & beta & beta=5 & sigma=2 & n=100 & 259591.79 \\ 
  99 & PWM & beta & beta=5 & sigma=2 & n=100 & 101.66 \\ 
  100 & MLE & sigma & beta=5 & sigma=2 & n=100 & 617.23 \\ 
  101 & MLE.b & sigma & beta=5 & sigma=2 & n=100 & 617.53 \\ 
  102 & LME & sigma & beta=5 & sigma=2 & n=100 & 22.47 \\ 
  103 & MDE.Phi.chisq & sigma & beta=5 & sigma=2 & n=100 & 957.78 \\ 
  104 & MDE.Phi.tv & sigma & beta=5 & sigma=2 & n=100 & 1007.91 \\ 
  105 & MDE.Phi.kl & sigma & beta=5 & sigma=2 & n=100 & 82.63 \\ 
  106 & MME & sigma & beta=5 & sigma=2 & n=100 & 4176.97 \\ 
  107 & MME.b & sigma & beta=5 & sigma=2 & n=100 & 62177.40 \\ 
  108 & PWM & sigma & beta=5 & sigma=2 & n=100 & 22.47 \\ 
  109 & MLE & beta & beta=1.5 & sigma=2 & n=200 & 0.16 \\ 
  110 & MLE.b & beta & beta=1.5 & sigma=2 & n=200 & 0.09 \\ 
  111 & LME & beta & beta=1.5 & sigma=2 & n=200 & 0.15 \\ 
  112 & MDE.Phi.chisq & beta & beta=1.5 & sigma=2 & n=200 & 23.55 \\ 
  113 & MDE.Phi.tv & beta & beta=1.5 & sigma=2 & n=200 & 0.42 \\ 
  114 & MDE.Phi.kl & beta & beta=1.5 & sigma=2 & n=200 & 0.11 \\ 
  115 & MME & beta & beta=1.5 & sigma=2 & n=200 & 1.15 \\ 
  116 & MME.b & beta & beta=1.5 & sigma=2 & n=200 & 0.89 \\ 
  117 & PWM & beta & beta=1.5 & sigma=2 & n=200 & 0.15 \\ 
  118 & MLE & sigma & beta=1.5 & sigma=2 & n=200 & 0.68 \\ 
  119 & MLE.b & sigma & beta=1.5 & sigma=2 & n=200 & 0.40 \\ 
  120 & LME & sigma & beta=1.5 & sigma=2 & n=200 & 0.66 \\ 
  121 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=2 & n=200 & 3.42 \\ 
  122 & MDE.Phi.tv & sigma & beta=1.5 & sigma=2 & n=200 & 1.42 \\ 
  123 & MDE.Phi.kl & sigma & beta=1.5 & sigma=2 & n=200 & 0.46 \\ 
  124 & MME & sigma & beta=1.5 & sigma=2 & n=200 & 18.82 \\ 
  125 & MME.b & sigma & beta=1.5 & sigma=2 & n=200 & 15.56 \\ 
  126 & PWM & sigma & beta=1.5 & sigma=2 & n=200 & 0.66 \\ 
  127 & MLE & beta & beta=2 & sigma=2 & n=200 & 0.37 \\ 
  128 & MLE.b & beta & beta=2 & sigma=2 & n=200 & 0.20 \\ 
  129 & LME & beta & beta=2 & sigma=2 & n=200 & 0.35 \\ 
  130 & MDE.Phi.chisq & beta & beta=2 & sigma=2 & n=200 & 2.62 \\ 
  131 & MDE.Phi.tv & beta & beta=2 & sigma=2 & n=200 & 2.40 \\ 
  132 & MDE.Phi.kl & beta & beta=2 & sigma=2 & n=200 & 0.32 \\ 
  133 & MME & beta & beta=2 & sigma=2 & n=200 & 1.48 \\ 
  134 & MME.b & beta & beta=2 & sigma=2 & n=200 & 5.87 \\ 
  135 & PWM & beta & beta=2 & sigma=2 & n=200 & 0.35 \\ 
  136 & MLE & sigma & beta=2 & sigma=2 & n=200 & 0.73 \\ 
  137 & MLE.b & sigma & beta=2 & sigma=2 & n=200 & 0.40 \\ 
  138 & LME & sigma & beta=2 & sigma=2 & n=200 & 0.68 \\ 
  139 & MDE.Phi.chisq & sigma & beta=2 & sigma=2 & n=200 & 7.26 \\ 
  140 & MDE.Phi.tv & sigma & beta=2 & sigma=2 & n=200 & 9.45 \\ 
  141 & MDE.Phi.kl & sigma & beta=2 & sigma=2 & n=200 & 0.63 \\ 
  142 & MME & sigma & beta=2 & sigma=2 & n=200 & 4.27 \\ 
  143 & MME.b & sigma & beta=2 & sigma=2 & n=200 & 11.87 \\ 
  144 & PWM & sigma & beta=2 & sigma=2 & n=200 & 0.68 \\ 
  145 & MLE & beta & beta=2.5 & sigma=2 & n=200 & 1.52 \\ 
  146 & MLE.b & beta & beta=2.5 & sigma=2 & n=200 & 1.13 \\ 
  147 & LME & beta & beta=2.5 & sigma=2 & n=200 & 1.28 \\ 
  148 & MDE.Phi.chisq & beta & beta=2.5 & sigma=2 & n=200 & 18.08 \\ 
  149 & MDE.Phi.tv & beta & beta=2.5 & sigma=2 & n=200 & 13.86 \\ 
  150 & MDE.Phi.kl & beta & beta=2.5 & sigma=2 & n=200 & 1.18 \\ 
  151 & MME & beta & beta=2.5 & sigma=2 & n=200 & 2.90 \\ 
  152 & MME.b & beta & beta=2.5 & sigma=2 & n=200 & 44.44 \\ 
  153 & PWM & beta & beta=2.5 & sigma=2 & n=200 & 1.28 \\ 
  154 & MLE & sigma & beta=2.5 & sigma=2 & n=200 & 1.79 \\ 
  155 & MLE.b & sigma & beta=2.5 & sigma=2 & n=200 & 1.32 \\ 
  156 & LME & sigma & beta=2.5 & sigma=2 & n=200 & 1.45 \\ 
  157 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=2 & n=200 & 36.59 \\ 
  158 & MDE.Phi.tv & sigma & beta=2.5 & sigma=2 & n=200 & 27.27 \\ 
  159 & MDE.Phi.kl & sigma & beta=2.5 & sigma=2 & n=200 & 1.40 \\ 
  160 & MME & sigma & beta=2.5 & sigma=2 & n=200 & 3.84 \\ 
  161 & MME.b & sigma & beta=2.5 & sigma=2 & n=200 & 50.28 \\ 
  162 & PWM & sigma & beta=2.5 & sigma=2 & n=200 & 1.45 \\ 
  163 & MLE & beta & beta=3 & sigma=2 & n=200 & 176.07 \\ 
  164 & MLE.b & beta & beta=3 & sigma=2 & n=200 & 175.46 \\ 
  165 & LME & beta & beta=3 & sigma=2 & n=200 & 4.35 \\ 
  166 & MDE.Phi.chisq & beta & beta=3 & sigma=2 & n=200 & 89.09 \\ 
  167 & MDE.Phi.tv & beta & beta=3 & sigma=2 & n=200 & 42.73 \\ 
  168 & MDE.Phi.kl & beta & beta=3 & sigma=2 & n=200 & 7.97 \\ 
  169 & MME & beta & beta=3 & sigma=2 & n=200 & 74.99 \\ 
  170 & MME.b & beta & beta=3 & sigma=2 & n=200 & 7353.37 \\ 
  171 & PWM & beta & beta=3 & sigma=2 & n=200 & 4.35 \\ 
  172 & MLE & sigma & beta=3 & sigma=2 & n=200 & 117.01 \\ 
  173 & MLE.b & sigma & beta=3 & sigma=2 & n=200 & 116.53 \\ 
  174 & LME & sigma & beta=3 & sigma=2 & n=200 & 3.12 \\ 
  175 & MDE.Phi.chisq & sigma & beta=3 & sigma=2 & n=200 & 119.51 \\ 
  176 & MDE.Phi.tv & sigma & beta=3 & sigma=2 & n=200 & 53.42 \\ 
  177 & MDE.Phi.kl & sigma & beta=3 & sigma=2 & n=200 & 5.68 \\ 
  178 & MME & sigma & beta=3 & sigma=2 & n=200 & 49.12 \\ 
  179 & MME.b & sigma & beta=3 & sigma=2 & n=200 & 6731.37 \\ 
  180 & PWM & sigma & beta=3 & sigma=2 & n=200 & 3.12 \\ 
  181 & MLE & beta & beta=4 & sigma=2 & n=200 & 161.27 \\ 
  182 & MLE.b & beta & beta=4 & sigma=2 & n=200 & 161.05 \\ 
  183 & LME & beta & beta=4 & sigma=2 & n=200 & 18.28 \\ 
  184 & MDE.Phi.chisq & beta & beta=4 & sigma=2 & n=200 & 478.77 \\ 
  185 & MDE.Phi.tv & beta & beta=4 & sigma=2 & n=200 & 354.77 \\ 
  186 & MDE.Phi.kl & beta & beta=4 & sigma=2 & n=200 & 42.82 \\ 
  187 & MME & beta & beta=4 & sigma=2 & n=200 & 550.99 \\ 
  188 & MME.b & beta & beta=4 & sigma=2 & n=200 & 40296.90 \\ 
  189 & PWM & beta & beta=4 & sigma=2 & n=200 & 18.28 \\ 
  190 & MLE & sigma & beta=4 & sigma=2 & n=200 & 63.60 \\ 
  191 & MLE.b & sigma & beta=4 & sigma=2 & n=200 & 63.50 \\ 
  192 & LME & sigma & beta=4 & sigma=2 & n=200 & 6.86 \\ 
  193 & MDE.Phi.chisq & sigma & beta=4 & sigma=2 & n=200 & 319.57 \\ 
  194 & MDE.Phi.tv & sigma & beta=4 & sigma=2 & n=200 & 229.78 \\ 
  195 & MDE.Phi.kl & sigma & beta=4 & sigma=2 & n=200 & 16.19 \\ 
  196 & MME & sigma & beta=4 & sigma=2 & n=200 & 213.66 \\ 
  197 & MME.b & sigma & beta=4 & sigma=2 & n=200 & 19808.00 \\ 
  198 & PWM & sigma & beta=4 & sigma=2 & n=200 & 6.86 \\ 
  199 & MLE & beta & beta=5 & sigma=2 & n=200 & 10597.50 \\ 
  200 & MLE.b & beta & beta=5 & sigma=2 & n=200 & 10598.33 \\ 
  201 & LME & beta & beta=5 & sigma=2 & n=200 & 66.24 \\ 
  202 & MDE.Phi.chisq & beta & beta=5 & sigma=2 & n=200 & 1220.28 \\ 
  203 & MDE.Phi.tv & beta & beta=5 & sigma=2 & n=200 & 806.89 \\ 
  204 & MDE.Phi.kl & beta & beta=5 & sigma=2 & n=200 & 141.62 \\ 
  205 & MME & beta & beta=5 & sigma=2 & n=200 & 2746.13 \\ 
  206 & MME.b & beta & beta=5 & sigma=2 & n=200 & 30984.95 \\ 
  207 & PWM & beta & beta=5 & sigma=2 & n=200 & 66.24 \\ 
  208 & MLE & sigma & beta=5 & sigma=2 & n=200 & 2451.72 \\ 
  209 & MLE.b & sigma & beta=5 & sigma=2 & n=200 & 2451.89 \\ 
  210 & LME & sigma & beta=5 & sigma=2 & n=200 & 14.82 \\ 
  211 & MDE.Phi.chisq & sigma & beta=5 & sigma=2 & n=200 & 478.48 \\ 
  212 & MDE.Phi.tv & sigma & beta=5 & sigma=2 & n=200 & 299.43 \\ 
  213 & MDE.Phi.kl & sigma & beta=5 & sigma=2 & n=200 & 31.59 \\ 
  214 & MME & sigma & beta=5 & sigma=2 & n=200 & 597.26 \\ 
  215 & MME.b & sigma & beta=5 & sigma=2 & n=200 & 7010.66 \\ 
  216 & PWM & sigma & beta=5 & sigma=2 & n=200 & 14.82 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220203/Output.var.LaTeX.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Tue Feb 01 15:49:34 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=2 & n=100 & 0.44 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=2 & n=100 & 0.32 \\ 
  3 & LME & beta & beta=1.5 & sigma=2 & n=100 & 0.30 \\ 
  4 & MDE.Phi.chisq & beta & beta=1.5 & sigma=2 & n=100 & 97.61 \\ 
  5 & MDE.Phi.tv & beta & beta=1.5 & sigma=2 & n=100 & 6.78 \\ 
  6 & MDE.Phi.kl & beta & beta=1.5 & sigma=2 & n=100 & 0.44 \\ 
  7 & MME & beta & beta=1.5 & sigma=2 & n=100 & 0.90 \\ 
  8 & MME.b & beta & beta=1.5 & sigma=2 & n=100 & 130047.07 \\ 
  9 & PWM & beta & beta=1.5 & sigma=2 & n=100 & 0.30 \\ 
  10 & MLE & sigma & beta=1.5 & sigma=2 & n=100 & 1.96 \\ 
  11 & MLE.b & sigma & beta=1.5 & sigma=2 & n=100 & 1.45 \\ 
  12 & LME & sigma & beta=1.5 & sigma=2 & n=100 & 1.33 \\ 
  13 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=2 & n=100 & 82.05 \\ 
  14 & MDE.Phi.tv & sigma & beta=1.5 & sigma=2 & n=100 & 70.77 \\ 
  15 & MDE.Phi.kl & sigma & beta=1.5 & sigma=2 & n=100 & 1.96 \\ 
  16 & MME & sigma & beta=1.5 & sigma=2 & n=100 & 7.97 \\ 
  17 & MME.b & sigma & beta=1.5 & sigma=2 & n=100 & 595564.32 \\ 
  18 & PWM & sigma & beta=1.5 & sigma=2 & n=100 & 1.33 \\ 
  19 & MLE & beta & beta=2 & sigma=2 & n=100 & 66.06 \\ 
  20 & MLE.b & beta & beta=2 & sigma=2 & n=100 & 66.06 \\ 
  21 & LME & beta & beta=2 & sigma=2 & n=100 & 3.11 \\ 
  22 & MDE.Phi.chisq & beta & beta=2 & sigma=2 & n=100 & 65.39 \\ 
  23 & MDE.Phi.tv & beta & beta=2 & sigma=2 & n=100 & 87.28 \\ 
  24 & MDE.Phi.kl & beta & beta=2 & sigma=2 & n=100 & 12.19 \\ 
  25 & MME & beta & beta=2 & sigma=2 & n=100 & 52.88 \\ 
  26 & MME.b & beta & beta=2 & sigma=2 & n=100 & 151218.71 \\ 
  27 & PWM & beta & beta=2 & sigma=2 & n=100 & 3.11 \\ 
  28 & MLE & sigma & beta=2 & sigma=2 & n=100 & 93.66 \\ 
  29 & MLE.b & sigma & beta=2 & sigma=2 & n=100 & 93.60 \\ 
  30 & LME & sigma & beta=2 & sigma=2 & n=100 & 5.78 \\ 
  31 & MDE.Phi.chisq & sigma & beta=2 & sigma=2 & n=100 & 298.76 \\ 
  32 & MDE.Phi.tv & sigma & beta=2 & sigma=2 & n=100 & 379.09 \\ 
  33 & MDE.Phi.kl & sigma & beta=2 & sigma=2 & n=100 & 20.44 \\ 
  34 & MME & sigma & beta=2 & sigma=2 & n=100 & 91.42 \\ 
  35 & MME.b & sigma & beta=2 & sigma=2 & n=100 & 334195.41 \\ 
  36 & PWM & sigma & beta=2 & sigma=2 & n=100 & 5.78 \\ 
  37 & MLE & beta & beta=2.5 & sigma=2 & n=100 & 140.17 \\ 
  38 & MLE.b & beta & beta=2.5 & sigma=2 & n=100 & 140.83 \\ 
  39 & LME & beta & beta=2.5 & sigma=2 & n=100 & 8.34 \\ 
  40 & MDE.Phi.chisq & beta & beta=2.5 & sigma=2 & n=100 & 224.57 \\ 
  41 & MDE.Phi.tv & beta & beta=2.5 & sigma=2 & n=100 & 256.61 \\ 
  42 & MDE.Phi.kl & beta & beta=2.5 & sigma=2 & n=100 & 29.78 \\ 
  43 & MME & beta & beta=2.5 & sigma=2 & n=100 & 144.30 \\ 
  44 & MME.b & beta & beta=2.5 & sigma=2 & n=100 & 2205.73 \\ 
  45 & PWM & beta & beta=2.5 & sigma=2 & n=100 & 8.34 \\ 
  46 & MLE & sigma & beta=2.5 & sigma=2 & n=100 & 160.69 \\ 
  47 & MLE.b & sigma & beta=2.5 & sigma=2 & n=100 & 161.42 \\ 
  48 & LME & sigma & beta=2.5 & sigma=2 & n=100 & 8.99 \\ 
  49 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=2 & n=100 & 535.71 \\ 
  50 & MDE.Phi.tv & sigma & beta=2.5 & sigma=2 & n=100 & 611.37 \\ 
  51 & MDE.Phi.kl & sigma & beta=2.5 & sigma=2 & n=100 & 32.58 \\ 
  52 & MME & sigma & beta=2.5 & sigma=2 & n=100 & 150.14 \\ 
  53 & MME.b & sigma & beta=2.5 & sigma=2 & n=100 & 2520.30 \\ 
  54 & PWM & sigma & beta=2.5 & sigma=2 & n=100 & 8.99 \\ 
  55 & MLE & beta & beta=3 & sigma=2 & n=100 & 872.85 \\ 
  56 & MLE.b & beta & beta=3 & sigma=2 & n=100 & 875.53 \\ 
  57 & LME & beta & beta=3 & sigma=2 & n=100 & 15.99 \\ 
  58 & MDE.Phi.chisq & beta & beta=3 & sigma=2 & n=100 & 480.90 \\ 
  59 & MDE.Phi.tv & beta & beta=3 & sigma=2 & n=100 & 575.77 \\ 
  60 & MDE.Phi.kl & beta & beta=3 & sigma=2 & n=100 & 100.86 \\ 
  61 & MME & beta & beta=3 & sigma=2 & n=100 & 313146.34 \\ 
  62 & MME.b & beta & beta=3 & sigma=2 & n=100 & 2977375.72 \\ 
  63 & PWM & beta & beta=3 & sigma=2 & n=100 & 15.99 \\ 
  64 & MLE & sigma & beta=3 & sigma=2 & n=100 & 673.84 \\ 
  65 & MLE.b & sigma & beta=3 & sigma=2 & n=100 & 675.79 \\ 
  66 & LME & sigma & beta=3 & sigma=2 & n=100 & 12.33 \\ 
  67 & MDE.Phi.chisq & sigma & beta=3 & sigma=2 & n=100 & 759.10 \\ 
  68 & MDE.Phi.tv & sigma & beta=3 & sigma=2 & n=100 & 886.52 \\ 
  69 & MDE.Phi.kl & sigma & beta=3 & sigma=2 & n=100 & 75.13 \\ 
  70 & MME & sigma & beta=3 & sigma=2 & n=100 & 180846.34 \\ 
  71 & MME.b & sigma & beta=3 & sigma=2 & n=100 & 1721384.96 \\ 
  72 & PWM & sigma & beta=3 & sigma=2 & n=100 & 12.33 \\ 
  73 & MLE & beta & beta=4 & sigma=2 & n=100 & 1525.38 \\ 
  74 & MLE.b & beta & beta=4 & sigma=2 & n=100 & 1530.36 \\ 
  75 & LME & beta & beta=4 & sigma=2 & n=100 & 48.77 \\ 
  76 & MDE.Phi.chisq & beta & beta=4 & sigma=2 & n=100 & 1195.04 \\ 
  77 & MDE.Phi.tv & beta & beta=4 & sigma=2 & n=100 & 1368.63 \\ 
  78 & MDE.Phi.kl & beta & beta=4 & sigma=2 & n=100 & 201.29 \\ 
  79 & MME & beta & beta=4 & sigma=2 & n=100 & 11556.91 \\ 
  80 & MME.b & beta & beta=4 & sigma=2 & n=100 & 1921162.31 \\ 
  81 & PWM & beta & beta=4 & sigma=2 & n=100 & 48.77 \\ 
  82 & MLE & sigma & beta=4 & sigma=2 & n=100 & 574.92 \\ 
  83 & MLE.b & sigma & beta=4 & sigma=2 & n=100 & 576.76 \\ 
  84 & LME & sigma & beta=4 & sigma=2 & n=100 & 18.76 \\ 
  85 & MDE.Phi.chisq & sigma & beta=4 & sigma=2 & n=100 & 926.76 \\ 
  86 & MDE.Phi.tv & sigma & beta=4 & sigma=2 & n=100 & 1007.89 \\ 
  87 & MDE.Phi.kl & sigma & beta=4 & sigma=2 & n=100 & 79.61 \\ 
  88 & MME & sigma & beta=4 & sigma=2 & n=100 & 4346.18 \\ 
  89 & MME.b & sigma & beta=4 & sigma=2 & n=100 & 1082212.14 \\ 
  90 & PWM & sigma & beta=4 & sigma=2 & n=100 & 18.76 \\ 
  91 & MLE & beta & beta=5 & sigma=2 & n=100 & 2693.78 \\ 
  92 & MLE.b & beta & beta=5 & sigma=2 & n=100 & 2700.47 \\ 
  93 & LME & beta & beta=5 & sigma=2 & n=100 & 96.10 \\ 
  94 & MDE.Phi.chisq & beta & beta=5 & sigma=2 & n=100 & 1864.51 \\ 
  95 & MDE.Phi.tv & beta & beta=5 & sigma=2 & n=100 & 2004.22 \\ 
  96 & MDE.Phi.kl & beta & beta=5 & sigma=2 & n=100 & 347.29 \\ 
  97 & MME & beta & beta=5 & sigma=2 & n=100 & 18587.85 \\ 
  98 & MME.b & beta & beta=5 & sigma=2 & n=100 & 257840.15 \\ 
  99 & PWM & beta & beta=5 & sigma=2 & n=100 & 96.10 \\ 
  100 & MLE & sigma & beta=5 & sigma=2 & n=100 & 605.40 \\ 
  101 & MLE.b & sigma & beta=5 & sigma=2 & n=100 & 606.86 \\ 
  102 & LME & sigma & beta=5 & sigma=2 & n=100 & 21.26 \\ 
  103 & MDE.Phi.chisq & sigma & beta=5 & sigma=2 & n=100 & 832.80 \\ 
  104 & MDE.Phi.tv & sigma & beta=5 & sigma=2 & n=100 & 860.14 \\ 
  105 & MDE.Phi.kl & sigma & beta=5 & sigma=2 & n=100 & 76.96 \\ 
  106 & MME & sigma & beta=5 & sigma=2 & n=100 & 4147.18 \\ 
  107 & MME.b & sigma & beta=5 & sigma=2 & n=100 & 61786.34 \\ 
  108 & PWM & sigma & beta=5 & sigma=2 & n=100 & 21.26 \\ 
  109 & MLE & beta & beta=1.5 & sigma=2 & n=200 & 0.10 \\ 
  110 & MLE.b & beta & beta=1.5 & sigma=2 & n=200 & 0.08 \\ 
  111 & LME & beta & beta=1.5 & sigma=2 & n=200 & 0.11 \\ 
  112 & MDE.Phi.chisq & beta & beta=1.5 & sigma=2 & n=200 & 22.83 \\ 
  113 & MDE.Phi.tv & beta & beta=1.5 & sigma=2 & n=200 & 0.17 \\ 
  114 & MDE.Phi.kl & beta & beta=1.5 & sigma=2 & n=200 & 0.10 \\ 
  115 & MME & beta & beta=1.5 & sigma=2 & n=200 & 0.16 \\ 
  116 & MME.b & beta & beta=1.5 & sigma=2 & n=200 & 0.26 \\ 
  117 & PWM & beta & beta=1.5 & sigma=2 & n=200 & 0.11 \\ 
  118 & MLE & sigma & beta=1.5 & sigma=2 & n=200 & 0.46 \\ 
  119 & MLE.b & sigma & beta=1.5 & sigma=2 & n=200 & 0.33 \\ 
  120 & LME & sigma & beta=1.5 & sigma=2 & n=200 & 0.49 \\ 
  121 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=2 & n=200 & 3.32 \\ 
  122 & MDE.Phi.tv & sigma & beta=1.5 & sigma=2 & n=200 & 1.16 \\ 
  123 & MDE.Phi.kl & sigma & beta=1.5 & sigma=2 & n=200 & 0.43 \\ 
  124 & MME & sigma & beta=1.5 & sigma=2 & n=200 & 6.07 \\ 
  125 & MME.b & sigma & beta=1.5 & sigma=2 & n=200 & 6.44 \\ 
  126 & PWM & sigma & beta=1.5 & sigma=2 & n=200 & 0.49 \\ 
  127 & MLE & beta & beta=2 & sigma=2 & n=200 & 0.31 \\ 
  128 & MLE.b & beta & beta=2 & sigma=2 & n=200 & 0.20 \\ 
  129 & LME & beta & beta=2 & sigma=2 & n=200 & 0.30 \\ 
  130 & MDE.Phi.chisq & beta & beta=2 & sigma=2 & n=200 & 2.19 \\ 
  131 & MDE.Phi.tv & beta & beta=2 & sigma=2 & n=200 & 2.21 \\ 
  132 & MDE.Phi.kl & beta & beta=2 & sigma=2 & n=200 & 0.30 \\ 
  133 & MME & beta & beta=2 & sigma=2 & n=200 & 0.53 \\ 
  134 & MME.b & beta & beta=2 & sigma=2 & n=200 & 5.40 \\ 
  135 & PWM & beta & beta=2 & sigma=2 & n=200 & 0.30 \\ 
  136 & MLE & sigma & beta=2 & sigma=2 & n=200 & 0.61 \\ 
  137 & MLE.b & sigma & beta=2 & sigma=2 & n=200 & 0.39 \\ 
  138 & LME & sigma & beta=2 & sigma=2 & n=200 & 0.60 \\ 
  139 & MDE.Phi.chisq & sigma & beta=2 & sigma=2 & n=200 & 7.14 \\ 
  140 & MDE.Phi.tv & sigma & beta=2 & sigma=2 & n=200 & 9.14 \\ 
  141 & MDE.Phi.kl & sigma & beta=2 & sigma=2 & n=200 & 0.59 \\ 
  142 & MME & sigma & beta=2 & sigma=2 & n=200 & 1.11 \\ 
  143 & MME.b & sigma & beta=2 & sigma=2 & n=200 & 10.20 \\ 
  144 & PWM & sigma & beta=2 & sigma=2 & n=200 & 0.60 \\ 
  145 & MLE & beta & beta=2.5 & sigma=2 & n=200 & 1.41 \\ 
  146 & MLE.b & beta & beta=2.5 & sigma=2 & n=200 & 1.13 \\ 
  147 & LME & beta & beta=2.5 & sigma=2 & n=200 & 1.20 \\ 
  148 & MDE.Phi.chisq & beta & beta=2.5 & sigma=2 & n=200 & 17.88 \\ 
  149 & MDE.Phi.tv & beta & beta=2.5 & sigma=2 & n=200 & 13.81 \\ 
  150 & MDE.Phi.kl & beta & beta=2.5 & sigma=2 & n=200 & 1.12 \\ 
  151 & MME & beta & beta=2.5 & sigma=2 & n=200 & 1.77 \\ 
  152 & MME.b & beta & beta=2.5 & sigma=2 & n=200 & 43.75 \\ 
  153 & PWM & beta & beta=2.5 & sigma=2 & n=200 & 1.20 \\ 
  154 & MLE & sigma & beta=2.5 & sigma=2 & n=200 & 1.66 \\ 
  155 & MLE.b & sigma & beta=2.5 & sigma=2 & n=200 & 1.32 \\ 
  156 & LME & sigma & beta=2.5 & sigma=2 & n=200 & 1.36 \\ 
  157 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=2 & n=200 & 36.10 \\ 
  158 & MDE.Phi.tv & sigma & beta=2.5 & sigma=2 & n=200 & 26.62 \\ 
  159 & MDE.Phi.kl & sigma & beta=2.5 & sigma=2 & n=200 & 1.33 \\ 
  160 & MME & sigma & beta=2.5 & sigma=2 & n=200 & 2.13 \\ 
  161 & MME.b & sigma & beta=2.5 & sigma=2 & n=200 & 49.26 \\ 
  162 & PWM & sigma & beta=2.5 & sigma=2 & n=200 & 1.36 \\ 
  163 & MLE & beta & beta=3 & sigma=2 & n=200 & 175.57 \\ 
  164 & MLE.b & beta & beta=3 & sigma=2 & n=200 & 175.42 \\ 
  165 & LME & beta & beta=3 & sigma=2 & n=200 & 4.14 \\ 
  166 & MDE.Phi.chisq & beta & beta=3 & sigma=2 & n=200 & 89.01 \\ 
  167 & MDE.Phi.tv & beta & beta=3 & sigma=2 & n=200 & 42.69 \\ 
  168 & MDE.Phi.kl & beta & beta=3 & sigma=2 & n=200 & 7.73 \\ 
  169 & MME & beta & beta=3 & sigma=2 & n=200 & 73.03 \\ 
  170 & MME.b & beta & beta=3 & sigma=2 & n=200 & 7346.85 \\ 
  171 & PWM & beta & beta=3 & sigma=2 & n=200 & 4.14 \\ 
  172 & MLE & sigma & beta=3 & sigma=2 & n=200 & 116.64 \\ 
  173 & MLE.b & sigma & beta=3 & sigma=2 & n=200 & 116.50 \\ 
  174 & LME & sigma & beta=3 & sigma=2 & n=200 & 2.98 \\ 
  175 & MDE.Phi.chisq & sigma & beta=3 & sigma=2 & n=200 & 117.14 \\ 
  176 & MDE.Phi.tv & sigma & beta=3 & sigma=2 & n=200 & 52.01 \\ 
  177 & MDE.Phi.kl & sigma & beta=3 & sigma=2 & n=200 & 5.50 \\ 
  178 & MME & sigma & beta=3 & sigma=2 & n=200 & 47.45 \\ 
  179 & MME.b & sigma & beta=3 & sigma=2 & n=200 & 6725.97 \\ 
  180 & PWM & sigma & beta=3 & sigma=2 & n=200 & 2.98 \\ 
  181 & MLE & beta & beta=4 & sigma=2 & n=200 & 158.85 \\ 
  182 & MLE.b & beta & beta=4 & sigma=2 & n=200 & 160.30 \\ 
  183 & LME & beta & beta=4 & sigma=2 & n=200 & 17.45 \\ 
  184 & MDE.Phi.chisq & beta & beta=4 & sigma=2 & n=200 & 465.08 \\ 
  185 & MDE.Phi.tv & beta & beta=4 & sigma=2 & n=200 & 346.11 \\ 
  186 & MDE.Phi.kl & beta & beta=4 & sigma=2 & n=200 & 41.24 \\ 
  187 & MME & beta & beta=4 & sigma=2 & n=200 & 544.09 \\ 
  188 & MME.b & beta & beta=4 & sigma=2 & n=200 & 40207.12 \\ 
  189 & PWM & beta & beta=4 & sigma=2 & n=200 & 17.45 \\ 
  190 & MLE & sigma & beta=4 & sigma=2 & n=200 & 62.64 \\ 
  191 & MLE.b & sigma & beta=4 & sigma=2 & n=200 & 63.19 \\ 
  192 & LME & sigma & beta=4 & sigma=2 & n=200 & 6.55 \\ 
  193 & MDE.Phi.chisq & sigma & beta=4 & sigma=2 & n=200 & 303.58 \\ 
  194 & MDE.Phi.tv & sigma & beta=4 & sigma=2 & n=200 & 220.00 \\ 
  195 & MDE.Phi.kl & sigma & beta=4 & sigma=2 & n=200 & 15.59 \\ 
  196 & MME & sigma & beta=4 & sigma=2 & n=200 & 210.92 \\ 
  197 & MME.b & sigma & beta=4 & sigma=2 & n=200 & 19770.86 \\ 
  198 & PWM & sigma & beta=4 & sigma=2 & n=200 & 6.55 \\ 
  199 & MLE & beta & beta=5 & sigma=2 & n=200 & 10574.34 \\ 
  200 & MLE.b & beta & beta=5 & sigma=2 & n=200 & 10581.67 \\ 
  201 & LME & beta & beta=5 & sigma=2 & n=200 & 63.08 \\ 
  202 & MDE.Phi.chisq & beta & beta=5 & sigma=2 & n=200 & 1137.09 \\ 
  203 & MDE.Phi.tv & beta & beta=5 & sigma=2 & n=200 & 766.54 \\ 
  204 & MDE.Phi.kl & beta & beta=5 & sigma=2 & n=200 & 134.88 \\ 
  205 & MME & beta & beta=5 & sigma=2 & n=200 & 2723.73 \\ 
  206 & MME.b & beta & beta=5 & sigma=2 & n=200 & 30712.87 \\ 
  207 & PWM & beta & beta=5 & sigma=2 & n=200 & 63.08 \\ 
  208 & MLE & sigma & beta=5 & sigma=2 & n=200 & 2446.31 \\ 
  209 & MLE.b & sigma & beta=5 & sigma=2 & n=200 & 2447.97 \\ 
  210 & LME & sigma & beta=5 & sigma=2 & n=200 & 14.12 \\ 
  211 & MDE.Phi.chisq & sigma & beta=5 & sigma=2 & n=200 & 435.77 \\ 
  212 & MDE.Phi.tv & sigma & beta=5 & sigma=2 & n=200 & 279.11 \\ 
  213 & MDE.Phi.kl & sigma & beta=5 & sigma=2 & n=200 & 30.09 \\ 
  214 & MME & sigma & beta=5 & sigma=2 & n=200 & 592.18 \\ 
  215 & MME.b & sigma & beta=5 & sigma=2 & n=200 & 6949.35 \\ 
  216 & PWM & sigma & beta=5 & sigma=2 & n=200 & 14.12 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220204/Full.beta=1.5.sig=3.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=1.5,  \sigma=3$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.6717&1.4777&1.8288&-1.8659&1.2349&1.6717&2.7927&6.3149&1.8288
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
3.5467&2.9322&3.976&5.2184&5.488&3.5467&9.4574&20.5029&3.976
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.435&0.3213&0.2958&347.7844&6.2223&0.4353&0.8967&130047.0665&0.2958
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
4.4042&3.2523&2.9924&173.3936&144.6706&4.4068&17.9315&1340019.7055&2.9924
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1717&-0.0223&0.3288&-3.3659&-0.2651&0.1717&1.2927&4.8149&0.3288
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.5467&-0.0678&0.976&2.2184&2.488&0.5467&6.4574&17.5029&0.976
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.4644&0.3217&0.4039&359.079&6.292&0.4647&2.5678&130057.2449&0.4039
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
4.7026&3.2566&3.9447&178.2978&150.8462&4.7053&59.6278&1340192.0551&3.9447
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 5.167&3.5783&4.3485&537.3768&157.1382&5.17&62.1955&1470249.3&4.3485\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0011&0.0011&2.9905720362169e+301&0.0459&0.0011&0.0099&7.105&0.0011\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220204/Full.beta=1.5.sig=3.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=1.5,  \sigma=3$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.7307&1.63&1.7058&0.1828&0.9983&1.5786&2.4958&2.2963&1.7058
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
3.718&3.3972&3.6086&3.6521&3.7774&3.2459&8.3565&7.529&3.6086
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1036&0.0761&0.112&70.3221&0.1791&0.1016&0.1649&0.2558&0.112
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.0264&0.7443&1.113&12.7062&2.5972&0.9744&13.6369&14.4779&1.113
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.2307&0.13&0.2058&-1.3172&-0.5017&0.0786&0.9958&0.7963&0.2058
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.718&0.3972&0.6086&0.6521&0.7774&0.2459&5.3565&4.529&0.6086
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1567&0.093&0.1543&72.0501&0.4308&0.1078&1.1565&0.8899&0.1543
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.5418&0.902&1.4833&13.1301&3.2014&1.0347&42.3274&34.9885&1.4833
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 1.6986&0.995&1.6376&85.1802&3.6321&1.1425&43.4839&35.8784&1.6376\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 6e-04&6e-04&6e-04&9.83790728945794e+300&0.0309&6e-04&0.0089&0.0103&6e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220204/Full.beta=2.5.sig=3.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2.5,  \sigma=3$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 3.5586&3.1014&3.1958&4.0175&4.8287&3.4298&4.8214&7.9937&3.1958
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
4.7041&3.9609&4.0776&9.0167&10.566&4.4977&7.0633&12.0647&4.0776
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 107.9591&108.5927&8.3445&201.5068&230.7047&27.8278&144.3027&2205.727&8.3445
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
276.9014&278.4705&20.2358&1089.1693&1237.7166&68.5196&337.8156&5670.6747&20.2358
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.0586&0.6014&0.6958&1.5175&2.3287&0.9298&2.3214&5.4937&0.6958
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.7041&0.9609&1.0776&6.0167&7.566&1.4977&4.0633&9.0647&1.0776
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 109.0689&108.9435&8.8279&203.7893&236.1046&28.6896&149.6771&2235.6866&8.8279
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
279.7778&279.3659&21.395&1125.2616&1294.8367&70.7557&354.2926&5752.2769&21.395
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 388.8467&388.3094&30.2229&1329.0509&1530.9413&99.4453&503.9697&7987.9635&30.2229\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0012&0.0011&0.0234&0.0179&0.0011&0.0019&8.078&0.0011\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220204/Full.beta=2.5.sig=3.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2.5,  \sigma=3$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.8442&2.5199&2.784&2.0424&2.2722&2.7519&3.5622&3.3354&2.784
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
3.5565&3.0289&3.4341&4.0362&4.2035&3.4071&4.9641&4.5203&3.4341
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.4068&1.1262&1.1974&15.987&12.5394&1.1169&1.7744&43.7481&1.1974
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
3.7288&2.9703&3.0677&72.6552&54.464&2.985&4.7924&110.8394&3.0677
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.3442&0.0199&0.284&-0.4576&-0.2278&0.2519&1.0622&0.8354&0.284
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.5565&0.0289&0.4341&1.0362&1.2035&0.4071&1.9641&1.5203&0.4341
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.5251&1.1264&1.278&16.1948&12.5901&1.1802&2.9024&44.4416&1.278
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
4.0381&2.9709&3.2558&73.7217&55.907&3.1505&8.6494&113.1395&3.2558
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 5.5633&4.0973&4.5338&89.9165&68.497&4.3307&11.5518&157.5811&4.5338\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&5e-04&5e-04&0.0174&0.0121&5e-04&0.0011&0.0017&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220204/Full.beta=2.sig=3.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2,  \sigma=3$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.5229&2.1732&2.4461&2.0099&2.6563&2.4547&3.6775&9.4751&2.4461
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
4.0876&3.3298&3.9049&6.227&7.7111&3.9647&7.312&19.7596&3.9049
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 50.2397&50.2304&3.1121&65.3242&78.4711&11.3227&52.8831&151218.7131&3.1121
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
162.8935&162.7118&13.005&604.2028&766.9694&42.7687&205.6852&751939.6683&13.005
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.5229&0.1732&0.4461&0.0099&0.6563&0.4547&1.6775&7.4751&0.4461
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.0876&0.3298&0.9049&3.227&4.7111&0.9647&4.312&16.7596&0.9049
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 50.5081&50.2554&3.3109&65.3177&78.894&11.5283&55.6919&151259.4685&3.3109
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
164.0601&162.8043&13.8227&614.5561&789.0876&43.6951&224.2577&752145.3587&13.8227
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 214.5682&213.0597&17.1335&679.8738&867.9815&55.2234&279.9497&903404.8272&17.1335\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0011&0.0011&2.00401541349742e+299&0.0234&0.0011&0.0035&0.0115&0.0011\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220204/Full.beta=2.sig=3.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2,  \sigma=3$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.2512&2.0631&2.2155&1.3244&1.5621&2.1371&2.9719&2.6875&2.2155
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
3.5287&3.1235&3.4254&3.5195&3.8315&3.289&5.6652&4.9393&3.4254
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.3049&0.2006&0.3033&4.286&2.0349&0.2964&0.5313&5.3982&0.3033
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.3651&0.8875&1.3479&14.8622&18.7607&1.3225&2.4965&22.9529&1.3479
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.2512&0.0631&0.2155&-0.6756&-0.4379&0.1371&0.9719&0.6875&0.2155
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.5287&0.1235&0.4254&0.5195&0.8315&0.289&2.6652&1.9393&0.4254
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.368&0.2046&0.3497&4.742&2.2264&0.3151&1.4758&5.8704&0.3497
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.6446&0.9027&1.5288&15.1305&19.4502&1.4058&9.5997&26.7113&1.5288
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 2.0126&1.1072&1.8785&19.8726&21.6766&1.721&11.0756&32.5817&1.8785\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 6e-04&5e-04&5e-04&3.22760432783316e+298&0.0166&5e-04&0.0024&0.0024&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220204/Full.beta=3.sig=3.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=3,  \sigma=3$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 5.5962&5.1021&4.0159&6.617&7.9612&4.8283&17.4875&49.9897&4.0159
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
6.3536&5.7131&4.2766&11.9928&14.0518&5.3637&20.2254&58.7064&4.2766
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 677.8707&680.396&15.9909&428.3696&508.6058&92.1956&313146.3373&2977375.6111&15.9909
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1161.8209&1165.9628&27.7502&1517.48&1763.6669&154.9947&406904.261&3873116.014&27.7502
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.5962&2.1021&1.0159&3.617&4.9612&1.8283&14.4875&46.9897&1.0159
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
3.3536&2.7131&1.2766&8.9928&11.0518&2.3637&17.2254&55.7064&1.2766
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 684.5434&684.7467&17.0213&441.4096&533.1686&95.5289&313324.9101&2979285.9022&17.0213
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1172.9512&1173.2073&29.3771&1598.1991&1885.633&160.5662&407160.2857&3875831.9031&29.3771
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 1857.4946&1857.954&46.3984&2039.6087&2418.8016&256.0951&720485.1958&6855117.8054&46.3984\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0012&0.0011&0.02&0.0151&0.0011&0.0014&0.0075&0.0011\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220204/Full.beta=3.sig=3.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=3,  \sigma=3$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 3.7153&3.2326&3.4534&3.2673&3.1906&3.4913&4.4029&5.6932&3.4534
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
3.9273&3.298&3.5675&5.2489&4.7619&3.6371&4.9384&6.6949&3.5675
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 175.5731&175.4234&4.1436&79.1389&38.5027&7.4645&73.0294&7346.8516&4.1436
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
262.4301&262.1231&6.6999&234.3241&105.5015&11.9975&106.7695&15133.4347&6.6999
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.7153&0.2326&0.4534&0.2673&0.1906&0.4913&1.4029&2.6932&0.4534
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.9273&0.298&0.5675&2.2489&1.7619&0.6371&1.9384&3.6949&0.5675
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 176.0671&175.46&4.3487&79.2024&38.5351&7.7052&74.9902&7353.3704&4.3487
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
263.2636&262.1857&7.0213&239.3581&108.5952&12.4021&110.5163&15145.5737&7.0213
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 439.3307&437.6457&11.3701&318.5604&147.1303&20.1073&185.5064&22498.9441&11.3701\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&5e-04&5e-04&0.0143&0.0096&5e-04&7e-04&0.0018&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220204/Full.beta=4.sig=3.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=4,  \sigma=3$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 8.5662&8.1167&5.7439&13.1726&15.2643&7.3722&11.3526&40.9056&5.7439
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
7.235&6.826&4.594&16.9728&19.0218&6.1367&9.9959&40.2968&4.594
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1294.7943&1299.6285&46.4798&1047.1043&1197.4337&187.367&11556.8269&1921162.0988&46.4798
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1086.9726&1091.0031&40.891&1826.9501&1987.6973&166.4248&9778.8741&2434977.1101&40.891
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 4.5662&4.1167&1.7439&9.1726&11.2643&3.3722&7.3526&36.9056&1.7439
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
4.235&3.826&1.594&13.9728&16.0218&3.1367&6.9959&37.2968&1.594
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1315.5149&1316.4455&49.5164&1131.1369&1324.1976&198.7199&11609.7317&1922332.0076&49.5164
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1104.7991&1105.5326&43.4277&2022.0065&2244.1963&176.2473&9826.8391&2436124.6612&43.4277
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 2420.314&2421.9781&92.9441&3153.1434&3568.3939&374.9672&21436.5708&4358456.6688&92.9441\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0012&0.001&0.0165&0.0123&0.0011&0.0011&4041.9544&0.001\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220204/Full.beta=4.sig=3.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=4,  \sigma=3$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 5.5599&4.8766&4.9153&7.4836&6.8028&5.2485&6.6383&13.686&4.9153
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
4.4747&3.8444&3.83&8.7342&7.5207&4.1543&5.4936&12.3829&3.83
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 158.832&160.2805&17.4518&406.8515&306.737&38.6007&544.0967&40207.1077&17.4518
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
140.9278&142.154&14.7413&597.7916&438.3287&32.9084&474.5803&44484.4247&14.7413
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.5599&0.8766&0.9153&3.4836&2.8028&1.2485&2.6383&9.686&0.9153
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.4747&0.8444&0.83&5.7342&4.5207&1.1543&2.4936&9.3829&0.83
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 161.2495&161.0329&18.2878&418.9461&314.562&40.1556&551.0031&40296.9063&18.2878
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
143.0885&142.8528&15.4287&630.6127&458.7218&34.2375&480.751&44568.0157&15.4287
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 304.338&303.8857&33.7166&1049.5588&773.2838&74.3932&1031.7541&84864.922&33.7166\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&6e-04&5e-04&0.0111&0.0074&5e-04&6e-04&0.0029&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220204/Full.beta=5.sig=3.n=100.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=5,  \sigma=3$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 12.1322&11.7636&7.3006&19.1382&21.1952&9.9529&16.7085&47.1193&7.3006
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
8.0345&7.7775&4.612&18.8325&20.2195&6.4976&11.2323&32.8693&4.612
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2400.466&2407.0166&87.3263&1624.2501&1742.1592&319.0036&18586.5629&257834.8442&87.3263
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1208.854&1212.0576&44.0403&1635.5487&1683.5124&159.4715&9330.5751&139016.8681&44.0403
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 7.1322&6.7636&2.3006&14.1382&16.1952&4.9529&11.7085&42.1193&2.3006
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
5.0345&4.7775&1.612&15.8325&17.2195&3.4976&8.2323&29.8693&1.612
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2451.0939&2452.5221&92.6105&1823.977&2004.2705&343.5029&18721.7941&259583.0957&92.6105
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1234.0788&1234.7608&46.6346&1886.0545&1979.8559&171.6886&9397.4128&139895.1389&46.6346
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 3685.1727&3687.2829&139.2451&3710.0314&3984.1265&515.1915&28119.2069&399478.2346&139.2451\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.001&0.0012&0.001&0.0144&0.0106&0.001&0.001&5.1562081310583e+29&0.001\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220204/Full.beta=5.sig=3.n=200.LaTeX.tex <==

      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=5,  \sigma=3$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 9.0465&8.3356&6.7653&13.5709&11.0065&7.555&9.766&21.612&6.7653
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
5.9409&5.4356&4.2398&12.2902&9.447&4.8087&6.4025&14.8283&4.2398
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2973.6531&2979.7388&60.6859&990.7491&670.8996&123.7823&2723.6789&30716.4258&60.6859
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1595.9447&1599.0409&30.8252&853.3593&548.9097&62.3844&1332.3982&15637.6016&30.8252
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 4.0465&3.3356&1.7653&8.5709&6.0065&2.555&4.766&16.612&1.7653
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2.9409&2.4356&1.2398&9.2902&6.447&1.8087&3.4025&11.8283&1.2398
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2989.73&2990.567&63.7962&1064.1106&706.9112&130.2977&2746.1214&30989.3115&63.7962
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1604.4341&1604.8131&32.3591&939.5812&590.4183&65.6497&1343.8421&15775.946&32.3591
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 4594.1641&4595.3802&96.1554&2003.6918&1297.3295&195.9474&4089.9635&46765.2574&96.1554\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&6e-04&5e-04&0.0096&0.0062&5e-04&5e-04&2.018&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220204/Output.accuracy.LaTeX.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Tue Feb 01 16:33:07 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & Measure & beta=1.5 & sigma=3 & n=100 & 5.17 \\ 
  2 & MLE.b & Measure & beta=1.5 & sigma=3 & n=100 & 3.58 \\ 
  3 & LME & Measure & beta=1.5 & sigma=3 & n=100 & 4.35 \\ 
  4 & MDE.Phi.chisq & Measure & beta=1.5 & sigma=3 & n=100 & 537.38 \\ 
  5 & MDE.Phi.tv & Measure & beta=1.5 & sigma=3 & n=100 & 157.14 \\ 
  6 & MDE.Phi.kl & Measure & beta=1.5 & sigma=3 & n=100 & 5.17 \\ 
  7 & MME & Measure & beta=1.5 & sigma=3 & n=100 & 62.20 \\ 
  8 & MME.b & Measure & beta=1.5 & sigma=3 & n=100 & 1470249.30 \\ 
  9 & PWM & Measure & beta=1.5 & sigma=3 & n=100 & 4.35 \\ 
  10 & MLE & Measure & beta=2 & sigma=3 & n=100 & 214.57 \\ 
  11 & MLE.b & Measure & beta=2 & sigma=3 & n=100 & 213.06 \\ 
  12 & LME & Measure & beta=2 & sigma=3 & n=100 & 17.13 \\ 
  13 & MDE.Phi.chisq & Measure & beta=2 & sigma=3 & n=100 & 679.87 \\ 
  14 & MDE.Phi.tv & Measure & beta=2 & sigma=3 & n=100 & 867.98 \\ 
  15 & MDE.Phi.kl & Measure & beta=2 & sigma=3 & n=100 & 55.22 \\ 
  16 & MME & Measure & beta=2 & sigma=3 & n=100 & 279.95 \\ 
  17 & MME.b & Measure & beta=2 & sigma=3 & n=100 & 903404.83 \\ 
  18 & PWM & Measure & beta=2 & sigma=3 & n=100 & 17.13 \\ 
  19 & MLE & Measure & beta=2.5 & sigma=3 & n=100 & 388.85 \\ 
  20 & MLE.b & Measure & beta=2.5 & sigma=3 & n=100 & 388.31 \\ 
  21 & LME & Measure & beta=2.5 & sigma=3 & n=100 & 30.22 \\ 
  22 & MDE.Phi.chisq & Measure & beta=2.5 & sigma=3 & n=100 & 1329.05 \\ 
  23 & MDE.Phi.tv & Measure & beta=2.5 & sigma=3 & n=100 & 1530.94 \\ 
  24 & MDE.Phi.kl & Measure & beta=2.5 & sigma=3 & n=100 & 99.45 \\ 
  25 & MME & Measure & beta=2.5 & sigma=3 & n=100 & 503.97 \\ 
  26 & MME.b & Measure & beta=2.5 & sigma=3 & n=100 & 7987.96 \\ 
  27 & PWM & Measure & beta=2.5 & sigma=3 & n=100 & 30.22 \\ 
  28 & MLE & Measure & beta=3 & sigma=3 & n=100 & 1857.49 \\ 
  29 & MLE.b & Measure & beta=3 & sigma=3 & n=100 & 1857.95 \\ 
  30 & LME & Measure & beta=3 & sigma=3 & n=100 & 46.40 \\ 
  31 & MDE.Phi.chisq & Measure & beta=3 & sigma=3 & n=100 & 2039.61 \\ 
  32 & MDE.Phi.tv & Measure & beta=3 & sigma=3 & n=100 & 2418.80 \\ 
  33 & MDE.Phi.kl & Measure & beta=3 & sigma=3 & n=100 & 256.10 \\ 
  34 & MME & Measure & beta=3 & sigma=3 & n=100 & 720485.20 \\ 
  35 & MME.b & Measure & beta=3 & sigma=3 & n=100 & 6855117.81 \\ 
  36 & PWM & Measure & beta=3 & sigma=3 & n=100 & 46.40 \\ 
  37 & MLE & Measure & beta=4 & sigma=3 & n=100 & 2420.31 \\ 
  38 & MLE.b & Measure & beta=4 & sigma=3 & n=100 & 2421.98 \\ 
  39 & LME & Measure & beta=4 & sigma=3 & n=100 & 92.94 \\ 
  40 & MDE.Phi.chisq & Measure & beta=4 & sigma=3 & n=100 & 3153.14 \\ 
  41 & MDE.Phi.tv & Measure & beta=4 & sigma=3 & n=100 & 3568.39 \\ 
  42 & MDE.Phi.kl & Measure & beta=4 & sigma=3 & n=100 & 374.97 \\ 
  43 & MME & Measure & beta=4 & sigma=3 & n=100 & 21436.57 \\ 
  44 & MME.b & Measure & beta=4 & sigma=3 & n=100 & 4358456.67 \\ 
  45 & PWM & Measure & beta=4 & sigma=3 & n=100 & 92.94 \\ 
  46 & MLE & Measure & beta=5 & sigma=3 & n=100 & 3685.17 \\ 
  47 & MLE.b & Measure & beta=5 & sigma=3 & n=100 & 3687.28 \\ 
  48 & LME & Measure & beta=5 & sigma=3 & n=100 & 139.25 \\ 
  49 & MDE.Phi.chisq & Measure & beta=5 & sigma=3 & n=100 & 3710.03 \\ 
  50 & MDE.Phi.tv & Measure & beta=5 & sigma=3 & n=100 & 3984.13 \\ 
  51 & MDE.Phi.kl & Measure & beta=5 & sigma=3 & n=100 & 515.19 \\ 
  52 & MME & Measure & beta=5 & sigma=3 & n=100 & 28119.21 \\ 
  53 & MME.b & Measure & beta=5 & sigma=3 & n=100 & 399478.23 \\ 
  54 & PWM & Measure & beta=5 & sigma=3 & n=100 & 139.25 \\ 
  55 & MLE & Measure & beta=1.5 & sigma=3 & n=200 & 1.70 \\ 
  56 & MLE.b & Measure & beta=1.5 & sigma=3 & n=200 & 0.99 \\ 
  57 & LME & Measure & beta=1.5 & sigma=3 & n=200 & 1.64 \\ 
  58 & MDE.Phi.chisq & Measure & beta=1.5 & sigma=3 & n=200 & 85.18 \\ 
  59 & MDE.Phi.tv & Measure & beta=1.5 & sigma=3 & n=200 & 3.63 \\ 
  60 & MDE.Phi.kl & Measure & beta=1.5 & sigma=3 & n=200 & 1.14 \\ 
  61 & MME & Measure & beta=1.5 & sigma=3 & n=200 & 43.48 \\ 
  62 & MME.b & Measure & beta=1.5 & sigma=3 & n=200 & 35.88 \\ 
  63 & PWM & Measure & beta=1.5 & sigma=3 & n=200 & 1.64 \\ 
  64 & MLE & Measure & beta=2 & sigma=3 & n=200 & 2.01 \\ 
  65 & MLE.b & Measure & beta=2 & sigma=3 & n=200 & 1.11 \\ 
  66 & LME & Measure & beta=2 & sigma=3 & n=200 & 1.88 \\ 
  67 & MDE.Phi.chisq & Measure & beta=2 & sigma=3 & n=200 & 19.87 \\ 
  68 & MDE.Phi.tv & Measure & beta=2 & sigma=3 & n=200 & 21.68 \\ 
  69 & MDE.Phi.kl & Measure & beta=2 & sigma=3 & n=200 & 1.72 \\ 
  70 & MME & Measure & beta=2 & sigma=3 & n=200 & 11.08 \\ 
  71 & MME.b & Measure & beta=2 & sigma=3 & n=200 & 32.58 \\ 
  72 & PWM & Measure & beta=2 & sigma=3 & n=200 & 1.88 \\ 
  73 & MLE & Measure & beta=2.5 & sigma=3 & n=200 & 5.56 \\ 
  74 & MLE.b & Measure & beta=2.5 & sigma=3 & n=200 & 4.10 \\ 
  75 & LME & Measure & beta=2.5 & sigma=3 & n=200 & 4.53 \\ 
  76 & MDE.Phi.chisq & Measure & beta=2.5 & sigma=3 & n=200 & 89.92 \\ 
  77 & MDE.Phi.tv & Measure & beta=2.5 & sigma=3 & n=200 & 68.50 \\ 
  78 & MDE.Phi.kl & Measure & beta=2.5 & sigma=3 & n=200 & 4.33 \\ 
  79 & MME & Measure & beta=2.5 & sigma=3 & n=200 & 11.55 \\ 
  80 & MME.b & Measure & beta=2.5 & sigma=3 & n=200 & 157.58 \\ 
  81 & PWM & Measure & beta=2.5 & sigma=3 & n=200 & 4.53 \\ 
  82 & MLE & Measure & beta=3 & sigma=3 & n=200 & 439.33 \\ 
  83 & MLE.b & Measure & beta=3 & sigma=3 & n=200 & 437.65 \\ 
  84 & LME & Measure & beta=3 & sigma=3 & n=200 & 11.37 \\ 
  85 & MDE.Phi.chisq & Measure & beta=3 & sigma=3 & n=200 & 318.56 \\ 
  86 & MDE.Phi.tv & Measure & beta=3 & sigma=3 & n=200 & 147.13 \\ 
  87 & MDE.Phi.kl & Measure & beta=3 & sigma=3 & n=200 & 20.11 \\ 
  88 & MME & Measure & beta=3 & sigma=3 & n=200 & 185.51 \\ 
  89 & MME.b & Measure & beta=3 & sigma=3 & n=200 & 22498.94 \\ 
  90 & PWM & Measure & beta=3 & sigma=3 & n=200 & 11.37 \\ 
  91 & MLE & Measure & beta=4 & sigma=3 & n=200 & 304.34 \\ 
  92 & MLE.b & Measure & beta=4 & sigma=3 & n=200 & 303.89 \\ 
  93 & LME & Measure & beta=4 & sigma=3 & n=200 & 33.72 \\ 
  94 & MDE.Phi.chisq & Measure & beta=4 & sigma=3 & n=200 & 1049.56 \\ 
  95 & MDE.Phi.tv & Measure & beta=4 & sigma=3 & n=200 & 773.28 \\ 
  96 & MDE.Phi.kl & Measure & beta=4 & sigma=3 & n=200 & 74.39 \\ 
  97 & MME & Measure & beta=4 & sigma=3 & n=200 & 1031.75 \\ 
  98 & MME.b & Measure & beta=4 & sigma=3 & n=200 & 84864.92 \\ 
  99 & PWM & Measure & beta=4 & sigma=3 & n=200 & 33.72 \\ 
  100 & MLE & Measure & beta=5 & sigma=3 & n=200 & 4594.16 \\ 
  101 & MLE.b & Measure & beta=5 & sigma=3 & n=200 & 4595.38 \\ 
  102 & LME & Measure & beta=5 & sigma=3 & n=200 & 96.16 \\ 
  103 & MDE.Phi.chisq & Measure & beta=5 & sigma=3 & n=200 & 2003.69 \\ 
  104 & MDE.Phi.tv & Measure & beta=5 & sigma=3 & n=200 & 1297.33 \\ 
  105 & MDE.Phi.kl & Measure & beta=5 & sigma=3 & n=200 & 195.95 \\ 
  106 & MME & Measure & beta=5 & sigma=3 & n=200 & 4089.96 \\ 
  107 & MME.b & Measure & beta=5 & sigma=3 & n=200 & 46765.26 \\ 
  108 & PWM & Measure & beta=5 & sigma=3 & n=200 & 96.16 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220204/Output.accuracy2.LaTeX.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Tue Feb 01 16:33:07 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & Measure & beta=1.5 & sigma=3 & n=100 & 0.00 \\ 
  2 & MLE.b & Measure & beta=1.5 & sigma=3 & n=100 & 0.00 \\ 
  3 & LME & Measure & beta=1.5 & sigma=3 & n=100 & 0.00 \\ 
  4 & MDE.Phi.chisq & Measure & beta=1.5 & sigma=3 & n=100 & 29905720362168969996808464202462800682084228428422286624866604884622022480262860460682862862686226040624222482222048606602484402222646462462484864666660068682042200040840686000648880046024888628684680884420400648460404606406286026460640028240266822446048208046826248202606046862408260486282006042842840.00 \\ 
  5 & MDE.Phi.tv & Measure & beta=1.5 & sigma=3 & n=100 & 0.05 \\ 
  6 & MDE.Phi.kl & Measure & beta=1.5 & sigma=3 & n=100 & 0.00 \\ 
  7 & MME & Measure & beta=1.5 & sigma=3 & n=100 & 0.01 \\ 
  8 & MME.b & Measure & beta=1.5 & sigma=3 & n=100 & 7.11 \\ 
  9 & PWM & Measure & beta=1.5 & sigma=3 & n=100 & 0.00 \\ 
  10 & MLE & Measure & beta=2 & sigma=3 & n=100 & 0.00 \\ 
  11 & MLE.b & Measure & beta=2 & sigma=3 & n=100 & 0.00 \\ 
  12 & LME & Measure & beta=2 & sigma=3 & n=100 & 0.00 \\ 
  13 & MDE.Phi.chisq & Measure & beta=2 & sigma=3 & n=100 & 200401541349741565044622684624444464828280006842260482802402460840480462420442408484064028888884208868082024240488464422404022004826686464640022442426206826664828668088026884008426280242408868226824242822022244844842404026644404868866080088628264048220088826862228624862888066442022220866444444086022.00 \\ 
  14 & MDE.Phi.tv & Measure & beta=2 & sigma=3 & n=100 & 0.02 \\ 
  15 & MDE.Phi.kl & Measure & beta=2 & sigma=3 & n=100 & 0.00 \\ 
  16 & MME & Measure & beta=2 & sigma=3 & n=100 & 0.00 \\ 
  17 & MME.b & Measure & beta=2 & sigma=3 & n=100 & 0.01 \\ 
  18 & PWM & Measure & beta=2 & sigma=3 & n=100 & 0.00 \\ 
  19 & MLE & Measure & beta=2.5 & sigma=3 & n=100 & 0.00 \\ 
  20 & MLE.b & Measure & beta=2.5 & sigma=3 & n=100 & 0.00 \\ 
  21 & LME & Measure & beta=2.5 & sigma=3 & n=100 & 0.00 \\ 
  22 & MDE.Phi.chisq & Measure & beta=2.5 & sigma=3 & n=100 & 0.02 \\ 
  23 & MDE.Phi.tv & Measure & beta=2.5 & sigma=3 & n=100 & 0.02 \\ 
  24 & MDE.Phi.kl & Measure & beta=2.5 & sigma=3 & n=100 & 0.00 \\ 
  25 & MME & Measure & beta=2.5 & sigma=3 & n=100 & 0.00 \\ 
  26 & MME.b & Measure & beta=2.5 & sigma=3 & n=100 & 8.08 \\ 
  27 & PWM & Measure & beta=2.5 & sigma=3 & n=100 & 0.00 \\ 
  28 & MLE & Measure & beta=3 & sigma=3 & n=100 & 0.00 \\ 
  29 & MLE.b & Measure & beta=3 & sigma=3 & n=100 & 0.00 \\ 
  30 & LME & Measure & beta=3 & sigma=3 & n=100 & 0.00 \\ 
  31 & MDE.Phi.chisq & Measure & beta=3 & sigma=3 & n=100 & 0.02 \\ 
  32 & MDE.Phi.tv & Measure & beta=3 & sigma=3 & n=100 & 0.02 \\ 
  33 & MDE.Phi.kl & Measure & beta=3 & sigma=3 & n=100 & 0.00 \\ 
  34 & MME & Measure & beta=3 & sigma=3 & n=100 & 0.00 \\ 
  35 & MME.b & Measure & beta=3 & sigma=3 & n=100 & 0.01 \\ 
  36 & PWM & Measure & beta=3 & sigma=3 & n=100 & 0.00 \\ 
  37 & MLE & Measure & beta=4 & sigma=3 & n=100 & 0.00 \\ 
  38 & MLE.b & Measure & beta=4 & sigma=3 & n=100 & 0.00 \\ 
  39 & LME & Measure & beta=4 & sigma=3 & n=100 & 0.00 \\ 
  40 & MDE.Phi.chisq & Measure & beta=4 & sigma=3 & n=100 & 0.02 \\ 
  41 & MDE.Phi.tv & Measure & beta=4 & sigma=3 & n=100 & 0.01 \\ 
  42 & MDE.Phi.kl & Measure & beta=4 & sigma=3 & n=100 & 0.00 \\ 
  43 & MME & Measure & beta=4 & sigma=3 & n=100 & 0.00 \\ 
  44 & MME.b & Measure & beta=4 & sigma=3 & n=100 & 4041.95 \\ 
  45 & PWM & Measure & beta=4 & sigma=3 & n=100 & 0.00 \\ 
  46 & MLE & Measure & beta=5 & sigma=3 & n=100 & 0.00 \\ 
  47 & MLE.b & Measure & beta=5 & sigma=3 & n=100 & 0.00 \\ 
  48 & LME & Measure & beta=5 & sigma=3 & n=100 & 0.00 \\ 
  49 & MDE.Phi.chisq & Measure & beta=5 & sigma=3 & n=100 & 0.01 \\ 
  50 & MDE.Phi.tv & Measure & beta=5 & sigma=3 & n=100 & 0.01 \\ 
  51 & MDE.Phi.kl & Measure & beta=5 & sigma=3 & n=100 & 0.00 \\ 
  52 & MME & Measure & beta=5 & sigma=3 & n=100 & 0.00 \\ 
  53 & MME.b & Measure & beta=5 & sigma=3 & n=100 & 515620813105830396128066264404.00 \\ 
  54 & PWM & Measure & beta=5 & sigma=3 & n=100 & 0.00 \\ 
  55 & MLE & Measure & beta=1.5 & sigma=3 & n=200 & 0.00 \\ 
  56 & MLE.b & Measure & beta=1.5 & sigma=3 & n=200 & 0.00 \\ 
  57 & LME & Measure & beta=1.5 & sigma=3 & n=200 & 0.00 \\ 
  58 & MDE.Phi.chisq & Measure & beta=1.5 & sigma=3 & n=200 & 9837907289457943076080860424686002862804084088868622806442288428220800848484046804640642828004806408848424602226224084064024022806886482060404828246848420044624888240228486882868422448202288484888486048048064060080266048086240822008882402206646624846664426442640206820402646048266080424848440048866046.00 \\ 
  59 & MDE.Phi.tv & Measure & beta=1.5 & sigma=3 & n=200 & 0.03 \\ 
  60 & MDE.Phi.kl & Measure & beta=1.5 & sigma=3 & n=200 & 0.00 \\ 
  61 & MME & Measure & beta=1.5 & sigma=3 & n=200 & 0.01 \\ 
  62 & MME.b & Measure & beta=1.5 & sigma=3 & n=200 & 0.01 \\ 
  63 & PWM & Measure & beta=1.5 & sigma=3 & n=200 & 0.00 \\ 
  64 & MLE & Measure & beta=2 & sigma=3 & n=200 & 0.00 \\ 
  65 & MLE.b & Measure & beta=2 & sigma=3 & n=200 & 0.00 \\ 
  66 & LME & Measure & beta=2 & sigma=3 & n=200 & 0.00 \\ 
  67 & MDE.Phi.chisq & Measure & beta=2 & sigma=3 & n=200 & 32276043278331587168486406646400660846806662666882604688464600480080426200002426084864284604086888482064664462866022264662644460466200220466224048842804640228082260680666222026220280482886440280228488686208846202006202806206086068882000024880682008846244444802282084408880600888628866268624424440842.00 \\ 
  68 & MDE.Phi.tv & Measure & beta=2 & sigma=3 & n=200 & 0.02 \\ 
  69 & MDE.Phi.kl & Measure & beta=2 & sigma=3 & n=200 & 0.00 \\ 
  70 & MME & Measure & beta=2 & sigma=3 & n=200 & 0.00 \\ 
  71 & MME.b & Measure & beta=2 & sigma=3 & n=200 & 0.00 \\ 
  72 & PWM & Measure & beta=2 & sigma=3 & n=200 & 0.00 \\ 
  73 & MLE & Measure & beta=2.5 & sigma=3 & n=200 & 0.00 \\ 
  74 & MLE.b & Measure & beta=2.5 & sigma=3 & n=200 & 0.00 \\ 
  75 & LME & Measure & beta=2.5 & sigma=3 & n=200 & 0.00 \\ 
  76 & MDE.Phi.chisq & Measure & beta=2.5 & sigma=3 & n=200 & 0.02 \\ 
  77 & MDE.Phi.tv & Measure & beta=2.5 & sigma=3 & n=200 & 0.01 \\ 
  78 & MDE.Phi.kl & Measure & beta=2.5 & sigma=3 & n=200 & 0.00 \\ 
  79 & MME & Measure & beta=2.5 & sigma=3 & n=200 & 0.00 \\ 
  80 & MME.b & Measure & beta=2.5 & sigma=3 & n=200 & 0.00 \\ 
  81 & PWM & Measure & beta=2.5 & sigma=3 & n=200 & 0.00 \\ 
  82 & MLE & Measure & beta=3 & sigma=3 & n=200 & 0.00 \\ 
  83 & MLE.b & Measure & beta=3 & sigma=3 & n=200 & 0.00 \\ 
  84 & LME & Measure & beta=3 & sigma=3 & n=200 & 0.00 \\ 
  85 & MDE.Phi.chisq & Measure & beta=3 & sigma=3 & n=200 & 0.01 \\ 
  86 & MDE.Phi.tv & Measure & beta=3 & sigma=3 & n=200 & 0.01 \\ 
  87 & MDE.Phi.kl & Measure & beta=3 & sigma=3 & n=200 & 0.00 \\ 
  88 & MME & Measure & beta=3 & sigma=3 & n=200 & 0.00 \\ 
  89 & MME.b & Measure & beta=3 & sigma=3 & n=200 & 0.00 \\ 
  90 & PWM & Measure & beta=3 & sigma=3 & n=200 & 0.00 \\ 
  91 & MLE & Measure & beta=4 & sigma=3 & n=200 & 0.00 \\ 
  92 & MLE.b & Measure & beta=4 & sigma=3 & n=200 & 0.00 \\ 
  93 & LME & Measure & beta=4 & sigma=3 & n=200 & 0.00 \\ 
  94 & MDE.Phi.chisq & Measure & beta=4 & sigma=3 & n=200 & 0.01 \\ 
  95 & MDE.Phi.tv & Measure & beta=4 & sigma=3 & n=200 & 0.01 \\ 
  96 & MDE.Phi.kl & Measure & beta=4 & sigma=3 & n=200 & 0.00 \\ 
  97 & MME & Measure & beta=4 & sigma=3 & n=200 & 0.00 \\ 
  98 & MME.b & Measure & beta=4 & sigma=3 & n=200 & 0.00 \\ 
  99 & PWM & Measure & beta=4 & sigma=3 & n=200 & 0.00 \\ 
  100 & MLE & Measure & beta=5 & sigma=3 & n=200 & 0.00 \\ 
  101 & MLE.b & Measure & beta=5 & sigma=3 & n=200 & 0.00 \\ 
  102 & LME & Measure & beta=5 & sigma=3 & n=200 & 0.00 \\ 
  103 & MDE.Phi.chisq & Measure & beta=5 & sigma=3 & n=200 & 0.01 \\ 
  104 & MDE.Phi.tv & Measure & beta=5 & sigma=3 & n=200 & 0.01 \\ 
  105 & MDE.Phi.kl & Measure & beta=5 & sigma=3 & n=200 & 0.00 \\ 
  106 & MME & Measure & beta=5 & sigma=3 & n=200 & 0.00 \\ 
  107 & MME.b & Measure & beta=5 & sigma=3 & n=200 & 2.02 \\ 
  108 & PWM & Measure & beta=5 & sigma=3 & n=200 & 0.00 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220204/Output.bias.LaTeX.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Tue Feb 01 16:33:07 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=3 & n=100 & 0.17 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=3 & n=100 & -0.02 \\ 
  3 & LME & beta & beta=1.5 & sigma=3 & n=100 & 0.33 \\ 
  4 & MDE.Phi.chisq & beta & beta=1.5 & sigma=3 & n=100 & -3.37 \\ 
  5 & MDE.Phi.tv & beta & beta=1.5 & sigma=3 & n=100 & -0.27 \\ 
  6 & MDE.Phi.kl & beta & beta=1.5 & sigma=3 & n=100 & 0.17 \\ 
  7 & MME & beta & beta=1.5 & sigma=3 & n=100 & 1.29 \\ 
  8 & MME.b & beta & beta=1.5 & sigma=3 & n=100 & 4.81 \\ 
  9 & PWM & beta & beta=1.5 & sigma=3 & n=100 & 0.33 \\ 
  10 & MLE & sigma & beta=1.5 & sigma=3 & n=100 & 0.55 \\ 
  11 & MLE.b & sigma & beta=1.5 & sigma=3 & n=100 & -0.07 \\ 
  12 & LME & sigma & beta=1.5 & sigma=3 & n=100 & 0.98 \\ 
  13 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=3 & n=100 & 2.22 \\ 
  14 & MDE.Phi.tv & sigma & beta=1.5 & sigma=3 & n=100 & 2.49 \\ 
  15 & MDE.Phi.kl & sigma & beta=1.5 & sigma=3 & n=100 & 0.55 \\ 
  16 & MME & sigma & beta=1.5 & sigma=3 & n=100 & 6.46 \\ 
  17 & MME.b & sigma & beta=1.5 & sigma=3 & n=100 & 17.50 \\ 
  18 & PWM & sigma & beta=1.5 & sigma=3 & n=100 & 0.98 \\ 
  19 & MLE & beta & beta=2 & sigma=3 & n=100 & 0.52 \\ 
  20 & MLE.b & beta & beta=2 & sigma=3 & n=100 & 0.17 \\ 
  21 & LME & beta & beta=2 & sigma=3 & n=100 & 0.45 \\ 
  22 & MDE.Phi.chisq & beta & beta=2 & sigma=3 & n=100 & 0.01 \\ 
  23 & MDE.Phi.tv & beta & beta=2 & sigma=3 & n=100 & 0.66 \\ 
  24 & MDE.Phi.kl & beta & beta=2 & sigma=3 & n=100 & 0.45 \\ 
  25 & MME & beta & beta=2 & sigma=3 & n=100 & 1.68 \\ 
  26 & MME.b & beta & beta=2 & sigma=3 & n=100 & 7.48 \\ 
  27 & PWM & beta & beta=2 & sigma=3 & n=100 & 0.45 \\ 
  28 & MLE & sigma & beta=2 & sigma=3 & n=100 & 1.09 \\ 
  29 & MLE.b & sigma & beta=2 & sigma=3 & n=100 & 0.33 \\ 
  30 & LME & sigma & beta=2 & sigma=3 & n=100 & 0.90 \\ 
  31 & MDE.Phi.chisq & sigma & beta=2 & sigma=3 & n=100 & 3.23 \\ 
  32 & MDE.Phi.tv & sigma & beta=2 & sigma=3 & n=100 & 4.71 \\ 
  33 & MDE.Phi.kl & sigma & beta=2 & sigma=3 & n=100 & 0.96 \\ 
  34 & MME & sigma & beta=2 & sigma=3 & n=100 & 4.31 \\ 
  35 & MME.b & sigma & beta=2 & sigma=3 & n=100 & 16.76 \\ 
  36 & PWM & sigma & beta=2 & sigma=3 & n=100 & 0.90 \\ 
  37 & MLE & beta & beta=2.5 & sigma=3 & n=100 & 1.06 \\ 
  38 & MLE.b & beta & beta=2.5 & sigma=3 & n=100 & 0.60 \\ 
  39 & LME & beta & beta=2.5 & sigma=3 & n=100 & 0.70 \\ 
  40 & MDE.Phi.chisq & beta & beta=2.5 & sigma=3 & n=100 & 1.52 \\ 
  41 & MDE.Phi.tv & beta & beta=2.5 & sigma=3 & n=100 & 2.33 \\ 
  42 & MDE.Phi.kl & beta & beta=2.5 & sigma=3 & n=100 & 0.93 \\ 
  43 & MME & beta & beta=2.5 & sigma=3 & n=100 & 2.32 \\ 
  44 & MME.b & beta & beta=2.5 & sigma=3 & n=100 & 5.49 \\ 
  45 & PWM & beta & beta=2.5 & sigma=3 & n=100 & 0.70 \\ 
  46 & MLE & sigma & beta=2.5 & sigma=3 & n=100 & 1.70 \\ 
  47 & MLE.b & sigma & beta=2.5 & sigma=3 & n=100 & 0.96 \\ 
  48 & LME & sigma & beta=2.5 & sigma=3 & n=100 & 1.08 \\ 
  49 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=3 & n=100 & 6.02 \\ 
  50 & MDE.Phi.tv & sigma & beta=2.5 & sigma=3 & n=100 & 7.57 \\ 
  51 & MDE.Phi.kl & sigma & beta=2.5 & sigma=3 & n=100 & 1.50 \\ 
  52 & MME & sigma & beta=2.5 & sigma=3 & n=100 & 4.06 \\ 
  53 & MME.b & sigma & beta=2.5 & sigma=3 & n=100 & 9.06 \\ 
  54 & PWM & sigma & beta=2.5 & sigma=3 & n=100 & 1.08 \\ 
  55 & MLE & beta & beta=3 & sigma=3 & n=100 & 2.60 \\ 
  56 & MLE.b & beta & beta=3 & sigma=3 & n=100 & 2.10 \\ 
  57 & LME & beta & beta=3 & sigma=3 & n=100 & 1.02 \\ 
  58 & MDE.Phi.chisq & beta & beta=3 & sigma=3 & n=100 & 3.62 \\ 
  59 & MDE.Phi.tv & beta & beta=3 & sigma=3 & n=100 & 4.96 \\ 
  60 & MDE.Phi.kl & beta & beta=3 & sigma=3 & n=100 & 1.83 \\ 
  61 & MME & beta & beta=3 & sigma=3 & n=100 & 14.49 \\ 
  62 & MME.b & beta & beta=3 & sigma=3 & n=100 & 46.99 \\ 
  63 & PWM & beta & beta=3 & sigma=3 & n=100 & 1.02 \\ 
  64 & MLE & sigma & beta=3 & sigma=3 & n=100 & 3.35 \\ 
  65 & MLE.b & sigma & beta=3 & sigma=3 & n=100 & 2.71 \\ 
  66 & LME & sigma & beta=3 & sigma=3 & n=100 & 1.28 \\ 
  67 & MDE.Phi.chisq & sigma & beta=3 & sigma=3 & n=100 & 8.99 \\ 
  68 & MDE.Phi.tv & sigma & beta=3 & sigma=3 & n=100 & 11.05 \\ 
  69 & MDE.Phi.kl & sigma & beta=3 & sigma=3 & n=100 & 2.36 \\ 
  70 & MME & sigma & beta=3 & sigma=3 & n=100 & 17.23 \\ 
  71 & MME.b & sigma & beta=3 & sigma=3 & n=100 & 55.71 \\ 
  72 & PWM & sigma & beta=3 & sigma=3 & n=100 & 1.28 \\ 
  73 & MLE & beta & beta=4 & sigma=3 & n=100 & 4.57 \\ 
  74 & MLE.b & beta & beta=4 & sigma=3 & n=100 & 4.12 \\ 
  75 & LME & beta & beta=4 & sigma=3 & n=100 & 1.74 \\ 
  76 & MDE.Phi.chisq & beta & beta=4 & sigma=3 & n=100 & 9.17 \\ 
  77 & MDE.Phi.tv & beta & beta=4 & sigma=3 & n=100 & 11.26 \\ 
  78 & MDE.Phi.kl & beta & beta=4 & sigma=3 & n=100 & 3.37 \\ 
  79 & MME & beta & beta=4 & sigma=3 & n=100 & 7.35 \\ 
  80 & MME.b & beta & beta=4 & sigma=3 & n=100 & 36.91 \\ 
  81 & PWM & beta & beta=4 & sigma=3 & n=100 & 1.74 \\ 
  82 & MLE & sigma & beta=4 & sigma=3 & n=100 & 4.23 \\ 
  83 & MLE.b & sigma & beta=4 & sigma=3 & n=100 & 3.83 \\ 
  84 & LME & sigma & beta=4 & sigma=3 & n=100 & 1.59 \\ 
  85 & MDE.Phi.chisq & sigma & beta=4 & sigma=3 & n=100 & 13.97 \\ 
  86 & MDE.Phi.tv & sigma & beta=4 & sigma=3 & n=100 & 16.02 \\ 
  87 & MDE.Phi.kl & sigma & beta=4 & sigma=3 & n=100 & 3.14 \\ 
  88 & MME & sigma & beta=4 & sigma=3 & n=100 & 7.00 \\ 
  89 & MME.b & sigma & beta=4 & sigma=3 & n=100 & 37.30 \\ 
  90 & PWM & sigma & beta=4 & sigma=3 & n=100 & 1.59 \\ 
  91 & MLE & beta & beta=5 & sigma=3 & n=100 & 7.13 \\ 
  92 & MLE.b & beta & beta=5 & sigma=3 & n=100 & 6.76 \\ 
  93 & LME & beta & beta=5 & sigma=3 & n=100 & 2.30 \\ 
  94 & MDE.Phi.chisq & beta & beta=5 & sigma=3 & n=100 & 14.14 \\ 
  95 & MDE.Phi.tv & beta & beta=5 & sigma=3 & n=100 & 16.20 \\ 
  96 & MDE.Phi.kl & beta & beta=5 & sigma=3 & n=100 & 4.95 \\ 
  97 & MME & beta & beta=5 & sigma=3 & n=100 & 11.71 \\ 
  98 & MME.b & beta & beta=5 & sigma=3 & n=100 & 42.12 \\ 
  99 & PWM & beta & beta=5 & sigma=3 & n=100 & 2.30 \\ 
  100 & MLE & sigma & beta=5 & sigma=3 & n=100 & 5.03 \\ 
  101 & MLE.b & sigma & beta=5 & sigma=3 & n=100 & 4.78 \\ 
  102 & LME & sigma & beta=5 & sigma=3 & n=100 & 1.61 \\ 
  103 & MDE.Phi.chisq & sigma & beta=5 & sigma=3 & n=100 & 15.83 \\ 
  104 & MDE.Phi.tv & sigma & beta=5 & sigma=3 & n=100 & 17.22 \\ 
  105 & MDE.Phi.kl & sigma & beta=5 & sigma=3 & n=100 & 3.50 \\ 
  106 & MME & sigma & beta=5 & sigma=3 & n=100 & 8.23 \\ 
  107 & MME.b & sigma & beta=5 & sigma=3 & n=100 & 29.87 \\ 
  108 & PWM & sigma & beta=5 & sigma=3 & n=100 & 1.61 \\ 
  109 & MLE & beta & beta=1.5 & sigma=3 & n=200 & 0.23 \\ 
  110 & MLE.b & beta & beta=1.5 & sigma=3 & n=200 & 0.13 \\ 
  111 & LME & beta & beta=1.5 & sigma=3 & n=200 & 0.21 \\ 
  112 & MDE.Phi.chisq & beta & beta=1.5 & sigma=3 & n=200 & -1.32 \\ 
  113 & MDE.Phi.tv & beta & beta=1.5 & sigma=3 & n=200 & -0.50 \\ 
  114 & MDE.Phi.kl & beta & beta=1.5 & sigma=3 & n=200 & 0.08 \\ 
  115 & MME & beta & beta=1.5 & sigma=3 & n=200 & 1.00 \\ 
  116 & MME.b & beta & beta=1.5 & sigma=3 & n=200 & 0.80 \\ 
  117 & PWM & beta & beta=1.5 & sigma=3 & n=200 & 0.21 \\ 
  118 & MLE & sigma & beta=1.5 & sigma=3 & n=200 & 0.72 \\ 
  119 & MLE.b & sigma & beta=1.5 & sigma=3 & n=200 & 0.40 \\ 
  120 & LME & sigma & beta=1.5 & sigma=3 & n=200 & 0.61 \\ 
  121 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=3 & n=200 & 0.65 \\ 
  122 & MDE.Phi.tv & sigma & beta=1.5 & sigma=3 & n=200 & 0.78 \\ 
  123 & MDE.Phi.kl & sigma & beta=1.5 & sigma=3 & n=200 & 0.25 \\ 
  124 & MME & sigma & beta=1.5 & sigma=3 & n=200 & 5.36 \\ 
  125 & MME.b & sigma & beta=1.5 & sigma=3 & n=200 & 4.53 \\ 
  126 & PWM & sigma & beta=1.5 & sigma=3 & n=200 & 0.61 \\ 
  127 & MLE & beta & beta=2 & sigma=3 & n=200 & 0.25 \\ 
  128 & MLE.b & beta & beta=2 & sigma=3 & n=200 & 0.06 \\ 
  129 & LME & beta & beta=2 & sigma=3 & n=200 & 0.22 \\ 
  130 & MDE.Phi.chisq & beta & beta=2 & sigma=3 & n=200 & -0.68 \\ 
  131 & MDE.Phi.tv & beta & beta=2 & sigma=3 & n=200 & -0.44 \\ 
  132 & MDE.Phi.kl & beta & beta=2 & sigma=3 & n=200 & 0.14 \\ 
  133 & MME & beta & beta=2 & sigma=3 & n=200 & 0.97 \\ 
  134 & MME.b & beta & beta=2 & sigma=3 & n=200 & 0.69 \\ 
  135 & PWM & beta & beta=2 & sigma=3 & n=200 & 0.22 \\ 
  136 & MLE & sigma & beta=2 & sigma=3 & n=200 & 0.53 \\ 
  137 & MLE.b & sigma & beta=2 & sigma=3 & n=200 & 0.12 \\ 
  138 & LME & sigma & beta=2 & sigma=3 & n=200 & 0.43 \\ 
  139 & MDE.Phi.chisq & sigma & beta=2 & sigma=3 & n=200 & 0.52 \\ 
  140 & MDE.Phi.tv & sigma & beta=2 & sigma=3 & n=200 & 0.83 \\ 
  141 & MDE.Phi.kl & sigma & beta=2 & sigma=3 & n=200 & 0.29 \\ 
  142 & MME & sigma & beta=2 & sigma=3 & n=200 & 2.67 \\ 
  143 & MME.b & sigma & beta=2 & sigma=3 & n=200 & 1.94 \\ 
  144 & PWM & sigma & beta=2 & sigma=3 & n=200 & 0.43 \\ 
  145 & MLE & beta & beta=2.5 & sigma=3 & n=200 & 0.34 \\ 
  146 & MLE.b & beta & beta=2.5 & sigma=3 & n=200 & 0.02 \\ 
  147 & LME & beta & beta=2.5 & sigma=3 & n=200 & 0.28 \\ 
  148 & MDE.Phi.chisq & beta & beta=2.5 & sigma=3 & n=200 & -0.46 \\ 
  149 & MDE.Phi.tv & beta & beta=2.5 & sigma=3 & n=200 & -0.23 \\ 
  150 & MDE.Phi.kl & beta & beta=2.5 & sigma=3 & n=200 & 0.25 \\ 
  151 & MME & beta & beta=2.5 & sigma=3 & n=200 & 1.06 \\ 
  152 & MME.b & beta & beta=2.5 & sigma=3 & n=200 & 0.84 \\ 
  153 & PWM & beta & beta=2.5 & sigma=3 & n=200 & 0.28 \\ 
  154 & MLE & sigma & beta=2.5 & sigma=3 & n=200 & 0.56 \\ 
  155 & MLE.b & sigma & beta=2.5 & sigma=3 & n=200 & 0.03 \\ 
  156 & LME & sigma & beta=2.5 & sigma=3 & n=200 & 0.43 \\ 
  157 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=3 & n=200 & 1.04 \\ 
  158 & MDE.Phi.tv & sigma & beta=2.5 & sigma=3 & n=200 & 1.20 \\ 
  159 & MDE.Phi.kl & sigma & beta=2.5 & sigma=3 & n=200 & 0.41 \\ 
  160 & MME & sigma & beta=2.5 & sigma=3 & n=200 & 1.96 \\ 
  161 & MME.b & sigma & beta=2.5 & sigma=3 & n=200 & 1.52 \\ 
  162 & PWM & sigma & beta=2.5 & sigma=3 & n=200 & 0.43 \\ 
  163 & MLE & beta & beta=3 & sigma=3 & n=200 & 0.72 \\ 
  164 & MLE.b & beta & beta=3 & sigma=3 & n=200 & 0.23 \\ 
  165 & LME & beta & beta=3 & sigma=3 & n=200 & 0.45 \\ 
  166 & MDE.Phi.chisq & beta & beta=3 & sigma=3 & n=200 & 0.27 \\ 
  167 & MDE.Phi.tv & beta & beta=3 & sigma=3 & n=200 & 0.19 \\ 
  168 & MDE.Phi.kl & beta & beta=3 & sigma=3 & n=200 & 0.49 \\ 
  169 & MME & beta & beta=3 & sigma=3 & n=200 & 1.40 \\ 
  170 & MME.b & beta & beta=3 & sigma=3 & n=200 & 2.69 \\ 
  171 & PWM & beta & beta=3 & sigma=3 & n=200 & 0.45 \\ 
  172 & MLE & sigma & beta=3 & sigma=3 & n=200 & 0.93 \\ 
  173 & MLE.b & sigma & beta=3 & sigma=3 & n=200 & 0.30 \\ 
  174 & LME & sigma & beta=3 & sigma=3 & n=200 & 0.57 \\ 
  175 & MDE.Phi.chisq & sigma & beta=3 & sigma=3 & n=200 & 2.25 \\ 
  176 & MDE.Phi.tv & sigma & beta=3 & sigma=3 & n=200 & 1.76 \\ 
  177 & MDE.Phi.kl & sigma & beta=3 & sigma=3 & n=200 & 0.64 \\ 
  178 & MME & sigma & beta=3 & sigma=3 & n=200 & 1.94 \\ 
  179 & MME.b & sigma & beta=3 & sigma=3 & n=200 & 3.69 \\ 
  180 & PWM & sigma & beta=3 & sigma=3 & n=200 & 0.57 \\ 
  181 & MLE & beta & beta=4 & sigma=3 & n=200 & 1.56 \\ 
  182 & MLE.b & beta & beta=4 & sigma=3 & n=200 & 0.88 \\ 
  183 & LME & beta & beta=4 & sigma=3 & n=200 & 0.92 \\ 
  184 & MDE.Phi.chisq & beta & beta=4 & sigma=3 & n=200 & 3.48 \\ 
  185 & MDE.Phi.tv & beta & beta=4 & sigma=3 & n=200 & 2.80 \\ 
  186 & MDE.Phi.kl & beta & beta=4 & sigma=3 & n=200 & 1.25 \\ 
  187 & MME & beta & beta=4 & sigma=3 & n=200 & 2.64 \\ 
  188 & MME.b & beta & beta=4 & sigma=3 & n=200 & 9.69 \\ 
  189 & PWM & beta & beta=4 & sigma=3 & n=200 & 0.92 \\ 
  190 & MLE & sigma & beta=4 & sigma=3 & n=200 & 1.47 \\ 
  191 & MLE.b & sigma & beta=4 & sigma=3 & n=200 & 0.84 \\ 
  192 & LME & sigma & beta=4 & sigma=3 & n=200 & 0.83 \\ 
  193 & MDE.Phi.chisq & sigma & beta=4 & sigma=3 & n=200 & 5.73 \\ 
  194 & MDE.Phi.tv & sigma & beta=4 & sigma=3 & n=200 & 4.52 \\ 
  195 & MDE.Phi.kl & sigma & beta=4 & sigma=3 & n=200 & 1.15 \\ 
  196 & MME & sigma & beta=4 & sigma=3 & n=200 & 2.49 \\ 
  197 & MME.b & sigma & beta=4 & sigma=3 & n=200 & 9.38 \\ 
  198 & PWM & sigma & beta=4 & sigma=3 & n=200 & 0.83 \\ 
  199 & MLE & beta & beta=5 & sigma=3 & n=200 & 4.05 \\ 
  200 & MLE.b & beta & beta=5 & sigma=3 & n=200 & 3.34 \\ 
  201 & LME & beta & beta=5 & sigma=3 & n=200 & 1.77 \\ 
  202 & MDE.Phi.chisq & beta & beta=5 & sigma=3 & n=200 & 8.57 \\ 
  203 & MDE.Phi.tv & beta & beta=5 & sigma=3 & n=200 & 6.01 \\ 
  204 & MDE.Phi.kl & beta & beta=5 & sigma=3 & n=200 & 2.55 \\ 
  205 & MME & beta & beta=5 & sigma=3 & n=200 & 4.77 \\ 
  206 & MME.b & beta & beta=5 & sigma=3 & n=200 & 16.61 \\ 
  207 & PWM & beta & beta=5 & sigma=3 & n=200 & 1.77 \\ 
  208 & MLE & sigma & beta=5 & sigma=3 & n=200 & 2.94 \\ 
  209 & MLE.b & sigma & beta=5 & sigma=3 & n=200 & 2.44 \\ 
  210 & LME & sigma & beta=5 & sigma=3 & n=200 & 1.24 \\ 
  211 & MDE.Phi.chisq & sigma & beta=5 & sigma=3 & n=200 & 9.29 \\ 
  212 & MDE.Phi.tv & sigma & beta=5 & sigma=3 & n=200 & 6.45 \\ 
  213 & MDE.Phi.kl & sigma & beta=5 & sigma=3 & n=200 & 1.81 \\ 
  214 & MME & sigma & beta=5 & sigma=3 & n=200 & 3.40 \\ 
  215 & MME.b & sigma & beta=5 & sigma=3 & n=200 & 11.83 \\ 
  216 & PWM & sigma & beta=5 & sigma=3 & n=200 & 1.24 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220204/Output.mean.LaTeX.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Tue Feb 01 16:33:07 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=3 & n=100 & 1.67 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=3 & n=100 & 1.48 \\ 
  3 & LME & beta & beta=1.5 & sigma=3 & n=100 & 1.83 \\ 
  4 & MDE.Phi.chisq & beta & beta=1.5 & sigma=3 & n=100 & -1.87 \\ 
  5 & MDE.Phi.tv & beta & beta=1.5 & sigma=3 & n=100 & 1.23 \\ 
  6 & MDE.Phi.kl & beta & beta=1.5 & sigma=3 & n=100 & 1.67 \\ 
  7 & MME & beta & beta=1.5 & sigma=3 & n=100 & 2.79 \\ 
  8 & MME.b & beta & beta=1.5 & sigma=3 & n=100 & 6.31 \\ 
  9 & PWM & beta & beta=1.5 & sigma=3 & n=100 & 1.83 \\ 
  10 & MLE & sigma & beta=1.5 & sigma=3 & n=100 & 3.55 \\ 
  11 & MLE.b & sigma & beta=1.5 & sigma=3 & n=100 & 2.93 \\ 
  12 & LME & sigma & beta=1.5 & sigma=3 & n=100 & 3.98 \\ 
  13 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=3 & n=100 & 5.22 \\ 
  14 & MDE.Phi.tv & sigma & beta=1.5 & sigma=3 & n=100 & 5.49 \\ 
  15 & MDE.Phi.kl & sigma & beta=1.5 & sigma=3 & n=100 & 3.55 \\ 
  16 & MME & sigma & beta=1.5 & sigma=3 & n=100 & 9.46 \\ 
  17 & MME.b & sigma & beta=1.5 & sigma=3 & n=100 & 20.50 \\ 
  18 & PWM & sigma & beta=1.5 & sigma=3 & n=100 & 3.98 \\ 
  19 & MLE & beta & beta=2 & sigma=3 & n=100 & 2.52 \\ 
  20 & MLE.b & beta & beta=2 & sigma=3 & n=100 & 2.17 \\ 
  21 & LME & beta & beta=2 & sigma=3 & n=100 & 2.45 \\ 
  22 & MDE.Phi.chisq & beta & beta=2 & sigma=3 & n=100 & 2.01 \\ 
  23 & MDE.Phi.tv & beta & beta=2 & sigma=3 & n=100 & 2.66 \\ 
  24 & MDE.Phi.kl & beta & beta=2 & sigma=3 & n=100 & 2.45 \\ 
  25 & MME & beta & beta=2 & sigma=3 & n=100 & 3.68 \\ 
  26 & MME.b & beta & beta=2 & sigma=3 & n=100 & 9.48 \\ 
  27 & PWM & beta & beta=2 & sigma=3 & n=100 & 2.45 \\ 
  28 & MLE & sigma & beta=2 & sigma=3 & n=100 & 4.09 \\ 
  29 & MLE.b & sigma & beta=2 & sigma=3 & n=100 & 3.33 \\ 
  30 & LME & sigma & beta=2 & sigma=3 & n=100 & 3.90 \\ 
  31 & MDE.Phi.chisq & sigma & beta=2 & sigma=3 & n=100 & 6.23 \\ 
  32 & MDE.Phi.tv & sigma & beta=2 & sigma=3 & n=100 & 7.71 \\ 
  33 & MDE.Phi.kl & sigma & beta=2 & sigma=3 & n=100 & 3.96 \\ 
  34 & MME & sigma & beta=2 & sigma=3 & n=100 & 7.31 \\ 
  35 & MME.b & sigma & beta=2 & sigma=3 & n=100 & 19.76 \\ 
  36 & PWM & sigma & beta=2 & sigma=3 & n=100 & 3.90 \\ 
  37 & MLE & beta & beta=2.5 & sigma=3 & n=100 & 3.56 \\ 
  38 & MLE.b & beta & beta=2.5 & sigma=3 & n=100 & 3.10 \\ 
  39 & LME & beta & beta=2.5 & sigma=3 & n=100 & 3.20 \\ 
  40 & MDE.Phi.chisq & beta & beta=2.5 & sigma=3 & n=100 & 4.02 \\ 
  41 & MDE.Phi.tv & beta & beta=2.5 & sigma=3 & n=100 & 4.83 \\ 
  42 & MDE.Phi.kl & beta & beta=2.5 & sigma=3 & n=100 & 3.43 \\ 
  43 & MME & beta & beta=2.5 & sigma=3 & n=100 & 4.82 \\ 
  44 & MME.b & beta & beta=2.5 & sigma=3 & n=100 & 7.99 \\ 
  45 & PWM & beta & beta=2.5 & sigma=3 & n=100 & 3.20 \\ 
  46 & MLE & sigma & beta=2.5 & sigma=3 & n=100 & 4.70 \\ 
  47 & MLE.b & sigma & beta=2.5 & sigma=3 & n=100 & 3.96 \\ 
  48 & LME & sigma & beta=2.5 & sigma=3 & n=100 & 4.08 \\ 
  49 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=3 & n=100 & 9.02 \\ 
  50 & MDE.Phi.tv & sigma & beta=2.5 & sigma=3 & n=100 & 10.57 \\ 
  51 & MDE.Phi.kl & sigma & beta=2.5 & sigma=3 & n=100 & 4.50 \\ 
  52 & MME & sigma & beta=2.5 & sigma=3 & n=100 & 7.06 \\ 
  53 & MME.b & sigma & beta=2.5 & sigma=3 & n=100 & 12.06 \\ 
  54 & PWM & sigma & beta=2.5 & sigma=3 & n=100 & 4.08 \\ 
  55 & MLE & beta & beta=3 & sigma=3 & n=100 & 5.60 \\ 
  56 & MLE.b & beta & beta=3 & sigma=3 & n=100 & 5.10 \\ 
  57 & LME & beta & beta=3 & sigma=3 & n=100 & 4.02 \\ 
  58 & MDE.Phi.chisq & beta & beta=3 & sigma=3 & n=100 & 6.62 \\ 
  59 & MDE.Phi.tv & beta & beta=3 & sigma=3 & n=100 & 7.96 \\ 
  60 & MDE.Phi.kl & beta & beta=3 & sigma=3 & n=100 & 4.83 \\ 
  61 & MME & beta & beta=3 & sigma=3 & n=100 & 17.49 \\ 
  62 & MME.b & beta & beta=3 & sigma=3 & n=100 & 49.99 \\ 
  63 & PWM & beta & beta=3 & sigma=3 & n=100 & 4.02 \\ 
  64 & MLE & sigma & beta=3 & sigma=3 & n=100 & 6.35 \\ 
  65 & MLE.b & sigma & beta=3 & sigma=3 & n=100 & 5.71 \\ 
  66 & LME & sigma & beta=3 & sigma=3 & n=100 & 4.28 \\ 
  67 & MDE.Phi.chisq & sigma & beta=3 & sigma=3 & n=100 & 11.99 \\ 
  68 & MDE.Phi.tv & sigma & beta=3 & sigma=3 & n=100 & 14.05 \\ 
  69 & MDE.Phi.kl & sigma & beta=3 & sigma=3 & n=100 & 5.36 \\ 
  70 & MME & sigma & beta=3 & sigma=3 & n=100 & 20.23 \\ 
  71 & MME.b & sigma & beta=3 & sigma=3 & n=100 & 58.71 \\ 
  72 & PWM & sigma & beta=3 & sigma=3 & n=100 & 4.28 \\ 
  73 & MLE & beta & beta=4 & sigma=3 & n=100 & 8.57 \\ 
  74 & MLE.b & beta & beta=4 & sigma=3 & n=100 & 8.12 \\ 
  75 & LME & beta & beta=4 & sigma=3 & n=100 & 5.74 \\ 
  76 & MDE.Phi.chisq & beta & beta=4 & sigma=3 & n=100 & 13.17 \\ 
  77 & MDE.Phi.tv & beta & beta=4 & sigma=3 & n=100 & 15.26 \\ 
  78 & MDE.Phi.kl & beta & beta=4 & sigma=3 & n=100 & 7.37 \\ 
  79 & MME & beta & beta=4 & sigma=3 & n=100 & 11.35 \\ 
  80 & MME.b & beta & beta=4 & sigma=3 & n=100 & 40.91 \\ 
  81 & PWM & beta & beta=4 & sigma=3 & n=100 & 5.74 \\ 
  82 & MLE & sigma & beta=4 & sigma=3 & n=100 & 7.23 \\ 
  83 & MLE.b & sigma & beta=4 & sigma=3 & n=100 & 6.83 \\ 
  84 & LME & sigma & beta=4 & sigma=3 & n=100 & 4.59 \\ 
  85 & MDE.Phi.chisq & sigma & beta=4 & sigma=3 & n=100 & 16.97 \\ 
  86 & MDE.Phi.tv & sigma & beta=4 & sigma=3 & n=100 & 19.02 \\ 
  87 & MDE.Phi.kl & sigma & beta=4 & sigma=3 & n=100 & 6.14 \\ 
  88 & MME & sigma & beta=4 & sigma=3 & n=100 & 10.00 \\ 
  89 & MME.b & sigma & beta=4 & sigma=3 & n=100 & 40.30 \\ 
  90 & PWM & sigma & beta=4 & sigma=3 & n=100 & 4.59 \\ 
  91 & MLE & beta & beta=5 & sigma=3 & n=100 & 12.13 \\ 
  92 & MLE.b & beta & beta=5 & sigma=3 & n=100 & 11.76 \\ 
  93 & LME & beta & beta=5 & sigma=3 & n=100 & 7.30 \\ 
  94 & MDE.Phi.chisq & beta & beta=5 & sigma=3 & n=100 & 19.14 \\ 
  95 & MDE.Phi.tv & beta & beta=5 & sigma=3 & n=100 & 21.20 \\ 
  96 & MDE.Phi.kl & beta & beta=5 & sigma=3 & n=100 & 9.95 \\ 
  97 & MME & beta & beta=5 & sigma=3 & n=100 & 16.71 \\ 
  98 & MME.b & beta & beta=5 & sigma=3 & n=100 & 47.12 \\ 
  99 & PWM & beta & beta=5 & sigma=3 & n=100 & 7.30 \\ 
  100 & MLE & sigma & beta=5 & sigma=3 & n=100 & 8.03 \\ 
  101 & MLE.b & sigma & beta=5 & sigma=3 & n=100 & 7.78 \\ 
  102 & LME & sigma & beta=5 & sigma=3 & n=100 & 4.61 \\ 
  103 & MDE.Phi.chisq & sigma & beta=5 & sigma=3 & n=100 & 18.83 \\ 
  104 & MDE.Phi.tv & sigma & beta=5 & sigma=3 & n=100 & 20.22 \\ 
  105 & MDE.Phi.kl & sigma & beta=5 & sigma=3 & n=100 & 6.50 \\ 
  106 & MME & sigma & beta=5 & sigma=3 & n=100 & 11.23 \\ 
  107 & MME.b & sigma & beta=5 & sigma=3 & n=100 & 32.87 \\ 
  108 & PWM & sigma & beta=5 & sigma=3 & n=100 & 4.61 \\ 
  109 & MLE & beta & beta=1.5 & sigma=3 & n=200 & 1.73 \\ 
  110 & MLE.b & beta & beta=1.5 & sigma=3 & n=200 & 1.63 \\ 
  111 & LME & beta & beta=1.5 & sigma=3 & n=200 & 1.71 \\ 
  112 & MDE.Phi.chisq & beta & beta=1.5 & sigma=3 & n=200 & 0.18 \\ 
  113 & MDE.Phi.tv & beta & beta=1.5 & sigma=3 & n=200 & 1.00 \\ 
  114 & MDE.Phi.kl & beta & beta=1.5 & sigma=3 & n=200 & 1.58 \\ 
  115 & MME & beta & beta=1.5 & sigma=3 & n=200 & 2.50 \\ 
  116 & MME.b & beta & beta=1.5 & sigma=3 & n=200 & 2.30 \\ 
  117 & PWM & beta & beta=1.5 & sigma=3 & n=200 & 1.71 \\ 
  118 & MLE & sigma & beta=1.5 & sigma=3 & n=200 & 3.72 \\ 
  119 & MLE.b & sigma & beta=1.5 & sigma=3 & n=200 & 3.40 \\ 
  120 & LME & sigma & beta=1.5 & sigma=3 & n=200 & 3.61 \\ 
  121 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=3 & n=200 & 3.65 \\ 
  122 & MDE.Phi.tv & sigma & beta=1.5 & sigma=3 & n=200 & 3.78 \\ 
  123 & MDE.Phi.kl & sigma & beta=1.5 & sigma=3 & n=200 & 3.25 \\ 
  124 & MME & sigma & beta=1.5 & sigma=3 & n=200 & 8.36 \\ 
  125 & MME.b & sigma & beta=1.5 & sigma=3 & n=200 & 7.53 \\ 
  126 & PWM & sigma & beta=1.5 & sigma=3 & n=200 & 3.61 \\ 
  127 & MLE & beta & beta=2 & sigma=3 & n=200 & 2.25 \\ 
  128 & MLE.b & beta & beta=2 & sigma=3 & n=200 & 2.06 \\ 
  129 & LME & beta & beta=2 & sigma=3 & n=200 & 2.22 \\ 
  130 & MDE.Phi.chisq & beta & beta=2 & sigma=3 & n=200 & 1.32 \\ 
  131 & MDE.Phi.tv & beta & beta=2 & sigma=3 & n=200 & 1.56 \\ 
  132 & MDE.Phi.kl & beta & beta=2 & sigma=3 & n=200 & 2.14 \\ 
  133 & MME & beta & beta=2 & sigma=3 & n=200 & 2.97 \\ 
  134 & MME.b & beta & beta=2 & sigma=3 & n=200 & 2.69 \\ 
  135 & PWM & beta & beta=2 & sigma=3 & n=200 & 2.22 \\ 
  136 & MLE & sigma & beta=2 & sigma=3 & n=200 & 3.53 \\ 
  137 & MLE.b & sigma & beta=2 & sigma=3 & n=200 & 3.12 \\ 
  138 & LME & sigma & beta=2 & sigma=3 & n=200 & 3.43 \\ 
  139 & MDE.Phi.chisq & sigma & beta=2 & sigma=3 & n=200 & 3.52 \\ 
  140 & MDE.Phi.tv & sigma & beta=2 & sigma=3 & n=200 & 3.83 \\ 
  141 & MDE.Phi.kl & sigma & beta=2 & sigma=3 & n=200 & 3.29 \\ 
  142 & MME & sigma & beta=2 & sigma=3 & n=200 & 5.67 \\ 
  143 & MME.b & sigma & beta=2 & sigma=3 & n=200 & 4.94 \\ 
  144 & PWM & sigma & beta=2 & sigma=3 & n=200 & 3.43 \\ 
  145 & MLE & beta & beta=2.5 & sigma=3 & n=200 & 2.84 \\ 
  146 & MLE.b & beta & beta=2.5 & sigma=3 & n=200 & 2.52 \\ 
  147 & LME & beta & beta=2.5 & sigma=3 & n=200 & 2.78 \\ 
  148 & MDE.Phi.chisq & beta & beta=2.5 & sigma=3 & n=200 & 2.04 \\ 
  149 & MDE.Phi.tv & beta & beta=2.5 & sigma=3 & n=200 & 2.27 \\ 
  150 & MDE.Phi.kl & beta & beta=2.5 & sigma=3 & n=200 & 2.75 \\ 
  151 & MME & beta & beta=2.5 & sigma=3 & n=200 & 3.56 \\ 
  152 & MME.b & beta & beta=2.5 & sigma=3 & n=200 & 3.34 \\ 
  153 & PWM & beta & beta=2.5 & sigma=3 & n=200 & 2.78 \\ 
  154 & MLE & sigma & beta=2.5 & sigma=3 & n=200 & 3.56 \\ 
  155 & MLE.b & sigma & beta=2.5 & sigma=3 & n=200 & 3.03 \\ 
  156 & LME & sigma & beta=2.5 & sigma=3 & n=200 & 3.43 \\ 
  157 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=3 & n=200 & 4.04 \\ 
  158 & MDE.Phi.tv & sigma & beta=2.5 & sigma=3 & n=200 & 4.20 \\ 
  159 & MDE.Phi.kl & sigma & beta=2.5 & sigma=3 & n=200 & 3.41 \\ 
  160 & MME & sigma & beta=2.5 & sigma=3 & n=200 & 4.96 \\ 
  161 & MME.b & sigma & beta=2.5 & sigma=3 & n=200 & 4.52 \\ 
  162 & PWM & sigma & beta=2.5 & sigma=3 & n=200 & 3.43 \\ 
  163 & MLE & beta & beta=3 & sigma=3 & n=200 & 3.72 \\ 
  164 & MLE.b & beta & beta=3 & sigma=3 & n=200 & 3.23 \\ 
  165 & LME & beta & beta=3 & sigma=3 & n=200 & 3.45 \\ 
  166 & MDE.Phi.chisq & beta & beta=3 & sigma=3 & n=200 & 3.27 \\ 
  167 & MDE.Phi.tv & beta & beta=3 & sigma=3 & n=200 & 3.19 \\ 
  168 & MDE.Phi.kl & beta & beta=3 & sigma=3 & n=200 & 3.49 \\ 
  169 & MME & beta & beta=3 & sigma=3 & n=200 & 4.40 \\ 
  170 & MME.b & beta & beta=3 & sigma=3 & n=200 & 5.69 \\ 
  171 & PWM & beta & beta=3 & sigma=3 & n=200 & 3.45 \\ 
  172 & MLE & sigma & beta=3 & sigma=3 & n=200 & 3.93 \\ 
  173 & MLE.b & sigma & beta=3 & sigma=3 & n=200 & 3.30 \\ 
  174 & LME & sigma & beta=3 & sigma=3 & n=200 & 3.57 \\ 
  175 & MDE.Phi.chisq & sigma & beta=3 & sigma=3 & n=200 & 5.25 \\ 
  176 & MDE.Phi.tv & sigma & beta=3 & sigma=3 & n=200 & 4.76 \\ 
  177 & MDE.Phi.kl & sigma & beta=3 & sigma=3 & n=200 & 3.64 \\ 
  178 & MME & sigma & beta=3 & sigma=3 & n=200 & 4.94 \\ 
  179 & MME.b & sigma & beta=3 & sigma=3 & n=200 & 6.69 \\ 
  180 & PWM & sigma & beta=3 & sigma=3 & n=200 & 3.57 \\ 
  181 & MLE & beta & beta=4 & sigma=3 & n=200 & 5.56 \\ 
  182 & MLE.b & beta & beta=4 & sigma=3 & n=200 & 4.88 \\ 
  183 & LME & beta & beta=4 & sigma=3 & n=200 & 4.92 \\ 
  184 & MDE.Phi.chisq & beta & beta=4 & sigma=3 & n=200 & 7.48 \\ 
  185 & MDE.Phi.tv & beta & beta=4 & sigma=3 & n=200 & 6.80 \\ 
  186 & MDE.Phi.kl & beta & beta=4 & sigma=3 & n=200 & 5.25 \\ 
  187 & MME & beta & beta=4 & sigma=3 & n=200 & 6.64 \\ 
  188 & MME.b & beta & beta=4 & sigma=3 & n=200 & 13.69 \\ 
  189 & PWM & beta & beta=4 & sigma=3 & n=200 & 4.92 \\ 
  190 & MLE & sigma & beta=4 & sigma=3 & n=200 & 4.47 \\ 
  191 & MLE.b & sigma & beta=4 & sigma=3 & n=200 & 3.84 \\ 
  192 & LME & sigma & beta=4 & sigma=3 & n=200 & 3.83 \\ 
  193 & MDE.Phi.chisq & sigma & beta=4 & sigma=3 & n=200 & 8.73 \\ 
  194 & MDE.Phi.tv & sigma & beta=4 & sigma=3 & n=200 & 7.52 \\ 
  195 & MDE.Phi.kl & sigma & beta=4 & sigma=3 & n=200 & 4.15 \\ 
  196 & MME & sigma & beta=4 & sigma=3 & n=200 & 5.49 \\ 
  197 & MME.b & sigma & beta=4 & sigma=3 & n=200 & 12.38 \\ 
  198 & PWM & sigma & beta=4 & sigma=3 & n=200 & 3.83 \\ 
  199 & MLE & beta & beta=5 & sigma=3 & n=200 & 9.05 \\ 
  200 & MLE.b & beta & beta=5 & sigma=3 & n=200 & 8.34 \\ 
  201 & LME & beta & beta=5 & sigma=3 & n=200 & 6.77 \\ 
  202 & MDE.Phi.chisq & beta & beta=5 & sigma=3 & n=200 & 13.57 \\ 
  203 & MDE.Phi.tv & beta & beta=5 & sigma=3 & n=200 & 11.01 \\ 
  204 & MDE.Phi.kl & beta & beta=5 & sigma=3 & n=200 & 7.55 \\ 
  205 & MME & beta & beta=5 & sigma=3 & n=200 & 9.77 \\ 
  206 & MME.b & beta & beta=5 & sigma=3 & n=200 & 21.61 \\ 
  207 & PWM & beta & beta=5 & sigma=3 & n=200 & 6.77 \\ 
  208 & MLE & sigma & beta=5 & sigma=3 & n=200 & 5.94 \\ 
  209 & MLE.b & sigma & beta=5 & sigma=3 & n=200 & 5.44 \\ 
  210 & LME & sigma & beta=5 & sigma=3 & n=200 & 4.24 \\ 
  211 & MDE.Phi.chisq & sigma & beta=5 & sigma=3 & n=200 & 12.29 \\ 
  212 & MDE.Phi.tv & sigma & beta=5 & sigma=3 & n=200 & 9.45 \\ 
  213 & MDE.Phi.kl & sigma & beta=5 & sigma=3 & n=200 & 4.81 \\ 
  214 & MME & sigma & beta=5 & sigma=3 & n=200 & 6.40 \\ 
  215 & MME.b & sigma & beta=5 & sigma=3 & n=200 & 14.83 \\ 
  216 & PWM & sigma & beta=5 & sigma=3 & n=200 & 4.24 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220204/Output.mse.LaTeX.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Tue Feb 01 16:33:07 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=3 & n=100 & 0.46 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=3 & n=100 & 0.32 \\ 
  3 & LME & beta & beta=1.5 & sigma=3 & n=100 & 0.40 \\ 
  4 & MDE.Phi.chisq & beta & beta=1.5 & sigma=3 & n=100 & 359.08 \\ 
  5 & MDE.Phi.tv & beta & beta=1.5 & sigma=3 & n=100 & 6.29 \\ 
  6 & MDE.Phi.kl & beta & beta=1.5 & sigma=3 & n=100 & 0.46 \\ 
  7 & MME & beta & beta=1.5 & sigma=3 & n=100 & 2.57 \\ 
  8 & MME.b & beta & beta=1.5 & sigma=3 & n=100 & 130057.24 \\ 
  9 & PWM & beta & beta=1.5 & sigma=3 & n=100 & 0.40 \\ 
  10 & MLE & sigma & beta=1.5 & sigma=3 & n=100 & 4.70 \\ 
  11 & MLE.b & sigma & beta=1.5 & sigma=3 & n=100 & 3.26 \\ 
  12 & LME & sigma & beta=1.5 & sigma=3 & n=100 & 3.94 \\ 
  13 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=3 & n=100 & 178.30 \\ 
  14 & MDE.Phi.tv & sigma & beta=1.5 & sigma=3 & n=100 & 150.85 \\ 
  15 & MDE.Phi.kl & sigma & beta=1.5 & sigma=3 & n=100 & 4.71 \\ 
  16 & MME & sigma & beta=1.5 & sigma=3 & n=100 & 59.63 \\ 
  17 & MME.b & sigma & beta=1.5 & sigma=3 & n=100 & 1340192.06 \\ 
  18 & PWM & sigma & beta=1.5 & sigma=3 & n=100 & 3.94 \\ 
  19 & MLE & beta & beta=2 & sigma=3 & n=100 & 50.51 \\ 
  20 & MLE.b & beta & beta=2 & sigma=3 & n=100 & 50.26 \\ 
  21 & LME & beta & beta=2 & sigma=3 & n=100 & 3.31 \\ 
  22 & MDE.Phi.chisq & beta & beta=2 & sigma=3 & n=100 & 65.32 \\ 
  23 & MDE.Phi.tv & beta & beta=2 & sigma=3 & n=100 & 78.89 \\ 
  24 & MDE.Phi.kl & beta & beta=2 & sigma=3 & n=100 & 11.53 \\ 
  25 & MME & beta & beta=2 & sigma=3 & n=100 & 55.69 \\ 
  26 & MME.b & beta & beta=2 & sigma=3 & n=100 & 151259.47 \\ 
  27 & PWM & beta & beta=2 & sigma=3 & n=100 & 3.31 \\ 
  28 & MLE & sigma & beta=2 & sigma=3 & n=100 & 164.06 \\ 
  29 & MLE.b & sigma & beta=2 & sigma=3 & n=100 & 162.80 \\ 
  30 & LME & sigma & beta=2 & sigma=3 & n=100 & 13.82 \\ 
  31 & MDE.Phi.chisq & sigma & beta=2 & sigma=3 & n=100 & 614.56 \\ 
  32 & MDE.Phi.tv & sigma & beta=2 & sigma=3 & n=100 & 789.09 \\ 
  33 & MDE.Phi.kl & sigma & beta=2 & sigma=3 & n=100 & 43.70 \\ 
  34 & MME & sigma & beta=2 & sigma=3 & n=100 & 224.26 \\ 
  35 & MME.b & sigma & beta=2 & sigma=3 & n=100 & 752145.36 \\ 
  36 & PWM & sigma & beta=2 & sigma=3 & n=100 & 13.82 \\ 
  37 & MLE & beta & beta=2.5 & sigma=3 & n=100 & 109.07 \\ 
  38 & MLE.b & beta & beta=2.5 & sigma=3 & n=100 & 108.94 \\ 
  39 & LME & beta & beta=2.5 & sigma=3 & n=100 & 8.83 \\ 
  40 & MDE.Phi.chisq & beta & beta=2.5 & sigma=3 & n=100 & 203.79 \\ 
  41 & MDE.Phi.tv & beta & beta=2.5 & sigma=3 & n=100 & 236.10 \\ 
  42 & MDE.Phi.kl & beta & beta=2.5 & sigma=3 & n=100 & 28.69 \\ 
  43 & MME & beta & beta=2.5 & sigma=3 & n=100 & 149.68 \\ 
  44 & MME.b & beta & beta=2.5 & sigma=3 & n=100 & 2235.69 \\ 
  45 & PWM & beta & beta=2.5 & sigma=3 & n=100 & 8.83 \\ 
  46 & MLE & sigma & beta=2.5 & sigma=3 & n=100 & 279.78 \\ 
  47 & MLE.b & sigma & beta=2.5 & sigma=3 & n=100 & 279.37 \\ 
  48 & LME & sigma & beta=2.5 & sigma=3 & n=100 & 21.39 \\ 
  49 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=3 & n=100 & 1125.26 \\ 
  50 & MDE.Phi.tv & sigma & beta=2.5 & sigma=3 & n=100 & 1294.84 \\ 
  51 & MDE.Phi.kl & sigma & beta=2.5 & sigma=3 & n=100 & 70.76 \\ 
  52 & MME & sigma & beta=2.5 & sigma=3 & n=100 & 354.29 \\ 
  53 & MME.b & sigma & beta=2.5 & sigma=3 & n=100 & 5752.28 \\ 
  54 & PWM & sigma & beta=2.5 & sigma=3 & n=100 & 21.39 \\ 
  55 & MLE & beta & beta=3 & sigma=3 & n=100 & 684.54 \\ 
  56 & MLE.b & beta & beta=3 & sigma=3 & n=100 & 684.75 \\ 
  57 & LME & beta & beta=3 & sigma=3 & n=100 & 17.02 \\ 
  58 & MDE.Phi.chisq & beta & beta=3 & sigma=3 & n=100 & 441.41 \\ 
  59 & MDE.Phi.tv & beta & beta=3 & sigma=3 & n=100 & 533.17 \\ 
  60 & MDE.Phi.kl & beta & beta=3 & sigma=3 & n=100 & 95.53 \\ 
  61 & MME & beta & beta=3 & sigma=3 & n=100 & 313324.91 \\ 
  62 & MME.b & beta & beta=3 & sigma=3 & n=100 & 2979285.90 \\ 
  63 & PWM & beta & beta=3 & sigma=3 & n=100 & 17.02 \\ 
  64 & MLE & sigma & beta=3 & sigma=3 & n=100 & 1172.95 \\ 
  65 & MLE.b & sigma & beta=3 & sigma=3 & n=100 & 1173.21 \\ 
  66 & LME & sigma & beta=3 & sigma=3 & n=100 & 29.38 \\ 
  67 & MDE.Phi.chisq & sigma & beta=3 & sigma=3 & n=100 & 1598.20 \\ 
  68 & MDE.Phi.tv & sigma & beta=3 & sigma=3 & n=100 & 1885.63 \\ 
  69 & MDE.Phi.kl & sigma & beta=3 & sigma=3 & n=100 & 160.57 \\ 
  70 & MME & sigma & beta=3 & sigma=3 & n=100 & 407160.29 \\ 
  71 & MME.b & sigma & beta=3 & sigma=3 & n=100 & 3875831.90 \\ 
  72 & PWM & sigma & beta=3 & sigma=3 & n=100 & 29.38 \\ 
  73 & MLE & beta & beta=4 & sigma=3 & n=100 & 1315.51 \\ 
  74 & MLE.b & beta & beta=4 & sigma=3 & n=100 & 1316.45 \\ 
  75 & LME & beta & beta=4 & sigma=3 & n=100 & 49.52 \\ 
  76 & MDE.Phi.chisq & beta & beta=4 & sigma=3 & n=100 & 1131.14 \\ 
  77 & MDE.Phi.tv & beta & beta=4 & sigma=3 & n=100 & 1324.20 \\ 
  78 & MDE.Phi.kl & beta & beta=4 & sigma=3 & n=100 & 198.72 \\ 
  79 & MME & beta & beta=4 & sigma=3 & n=100 & 11609.73 \\ 
  80 & MME.b & beta & beta=4 & sigma=3 & n=100 & 1922332.01 \\ 
  81 & PWM & beta & beta=4 & sigma=3 & n=100 & 49.52 \\ 
  82 & MLE & sigma & beta=4 & sigma=3 & n=100 & 1104.80 \\ 
  83 & MLE.b & sigma & beta=4 & sigma=3 & n=100 & 1105.53 \\ 
  84 & LME & sigma & beta=4 & sigma=3 & n=100 & 43.43 \\ 
  85 & MDE.Phi.chisq & sigma & beta=4 & sigma=3 & n=100 & 2022.01 \\ 
  86 & MDE.Phi.tv & sigma & beta=4 & sigma=3 & n=100 & 2244.20 \\ 
  87 & MDE.Phi.kl & sigma & beta=4 & sigma=3 & n=100 & 176.25 \\ 
  88 & MME & sigma & beta=4 & sigma=3 & n=100 & 9826.84 \\ 
  89 & MME.b & sigma & beta=4 & sigma=3 & n=100 & 2436124.66 \\ 
  90 & PWM & sigma & beta=4 & sigma=3 & n=100 & 43.43 \\ 
  91 & MLE & beta & beta=5 & sigma=3 & n=100 & 2451.09 \\ 
  92 & MLE.b & beta & beta=5 & sigma=3 & n=100 & 2452.52 \\ 
  93 & LME & beta & beta=5 & sigma=3 & n=100 & 92.61 \\ 
  94 & MDE.Phi.chisq & beta & beta=5 & sigma=3 & n=100 & 1823.98 \\ 
  95 & MDE.Phi.tv & beta & beta=5 & sigma=3 & n=100 & 2004.27 \\ 
  96 & MDE.Phi.kl & beta & beta=5 & sigma=3 & n=100 & 343.50 \\ 
  97 & MME & beta & beta=5 & sigma=3 & n=100 & 18721.79 \\ 
  98 & MME.b & beta & beta=5 & sigma=3 & n=100 & 259583.10 \\ 
  99 & PWM & beta & beta=5 & sigma=3 & n=100 & 92.61 \\ 
  100 & MLE & sigma & beta=5 & sigma=3 & n=100 & 1234.08 \\ 
  101 & MLE.b & sigma & beta=5 & sigma=3 & n=100 & 1234.76 \\ 
  102 & LME & sigma & beta=5 & sigma=3 & n=100 & 46.63 \\ 
  103 & MDE.Phi.chisq & sigma & beta=5 & sigma=3 & n=100 & 1886.05 \\ 
  104 & MDE.Phi.tv & sigma & beta=5 & sigma=3 & n=100 & 1979.86 \\ 
  105 & MDE.Phi.kl & sigma & beta=5 & sigma=3 & n=100 & 171.69 \\ 
  106 & MME & sigma & beta=5 & sigma=3 & n=100 & 9397.41 \\ 
  107 & MME.b & sigma & beta=5 & sigma=3 & n=100 & 139895.14 \\ 
  108 & PWM & sigma & beta=5 & sigma=3 & n=100 & 46.63 \\ 
  109 & MLE & beta & beta=1.5 & sigma=3 & n=200 & 0.16 \\ 
  110 & MLE.b & beta & beta=1.5 & sigma=3 & n=200 & 0.09 \\ 
  111 & LME & beta & beta=1.5 & sigma=3 & n=200 & 0.15 \\ 
  112 & MDE.Phi.chisq & beta & beta=1.5 & sigma=3 & n=200 & 72.05 \\ 
  113 & MDE.Phi.tv & beta & beta=1.5 & sigma=3 & n=200 & 0.43 \\ 
  114 & MDE.Phi.kl & beta & beta=1.5 & sigma=3 & n=200 & 0.11 \\ 
  115 & MME & beta & beta=1.5 & sigma=3 & n=200 & 1.16 \\ 
  116 & MME.b & beta & beta=1.5 & sigma=3 & n=200 & 0.89 \\ 
  117 & PWM & beta & beta=1.5 & sigma=3 & n=200 & 0.15 \\ 
  118 & MLE & sigma & beta=1.5 & sigma=3 & n=200 & 1.54 \\ 
  119 & MLE.b & sigma & beta=1.5 & sigma=3 & n=200 & 0.90 \\ 
  120 & LME & sigma & beta=1.5 & sigma=3 & n=200 & 1.48 \\ 
  121 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=3 & n=200 & 13.13 \\ 
  122 & MDE.Phi.tv & sigma & beta=1.5 & sigma=3 & n=200 & 3.20 \\ 
  123 & MDE.Phi.kl & sigma & beta=1.5 & sigma=3 & n=200 & 1.03 \\ 
  124 & MME & sigma & beta=1.5 & sigma=3 & n=200 & 42.33 \\ 
  125 & MME.b & sigma & beta=1.5 & sigma=3 & n=200 & 34.99 \\ 
  126 & PWM & sigma & beta=1.5 & sigma=3 & n=200 & 1.48 \\ 
  127 & MLE & beta & beta=2 & sigma=3 & n=200 & 0.37 \\ 
  128 & MLE.b & beta & beta=2 & sigma=3 & n=200 & 0.20 \\ 
  129 & LME & beta & beta=2 & sigma=3 & n=200 & 0.35 \\ 
  130 & MDE.Phi.chisq & beta & beta=2 & sigma=3 & n=200 & 4.74 \\ 
  131 & MDE.Phi.tv & beta & beta=2 & sigma=3 & n=200 & 2.23 \\ 
  132 & MDE.Phi.kl & beta & beta=2 & sigma=3 & n=200 & 0.32 \\ 
  133 & MME & beta & beta=2 & sigma=3 & n=200 & 1.48 \\ 
  134 & MME.b & beta & beta=2 & sigma=3 & n=200 & 5.87 \\ 
  135 & PWM & beta & beta=2 & sigma=3 & n=200 & 0.35 \\ 
  136 & MLE & sigma & beta=2 & sigma=3 & n=200 & 1.64 \\ 
  137 & MLE.b & sigma & beta=2 & sigma=3 & n=200 & 0.90 \\ 
  138 & LME & sigma & beta=2 & sigma=3 & n=200 & 1.53 \\ 
  139 & MDE.Phi.chisq & sigma & beta=2 & sigma=3 & n=200 & 15.13 \\ 
  140 & MDE.Phi.tv & sigma & beta=2 & sigma=3 & n=200 & 19.45 \\ 
  141 & MDE.Phi.kl & sigma & beta=2 & sigma=3 & n=200 & 1.41 \\ 
  142 & MME & sigma & beta=2 & sigma=3 & n=200 & 9.60 \\ 
  143 & MME.b & sigma & beta=2 & sigma=3 & n=200 & 26.71 \\ 
  144 & PWM & sigma & beta=2 & sigma=3 & n=200 & 1.53 \\ 
  145 & MLE & beta & beta=2.5 & sigma=3 & n=200 & 1.53 \\ 
  146 & MLE.b & beta & beta=2.5 & sigma=3 & n=200 & 1.13 \\ 
  147 & LME & beta & beta=2.5 & sigma=3 & n=200 & 1.28 \\ 
  148 & MDE.Phi.chisq & beta & beta=2.5 & sigma=3 & n=200 & 16.19 \\ 
  149 & MDE.Phi.tv & beta & beta=2.5 & sigma=3 & n=200 & 12.59 \\ 
  150 & MDE.Phi.kl & beta & beta=2.5 & sigma=3 & n=200 & 1.18 \\ 
  151 & MME & beta & beta=2.5 & sigma=3 & n=200 & 2.90 \\ 
  152 & MME.b & beta & beta=2.5 & sigma=3 & n=200 & 44.44 \\ 
  153 & PWM & beta & beta=2.5 & sigma=3 & n=200 & 1.28 \\ 
  154 & MLE & sigma & beta=2.5 & sigma=3 & n=200 & 4.04 \\ 
  155 & MLE.b & sigma & beta=2.5 & sigma=3 & n=200 & 2.97 \\ 
  156 & LME & sigma & beta=2.5 & sigma=3 & n=200 & 3.26 \\ 
  157 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=3 & n=200 & 73.72 \\ 
  158 & MDE.Phi.tv & sigma & beta=2.5 & sigma=3 & n=200 & 55.91 \\ 
  159 & MDE.Phi.kl & sigma & beta=2.5 & sigma=3 & n=200 & 3.15 \\ 
  160 & MME & sigma & beta=2.5 & sigma=3 & n=200 & 8.65 \\ 
  161 & MME.b & sigma & beta=2.5 & sigma=3 & n=200 & 113.14 \\ 
  162 & PWM & sigma & beta=2.5 & sigma=3 & n=200 & 3.26 \\ 
  163 & MLE & beta & beta=3 & sigma=3 & n=200 & 176.07 \\ 
  164 & MLE.b & beta & beta=3 & sigma=3 & n=200 & 175.46 \\ 
  165 & LME & beta & beta=3 & sigma=3 & n=200 & 4.35 \\ 
  166 & MDE.Phi.chisq & beta & beta=3 & sigma=3 & n=200 & 79.20 \\ 
  167 & MDE.Phi.tv & beta & beta=3 & sigma=3 & n=200 & 38.54 \\ 
  168 & MDE.Phi.kl & beta & beta=3 & sigma=3 & n=200 & 7.71 \\ 
  169 & MME & beta & beta=3 & sigma=3 & n=200 & 74.99 \\ 
  170 & MME.b & beta & beta=3 & sigma=3 & n=200 & 7353.37 \\ 
  171 & PWM & beta & beta=3 & sigma=3 & n=200 & 4.35 \\ 
  172 & MLE & sigma & beta=3 & sigma=3 & n=200 & 263.26 \\ 
  173 & MLE.b & sigma & beta=3 & sigma=3 & n=200 & 262.19 \\ 
  174 & LME & sigma & beta=3 & sigma=3 & n=200 & 7.02 \\ 
  175 & MDE.Phi.chisq & sigma & beta=3 & sigma=3 & n=200 & 239.36 \\ 
  176 & MDE.Phi.tv & sigma & beta=3 & sigma=3 & n=200 & 108.60 \\ 
  177 & MDE.Phi.kl & sigma & beta=3 & sigma=3 & n=200 & 12.40 \\ 
  178 & MME & sigma & beta=3 & sigma=3 & n=200 & 110.52 \\ 
  179 & MME.b & sigma & beta=3 & sigma=3 & n=200 & 15145.57 \\ 
  180 & PWM & sigma & beta=3 & sigma=3 & n=200 & 7.02 \\ 
  181 & MLE & beta & beta=4 & sigma=3 & n=200 & 161.25 \\ 
  182 & MLE.b & beta & beta=4 & sigma=3 & n=200 & 161.03 \\ 
  183 & LME & beta & beta=4 & sigma=3 & n=200 & 18.29 \\ 
  184 & MDE.Phi.chisq & beta & beta=4 & sigma=3 & n=200 & 418.95 \\ 
  185 & MDE.Phi.tv & beta & beta=4 & sigma=3 & n=200 & 314.56 \\ 
  186 & MDE.Phi.kl & beta & beta=4 & sigma=3 & n=200 & 40.16 \\ 
  187 & MME & beta & beta=4 & sigma=3 & n=200 & 551.00 \\ 
  188 & MME.b & beta & beta=4 & sigma=3 & n=200 & 40296.91 \\ 
  189 & PWM & beta & beta=4 & sigma=3 & n=200 & 18.29 \\ 
  190 & MLE & sigma & beta=4 & sigma=3 & n=200 & 143.09 \\ 
  191 & MLE.b & sigma & beta=4 & sigma=3 & n=200 & 142.85 \\ 
  192 & LME & sigma & beta=4 & sigma=3 & n=200 & 15.43 \\ 
  193 & MDE.Phi.chisq & sigma & beta=4 & sigma=3 & n=200 & 630.61 \\ 
  194 & MDE.Phi.tv & sigma & beta=4 & sigma=3 & n=200 & 458.72 \\ 
  195 & MDE.Phi.kl & sigma & beta=4 & sigma=3 & n=200 & 34.24 \\ 
  196 & MME & sigma & beta=4 & sigma=3 & n=200 & 480.75 \\ 
  197 & MME.b & sigma & beta=4 & sigma=3 & n=200 & 44568.02 \\ 
  198 & PWM & sigma & beta=4 & sigma=3 & n=200 & 15.43 \\ 
  199 & MLE & beta & beta=5 & sigma=3 & n=200 & 2989.73 \\ 
  200 & MLE.b & beta & beta=5 & sigma=3 & n=200 & 2990.57 \\ 
  201 & LME & beta & beta=5 & sigma=3 & n=200 & 63.80 \\ 
  202 & MDE.Phi.chisq & beta & beta=5 & sigma=3 & n=200 & 1064.11 \\ 
  203 & MDE.Phi.tv & beta & beta=5 & sigma=3 & n=200 & 706.91 \\ 
  204 & MDE.Phi.kl & beta & beta=5 & sigma=3 & n=200 & 130.30 \\ 
  205 & MME & beta & beta=5 & sigma=3 & n=200 & 2746.12 \\ 
  206 & MME.b & beta & beta=5 & sigma=3 & n=200 & 30989.31 \\ 
  207 & PWM & beta & beta=5 & sigma=3 & n=200 & 63.80 \\ 
  208 & MLE & sigma & beta=5 & sigma=3 & n=200 & 1604.43 \\ 
  209 & MLE.b & sigma & beta=5 & sigma=3 & n=200 & 1604.81 \\ 
  210 & LME & sigma & beta=5 & sigma=3 & n=200 & 32.36 \\ 
  211 & MDE.Phi.chisq & sigma & beta=5 & sigma=3 & n=200 & 939.58 \\ 
  212 & MDE.Phi.tv & sigma & beta=5 & sigma=3 & n=200 & 590.42 \\ 
  213 & MDE.Phi.kl & sigma & beta=5 & sigma=3 & n=200 & 65.65 \\ 
  214 & MME & sigma & beta=5 & sigma=3 & n=200 & 1343.84 \\ 
  215 & MME.b & sigma & beta=5 & sigma=3 & n=200 & 15775.95 \\ 
  216 & PWM & sigma & beta=5 & sigma=3 & n=200 & 32.36 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220204/Output.var.LaTeX.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Tue Feb 01 16:33:07 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=3 & n=100 & 0.44 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=3 & n=100 & 0.32 \\ 
  3 & LME & beta & beta=1.5 & sigma=3 & n=100 & 0.30 \\ 
  4 & MDE.Phi.chisq & beta & beta=1.5 & sigma=3 & n=100 & 347.78 \\ 
  5 & MDE.Phi.tv & beta & beta=1.5 & sigma=3 & n=100 & 6.22 \\ 
  6 & MDE.Phi.kl & beta & beta=1.5 & sigma=3 & n=100 & 0.44 \\ 
  7 & MME & beta & beta=1.5 & sigma=3 & n=100 & 0.90 \\ 
  8 & MME.b & beta & beta=1.5 & sigma=3 & n=100 & 130047.07 \\ 
  9 & PWM & beta & beta=1.5 & sigma=3 & n=100 & 0.30 \\ 
  10 & MLE & sigma & beta=1.5 & sigma=3 & n=100 & 4.40 \\ 
  11 & MLE.b & sigma & beta=1.5 & sigma=3 & n=100 & 3.25 \\ 
  12 & LME & sigma & beta=1.5 & sigma=3 & n=100 & 2.99 \\ 
  13 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=3 & n=100 & 173.39 \\ 
  14 & MDE.Phi.tv & sigma & beta=1.5 & sigma=3 & n=100 & 144.67 \\ 
  15 & MDE.Phi.kl & sigma & beta=1.5 & sigma=3 & n=100 & 4.41 \\ 
  16 & MME & sigma & beta=1.5 & sigma=3 & n=100 & 17.93 \\ 
  17 & MME.b & sigma & beta=1.5 & sigma=3 & n=100 & 1340019.71 \\ 
  18 & PWM & sigma & beta=1.5 & sigma=3 & n=100 & 2.99 \\ 
  19 & MLE & beta & beta=2 & sigma=3 & n=100 & 50.24 \\ 
  20 & MLE.b & beta & beta=2 & sigma=3 & n=100 & 50.23 \\ 
  21 & LME & beta & beta=2 & sigma=3 & n=100 & 3.11 \\ 
  22 & MDE.Phi.chisq & beta & beta=2 & sigma=3 & n=100 & 65.32 \\ 
  23 & MDE.Phi.tv & beta & beta=2 & sigma=3 & n=100 & 78.47 \\ 
  24 & MDE.Phi.kl & beta & beta=2 & sigma=3 & n=100 & 11.32 \\ 
  25 & MME & beta & beta=2 & sigma=3 & n=100 & 52.88 \\ 
  26 & MME.b & beta & beta=2 & sigma=3 & n=100 & 151218.71 \\ 
  27 & PWM & beta & beta=2 & sigma=3 & n=100 & 3.11 \\ 
  28 & MLE & sigma & beta=2 & sigma=3 & n=100 & 162.89 \\ 
  29 & MLE.b & sigma & beta=2 & sigma=3 & n=100 & 162.71 \\ 
  30 & LME & sigma & beta=2 & sigma=3 & n=100 & 13.01 \\ 
  31 & MDE.Phi.chisq & sigma & beta=2 & sigma=3 & n=100 & 604.20 \\ 
  32 & MDE.Phi.tv & sigma & beta=2 & sigma=3 & n=100 & 766.97 \\ 
  33 & MDE.Phi.kl & sigma & beta=2 & sigma=3 & n=100 & 42.77 \\ 
  34 & MME & sigma & beta=2 & sigma=3 & n=100 & 205.69 \\ 
  35 & MME.b & sigma & beta=2 & sigma=3 & n=100 & 751939.67 \\ 
  36 & PWM & sigma & beta=2 & sigma=3 & n=100 & 13.01 \\ 
  37 & MLE & beta & beta=2.5 & sigma=3 & n=100 & 107.96 \\ 
  38 & MLE.b & beta & beta=2.5 & sigma=3 & n=100 & 108.59 \\ 
  39 & LME & beta & beta=2.5 & sigma=3 & n=100 & 8.34 \\ 
  40 & MDE.Phi.chisq & beta & beta=2.5 & sigma=3 & n=100 & 201.51 \\ 
  41 & MDE.Phi.tv & beta & beta=2.5 & sigma=3 & n=100 & 230.70 \\ 
  42 & MDE.Phi.kl & beta & beta=2.5 & sigma=3 & n=100 & 27.83 \\ 
  43 & MME & beta & beta=2.5 & sigma=3 & n=100 & 144.30 \\ 
  44 & MME.b & beta & beta=2.5 & sigma=3 & n=100 & 2205.73 \\ 
  45 & PWM & beta & beta=2.5 & sigma=3 & n=100 & 8.34 \\ 
  46 & MLE & sigma & beta=2.5 & sigma=3 & n=100 & 276.90 \\ 
  47 & MLE.b & sigma & beta=2.5 & sigma=3 & n=100 & 278.47 \\ 
  48 & LME & sigma & beta=2.5 & sigma=3 & n=100 & 20.24 \\ 
  49 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=3 & n=100 & 1089.17 \\ 
  50 & MDE.Phi.tv & sigma & beta=2.5 & sigma=3 & n=100 & 1237.72 \\ 
  51 & MDE.Phi.kl & sigma & beta=2.5 & sigma=3 & n=100 & 68.52 \\ 
  52 & MME & sigma & beta=2.5 & sigma=3 & n=100 & 337.82 \\ 
  53 & MME.b & sigma & beta=2.5 & sigma=3 & n=100 & 5670.67 \\ 
  54 & PWM & sigma & beta=2.5 & sigma=3 & n=100 & 20.24 \\ 
  55 & MLE & beta & beta=3 & sigma=3 & n=100 & 677.87 \\ 
  56 & MLE.b & beta & beta=3 & sigma=3 & n=100 & 680.40 \\ 
  57 & LME & beta & beta=3 & sigma=3 & n=100 & 15.99 \\ 
  58 & MDE.Phi.chisq & beta & beta=3 & sigma=3 & n=100 & 428.37 \\ 
  59 & MDE.Phi.tv & beta & beta=3 & sigma=3 & n=100 & 508.61 \\ 
  60 & MDE.Phi.kl & beta & beta=3 & sigma=3 & n=100 & 92.20 \\ 
  61 & MME & beta & beta=3 & sigma=3 & n=100 & 313146.34 \\ 
  62 & MME.b & beta & beta=3 & sigma=3 & n=100 & 2977375.61 \\ 
  63 & PWM & beta & beta=3 & sigma=3 & n=100 & 15.99 \\ 
  64 & MLE & sigma & beta=3 & sigma=3 & n=100 & 1161.82 \\ 
  65 & MLE.b & sigma & beta=3 & sigma=3 & n=100 & 1165.96 \\ 
  66 & LME & sigma & beta=3 & sigma=3 & n=100 & 27.75 \\ 
  67 & MDE.Phi.chisq & sigma & beta=3 & sigma=3 & n=100 & 1517.48 \\ 
  68 & MDE.Phi.tv & sigma & beta=3 & sigma=3 & n=100 & 1763.67 \\ 
  69 & MDE.Phi.kl & sigma & beta=3 & sigma=3 & n=100 & 154.99 \\ 
  70 & MME & sigma & beta=3 & sigma=3 & n=100 & 406904.26 \\ 
  71 & MME.b & sigma & beta=3 & sigma=3 & n=100 & 3873116.01 \\ 
  72 & PWM & sigma & beta=3 & sigma=3 & n=100 & 27.75 \\ 
  73 & MLE & beta & beta=4 & sigma=3 & n=100 & 1294.79 \\ 
  74 & MLE.b & beta & beta=4 & sigma=3 & n=100 & 1299.63 \\ 
  75 & LME & beta & beta=4 & sigma=3 & n=100 & 46.48 \\ 
  76 & MDE.Phi.chisq & beta & beta=4 & sigma=3 & n=100 & 1047.10 \\ 
  77 & MDE.Phi.tv & beta & beta=4 & sigma=3 & n=100 & 1197.43 \\ 
  78 & MDE.Phi.kl & beta & beta=4 & sigma=3 & n=100 & 187.37 \\ 
  79 & MME & beta & beta=4 & sigma=3 & n=100 & 11556.83 \\ 
  80 & MME.b & beta & beta=4 & sigma=3 & n=100 & 1921162.10 \\ 
  81 & PWM & beta & beta=4 & sigma=3 & n=100 & 46.48 \\ 
  82 & MLE & sigma & beta=4 & sigma=3 & n=100 & 1086.97 \\ 
  83 & MLE.b & sigma & beta=4 & sigma=3 & n=100 & 1091.00 \\ 
  84 & LME & sigma & beta=4 & sigma=3 & n=100 & 40.89 \\ 
  85 & MDE.Phi.chisq & sigma & beta=4 & sigma=3 & n=100 & 1826.95 \\ 
  86 & MDE.Phi.tv & sigma & beta=4 & sigma=3 & n=100 & 1987.70 \\ 
  87 & MDE.Phi.kl & sigma & beta=4 & sigma=3 & n=100 & 166.42 \\ 
  88 & MME & sigma & beta=4 & sigma=3 & n=100 & 9778.87 \\ 
  89 & MME.b & sigma & beta=4 & sigma=3 & n=100 & 2434977.11 \\ 
  90 & PWM & sigma & beta=4 & sigma=3 & n=100 & 40.89 \\ 
  91 & MLE & beta & beta=5 & sigma=3 & n=100 & 2400.47 \\ 
  92 & MLE.b & beta & beta=5 & sigma=3 & n=100 & 2407.02 \\ 
  93 & LME & beta & beta=5 & sigma=3 & n=100 & 87.33 \\ 
  94 & MDE.Phi.chisq & beta & beta=5 & sigma=3 & n=100 & 1624.25 \\ 
  95 & MDE.Phi.tv & beta & beta=5 & sigma=3 & n=100 & 1742.16 \\ 
  96 & MDE.Phi.kl & beta & beta=5 & sigma=3 & n=100 & 319.00 \\ 
  97 & MME & beta & beta=5 & sigma=3 & n=100 & 18586.56 \\ 
  98 & MME.b & beta & beta=5 & sigma=3 & n=100 & 257834.84 \\ 
  99 & PWM & beta & beta=5 & sigma=3 & n=100 & 87.33 \\ 
  100 & MLE & sigma & beta=5 & sigma=3 & n=100 & 1208.85 \\ 
  101 & MLE.b & sigma & beta=5 & sigma=3 & n=100 & 1212.06 \\ 
  102 & LME & sigma & beta=5 & sigma=3 & n=100 & 44.04 \\ 
  103 & MDE.Phi.chisq & sigma & beta=5 & sigma=3 & n=100 & 1635.55 \\ 
  104 & MDE.Phi.tv & sigma & beta=5 & sigma=3 & n=100 & 1683.51 \\ 
  105 & MDE.Phi.kl & sigma & beta=5 & sigma=3 & n=100 & 159.47 \\ 
  106 & MME & sigma & beta=5 & sigma=3 & n=100 & 9330.58 \\ 
  107 & MME.b & sigma & beta=5 & sigma=3 & n=100 & 139016.87 \\ 
  108 & PWM & sigma & beta=5 & sigma=3 & n=100 & 44.04 \\ 
  109 & MLE & beta & beta=1.5 & sigma=3 & n=200 & 0.10 \\ 
  110 & MLE.b & beta & beta=1.5 & sigma=3 & n=200 & 0.08 \\ 
  111 & LME & beta & beta=1.5 & sigma=3 & n=200 & 0.11 \\ 
  112 & MDE.Phi.chisq & beta & beta=1.5 & sigma=3 & n=200 & 70.32 \\ 
  113 & MDE.Phi.tv & beta & beta=1.5 & sigma=3 & n=200 & 0.18 \\ 
  114 & MDE.Phi.kl & beta & beta=1.5 & sigma=3 & n=200 & 0.10 \\ 
  115 & MME & beta & beta=1.5 & sigma=3 & n=200 & 0.16 \\ 
  116 & MME.b & beta & beta=1.5 & sigma=3 & n=200 & 0.26 \\ 
  117 & PWM & beta & beta=1.5 & sigma=3 & n=200 & 0.11 \\ 
  118 & MLE & sigma & beta=1.5 & sigma=3 & n=200 & 1.03 \\ 
  119 & MLE.b & sigma & beta=1.5 & sigma=3 & n=200 & 0.74 \\ 
  120 & LME & sigma & beta=1.5 & sigma=3 & n=200 & 1.11 \\ 
  121 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=3 & n=200 & 12.71 \\ 
  122 & MDE.Phi.tv & sigma & beta=1.5 & sigma=3 & n=200 & 2.60 \\ 
  123 & MDE.Phi.kl & sigma & beta=1.5 & sigma=3 & n=200 & 0.97 \\ 
  124 & MME & sigma & beta=1.5 & sigma=3 & n=200 & 13.64 \\ 
  125 & MME.b & sigma & beta=1.5 & sigma=3 & n=200 & 14.48 \\ 
  126 & PWM & sigma & beta=1.5 & sigma=3 & n=200 & 1.11 \\ 
  127 & MLE & beta & beta=2 & sigma=3 & n=200 & 0.30 \\ 
  128 & MLE.b & beta & beta=2 & sigma=3 & n=200 & 0.20 \\ 
  129 & LME & beta & beta=2 & sigma=3 & n=200 & 0.30 \\ 
  130 & MDE.Phi.chisq & beta & beta=2 & sigma=3 & n=200 & 4.29 \\ 
  131 & MDE.Phi.tv & beta & beta=2 & sigma=3 & n=200 & 2.03 \\ 
  132 & MDE.Phi.kl & beta & beta=2 & sigma=3 & n=200 & 0.30 \\ 
  133 & MME & beta & beta=2 & sigma=3 & n=200 & 0.53 \\ 
  134 & MME.b & beta & beta=2 & sigma=3 & n=200 & 5.40 \\ 
  135 & PWM & beta & beta=2 & sigma=3 & n=200 & 0.30 \\ 
  136 & MLE & sigma & beta=2 & sigma=3 & n=200 & 1.37 \\ 
  137 & MLE.b & sigma & beta=2 & sigma=3 & n=200 & 0.89 \\ 
  138 & LME & sigma & beta=2 & sigma=3 & n=200 & 1.35 \\ 
  139 & MDE.Phi.chisq & sigma & beta=2 & sigma=3 & n=200 & 14.86 \\ 
  140 & MDE.Phi.tv & sigma & beta=2 & sigma=3 & n=200 & 18.76 \\ 
  141 & MDE.Phi.kl & sigma & beta=2 & sigma=3 & n=200 & 1.32 \\ 
  142 & MME & sigma & beta=2 & sigma=3 & n=200 & 2.50 \\ 
  143 & MME.b & sigma & beta=2 & sigma=3 & n=200 & 22.95 \\ 
  144 & PWM & sigma & beta=2 & sigma=3 & n=200 & 1.35 \\ 
  145 & MLE & beta & beta=2.5 & sigma=3 & n=200 & 1.41 \\ 
  146 & MLE.b & beta & beta=2.5 & sigma=3 & n=200 & 1.13 \\ 
  147 & LME & beta & beta=2.5 & sigma=3 & n=200 & 1.20 \\ 
  148 & MDE.Phi.chisq & beta & beta=2.5 & sigma=3 & n=200 & 15.99 \\ 
  149 & MDE.Phi.tv & beta & beta=2.5 & sigma=3 & n=200 & 12.54 \\ 
  150 & MDE.Phi.kl & beta & beta=2.5 & sigma=3 & n=200 & 1.12 \\ 
  151 & MME & beta & beta=2.5 & sigma=3 & n=200 & 1.77 \\ 
  152 & MME.b & beta & beta=2.5 & sigma=3 & n=200 & 43.75 \\ 
  153 & PWM & beta & beta=2.5 & sigma=3 & n=200 & 1.20 \\ 
  154 & MLE & sigma & beta=2.5 & sigma=3 & n=200 & 3.73 \\ 
  155 & MLE.b & sigma & beta=2.5 & sigma=3 & n=200 & 2.97 \\ 
  156 & LME & sigma & beta=2.5 & sigma=3 & n=200 & 3.07 \\ 
  157 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=3 & n=200 & 72.66 \\ 
  158 & MDE.Phi.tv & sigma & beta=2.5 & sigma=3 & n=200 & 54.46 \\ 
  159 & MDE.Phi.kl & sigma & beta=2.5 & sigma=3 & n=200 & 2.98 \\ 
  160 & MME & sigma & beta=2.5 & sigma=3 & n=200 & 4.79 \\ 
  161 & MME.b & sigma & beta=2.5 & sigma=3 & n=200 & 110.84 \\ 
  162 & PWM & sigma & beta=2.5 & sigma=3 & n=200 & 3.07 \\ 
  163 & MLE & beta & beta=3 & sigma=3 & n=200 & 175.57 \\ 
  164 & MLE.b & beta & beta=3 & sigma=3 & n=200 & 175.42 \\ 
  165 & LME & beta & beta=3 & sigma=3 & n=200 & 4.14 \\ 
  166 & MDE.Phi.chisq & beta & beta=3 & sigma=3 & n=200 & 79.14 \\ 
  167 & MDE.Phi.tv & beta & beta=3 & sigma=3 & n=200 & 38.50 \\ 
  168 & MDE.Phi.kl & beta & beta=3 & sigma=3 & n=200 & 7.46 \\ 
  169 & MME & beta & beta=3 & sigma=3 & n=200 & 73.03 \\ 
  170 & MME.b & beta & beta=3 & sigma=3 & n=200 & 7346.85 \\ 
  171 & PWM & beta & beta=3 & sigma=3 & n=200 & 4.14 \\ 
  172 & MLE & sigma & beta=3 & sigma=3 & n=200 & 262.43 \\ 
  173 & MLE.b & sigma & beta=3 & sigma=3 & n=200 & 262.12 \\ 
  174 & LME & sigma & beta=3 & sigma=3 & n=200 & 6.70 \\ 
  175 & MDE.Phi.chisq & sigma & beta=3 & sigma=3 & n=200 & 234.32 \\ 
  176 & MDE.Phi.tv & sigma & beta=3 & sigma=3 & n=200 & 105.50 \\ 
  177 & MDE.Phi.kl & sigma & beta=3 & sigma=3 & n=200 & 12.00 \\ 
  178 & MME & sigma & beta=3 & sigma=3 & n=200 & 106.77 \\ 
  179 & MME.b & sigma & beta=3 & sigma=3 & n=200 & 15133.43 \\ 
  180 & PWM & sigma & beta=3 & sigma=3 & n=200 & 6.70 \\ 
  181 & MLE & beta & beta=4 & sigma=3 & n=200 & 158.83 \\ 
  182 & MLE.b & beta & beta=4 & sigma=3 & n=200 & 160.28 \\ 
  183 & LME & beta & beta=4 & sigma=3 & n=200 & 17.45 \\ 
  184 & MDE.Phi.chisq & beta & beta=4 & sigma=3 & n=200 & 406.85 \\ 
  185 & MDE.Phi.tv & beta & beta=4 & sigma=3 & n=200 & 306.74 \\ 
  186 & MDE.Phi.kl & beta & beta=4 & sigma=3 & n=200 & 38.60 \\ 
  187 & MME & beta & beta=4 & sigma=3 & n=200 & 544.10 \\ 
  188 & MME.b & beta & beta=4 & sigma=3 & n=200 & 40207.11 \\ 
  189 & PWM & beta & beta=4 & sigma=3 & n=200 & 17.45 \\ 
  190 & MLE & sigma & beta=4 & sigma=3 & n=200 & 140.93 \\ 
  191 & MLE.b & sigma & beta=4 & sigma=3 & n=200 & 142.15 \\ 
  192 & LME & sigma & beta=4 & sigma=3 & n=200 & 14.74 \\ 
  193 & MDE.Phi.chisq & sigma & beta=4 & sigma=3 & n=200 & 597.79 \\ 
  194 & MDE.Phi.tv & sigma & beta=4 & sigma=3 & n=200 & 438.33 \\ 
  195 & MDE.Phi.kl & sigma & beta=4 & sigma=3 & n=200 & 32.91 \\ 
  196 & MME & sigma & beta=4 & sigma=3 & n=200 & 474.58 \\ 
  197 & MME.b & sigma & beta=4 & sigma=3 & n=200 & 44484.42 \\ 
  198 & PWM & sigma & beta=4 & sigma=3 & n=200 & 14.74 \\ 
  199 & MLE & beta & beta=5 & sigma=3 & n=200 & 2973.65 \\ 
  200 & MLE.b & beta & beta=5 & sigma=3 & n=200 & 2979.74 \\ 
  201 & LME & beta & beta=5 & sigma=3 & n=200 & 60.69 \\ 
  202 & MDE.Phi.chisq & beta & beta=5 & sigma=3 & n=200 & 990.75 \\ 
  203 & MDE.Phi.tv & beta & beta=5 & sigma=3 & n=200 & 670.90 \\ 
  204 & MDE.Phi.kl & beta & beta=5 & sigma=3 & n=200 & 123.78 \\ 
  205 & MME & beta & beta=5 & sigma=3 & n=200 & 2723.68 \\ 
  206 & MME.b & beta & beta=5 & sigma=3 & n=200 & 30716.43 \\ 
  207 & PWM & beta & beta=5 & sigma=3 & n=200 & 60.69 \\ 
  208 & MLE & sigma & beta=5 & sigma=3 & n=200 & 1595.94 \\ 
  209 & MLE.b & sigma & beta=5 & sigma=3 & n=200 & 1599.04 \\ 
  210 & LME & sigma & beta=5 & sigma=3 & n=200 & 30.83 \\ 
  211 & MDE.Phi.chisq & sigma & beta=5 & sigma=3 & n=200 & 853.36 \\ 
  212 & MDE.Phi.tv & sigma & beta=5 & sigma=3 & n=200 & 548.91 \\ 
  213 & MDE.Phi.kl & sigma & beta=5 & sigma=3 & n=200 & 62.38 \\ 
  214 & MME & sigma & beta=5 & sigma=3 & n=200 & 1332.40 \\ 
  215 & MME.b & sigma & beta=5 & sigma=3 & n=200 & 15637.60 \\ 
  216 & PWM & sigma & beta=5 & sigma=3 & n=200 & 30.83 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220207/20220208-11h06-Full.beta=1.5.sig=1.n=100.LaTeX.tex <==
% START DATE AND TIME=20220208-11h06
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=1.5,  \sigma=1$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.6717&1.4777&1.8288&0.9856&1.2647&1.6717&2.7927&6.3149&1.8288
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.1822&0.9774&1.3253&1.5496&1.8315&1.1823&3.1525&6.8343&1.3253
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.4353&0.3215&0.2958&12.6553&8.0716&0.4353&0.8967&130047.0683&0.2958
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.4896&0.3616&0.3325&22.0969&21.1246&0.4898&1.9924&148891.0805&0.3325
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1717&-0.0223&0.3288&-0.5144&-0.2353&0.1717&1.2927&4.8149&0.3288
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.1822&-0.0226&0.3253&0.5496&0.8315&0.1823&2.1525&5.8343&0.3253
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.4647&0.322&0.4039&12.9187&8.1262&0.4648&2.5678&130057.2467&0.4039
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.5228&0.3621&0.4383&22.3968&21.8139&0.523&6.6253&148910.2304&0.4383
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 0.9875&0.6841&0.8422&35.3154&29.9401&0.9877&9.1931&278967.4771&0.8422\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0011&0.0011&1.81787018350624e+299&0.0349&0.0011&0.0099&7.105&0.0011\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220207/20220208-11h06-Full.beta=1.5.sig=1.n=200.LaTeX.tex <==
% START DATE AND TIME=20220208-11h06
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=1.5,  \sigma=1$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.5782&1.4954&1.7056&0.8492&1.005&1.5782&2.495&2.296&1.7056
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.0818&0.9949&1.2029&1.1239&1.2543&1.0818&2.7893&2.514&1.2029
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1022&0.0773&0.1121&0.1223&0.1688&0.1022&0.1646&0.258&0.1121
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.1092&0.081&0.1242&0.2226&0.2908&0.1092&1.7813&1.8685&0.1242
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.0782&-0.0046&0.2056&-0.6508&-0.495&0.0782&0.995&0.796&0.2056
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.0818&-0.0051&0.2029&0.1239&0.2543&0.0818&1.7893&1.514&0.2029
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1083&0.0773&0.1544&0.5458&0.4138&0.1083&1.1547&0.8917&0.1544
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.1159&0.0811&0.1654&0.238&0.3554&0.1159&4.9829&4.1604&0.1654
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 0.2242&0.1584&0.3197&0.7838&0.7692&0.2242&6.1376&5.0521&0.3197\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 6e-04&6e-04&6e-04&0.0346&0.0271&6e-04&0.0089&0.0103&6e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220207/20220208-11h06-Full.beta=2.5.sig=1.n=100.LaTeX.tex <==
% START DATE AND TIME=20220208-11h06
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2.5,  \sigma=1$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 4.9476&4.4903&3.1958&4.3081&5.1489&3.4521&4.8214&7.9937&3.1958
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2.3219&2.0741&1.3592&3.2275&3.7662&1.5109&2.3544&4.0216&1.3592
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 10477.4379&10479.3418&8.3445&278.8&316.2569&34.0267&144.3027&2205.727&8.3445
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
3098.2823&3098.8302&2.2484&166.8837&188.2544&9.3086&37.5351&630.075&2.2484
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.4476&1.9903&0.6958&1.8081&2.6489&0.9521&2.3214&5.4937&0.6958
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.3219&1.0741&0.3592&2.2275&2.7662&0.5109&1.3544&3.0216&0.3592
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 10482.3807&10482.2552&8.8279&282.0412&323.2418&34.9299&149.6771&2235.6866&8.8279
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
3099.7197&3099.674&2.3772&171.8288&195.8876&9.5687&39.3658&639.1419&2.3772
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 13582.1004&13581.9292&11.2051&453.8699&519.1293&44.4986&189.0429&2874.8285&11.2051\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0012&0.0011&0.0233&0.0178&0.0011&0.0019&8.078&0.0011\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220207/20220208-11h06-Full.beta=2.5.sig=1.n=200.LaTeX.tex <==
% START DATE AND TIME=20220208-11h06
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2.5,  \sigma=1$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.7517&2.447&2.7839&2.0647&2.2867&2.7517&3.5621&3.3352&2.7839
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.1356&0.9708&1.1446&1.3611&1.411&1.1356&1.6546&1.5066&1.1446
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.1167&0.8305&1.1971&22.0676&16.6289&1.1166&1.774&43.7477&1.1971
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.3315&0.2473&0.3407&11.1329&7.9925&0.3315&0.5323&12.3153&0.3407
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.2517&-0.053&0.2839&-0.4353&-0.2133&0.2517&1.0621&0.8352&0.2839
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.1356&-0.0292&0.1446&0.3611&0.411&0.1356&0.6546&0.5066&0.1446
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.1799&0.8332&1.2776&22.2549&16.6727&1.1799&2.9019&44.4409&1.2776
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.3499&0.2482&0.3616&11.2622&8.1606&0.3499&0.9608&12.5708&0.3616
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 1.5298&1.0814&1.6392&33.5171&24.8333&1.5297&3.8627&57.0117&1.6392\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&5e-04&5e-04&0.0174&0.0121&5e-04&0.0011&0.0017&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220207/20220208-11h06-Full.beta=2.sig=1.n=100.LaTeX.tex <==
% START DATE AND TIME=20220208-11h06
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2,  \sigma=1$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 3.2019&2.8522&2.4461&2.1496&2.768&2.465&3.6775&9.4751&2.4461
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.747&1.4944&1.3016&2.1521&2.6841&1.3282&2.4373&6.5865&1.3016
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 4900.5952&4901.0608&3.1121&79.2502&106.4853&14.1658&52.8831&151218.7131&3.1121
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1541.2596&1541.4336&1.445&90.4215&115.3987&5.9178&22.8539&83548.852&1.445
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.2019&0.8522&0.4461&0.1496&0.768&0.465&1.6775&7.4751&0.4461
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.747&0.4944&0.3016&1.1521&1.6841&0.3282&1.4373&5.5865&0.3016
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 4901.5497&4901.2969&3.3109&79.2647&107.0645&14.3806&55.6919&151259.4685&3.3109
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1541.6634&1541.5239&1.5359&91.7397&118.2232&6.0249&24.9175&83571.7065&1.5359
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 6443.2131&6442.8208&4.8467&171.0044&225.2877&20.4055&80.6095&234831.175&4.8467\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0011&0.0011&0.0291&0.0229&0.0011&0.0035&0.0115&0.0011\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220207/20220208-11h06-Full.beta=2.sig=1.n=200.LaTeX.tex <==
% START DATE AND TIME=20220208-11h06
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2,  \sigma=1$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.1373&1.9682&2.2157&1.3484&1.5649&2.1373&2.9722&2.6877&2.2157
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.0964&0.9754&1.1419&1.1731&1.2796&1.0964&1.8886&1.6465&1.1419
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.2965&0.1915&0.3034&2.6102&2.5953&0.2965&0.5321&5.3987&0.3034
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.147&0.0935&0.1498&2.1169&2.7239&0.147&0.2778&2.5505&0.1498
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1373&-0.0318&0.2157&-0.6516&-0.4351&0.1373&0.9722&0.6877&0.2157
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.0964&-0.0246&0.1419&0.1731&0.2796&0.0964&0.8886&0.6465&0.1419
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.3153&0.1925&0.3499&3.0345&2.7844&0.3153&1.4772&5.8711&0.3499
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.1562&0.0941&0.1699&2.1466&2.8018&0.1563&1.0673&2.9682&0.1699
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 0.4715&0.2866&0.5198&5.1811&5.5862&0.4715&2.5445&8.8394&0.5198\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&5e-04&5e-04&0.0226&0.0164&5e-04&0.0024&0.0024&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220207/20220208-11h06-Full.beta=3.sig=1.n=100.LaTeX.tex <==
% START DATE AND TIME=20220208-11h06
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=3,  \sigma=1$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 13.4515&12.9573&4.0159&7.279&8.7601&4.9247&17.4875&49.9897&4.0159
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
5.5634&5.3499&1.4255&4.4093&5.1734&1.8285&6.7418&19.5688&1.4255
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 67534.2993&67544.5892&15.9909&606.1818&721.51&120.2505&$3.131\times10^5$&$2.977\times10^6$&15.9909
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
13715.9368&13717.8682&3.0834&238.2619&277.2428&22.264&45211.5846&430346.239&3.0834
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 10.4515&9.9573&1.0159&4.279&5.7601&1.9247&14.4875&46.9897&1.0159
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
4.5634&4.3499&0.4255&3.4093&4.1734&0.8285&5.7418&18.5688&0.4255
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & $6.764\times10^4$&$6.764\times10^4$&17.0213&624.4312&754.6165&123.9428&$3.133\times10^5$24.9101&$2.979\times10^6$&17.0213
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
$1.374\times10^4$&$1.374\times10^4$&3.2641&249.8612&294.6323&22.9483&45240.0317&$4.306\times10^5$&3.2641
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & $8.137\times10^4$&$8137\times10^4$&20.2855&874.2924&1049.2488&146.8911&$3.586\times10^5$&$3.410\time10^7$&20.2855\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0012&0.0011&0.02&0.0152&0.0011&0.0014&0.0075&0.0011\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220207/20220208-11h06-Full.beta=3.sig=1.n=200.LaTeX.tex <==
% START DATE AND TIME=20220208-11h06
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=3,  \sigma=1$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 3.5549&3.0903&3.4536&3.382&3.2394&3.4946&4.4031&5.6933&3.4536
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.2377&1.0366&1.1893&1.8153&1.6143&1.2137&1.6462&2.2317&1.1893
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 64.3917&64.1342&4.1441&111.0688&52.0856&8.3477&73.0305&7346.8537&4.1441
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
10.3835&10.3317&0.7446&36.5505&15.8832&1.4733&11.8636&1681.4932&0.7446
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.5549&0.0903&0.4536&0.382&0.2394&0.4946&1.4031&2.6933&0.4536
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.2377&0.0366&0.1893&0.8153&0.6143&0.2137&0.6462&1.2317&0.1893
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 64.6931&64.1359&4.3494&111.2036&52.1377&8.5915&74.9919&7353.3729&4.3494
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
10.439&10.332&0.7803&37.2115&16.259&1.5188&12.2801&1682.8422&0.7803
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 75.1321&74.4679&5.1297&148.4151&68.3966&10.1102&87.272&9036.2151&5.1297\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&5e-04&5e-04&0.0143&0.0096&5e-04&7e-04&0.0018&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220207/20220208-11h06-Full.beta=4.sig=1.n=100.LaTeX.tex <==
% START DATE AND TIME=20220208-11h06
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=4,  \sigma=1$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 19.056&18.6069&5.759&14.9157&17.2826&7.523&11.3558&40.9124&5.759
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
5.589&5.4528&1.5351&6.4198&7.1968&2.0933&3.3327&13.4339&1.5351
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & $1.052\times10^5$&$1.052\times10^5$&48.7724&1518.0529&1741.1556&232.1719&11556.9085&$1.921\times10^6$&48.7724
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
9760.4724&9761.7857&4.6902&294.1121&320.3164&23.0733&1086.5459&$2.706\times10^5$&4.6902
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 15.056&14.6069&1.759&10.9157&13.2826&3.523&7.3558&36.9124&1.759
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
4.589&4.4528&0.5351&5.4198&6.1968&1.0933&2.3327&12.4339&0.5351
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & $1.054\times10^5$&$1.054\times10^5$&51.8617&1637.0525&1917.4101&244.5603&11609.8605&$1.922\times^10^6$&51.8617
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
9780.5554&9780.6369&4.9761&323.4568&358.6841&24.2662&1091.8789&$2.707\times10^5$&4.9761
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & $1.152\times10^5$&$1.152\times10^5$&56.8378&1960.5093&2276.0942&268.8265&12701.7394&$2.193\times10^6$&56.8378\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0012&0.001&0.0165&0.0123&0.0011&0.0011&4041.9544&0.001\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220207/20220208-11h06-Full.beta=4.sig=1.n=200.LaTeX.tex <==
% START DATE AND TIME=20220208-11h06
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=4,  \sigma=1$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 5.5422&4.873&4.9147&8.1162&7.207&5.2726&6.6376&13.6854&4.9147
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.4764&1.2715&1.2765&3.1661&2.6666&1.3921&1.831&4.1275&1.2765
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 358.9688&360.4124&17.4485&586.961&428.971&46.2556&544.088&40207.1123&17.4485
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
34.6869&34.8206&1.6376&95.7863&68.0682&4.3695&52.7303&4942.7143&1.6376
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.5422&0.873&0.9147&4.1162&3.207&1.2726&2.6376&9.6854&0.9147
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.4764&0.2715&0.2765&2.1661&1.6666&0.3921&0.831&3.1275&0.2765
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 361.3113&361.1385&18.2835&603.8454&439.2132&47.8704&550.9903&40296.8991&18.2835
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
34.9104&34.8909&1.7139&100.4688&70.839&4.5228&53.4156&4952.0011&1.7139
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 396.2217&396.0294&19.9974&704.3142&510.0522&52.3933&604.4059&45248.9002&19.9974\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&6e-04&5e-04&0.0111&0.0074&5e-04&6e-04&0.0029&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220207/20220208-11h06-Full.beta=5.sig=1.n=100.LaTeX.tex <==
% START DATE AND TIME=20220208-11h06
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=5,  \sigma=1$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 30.6098&30.2417&7.4119&21.9994&24.3588&10.2719&16.7627&47.2333&7.4119
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
7.0678&6.9822&1.5623&7.2267&7.7657&2.2393&3.7561&10.9819&1.5623
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & $1.824\times10^5$8&$1.824\times10^5$&104.922&2403.7816&2594.7578&410.2926&$1.860\times10^4$&$2.579\times10^5$&104.922
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
$1.039\times10^4$&$1.039\times10^4$&5.7845&268.5518&277.9779&22.5935&1037.1617&$1.545\times10^4$&5.7845
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 25.6098&25.2417&2.4119&16.9994&19.3588&5.2719&11.7627&42.2333&2.4119
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
6.0678&5.9822&0.5623&6.2267&6.7657&1.2393&2.7561&9.9819&0.5623
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & $1.830\times10^5$&$1.830\times10^5$&110.7288&2692.5197&2969.2601&438.0446&$1.873\times10^4$&$2.596\times10^5$&110.7288
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
10426.8814&10426.9571&6.1001&307.2964&323.7252&24.127&1044.6541&15546.0299&6.1001
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & $1.935\times10^5$&$1.935\times10^5$&116.8289&2999.8162&3292.9853&462.1716&$1.978\times10^4$&$2.752\times10^5$&116.8289\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.001&0.0012&0.001&0.0145&0.0106&0.001&0.001&5.15621e+29&0.001\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220207/20220208-11h06-Full.beta=5.sig=1.n=200.LaTeX.tex <==
% START DATE AND TIME=20220208-11h06
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=5,  \sigma=1$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 13.9897&13.2822&6.8132&15.1377&12.05&7.6564&9.7632&21.5972&6.8132
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
3.0754&2.9086&1.4243&4.5829&3.4635&1.6264&2.1335&4.9397&1.4243
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 73492.0862&73505.1699&68.4932&1448.479&977.1387&152.8998&2723.7425&30713.324&68.4932
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
3820.9013&3821.6108&3.8465&138.9351&88.9894&8.5202&148.047&1737.3608&3.8465
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 8.9897&8.2822&1.8132&10.1377&7.05&2.6564&4.7632&16.5972&1.8132
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2.0754&1.9086&0.4243&3.5829&2.4635&0.6264&1.1335&3.9397&0.4243
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 73565.5518&73566.414&71.774&1551.1072&1026.7434&159.9411&2746.1583&30985.7195&71.774
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
3824.8263&3824.8713&4.0261&151.7583&95.0495&8.9117&149.3171&1752.7085&4.0261
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 77390.3781&77391.2853&75.8002&1702.8655&1121.7929&168.8527&2895.4754&32738.428&75.8002\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&6e-04&5e-04&0.0096&0.0062&5e-04&5e-04&2.018&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220207/Output.accuracy.LaTeX.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Wed Feb 09 03:12:51 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & Measure & beta=1.5 & sigma=1 & n=100 & 0.99 \\ 
  2 & MLE.b & Measure & beta=1.5 & sigma=1 & n=100 & 0.68 \\ 
  3 & LME & Measure & beta=1.5 & sigma=1 & n=100 & 0.84 \\ 
  4 & MDE.Phi.chisq & Measure & beta=1.5 & sigma=1 & n=100 & 35.32 \\ 
  5 & MDE.Phi.tv & Measure & beta=1.5 & sigma=1 & n=100 & 29.94 \\ 
  6 & MDE.Phi.kl & Measure & beta=1.5 & sigma=1 & n=100 & 0.99 \\ 
  7 & MME & Measure & beta=1.5 & sigma=1 & n=100 & 9.19 \\ 
  8 & MME.b & Measure & beta=1.5 & sigma=1 & n=100 & 278967.48 \\ 
  9 & PWM & Measure & beta=1.5 & sigma=1 & n=100 & 0.84 \\ 
  10 & MLE & Measure & beta=2 & sigma=1 & n=100 & 6443.21 \\ 
  11 & MLE.b & Measure & beta=2 & sigma=1 & n=100 & 6442.82 \\ 
  12 & LME & Measure & beta=2 & sigma=1 & n=100 & 4.85 \\ 
  13 & MDE.Phi.chisq & Measure & beta=2 & sigma=1 & n=100 & 171.00 \\ 
  14 & MDE.Phi.tv & Measure & beta=2 & sigma=1 & n=100 & 225.29 \\ 
  15 & MDE.Phi.kl & Measure & beta=2 & sigma=1 & n=100 & 20.41 \\ 
  16 & MME & Measure & beta=2 & sigma=1 & n=100 & 80.61 \\ 
  17 & MME.b & Measure & beta=2 & sigma=1 & n=100 & 234831.18 \\ 
  18 & PWM & Measure & beta=2 & sigma=1 & n=100 & 4.85 \\ 
  19 & MLE & Measure & beta=2.5 & sigma=1 & n=100 & 13582.10 \\ 
  20 & MLE.b & Measure & beta=2.5 & sigma=1 & n=100 & 13581.93 \\ 
  21 & LME & Measure & beta=2.5 & sigma=1 & n=100 & 11.21 \\ 
  22 & MDE.Phi.chisq & Measure & beta=2.5 & sigma=1 & n=100 & 453.87 \\ 
  23 & MDE.Phi.tv & Measure & beta=2.5 & sigma=1 & n=100 & 519.13 \\ 
  24 & MDE.Phi.kl & Measure & beta=2.5 & sigma=1 & n=100 & 44.50 \\ 
  25 & MME & Measure & beta=2.5 & sigma=1 & n=100 & 189.04 \\ 
  26 & MME.b & Measure & beta=2.5 & sigma=1 & n=100 & 2874.83 \\ 
  27 & PWM & Measure & beta=2.5 & sigma=1 & n=100 & 11.21 \\ 
  28 & MLE & Measure & beta=3 & sigma=1 & n=100 & 81372.17 \\ 
  29 & MLE.b & Measure & beta=3 & sigma=1 & n=100 & 81372.40 \\ 
  30 & LME & Measure & beta=3 & sigma=1 & n=100 & 20.29 \\ 
  31 & MDE.Phi.chisq & Measure & beta=3 & sigma=1 & n=100 & 874.29 \\ 
  32 & MDE.Phi.tv & Measure & beta=3 & sigma=1 & n=100 & 1049.25 \\ 
  33 & MDE.Phi.kl & Measure & beta=3 & sigma=1 & n=100 & 146.89 \\ 
  34 & MME & Measure & beta=3 & sigma=1 & n=100 & 358564.94 \\ 
  35 & MME.b & Measure & beta=3 & sigma=1 & n=100 & 3409934.01 \\ 
  36 & PWM & Measure & beta=3 & sigma=1 & n=100 & 20.29 \\ 
  37 & MLE & Measure & beta=4 & sigma=1 & n=100 & 115184.49 \\ 
  38 & MLE.b & Measure & beta=4 & sigma=1 & n=100 & 115185.50 \\ 
  39 & LME & Measure & beta=4 & sigma=1 & n=100 & 56.84 \\ 
  40 & MDE.Phi.chisq & Measure & beta=4 & sigma=1 & n=100 & 1960.51 \\ 
  41 & MDE.Phi.tv & Measure & beta=4 & sigma=1 & n=100 & 2276.09 \\ 
  42 & MDE.Phi.kl & Measure & beta=4 & sigma=1 & n=100 & 268.83 \\ 
  43 & MME & Measure & beta=4 & sigma=1 & n=100 & 12701.74 \\ 
  44 & MME.b & Measure & beta=4 & sigma=1 & n=100 & 2193013.30 \\ 
  45 & PWM & Measure & beta=4 & sigma=1 & n=100 & 56.84 \\ 
  46 & MLE & Measure & beta=5 & sigma=1 & n=100 & 193456.52 \\ 
  47 & MLE.b & Measure & beta=5 & sigma=1 & n=100 & 193458.02 \\ 
  48 & LME & Measure & beta=5 & sigma=1 & n=100 & 116.83 \\ 
  49 & MDE.Phi.chisq & Measure & beta=5 & sigma=1 & n=100 & 2999.82 \\ 
  50 & MDE.Phi.tv & Measure & beta=5 & sigma=1 & n=100 & 3292.99 \\ 
  51 & MDE.Phi.kl & Measure & beta=5 & sigma=1 & n=100 & 462.17 \\ 
  52 & MME & Measure & beta=5 & sigma=1 & n=100 & 19776.94 \\ 
  53 & MME.b & Measure & beta=5 & sigma=1 & n=100 & 275173.69 \\ 
  54 & PWM & Measure & beta=5 & sigma=1 & n=100 & 116.83 \\ 
  55 & MLE & Measure & beta=1.5 & sigma=1 & n=200 & 0.22 \\ 
  56 & MLE.b & Measure & beta=1.5 & sigma=1 & n=200 & 0.16 \\ 
  57 & LME & Measure & beta=1.5 & sigma=1 & n=200 & 0.32 \\ 
  58 & MDE.Phi.chisq & Measure & beta=1.5 & sigma=1 & n=200 & 0.78 \\ 
  59 & MDE.Phi.tv & Measure & beta=1.5 & sigma=1 & n=200 & 0.77 \\ 
  60 & MDE.Phi.kl & Measure & beta=1.5 & sigma=1 & n=200 & 0.22 \\ 
  61 & MME & Measure & beta=1.5 & sigma=1 & n=200 & 6.14 \\ 
  62 & MME.b & Measure & beta=1.5 & sigma=1 & n=200 & 5.05 \\ 
  63 & PWM & Measure & beta=1.5 & sigma=1 & n=200 & 0.32 \\ 
  64 & MLE & Measure & beta=2 & sigma=1 & n=200 & 0.47 \\ 
  65 & MLE.b & Measure & beta=2 & sigma=1 & n=200 & 0.29 \\ 
  66 & LME & Measure & beta=2 & sigma=1 & n=200 & 0.52 \\ 
  67 & MDE.Phi.chisq & Measure & beta=2 & sigma=1 & n=200 & 5.18 \\ 
  68 & MDE.Phi.tv & Measure & beta=2 & sigma=1 & n=200 & 5.59 \\ 
  69 & MDE.Phi.kl & Measure & beta=2 & sigma=1 & n=200 & 0.47 \\ 
  70 & MME & Measure & beta=2 & sigma=1 & n=200 & 2.54 \\ 
  71 & MME.b & Measure & beta=2 & sigma=1 & n=200 & 8.84 \\ 
  72 & PWM & Measure & beta=2 & sigma=1 & n=200 & 0.52 \\ 
  73 & MLE & Measure & beta=2.5 & sigma=1 & n=200 & 1.53 \\ 
  74 & MLE.b & Measure & beta=2.5 & sigma=1 & n=200 & 1.08 \\ 
  75 & LME & Measure & beta=2.5 & sigma=1 & n=200 & 1.64 \\ 
  76 & MDE.Phi.chisq & Measure & beta=2.5 & sigma=1 & n=200 & 33.52 \\ 
  77 & MDE.Phi.tv & Measure & beta=2.5 & sigma=1 & n=200 & 24.83 \\ 
  78 & MDE.Phi.kl & Measure & beta=2.5 & sigma=1 & n=200 & 1.53 \\ 
  79 & MME & Measure & beta=2.5 & sigma=1 & n=200 & 3.86 \\ 
  80 & MME.b & Measure & beta=2.5 & sigma=1 & n=200 & 57.01 \\ 
  81 & PWM & Measure & beta=2.5 & sigma=1 & n=200 & 1.64 \\ 
  82 & MLE & Measure & beta=3 & sigma=1 & n=200 & 75.13 \\ 
  83 & MLE.b & Measure & beta=3 & sigma=1 & n=200 & 74.47 \\ 
  84 & LME & Measure & beta=3 & sigma=1 & n=200 & 5.13 \\ 
  85 & MDE.Phi.chisq & Measure & beta=3 & sigma=1 & n=200 & 148.42 \\ 
  86 & MDE.Phi.tv & Measure & beta=3 & sigma=1 & n=200 & 68.40 \\ 
  87 & MDE.Phi.kl & Measure & beta=3 & sigma=1 & n=200 & 10.11 \\ 
  88 & MME & Measure & beta=3 & sigma=1 & n=200 & 87.27 \\ 
  89 & MME.b & Measure & beta=3 & sigma=1 & n=200 & 9036.22 \\ 
  90 & PWM & Measure & beta=3 & sigma=1 & n=200 & 5.13 \\ 
  91 & MLE & Measure & beta=4 & sigma=1 & n=200 & 396.22 \\ 
  92 & MLE.b & Measure & beta=4 & sigma=1 & n=200 & 396.03 \\ 
  93 & LME & Measure & beta=4 & sigma=1 & n=200 & 20.00 \\ 
  94 & MDE.Phi.chisq & Measure & beta=4 & sigma=1 & n=200 & 704.31 \\ 
  95 & MDE.Phi.tv & Measure & beta=4 & sigma=1 & n=200 & 510.05 \\ 
  96 & MDE.Phi.kl & Measure & beta=4 & sigma=1 & n=200 & 52.39 \\ 
  97 & MME & Measure & beta=4 & sigma=1 & n=200 & 604.41 \\ 
  98 & MME.b & Measure & beta=4 & sigma=1 & n=200 & 45248.90 \\ 
  99 & PWM & Measure & beta=4 & sigma=1 & n=200 & 20.00 \\ 
  100 & MLE & Measure & beta=5 & sigma=1 & n=200 & 77390.38 \\ 
  101 & MLE.b & Measure & beta=5 & sigma=1 & n=200 & 77391.29 \\ 
  102 & LME & Measure & beta=5 & sigma=1 & n=200 & 75.80 \\ 
  103 & MDE.Phi.chisq & Measure & beta=5 & sigma=1 & n=200 & 1702.87 \\ 
  104 & MDE.Phi.tv & Measure & beta=5 & sigma=1 & n=200 & 1121.79 \\ 
  105 & MDE.Phi.kl & Measure & beta=5 & sigma=1 & n=200 & 168.85 \\ 
  106 & MME & Measure & beta=5 & sigma=1 & n=200 & 2895.48 \\ 
  107 & MME.b & Measure & beta=5 & sigma=1 & n=200 & 32738.43 \\ 
  108 & PWM & Measure & beta=5 & sigma=1 & n=200 & 75.80 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220207/Output.accuracy2.LaTeX.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Wed Feb 09 03:12:51 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & Measure & beta=1.5 & sigma=1 & n=100 & 0.00 \\ 
  2 & MLE.b & Measure & beta=1.5 & sigma=1 & n=100 & 0.00 \\ 
  3 & LME & Measure & beta=1.5 & sigma=1 & n=100 & 0.00 \\ 
  4 & MDE.Phi.chisq & Measure & beta=1.5 & sigma=1 & n=100 & 181787018350624229332064482482084282602604822808686222086826422600406468626442880202480026068600642028200282242280222024246020860022848620402880404466644668026044682262046000244464684680404040648066066624288048682020048688026826682826820642682280002668866466086886864424642802262886688486208806684284.00 \\ 
  5 & MDE.Phi.tv & Measure & beta=1.5 & sigma=1 & n=100 & 0.03 \\ 
  6 & MDE.Phi.kl & Measure & beta=1.5 & sigma=1 & n=100 & 0.00 \\ 
  7 & MME & Measure & beta=1.5 & sigma=1 & n=100 & 0.01 \\ 
  8 & MME.b & Measure & beta=1.5 & sigma=1 & n=100 & 7.11 \\ 
  9 & PWM & Measure & beta=1.5 & sigma=1 & n=100 & 0.00 \\ 
  10 & MLE & Measure & beta=2 & sigma=1 & n=100 & 0.00 \\ 
  11 & MLE.b & Measure & beta=2 & sigma=1 & n=100 & 0.00 \\ 
  12 & LME & Measure & beta=2 & sigma=1 & n=100 & 0.00 \\ 
  13 & MDE.Phi.chisq & Measure & beta=2 & sigma=1 & n=100 & 0.03 \\ 
  14 & MDE.Phi.tv & Measure & beta=2 & sigma=1 & n=100 & 0.02 \\ 
  15 & MDE.Phi.kl & Measure & beta=2 & sigma=1 & n=100 & 0.00 \\ 
  16 & MME & Measure & beta=2 & sigma=1 & n=100 & 0.00 \\ 
  17 & MME.b & Measure & beta=2 & sigma=1 & n=100 & 0.01 \\ 
  18 & PWM & Measure & beta=2 & sigma=1 & n=100 & 0.00 \\ 
  19 & MLE & Measure & beta=2.5 & sigma=1 & n=100 & 0.00 \\ 
  20 & MLE.b & Measure & beta=2.5 & sigma=1 & n=100 & 0.00 \\ 
  21 & LME & Measure & beta=2.5 & sigma=1 & n=100 & 0.00 \\ 
  22 & MDE.Phi.chisq & Measure & beta=2.5 & sigma=1 & n=100 & 0.02 \\ 
  23 & MDE.Phi.tv & Measure & beta=2.5 & sigma=1 & n=100 & 0.02 \\ 
  24 & MDE.Phi.kl & Measure & beta=2.5 & sigma=1 & n=100 & 0.00 \\ 
  25 & MME & Measure & beta=2.5 & sigma=1 & n=100 & 0.00 \\ 
  26 & MME.b & Measure & beta=2.5 & sigma=1 & n=100 & 8.08 \\ 
  27 & PWM & Measure & beta=2.5 & sigma=1 & n=100 & 0.00 \\ 
  28 & MLE & Measure & beta=3 & sigma=1 & n=100 & 0.00 \\ 
  29 & MLE.b & Measure & beta=3 & sigma=1 & n=100 & 0.00 \\ 
  30 & LME & Measure & beta=3 & sigma=1 & n=100 & 0.00 \\ 
  31 & MDE.Phi.chisq & Measure & beta=3 & sigma=1 & n=100 & 0.02 \\ 
  32 & MDE.Phi.tv & Measure & beta=3 & sigma=1 & n=100 & 0.02 \\ 
  33 & MDE.Phi.kl & Measure & beta=3 & sigma=1 & n=100 & 0.00 \\ 
  34 & MME & Measure & beta=3 & sigma=1 & n=100 & 0.00 \\ 
  35 & MME.b & Measure & beta=3 & sigma=1 & n=100 & 0.01 \\ 
  36 & PWM & Measure & beta=3 & sigma=1 & n=100 & 0.00 \\ 
  37 & MLE & Measure & beta=4 & sigma=1 & n=100 & 0.00 \\ 
  38 & MLE.b & Measure & beta=4 & sigma=1 & n=100 & 0.00 \\ 
  39 & LME & Measure & beta=4 & sigma=1 & n=100 & 0.00 \\ 
  40 & MDE.Phi.chisq & Measure & beta=4 & sigma=1 & n=100 & 0.02 \\ 
  41 & MDE.Phi.tv & Measure & beta=4 & sigma=1 & n=100 & 0.01 \\ 
  42 & MDE.Phi.kl & Measure & beta=4 & sigma=1 & n=100 & 0.00 \\ 
  43 & MME & Measure & beta=4 & sigma=1 & n=100 & 0.00 \\ 
  44 & MME.b & Measure & beta=4 & sigma=1 & n=100 & 4041.95 \\ 
  45 & PWM & Measure & beta=4 & sigma=1 & n=100 & 0.00 \\ 
  46 & MLE & Measure & beta=5 & sigma=1 & n=100 & 0.00 \\ 
  47 & MLE.b & Measure & beta=5 & sigma=1 & n=100 & 0.00 \\ 
  48 & LME & Measure & beta=5 & sigma=1 & n=100 & 0.00 \\ 
  49 & MDE.Phi.chisq & Measure & beta=5 & sigma=1 & n=100 & 0.01 \\ 
  50 & MDE.Phi.tv & Measure & beta=5 & sigma=1 & n=100 & 0.01 \\ 
  51 & MDE.Phi.kl & Measure & beta=5 & sigma=1 & n=100 & 0.00 \\ 
  52 & MME & Measure & beta=5 & sigma=1 & n=100 & 0.00 \\ 
  53 & MME.b & Measure & beta=5 & sigma=1 & n=100 & 515620838018138634806240604226.00 \\ 
  54 & PWM & Measure & beta=5 & sigma=1 & n=100 & 0.00 \\ 
  55 & MLE & Measure & beta=1.5 & sigma=1 & n=200 & 0.00 \\ 
  56 & MLE.b & Measure & beta=1.5 & sigma=1 & n=200 & 0.00 \\ 
  57 & LME & Measure & beta=1.5 & sigma=1 & n=200 & 0.00 \\ 
  58 & MDE.Phi.chisq & Measure & beta=1.5 & sigma=1 & n=200 & 0.03 \\ 
  59 & MDE.Phi.tv & Measure & beta=1.5 & sigma=1 & n=200 & 0.03 \\ 
  60 & MDE.Phi.kl & Measure & beta=1.5 & sigma=1 & n=200 & 0.00 \\ 
  61 & MME & Measure & beta=1.5 & sigma=1 & n=200 & 0.01 \\ 
  62 & MME.b & Measure & beta=1.5 & sigma=1 & n=200 & 0.01 \\ 
  63 & PWM & Measure & beta=1.5 & sigma=1 & n=200 & 0.00 \\ 
  64 & MLE & Measure & beta=2 & sigma=1 & n=200 & 0.00 \\ 
  65 & MLE.b & Measure & beta=2 & sigma=1 & n=200 & 0.00 \\ 
  66 & LME & Measure & beta=2 & sigma=1 & n=200 & 0.00 \\ 
  67 & MDE.Phi.chisq & Measure & beta=2 & sigma=1 & n=200 & 0.02 \\ 
  68 & MDE.Phi.tv & Measure & beta=2 & sigma=1 & n=200 & 0.02 \\ 
  69 & MDE.Phi.kl & Measure & beta=2 & sigma=1 & n=200 & 0.00 \\ 
  70 & MME & Measure & beta=2 & sigma=1 & n=200 & 0.00 \\ 
  71 & MME.b & Measure & beta=2 & sigma=1 & n=200 & 0.00 \\ 
  72 & PWM & Measure & beta=2 & sigma=1 & n=200 & 0.00 \\ 
  73 & MLE & Measure & beta=2.5 & sigma=1 & n=200 & 0.00 \\ 
  74 & MLE.b & Measure & beta=2.5 & sigma=1 & n=200 & 0.00 \\ 
  75 & LME & Measure & beta=2.5 & sigma=1 & n=200 & 0.00 \\ 
  76 & MDE.Phi.chisq & Measure & beta=2.5 & sigma=1 & n=200 & 0.02 \\ 
  77 & MDE.Phi.tv & Measure & beta=2.5 & sigma=1 & n=200 & 0.01 \\ 
  78 & MDE.Phi.kl & Measure & beta=2.5 & sigma=1 & n=200 & 0.00 \\ 
  79 & MME & Measure & beta=2.5 & sigma=1 & n=200 & 0.00 \\ 
  80 & MME.b & Measure & beta=2.5 & sigma=1 & n=200 & 0.00 \\ 
  81 & PWM & Measure & beta=2.5 & sigma=1 & n=200 & 0.00 \\ 
  82 & MLE & Measure & beta=3 & sigma=1 & n=200 & 0.00 \\ 
  83 & MLE.b & Measure & beta=3 & sigma=1 & n=200 & 0.00 \\ 
  84 & LME & Measure & beta=3 & sigma=1 & n=200 & 0.00 \\ 
  85 & MDE.Phi.chisq & Measure & beta=3 & sigma=1 & n=200 & 0.01 \\ 
  86 & MDE.Phi.tv & Measure & beta=3 & sigma=1 & n=200 & 0.01 \\ 
  87 & MDE.Phi.kl & Measure & beta=3 & sigma=1 & n=200 & 0.00 \\ 
  88 & MME & Measure & beta=3 & sigma=1 & n=200 & 0.00 \\ 
  89 & MME.b & Measure & beta=3 & sigma=1 & n=200 & 0.00 \\ 
  90 & PWM & Measure & beta=3 & sigma=1 & n=200 & 0.00 \\ 
  91 & MLE & Measure & beta=4 & sigma=1 & n=200 & 0.00 \\ 
  92 & MLE.b & Measure & beta=4 & sigma=1 & n=200 & 0.00 \\ 
  93 & LME & Measure & beta=4 & sigma=1 & n=200 & 0.00 \\ 
  94 & MDE.Phi.chisq & Measure & beta=4 & sigma=1 & n=200 & 0.01 \\ 
  95 & MDE.Phi.tv & Measure & beta=4 & sigma=1 & n=200 & 0.01 \\ 
  96 & MDE.Phi.kl & Measure & beta=4 & sigma=1 & n=200 & 0.00 \\ 
  97 & MME & Measure & beta=4 & sigma=1 & n=200 & 0.00 \\ 
  98 & MME.b & Measure & beta=4 & sigma=1 & n=200 & 0.00 \\ 
  99 & PWM & Measure & beta=4 & sigma=1 & n=200 & 0.00 \\ 
  100 & MLE & Measure & beta=5 & sigma=1 & n=200 & 0.00 \\ 
  101 & MLE.b & Measure & beta=5 & sigma=1 & n=200 & 0.00 \\ 
  102 & LME & Measure & beta=5 & sigma=1 & n=200 & 0.00 \\ 
  103 & MDE.Phi.chisq & Measure & beta=5 & sigma=1 & n=200 & 0.01 \\ 
  104 & MDE.Phi.tv & Measure & beta=5 & sigma=1 & n=200 & 0.01 \\ 
  105 & MDE.Phi.kl & Measure & beta=5 & sigma=1 & n=200 & 0.00 \\ 
  106 & MME & Measure & beta=5 & sigma=1 & n=200 & 0.00 \\ 
  107 & MME.b & Measure & beta=5 & sigma=1 & n=200 & 2.02 \\ 
  108 & PWM & Measure & beta=5 & sigma=1 & n=200 & 0.00 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220207/Output.bias.LaTeX.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Wed Feb 09 03:12:51 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=1 & n=100 & 0.17 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=1 & n=100 & -0.02 \\ 
  3 & LME & beta & beta=1.5 & sigma=1 & n=100 & 0.33 \\ 
  4 & MDE.Phi.chisq & beta & beta=1.5 & sigma=1 & n=100 & -0.51 \\ 
  5 & MDE.Phi.tv & beta & beta=1.5 & sigma=1 & n=100 & -0.24 \\ 
  6 & MDE.Phi.kl & beta & beta=1.5 & sigma=1 & n=100 & 0.17 \\ 
  7 & MME & beta & beta=1.5 & sigma=1 & n=100 & 1.29 \\ 
  8 & MME.b & beta & beta=1.5 & sigma=1 & n=100 & 4.81 \\ 
  9 & PWM & beta & beta=1.5 & sigma=1 & n=100 & 0.33 \\ 
  10 & MLE & sigma & beta=1.5 & sigma=1 & n=100 & 0.18 \\ 
  11 & MLE.b & sigma & beta=1.5 & sigma=1 & n=100 & -0.02 \\ 
  12 & LME & sigma & beta=1.5 & sigma=1 & n=100 & 0.33 \\ 
  13 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=1 & n=100 & 0.55 \\ 
  14 & MDE.Phi.tv & sigma & beta=1.5 & sigma=1 & n=100 & 0.83 \\ 
  15 & MDE.Phi.kl & sigma & beta=1.5 & sigma=1 & n=100 & 0.18 \\ 
  16 & MME & sigma & beta=1.5 & sigma=1 & n=100 & 2.15 \\ 
  17 & MME.b & sigma & beta=1.5 & sigma=1 & n=100 & 5.83 \\ 
  18 & PWM & sigma & beta=1.5 & sigma=1 & n=100 & 0.33 \\ 
  19 & MLE & beta & beta=2 & sigma=1 & n=100 & 1.20 \\ 
  20 & MLE.b & beta & beta=2 & sigma=1 & n=100 & 0.85 \\ 
  21 & LME & beta & beta=2 & sigma=1 & n=100 & 0.45 \\ 
  22 & MDE.Phi.chisq & beta & beta=2 & sigma=1 & n=100 & 0.15 \\ 
  23 & MDE.Phi.tv & beta & beta=2 & sigma=1 & n=100 & 0.77 \\ 
  24 & MDE.Phi.kl & beta & beta=2 & sigma=1 & n=100 & 0.47 \\ 
  25 & MME & beta & beta=2 & sigma=1 & n=100 & 1.68 \\ 
  26 & MME.b & beta & beta=2 & sigma=1 & n=100 & 7.48 \\ 
  27 & PWM & beta & beta=2 & sigma=1 & n=100 & 0.45 \\ 
  28 & MLE & sigma & beta=2 & sigma=1 & n=100 & 0.75 \\ 
  29 & MLE.b & sigma & beta=2 & sigma=1 & n=100 & 0.49 \\ 
  30 & LME & sigma & beta=2 & sigma=1 & n=100 & 0.30 \\ 
  31 & MDE.Phi.chisq & sigma & beta=2 & sigma=1 & n=100 & 1.15 \\ 
  32 & MDE.Phi.tv & sigma & beta=2 & sigma=1 & n=100 & 1.68 \\ 
  33 & MDE.Phi.kl & sigma & beta=2 & sigma=1 & n=100 & 0.33 \\ 
  34 & MME & sigma & beta=2 & sigma=1 & n=100 & 1.44 \\ 
  35 & MME.b & sigma & beta=2 & sigma=1 & n=100 & 5.59 \\ 
  36 & PWM & sigma & beta=2 & sigma=1 & n=100 & 0.30 \\ 
  37 & MLE & beta & beta=2.5 & sigma=1 & n=100 & 2.45 \\ 
  38 & MLE.b & beta & beta=2.5 & sigma=1 & n=100 & 1.99 \\ 
  39 & LME & beta & beta=2.5 & sigma=1 & n=100 & 0.70 \\ 
  40 & MDE.Phi.chisq & beta & beta=2.5 & sigma=1 & n=100 & 1.81 \\ 
  41 & MDE.Phi.tv & beta & beta=2.5 & sigma=1 & n=100 & 2.65 \\ 
  42 & MDE.Phi.kl & beta & beta=2.5 & sigma=1 & n=100 & 0.95 \\ 
  43 & MME & beta & beta=2.5 & sigma=1 & n=100 & 2.32 \\ 
  44 & MME.b & beta & beta=2.5 & sigma=1 & n=100 & 5.49 \\ 
  45 & PWM & beta & beta=2.5 & sigma=1 & n=100 & 0.70 \\ 
  46 & MLE & sigma & beta=2.5 & sigma=1 & n=100 & 1.32 \\ 
  47 & MLE.b & sigma & beta=2.5 & sigma=1 & n=100 & 1.07 \\ 
  48 & LME & sigma & beta=2.5 & sigma=1 & n=100 & 0.36 \\ 
  49 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=1 & n=100 & 2.23 \\ 
  50 & MDE.Phi.tv & sigma & beta=2.5 & sigma=1 & n=100 & 2.77 \\ 
  51 & MDE.Phi.kl & sigma & beta=2.5 & sigma=1 & n=100 & 0.51 \\ 
  52 & MME & sigma & beta=2.5 & sigma=1 & n=100 & 1.35 \\ 
  53 & MME.b & sigma & beta=2.5 & sigma=1 & n=100 & 3.02 \\ 
  54 & PWM & sigma & beta=2.5 & sigma=1 & n=100 & 0.36 \\ 
  55 & MLE & beta & beta=3 & sigma=1 & n=100 & 10.45 \\ 
  56 & MLE.b & beta & beta=3 & sigma=1 & n=100 & 9.96 \\ 
  57 & LME & beta & beta=3 & sigma=1 & n=100 & 1.02 \\ 
  58 & MDE.Phi.chisq & beta & beta=3 & sigma=1 & n=100 & 4.28 \\ 
  59 & MDE.Phi.tv & beta & beta=3 & sigma=1 & n=100 & 5.76 \\ 
  60 & MDE.Phi.kl & beta & beta=3 & sigma=1 & n=100 & 1.92 \\ 
  61 & MME & beta & beta=3 & sigma=1 & n=100 & 14.49 \\ 
  62 & MME.b & beta & beta=3 & sigma=1 & n=100 & 46.99 \\ 
  63 & PWM & beta & beta=3 & sigma=1 & n=100 & 1.02 \\ 
  64 & MLE & sigma & beta=3 & sigma=1 & n=100 & 4.56 \\ 
  65 & MLE.b & sigma & beta=3 & sigma=1 & n=100 & 4.35 \\ 
  66 & LME & sigma & beta=3 & sigma=1 & n=100 & 0.43 \\ 
  67 & MDE.Phi.chisq & sigma & beta=3 & sigma=1 & n=100 & 3.41 \\ 
  68 & MDE.Phi.tv & sigma & beta=3 & sigma=1 & n=100 & 4.17 \\ 
  69 & MDE.Phi.kl & sigma & beta=3 & sigma=1 & n=100 & 0.83 \\ 
  70 & MME & sigma & beta=3 & sigma=1 & n=100 & 5.74 \\ 
  71 & MME.b & sigma & beta=3 & sigma=1 & n=100 & 18.57 \\ 
  72 & PWM & sigma & beta=3 & sigma=1 & n=100 & 0.43 \\ 
  73 & MLE & beta & beta=4 & sigma=1 & n=100 & 15.06 \\ 
  74 & MLE.b & beta & beta=4 & sigma=1 & n=100 & 14.61 \\ 
  75 & LME & beta & beta=4 & sigma=1 & n=100 & 1.76 \\ 
  76 & MDE.Phi.chisq & beta & beta=4 & sigma=1 & n=100 & 10.92 \\ 
  77 & MDE.Phi.tv & beta & beta=4 & sigma=1 & n=100 & 13.28 \\ 
  78 & MDE.Phi.kl & beta & beta=4 & sigma=1 & n=100 & 3.52 \\ 
  79 & MME & beta & beta=4 & sigma=1 & n=100 & 7.36 \\ 
  80 & MME.b & beta & beta=4 & sigma=1 & n=100 & 36.91 \\ 
  81 & PWM & beta & beta=4 & sigma=1 & n=100 & 1.76 \\ 
  82 & MLE & sigma & beta=4 & sigma=1 & n=100 & 4.59 \\ 
  83 & MLE.b & sigma & beta=4 & sigma=1 & n=100 & 4.45 \\ 
  84 & LME & sigma & beta=4 & sigma=1 & n=100 & 0.54 \\ 
  85 & MDE.Phi.chisq & sigma & beta=4 & sigma=1 & n=100 & 5.42 \\ 
  86 & MDE.Phi.tv & sigma & beta=4 & sigma=1 & n=100 & 6.20 \\ 
  87 & MDE.Phi.kl & sigma & beta=4 & sigma=1 & n=100 & 1.09 \\ 
  88 & MME & sigma & beta=4 & sigma=1 & n=100 & 2.33 \\ 
  89 & MME.b & sigma & beta=4 & sigma=1 & n=100 & 12.43 \\ 
  90 & PWM & sigma & beta=4 & sigma=1 & n=100 & 0.54 \\ 
  91 & MLE & beta & beta=5 & sigma=1 & n=100 & 25.61 \\ 
  92 & MLE.b & beta & beta=5 & sigma=1 & n=100 & 25.24 \\ 
  93 & LME & beta & beta=5 & sigma=1 & n=100 & 2.41 \\ 
  94 & MDE.Phi.chisq & beta & beta=5 & sigma=1 & n=100 & 17.00 \\ 
  95 & MDE.Phi.tv & beta & beta=5 & sigma=1 & n=100 & 19.36 \\ 
  96 & MDE.Phi.kl & beta & beta=5 & sigma=1 & n=100 & 5.27 \\ 
  97 & MME & beta & beta=5 & sigma=1 & n=100 & 11.76 \\ 
  98 & MME.b & beta & beta=5 & sigma=1 & n=100 & 42.23 \\ 
  99 & PWM & beta & beta=5 & sigma=1 & n=100 & 2.41 \\ 
  100 & MLE & sigma & beta=5 & sigma=1 & n=100 & 6.07 \\ 
  101 & MLE.b & sigma & beta=5 & sigma=1 & n=100 & 5.98 \\ 
  102 & LME & sigma & beta=5 & sigma=1 & n=100 & 0.56 \\ 
  103 & MDE.Phi.chisq & sigma & beta=5 & sigma=1 & n=100 & 6.23 \\ 
  104 & MDE.Phi.tv & sigma & beta=5 & sigma=1 & n=100 & 6.77 \\ 
  105 & MDE.Phi.kl & sigma & beta=5 & sigma=1 & n=100 & 1.24 \\ 
  106 & MME & sigma & beta=5 & sigma=1 & n=100 & 2.76 \\ 
  107 & MME.b & sigma & beta=5 & sigma=1 & n=100 & 9.98 \\ 
  108 & PWM & sigma & beta=5 & sigma=1 & n=100 & 0.56 \\ 
  109 & MLE & beta & beta=1.5 & sigma=1 & n=200 & 0.08 \\ 
  110 & MLE.b & beta & beta=1.5 & sigma=1 & n=200 & -0.00 \\ 
  111 & LME & beta & beta=1.5 & sigma=1 & n=200 & 0.21 \\ 
  112 & MDE.Phi.chisq & beta & beta=1.5 & sigma=1 & n=200 & -0.65 \\ 
  113 & MDE.Phi.tv & beta & beta=1.5 & sigma=1 & n=200 & -0.49 \\ 
  114 & MDE.Phi.kl & beta & beta=1.5 & sigma=1 & n=200 & 0.08 \\ 
  115 & MME & beta & beta=1.5 & sigma=1 & n=200 & 1.00 \\ 
  116 & MME.b & beta & beta=1.5 & sigma=1 & n=200 & 0.80 \\ 
  117 & PWM & beta & beta=1.5 & sigma=1 & n=200 & 0.21 \\ 
  118 & MLE & sigma & beta=1.5 & sigma=1 & n=200 & 0.08 \\ 
  119 & MLE.b & sigma & beta=1.5 & sigma=1 & n=200 & -0.01 \\ 
  120 & LME & sigma & beta=1.5 & sigma=1 & n=200 & 0.20 \\ 
  121 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=1 & n=200 & 0.12 \\ 
  122 & MDE.Phi.tv & sigma & beta=1.5 & sigma=1 & n=200 & 0.25 \\ 
  123 & MDE.Phi.kl & sigma & beta=1.5 & sigma=1 & n=200 & 0.08 \\ 
  124 & MME & sigma & beta=1.5 & sigma=1 & n=200 & 1.79 \\ 
  125 & MME.b & sigma & beta=1.5 & sigma=1 & n=200 & 1.51 \\ 
  126 & PWM & sigma & beta=1.5 & sigma=1 & n=200 & 0.20 \\ 
  127 & MLE & beta & beta=2 & sigma=1 & n=200 & 0.14 \\ 
  128 & MLE.b & beta & beta=2 & sigma=1 & n=200 & -0.03 \\ 
  129 & LME & beta & beta=2 & sigma=1 & n=200 & 0.22 \\ 
  130 & MDE.Phi.chisq & beta & beta=2 & sigma=1 & n=200 & -0.65 \\ 
  131 & MDE.Phi.tv & beta & beta=2 & sigma=1 & n=200 & -0.44 \\ 
  132 & MDE.Phi.kl & beta & beta=2 & sigma=1 & n=200 & 0.14 \\ 
  133 & MME & beta & beta=2 & sigma=1 & n=200 & 0.97 \\ 
  134 & MME.b & beta & beta=2 & sigma=1 & n=200 & 0.69 \\ 
  135 & PWM & beta & beta=2 & sigma=1 & n=200 & 0.22 \\ 
  136 & MLE & sigma & beta=2 & sigma=1 & n=200 & 0.10 \\ 
  137 & MLE.b & sigma & beta=2 & sigma=1 & n=200 & -0.02 \\ 
  138 & LME & sigma & beta=2 & sigma=1 & n=200 & 0.14 \\ 
  139 & MDE.Phi.chisq & sigma & beta=2 & sigma=1 & n=200 & 0.17 \\ 
  140 & MDE.Phi.tv & sigma & beta=2 & sigma=1 & n=200 & 0.28 \\ 
  141 & MDE.Phi.kl & sigma & beta=2 & sigma=1 & n=200 & 0.10 \\ 
  142 & MME & sigma & beta=2 & sigma=1 & n=200 & 0.89 \\ 
  143 & MME.b & sigma & beta=2 & sigma=1 & n=200 & 0.65 \\ 
  144 & PWM & sigma & beta=2 & sigma=1 & n=200 & 0.14 \\ 
  145 & MLE & beta & beta=2.5 & sigma=1 & n=200 & 0.25 \\ 
  146 & MLE.b & beta & beta=2.5 & sigma=1 & n=200 & -0.05 \\ 
  147 & LME & beta & beta=2.5 & sigma=1 & n=200 & 0.28 \\ 
  148 & MDE.Phi.chisq & beta & beta=2.5 & sigma=1 & n=200 & -0.44 \\ 
  149 & MDE.Phi.tv & beta & beta=2.5 & sigma=1 & n=200 & -0.21 \\ 
  150 & MDE.Phi.kl & beta & beta=2.5 & sigma=1 & n=200 & 0.25 \\ 
  151 & MME & beta & beta=2.5 & sigma=1 & n=200 & 1.06 \\ 
  152 & MME.b & beta & beta=2.5 & sigma=1 & n=200 & 0.84 \\ 
  153 & PWM & beta & beta=2.5 & sigma=1 & n=200 & 0.28 \\ 
  154 & MLE & sigma & beta=2.5 & sigma=1 & n=200 & 0.14 \\ 
  155 & MLE.b & sigma & beta=2.5 & sigma=1 & n=200 & -0.03 \\ 
  156 & LME & sigma & beta=2.5 & sigma=1 & n=200 & 0.14 \\ 
  157 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=1 & n=200 & 0.36 \\ 
  158 & MDE.Phi.tv & sigma & beta=2.5 & sigma=1 & n=200 & 0.41 \\ 
  159 & MDE.Phi.kl & sigma & beta=2.5 & sigma=1 & n=200 & 0.14 \\ 
  160 & MME & sigma & beta=2.5 & sigma=1 & n=200 & 0.65 \\ 
  161 & MME.b & sigma & beta=2.5 & sigma=1 & n=200 & 0.51 \\ 
  162 & PWM & sigma & beta=2.5 & sigma=1 & n=200 & 0.14 \\ 
  163 & MLE & beta & beta=3 & sigma=1 & n=200 & 0.55 \\ 
  164 & MLE.b & beta & beta=3 & sigma=1 & n=200 & 0.09 \\ 
  165 & LME & beta & beta=3 & sigma=1 & n=200 & 0.45 \\ 
  166 & MDE.Phi.chisq & beta & beta=3 & sigma=1 & n=200 & 0.38 \\ 
  167 & MDE.Phi.tv & beta & beta=3 & sigma=1 & n=200 & 0.24 \\ 
  168 & MDE.Phi.kl & beta & beta=3 & sigma=1 & n=200 & 0.49 \\ 
  169 & MME & beta & beta=3 & sigma=1 & n=200 & 1.40 \\ 
  170 & MME.b & beta & beta=3 & sigma=1 & n=200 & 2.69 \\ 
  171 & PWM & beta & beta=3 & sigma=1 & n=200 & 0.45 \\ 
  172 & MLE & sigma & beta=3 & sigma=1 & n=200 & 0.24 \\ 
  173 & MLE.b & sigma & beta=3 & sigma=1 & n=200 & 0.04 \\ 
  174 & LME & sigma & beta=3 & sigma=1 & n=200 & 0.19 \\ 
  175 & MDE.Phi.chisq & sigma & beta=3 & sigma=1 & n=200 & 0.82 \\ 
  176 & MDE.Phi.tv & sigma & beta=3 & sigma=1 & n=200 & 0.61 \\ 
  177 & MDE.Phi.kl & sigma & beta=3 & sigma=1 & n=200 & 0.21 \\ 
  178 & MME & sigma & beta=3 & sigma=1 & n=200 & 0.65 \\ 
  179 & MME.b & sigma & beta=3 & sigma=1 & n=200 & 1.23 \\ 
  180 & PWM & sigma & beta=3 & sigma=1 & n=200 & 0.19 \\ 
  181 & MLE & beta & beta=4 & sigma=1 & n=200 & 1.54 \\ 
  182 & MLE.b & beta & beta=4 & sigma=1 & n=200 & 0.87 \\ 
  183 & LME & beta & beta=4 & sigma=1 & n=200 & 0.91 \\ 
  184 & MDE.Phi.chisq & beta & beta=4 & sigma=1 & n=200 & 4.12 \\ 
  185 & MDE.Phi.tv & beta & beta=4 & sigma=1 & n=200 & 3.21 \\ 
  186 & MDE.Phi.kl & beta & beta=4 & sigma=1 & n=200 & 1.27 \\ 
  187 & MME & beta & beta=4 & sigma=1 & n=200 & 2.64 \\ 
  188 & MME.b & beta & beta=4 & sigma=1 & n=200 & 9.69 \\ 
  189 & PWM & beta & beta=4 & sigma=1 & n=200 & 0.91 \\ 
  190 & MLE & sigma & beta=4 & sigma=1 & n=200 & 0.48 \\ 
  191 & MLE.b & sigma & beta=4 & sigma=1 & n=200 & 0.27 \\ 
  192 & LME & sigma & beta=4 & sigma=1 & n=200 & 0.28 \\ 
  193 & MDE.Phi.chisq & sigma & beta=4 & sigma=1 & n=200 & 2.17 \\ 
  194 & MDE.Phi.tv & sigma & beta=4 & sigma=1 & n=200 & 1.67 \\ 
  195 & MDE.Phi.kl & sigma & beta=4 & sigma=1 & n=200 & 0.39 \\ 
  196 & MME & sigma & beta=4 & sigma=1 & n=200 & 0.83 \\ 
  197 & MME.b & sigma & beta=4 & sigma=1 & n=200 & 3.13 \\ 
  198 & PWM & sigma & beta=4 & sigma=1 & n=200 & 0.28 \\ 
  199 & MLE & beta & beta=5 & sigma=1 & n=200 & 8.99 \\ 
  200 & MLE.b & beta & beta=5 & sigma=1 & n=200 & 8.28 \\ 
  201 & LME & beta & beta=5 & sigma=1 & n=200 & 1.81 \\ 
  202 & MDE.Phi.chisq & beta & beta=5 & sigma=1 & n=200 & 10.14 \\ 
  203 & MDE.Phi.tv & beta & beta=5 & sigma=1 & n=200 & 7.05 \\ 
  204 & MDE.Phi.kl & beta & beta=5 & sigma=1 & n=200 & 2.66 \\ 
  205 & MME & beta & beta=5 & sigma=1 & n=200 & 4.76 \\ 
  206 & MME.b & beta & beta=5 & sigma=1 & n=200 & 16.60 \\ 
  207 & PWM & beta & beta=5 & sigma=1 & n=200 & 1.81 \\ 
  208 & MLE & sigma & beta=5 & sigma=1 & n=200 & 2.08 \\ 
  209 & MLE.b & sigma & beta=5 & sigma=1 & n=200 & 1.91 \\ 
  210 & LME & sigma & beta=5 & sigma=1 & n=200 & 0.42 \\ 
  211 & MDE.Phi.chisq & sigma & beta=5 & sigma=1 & n=200 & 3.58 \\ 
  212 & MDE.Phi.tv & sigma & beta=5 & sigma=1 & n=200 & 2.46 \\ 
  213 & MDE.Phi.kl & sigma & beta=5 & sigma=1 & n=200 & 0.63 \\ 
  214 & MME & sigma & beta=5 & sigma=1 & n=200 & 1.13 \\ 
  215 & MME.b & sigma & beta=5 & sigma=1 & n=200 & 3.94 \\ 
  216 & PWM & sigma & beta=5 & sigma=1 & n=200 & 0.42 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220207/Output.mean.LaTeX.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Wed Feb 09 03:12:51 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=1 & n=100 & 1.67 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=1 & n=100 & 1.48 \\ 
  3 & LME & beta & beta=1.5 & sigma=1 & n=100 & 1.83 \\ 
  4 & MDE.Phi.chisq & beta & beta=1.5 & sigma=1 & n=100 & 0.99 \\ 
  5 & MDE.Phi.tv & beta & beta=1.5 & sigma=1 & n=100 & 1.26 \\ 
  6 & MDE.Phi.kl & beta & beta=1.5 & sigma=1 & n=100 & 1.67 \\ 
  7 & MME & beta & beta=1.5 & sigma=1 & n=100 & 2.79 \\ 
  8 & MME.b & beta & beta=1.5 & sigma=1 & n=100 & 6.31 \\ 
  9 & PWM & beta & beta=1.5 & sigma=1 & n=100 & 1.83 \\ 
  10 & MLE & sigma & beta=1.5 & sigma=1 & n=100 & 1.18 \\ 
  11 & MLE.b & sigma & beta=1.5 & sigma=1 & n=100 & 0.98 \\ 
  12 & LME & sigma & beta=1.5 & sigma=1 & n=100 & 1.33 \\ 
  13 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=1 & n=100 & 1.55 \\ 
  14 & MDE.Phi.tv & sigma & beta=1.5 & sigma=1 & n=100 & 1.83 \\ 
  15 & MDE.Phi.kl & sigma & beta=1.5 & sigma=1 & n=100 & 1.18 \\ 
  16 & MME & sigma & beta=1.5 & sigma=1 & n=100 & 3.15 \\ 
  17 & MME.b & sigma & beta=1.5 & sigma=1 & n=100 & 6.83 \\ 
  18 & PWM & sigma & beta=1.5 & sigma=1 & n=100 & 1.33 \\ 
  19 & MLE & beta & beta=2 & sigma=1 & n=100 & 3.20 \\ 
  20 & MLE.b & beta & beta=2 & sigma=1 & n=100 & 2.85 \\ 
  21 & LME & beta & beta=2 & sigma=1 & n=100 & 2.45 \\ 
  22 & MDE.Phi.chisq & beta & beta=2 & sigma=1 & n=100 & 2.15 \\ 
  23 & MDE.Phi.tv & beta & beta=2 & sigma=1 & n=100 & 2.77 \\ 
  24 & MDE.Phi.kl & beta & beta=2 & sigma=1 & n=100 & 2.47 \\ 
  25 & MME & beta & beta=2 & sigma=1 & n=100 & 3.68 \\ 
  26 & MME.b & beta & beta=2 & sigma=1 & n=100 & 9.48 \\ 
  27 & PWM & beta & beta=2 & sigma=1 & n=100 & 2.45 \\ 
  28 & MLE & sigma & beta=2 & sigma=1 & n=100 & 1.75 \\ 
  29 & MLE.b & sigma & beta=2 & sigma=1 & n=100 & 1.49 \\ 
  30 & LME & sigma & beta=2 & sigma=1 & n=100 & 1.30 \\ 
  31 & MDE.Phi.chisq & sigma & beta=2 & sigma=1 & n=100 & 2.15 \\ 
  32 & MDE.Phi.tv & sigma & beta=2 & sigma=1 & n=100 & 2.68 \\ 
  33 & MDE.Phi.kl & sigma & beta=2 & sigma=1 & n=100 & 1.33 \\ 
  34 & MME & sigma & beta=2 & sigma=1 & n=100 & 2.44 \\ 
  35 & MME.b & sigma & beta=2 & sigma=1 & n=100 & 6.59 \\ 
  36 & PWM & sigma & beta=2 & sigma=1 & n=100 & 1.30 \\ 
  37 & MLE & beta & beta=2.5 & sigma=1 & n=100 & 4.95 \\ 
  38 & MLE.b & beta & beta=2.5 & sigma=1 & n=100 & 4.49 \\ 
  39 & LME & beta & beta=2.5 & sigma=1 & n=100 & 3.20 \\ 
  40 & MDE.Phi.chisq & beta & beta=2.5 & sigma=1 & n=100 & 4.31 \\ 
  41 & MDE.Phi.tv & beta & beta=2.5 & sigma=1 & n=100 & 5.15 \\ 
  42 & MDE.Phi.kl & beta & beta=2.5 & sigma=1 & n=100 & 3.45 \\ 
  43 & MME & beta & beta=2.5 & sigma=1 & n=100 & 4.82 \\ 
  44 & MME.b & beta & beta=2.5 & sigma=1 & n=100 & 7.99 \\ 
  45 & PWM & beta & beta=2.5 & sigma=1 & n=100 & 3.20 \\ 
  46 & MLE & sigma & beta=2.5 & sigma=1 & n=100 & 2.32 \\ 
  47 & MLE.b & sigma & beta=2.5 & sigma=1 & n=100 & 2.07 \\ 
  48 & LME & sigma & beta=2.5 & sigma=1 & n=100 & 1.36 \\ 
  49 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=1 & n=100 & 3.23 \\ 
  50 & MDE.Phi.tv & sigma & beta=2.5 & sigma=1 & n=100 & 3.77 \\ 
  51 & MDE.Phi.kl & sigma & beta=2.5 & sigma=1 & n=100 & 1.51 \\ 
  52 & MME & sigma & beta=2.5 & sigma=1 & n=100 & 2.35 \\ 
  53 & MME.b & sigma & beta=2.5 & sigma=1 & n=100 & 4.02 \\ 
  54 & PWM & sigma & beta=2.5 & sigma=1 & n=100 & 1.36 \\ 
  55 & MLE & beta & beta=3 & sigma=1 & n=100 & 13.45 \\ 
  56 & MLE.b & beta & beta=3 & sigma=1 & n=100 & 12.96 \\ 
  57 & LME & beta & beta=3 & sigma=1 & n=100 & 4.02 \\ 
  58 & MDE.Phi.chisq & beta & beta=3 & sigma=1 & n=100 & 7.28 \\ 
  59 & MDE.Phi.tv & beta & beta=3 & sigma=1 & n=100 & 8.76 \\ 
  60 & MDE.Phi.kl & beta & beta=3 & sigma=1 & n=100 & 4.92 \\ 
  61 & MME & beta & beta=3 & sigma=1 & n=100 & 17.49 \\ 
  62 & MME.b & beta & beta=3 & sigma=1 & n=100 & 49.99 \\ 
  63 & PWM & beta & beta=3 & sigma=1 & n=100 & 4.02 \\ 
  64 & MLE & sigma & beta=3 & sigma=1 & n=100 & 5.56 \\ 
  65 & MLE.b & sigma & beta=3 & sigma=1 & n=100 & 5.35 \\ 
  66 & LME & sigma & beta=3 & sigma=1 & n=100 & 1.43 \\ 
  67 & MDE.Phi.chisq & sigma & beta=3 & sigma=1 & n=100 & 4.41 \\ 
  68 & MDE.Phi.tv & sigma & beta=3 & sigma=1 & n=100 & 5.17 \\ 
  69 & MDE.Phi.kl & sigma & beta=3 & sigma=1 & n=100 & 1.83 \\ 
  70 & MME & sigma & beta=3 & sigma=1 & n=100 & 6.74 \\ 
  71 & MME.b & sigma & beta=3 & sigma=1 & n=100 & 19.57 \\ 
  72 & PWM & sigma & beta=3 & sigma=1 & n=100 & 1.43 \\ 
  73 & MLE & beta & beta=4 & sigma=1 & n=100 & 19.06 \\ 
  74 & MLE.b & beta & beta=4 & sigma=1 & n=100 & 18.61 \\ 
  75 & LME & beta & beta=4 & sigma=1 & n=100 & 5.76 \\ 
  76 & MDE.Phi.chisq & beta & beta=4 & sigma=1 & n=100 & 14.92 \\ 
  77 & MDE.Phi.tv & beta & beta=4 & sigma=1 & n=100 & 17.28 \\ 
  78 & MDE.Phi.kl & beta & beta=4 & sigma=1 & n=100 & 7.52 \\ 
  79 & MME & beta & beta=4 & sigma=1 & n=100 & 11.36 \\ 
  80 & MME.b & beta & beta=4 & sigma=1 & n=100 & 40.91 \\ 
  81 & PWM & beta & beta=4 & sigma=1 & n=100 & 5.76 \\ 
  82 & MLE & sigma & beta=4 & sigma=1 & n=100 & 5.59 \\ 
  83 & MLE.b & sigma & beta=4 & sigma=1 & n=100 & 5.45 \\ 
  84 & LME & sigma & beta=4 & sigma=1 & n=100 & 1.54 \\ 
  85 & MDE.Phi.chisq & sigma & beta=4 & sigma=1 & n=100 & 6.42 \\ 
  86 & MDE.Phi.tv & sigma & beta=4 & sigma=1 & n=100 & 7.20 \\ 
  87 & MDE.Phi.kl & sigma & beta=4 & sigma=1 & n=100 & 2.09 \\ 
  88 & MME & sigma & beta=4 & sigma=1 & n=100 & 3.33 \\ 
  89 & MME.b & sigma & beta=4 & sigma=1 & n=100 & 13.43 \\ 
  90 & PWM & sigma & beta=4 & sigma=1 & n=100 & 1.54 \\ 
  91 & MLE & beta & beta=5 & sigma=1 & n=100 & 30.61 \\ 
  92 & MLE.b & beta & beta=5 & sigma=1 & n=100 & 30.24 \\ 
  93 & LME & beta & beta=5 & sigma=1 & n=100 & 7.41 \\ 
  94 & MDE.Phi.chisq & beta & beta=5 & sigma=1 & n=100 & 22.00 \\ 
  95 & MDE.Phi.tv & beta & beta=5 & sigma=1 & n=100 & 24.36 \\ 
  96 & MDE.Phi.kl & beta & beta=5 & sigma=1 & n=100 & 10.27 \\ 
  97 & MME & beta & beta=5 & sigma=1 & n=100 & 16.76 \\ 
  98 & MME.b & beta & beta=5 & sigma=1 & n=100 & 47.23 \\ 
  99 & PWM & beta & beta=5 & sigma=1 & n=100 & 7.41 \\ 
  100 & MLE & sigma & beta=5 & sigma=1 & n=100 & 7.07 \\ 
  101 & MLE.b & sigma & beta=5 & sigma=1 & n=100 & 6.98 \\ 
  102 & LME & sigma & beta=5 & sigma=1 & n=100 & 1.56 \\ 
  103 & MDE.Phi.chisq & sigma & beta=5 & sigma=1 & n=100 & 7.23 \\ 
  104 & MDE.Phi.tv & sigma & beta=5 & sigma=1 & n=100 & 7.77 \\ 
  105 & MDE.Phi.kl & sigma & beta=5 & sigma=1 & n=100 & 2.24 \\ 
  106 & MME & sigma & beta=5 & sigma=1 & n=100 & 3.76 \\ 
  107 & MME.b & sigma & beta=5 & sigma=1 & n=100 & 10.98 \\ 
  108 & PWM & sigma & beta=5 & sigma=1 & n=100 & 1.56 \\ 
  109 & MLE & beta & beta=1.5 & sigma=1 & n=200 & 1.58 \\ 
  110 & MLE.b & beta & beta=1.5 & sigma=1 & n=200 & 1.50 \\ 
  111 & LME & beta & beta=1.5 & sigma=1 & n=200 & 1.71 \\ 
  112 & MDE.Phi.chisq & beta & beta=1.5 & sigma=1 & n=200 & 0.85 \\ 
  113 & MDE.Phi.tv & beta & beta=1.5 & sigma=1 & n=200 & 1.01 \\ 
  114 & MDE.Phi.kl & beta & beta=1.5 & sigma=1 & n=200 & 1.58 \\ 
  115 & MME & beta & beta=1.5 & sigma=1 & n=200 & 2.50 \\ 
  116 & MME.b & beta & beta=1.5 & sigma=1 & n=200 & 2.30 \\ 
  117 & PWM & beta & beta=1.5 & sigma=1 & n=200 & 1.71 \\ 
  118 & MLE & sigma & beta=1.5 & sigma=1 & n=200 & 1.08 \\ 
  119 & MLE.b & sigma & beta=1.5 & sigma=1 & n=200 & 0.99 \\ 
  120 & LME & sigma & beta=1.5 & sigma=1 & n=200 & 1.20 \\ 
  121 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=1 & n=200 & 1.12 \\ 
  122 & MDE.Phi.tv & sigma & beta=1.5 & sigma=1 & n=200 & 1.25 \\ 
  123 & MDE.Phi.kl & sigma & beta=1.5 & sigma=1 & n=200 & 1.08 \\ 
  124 & MME & sigma & beta=1.5 & sigma=1 & n=200 & 2.79 \\ 
  125 & MME.b & sigma & beta=1.5 & sigma=1 & n=200 & 2.51 \\ 
  126 & PWM & sigma & beta=1.5 & sigma=1 & n=200 & 1.20 \\ 
  127 & MLE & beta & beta=2 & sigma=1 & n=200 & 2.14 \\ 
  128 & MLE.b & beta & beta=2 & sigma=1 & n=200 & 1.97 \\ 
  129 & LME & beta & beta=2 & sigma=1 & n=200 & 2.22 \\ 
  130 & MDE.Phi.chisq & beta & beta=2 & sigma=1 & n=200 & 1.35 \\ 
  131 & MDE.Phi.tv & beta & beta=2 & sigma=1 & n=200 & 1.56 \\ 
  132 & MDE.Phi.kl & beta & beta=2 & sigma=1 & n=200 & 2.14 \\ 
  133 & MME & beta & beta=2 & sigma=1 & n=200 & 2.97 \\ 
  134 & MME.b & beta & beta=2 & sigma=1 & n=200 & 2.69 \\ 
  135 & PWM & beta & beta=2 & sigma=1 & n=200 & 2.22 \\ 
  136 & MLE & sigma & beta=2 & sigma=1 & n=200 & 1.10 \\ 
  137 & MLE.b & sigma & beta=2 & sigma=1 & n=200 & 0.98 \\ 
  138 & LME & sigma & beta=2 & sigma=1 & n=200 & 1.14 \\ 
  139 & MDE.Phi.chisq & sigma & beta=2 & sigma=1 & n=200 & 1.17 \\ 
  140 & MDE.Phi.tv & sigma & beta=2 & sigma=1 & n=200 & 1.28 \\ 
  141 & MDE.Phi.kl & sigma & beta=2 & sigma=1 & n=200 & 1.10 \\ 
  142 & MME & sigma & beta=2 & sigma=1 & n=200 & 1.89 \\ 
  143 & MME.b & sigma & beta=2 & sigma=1 & n=200 & 1.65 \\ 
  144 & PWM & sigma & beta=2 & sigma=1 & n=200 & 1.14 \\ 
  145 & MLE & beta & beta=2.5 & sigma=1 & n=200 & 2.75 \\ 
  146 & MLE.b & beta & beta=2.5 & sigma=1 & n=200 & 2.45 \\ 
  147 & LME & beta & beta=2.5 & sigma=1 & n=200 & 2.78 \\ 
  148 & MDE.Phi.chisq & beta & beta=2.5 & sigma=1 & n=200 & 2.06 \\ 
  149 & MDE.Phi.tv & beta & beta=2.5 & sigma=1 & n=200 & 2.29 \\ 
  150 & MDE.Phi.kl & beta & beta=2.5 & sigma=1 & n=200 & 2.75 \\ 
  151 & MME & beta & beta=2.5 & sigma=1 & n=200 & 3.56 \\ 
  152 & MME.b & beta & beta=2.5 & sigma=1 & n=200 & 3.34 \\ 
  153 & PWM & beta & beta=2.5 & sigma=1 & n=200 & 2.78 \\ 
  154 & MLE & sigma & beta=2.5 & sigma=1 & n=200 & 1.14 \\ 
  155 & MLE.b & sigma & beta=2.5 & sigma=1 & n=200 & 0.97 \\ 
  156 & LME & sigma & beta=2.5 & sigma=1 & n=200 & 1.14 \\ 
  157 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=1 & n=200 & 1.36 \\ 
  158 & MDE.Phi.tv & sigma & beta=2.5 & sigma=1 & n=200 & 1.41 \\ 
  159 & MDE.Phi.kl & sigma & beta=2.5 & sigma=1 & n=200 & 1.14 \\ 
  160 & MME & sigma & beta=2.5 & sigma=1 & n=200 & 1.65 \\ 
  161 & MME.b & sigma & beta=2.5 & sigma=1 & n=200 & 1.51 \\ 
  162 & PWM & sigma & beta=2.5 & sigma=1 & n=200 & 1.14 \\ 
  163 & MLE & beta & beta=3 & sigma=1 & n=200 & 3.55 \\ 
  164 & MLE.b & beta & beta=3 & sigma=1 & n=200 & 3.09 \\ 
  165 & LME & beta & beta=3 & sigma=1 & n=200 & 3.45 \\ 
  166 & MDE.Phi.chisq & beta & beta=3 & sigma=1 & n=200 & 3.38 \\ 
  167 & MDE.Phi.tv & beta & beta=3 & sigma=1 & n=200 & 3.24 \\ 
  168 & MDE.Phi.kl & beta & beta=3 & sigma=1 & n=200 & 3.49 \\ 
  169 & MME & beta & beta=3 & sigma=1 & n=200 & 4.40 \\ 
  170 & MME.b & beta & beta=3 & sigma=1 & n=200 & 5.69 \\ 
  171 & PWM & beta & beta=3 & sigma=1 & n=200 & 3.45 \\ 
  172 & MLE & sigma & beta=3 & sigma=1 & n=200 & 1.24 \\ 
  173 & MLE.b & sigma & beta=3 & sigma=1 & n=200 & 1.04 \\ 
  174 & LME & sigma & beta=3 & sigma=1 & n=200 & 1.19 \\ 
  175 & MDE.Phi.chisq & sigma & beta=3 & sigma=1 & n=200 & 1.82 \\ 
  176 & MDE.Phi.tv & sigma & beta=3 & sigma=1 & n=200 & 1.61 \\ 
  177 & MDE.Phi.kl & sigma & beta=3 & sigma=1 & n=200 & 1.21 \\ 
  178 & MME & sigma & beta=3 & sigma=1 & n=200 & 1.65 \\ 
  179 & MME.b & sigma & beta=3 & sigma=1 & n=200 & 2.23 \\ 
  180 & PWM & sigma & beta=3 & sigma=1 & n=200 & 1.19 \\ 
  181 & MLE & beta & beta=4 & sigma=1 & n=200 & 5.54 \\ 
  182 & MLE.b & beta & beta=4 & sigma=1 & n=200 & 4.87 \\ 
  183 & LME & beta & beta=4 & sigma=1 & n=200 & 4.91 \\ 
  184 & MDE.Phi.chisq & beta & beta=4 & sigma=1 & n=200 & 8.12 \\ 
  185 & MDE.Phi.tv & beta & beta=4 & sigma=1 & n=200 & 7.21 \\ 
  186 & MDE.Phi.kl & beta & beta=4 & sigma=1 & n=200 & 5.27 \\ 
  187 & MME & beta & beta=4 & sigma=1 & n=200 & 6.64 \\ 
  188 & MME.b & beta & beta=4 & sigma=1 & n=200 & 13.69 \\ 
  189 & PWM & beta & beta=4 & sigma=1 & n=200 & 4.91 \\ 
  190 & MLE & sigma & beta=4 & sigma=1 & n=200 & 1.48 \\ 
  191 & MLE.b & sigma & beta=4 & sigma=1 & n=200 & 1.27 \\ 
  192 & LME & sigma & beta=4 & sigma=1 & n=200 & 1.28 \\ 
  193 & MDE.Phi.chisq & sigma & beta=4 & sigma=1 & n=200 & 3.17 \\ 
  194 & MDE.Phi.tv & sigma & beta=4 & sigma=1 & n=200 & 2.67 \\ 
  195 & MDE.Phi.kl & sigma & beta=4 & sigma=1 & n=200 & 1.39 \\ 
  196 & MME & sigma & beta=4 & sigma=1 & n=200 & 1.83 \\ 
  197 & MME.b & sigma & beta=4 & sigma=1 & n=200 & 4.13 \\ 
  198 & PWM & sigma & beta=4 & sigma=1 & n=200 & 1.28 \\ 
  199 & MLE & beta & beta=5 & sigma=1 & n=200 & 13.99 \\ 
  200 & MLE.b & beta & beta=5 & sigma=1 & n=200 & 13.28 \\ 
  201 & LME & beta & beta=5 & sigma=1 & n=200 & 6.81 \\ 
  202 & MDE.Phi.chisq & beta & beta=5 & sigma=1 & n=200 & 15.14 \\ 
  203 & MDE.Phi.tv & beta & beta=5 & sigma=1 & n=200 & 12.05 \\ 
  204 & MDE.Phi.kl & beta & beta=5 & sigma=1 & n=200 & 7.66 \\ 
  205 & MME & beta & beta=5 & sigma=1 & n=200 & 9.76 \\ 
  206 & MME.b & beta & beta=5 & sigma=1 & n=200 & 21.60 \\ 
  207 & PWM & beta & beta=5 & sigma=1 & n=200 & 6.81 \\ 
  208 & MLE & sigma & beta=5 & sigma=1 & n=200 & 3.08 \\ 
  209 & MLE.b & sigma & beta=5 & sigma=1 & n=200 & 2.91 \\ 
  210 & LME & sigma & beta=5 & sigma=1 & n=200 & 1.42 \\ 
  211 & MDE.Phi.chisq & sigma & beta=5 & sigma=1 & n=200 & 4.58 \\ 
  212 & MDE.Phi.tv & sigma & beta=5 & sigma=1 & n=200 & 3.46 \\ 
  213 & MDE.Phi.kl & sigma & beta=5 & sigma=1 & n=200 & 1.63 \\ 
  214 & MME & sigma & beta=5 & sigma=1 & n=200 & 2.13 \\ 
  215 & MME.b & sigma & beta=5 & sigma=1 & n=200 & 4.94 \\ 
  216 & PWM & sigma & beta=5 & sigma=1 & n=200 & 1.42 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220207/Output.mse.LaTeX.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Wed Feb 09 03:12:51 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=1 & n=100 & 0.46 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=1 & n=100 & 0.32 \\ 
  3 & LME & beta & beta=1.5 & sigma=1 & n=100 & 0.40 \\ 
  4 & MDE.Phi.chisq & beta & beta=1.5 & sigma=1 & n=100 & 12.92 \\ 
  5 & MDE.Phi.tv & beta & beta=1.5 & sigma=1 & n=100 & 8.13 \\ 
  6 & MDE.Phi.kl & beta & beta=1.5 & sigma=1 & n=100 & 0.46 \\ 
  7 & MME & beta & beta=1.5 & sigma=1 & n=100 & 2.57 \\ 
  8 & MME.b & beta & beta=1.5 & sigma=1 & n=100 & 130057.25 \\ 
  9 & PWM & beta & beta=1.5 & sigma=1 & n=100 & 0.40 \\ 
  10 & MLE & sigma & beta=1.5 & sigma=1 & n=100 & 0.52 \\ 
  11 & MLE.b & sigma & beta=1.5 & sigma=1 & n=100 & 0.36 \\ 
  12 & LME & sigma & beta=1.5 & sigma=1 & n=100 & 0.44 \\ 
  13 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=1 & n=100 & 22.40 \\ 
  14 & MDE.Phi.tv & sigma & beta=1.5 & sigma=1 & n=100 & 21.81 \\ 
  15 & MDE.Phi.kl & sigma & beta=1.5 & sigma=1 & n=100 & 0.52 \\ 
  16 & MME & sigma & beta=1.5 & sigma=1 & n=100 & 6.63 \\ 
  17 & MME.b & sigma & beta=1.5 & sigma=1 & n=100 & 148910.23 \\ 
  18 & PWM & sigma & beta=1.5 & sigma=1 & n=100 & 0.44 \\ 
  19 & MLE & beta & beta=2 & sigma=1 & n=100 & 4901.55 \\ 
  20 & MLE.b & beta & beta=2 & sigma=1 & n=100 & 4901.30 \\ 
  21 & LME & beta & beta=2 & sigma=1 & n=100 & 3.31 \\ 
  22 & MDE.Phi.chisq & beta & beta=2 & sigma=1 & n=100 & 79.26 \\ 
  23 & MDE.Phi.tv & beta & beta=2 & sigma=1 & n=100 & 107.06 \\ 
  24 & MDE.Phi.kl & beta & beta=2 & sigma=1 & n=100 & 14.38 \\ 
  25 & MME & beta & beta=2 & sigma=1 & n=100 & 55.69 \\ 
  26 & MME.b & beta & beta=2 & sigma=1 & n=100 & 151259.47 \\ 
  27 & PWM & beta & beta=2 & sigma=1 & n=100 & 3.31 \\ 
  28 & MLE & sigma & beta=2 & sigma=1 & n=100 & 1541.66 \\ 
  29 & MLE.b & sigma & beta=2 & sigma=1 & n=100 & 1541.52 \\ 
  30 & LME & sigma & beta=2 & sigma=1 & n=100 & 1.54 \\ 
  31 & MDE.Phi.chisq & sigma & beta=2 & sigma=1 & n=100 & 91.74 \\ 
  32 & MDE.Phi.tv & sigma & beta=2 & sigma=1 & n=100 & 118.22 \\ 
  33 & MDE.Phi.kl & sigma & beta=2 & sigma=1 & n=100 & 6.02 \\ 
  34 & MME & sigma & beta=2 & sigma=1 & n=100 & 24.92 \\ 
  35 & MME.b & sigma & beta=2 & sigma=1 & n=100 & 83571.71 \\ 
  36 & PWM & sigma & beta=2 & sigma=1 & n=100 & 1.54 \\ 
  37 & MLE & beta & beta=2.5 & sigma=1 & n=100 & 10482.38 \\ 
  38 & MLE.b & beta & beta=2.5 & sigma=1 & n=100 & 10482.26 \\ 
  39 & LME & beta & beta=2.5 & sigma=1 & n=100 & 8.83 \\ 
  40 & MDE.Phi.chisq & beta & beta=2.5 & sigma=1 & n=100 & 282.04 \\ 
  41 & MDE.Phi.tv & beta & beta=2.5 & sigma=1 & n=100 & 323.24 \\ 
  42 & MDE.Phi.kl & beta & beta=2.5 & sigma=1 & n=100 & 34.93 \\ 
  43 & MME & beta & beta=2.5 & sigma=1 & n=100 & 149.68 \\ 
  44 & MME.b & beta & beta=2.5 & sigma=1 & n=100 & 2235.69 \\ 
  45 & PWM & beta & beta=2.5 & sigma=1 & n=100 & 8.83 \\ 
  46 & MLE & sigma & beta=2.5 & sigma=1 & n=100 & 3099.72 \\ 
  47 & MLE.b & sigma & beta=2.5 & sigma=1 & n=100 & 3099.67 \\ 
  48 & LME & sigma & beta=2.5 & sigma=1 & n=100 & 2.38 \\ 
  49 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=1 & n=100 & 171.83 \\ 
  50 & MDE.Phi.tv & sigma & beta=2.5 & sigma=1 & n=100 & 195.89 \\ 
  51 & MDE.Phi.kl & sigma & beta=2.5 & sigma=1 & n=100 & 9.57 \\ 
  52 & MME & sigma & beta=2.5 & sigma=1 & n=100 & 39.37 \\ 
  53 & MME.b & sigma & beta=2.5 & sigma=1 & n=100 & 639.14 \\ 
  54 & PWM & sigma & beta=2.5 & sigma=1 & n=100 & 2.38 \\ 
  55 & MLE & beta & beta=3 & sigma=1 & n=100 & 67636.78 \\ 
  56 & MLE.b & beta & beta=3 & sigma=1 & n=100 & 67636.98 \\ 
  57 & LME & beta & beta=3 & sigma=1 & n=100 & 17.02 \\ 
  58 & MDE.Phi.chisq & beta & beta=3 & sigma=1 & n=100 & 624.43 \\ 
  59 & MDE.Phi.tv & beta & beta=3 & sigma=1 & n=100 & 754.62 \\ 
  60 & MDE.Phi.kl & beta & beta=3 & sigma=1 & n=100 & 123.94 \\ 
  61 & MME & beta & beta=3 & sigma=1 & n=100 & 313324.91 \\ 
  62 & MME.b & beta & beta=3 & sigma=1 & n=100 & 2979286.01 \\ 
  63 & PWM & beta & beta=3 & sigma=1 & n=100 & 17.02 \\ 
  64 & MLE & sigma & beta=3 & sigma=1 & n=100 & 13735.39 \\ 
  65 & MLE.b & sigma & beta=3 & sigma=1 & n=100 & 13735.42 \\ 
  66 & LME & sigma & beta=3 & sigma=1 & n=100 & 3.26 \\ 
  67 & MDE.Phi.chisq & sigma & beta=3 & sigma=1 & n=100 & 249.86 \\ 
  68 & MDE.Phi.tv & sigma & beta=3 & sigma=1 & n=100 & 294.63 \\ 
  69 & MDE.Phi.kl & sigma & beta=3 & sigma=1 & n=100 & 22.95 \\ 
  70 & MME & sigma & beta=3 & sigma=1 & n=100 & 45240.03 \\ 
  71 & MME.b & sigma & beta=3 & sigma=1 & n=100 & 430648.00 \\ 
  72 & PWM & sigma & beta=3 & sigma=1 & n=100 & 3.26 \\ 
  73 & MLE & beta & beta=4 & sigma=1 & n=100 & 105403.93 \\ 
  74 & MLE.b & beta & beta=4 & sigma=1 & n=100 & 105404.86 \\ 
  75 & LME & beta & beta=4 & sigma=1 & n=100 & 51.86 \\ 
  76 & MDE.Phi.chisq & beta & beta=4 & sigma=1 & n=100 & 1637.05 \\ 
  77 & MDE.Phi.tv & beta & beta=4 & sigma=1 & n=100 & 1917.41 \\ 
  78 & MDE.Phi.kl & beta & beta=4 & sigma=1 & n=100 & 244.56 \\ 
  79 & MME & beta & beta=4 & sigma=1 & n=100 & 11609.86 \\ 
  80 & MME.b & beta & beta=4 & sigma=1 & n=100 & 1922332.72 \\ 
  81 & PWM & beta & beta=4 & sigma=1 & n=100 & 51.86 \\ 
  82 & MLE & sigma & beta=4 & sigma=1 & n=100 & 9780.56 \\ 
  83 & MLE.b & sigma & beta=4 & sigma=1 & n=100 & 9780.64 \\ 
  84 & LME & sigma & beta=4 & sigma=1 & n=100 & 4.98 \\ 
  85 & MDE.Phi.chisq & sigma & beta=4 & sigma=1 & n=100 & 323.46 \\ 
  86 & MDE.Phi.tv & sigma & beta=4 & sigma=1 & n=100 & 358.68 \\ 
  87 & MDE.Phi.kl & sigma & beta=4 & sigma=1 & n=100 & 24.27 \\ 
  88 & MME & sigma & beta=4 & sigma=1 & n=100 & 1091.88 \\ 
  89 & MME.b & sigma & beta=4 & sigma=1 & n=100 & 270680.58 \\ 
  90 & PWM & sigma & beta=4 & sigma=1 & n=100 & 4.98 \\ 
  91 & MLE & beta & beta=5 & sigma=1 & n=100 & 183029.64 \\ 
  92 & MLE.b & beta & beta=5 & sigma=1 & n=100 & 183031.06 \\ 
  93 & LME & beta & beta=5 & sigma=1 & n=100 & 110.73 \\ 
  94 & MDE.Phi.chisq & beta & beta=5 & sigma=1 & n=100 & 2692.52 \\ 
  95 & MDE.Phi.tv & beta & beta=5 & sigma=1 & n=100 & 2969.26 \\ 
  96 & MDE.Phi.kl & beta & beta=5 & sigma=1 & n=100 & 438.04 \\ 
  97 & MME & beta & beta=5 & sigma=1 & n=100 & 18732.28 \\ 
  98 & MME.b & beta & beta=5 & sigma=1 & n=100 & 259627.66 \\ 
  99 & PWM & beta & beta=5 & sigma=1 & n=100 & 110.73 \\ 
  100 & MLE & sigma & beta=5 & sigma=1 & n=100 & 10426.88 \\ 
  101 & MLE.b & sigma & beta=5 & sigma=1 & n=100 & 10426.96 \\ 
  102 & LME & sigma & beta=5 & sigma=1 & n=100 & 6.10 \\ 
  103 & MDE.Phi.chisq & sigma & beta=5 & sigma=1 & n=100 & 307.30 \\ 
  104 & MDE.Phi.tv & sigma & beta=5 & sigma=1 & n=100 & 323.73 \\ 
  105 & MDE.Phi.kl & sigma & beta=5 & sigma=1 & n=100 & 24.13 \\ 
  106 & MME & sigma & beta=5 & sigma=1 & n=100 & 1044.65 \\ 
  107 & MME.b & sigma & beta=5 & sigma=1 & n=100 & 15546.03 \\ 
  108 & PWM & sigma & beta=5 & sigma=1 & n=100 & 6.10 \\ 
  109 & MLE & beta & beta=1.5 & sigma=1 & n=200 & 0.11 \\ 
  110 & MLE.b & beta & beta=1.5 & sigma=1 & n=200 & 0.08 \\ 
  111 & LME & beta & beta=1.5 & sigma=1 & n=200 & 0.15 \\ 
  112 & MDE.Phi.chisq & beta & beta=1.5 & sigma=1 & n=200 & 0.55 \\ 
  113 & MDE.Phi.tv & beta & beta=1.5 & sigma=1 & n=200 & 0.41 \\ 
  114 & MDE.Phi.kl & beta & beta=1.5 & sigma=1 & n=200 & 0.11 \\ 
  115 & MME & beta & beta=1.5 & sigma=1 & n=200 & 1.15 \\ 
  116 & MME.b & beta & beta=1.5 & sigma=1 & n=200 & 0.89 \\ 
  117 & PWM & beta & beta=1.5 & sigma=1 & n=200 & 0.15 \\ 
  118 & MLE & sigma & beta=1.5 & sigma=1 & n=200 & 0.12 \\ 
  119 & MLE.b & sigma & beta=1.5 & sigma=1 & n=200 & 0.08 \\ 
  120 & LME & sigma & beta=1.5 & sigma=1 & n=200 & 0.17 \\ 
  121 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=1 & n=200 & 0.24 \\ 
  122 & MDE.Phi.tv & sigma & beta=1.5 & sigma=1 & n=200 & 0.36 \\ 
  123 & MDE.Phi.kl & sigma & beta=1.5 & sigma=1 & n=200 & 0.12 \\ 
  124 & MME & sigma & beta=1.5 & sigma=1 & n=200 & 4.98 \\ 
  125 & MME.b & sigma & beta=1.5 & sigma=1 & n=200 & 4.16 \\ 
  126 & PWM & sigma & beta=1.5 & sigma=1 & n=200 & 0.17 \\ 
  127 & MLE & beta & beta=2 & sigma=1 & n=200 & 0.32 \\ 
  128 & MLE.b & beta & beta=2 & sigma=1 & n=200 & 0.19 \\ 
  129 & LME & beta & beta=2 & sigma=1 & n=200 & 0.35 \\ 
  130 & MDE.Phi.chisq & beta & beta=2 & sigma=1 & n=200 & 3.03 \\ 
  131 & MDE.Phi.tv & beta & beta=2 & sigma=1 & n=200 & 2.78 \\ 
  132 & MDE.Phi.kl & beta & beta=2 & sigma=1 & n=200 & 0.32 \\ 
  133 & MME & beta & beta=2 & sigma=1 & n=200 & 1.48 \\ 
  134 & MME.b & beta & beta=2 & sigma=1 & n=200 & 5.87 \\ 
  135 & PWM & beta & beta=2 & sigma=1 & n=200 & 0.35 \\ 
  136 & MLE & sigma & beta=2 & sigma=1 & n=200 & 0.16 \\ 
  137 & MLE.b & sigma & beta=2 & sigma=1 & n=200 & 0.09 \\ 
  138 & LME & sigma & beta=2 & sigma=1 & n=200 & 0.17 \\ 
  139 & MDE.Phi.chisq & sigma & beta=2 & sigma=1 & n=200 & 2.15 \\ 
  140 & MDE.Phi.tv & sigma & beta=2 & sigma=1 & n=200 & 2.80 \\ 
  141 & MDE.Phi.kl & sigma & beta=2 & sigma=1 & n=200 & 0.16 \\ 
  142 & MME & sigma & beta=2 & sigma=1 & n=200 & 1.07 \\ 
  143 & MME.b & sigma & beta=2 & sigma=1 & n=200 & 2.97 \\ 
  144 & PWM & sigma & beta=2 & sigma=1 & n=200 & 0.17 \\ 
  145 & MLE & beta & beta=2.5 & sigma=1 & n=200 & 1.18 \\ 
  146 & MLE.b & beta & beta=2.5 & sigma=1 & n=200 & 0.83 \\ 
  147 & LME & beta & beta=2.5 & sigma=1 & n=200 & 1.28 \\ 
  148 & MDE.Phi.chisq & beta & beta=2.5 & sigma=1 & n=200 & 22.25 \\ 
  149 & MDE.Phi.tv & beta & beta=2.5 & sigma=1 & n=200 & 16.67 \\ 
  150 & MDE.Phi.kl & beta & beta=2.5 & sigma=1 & n=200 & 1.18 \\ 
  151 & MME & beta & beta=2.5 & sigma=1 & n=200 & 2.90 \\ 
  152 & MME.b & beta & beta=2.5 & sigma=1 & n=200 & 44.44 \\ 
  153 & PWM & beta & beta=2.5 & sigma=1 & n=200 & 1.28 \\ 
  154 & MLE & sigma & beta=2.5 & sigma=1 & n=200 & 0.35 \\ 
  155 & MLE.b & sigma & beta=2.5 & sigma=1 & n=200 & 0.25 \\ 
  156 & LME & sigma & beta=2.5 & sigma=1 & n=200 & 0.36 \\ 
  157 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=1 & n=200 & 11.26 \\ 
  158 & MDE.Phi.tv & sigma & beta=2.5 & sigma=1 & n=200 & 8.16 \\ 
  159 & MDE.Phi.kl & sigma & beta=2.5 & sigma=1 & n=200 & 0.35 \\ 
  160 & MME & sigma & beta=2.5 & sigma=1 & n=200 & 0.96 \\ 
  161 & MME.b & sigma & beta=2.5 & sigma=1 & n=200 & 12.57 \\ 
  162 & PWM & sigma & beta=2.5 & sigma=1 & n=200 & 0.36 \\ 
  163 & MLE & beta & beta=3 & sigma=1 & n=200 & 64.69 \\ 
  164 & MLE.b & beta & beta=3 & sigma=1 & n=200 & 64.14 \\ 
  165 & LME & beta & beta=3 & sigma=1 & n=200 & 4.35 \\ 
  166 & MDE.Phi.chisq & beta & beta=3 & sigma=1 & n=200 & 111.20 \\ 
  167 & MDE.Phi.tv & beta & beta=3 & sigma=1 & n=200 & 52.14 \\ 
  168 & MDE.Phi.kl & beta & beta=3 & sigma=1 & n=200 & 8.59 \\ 
  169 & MME & beta & beta=3 & sigma=1 & n=200 & 74.99 \\ 
  170 & MME.b & beta & beta=3 & sigma=1 & n=200 & 7353.37 \\ 
  171 & PWM & beta & beta=3 & sigma=1 & n=200 & 4.35 \\ 
  172 & MLE & sigma & beta=3 & sigma=1 & n=200 & 10.44 \\ 
  173 & MLE.b & sigma & beta=3 & sigma=1 & n=200 & 10.33 \\ 
  174 & LME & sigma & beta=3 & sigma=1 & n=200 & 0.78 \\ 
  175 & MDE.Phi.chisq & sigma & beta=3 & sigma=1 & n=200 & 37.21 \\ 
  176 & MDE.Phi.tv & sigma & beta=3 & sigma=1 & n=200 & 16.26 \\ 
  177 & MDE.Phi.kl & sigma & beta=3 & sigma=1 & n=200 & 1.52 \\ 
  178 & MME & sigma & beta=3 & sigma=1 & n=200 & 12.28 \\ 
  179 & MME.b & sigma & beta=3 & sigma=1 & n=200 & 1682.84 \\ 
  180 & PWM & sigma & beta=3 & sigma=1 & n=200 & 0.78 \\ 
  181 & MLE & beta & beta=4 & sigma=1 & n=200 & 361.31 \\ 
  182 & MLE.b & beta & beta=4 & sigma=1 & n=200 & 361.14 \\ 
  183 & LME & beta & beta=4 & sigma=1 & n=200 & 18.28 \\ 
  184 & MDE.Phi.chisq & beta & beta=4 & sigma=1 & n=200 & 603.85 \\ 
  185 & MDE.Phi.tv & beta & beta=4 & sigma=1 & n=200 & 439.21 \\ 
  186 & MDE.Phi.kl & beta & beta=4 & sigma=1 & n=200 & 47.87 \\ 
  187 & MME & beta & beta=4 & sigma=1 & n=200 & 550.99 \\ 
  188 & MME.b & beta & beta=4 & sigma=1 & n=200 & 40296.90 \\ 
  189 & PWM & beta & beta=4 & sigma=1 & n=200 & 18.28 \\ 
  190 & MLE & sigma & beta=4 & sigma=1 & n=200 & 34.91 \\ 
  191 & MLE.b & sigma & beta=4 & sigma=1 & n=200 & 34.89 \\ 
  192 & LME & sigma & beta=4 & sigma=1 & n=200 & 1.71 \\ 
  193 & MDE.Phi.chisq & sigma & beta=4 & sigma=1 & n=200 & 100.47 \\ 
  194 & MDE.Phi.tv & sigma & beta=4 & sigma=1 & n=200 & 70.84 \\ 
  195 & MDE.Phi.kl & sigma & beta=4 & sigma=1 & n=200 & 4.52 \\ 
  196 & MME & sigma & beta=4 & sigma=1 & n=200 & 53.42 \\ 
  197 & MME.b & sigma & beta=4 & sigma=1 & n=200 & 4952.00 \\ 
  198 & PWM & sigma & beta=4 & sigma=1 & n=200 & 1.71 \\ 
  199 & MLE & beta & beta=5 & sigma=1 & n=200 & 73565.55 \\ 
  200 & MLE.b & beta & beta=5 & sigma=1 & n=200 & 73566.41 \\ 
  201 & LME & beta & beta=5 & sigma=1 & n=200 & 71.77 \\ 
  202 & MDE.Phi.chisq & beta & beta=5 & sigma=1 & n=200 & 1551.11 \\ 
  203 & MDE.Phi.tv & beta & beta=5 & sigma=1 & n=200 & 1026.74 \\ 
  204 & MDE.Phi.kl & beta & beta=5 & sigma=1 & n=200 & 159.94 \\ 
  205 & MME & beta & beta=5 & sigma=1 & n=200 & 2746.16 \\ 
  206 & MME.b & beta & beta=5 & sigma=1 & n=200 & 30985.72 \\ 
  207 & PWM & beta & beta=5 & sigma=1 & n=200 & 71.77 \\ 
  208 & MLE & sigma & beta=5 & sigma=1 & n=200 & 3824.83 \\ 
  209 & MLE.b & sigma & beta=5 & sigma=1 & n=200 & 3824.87 \\ 
  210 & LME & sigma & beta=5 & sigma=1 & n=200 & 4.03 \\ 
  211 & MDE.Phi.chisq & sigma & beta=5 & sigma=1 & n=200 & 151.76 \\ 
  212 & MDE.Phi.tv & sigma & beta=5 & sigma=1 & n=200 & 95.05 \\ 
  213 & MDE.Phi.kl & sigma & beta=5 & sigma=1 & n=200 & 8.91 \\ 
  214 & MME & sigma & beta=5 & sigma=1 & n=200 & 149.32 \\ 
  215 & MME.b & sigma & beta=5 & sigma=1 & n=200 & 1752.71 \\ 
  216 & PWM & sigma & beta=5 & sigma=1 & n=200 & 4.03 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220207/Output.var.LaTeX.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Wed Feb 09 03:12:51 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=1 & n=100 & 0.44 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=1 & n=100 & 0.32 \\ 
  3 & LME & beta & beta=1.5 & sigma=1 & n=100 & 0.30 \\ 
  4 & MDE.Phi.chisq & beta & beta=1.5 & sigma=1 & n=100 & 12.66 \\ 
  5 & MDE.Phi.tv & beta & beta=1.5 & sigma=1 & n=100 & 8.07 \\ 
  6 & MDE.Phi.kl & beta & beta=1.5 & sigma=1 & n=100 & 0.44 \\ 
  7 & MME & beta & beta=1.5 & sigma=1 & n=100 & 0.90 \\ 
  8 & MME.b & beta & beta=1.5 & sigma=1 & n=100 & 130047.07 \\ 
  9 & PWM & beta & beta=1.5 & sigma=1 & n=100 & 0.30 \\ 
  10 & MLE & sigma & beta=1.5 & sigma=1 & n=100 & 0.49 \\ 
  11 & MLE.b & sigma & beta=1.5 & sigma=1 & n=100 & 0.36 \\ 
  12 & LME & sigma & beta=1.5 & sigma=1 & n=100 & 0.33 \\ 
  13 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=1 & n=100 & 22.10 \\ 
  14 & MDE.Phi.tv & sigma & beta=1.5 & sigma=1 & n=100 & 21.12 \\ 
  15 & MDE.Phi.kl & sigma & beta=1.5 & sigma=1 & n=100 & 0.49 \\ 
  16 & MME & sigma & beta=1.5 & sigma=1 & n=100 & 1.99 \\ 
  17 & MME.b & sigma & beta=1.5 & sigma=1 & n=100 & 148891.08 \\ 
  18 & PWM & sigma & beta=1.5 & sigma=1 & n=100 & 0.33 \\ 
  19 & MLE & beta & beta=2 & sigma=1 & n=100 & 4900.60 \\ 
  20 & MLE.b & beta & beta=2 & sigma=1 & n=100 & 4901.06 \\ 
  21 & LME & beta & beta=2 & sigma=1 & n=100 & 3.11 \\ 
  22 & MDE.Phi.chisq & beta & beta=2 & sigma=1 & n=100 & 79.25 \\ 
  23 & MDE.Phi.tv & beta & beta=2 & sigma=1 & n=100 & 106.49 \\ 
  24 & MDE.Phi.kl & beta & beta=2 & sigma=1 & n=100 & 14.17 \\ 
  25 & MME & beta & beta=2 & sigma=1 & n=100 & 52.88 \\ 
  26 & MME.b & beta & beta=2 & sigma=1 & n=100 & 151218.71 \\ 
  27 & PWM & beta & beta=2 & sigma=1 & n=100 & 3.11 \\ 
  28 & MLE & sigma & beta=2 & sigma=1 & n=100 & 1541.26 \\ 
  29 & MLE.b & sigma & beta=2 & sigma=1 & n=100 & 1541.43 \\ 
  30 & LME & sigma & beta=2 & sigma=1 & n=100 & 1.45 \\ 
  31 & MDE.Phi.chisq & sigma & beta=2 & sigma=1 & n=100 & 90.42 \\ 
  32 & MDE.Phi.tv & sigma & beta=2 & sigma=1 & n=100 & 115.40 \\ 
  33 & MDE.Phi.kl & sigma & beta=2 & sigma=1 & n=100 & 5.92 \\ 
  34 & MME & sigma & beta=2 & sigma=1 & n=100 & 22.85 \\ 
  35 & MME.b & sigma & beta=2 & sigma=1 & n=100 & 83548.85 \\ 
  36 & PWM & sigma & beta=2 & sigma=1 & n=100 & 1.45 \\ 
  37 & MLE & beta & beta=2.5 & sigma=1 & n=100 & 10477.44 \\ 
  38 & MLE.b & beta & beta=2.5 & sigma=1 & n=100 & 10479.34 \\ 
  39 & LME & beta & beta=2.5 & sigma=1 & n=100 & 8.34 \\ 
  40 & MDE.Phi.chisq & beta & beta=2.5 & sigma=1 & n=100 & 278.80 \\ 
  41 & MDE.Phi.tv & beta & beta=2.5 & sigma=1 & n=100 & 316.26 \\ 
  42 & MDE.Phi.kl & beta & beta=2.5 & sigma=1 & n=100 & 34.03 \\ 
  43 & MME & beta & beta=2.5 & sigma=1 & n=100 & 144.30 \\ 
  44 & MME.b & beta & beta=2.5 & sigma=1 & n=100 & 2205.73 \\ 
  45 & PWM & beta & beta=2.5 & sigma=1 & n=100 & 8.34 \\ 
  46 & MLE & sigma & beta=2.5 & sigma=1 & n=100 & 3098.28 \\ 
  47 & MLE.b & sigma & beta=2.5 & sigma=1 & n=100 & 3098.83 \\ 
  48 & LME & sigma & beta=2.5 & sigma=1 & n=100 & 2.25 \\ 
  49 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=1 & n=100 & 166.88 \\ 
  50 & MDE.Phi.tv & sigma & beta=2.5 & sigma=1 & n=100 & 188.25 \\ 
  51 & MDE.Phi.kl & sigma & beta=2.5 & sigma=1 & n=100 & 9.31 \\ 
  52 & MME & sigma & beta=2.5 & sigma=1 & n=100 & 37.54 \\ 
  53 & MME.b & sigma & beta=2.5 & sigma=1 & n=100 & 630.07 \\ 
  54 & PWM & sigma & beta=2.5 & sigma=1 & n=100 & 2.25 \\ 
  55 & MLE & beta & beta=3 & sigma=1 & n=100 & 67534.30 \\ 
  56 & MLE.b & beta & beta=3 & sigma=1 & n=100 & 67544.59 \\ 
  57 & LME & beta & beta=3 & sigma=1 & n=100 & 15.99 \\ 
  58 & MDE.Phi.chisq & beta & beta=3 & sigma=1 & n=100 & 606.18 \\ 
  59 & MDE.Phi.tv & beta & beta=3 & sigma=1 & n=100 & 721.51 \\ 
  60 & MDE.Phi.kl & beta & beta=3 & sigma=1 & n=100 & 120.25 \\ 
  61 & MME & beta & beta=3 & sigma=1 & n=100 & 313146.34 \\ 
  62 & MME.b & beta & beta=3 & sigma=1 & n=100 & 2977375.72 \\ 
  63 & PWM & beta & beta=3 & sigma=1 & n=100 & 15.99 \\ 
  64 & MLE & sigma & beta=3 & sigma=1 & n=100 & 13715.94 \\ 
  65 & MLE.b & sigma & beta=3 & sigma=1 & n=100 & 13717.87 \\ 
  66 & LME & sigma & beta=3 & sigma=1 & n=100 & 3.08 \\ 
  67 & MDE.Phi.chisq & sigma & beta=3 & sigma=1 & n=100 & 238.26 \\ 
  68 & MDE.Phi.tv & sigma & beta=3 & sigma=1 & n=100 & 277.24 \\ 
  69 & MDE.Phi.kl & sigma & beta=3 & sigma=1 & n=100 & 22.26 \\ 
  70 & MME & sigma & beta=3 & sigma=1 & n=100 & 45211.58 \\ 
  71 & MME.b & sigma & beta=3 & sigma=1 & n=100 & 430346.24 \\ 
  72 & PWM & sigma & beta=3 & sigma=1 & n=100 & 3.08 \\ 
  73 & MLE & beta & beta=4 & sigma=1 & n=100 & 105187.76 \\ 
  74 & MLE.b & beta & beta=4 & sigma=1 & n=100 & 105202.02 \\ 
  75 & LME & beta & beta=4 & sigma=1 & n=100 & 48.77 \\ 
  76 & MDE.Phi.chisq & beta & beta=4 & sigma=1 & n=100 & 1518.05 \\ 
  77 & MDE.Phi.tv & beta & beta=4 & sigma=1 & n=100 & 1741.16 \\ 
  78 & MDE.Phi.kl & beta & beta=4 & sigma=1 & n=100 & 232.17 \\ 
  79 & MME & beta & beta=4 & sigma=1 & n=100 & 11556.91 \\ 
  80 & MME.b & beta & beta=4 & sigma=1 & n=100 & 1921162.31 \\ 
  81 & PWM & beta & beta=4 & sigma=1 & n=100 & 48.77 \\ 
  82 & MLE & sigma & beta=4 & sigma=1 & n=100 & 9760.47 \\ 
  83 & MLE.b & sigma & beta=4 & sigma=1 & n=100 & 9761.79 \\ 
  84 & LME & sigma & beta=4 & sigma=1 & n=100 & 4.69 \\ 
  85 & MDE.Phi.chisq & sigma & beta=4 & sigma=1 & n=100 & 294.11 \\ 
  86 & MDE.Phi.tv & sigma & beta=4 & sigma=1 & n=100 & 320.32 \\ 
  87 & MDE.Phi.kl & sigma & beta=4 & sigma=1 & n=100 & 23.07 \\ 
  88 & MME & sigma & beta=4 & sigma=1 & n=100 & 1086.55 \\ 
  89 & MME.b & sigma & beta=4 & sigma=1 & n=100 & 270553.04 \\ 
  90 & PWM & sigma & beta=4 & sigma=1 & n=100 & 4.69 \\ 
  91 & MLE & beta & beta=5 & sigma=1 & n=100 & 182392.02 \\ 
  92 & MLE.b & beta & beta=5 & sigma=1 & n=100 & 182412.16 \\ 
  93 & LME & beta & beta=5 & sigma=1 & n=100 & 104.92 \\ 
  94 & MDE.Phi.chisq & beta & beta=5 & sigma=1 & n=100 & 2403.78 \\ 
  95 & MDE.Phi.tv & beta & beta=5 & sigma=1 & n=100 & 2594.76 \\ 
  96 & MDE.Phi.kl & beta & beta=5 & sigma=1 & n=100 & 410.29 \\ 
  97 & MME & beta & beta=5 & sigma=1 & n=100 & 18595.78 \\ 
  98 & MME.b & beta & beta=5 & sigma=1 & n=100 & 257869.79 \\ 
  99 & PWM & beta & beta=5 & sigma=1 & n=100 & 104.92 \\ 
  100 & MLE & sigma & beta=5 & sigma=1 & n=100 & 10391.10 \\ 
  101 & MLE.b & sigma & beta=5 & sigma=1 & n=100 & 10392.21 \\ 
  102 & LME & sigma & beta=5 & sigma=1 & n=100 & 5.78 \\ 
  103 & MDE.Phi.chisq & sigma & beta=5 & sigma=1 & n=100 & 268.55 \\ 
  104 & MDE.Phi.tv & sigma & beta=5 & sigma=1 & n=100 & 277.98 \\ 
  105 & MDE.Phi.kl & sigma & beta=5 & sigma=1 & n=100 & 22.59 \\ 
  106 & MME & sigma & beta=5 & sigma=1 & n=100 & 1037.16 \\ 
  107 & MME.b & sigma & beta=5 & sigma=1 & n=100 & 15447.94 \\ 
  108 & PWM & sigma & beta=5 & sigma=1 & n=100 & 5.78 \\ 
  109 & MLE & beta & beta=1.5 & sigma=1 & n=200 & 0.10 \\ 
  110 & MLE.b & beta & beta=1.5 & sigma=1 & n=200 & 0.08 \\ 
  111 & LME & beta & beta=1.5 & sigma=1 & n=200 & 0.11 \\ 
  112 & MDE.Phi.chisq & beta & beta=1.5 & sigma=1 & n=200 & 0.12 \\ 
  113 & MDE.Phi.tv & beta & beta=1.5 & sigma=1 & n=200 & 0.17 \\ 
  114 & MDE.Phi.kl & beta & beta=1.5 & sigma=1 & n=200 & 0.10 \\ 
  115 & MME & beta & beta=1.5 & sigma=1 & n=200 & 0.16 \\ 
  116 & MME.b & beta & beta=1.5 & sigma=1 & n=200 & 0.26 \\ 
  117 & PWM & beta & beta=1.5 & sigma=1 & n=200 & 0.11 \\ 
  118 & MLE & sigma & beta=1.5 & sigma=1 & n=200 & 0.11 \\ 
  119 & MLE.b & sigma & beta=1.5 & sigma=1 & n=200 & 0.08 \\ 
  120 & LME & sigma & beta=1.5 & sigma=1 & n=200 & 0.12 \\ 
  121 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=1 & n=200 & 0.22 \\ 
  122 & MDE.Phi.tv & sigma & beta=1.5 & sigma=1 & n=200 & 0.29 \\ 
  123 & MDE.Phi.kl & sigma & beta=1.5 & sigma=1 & n=200 & 0.11 \\ 
  124 & MME & sigma & beta=1.5 & sigma=1 & n=200 & 1.78 \\ 
  125 & MME.b & sigma & beta=1.5 & sigma=1 & n=200 & 1.87 \\ 
  126 & PWM & sigma & beta=1.5 & sigma=1 & n=200 & 0.12 \\ 
  127 & MLE & beta & beta=2 & sigma=1 & n=200 & 0.30 \\ 
  128 & MLE.b & beta & beta=2 & sigma=1 & n=200 & 0.19 \\ 
  129 & LME & beta & beta=2 & sigma=1 & n=200 & 0.30 \\ 
  130 & MDE.Phi.chisq & beta & beta=2 & sigma=1 & n=200 & 2.61 \\ 
  131 & MDE.Phi.tv & beta & beta=2 & sigma=1 & n=200 & 2.60 \\ 
  132 & MDE.Phi.kl & beta & beta=2 & sigma=1 & n=200 & 0.30 \\ 
  133 & MME & beta & beta=2 & sigma=1 & n=200 & 0.53 \\ 
  134 & MME.b & beta & beta=2 & sigma=1 & n=200 & 5.40 \\ 
  135 & PWM & beta & beta=2 & sigma=1 & n=200 & 0.30 \\ 
  136 & MLE & sigma & beta=2 & sigma=1 & n=200 & 0.15 \\ 
  137 & MLE.b & sigma & beta=2 & sigma=1 & n=200 & 0.09 \\ 
  138 & LME & sigma & beta=2 & sigma=1 & n=200 & 0.15 \\ 
  139 & MDE.Phi.chisq & sigma & beta=2 & sigma=1 & n=200 & 2.12 \\ 
  140 & MDE.Phi.tv & sigma & beta=2 & sigma=1 & n=200 & 2.72 \\ 
  141 & MDE.Phi.kl & sigma & beta=2 & sigma=1 & n=200 & 0.15 \\ 
  142 & MME & sigma & beta=2 & sigma=1 & n=200 & 0.28 \\ 
  143 & MME.b & sigma & beta=2 & sigma=1 & n=200 & 2.55 \\ 
  144 & PWM & sigma & beta=2 & sigma=1 & n=200 & 0.15 \\ 
  145 & MLE & beta & beta=2.5 & sigma=1 & n=200 & 1.12 \\ 
  146 & MLE.b & beta & beta=2.5 & sigma=1 & n=200 & 0.83 \\ 
  147 & LME & beta & beta=2.5 & sigma=1 & n=200 & 1.20 \\ 
  148 & MDE.Phi.chisq & beta & beta=2.5 & sigma=1 & n=200 & 22.07 \\ 
  149 & MDE.Phi.tv & beta & beta=2.5 & sigma=1 & n=200 & 16.63 \\ 
  150 & MDE.Phi.kl & beta & beta=2.5 & sigma=1 & n=200 & 1.12 \\ 
  151 & MME & beta & beta=2.5 & sigma=1 & n=200 & 1.77 \\ 
  152 & MME.b & beta & beta=2.5 & sigma=1 & n=200 & 43.75 \\ 
  153 & PWM & beta & beta=2.5 & sigma=1 & n=200 & 1.20 \\ 
  154 & MLE & sigma & beta=2.5 & sigma=1 & n=200 & 0.33 \\ 
  155 & MLE.b & sigma & beta=2.5 & sigma=1 & n=200 & 0.25 \\ 
  156 & LME & sigma & beta=2.5 & sigma=1 & n=200 & 0.34 \\ 
  157 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=1 & n=200 & 11.13 \\ 
  158 & MDE.Phi.tv & sigma & beta=2.5 & sigma=1 & n=200 & 7.99 \\ 
  159 & MDE.Phi.kl & sigma & beta=2.5 & sigma=1 & n=200 & 0.33 \\ 
  160 & MME & sigma & beta=2.5 & sigma=1 & n=200 & 0.53 \\ 
  161 & MME.b & sigma & beta=2.5 & sigma=1 & n=200 & 12.32 \\ 
  162 & PWM & sigma & beta=2.5 & sigma=1 & n=200 & 0.34 \\ 
  163 & MLE & beta & beta=3 & sigma=1 & n=200 & 64.39 \\ 
  164 & MLE.b & beta & beta=3 & sigma=1 & n=200 & 64.13 \\ 
  165 & LME & beta & beta=3 & sigma=1 & n=200 & 4.14 \\ 
  166 & MDE.Phi.chisq & beta & beta=3 & sigma=1 & n=200 & 111.07 \\ 
  167 & MDE.Phi.tv & beta & beta=3 & sigma=1 & n=200 & 52.09 \\ 
  168 & MDE.Phi.kl & beta & beta=3 & sigma=1 & n=200 & 8.35 \\ 
  169 & MME & beta & beta=3 & sigma=1 & n=200 & 73.03 \\ 
  170 & MME.b & beta & beta=3 & sigma=1 & n=200 & 7346.85 \\ 
  171 & PWM & beta & beta=3 & sigma=1 & n=200 & 4.14 \\ 
  172 & MLE & sigma & beta=3 & sigma=1 & n=200 & 10.38 \\ 
  173 & MLE.b & sigma & beta=3 & sigma=1 & n=200 & 10.33 \\ 
  174 & LME & sigma & beta=3 & sigma=1 & n=200 & 0.74 \\ 
  175 & MDE.Phi.chisq & sigma & beta=3 & sigma=1 & n=200 & 36.55 \\ 
  176 & MDE.Phi.tv & sigma & beta=3 & sigma=1 & n=200 & 15.88 \\ 
  177 & MDE.Phi.kl & sigma & beta=3 & sigma=1 & n=200 & 1.47 \\ 
  178 & MME & sigma & beta=3 & sigma=1 & n=200 & 11.86 \\ 
  179 & MME.b & sigma & beta=3 & sigma=1 & n=200 & 1681.49 \\ 
  180 & PWM & sigma & beta=3 & sigma=1 & n=200 & 0.74 \\ 
  181 & MLE & beta & beta=4 & sigma=1 & n=200 & 358.97 \\ 
  182 & MLE.b & beta & beta=4 & sigma=1 & n=200 & 360.41 \\ 
  183 & LME & beta & beta=4 & sigma=1 & n=200 & 17.45 \\ 
  184 & MDE.Phi.chisq & beta & beta=4 & sigma=1 & n=200 & 586.96 \\ 
  185 & MDE.Phi.tv & beta & beta=4 & sigma=1 & n=200 & 428.97 \\ 
  186 & MDE.Phi.kl & beta & beta=4 & sigma=1 & n=200 & 46.26 \\ 
  187 & MME & beta & beta=4 & sigma=1 & n=200 & 544.09 \\ 
  188 & MME.b & beta & beta=4 & sigma=1 & n=200 & 40207.11 \\ 
  189 & PWM & beta & beta=4 & sigma=1 & n=200 & 17.45 \\ 
  190 & MLE & sigma & beta=4 & sigma=1 & n=200 & 34.69 \\ 
  191 & MLE.b & sigma & beta=4 & sigma=1 & n=200 & 34.82 \\ 
  192 & LME & sigma & beta=4 & sigma=1 & n=200 & 1.64 \\ 
  193 & MDE.Phi.chisq & sigma & beta=4 & sigma=1 & n=200 & 95.79 \\ 
  194 & MDE.Phi.tv & sigma & beta=4 & sigma=1 & n=200 & 68.07 \\ 
  195 & MDE.Phi.kl & sigma & beta=4 & sigma=1 & n=200 & 4.37 \\ 
  196 & MME & sigma & beta=4 & sigma=1 & n=200 & 52.73 \\ 
  197 & MME.b & sigma & beta=4 & sigma=1 & n=200 & 4942.71 \\ 
  198 & PWM & sigma & beta=4 & sigma=1 & n=200 & 1.64 \\ 
  199 & MLE & beta & beta=5 & sigma=1 & n=200 & 73492.09 \\ 
  200 & MLE.b & beta & beta=5 & sigma=1 & n=200 & 73505.17 \\ 
  201 & LME & beta & beta=5 & sigma=1 & n=200 & 68.49 \\ 
  202 & MDE.Phi.chisq & beta & beta=5 & sigma=1 & n=200 & 1448.48 \\ 
  203 & MDE.Phi.tv & beta & beta=5 & sigma=1 & n=200 & 977.14 \\ 
  204 & MDE.Phi.kl & beta & beta=5 & sigma=1 & n=200 & 152.90 \\ 
  205 & MME & beta & beta=5 & sigma=1 & n=200 & 2723.74 \\ 
  206 & MME.b & beta & beta=5 & sigma=1 & n=200 & 30713.32 \\ 
  207 & PWM & beta & beta=5 & sigma=1 & n=200 & 68.49 \\ 
  208 & MLE & sigma & beta=5 & sigma=1 & n=200 & 3820.90 \\ 
  209 & MLE.b & sigma & beta=5 & sigma=1 & n=200 & 3821.61 \\ 
  210 & LME & sigma & beta=5 & sigma=1 & n=200 & 3.85 \\ 
  211 & MDE.Phi.chisq & sigma & beta=5 & sigma=1 & n=200 & 138.94 \\ 
  212 & MDE.Phi.tv & sigma & beta=5 & sigma=1 & n=200 & 88.99 \\ 
  213 & MDE.Phi.kl & sigma & beta=5 & sigma=1 & n=200 & 8.52 \\ 
  214 & MME & sigma & beta=5 & sigma=1 & n=200 & 148.05 \\ 
  215 & MME.b & sigma & beta=5 & sigma=1 & n=200 & 1737.36 \\ 
  216 & PWM & sigma & beta=5 & sigma=1 & n=200 & 3.85 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220208/20220208-11h11-Full.beta=1.5.sig=2.n=100.LaTeX.tex <==
% START DATE AND TIME=20220208-11h11
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=1.5,  \sigma=2$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.6717&1.4777&1.8288&0.234&1.257&1.6717&2.7927&6.3149&1.8288
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2.3645&1.9549&2.6507&3.2891&3.6444&2.3645&6.3049&13.6686&2.6507
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.4353&0.3215&0.2958&97.6125&6.7844&0.4354&0.8967&130047.0683&0.2958
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.9585&1.4466&1.33&82.0458&70.7652&1.9589&7.9695&595564.3219&1.33
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1717&-0.0223&0.3288&-1.266&-0.243&0.1717&1.2927&4.8149&0.3288
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.3645&-0.0451&0.6507&1.2891&1.6444&0.3645&4.3049&11.6686&0.6507
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.4647&0.322&0.4039&99.2056&6.8428&0.4648&2.5678&130057.2467&0.4039
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2.0911&1.4485&1.7532&83.6994&73.4621&2.0916&26.5012&595640.9217&1.7532
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 2.5559&1.7705&2.1571&182.9049&80.3048&2.5564&29.069&725698.1684&2.1571\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0011&0.0011&1.63885457077832e+301&0.0364&0.0011&0.0099&7.105&0.0011\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220208/20220208-11h11-Full.beta=1.5.sig=2.n=200.LaTeX.tex <==
% START DATE AND TIME=20220208-11h11
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=1.5,  \sigma=2$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.578&1.4952&1.7053&0.6454&1.004&1.578&2.4952&2.2961&1.7053
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2.1625&1.989&2.4046&2.3164&2.507&2.1626&5.5704&5.0195&2.4046
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1014&0.0768&0.1117&22.8262&0.1705&0.1014&0.1645&0.2553&0.1117
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.4329&0.3216&0.4944&3.3191&1.1627&0.4329&6.0718&6.4445&0.4944
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.078&-0.0048&0.2053&-0.8546&-0.496&0.078&0.9952&0.7961&0.2053
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.1625&-0.011&0.4046&0.3164&0.507&0.1626&3.5704&3.0195&0.4046
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1074&0.0768&0.1539&23.5542&0.4165&0.1075&1.1549&0.889&0.1539
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.4593&0.3216&0.6581&3.4189&1.4196&0.4593&18.8191&15.5612&0.6581
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 0.5667&0.3985&0.8119&26.9731&1.8362&0.5667&19.974&16.4502&0.8119\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 6e-04&6e-04&6e-04&2.74643118624275e+299&0.0276&6e-04&0.0089&0.0103&6e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220208/20220208-11h11-Full.beta=2.5.sig=2.n=100.LaTeX.tex <==
% START DATE AND TIME=20220208-11h11
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2.5,  \sigma=2$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 4.7183&4.261&3.1958&4.1065&4.9271&3.4377&4.8214&7.9937&3.1958
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
4.3927&3.8972&2.7184&6.1414&7.1933&3.0067&4.7089&8.0431&2.7184
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 7443.0404&7444.7345&8.3445&224.5742&256.6062&29.7786&144.3027&2205.727&8.3445
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
8765.6335&8767.5764&8.9937&535.712&611.3674&32.5838&150.1403&2520.2999&8.9937
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.2183&1.761&0.6958&1.6065&2.4271&0.9377&2.3214&5.4937&0.6958
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2.3927&1.8972&0.7184&4.1414&5.1933&1.0067&2.7089&6.0431&0.7184
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 7447.2168&7447.0913&8.8279&227.1324&262.4715&30.6549&149.6771&2235.6866&8.8279
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
8770.4822&8770.299&9.5089&552.8092&638.2771&33.5939&157.4634&2556.5675&9.5089
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 16217.6989&16217.3903&18.3368&779.9416&900.7486&64.2488&307.1405&4792.2541&18.3368\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0012&0.0011&0.0233&0.0179&0.0011&0.0019&8.078&0.0011\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220208/20220208-11h11-Full.beta=2.5.sig=2.n=200.LaTeX.tex <==
% START DATE AND TIME=20220208-11h11
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2.5,  \sigma=2$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.7518&2.4471&2.784&2.0498&2.2768&2.7518&3.5622&3.3354&2.784
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2.2713&1.9417&2.2893&2.7012&2.8083&2.2713&3.3094&3.0134&2.2893
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.1167&0.8305&1.1971&17.8817&13.8093&1.1167&1.774&43.7476&1.1971
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.3261&0.9894&1.3628&36.102&26.6172&1.3262&2.1291&49.2611&1.3628
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.2518&-0.0529&0.284&-0.4502&-0.2232&0.2518&1.0622&0.8354&0.284
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.2713&-0.0583&0.2893&0.7012&0.8083&0.2713&1.3094&1.0134&0.2893
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.18&0.8332&1.2776&18.0826&13.8577&1.18&2.9021&44.441&1.2776
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.3995&0.9927&1.4463&36.59&27.2679&1.3996&3.8434&50.2833&1.4463
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 2.5795&1.8259&2.724&54.6726&41.1256&2.5796&6.7455&94.7243&2.724\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&5e-04&5e-04&0.0174&0.0121&5e-04&0.0011&0.0017&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220208/20220208-11h11-Full.beta=2.sig=2.n=100.LaTeX.tex <==
% START DATE AND TIME=20220208-11h11
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2,  \sigma=2$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 3.0872&2.7376&2.4461&2.0969&2.6942&2.458&3.6775&9.4751&2.4461
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
3.3656&2.8604&2.6033&4.195&5.2184&2.6474&4.8746&13.1731&2.6033
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 3433.35&3433.7354&3.1121&65.3915&87.2818&12.1947&52.8831&151218.7131&3.1121
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
4325.4076&4325.974&5.78&298.7604&379.0939&20.4426&91.4156&334195.4082&5.78
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.0872&0.7376&0.4461&0.0969&0.6942&0.458&1.6775&7.4751&0.4461
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.3656&0.8604&0.6033&2.195&3.2184&0.6474&2.8746&11.1731&0.6033
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 3434.1887&3433.936&3.3109&65.3943&87.755&12.4033&55.6919&151259.4685&3.3109
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
4326.8399&4326.2816&6.1434&303.5485&389.4141&20.8597&99.6701&334286.8261&6.1434
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 7761.0286&7760.2176&9.4543&368.9428&477.169&33.263&155.3621&485546.2946&9.4543\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0011&0.0011&0.0296&0.0232&0.0011&0.0035&0.0115&0.0011\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220208/20220208-11h11-Full.beta=2.sig=2.n=200.LaTeX.tex <==
% START DATE AND TIME=20220208-11h11
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2,  \sigma=2$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.1373&1.9682&2.2157&1.3468&1.5634&2.1374&2.9722&2.6877&2.2157
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2.1929&1.9508&2.2838&2.3432&2.5561&2.1929&3.7771&3.293&2.2838
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.2964&0.1915&0.3034&2.1912&2.2108&0.2964&0.5321&5.3987&0.3034
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.5879&0.3739&0.5992&7.138&9.1449&0.5879&1.1111&10.202&0.5992
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1373&-0.0318&0.2157&-0.6532&-0.4366&0.1374&0.9722&0.6877&0.2157
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.1929&-0.0492&0.2838&0.3432&0.5561&0.1929&1.7771&1.293&0.2838
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.3153&0.1925&0.3499&2.6177&2.4012&0.3153&1.4772&5.8711&0.3499
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.625&0.3763&0.6797&7.2551&9.4533&0.625&4.269&11.8728&0.6797
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 0.9403&0.5688&1.0296&9.8728&11.8545&0.9403&5.7463&17.744&1.0296\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&5e-04&5e-04&0.0227&0.0165&5e-04&0.0024&0.0024&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220208/20220208-11h11-Full.beta=3.sig=2.n=100.LaTeX.tex <==
% START DATE AND TIME=20220208-11h11
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=3,  \sigma=2$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 12.4733&11.9791&4.0159&6.8159&8.2326&4.8603&17.4875&49.9897&4.0159
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
10.2262&9.7993&2.851&8.2493&9.7002&3.6029&13.4836&39.1376&2.851
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 52170.3557&52179.6787&15.9909&480.8982&575.7729&100.8592&313146.3373&2977375.7167&15.9909
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
41292.1587&41299.1152&12.3334&759.0983&886.5153&75.1257&180846.3382&1721384.9561&12.3334
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 9.4733&8.9791&1.0159&3.8159&5.2326&1.8603&14.4875&46.9897&1.0159
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
8.2262&7.7993&0.851&6.2493&7.7002&1.6029&11.4836&37.1376&0.851
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 52254.8816&52255.0848&17.0213&495.4112&603.0956&104.31&313324.9101&2979286.0078&17.0213
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
41355.6997&41355.8138&13.0565&798.0758&945.7205&77.6873&180960.127&1722592.0179&13.0565
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 93610.5813&93610.8986&30.0778&1293.487&1548.8161&181.9974&494285.0371&4701878.0258&30.0778\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0012&0.0011&0.0201&0.0151&0.0011&0.0014&0.0075&0.0011\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220208/20220208-11h11-Full.beta=3.sig=2.n=200.LaTeX.tex <==
% START DATE AND TIME=20220208-11h11
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=3,  \sigma=2$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 3.5547&3.0901&3.4535&3.3052&3.2069&3.4926&4.4031&5.6933&3.4535
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2.4753&2.073&2.3785&3.5428&3.1929&2.4257&3.2925&4.4634&2.3785
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 64.2408&63.9832&4.1441&89.0057&42.6911&7.7328&73.0305&7346.8537&4.1441
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
41.438&41.2309&2.9784&117.1409&52.0072&5.5021&47.4545&6725.9729&2.9784
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.5547&0.0901&0.4535&0.3052&0.2069&0.4926&1.4031&2.6933&0.4535
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.4753&0.073&0.3785&1.5428&1.1929&0.4257&1.2925&2.4634&0.3785
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 64.5421&63.9849&4.3493&89.09&42.7296&7.9746&74.9918&7353.3729&4.3493
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
41.6598&41.2321&3.1213&119.5094&53.4249&5.6827&49.1203&6731.3689&3.1213
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 106.2018&105.217&7.4706&208.5993&96.1546&13.6574&124.1121&14084.7417&7.4706\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&5e-04&5e-04&0.0143&0.0096&5e-04&7e-04&0.0018&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220208/20220208-11h11-Full.beta=4.sig=2.n=100.LaTeX.tex <==
% START DATE AND TIME=20220208-11h11
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=4,  \sigma=2$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 18.2759&17.8267&5.759&13.7651&15.9545&7.4212&11.3558&40.9124&5.759
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
10.6879&10.4155&3.0703&11.8342&13.2625&4.1216&6.6655&26.8679&3.0703
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 90920.5806&90934.1355&48.7724&1195.0428&1368.6343&201.2946&11556.9085&1921162.3133&48.7724
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
33275.6034&33280.5894&18.7607&926.7579&1007.8946&79.6118&4346.1835&1082212.1431&18.7607
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 14.2759&13.8267&1.759&9.7651&11.9545&3.4212&7.3558&36.9124&1.759
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
8.6879&8.4155&1.0703&9.8342&11.2625&2.1216&4.6655&24.8679&1.0703
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 91115.2897&91116.2199&51.8617&1290.2814&1511.4083&212.9789&11609.8605&1922332.7188&51.8617
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
33347.756&33348.0818&19.9043&1023.3773&1134.6382&84.1049&4367.5156&1082722.332&19.9043
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 124463.0457&124464.3018&71.766&2313.6587&2646.0465&297.0838&15977.3761&3005055.0508&71.766\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0012&0.001&0.0165&0.0123&0.0011&0.0011&4041.9544&0.001\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220208/20220208-11h11-Full.beta=4.sig=2.n=200.LaTeX.tex <==
% START DATE AND TIME=20220208-11h11
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=4,  \sigma=2$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 5.5418&4.8726&4.9145&7.7069&6.9491&5.2566&6.6372&13.6851&4.9145
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2.9524&2.5429&2.5529&6.0025&5.1303&2.7745&3.6618&8.2547&2.5529
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 358.4132&359.8562&17.4492&465.0781&346.1052&41.244&544.0894&40207.1182&17.4492
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
138.5354&139.0699&6.5508&303.5793&220.0039&15.5934&210.9218&19770.8596&6.5508
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.5418&0.8726&0.9145&3.7069&2.9491&1.2566&2.6372&9.6851&0.9145
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.9524&0.5429&0.5529&4.0025&3.1303&0.7745&1.6618&6.2547&0.5529
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 360.7545&360.5817&18.2837&478.7729&354.7677&42.8191&550.9901&40296.899&18.2837
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
139.4287&139.3507&6.8558&319.5687&229.7807&16.1917&213.6621&19808.0043&6.8558
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 500.1832&499.9325&25.1395&798.3416&584.5484&59.0108&764.6522&60104.9033&25.1395\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&6e-04&5e-04&0.0111&0.0074&5e-04&6e-04&0.0029&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220208/20220208-11h11-Full.beta=5.sig=2.n=100.LaTeX.tex <==
% START DATE AND TIME=20220208-11h11
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=5,  \sigma=2$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 29.6277&29.2594&7.3605&20.093&22.2436&10.0638&16.7262&47.1595&7.3605
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
13.6619&13.4907&3.101&13.1832&14.1594&4.3827&7.4959&21.9309&3.101
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 165313.7721&165333.2068&96.0976&1864.5133&2004.2157&347.2915&18587.8467&257840.1544&96.0976
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
37555.483&37559.7493&21.2623&832.8022&860.1424&76.9632&4147.1761&61786.3409&21.2623
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 24.6277&24.2594&2.3605&15.093&17.2436&5.0638&11.7262&42.1595&2.3605
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
11.6619&11.4907&1.101&11.1832&12.1594&2.3827&5.4959&19.9309&1.101
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 165903.7667&165905.1939&101.6601&2092.1268&2301.358&372.8992&18723.4925&259591.7905&101.6601
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
37687.7273&37688.0302&22.4723&957.7827&1007.9069&82.6327&4176.9667&62177.4021&22.4723
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 203591.4941&203593.2241&124.1323&3049.9096&3309.2649&455.5319&22900.4592&321769.1926&124.1323\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.001&0.0012&0.001&0.0144&0.0106&0.001&0.001&5.15620838018139e+29&0.001\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220208/20220208-11h11-Full.beta=5.sig=2.n=200.LaTeX.tex <==
% START DATE AND TIME=20220208-11h11
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=5,  \sigma=2$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 13.7199&13.0122&6.7803&14.1274&11.358&7.6&9.7618&21.5876&6.7803
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
6.0267&5.6931&2.8327&8.5388&6.5108&3.2262&4.2663&9.8745&2.8327
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 67107.264&67119.9688&63.0773&1137.0862&766.5447&134.8763&2723.7306&30712.8683&63.0773
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
13936.8904&13939.6462&14.1243&435.7651&279.1057&30.091&592.1845&6949.345&14.1243
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 8.7199&8.0122&1.7803&9.1274&6.358&2.6&4.7618&16.5876&1.7803
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
4.0267&3.6931&0.8327&6.5388&4.5108&1.2262&2.2663&7.8745&0.8327
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 67176.5903&67177.4527&66.2407&1220.2826&806.8926&141.6228&2746.133&30984.9451&66.2407
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
13951.711&13951.891&14.8163&478.4768&299.425&31.5915&597.2612&7010.6574&14.8163
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 81128.3013&81129.3437&81.057&1698.7594&1106.3177&173.2143&3343.3942&37995.6025&81.057\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&6e-04&5e-04&0.0096&0.0062&5e-04&5e-04&2.018&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220208/Output.accuracy.LaTeX.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Wed Feb 09 03:15:34 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & Measure & beta=1.5 & sigma=2 & n=100 & 2.56 \\ 
  2 & MLE.b & Measure & beta=1.5 & sigma=2 & n=100 & 1.77 \\ 
  3 & LME & Measure & beta=1.5 & sigma=2 & n=100 & 2.16 \\ 
  4 & MDE.Phi.chisq & Measure & beta=1.5 & sigma=2 & n=100 & 182.90 \\ 
  5 & MDE.Phi.tv & Measure & beta=1.5 & sigma=2 & n=100 & 80.30 \\ 
  6 & MDE.Phi.kl & Measure & beta=1.5 & sigma=2 & n=100 & 2.56 \\ 
  7 & MME & Measure & beta=1.5 & sigma=2 & n=100 & 29.07 \\ 
  8 & MME.b & Measure & beta=1.5 & sigma=2 & n=100 & 725698.17 \\ 
  9 & PWM & Measure & beta=1.5 & sigma=2 & n=100 & 2.16 \\ 
  10 & MLE & Measure & beta=2 & sigma=2 & n=100 & 7761.03 \\ 
  11 & MLE.b & Measure & beta=2 & sigma=2 & n=100 & 7760.22 \\ 
  12 & LME & Measure & beta=2 & sigma=2 & n=100 & 9.45 \\ 
  13 & MDE.Phi.chisq & Measure & beta=2 & sigma=2 & n=100 & 368.94 \\ 
  14 & MDE.Phi.tv & Measure & beta=2 & sigma=2 & n=100 & 477.17 \\ 
  15 & MDE.Phi.kl & Measure & beta=2 & sigma=2 & n=100 & 33.26 \\ 
  16 & MME & Measure & beta=2 & sigma=2 & n=100 & 155.36 \\ 
  17 & MME.b & Measure & beta=2 & sigma=2 & n=100 & 485546.29 \\ 
  18 & PWM & Measure & beta=2 & sigma=2 & n=100 & 9.45 \\ 
  19 & MLE & Measure & beta=2.5 & sigma=2 & n=100 & 16217.70 \\ 
  20 & MLE.b & Measure & beta=2.5 & sigma=2 & n=100 & 16217.39 \\ 
  21 & LME & Measure & beta=2.5 & sigma=2 & n=100 & 18.34 \\ 
  22 & MDE.Phi.chisq & Measure & beta=2.5 & sigma=2 & n=100 & 779.94 \\ 
  23 & MDE.Phi.tv & Measure & beta=2.5 & sigma=2 & n=100 & 900.75 \\ 
  24 & MDE.Phi.kl & Measure & beta=2.5 & sigma=2 & n=100 & 64.25 \\ 
  25 & MME & Measure & beta=2.5 & sigma=2 & n=100 & 307.14 \\ 
  26 & MME.b & Measure & beta=2.5 & sigma=2 & n=100 & 4792.25 \\ 
  27 & PWM & Measure & beta=2.5 & sigma=2 & n=100 & 18.34 \\ 
  28 & MLE & Measure & beta=3 & sigma=2 & n=100 & 93610.58 \\ 
  29 & MLE.b & Measure & beta=3 & sigma=2 & n=100 & 93610.90 \\ 
  30 & LME & Measure & beta=3 & sigma=2 & n=100 & 30.08 \\ 
  31 & MDE.Phi.chisq & Measure & beta=3 & sigma=2 & n=100 & 1293.49 \\ 
  32 & MDE.Phi.tv & Measure & beta=3 & sigma=2 & n=100 & 1548.82 \\ 
  33 & MDE.Phi.kl & Measure & beta=3 & sigma=2 & n=100 & 182.00 \\ 
  34 & MME & Measure & beta=3 & sigma=2 & n=100 & 494285.04 \\ 
  35 & MME.b & Measure & beta=3 & sigma=2 & n=100 & 4701878.03 \\ 
  36 & PWM & Measure & beta=3 & sigma=2 & n=100 & 30.08 \\ 
  37 & MLE & Measure & beta=4 & sigma=2 & n=100 & 124463.05 \\ 
  38 & MLE.b & Measure & beta=4 & sigma=2 & n=100 & 124464.30 \\ 
  39 & LME & Measure & beta=4 & sigma=2 & n=100 & 71.77 \\ 
  40 & MDE.Phi.chisq & Measure & beta=4 & sigma=2 & n=100 & 2313.66 \\ 
  41 & MDE.Phi.tv & Measure & beta=4 & sigma=2 & n=100 & 2646.05 \\ 
  42 & MDE.Phi.kl & Measure & beta=4 & sigma=2 & n=100 & 297.08 \\ 
  43 & MME & Measure & beta=4 & sigma=2 & n=100 & 15977.38 \\ 
  44 & MME.b & Measure & beta=4 & sigma=2 & n=100 & 3005055.05 \\ 
  45 & PWM & Measure & beta=4 & sigma=2 & n=100 & 71.77 \\ 
  46 & MLE & Measure & beta=5 & sigma=2 & n=100 & 203591.49 \\ 
  47 & MLE.b & Measure & beta=5 & sigma=2 & n=100 & 203593.22 \\ 
  48 & LME & Measure & beta=5 & sigma=2 & n=100 & 124.13 \\ 
  49 & MDE.Phi.chisq & Measure & beta=5 & sigma=2 & n=100 & 3049.91 \\ 
  50 & MDE.Phi.tv & Measure & beta=5 & sigma=2 & n=100 & 3309.26 \\ 
  51 & MDE.Phi.kl & Measure & beta=5 & sigma=2 & n=100 & 455.53 \\ 
  52 & MME & Measure & beta=5 & sigma=2 & n=100 & 22900.46 \\ 
  53 & MME.b & Measure & beta=5 & sigma=2 & n=100 & 321769.19 \\ 
  54 & PWM & Measure & beta=5 & sigma=2 & n=100 & 124.13 \\ 
  55 & MLE & Measure & beta=1.5 & sigma=2 & n=200 & 0.57 \\ 
  56 & MLE.b & Measure & beta=1.5 & sigma=2 & n=200 & 0.40 \\ 
  57 & LME & Measure & beta=1.5 & sigma=2 & n=200 & 0.81 \\ 
  58 & MDE.Phi.chisq & Measure & beta=1.5 & sigma=2 & n=200 & 26.97 \\ 
  59 & MDE.Phi.tv & Measure & beta=1.5 & sigma=2 & n=200 & 1.84 \\ 
  60 & MDE.Phi.kl & Measure & beta=1.5 & sigma=2 & n=200 & 0.57 \\ 
  61 & MME & Measure & beta=1.5 & sigma=2 & n=200 & 19.97 \\ 
  62 & MME.b & Measure & beta=1.5 & sigma=2 & n=200 & 16.45 \\ 
  63 & PWM & Measure & beta=1.5 & sigma=2 & n=200 & 0.81 \\ 
  64 & MLE & Measure & beta=2 & sigma=2 & n=200 & 0.94 \\ 
  65 & MLE.b & Measure & beta=2 & sigma=2 & n=200 & 0.57 \\ 
  66 & LME & Measure & beta=2 & sigma=2 & n=200 & 1.03 \\ 
  67 & MDE.Phi.chisq & Measure & beta=2 & sigma=2 & n=200 & 9.87 \\ 
  68 & MDE.Phi.tv & Measure & beta=2 & sigma=2 & n=200 & 11.85 \\ 
  69 & MDE.Phi.kl & Measure & beta=2 & sigma=2 & n=200 & 0.94 \\ 
  70 & MME & Measure & beta=2 & sigma=2 & n=200 & 5.75 \\ 
  71 & MME.b & Measure & beta=2 & sigma=2 & n=200 & 17.74 \\ 
  72 & PWM & Measure & beta=2 & sigma=2 & n=200 & 1.03 \\ 
  73 & MLE & Measure & beta=2.5 & sigma=2 & n=200 & 2.58 \\ 
  74 & MLE.b & Measure & beta=2.5 & sigma=2 & n=200 & 1.83 \\ 
  75 & LME & Measure & beta=2.5 & sigma=2 & n=200 & 2.72 \\ 
  76 & MDE.Phi.chisq & Measure & beta=2.5 & sigma=2 & n=200 & 54.67 \\ 
  77 & MDE.Phi.tv & Measure & beta=2.5 & sigma=2 & n=200 & 41.13 \\ 
  78 & MDE.Phi.kl & Measure & beta=2.5 & sigma=2 & n=200 & 2.58 \\ 
  79 & MME & Measure & beta=2.5 & sigma=2 & n=200 & 6.75 \\ 
  80 & MME.b & Measure & beta=2.5 & sigma=2 & n=200 & 94.72 \\ 
  81 & PWM & Measure & beta=2.5 & sigma=2 & n=200 & 2.72 \\ 
  82 & MLE & Measure & beta=3 & sigma=2 & n=200 & 106.20 \\ 
  83 & MLE.b & Measure & beta=3 & sigma=2 & n=200 & 105.22 \\ 
  84 & LME & Measure & beta=3 & sigma=2 & n=200 & 7.47 \\ 
  85 & MDE.Phi.chisq & Measure & beta=3 & sigma=2 & n=200 & 208.60 \\ 
  86 & MDE.Phi.tv & Measure & beta=3 & sigma=2 & n=200 & 96.15 \\ 
  87 & MDE.Phi.kl & Measure & beta=3 & sigma=2 & n=200 & 13.66 \\ 
  88 & MME & Measure & beta=3 & sigma=2 & n=200 & 124.11 \\ 
  89 & MME.b & Measure & beta=3 & sigma=2 & n=200 & 14084.74 \\ 
  90 & PWM & Measure & beta=3 & sigma=2 & n=200 & 7.47 \\ 
  91 & MLE & Measure & beta=4 & sigma=2 & n=200 & 500.18 \\ 
  92 & MLE.b & Measure & beta=4 & sigma=2 & n=200 & 499.93 \\ 
  93 & LME & Measure & beta=4 & sigma=2 & n=200 & 25.14 \\ 
  94 & MDE.Phi.chisq & Measure & beta=4 & sigma=2 & n=200 & 798.34 \\ 
  95 & MDE.Phi.tv & Measure & beta=4 & sigma=2 & n=200 & 584.55 \\ 
  96 & MDE.Phi.kl & Measure & beta=4 & sigma=2 & n=200 & 59.01 \\ 
  97 & MME & Measure & beta=4 & sigma=2 & n=200 & 764.65 \\ 
  98 & MME.b & Measure & beta=4 & sigma=2 & n=200 & 60104.90 \\ 
  99 & PWM & Measure & beta=4 & sigma=2 & n=200 & 25.14 \\ 
  100 & MLE & Measure & beta=5 & sigma=2 & n=200 & 81128.30 \\ 
  101 & MLE.b & Measure & beta=5 & sigma=2 & n=200 & 81129.34 \\ 
  102 & LME & Measure & beta=5 & sigma=2 & n=200 & 81.06 \\ 
  103 & MDE.Phi.chisq & Measure & beta=5 & sigma=2 & n=200 & 1698.76 \\ 
  104 & MDE.Phi.tv & Measure & beta=5 & sigma=2 & n=200 & 1106.32 \\ 
  105 & MDE.Phi.kl & Measure & beta=5 & sigma=2 & n=200 & 173.21 \\ 
  106 & MME & Measure & beta=5 & sigma=2 & n=200 & 3343.39 \\ 
  107 & MME.b & Measure & beta=5 & sigma=2 & n=200 & 37995.60 \\ 
  108 & PWM & Measure & beta=5 & sigma=2 & n=200 & 81.06 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220208/Output.accuracy2.LaTeX.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Wed Feb 09 03:15:34 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & Measure & beta=1.5 & sigma=2 & n=100 & 0.00 \\ 
  2 & MLE.b & Measure & beta=1.5 & sigma=2 & n=100 & 0.00 \\ 
  3 & LME & Measure & beta=1.5 & sigma=2 & n=100 & 0.00 \\ 
  4 & MDE.Phi.chisq & Measure & beta=1.5 & sigma=2 & n=100 & 16388545707783178620260440008882462028666402824264064840002848602064644026068422688648064042426000406008404624648684664024604240882802040402642024426044402280264208866460866204284608004000428088080204864660402422800606024068664422446222660000246464448602468622826028820882884204864628226040022026806066.00 \\ 
  5 & MDE.Phi.tv & Measure & beta=1.5 & sigma=2 & n=100 & 0.04 \\ 
  6 & MDE.Phi.kl & Measure & beta=1.5 & sigma=2 & n=100 & 0.00 \\ 
  7 & MME & Measure & beta=1.5 & sigma=2 & n=100 & 0.01 \\ 
  8 & MME.b & Measure & beta=1.5 & sigma=2 & n=100 & 7.11 \\ 
  9 & PWM & Measure & beta=1.5 & sigma=2 & n=100 & 0.00 \\ 
  10 & MLE & Measure & beta=2 & sigma=2 & n=100 & 0.00 \\ 
  11 & MLE.b & Measure & beta=2 & sigma=2 & n=100 & 0.00 \\ 
  12 & LME & Measure & beta=2 & sigma=2 & n=100 & 0.00 \\ 
  13 & MDE.Phi.chisq & Measure & beta=2 & sigma=2 & n=100 & 0.03 \\ 
  14 & MDE.Phi.tv & Measure & beta=2 & sigma=2 & n=100 & 0.02 \\ 
  15 & MDE.Phi.kl & Measure & beta=2 & sigma=2 & n=100 & 0.00 \\ 
  16 & MME & Measure & beta=2 & sigma=2 & n=100 & 0.00 \\ 
  17 & MME.b & Measure & beta=2 & sigma=2 & n=100 & 0.01 \\ 
  18 & PWM & Measure & beta=2 & sigma=2 & n=100 & 0.00 \\ 
  19 & MLE & Measure & beta=2.5 & sigma=2 & n=100 & 0.00 \\ 
  20 & MLE.b & Measure & beta=2.5 & sigma=2 & n=100 & 0.00 \\ 
  21 & LME & Measure & beta=2.5 & sigma=2 & n=100 & 0.00 \\ 
  22 & MDE.Phi.chisq & Measure & beta=2.5 & sigma=2 & n=100 & 0.02 \\ 
  23 & MDE.Phi.tv & Measure & beta=2.5 & sigma=2 & n=100 & 0.02 \\ 
  24 & MDE.Phi.kl & Measure & beta=2.5 & sigma=2 & n=100 & 0.00 \\ 
  25 & MME & Measure & beta=2.5 & sigma=2 & n=100 & 0.00 \\ 
  26 & MME.b & Measure & beta=2.5 & sigma=2 & n=100 & 8.08 \\ 
  27 & PWM & Measure & beta=2.5 & sigma=2 & n=100 & 0.00 \\ 
  28 & MLE & Measure & beta=3 & sigma=2 & n=100 & 0.00 \\ 
  29 & MLE.b & Measure & beta=3 & sigma=2 & n=100 & 0.00 \\ 
  30 & LME & Measure & beta=3 & sigma=2 & n=100 & 0.00 \\ 
  31 & MDE.Phi.chisq & Measure & beta=3 & sigma=2 & n=100 & 0.02 \\ 
  32 & MDE.Phi.tv & Measure & beta=3 & sigma=2 & n=100 & 0.02 \\ 
  33 & MDE.Phi.kl & Measure & beta=3 & sigma=2 & n=100 & 0.00 \\ 
  34 & MME & Measure & beta=3 & sigma=2 & n=100 & 0.00 \\ 
  35 & MME.b & Measure & beta=3 & sigma=2 & n=100 & 0.01 \\ 
  36 & PWM & Measure & beta=3 & sigma=2 & n=100 & 0.00 \\ 
  37 & MLE & Measure & beta=4 & sigma=2 & n=100 & 0.00 \\ 
  38 & MLE.b & Measure & beta=4 & sigma=2 & n=100 & 0.00 \\ 
  39 & LME & Measure & beta=4 & sigma=2 & n=100 & 0.00 \\ 
  40 & MDE.Phi.chisq & Measure & beta=4 & sigma=2 & n=100 & 0.02 \\ 
  41 & MDE.Phi.tv & Measure & beta=4 & sigma=2 & n=100 & 0.01 \\ 
  42 & MDE.Phi.kl & Measure & beta=4 & sigma=2 & n=100 & 0.00 \\ 
  43 & MME & Measure & beta=4 & sigma=2 & n=100 & 0.00 \\ 
  44 & MME.b & Measure & beta=4 & sigma=2 & n=100 & 4041.95 \\ 
  45 & PWM & Measure & beta=4 & sigma=2 & n=100 & 0.00 \\ 
  46 & MLE & Measure & beta=5 & sigma=2 & n=100 & 0.00 \\ 
  47 & MLE.b & Measure & beta=5 & sigma=2 & n=100 & 0.00 \\ 
  48 & LME & Measure & beta=5 & sigma=2 & n=100 & 0.00 \\ 
  49 & MDE.Phi.chisq & Measure & beta=5 & sigma=2 & n=100 & 0.01 \\ 
  50 & MDE.Phi.tv & Measure & beta=5 & sigma=2 & n=100 & 0.01 \\ 
  51 & MDE.Phi.kl & Measure & beta=5 & sigma=2 & n=100 & 0.00 \\ 
  52 & MME & Measure & beta=5 & sigma=2 & n=100 & 0.00 \\ 
  53 & MME.b & Measure & beta=5 & sigma=2 & n=100 & 515620838018138634806240604226.00 \\ 
  54 & PWM & Measure & beta=5 & sigma=2 & n=100 & 0.00 \\ 
  55 & MLE & Measure & beta=1.5 & sigma=2 & n=200 & 0.00 \\ 
  56 & MLE.b & Measure & beta=1.5 & sigma=2 & n=200 & 0.00 \\ 
  57 & LME & Measure & beta=1.5 & sigma=2 & n=200 & 0.00 \\ 
  58 & MDE.Phi.chisq & Measure & beta=1.5 & sigma=2 & n=200 & 274643118624275331360628286448288226248464468022642204668864084082600222086880608668040080880424622046222024608200240484826064404080888868246080264664220228006844402404026242842008664860822820666228446808646200060266406262242888228420024466628024282446084862640644224086266044024064680440202202400842.00 \\ 
  59 & MDE.Phi.tv & Measure & beta=1.5 & sigma=2 & n=200 & 0.03 \\ 
  60 & MDE.Phi.kl & Measure & beta=1.5 & sigma=2 & n=200 & 0.00 \\ 
  61 & MME & Measure & beta=1.5 & sigma=2 & n=200 & 0.01 \\ 
  62 & MME.b & Measure & beta=1.5 & sigma=2 & n=200 & 0.01 \\ 
  63 & PWM & Measure & beta=1.5 & sigma=2 & n=200 & 0.00 \\ 
  64 & MLE & Measure & beta=2 & sigma=2 & n=200 & 0.00 \\ 
  65 & MLE.b & Measure & beta=2 & sigma=2 & n=200 & 0.00 \\ 
  66 & LME & Measure & beta=2 & sigma=2 & n=200 & 0.00 \\ 
  67 & MDE.Phi.chisq & Measure & beta=2 & sigma=2 & n=200 & 0.02 \\ 
  68 & MDE.Phi.tv & Measure & beta=2 & sigma=2 & n=200 & 0.02 \\ 
  69 & MDE.Phi.kl & Measure & beta=2 & sigma=2 & n=200 & 0.00 \\ 
  70 & MME & Measure & beta=2 & sigma=2 & n=200 & 0.00 \\ 
  71 & MME.b & Measure & beta=2 & sigma=2 & n=200 & 0.00 \\ 
  72 & PWM & Measure & beta=2 & sigma=2 & n=200 & 0.00 \\ 
  73 & MLE & Measure & beta=2.5 & sigma=2 & n=200 & 0.00 \\ 
  74 & MLE.b & Measure & beta=2.5 & sigma=2 & n=200 & 0.00 \\ 
  75 & LME & Measure & beta=2.5 & sigma=2 & n=200 & 0.00 \\ 
  76 & MDE.Phi.chisq & Measure & beta=2.5 & sigma=2 & n=200 & 0.02 \\ 
  77 & MDE.Phi.tv & Measure & beta=2.5 & sigma=2 & n=200 & 0.01 \\ 
  78 & MDE.Phi.kl & Measure & beta=2.5 & sigma=2 & n=200 & 0.00 \\ 
  79 & MME & Measure & beta=2.5 & sigma=2 & n=200 & 0.00 \\ 
  80 & MME.b & Measure & beta=2.5 & sigma=2 & n=200 & 0.00 \\ 
  81 & PWM & Measure & beta=2.5 & sigma=2 & n=200 & 0.00 \\ 
  82 & MLE & Measure & beta=3 & sigma=2 & n=200 & 0.00 \\ 
  83 & MLE.b & Measure & beta=3 & sigma=2 & n=200 & 0.00 \\ 
  84 & LME & Measure & beta=3 & sigma=2 & n=200 & 0.00 \\ 
  85 & MDE.Phi.chisq & Measure & beta=3 & sigma=2 & n=200 & 0.01 \\ 
  86 & MDE.Phi.tv & Measure & beta=3 & sigma=2 & n=200 & 0.01 \\ 
  87 & MDE.Phi.kl & Measure & beta=3 & sigma=2 & n=200 & 0.00 \\ 
  88 & MME & Measure & beta=3 & sigma=2 & n=200 & 0.00 \\ 
  89 & MME.b & Measure & beta=3 & sigma=2 & n=200 & 0.00 \\ 
  90 & PWM & Measure & beta=3 & sigma=2 & n=200 & 0.00 \\ 
  91 & MLE & Measure & beta=4 & sigma=2 & n=200 & 0.00 \\ 
  92 & MLE.b & Measure & beta=4 & sigma=2 & n=200 & 0.00 \\ 
  93 & LME & Measure & beta=4 & sigma=2 & n=200 & 0.00 \\ 
  94 & MDE.Phi.chisq & Measure & beta=4 & sigma=2 & n=200 & 0.01 \\ 
  95 & MDE.Phi.tv & Measure & beta=4 & sigma=2 & n=200 & 0.01 \\ 
  96 & MDE.Phi.kl & Measure & beta=4 & sigma=2 & n=200 & 0.00 \\ 
  97 & MME & Measure & beta=4 & sigma=2 & n=200 & 0.00 \\ 
  98 & MME.b & Measure & beta=4 & sigma=2 & n=200 & 0.00 \\ 
  99 & PWM & Measure & beta=4 & sigma=2 & n=200 & 0.00 \\ 
  100 & MLE & Measure & beta=5 & sigma=2 & n=200 & 0.00 \\ 
  101 & MLE.b & Measure & beta=5 & sigma=2 & n=200 & 0.00 \\ 
  102 & LME & Measure & beta=5 & sigma=2 & n=200 & 0.00 \\ 
  103 & MDE.Phi.chisq & Measure & beta=5 & sigma=2 & n=200 & 0.01 \\ 
  104 & MDE.Phi.tv & Measure & beta=5 & sigma=2 & n=200 & 0.01 \\ 
  105 & MDE.Phi.kl & Measure & beta=5 & sigma=2 & n=200 & 0.00 \\ 
  106 & MME & Measure & beta=5 & sigma=2 & n=200 & 0.00 \\ 
  107 & MME.b & Measure & beta=5 & sigma=2 & n=200 & 2.02 \\ 
  108 & PWM & Measure & beta=5 & sigma=2 & n=200 & 0.00 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220208/Output.bias.LaTeX.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Wed Feb 09 03:15:34 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=2 & n=100 & 0.17 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=2 & n=100 & -0.02 \\ 
  3 & LME & beta & beta=1.5 & sigma=2 & n=100 & 0.33 \\ 
  4 & MDE.Phi.chisq & beta & beta=1.5 & sigma=2 & n=100 & -1.27 \\ 
  5 & MDE.Phi.tv & beta & beta=1.5 & sigma=2 & n=100 & -0.24 \\ 
  6 & MDE.Phi.kl & beta & beta=1.5 & sigma=2 & n=100 & 0.17 \\ 
  7 & MME & beta & beta=1.5 & sigma=2 & n=100 & 1.29 \\ 
  8 & MME.b & beta & beta=1.5 & sigma=2 & n=100 & 4.81 \\ 
  9 & PWM & beta & beta=1.5 & sigma=2 & n=100 & 0.33 \\ 
  10 & MLE & sigma & beta=1.5 & sigma=2 & n=100 & 0.36 \\ 
  11 & MLE.b & sigma & beta=1.5 & sigma=2 & n=100 & -0.05 \\ 
  12 & LME & sigma & beta=1.5 & sigma=2 & n=100 & 0.65 \\ 
  13 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=2 & n=100 & 1.29 \\ 
  14 & MDE.Phi.tv & sigma & beta=1.5 & sigma=2 & n=100 & 1.64 \\ 
  15 & MDE.Phi.kl & sigma & beta=1.5 & sigma=2 & n=100 & 0.36 \\ 
  16 & MME & sigma & beta=1.5 & sigma=2 & n=100 & 4.30 \\ 
  17 & MME.b & sigma & beta=1.5 & sigma=2 & n=100 & 11.67 \\ 
  18 & PWM & sigma & beta=1.5 & sigma=2 & n=100 & 0.65 \\ 
  19 & MLE & beta & beta=2 & sigma=2 & n=100 & 1.09 \\ 
  20 & MLE.b & beta & beta=2 & sigma=2 & n=100 & 0.74 \\ 
  21 & LME & beta & beta=2 & sigma=2 & n=100 & 0.45 \\ 
  22 & MDE.Phi.chisq & beta & beta=2 & sigma=2 & n=100 & 0.10 \\ 
  23 & MDE.Phi.tv & beta & beta=2 & sigma=2 & n=100 & 0.69 \\ 
  24 & MDE.Phi.kl & beta & beta=2 & sigma=2 & n=100 & 0.46 \\ 
  25 & MME & beta & beta=2 & sigma=2 & n=100 & 1.68 \\ 
  26 & MME.b & beta & beta=2 & sigma=2 & n=100 & 7.48 \\ 
  27 & PWM & beta & beta=2 & sigma=2 & n=100 & 0.45 \\ 
  28 & MLE & sigma & beta=2 & sigma=2 & n=100 & 1.37 \\ 
  29 & MLE.b & sigma & beta=2 & sigma=2 & n=100 & 0.86 \\ 
  30 & LME & sigma & beta=2 & sigma=2 & n=100 & 0.60 \\ 
  31 & MDE.Phi.chisq & sigma & beta=2 & sigma=2 & n=100 & 2.19 \\ 
  32 & MDE.Phi.tv & sigma & beta=2 & sigma=2 & n=100 & 3.22 \\ 
  33 & MDE.Phi.kl & sigma & beta=2 & sigma=2 & n=100 & 0.65 \\ 
  34 & MME & sigma & beta=2 & sigma=2 & n=100 & 2.87 \\ 
  35 & MME.b & sigma & beta=2 & sigma=2 & n=100 & 11.17 \\ 
  36 & PWM & sigma & beta=2 & sigma=2 & n=100 & 0.60 \\ 
  37 & MLE & beta & beta=2.5 & sigma=2 & n=100 & 2.22 \\ 
  38 & MLE.b & beta & beta=2.5 & sigma=2 & n=100 & 1.76 \\ 
  39 & LME & beta & beta=2.5 & sigma=2 & n=100 & 0.70 \\ 
  40 & MDE.Phi.chisq & beta & beta=2.5 & sigma=2 & n=100 & 1.61 \\ 
  41 & MDE.Phi.tv & beta & beta=2.5 & sigma=2 & n=100 & 2.43 \\ 
  42 & MDE.Phi.kl & beta & beta=2.5 & sigma=2 & n=100 & 0.94 \\ 
  43 & MME & beta & beta=2.5 & sigma=2 & n=100 & 2.32 \\ 
  44 & MME.b & beta & beta=2.5 & sigma=2 & n=100 & 5.49 \\ 
  45 & PWM & beta & beta=2.5 & sigma=2 & n=100 & 0.70 \\ 
  46 & MLE & sigma & beta=2.5 & sigma=2 & n=100 & 2.39 \\ 
  47 & MLE.b & sigma & beta=2.5 & sigma=2 & n=100 & 1.90 \\ 
  48 & LME & sigma & beta=2.5 & sigma=2 & n=100 & 0.72 \\ 
  49 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=2 & n=100 & 4.14 \\ 
  50 & MDE.Phi.tv & sigma & beta=2.5 & sigma=2 & n=100 & 5.19 \\ 
  51 & MDE.Phi.kl & sigma & beta=2.5 & sigma=2 & n=100 & 1.01 \\ 
  52 & MME & sigma & beta=2.5 & sigma=2 & n=100 & 2.71 \\ 
  53 & MME.b & sigma & beta=2.5 & sigma=2 & n=100 & 6.04 \\ 
  54 & PWM & sigma & beta=2.5 & sigma=2 & n=100 & 0.72 \\ 
  55 & MLE & beta & beta=3 & sigma=2 & n=100 & 9.47 \\ 
  56 & MLE.b & beta & beta=3 & sigma=2 & n=100 & 8.98 \\ 
  57 & LME & beta & beta=3 & sigma=2 & n=100 & 1.02 \\ 
  58 & MDE.Phi.chisq & beta & beta=3 & sigma=2 & n=100 & 3.82 \\ 
  59 & MDE.Phi.tv & beta & beta=3 & sigma=2 & n=100 & 5.23 \\ 
  60 & MDE.Phi.kl & beta & beta=3 & sigma=2 & n=100 & 1.86 \\ 
  61 & MME & beta & beta=3 & sigma=2 & n=100 & 14.49 \\ 
  62 & MME.b & beta & beta=3 & sigma=2 & n=100 & 46.99 \\ 
  63 & PWM & beta & beta=3 & sigma=2 & n=100 & 1.02 \\ 
  64 & MLE & sigma & beta=3 & sigma=2 & n=100 & 8.23 \\ 
  65 & MLE.b & sigma & beta=3 & sigma=2 & n=100 & 7.80 \\ 
  66 & LME & sigma & beta=3 & sigma=2 & n=100 & 0.85 \\ 
  67 & MDE.Phi.chisq & sigma & beta=3 & sigma=2 & n=100 & 6.25 \\ 
  68 & MDE.Phi.tv & sigma & beta=3 & sigma=2 & n=100 & 7.70 \\ 
  69 & MDE.Phi.kl & sigma & beta=3 & sigma=2 & n=100 & 1.60 \\ 
  70 & MME & sigma & beta=3 & sigma=2 & n=100 & 11.48 \\ 
  71 & MME.b & sigma & beta=3 & sigma=2 & n=100 & 37.14 \\ 
  72 & PWM & sigma & beta=3 & sigma=2 & n=100 & 0.85 \\ 
  73 & MLE & beta & beta=4 & sigma=2 & n=100 & 14.28 \\ 
  74 & MLE.b & beta & beta=4 & sigma=2 & n=100 & 13.83 \\ 
  75 & LME & beta & beta=4 & sigma=2 & n=100 & 1.76 \\ 
  76 & MDE.Phi.chisq & beta & beta=4 & sigma=2 & n=100 & 9.77 \\ 
  77 & MDE.Phi.tv & beta & beta=4 & sigma=2 & n=100 & 11.95 \\ 
  78 & MDE.Phi.kl & beta & beta=4 & sigma=2 & n=100 & 3.42 \\ 
  79 & MME & beta & beta=4 & sigma=2 & n=100 & 7.36 \\ 
  80 & MME.b & beta & beta=4 & sigma=2 & n=100 & 36.91 \\ 
  81 & PWM & beta & beta=4 & sigma=2 & n=100 & 1.76 \\ 
  82 & MLE & sigma & beta=4 & sigma=2 & n=100 & 8.69 \\ 
  83 & MLE.b & sigma & beta=4 & sigma=2 & n=100 & 8.42 \\ 
  84 & LME & sigma & beta=4 & sigma=2 & n=100 & 1.07 \\ 
  85 & MDE.Phi.chisq & sigma & beta=4 & sigma=2 & n=100 & 9.83 \\ 
  86 & MDE.Phi.tv & sigma & beta=4 & sigma=2 & n=100 & 11.26 \\ 
  87 & MDE.Phi.kl & sigma & beta=4 & sigma=2 & n=100 & 2.12 \\ 
  88 & MME & sigma & beta=4 & sigma=2 & n=100 & 4.67 \\ 
  89 & MME.b & sigma & beta=4 & sigma=2 & n=100 & 24.87 \\ 
  90 & PWM & sigma & beta=4 & sigma=2 & n=100 & 1.07 \\ 
  91 & MLE & beta & beta=5 & sigma=2 & n=100 & 24.63 \\ 
  92 & MLE.b & beta & beta=5 & sigma=2 & n=100 & 24.26 \\ 
  93 & LME & beta & beta=5 & sigma=2 & n=100 & 2.36 \\ 
  94 & MDE.Phi.chisq & beta & beta=5 & sigma=2 & n=100 & 15.09 \\ 
  95 & MDE.Phi.tv & beta & beta=5 & sigma=2 & n=100 & 17.24 \\ 
  96 & MDE.Phi.kl & beta & beta=5 & sigma=2 & n=100 & 5.06 \\ 
  97 & MME & beta & beta=5 & sigma=2 & n=100 & 11.73 \\ 
  98 & MME.b & beta & beta=5 & sigma=2 & n=100 & 42.16 \\ 
  99 & PWM & beta & beta=5 & sigma=2 & n=100 & 2.36 \\ 
  100 & MLE & sigma & beta=5 & sigma=2 & n=100 & 11.66 \\ 
  101 & MLE.b & sigma & beta=5 & sigma=2 & n=100 & 11.49 \\ 
  102 & LME & sigma & beta=5 & sigma=2 & n=100 & 1.10 \\ 
  103 & MDE.Phi.chisq & sigma & beta=5 & sigma=2 & n=100 & 11.18 \\ 
  104 & MDE.Phi.tv & sigma & beta=5 & sigma=2 & n=100 & 12.16 \\ 
  105 & MDE.Phi.kl & sigma & beta=5 & sigma=2 & n=100 & 2.38 \\ 
  106 & MME & sigma & beta=5 & sigma=2 & n=100 & 5.50 \\ 
  107 & MME.b & sigma & beta=5 & sigma=2 & n=100 & 19.93 \\ 
  108 & PWM & sigma & beta=5 & sigma=2 & n=100 & 1.10 \\ 
  109 & MLE & beta & beta=1.5 & sigma=2 & n=200 & 0.08 \\ 
  110 & MLE.b & beta & beta=1.5 & sigma=2 & n=200 & -0.00 \\ 
  111 & LME & beta & beta=1.5 & sigma=2 & n=200 & 0.21 \\ 
  112 & MDE.Phi.chisq & beta & beta=1.5 & sigma=2 & n=200 & -0.85 \\ 
  113 & MDE.Phi.tv & beta & beta=1.5 & sigma=2 & n=200 & -0.50 \\ 
  114 & MDE.Phi.kl & beta & beta=1.5 & sigma=2 & n=200 & 0.08 \\ 
  115 & MME & beta & beta=1.5 & sigma=2 & n=200 & 1.00 \\ 
  116 & MME.b & beta & beta=1.5 & sigma=2 & n=200 & 0.80 \\ 
  117 & PWM & beta & beta=1.5 & sigma=2 & n=200 & 0.21 \\ 
  118 & MLE & sigma & beta=1.5 & sigma=2 & n=200 & 0.16 \\ 
  119 & MLE.b & sigma & beta=1.5 & sigma=2 & n=200 & -0.01 \\ 
  120 & LME & sigma & beta=1.5 & sigma=2 & n=200 & 0.40 \\ 
  121 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=2 & n=200 & 0.32 \\ 
  122 & MDE.Phi.tv & sigma & beta=1.5 & sigma=2 & n=200 & 0.51 \\ 
  123 & MDE.Phi.kl & sigma & beta=1.5 & sigma=2 & n=200 & 0.16 \\ 
  124 & MME & sigma & beta=1.5 & sigma=2 & n=200 & 3.57 \\ 
  125 & MME.b & sigma & beta=1.5 & sigma=2 & n=200 & 3.02 \\ 
  126 & PWM & sigma & beta=1.5 & sigma=2 & n=200 & 0.40 \\ 
  127 & MLE & beta & beta=2 & sigma=2 & n=200 & 0.14 \\ 
  128 & MLE.b & beta & beta=2 & sigma=2 & n=200 & -0.03 \\ 
  129 & LME & beta & beta=2 & sigma=2 & n=200 & 0.22 \\ 
  130 & MDE.Phi.chisq & beta & beta=2 & sigma=2 & n=200 & -0.65 \\ 
  131 & MDE.Phi.tv & beta & beta=2 & sigma=2 & n=200 & -0.44 \\ 
  132 & MDE.Phi.kl & beta & beta=2 & sigma=2 & n=200 & 0.14 \\ 
  133 & MME & beta & beta=2 & sigma=2 & n=200 & 0.97 \\ 
  134 & MME.b & beta & beta=2 & sigma=2 & n=200 & 0.69 \\ 
  135 & PWM & beta & beta=2 & sigma=2 & n=200 & 0.22 \\ 
  136 & MLE & sigma & beta=2 & sigma=2 & n=200 & 0.19 \\ 
  137 & MLE.b & sigma & beta=2 & sigma=2 & n=200 & -0.05 \\ 
  138 & LME & sigma & beta=2 & sigma=2 & n=200 & 0.28 \\ 
  139 & MDE.Phi.chisq & sigma & beta=2 & sigma=2 & n=200 & 0.34 \\ 
  140 & MDE.Phi.tv & sigma & beta=2 & sigma=2 & n=200 & 0.56 \\ 
  141 & MDE.Phi.kl & sigma & beta=2 & sigma=2 & n=200 & 0.19 \\ 
  142 & MME & sigma & beta=2 & sigma=2 & n=200 & 1.78 \\ 
  143 & MME.b & sigma & beta=2 & sigma=2 & n=200 & 1.29 \\ 
  144 & PWM & sigma & beta=2 & sigma=2 & n=200 & 0.28 \\ 
  145 & MLE & beta & beta=2.5 & sigma=2 & n=200 & 0.25 \\ 
  146 & MLE.b & beta & beta=2.5 & sigma=2 & n=200 & -0.05 \\ 
  147 & LME & beta & beta=2.5 & sigma=2 & n=200 & 0.28 \\ 
  148 & MDE.Phi.chisq & beta & beta=2.5 & sigma=2 & n=200 & -0.45 \\ 
  149 & MDE.Phi.tv & beta & beta=2.5 & sigma=2 & n=200 & -0.22 \\ 
  150 & MDE.Phi.kl & beta & beta=2.5 & sigma=2 & n=200 & 0.25 \\ 
  151 & MME & beta & beta=2.5 & sigma=2 & n=200 & 1.06 \\ 
  152 & MME.b & beta & beta=2.5 & sigma=2 & n=200 & 0.84 \\ 
  153 & PWM & beta & beta=2.5 & sigma=2 & n=200 & 0.28 \\ 
  154 & MLE & sigma & beta=2.5 & sigma=2 & n=200 & 0.27 \\ 
  155 & MLE.b & sigma & beta=2.5 & sigma=2 & n=200 & -0.06 \\ 
  156 & LME & sigma & beta=2.5 & sigma=2 & n=200 & 0.29 \\ 
  157 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=2 & n=200 & 0.70 \\ 
  158 & MDE.Phi.tv & sigma & beta=2.5 & sigma=2 & n=200 & 0.81 \\ 
  159 & MDE.Phi.kl & sigma & beta=2.5 & sigma=2 & n=200 & 0.27 \\ 
  160 & MME & sigma & beta=2.5 & sigma=2 & n=200 & 1.31 \\ 
  161 & MME.b & sigma & beta=2.5 & sigma=2 & n=200 & 1.01 \\ 
  162 & PWM & sigma & beta=2.5 & sigma=2 & n=200 & 0.29 \\ 
  163 & MLE & beta & beta=3 & sigma=2 & n=200 & 0.55 \\ 
  164 & MLE.b & beta & beta=3 & sigma=2 & n=200 & 0.09 \\ 
  165 & LME & beta & beta=3 & sigma=2 & n=200 & 0.45 \\ 
  166 & MDE.Phi.chisq & beta & beta=3 & sigma=2 & n=200 & 0.31 \\ 
  167 & MDE.Phi.tv & beta & beta=3 & sigma=2 & n=200 & 0.21 \\ 
  168 & MDE.Phi.kl & beta & beta=3 & sigma=2 & n=200 & 0.49 \\ 
  169 & MME & beta & beta=3 & sigma=2 & n=200 & 1.40 \\ 
  170 & MME.b & beta & beta=3 & sigma=2 & n=200 & 2.69 \\ 
  171 & PWM & beta & beta=3 & sigma=2 & n=200 & 0.45 \\ 
  172 & MLE & sigma & beta=3 & sigma=2 & n=200 & 0.48 \\ 
  173 & MLE.b & sigma & beta=3 & sigma=2 & n=200 & 0.07 \\ 
  174 & LME & sigma & beta=3 & sigma=2 & n=200 & 0.38 \\ 
  175 & MDE.Phi.chisq & sigma & beta=3 & sigma=2 & n=200 & 1.54 \\ 
  176 & MDE.Phi.tv & sigma & beta=3 & sigma=2 & n=200 & 1.19 \\ 
  177 & MDE.Phi.kl & sigma & beta=3 & sigma=2 & n=200 & 0.43 \\ 
  178 & MME & sigma & beta=3 & sigma=2 & n=200 & 1.29 \\ 
  179 & MME.b & sigma & beta=3 & sigma=2 & n=200 & 2.46 \\ 
  180 & PWM & sigma & beta=3 & sigma=2 & n=200 & 0.38 \\ 
  181 & MLE & beta & beta=4 & sigma=2 & n=200 & 1.54 \\ 
  182 & MLE.b & beta & beta=4 & sigma=2 & n=200 & 0.87 \\ 
  183 & LME & beta & beta=4 & sigma=2 & n=200 & 0.91 \\ 
  184 & MDE.Phi.chisq & beta & beta=4 & sigma=2 & n=200 & 3.71 \\ 
  185 & MDE.Phi.tv & beta & beta=4 & sigma=2 & n=200 & 2.95 \\ 
  186 & MDE.Phi.kl & beta & beta=4 & sigma=2 & n=200 & 1.26 \\ 
  187 & MME & beta & beta=4 & sigma=2 & n=200 & 2.64 \\ 
  188 & MME.b & beta & beta=4 & sigma=2 & n=200 & 9.69 \\ 
  189 & PWM & beta & beta=4 & sigma=2 & n=200 & 0.91 \\ 
  190 & MLE & sigma & beta=4 & sigma=2 & n=200 & 0.95 \\ 
  191 & MLE.b & sigma & beta=4 & sigma=2 & n=200 & 0.54 \\ 
  192 & LME & sigma & beta=4 & sigma=2 & n=200 & 0.55 \\ 
  193 & MDE.Phi.chisq & sigma & beta=4 & sigma=2 & n=200 & 4.00 \\ 
  194 & MDE.Phi.tv & sigma & beta=4 & sigma=2 & n=200 & 3.13 \\ 
  195 & MDE.Phi.kl & sigma & beta=4 & sigma=2 & n=200 & 0.77 \\ 
  196 & MME & sigma & beta=4 & sigma=2 & n=200 & 1.66 \\ 
  197 & MME.b & sigma & beta=4 & sigma=2 & n=200 & 6.25 \\ 
  198 & PWM & sigma & beta=4 & sigma=2 & n=200 & 0.55 \\ 
  199 & MLE & beta & beta=5 & sigma=2 & n=200 & 8.72 \\ 
  200 & MLE.b & beta & beta=5 & sigma=2 & n=200 & 8.01 \\ 
  201 & LME & beta & beta=5 & sigma=2 & n=200 & 1.78 \\ 
  202 & MDE.Phi.chisq & beta & beta=5 & sigma=2 & n=200 & 9.13 \\ 
  203 & MDE.Phi.tv & beta & beta=5 & sigma=2 & n=200 & 6.36 \\ 
  204 & MDE.Phi.kl & beta & beta=5 & sigma=2 & n=200 & 2.60 \\ 
  205 & MME & beta & beta=5 & sigma=2 & n=200 & 4.76 \\ 
  206 & MME.b & beta & beta=5 & sigma=2 & n=200 & 16.59 \\ 
  207 & PWM & beta & beta=5 & sigma=2 & n=200 & 1.78 \\ 
  208 & MLE & sigma & beta=5 & sigma=2 & n=200 & 4.03 \\ 
  209 & MLE.b & sigma & beta=5 & sigma=2 & n=200 & 3.69 \\ 
  210 & LME & sigma & beta=5 & sigma=2 & n=200 & 0.83 \\ 
  211 & MDE.Phi.chisq & sigma & beta=5 & sigma=2 & n=200 & 6.54 \\ 
  212 & MDE.Phi.tv & sigma & beta=5 & sigma=2 & n=200 & 4.51 \\ 
  213 & MDE.Phi.kl & sigma & beta=5 & sigma=2 & n=200 & 1.23 \\ 
  214 & MME & sigma & beta=5 & sigma=2 & n=200 & 2.27 \\ 
  215 & MME.b & sigma & beta=5 & sigma=2 & n=200 & 7.87 \\ 
  216 & PWM & sigma & beta=5 & sigma=2 & n=200 & 0.83 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220208/Output.mean.LaTeX.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Wed Feb 09 03:15:34 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=2 & n=100 & 1.67 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=2 & n=100 & 1.48 \\ 
  3 & LME & beta & beta=1.5 & sigma=2 & n=100 & 1.83 \\ 
  4 & MDE.Phi.chisq & beta & beta=1.5 & sigma=2 & n=100 & 0.23 \\ 
  5 & MDE.Phi.tv & beta & beta=1.5 & sigma=2 & n=100 & 1.26 \\ 
  6 & MDE.Phi.kl & beta & beta=1.5 & sigma=2 & n=100 & 1.67 \\ 
  7 & MME & beta & beta=1.5 & sigma=2 & n=100 & 2.79 \\ 
  8 & MME.b & beta & beta=1.5 & sigma=2 & n=100 & 6.31 \\ 
  9 & PWM & beta & beta=1.5 & sigma=2 & n=100 & 1.83 \\ 
  10 & MLE & sigma & beta=1.5 & sigma=2 & n=100 & 2.36 \\ 
  11 & MLE.b & sigma & beta=1.5 & sigma=2 & n=100 & 1.95 \\ 
  12 & LME & sigma & beta=1.5 & sigma=2 & n=100 & 2.65 \\ 
  13 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=2 & n=100 & 3.29 \\ 
  14 & MDE.Phi.tv & sigma & beta=1.5 & sigma=2 & n=100 & 3.64 \\ 
  15 & MDE.Phi.kl & sigma & beta=1.5 & sigma=2 & n=100 & 2.36 \\ 
  16 & MME & sigma & beta=1.5 & sigma=2 & n=100 & 6.30 \\ 
  17 & MME.b & sigma & beta=1.5 & sigma=2 & n=100 & 13.67 \\ 
  18 & PWM & sigma & beta=1.5 & sigma=2 & n=100 & 2.65 \\ 
  19 & MLE & beta & beta=2 & sigma=2 & n=100 & 3.09 \\ 
  20 & MLE.b & beta & beta=2 & sigma=2 & n=100 & 2.74 \\ 
  21 & LME & beta & beta=2 & sigma=2 & n=100 & 2.45 \\ 
  22 & MDE.Phi.chisq & beta & beta=2 & sigma=2 & n=100 & 2.10 \\ 
  23 & MDE.Phi.tv & beta & beta=2 & sigma=2 & n=100 & 2.69 \\ 
  24 & MDE.Phi.kl & beta & beta=2 & sigma=2 & n=100 & 2.46 \\ 
  25 & MME & beta & beta=2 & sigma=2 & n=100 & 3.68 \\ 
  26 & MME.b & beta & beta=2 & sigma=2 & n=100 & 9.48 \\ 
  27 & PWM & beta & beta=2 & sigma=2 & n=100 & 2.45 \\ 
  28 & MLE & sigma & beta=2 & sigma=2 & n=100 & 3.37 \\ 
  29 & MLE.b & sigma & beta=2 & sigma=2 & n=100 & 2.86 \\ 
  30 & LME & sigma & beta=2 & sigma=2 & n=100 & 2.60 \\ 
  31 & MDE.Phi.chisq & sigma & beta=2 & sigma=2 & n=100 & 4.19 \\ 
  32 & MDE.Phi.tv & sigma & beta=2 & sigma=2 & n=100 & 5.22 \\ 
  33 & MDE.Phi.kl & sigma & beta=2 & sigma=2 & n=100 & 2.65 \\ 
  34 & MME & sigma & beta=2 & sigma=2 & n=100 & 4.87 \\ 
  35 & MME.b & sigma & beta=2 & sigma=2 & n=100 & 13.17 \\ 
  36 & PWM & sigma & beta=2 & sigma=2 & n=100 & 2.60 \\ 
  37 & MLE & beta & beta=2.5 & sigma=2 & n=100 & 4.72 \\ 
  38 & MLE.b & beta & beta=2.5 & sigma=2 & n=100 & 4.26 \\ 
  39 & LME & beta & beta=2.5 & sigma=2 & n=100 & 3.20 \\ 
  40 & MDE.Phi.chisq & beta & beta=2.5 & sigma=2 & n=100 & 4.11 \\ 
  41 & MDE.Phi.tv & beta & beta=2.5 & sigma=2 & n=100 & 4.93 \\ 
  42 & MDE.Phi.kl & beta & beta=2.5 & sigma=2 & n=100 & 3.44 \\ 
  43 & MME & beta & beta=2.5 & sigma=2 & n=100 & 4.82 \\ 
  44 & MME.b & beta & beta=2.5 & sigma=2 & n=100 & 7.99 \\ 
  45 & PWM & beta & beta=2.5 & sigma=2 & n=100 & 3.20 \\ 
  46 & MLE & sigma & beta=2.5 & sigma=2 & n=100 & 4.39 \\ 
  47 & MLE.b & sigma & beta=2.5 & sigma=2 & n=100 & 3.90 \\ 
  48 & LME & sigma & beta=2.5 & sigma=2 & n=100 & 2.72 \\ 
  49 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=2 & n=100 & 6.14 \\ 
  50 & MDE.Phi.tv & sigma & beta=2.5 & sigma=2 & n=100 & 7.19 \\ 
  51 & MDE.Phi.kl & sigma & beta=2.5 & sigma=2 & n=100 & 3.01 \\ 
  52 & MME & sigma & beta=2.5 & sigma=2 & n=100 & 4.71 \\ 
  53 & MME.b & sigma & beta=2.5 & sigma=2 & n=100 & 8.04 \\ 
  54 & PWM & sigma & beta=2.5 & sigma=2 & n=100 & 2.72 \\ 
  55 & MLE & beta & beta=3 & sigma=2 & n=100 & 12.47 \\ 
  56 & MLE.b & beta & beta=3 & sigma=2 & n=100 & 11.98 \\ 
  57 & LME & beta & beta=3 & sigma=2 & n=100 & 4.02 \\ 
  58 & MDE.Phi.chisq & beta & beta=3 & sigma=2 & n=100 & 6.82 \\ 
  59 & MDE.Phi.tv & beta & beta=3 & sigma=2 & n=100 & 8.23 \\ 
  60 & MDE.Phi.kl & beta & beta=3 & sigma=2 & n=100 & 4.86 \\ 
  61 & MME & beta & beta=3 & sigma=2 & n=100 & 17.49 \\ 
  62 & MME.b & beta & beta=3 & sigma=2 & n=100 & 49.99 \\ 
  63 & PWM & beta & beta=3 & sigma=2 & n=100 & 4.02 \\ 
  64 & MLE & sigma & beta=3 & sigma=2 & n=100 & 10.23 \\ 
  65 & MLE.b & sigma & beta=3 & sigma=2 & n=100 & 9.80 \\ 
  66 & LME & sigma & beta=3 & sigma=2 & n=100 & 2.85 \\ 
  67 & MDE.Phi.chisq & sigma & beta=3 & sigma=2 & n=100 & 8.25 \\ 
  68 & MDE.Phi.tv & sigma & beta=3 & sigma=2 & n=100 & 9.70 \\ 
  69 & MDE.Phi.kl & sigma & beta=3 & sigma=2 & n=100 & 3.60 \\ 
  70 & MME & sigma & beta=3 & sigma=2 & n=100 & 13.48 \\ 
  71 & MME.b & sigma & beta=3 & sigma=2 & n=100 & 39.14 \\ 
  72 & PWM & sigma & beta=3 & sigma=2 & n=100 & 2.85 \\ 
  73 & MLE & beta & beta=4 & sigma=2 & n=100 & 18.28 \\ 
  74 & MLE.b & beta & beta=4 & sigma=2 & n=100 & 17.83 \\ 
  75 & LME & beta & beta=4 & sigma=2 & n=100 & 5.76 \\ 
  76 & MDE.Phi.chisq & beta & beta=4 & sigma=2 & n=100 & 13.77 \\ 
  77 & MDE.Phi.tv & beta & beta=4 & sigma=2 & n=100 & 15.95 \\ 
  78 & MDE.Phi.kl & beta & beta=4 & sigma=2 & n=100 & 7.42 \\ 
  79 & MME & beta & beta=4 & sigma=2 & n=100 & 11.36 \\ 
  80 & MME.b & beta & beta=4 & sigma=2 & n=100 & 40.91 \\ 
  81 & PWM & beta & beta=4 & sigma=2 & n=100 & 5.76 \\ 
  82 & MLE & sigma & beta=4 & sigma=2 & n=100 & 10.69 \\ 
  83 & MLE.b & sigma & beta=4 & sigma=2 & n=100 & 10.42 \\ 
  84 & LME & sigma & beta=4 & sigma=2 & n=100 & 3.07 \\ 
  85 & MDE.Phi.chisq & sigma & beta=4 & sigma=2 & n=100 & 11.83 \\ 
  86 & MDE.Phi.tv & sigma & beta=4 & sigma=2 & n=100 & 13.26 \\ 
  87 & MDE.Phi.kl & sigma & beta=4 & sigma=2 & n=100 & 4.12 \\ 
  88 & MME & sigma & beta=4 & sigma=2 & n=100 & 6.67 \\ 
  89 & MME.b & sigma & beta=4 & sigma=2 & n=100 & 26.87 \\ 
  90 & PWM & sigma & beta=4 & sigma=2 & n=100 & 3.07 \\ 
  91 & MLE & beta & beta=5 & sigma=2 & n=100 & 29.63 \\ 
  92 & MLE.b & beta & beta=5 & sigma=2 & n=100 & 29.26 \\ 
  93 & LME & beta & beta=5 & sigma=2 & n=100 & 7.36 \\ 
  94 & MDE.Phi.chisq & beta & beta=5 & sigma=2 & n=100 & 20.09 \\ 
  95 & MDE.Phi.tv & beta & beta=5 & sigma=2 & n=100 & 22.24 \\ 
  96 & MDE.Phi.kl & beta & beta=5 & sigma=2 & n=100 & 10.06 \\ 
  97 & MME & beta & beta=5 & sigma=2 & n=100 & 16.73 \\ 
  98 & MME.b & beta & beta=5 & sigma=2 & n=100 & 47.16 \\ 
  99 & PWM & beta & beta=5 & sigma=2 & n=100 & 7.36 \\ 
  100 & MLE & sigma & beta=5 & sigma=2 & n=100 & 13.66 \\ 
  101 & MLE.b & sigma & beta=5 & sigma=2 & n=100 & 13.49 \\ 
  102 & LME & sigma & beta=5 & sigma=2 & n=100 & 3.10 \\ 
  103 & MDE.Phi.chisq & sigma & beta=5 & sigma=2 & n=100 & 13.18 \\ 
  104 & MDE.Phi.tv & sigma & beta=5 & sigma=2 & n=100 & 14.16 \\ 
  105 & MDE.Phi.kl & sigma & beta=5 & sigma=2 & n=100 & 4.38 \\ 
  106 & MME & sigma & beta=5 & sigma=2 & n=100 & 7.50 \\ 
  107 & MME.b & sigma & beta=5 & sigma=2 & n=100 & 21.93 \\ 
  108 & PWM & sigma & beta=5 & sigma=2 & n=100 & 3.10 \\ 
  109 & MLE & beta & beta=1.5 & sigma=2 & n=200 & 1.58 \\ 
  110 & MLE.b & beta & beta=1.5 & sigma=2 & n=200 & 1.50 \\ 
  111 & LME & beta & beta=1.5 & sigma=2 & n=200 & 1.71 \\ 
  112 & MDE.Phi.chisq & beta & beta=1.5 & sigma=2 & n=200 & 0.65 \\ 
  113 & MDE.Phi.tv & beta & beta=1.5 & sigma=2 & n=200 & 1.00 \\ 
  114 & MDE.Phi.kl & beta & beta=1.5 & sigma=2 & n=200 & 1.58 \\ 
  115 & MME & beta & beta=1.5 & sigma=2 & n=200 & 2.50 \\ 
  116 & MME.b & beta & beta=1.5 & sigma=2 & n=200 & 2.30 \\ 
  117 & PWM & beta & beta=1.5 & sigma=2 & n=200 & 1.71 \\ 
  118 & MLE & sigma & beta=1.5 & sigma=2 & n=200 & 2.16 \\ 
  119 & MLE.b & sigma & beta=1.5 & sigma=2 & n=200 & 1.99 \\ 
  120 & LME & sigma & beta=1.5 & sigma=2 & n=200 & 2.40 \\ 
  121 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=2 & n=200 & 2.32 \\ 
  122 & MDE.Phi.tv & sigma & beta=1.5 & sigma=2 & n=200 & 2.51 \\ 
  123 & MDE.Phi.kl & sigma & beta=1.5 & sigma=2 & n=200 & 2.16 \\ 
  124 & MME & sigma & beta=1.5 & sigma=2 & n=200 & 5.57 \\ 
  125 & MME.b & sigma & beta=1.5 & sigma=2 & n=200 & 5.02 \\ 
  126 & PWM & sigma & beta=1.5 & sigma=2 & n=200 & 2.40 \\ 
  127 & MLE & beta & beta=2 & sigma=2 & n=200 & 2.14 \\ 
  128 & MLE.b & beta & beta=2 & sigma=2 & n=200 & 1.97 \\ 
  129 & LME & beta & beta=2 & sigma=2 & n=200 & 2.22 \\ 
  130 & MDE.Phi.chisq & beta & beta=2 & sigma=2 & n=200 & 1.35 \\ 
  131 & MDE.Phi.tv & beta & beta=2 & sigma=2 & n=200 & 1.56 \\ 
  132 & MDE.Phi.kl & beta & beta=2 & sigma=2 & n=200 & 2.14 \\ 
  133 & MME & beta & beta=2 & sigma=2 & n=200 & 2.97 \\ 
  134 & MME.b & beta & beta=2 & sigma=2 & n=200 & 2.69 \\ 
  135 & PWM & beta & beta=2 & sigma=2 & n=200 & 2.22 \\ 
  136 & MLE & sigma & beta=2 & sigma=2 & n=200 & 2.19 \\ 
  137 & MLE.b & sigma & beta=2 & sigma=2 & n=200 & 1.95 \\ 
  138 & LME & sigma & beta=2 & sigma=2 & n=200 & 2.28 \\ 
  139 & MDE.Phi.chisq & sigma & beta=2 & sigma=2 & n=200 & 2.34 \\ 
  140 & MDE.Phi.tv & sigma & beta=2 & sigma=2 & n=200 & 2.56 \\ 
  141 & MDE.Phi.kl & sigma & beta=2 & sigma=2 & n=200 & 2.19 \\ 
  142 & MME & sigma & beta=2 & sigma=2 & n=200 & 3.78 \\ 
  143 & MME.b & sigma & beta=2 & sigma=2 & n=200 & 3.29 \\ 
  144 & PWM & sigma & beta=2 & sigma=2 & n=200 & 2.28 \\ 
  145 & MLE & beta & beta=2.5 & sigma=2 & n=200 & 2.75 \\ 
  146 & MLE.b & beta & beta=2.5 & sigma=2 & n=200 & 2.45 \\ 
  147 & LME & beta & beta=2.5 & sigma=2 & n=200 & 2.78 \\ 
  148 & MDE.Phi.chisq & beta & beta=2.5 & sigma=2 & n=200 & 2.05 \\ 
  149 & MDE.Phi.tv & beta & beta=2.5 & sigma=2 & n=200 & 2.28 \\ 
  150 & MDE.Phi.kl & beta & beta=2.5 & sigma=2 & n=200 & 2.75 \\ 
  151 & MME & beta & beta=2.5 & sigma=2 & n=200 & 3.56 \\ 
  152 & MME.b & beta & beta=2.5 & sigma=2 & n=200 & 3.34 \\ 
  153 & PWM & beta & beta=2.5 & sigma=2 & n=200 & 2.78 \\ 
  154 & MLE & sigma & beta=2.5 & sigma=2 & n=200 & 2.27 \\ 
  155 & MLE.b & sigma & beta=2.5 & sigma=2 & n=200 & 1.94 \\ 
  156 & LME & sigma & beta=2.5 & sigma=2 & n=200 & 2.29 \\ 
  157 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=2 & n=200 & 2.70 \\ 
  158 & MDE.Phi.tv & sigma & beta=2.5 & sigma=2 & n=200 & 2.81 \\ 
  159 & MDE.Phi.kl & sigma & beta=2.5 & sigma=2 & n=200 & 2.27 \\ 
  160 & MME & sigma & beta=2.5 & sigma=2 & n=200 & 3.31 \\ 
  161 & MME.b & sigma & beta=2.5 & sigma=2 & n=200 & 3.01 \\ 
  162 & PWM & sigma & beta=2.5 & sigma=2 & n=200 & 2.29 \\ 
  163 & MLE & beta & beta=3 & sigma=2 & n=200 & 3.55 \\ 
  164 & MLE.b & beta & beta=3 & sigma=2 & n=200 & 3.09 \\ 
  165 & LME & beta & beta=3 & sigma=2 & n=200 & 3.45 \\ 
  166 & MDE.Phi.chisq & beta & beta=3 & sigma=2 & n=200 & 3.31 \\ 
  167 & MDE.Phi.tv & beta & beta=3 & sigma=2 & n=200 & 3.21 \\ 
  168 & MDE.Phi.kl & beta & beta=3 & sigma=2 & n=200 & 3.49 \\ 
  169 & MME & beta & beta=3 & sigma=2 & n=200 & 4.40 \\ 
  170 & MME.b & beta & beta=3 & sigma=2 & n=200 & 5.69 \\ 
  171 & PWM & beta & beta=3 & sigma=2 & n=200 & 3.45 \\ 
  172 & MLE & sigma & beta=3 & sigma=2 & n=200 & 2.48 \\ 
  173 & MLE.b & sigma & beta=3 & sigma=2 & n=200 & 2.07 \\ 
  174 & LME & sigma & beta=3 & sigma=2 & n=200 & 2.38 \\ 
  175 & MDE.Phi.chisq & sigma & beta=3 & sigma=2 & n=200 & 3.54 \\ 
  176 & MDE.Phi.tv & sigma & beta=3 & sigma=2 & n=200 & 3.19 \\ 
  177 & MDE.Phi.kl & sigma & beta=3 & sigma=2 & n=200 & 2.43 \\ 
  178 & MME & sigma & beta=3 & sigma=2 & n=200 & 3.29 \\ 
  179 & MME.b & sigma & beta=3 & sigma=2 & n=200 & 4.46 \\ 
  180 & PWM & sigma & beta=3 & sigma=2 & n=200 & 2.38 \\ 
  181 & MLE & beta & beta=4 & sigma=2 & n=200 & 5.54 \\ 
  182 & MLE.b & beta & beta=4 & sigma=2 & n=200 & 4.87 \\ 
  183 & LME & beta & beta=4 & sigma=2 & n=200 & 4.91 \\ 
  184 & MDE.Phi.chisq & beta & beta=4 & sigma=2 & n=200 & 7.71 \\ 
  185 & MDE.Phi.tv & beta & beta=4 & sigma=2 & n=200 & 6.95 \\ 
  186 & MDE.Phi.kl & beta & beta=4 & sigma=2 & n=200 & 5.26 \\ 
  187 & MME & beta & beta=4 & sigma=2 & n=200 & 6.64 \\ 
  188 & MME.b & beta & beta=4 & sigma=2 & n=200 & 13.69 \\ 
  189 & PWM & beta & beta=4 & sigma=2 & n=200 & 4.91 \\ 
  190 & MLE & sigma & beta=4 & sigma=2 & n=200 & 2.95 \\ 
  191 & MLE.b & sigma & beta=4 & sigma=2 & n=200 & 2.54 \\ 
  192 & LME & sigma & beta=4 & sigma=2 & n=200 & 2.55 \\ 
  193 & MDE.Phi.chisq & sigma & beta=4 & sigma=2 & n=200 & 6.00 \\ 
  194 & MDE.Phi.tv & sigma & beta=4 & sigma=2 & n=200 & 5.13 \\ 
  195 & MDE.Phi.kl & sigma & beta=4 & sigma=2 & n=200 & 2.77 \\ 
  196 & MME & sigma & beta=4 & sigma=2 & n=200 & 3.66 \\ 
  197 & MME.b & sigma & beta=4 & sigma=2 & n=200 & 8.25 \\ 
  198 & PWM & sigma & beta=4 & sigma=2 & n=200 & 2.55 \\ 
  199 & MLE & beta & beta=5 & sigma=2 & n=200 & 13.72 \\ 
  200 & MLE.b & beta & beta=5 & sigma=2 & n=200 & 13.01 \\ 
  201 & LME & beta & beta=5 & sigma=2 & n=200 & 6.78 \\ 
  202 & MDE.Phi.chisq & beta & beta=5 & sigma=2 & n=200 & 14.13 \\ 
  203 & MDE.Phi.tv & beta & beta=5 & sigma=2 & n=200 & 11.36 \\ 
  204 & MDE.Phi.kl & beta & beta=5 & sigma=2 & n=200 & 7.60 \\ 
  205 & MME & beta & beta=5 & sigma=2 & n=200 & 9.76 \\ 
  206 & MME.b & beta & beta=5 & sigma=2 & n=200 & 21.59 \\ 
  207 & PWM & beta & beta=5 & sigma=2 & n=200 & 6.78 \\ 
  208 & MLE & sigma & beta=5 & sigma=2 & n=200 & 6.03 \\ 
  209 & MLE.b & sigma & beta=5 & sigma=2 & n=200 & 5.69 \\ 
  210 & LME & sigma & beta=5 & sigma=2 & n=200 & 2.83 \\ 
  211 & MDE.Phi.chisq & sigma & beta=5 & sigma=2 & n=200 & 8.54 \\ 
  212 & MDE.Phi.tv & sigma & beta=5 & sigma=2 & n=200 & 6.51 \\ 
  213 & MDE.Phi.kl & sigma & beta=5 & sigma=2 & n=200 & 3.23 \\ 
  214 & MME & sigma & beta=5 & sigma=2 & n=200 & 4.27 \\ 
  215 & MME.b & sigma & beta=5 & sigma=2 & n=200 & 9.87 \\ 
  216 & PWM & sigma & beta=5 & sigma=2 & n=200 & 2.83 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220208/Output.var.LaTeX.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Wed Feb 09 03:15:34 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=2 & n=100 & 0.44 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=2 & n=100 & 0.32 \\ 
  3 & LME & beta & beta=1.5 & sigma=2 & n=100 & 0.30 \\ 
  4 & MDE.Phi.chisq & beta & beta=1.5 & sigma=2 & n=100 & 97.61 \\ 
  5 & MDE.Phi.tv & beta & beta=1.5 & sigma=2 & n=100 & 6.78 \\ 
  6 & MDE.Phi.kl & beta & beta=1.5 & sigma=2 & n=100 & 0.44 \\ 
  7 & MME & beta & beta=1.5 & sigma=2 & n=100 & 0.90 \\ 
  8 & MME.b & beta & beta=1.5 & sigma=2 & n=100 & 130047.07 \\ 
  9 & PWM & beta & beta=1.5 & sigma=2 & n=100 & 0.30 \\ 
  10 & MLE & sigma & beta=1.5 & sigma=2 & n=100 & 1.96 \\ 
  11 & MLE.b & sigma & beta=1.5 & sigma=2 & n=100 & 1.45 \\ 
  12 & LME & sigma & beta=1.5 & sigma=2 & n=100 & 1.33 \\ 
  13 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=2 & n=100 & 82.05 \\ 
  14 & MDE.Phi.tv & sigma & beta=1.5 & sigma=2 & n=100 & 70.77 \\ 
  15 & MDE.Phi.kl & sigma & beta=1.5 & sigma=2 & n=100 & 1.96 \\ 
  16 & MME & sigma & beta=1.5 & sigma=2 & n=100 & 7.97 \\ 
  17 & MME.b & sigma & beta=1.5 & sigma=2 & n=100 & 595564.32 \\ 
  18 & PWM & sigma & beta=1.5 & sigma=2 & n=100 & 1.33 \\ 
  19 & MLE & beta & beta=2 & sigma=2 & n=100 & 3433.35 \\ 
  20 & MLE.b & beta & beta=2 & sigma=2 & n=100 & 3433.74 \\ 
  21 & LME & beta & beta=2 & sigma=2 & n=100 & 3.11 \\ 
  22 & MDE.Phi.chisq & beta & beta=2 & sigma=2 & n=100 & 65.39 \\ 
  23 & MDE.Phi.tv & beta & beta=2 & sigma=2 & n=100 & 87.28 \\ 
  24 & MDE.Phi.kl & beta & beta=2 & sigma=2 & n=100 & 12.19 \\ 
  25 & MME & beta & beta=2 & sigma=2 & n=100 & 52.88 \\ 
  26 & MME.b & beta & beta=2 & sigma=2 & n=100 & 151218.71 \\ 
  27 & PWM & beta & beta=2 & sigma=2 & n=100 & 3.11 \\ 
  28 & MLE & sigma & beta=2 & sigma=2 & n=100 & 4325.41 \\ 
  29 & MLE.b & sigma & beta=2 & sigma=2 & n=100 & 4325.97 \\ 
  30 & LME & sigma & beta=2 & sigma=2 & n=100 & 5.78 \\ 
  31 & MDE.Phi.chisq & sigma & beta=2 & sigma=2 & n=100 & 298.76 \\ 
  32 & MDE.Phi.tv & sigma & beta=2 & sigma=2 & n=100 & 379.09 \\ 
  33 & MDE.Phi.kl & sigma & beta=2 & sigma=2 & n=100 & 20.44 \\ 
  34 & MME & sigma & beta=2 & sigma=2 & n=100 & 91.42 \\ 
  35 & MME.b & sigma & beta=2 & sigma=2 & n=100 & 334195.41 \\ 
  36 & PWM & sigma & beta=2 & sigma=2 & n=100 & 5.78 \\ 
  37 & MLE & beta & beta=2.5 & sigma=2 & n=100 & 7443.04 \\ 
  38 & MLE.b & beta & beta=2.5 & sigma=2 & n=100 & 7444.73 \\ 
  39 & LME & beta & beta=2.5 & sigma=2 & n=100 & 8.34 \\ 
  40 & MDE.Phi.chisq & beta & beta=2.5 & sigma=2 & n=100 & 224.57 \\ 
  41 & MDE.Phi.tv & beta & beta=2.5 & sigma=2 & n=100 & 256.61 \\ 
  42 & MDE.Phi.kl & beta & beta=2.5 & sigma=2 & n=100 & 29.78 \\ 
  43 & MME & beta & beta=2.5 & sigma=2 & n=100 & 144.30 \\ 
  44 & MME.b & beta & beta=2.5 & sigma=2 & n=100 & 2205.73 \\ 
  45 & PWM & beta & beta=2.5 & sigma=2 & n=100 & 8.34 \\ 
  46 & MLE & sigma & beta=2.5 & sigma=2 & n=100 & 8765.63 \\ 
  47 & MLE.b & sigma & beta=2.5 & sigma=2 & n=100 & 8767.58 \\ 
  48 & LME & sigma & beta=2.5 & sigma=2 & n=100 & 8.99 \\ 
  49 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=2 & n=100 & 535.71 \\ 
  50 & MDE.Phi.tv & sigma & beta=2.5 & sigma=2 & n=100 & 611.37 \\ 
  51 & MDE.Phi.kl & sigma & beta=2.5 & sigma=2 & n=100 & 32.58 \\ 
  52 & MME & sigma & beta=2.5 & sigma=2 & n=100 & 150.14 \\ 
  53 & MME.b & sigma & beta=2.5 & sigma=2 & n=100 & 2520.30 \\ 
  54 & PWM & sigma & beta=2.5 & sigma=2 & n=100 & 8.99 \\ 
  55 & MLE & beta & beta=3 & sigma=2 & n=100 & 52170.36 \\ 
  56 & MLE.b & beta & beta=3 & sigma=2 & n=100 & 52179.68 \\ 
  57 & LME & beta & beta=3 & sigma=2 & n=100 & 15.99 \\ 
  58 & MDE.Phi.chisq & beta & beta=3 & sigma=2 & n=100 & 480.90 \\ 
  59 & MDE.Phi.tv & beta & beta=3 & sigma=2 & n=100 & 575.77 \\ 
  60 & MDE.Phi.kl & beta & beta=3 & sigma=2 & n=100 & 100.86 \\ 
  61 & MME & beta & beta=3 & sigma=2 & n=100 & 313146.34 \\ 
  62 & MME.b & beta & beta=3 & sigma=2 & n=100 & 2977375.72 \\ 
  63 & PWM & beta & beta=3 & sigma=2 & n=100 & 15.99 \\ 
  64 & MLE & sigma & beta=3 & sigma=2 & n=100 & 41292.16 \\ 
  65 & MLE.b & sigma & beta=3 & sigma=2 & n=100 & 41299.12 \\ 
  66 & LME & sigma & beta=3 & sigma=2 & n=100 & 12.33 \\ 
  67 & MDE.Phi.chisq & sigma & beta=3 & sigma=2 & n=100 & 759.10 \\ 
  68 & MDE.Phi.tv & sigma & beta=3 & sigma=2 & n=100 & 886.52 \\ 
  69 & MDE.Phi.kl & sigma & beta=3 & sigma=2 & n=100 & 75.13 \\ 
  70 & MME & sigma & beta=3 & sigma=2 & n=100 & 180846.34 \\ 
  71 & MME.b & sigma & beta=3 & sigma=2 & n=100 & 1721384.96 \\ 
  72 & PWM & sigma & beta=3 & sigma=2 & n=100 & 12.33 \\ 
  73 & MLE & beta & beta=4 & sigma=2 & n=100 & 90920.58 \\ 
  74 & MLE.b & beta & beta=4 & sigma=2 & n=100 & 90934.14 \\ 
  75 & LME & beta & beta=4 & sigma=2 & n=100 & 48.77 \\ 
  76 & MDE.Phi.chisq & beta & beta=4 & sigma=2 & n=100 & 1195.04 \\ 
  77 & MDE.Phi.tv & beta & beta=4 & sigma=2 & n=100 & 1368.63 \\ 
  78 & MDE.Phi.kl & beta & beta=4 & sigma=2 & n=100 & 201.29 \\ 
  79 & MME & beta & beta=4 & sigma=2 & n=100 & 11556.91 \\ 
  80 & MME.b & beta & beta=4 & sigma=2 & n=100 & 1921162.31 \\ 
  81 & PWM & beta & beta=4 & sigma=2 & n=100 & 48.77 \\ 
  82 & MLE & sigma & beta=4 & sigma=2 & n=100 & 33275.60 \\ 
  83 & MLE.b & sigma & beta=4 & sigma=2 & n=100 & 33280.59 \\ 
  84 & LME & sigma & beta=4 & sigma=2 & n=100 & 18.76 \\ 
  85 & MDE.Phi.chisq & sigma & beta=4 & sigma=2 & n=100 & 926.76 \\ 
  86 & MDE.Phi.tv & sigma & beta=4 & sigma=2 & n=100 & 1007.89 \\ 
  87 & MDE.Phi.kl & sigma & beta=4 & sigma=2 & n=100 & 79.61 \\ 
  88 & MME & sigma & beta=4 & sigma=2 & n=100 & 4346.18 \\ 
  89 & MME.b & sigma & beta=4 & sigma=2 & n=100 & 1082212.14 \\ 
  90 & PWM & sigma & beta=4 & sigma=2 & n=100 & 18.76 \\ 
  91 & MLE & beta & beta=5 & sigma=2 & n=100 & 165313.77 \\ 
  92 & MLE.b & beta & beta=5 & sigma=2 & n=100 & 165333.21 \\ 
  93 & LME & beta & beta=5 & sigma=2 & n=100 & 96.10 \\ 
  94 & MDE.Phi.chisq & beta & beta=5 & sigma=2 & n=100 & 1864.51 \\ 
  95 & MDE.Phi.tv & beta & beta=5 & sigma=2 & n=100 & 2004.22 \\ 
  96 & MDE.Phi.kl & beta & beta=5 & sigma=2 & n=100 & 347.29 \\ 
  97 & MME & beta & beta=5 & sigma=2 & n=100 & 18587.85 \\ 
  98 & MME.b & beta & beta=5 & sigma=2 & n=100 & 257840.15 \\ 
  99 & PWM & beta & beta=5 & sigma=2 & n=100 & 96.10 \\ 
  100 & MLE & sigma & beta=5 & sigma=2 & n=100 & 37555.48 \\ 
  101 & MLE.b & sigma & beta=5 & sigma=2 & n=100 & 37559.75 \\ 
  102 & LME & sigma & beta=5 & sigma=2 & n=100 & 21.26 \\ 
  103 & MDE.Phi.chisq & sigma & beta=5 & sigma=2 & n=100 & 832.80 \\ 
  104 & MDE.Phi.tv & sigma & beta=5 & sigma=2 & n=100 & 860.14 \\ 
  105 & MDE.Phi.kl & sigma & beta=5 & sigma=2 & n=100 & 76.96 \\ 
  106 & MME & sigma & beta=5 & sigma=2 & n=100 & 4147.18 \\ 
  107 & MME.b & sigma & beta=5 & sigma=2 & n=100 & 61786.34 \\ 
  108 & PWM & sigma & beta=5 & sigma=2 & n=100 & 21.26 \\ 
  109 & MLE & beta & beta=1.5 & sigma=2 & n=200 & 0.10 \\ 
  110 & MLE.b & beta & beta=1.5 & sigma=2 & n=200 & 0.08 \\ 
  111 & LME & beta & beta=1.5 & sigma=2 & n=200 & 0.11 \\ 
  112 & MDE.Phi.chisq & beta & beta=1.5 & sigma=2 & n=200 & 22.83 \\ 
  113 & MDE.Phi.tv & beta & beta=1.5 & sigma=2 & n=200 & 0.17 \\ 
  114 & MDE.Phi.kl & beta & beta=1.5 & sigma=2 & n=200 & 0.10 \\ 
  115 & MME & beta & beta=1.5 & sigma=2 & n=200 & 0.16 \\ 
  116 & MME.b & beta & beta=1.5 & sigma=2 & n=200 & 0.26 \\ 
  117 & PWM & beta & beta=1.5 & sigma=2 & n=200 & 0.11 \\ 
  118 & MLE & sigma & beta=1.5 & sigma=2 & n=200 & 0.43 \\ 
  119 & MLE.b & sigma & beta=1.5 & sigma=2 & n=200 & 0.32 \\ 
  120 & LME & sigma & beta=1.5 & sigma=2 & n=200 & 0.49 \\ 
  121 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=2 & n=200 & 3.32 \\ 
  122 & MDE.Phi.tv & sigma & beta=1.5 & sigma=2 & n=200 & 1.16 \\ 
  123 & MDE.Phi.kl & sigma & beta=1.5 & sigma=2 & n=200 & 0.43 \\ 
  124 & MME & sigma & beta=1.5 & sigma=2 & n=200 & 6.07 \\ 
  125 & MME.b & sigma & beta=1.5 & sigma=2 & n=200 & 6.44 \\ 
  126 & PWM & sigma & beta=1.5 & sigma=2 & n=200 & 0.49 \\ 
  127 & MLE & beta & beta=2 & sigma=2 & n=200 & 0.30 \\ 
  128 & MLE.b & beta & beta=2 & sigma=2 & n=200 & 0.19 \\ 
  129 & LME & beta & beta=2 & sigma=2 & n=200 & 0.30 \\ 
  130 & MDE.Phi.chisq & beta & beta=2 & sigma=2 & n=200 & 2.19 \\ 
  131 & MDE.Phi.tv & beta & beta=2 & sigma=2 & n=200 & 2.21 \\ 
  132 & MDE.Phi.kl & beta & beta=2 & sigma=2 & n=200 & 0.30 \\ 
  133 & MME & beta & beta=2 & sigma=2 & n=200 & 0.53 \\ 
  134 & MME.b & beta & beta=2 & sigma=2 & n=200 & 5.40 \\ 
  135 & PWM & beta & beta=2 & sigma=2 & n=200 & 0.30 \\ 
  136 & MLE & sigma & beta=2 & sigma=2 & n=200 & 0.59 \\ 
  137 & MLE.b & sigma & beta=2 & sigma=2 & n=200 & 0.37 \\ 
  138 & LME & sigma & beta=2 & sigma=2 & n=200 & 0.60 \\ 
  139 & MDE.Phi.chisq & sigma & beta=2 & sigma=2 & n=200 & 7.14 \\ 
  140 & MDE.Phi.tv & sigma & beta=2 & sigma=2 & n=200 & 9.14 \\ 
  141 & MDE.Phi.kl & sigma & beta=2 & sigma=2 & n=200 & 0.59 \\ 
  142 & MME & sigma & beta=2 & sigma=2 & n=200 & 1.11 \\ 
  143 & MME.b & sigma & beta=2 & sigma=2 & n=200 & 10.20 \\ 
  144 & PWM & sigma & beta=2 & sigma=2 & n=200 & 0.60 \\ 
  145 & MLE & beta & beta=2.5 & sigma=2 & n=200 & 1.12 \\ 
  146 & MLE.b & beta & beta=2.5 & sigma=2 & n=200 & 0.83 \\ 
  147 & LME & beta & beta=2.5 & sigma=2 & n=200 & 1.20 \\ 
  148 & MDE.Phi.chisq & beta & beta=2.5 & sigma=2 & n=200 & 17.88 \\ 
  149 & MDE.Phi.tv & beta & beta=2.5 & sigma=2 & n=200 & 13.81 \\ 
  150 & MDE.Phi.kl & beta & beta=2.5 & sigma=2 & n=200 & 1.12 \\ 
  151 & MME & beta & beta=2.5 & sigma=2 & n=200 & 1.77 \\ 
  152 & MME.b & beta & beta=2.5 & sigma=2 & n=200 & 43.75 \\ 
  153 & PWM & beta & beta=2.5 & sigma=2 & n=200 & 1.20 \\ 
  154 & MLE & sigma & beta=2.5 & sigma=2 & n=200 & 1.33 \\ 
  155 & MLE.b & sigma & beta=2.5 & sigma=2 & n=200 & 0.99 \\ 
  156 & LME & sigma & beta=2.5 & sigma=2 & n=200 & 1.36 \\ 
  157 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=2 & n=200 & 36.10 \\ 
  158 & MDE.Phi.tv & sigma & beta=2.5 & sigma=2 & n=200 & 26.62 \\ 
  159 & MDE.Phi.kl & sigma & beta=2.5 & sigma=2 & n=200 & 1.33 \\ 
  160 & MME & sigma & beta=2.5 & sigma=2 & n=200 & 2.13 \\ 
  161 & MME.b & sigma & beta=2.5 & sigma=2 & n=200 & 49.26 \\ 
  162 & PWM & sigma & beta=2.5 & sigma=2 & n=200 & 1.36 \\ 
  163 & MLE & beta & beta=3 & sigma=2 & n=200 & 64.24 \\ 
  164 & MLE.b & beta & beta=3 & sigma=2 & n=200 & 63.98 \\ 
  165 & LME & beta & beta=3 & sigma=2 & n=200 & 4.14 \\ 
  166 & MDE.Phi.chisq & beta & beta=3 & sigma=2 & n=200 & 89.01 \\ 
  167 & MDE.Phi.tv & beta & beta=3 & sigma=2 & n=200 & 42.69 \\ 
  168 & MDE.Phi.kl & beta & beta=3 & sigma=2 & n=200 & 7.73 \\ 
  169 & MME & beta & beta=3 & sigma=2 & n=200 & 73.03 \\ 
  170 & MME.b & beta & beta=3 & sigma=2 & n=200 & 7346.85 \\ 
  171 & PWM & beta & beta=3 & sigma=2 & n=200 & 4.14 \\ 
  172 & MLE & sigma & beta=3 & sigma=2 & n=200 & 41.44 \\ 
  173 & MLE.b & sigma & beta=3 & sigma=2 & n=200 & 41.23 \\ 
  174 & LME & sigma & beta=3 & sigma=2 & n=200 & 2.98 \\ 
  175 & MDE.Phi.chisq & sigma & beta=3 & sigma=2 & n=200 & 117.14 \\ 
  176 & MDE.Phi.tv & sigma & beta=3 & sigma=2 & n=200 & 52.01 \\ 
  177 & MDE.Phi.kl & sigma & beta=3 & sigma=2 & n=200 & 5.50 \\ 
  178 & MME & sigma & beta=3 & sigma=2 & n=200 & 47.45 \\ 
  179 & MME.b & sigma & beta=3 & sigma=2 & n=200 & 6725.97 \\ 
  180 & PWM & sigma & beta=3 & sigma=2 & n=200 & 2.98 \\ 
  181 & MLE & beta & beta=4 & sigma=2 & n=200 & 358.41 \\ 
  182 & MLE.b & beta & beta=4 & sigma=2 & n=200 & 359.86 \\ 
  183 & LME & beta & beta=4 & sigma=2 & n=200 & 17.45 \\ 
  184 & MDE.Phi.chisq & beta & beta=4 & sigma=2 & n=200 & 465.08 \\ 
  185 & MDE.Phi.tv & beta & beta=4 & sigma=2 & n=200 & 346.11 \\ 
  186 & MDE.Phi.kl & beta & beta=4 & sigma=2 & n=200 & 41.24 \\ 
  187 & MME & beta & beta=4 & sigma=2 & n=200 & 544.09 \\ 
  188 & MME.b & beta & beta=4 & sigma=2 & n=200 & 40207.12 \\ 
  189 & PWM & beta & beta=4 & sigma=2 & n=200 & 17.45 \\ 
  190 & MLE & sigma & beta=4 & sigma=2 & n=200 & 138.54 \\ 
  191 & MLE.b & sigma & beta=4 & sigma=2 & n=200 & 139.07 \\ 
  192 & LME & sigma & beta=4 & sigma=2 & n=200 & 6.55 \\ 
  193 & MDE.Phi.chisq & sigma & beta=4 & sigma=2 & n=200 & 303.58 \\ 
  194 & MDE.Phi.tv & sigma & beta=4 & sigma=2 & n=200 & 220.00 \\ 
  195 & MDE.Phi.kl & sigma & beta=4 & sigma=2 & n=200 & 15.59 \\ 
  196 & MME & sigma & beta=4 & sigma=2 & n=200 & 210.92 \\ 
  197 & MME.b & sigma & beta=4 & sigma=2 & n=200 & 19770.86 \\ 
  198 & PWM & sigma & beta=4 & sigma=2 & n=200 & 6.55 \\ 
  199 & MLE & beta & beta=5 & sigma=2 & n=200 & 67107.26 \\ 
  200 & MLE.b & beta & beta=5 & sigma=2 & n=200 & 67119.97 \\ 
  201 & LME & beta & beta=5 & sigma=2 & n=200 & 63.08 \\ 
  202 & MDE.Phi.chisq & beta & beta=5 & sigma=2 & n=200 & 1137.09 \\ 
  203 & MDE.Phi.tv & beta & beta=5 & sigma=2 & n=200 & 766.54 \\ 
  204 & MDE.Phi.kl & beta & beta=5 & sigma=2 & n=200 & 134.88 \\ 
  205 & MME & beta & beta=5 & sigma=2 & n=200 & 2723.73 \\ 
  206 & MME.b & beta & beta=5 & sigma=2 & n=200 & 30712.87 \\ 
  207 & PWM & beta & beta=5 & sigma=2 & n=200 & 63.08 \\ 
  208 & MLE & sigma & beta=5 & sigma=2 & n=200 & 13936.89 \\ 
  209 & MLE.b & sigma & beta=5 & sigma=2 & n=200 & 13939.65 \\ 
  210 & LME & sigma & beta=5 & sigma=2 & n=200 & 14.12 \\ 
  211 & MDE.Phi.chisq & sigma & beta=5 & sigma=2 & n=200 & 435.77 \\ 
  212 & MDE.Phi.tv & sigma & beta=5 & sigma=2 & n=200 & 279.11 \\ 
  213 & MDE.Phi.kl & sigma & beta=5 & sigma=2 & n=200 & 30.09 \\ 
  214 & MME & sigma & beta=5 & sigma=2 & n=200 & 592.18 \\ 
  215 & MME.b & sigma & beta=5 & sigma=2 & n=200 & 6949.35 \\ 
  216 & PWM & sigma & beta=5 & sigma=2 & n=200 & 14.12 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220209/20220208-11h15-Full.beta=1.5.sig=3.n=100.LaTeX.tex <==
% START DATE AND TIME=20220208-11h15
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=1.5,  \sigma=3$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.6717&1.4777&1.8288&-1.8659&1.2349&1.6717&2.7927&6.3149&1.8288
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
3.5467&2.9323&3.976&5.2184&5.488&3.5467&9.4574&20.5029&3.976
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.4353&0.3215&0.2958&347.7844&6.2223&0.4353&0.8967&130047.0665&0.2958
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
4.4066&3.2548&2.9924&173.3936&144.6706&4.4068&17.9315&1340019.7055&2.9924
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1717&-0.0223&0.3288&-3.3659&-0.2651&0.1717&1.2927&4.8149&0.3288
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.5467&-0.0677&0.976&2.2184&2.488&0.5467&6.4574&17.5029&0.976
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.4647&0.322&0.4039&359.079&6.292&0.4647&2.5678&130057.2449&0.4039
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
4.7051&3.2591&3.9447&178.2978&150.8462&4.7053&59.6278&1340192.0551&3.9447
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 5.1698&3.5811&4.3485&537.3768&157.1382&5.17&62.1955&1470249.3&4.3485\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0011&0.0011&2.9905720362169e+301&0.0459&0.0011&0.0099&7.105&0.0011\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220209/20220208-11h15-Full.beta=1.5.sig=3.n=200.LaTeX.tex <==
% START DATE AND TIME=20220208-11h15
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=1.5,  \sigma=3$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.5786&1.4957&1.7058&0.1828&0.9983&1.5786&2.4958&2.2963&1.7058
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
3.2459&2.9853&3.6086&3.6521&3.7774&3.2459&8.3565&7.529&3.6086
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1016&0.077&0.112&70.3221&0.1791&0.1016&0.1649&0.2558&0.112
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.9743&0.7236&1.113&12.7062&2.5972&0.9744&13.6369&14.4779&1.113
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.0786&-0.0043&0.2058&-1.3172&-0.5017&0.0786&0.9958&0.7963&0.2058
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.2459&-0.0147&0.6086&0.6521&0.7774&0.2459&5.3565&4.529&0.6086
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1078&0.077&0.1543&72.0501&0.4308&0.1078&1.1565&0.8899&0.1543
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.0347&0.7238&1.4833&13.1301&3.2014&1.0347&42.3274&34.9885&1.4833
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 1.1424&0.8008&1.6376&85.1802&3.6321&1.1425&43.4839&35.8784&1.6376\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 6e-04&6e-04&6e-04&9.83790728945794e+300&0.0309&6e-04&0.0089&0.0103&6e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220209/20220208-11h15-Full.beta=2.5.sig=3.n=100.LaTeX.tex <==
% START DATE AND TIME=20220208-11h15
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2.5,  \sigma=3$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 4.5273&4.0701&3.1958&4.0175&4.8287&3.4298&4.8214&7.9937&3.1958
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
6.2766&5.5333&4.0776&9.0167&10.566&4.4977&7.0633&12.0647&4.0776
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 5311.4494&5312.969&8.3445&201.5068&230.7047&27.8278&144.3027&2205.727&8.3445
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
14034.8595&14038.7664&20.2358&1089.1693&1237.7166&68.5196&337.8156&5670.6747&20.2358
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.0273&1.5701&0.6958&1.5175&2.3287&0.9298&2.3214&5.4937&0.6958
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
3.2766&2.5333&1.0776&6.0167&7.566&1.4977&4.0633&9.0647&1.0776
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 5315.0284&5314.9029&8.8279&203.7893&236.1046&28.6896&149.6771&2235.6866&8.8279
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
14044.1924&14043.7803&21.395&1125.2616&1294.8367&70.7557&354.2926&5752.2769&21.395
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 19359.2208&19358.6832&30.2229&1329.0509&1530.9413&99.4453&503.9697&7987.9635&30.2229\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0012&0.0011&0.0234&0.0179&0.0011&0.0019&8.078&0.0011\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220209/20220208-11h15-Full.beta=2.5.sig=3.n=200.LaTeX.tex <==
% START DATE AND TIME=20220208-11h15
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2.5,  \sigma=3$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.7519&2.4472&2.784&2.0424&2.2722&2.7519&3.5622&3.3354&2.784
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
3.4072&2.9128&3.4341&4.0362&4.2035&3.4071&4.9641&4.5203&3.4341
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.1169&0.8306&1.1974&15.987&12.5394&1.1169&1.7744&43.7481&1.1974
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
2.985&2.2267&3.0677&72.6552&54.464&2.985&4.7924&110.8394&3.0677
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.2519&-0.0528&0.284&-0.4576&-0.2278&0.2519&1.0622&0.8354&0.284
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.4072&-0.0872&0.4341&1.0362&1.2035&0.4071&1.9641&1.5203&0.4341
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.1803&0.8333&1.278&16.1948&12.5901&1.1802&2.9024&44.4416&1.278
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
3.1505&2.2341&3.2558&73.7217&55.907&3.1505&8.6494&113.1395&3.2558
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 4.3308&3.0674&4.5338&89.9165&68.497&4.3307&11.5518&157.5811&4.5338\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&5e-04&5e-04&0.0174&0.0121&5e-04&0.0011&0.0017&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220209/20220208-11h15-Full.beta=2.sig=3.n=100.LaTeX.tex <==
% START DATE AND TIME=20220208-11h15
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2,  \sigma=3$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.9934&2.6437&2.4461&2.0099&2.6563&2.4547&3.6775&9.4751&2.4461
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
4.8908&4.1329&3.9049&6.227&7.7111&3.9647&7.312&19.7596&3.9049
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2428.2951&2428.6148&3.1121&65.3242&78.4711&11.3227&52.8831&151218.7131&3.1121
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
6896.9284&6897.964&13.005&604.2028&766.9694&42.7687&205.6852&751939.6683&13.005
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.9934&0.6437&0.4461&0.0099&0.6563&0.4547&1.6775&7.4751&0.4461
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.8908&1.1329&0.9049&3.227&4.7111&0.9647&4.312&16.7596&0.9049
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2429.0391&2428.7863&3.3109&65.3177&78.894&11.5283&55.6919&151259.4685&3.3109
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
6899.8137&6898.5578&13.8227&614.5561&789.0876&43.6951&224.2577&752145.3587&13.8227
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 9328.8528&9327.3441&17.1335&679.8738&867.9815&55.2234&279.9497&903404.8272&17.1335\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0011&0.0011&2.00401541349742e+299&0.0234&0.0011&0.0035&0.0115&0.0011\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220209/20220208-11h15-Full.beta=2.sig=3.n=200.LaTeX.tex <==
% START DATE AND TIME=20220208-11h15
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2,  \sigma=3$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.1371&1.968&2.2155&1.3244&1.5621&2.1371&2.9719&2.6875&2.2155
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
3.289&2.9259&3.4254&3.5195&3.8315&3.289&5.6652&4.9393&3.4254
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.2964&0.1915&0.3033&4.286&2.0349&0.2964&0.5313&5.3982&0.3033
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.3225&0.8411&1.3479&14.8622&18.7607&1.3225&2.4965&22.9529&1.3479
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1371&-0.032&0.2155&-0.6756&-0.4379&0.1371&0.9719&0.6875&0.2155
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.289&-0.0741&0.4254&0.5195&0.8315&0.289&2.6652&1.9393&0.4254
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.3151&0.1925&0.3497&4.742&2.2264&0.3151&1.4758&5.8704&0.3497
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.4058&0.8465&1.5288&15.1305&19.4502&1.4058&9.5997&26.7113&1.5288
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 1.721&1.039&1.8785&19.8726&21.6766&1.721&11.0756&32.5817&1.8785\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&5e-04&5e-04&3.22760432783316e+298&0.0166&5e-04&0.0024&0.0024&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220209/20220208-11h15-Full.beta=3.sig=3.n=100.LaTeX.tex <==
% START DATE AND TIME=20220208-11h15
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=3,  \sigma=3$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 11.5407&11.0465&4.0159&6.617&7.9612&4.8283&17.4875&49.9897&4.0159
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
14.0828&13.4424&4.2766&11.9928&14.0518&5.3637&20.2254&58.7064&4.2766
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 39517.8662&39526.2673&15.9909&428.3696&508.6058&92.1956&313146.3373&2977375.6111&15.9909
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
69270.6739&69284.7165&27.7502&1517.48&1763.6669&154.9947&406904.261&3873116.014&27.7502
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 8.5407&8.0465&1.0159&3.617&4.9612&1.8283&14.4875&46.9897&1.0159
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
11.0828&10.4424&1.2766&8.9928&11.0518&2.3637&17.2254&55.7064&1.2766
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 39586.8571&39587.0603&17.0213&441.4096&533.1686&95.5289&313324.9101&2979285.9022&17.0213
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
69386.575&69386.8316&29.3771&1598.1991&1885.633&160.5662&407160.2857&3875831.9031&29.3771
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 108973.4321&108973.8919&46.3984&2039.6087&2418.8016&256.0951&720485.1958&6855117.8054&46.3984\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0012&0.0011&0.02&0.0151&0.0011&0.0014&0.0075&0.0011\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220209/20220208-11h15-Full.beta=3.sig=3.n=200.LaTeX.tex <==
% START DATE AND TIME=20220208-11h15
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=3,  \sigma=3$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 3.5544&3.09&3.4534&3.2673&3.1906&3.4913&4.4029&5.6932&3.4534
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
3.7125&3.1093&3.5675&5.2489&4.7619&3.6371&4.9384&6.6949&3.5675
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 64.1243&63.867&4.1436&79.1389&38.5027&7.4645&73.0294&7346.8516&4.1436
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
93.0678&92.603&6.6999&234.3241&105.5015&11.9975&106.7695&15133.4347&6.6999
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.5544&0.09&0.4534&0.2673&0.1906&0.4913&1.4029&2.6932&0.4534
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
0.7125&0.1093&0.5675&2.2489&1.7619&0.6371&1.9384&3.6949&0.5675
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 64.4252&63.8688&4.3487&79.2024&38.5351&7.7052&74.9902&7353.3704&4.3487
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
93.5662&92.6057&7.0213&239.3581&108.5952&12.4021&110.5163&15145.5737&7.0213
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 157.9914&156.4744&11.3701&318.5604&147.1303&20.1073&185.5064&22498.9441&11.3701\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&5e-04&5e-04&0.0143&0.0096&5e-04&7e-04&0.0018&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220209/20220208-11h15-Full.beta=4.sig=3.n=100.LaTeX.tex <==
% START DATE AND TIME=20220208-11h15
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=4,  \sigma=3$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 17.3595&16.9104&5.7439&13.1726&15.2643&7.3722&11.3526&40.9056&5.7439
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
15.1818&14.7731&4.594&16.9728&19.0218&6.1367&9.9959&40.2968&4.594
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 75623.3701&75636.1017&46.4798&1047.1043&1197.4337&187.367&11556.8269&1921162.0988&46.4798
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
61498.8136&61509.3374&40.891&1826.9501&1987.6973&166.4248&9778.8741&2434977.1101&40.891
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 13.3595&12.9104&1.7439&9.1726&11.2643&3.3722&7.3526&36.9056&1.7439
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
12.1818&11.7731&1.594&13.9728&16.0218&3.1367&6.9959&37.2968&1.594
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 75794.2851&75795.2153&49.5164&1131.1369&1324.1976&198.7199&11609.7317&1922332.0076&49.5164
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
61641.0603&61641.7935&43.4277&2022.0065&2244.1963&176.2473&9826.8391&2436124.6612&43.4277
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 137435.3454&137437.0088&92.9441&3153.1434&3568.3939&374.9672&21436.5708&4358456.6688&92.9441\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0012&0.001&0.0165&0.0123&0.0011&0.0011&4041.9544&0.001\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220209/20220208-11h15-Full.beta=4.sig=3.n=200.LaTeX.tex <==
% START DATE AND TIME=20220208-11h15
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=4,  \sigma=3$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 5.541&4.8719&4.9153&7.4836&6.8028&5.2485&6.6383&13.686&4.9153
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
4.4279&3.8136&3.83&8.7342&7.5207&4.1543&5.4936&12.3829&3.83
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 353.0514&354.4934&17.4518&406.8515&306.737&38.6007&544.0967&40207.1077&17.4518
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
307.0894&308.2915&14.7413&597.7916&438.3287&32.9084&474.5803&44484.4247&14.7413
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.541&0.8719&0.9153&3.4836&2.8028&1.2485&2.6383&9.686&0.9153
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
1.4279&0.8136&0.83&5.7342&4.5207&1.1543&2.4936&9.3829&0.83
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 355.3908&355.2183&18.2878&418.9461&314.562&40.1556&551.0031&40296.9063&18.2878
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
309.0977&308.9226&15.4287&630.6127&458.7218&34.2375&480.751&44568.0157&15.4287
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 664.4885&664.1409&33.7166&1049.5588&773.2838&74.3932&1031.7541&84864.922&33.7166\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&6e-04&5e-04&0.0111&0.0074&5e-04&6e-04&0.0029&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220209/20220208-11h15-Full.beta=5.sig=3.n=100.LaTeX.tex <==
% START DATE AND TIME=20220208-11h15
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=5,  \sigma=3$ $n=100$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 28.3725&28.0041&7.3006&19.1382&21.1952&9.9529&16.7085&47.1193&7.3006
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
19.5867&19.3299&4.612&18.8325&20.2195&6.4976&11.2323&32.8693&4.612
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 144295.0991&144313.6151&87.3263&1624.2501&1742.1592&319.0036&18586.5629&257834.8442&87.3263
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
73489.8444&73498.9813&44.0403&1635.5487&1683.5124&159.4715&9330.5751&139016.8681&44.0403
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 23.3725&23.0041&2.3006&14.1382&16.1952&4.9529&11.7085&42.1193&2.3006
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
16.5867&16.3299&1.612&15.8325&17.2195&3.4976&8.2323&29.8693&1.612
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 144826.9444&144828.3722&92.6105&1823.977&2004.2705&343.5029&18721.7941&259583.0957&92.6105
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
73757.6153&73758.2971&46.6346&1886.0545&1979.8559&171.6886&9397.4128&139895.1389&46.6346
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 218584.5597&218586.6692&139.2451&3710.0314&3984.1265&515.1915&28119.2069&399478.2346&139.2451\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.001&0.0012&0.001&0.0144&0.0106&0.001&0.001&5.1562081310583e+29&0.001\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220209/20220208-11h15-Full.beta=5.sig=3.n=200.LaTeX.tex <==
% START DATE AND TIME=20220208-11h15
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=5,  \sigma=3$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 12.0233&11.3158&6.7653&13.5709&11.0065&7.555&9.766&21.612&6.7653
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
7.9373&7.437&4.2398&12.2902&9.447&4.8087&6.4025&14.8283&4.2398
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 41080.7111&41091.0122&60.6859&990.7491&670.8996&123.7823&2723.6789&30716.4258&60.6859
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
20188.4973&20193.5931&30.8252&853.3593&548.9097&62.3844&1332.3982&15637.6016&30.8252
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 7.0233&6.3158&1.7653&8.5709&6.0065&2.555&4.766&16.612&1.7653
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
4.9373&4.437&1.2398&9.2902&6.447&1.8087&3.4025&11.8283&1.2398
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 41125.9299&41126.7925&63.7962&1064.1106&706.9112&130.2977&2746.1214&30989.3115&63.7962
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} & 
20210.8553&20211.2605&32.3591&939.5812&590.4183&65.6497&1343.8421&15775.946&32.3591
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 61336.7853&61338.053&96.1554&2003.6918&1297.3295&195.9474&4089.9635&46765.2574&96.1554\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&6e-04&5e-04&0.0096&0.0062&5e-04&5e-04&2.018&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220209/Output.accuracy.LaTeX.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Wed Feb 09 03:24:10 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & Measure & beta=1.5 & sigma=3 & n=100 & 5.17 \\ 
  2 & MLE.b & Measure & beta=1.5 & sigma=3 & n=100 & 3.58 \\ 
  3 & LME & Measure & beta=1.5 & sigma=3 & n=100 & 4.35 \\ 
  4 & MDE.Phi.chisq & Measure & beta=1.5 & sigma=3 & n=100 & 537.38 \\ 
  5 & MDE.Phi.tv & Measure & beta=1.5 & sigma=3 & n=100 & 157.14 \\ 
  6 & MDE.Phi.kl & Measure & beta=1.5 & sigma=3 & n=100 & 5.17 \\ 
  7 & MME & Measure & beta=1.5 & sigma=3 & n=100 & 62.20 \\ 
  8 & MME.b & Measure & beta=1.5 & sigma=3 & n=100 & 1470249.30 \\ 
  9 & PWM & Measure & beta=1.5 & sigma=3 & n=100 & 4.35 \\ 
  10 & MLE & Measure & beta=2 & sigma=3 & n=100 & 9328.85 \\ 
  11 & MLE.b & Measure & beta=2 & sigma=3 & n=100 & 9327.34 \\ 
  12 & LME & Measure & beta=2 & sigma=3 & n=100 & 17.13 \\ 
  13 & MDE.Phi.chisq & Measure & beta=2 & sigma=3 & n=100 & 679.87 \\ 
  14 & MDE.Phi.tv & Measure & beta=2 & sigma=3 & n=100 & 867.98 \\ 
  15 & MDE.Phi.kl & Measure & beta=2 & sigma=3 & n=100 & 55.22 \\ 
  16 & MME & Measure & beta=2 & sigma=3 & n=100 & 279.95 \\ 
  17 & MME.b & Measure & beta=2 & sigma=3 & n=100 & 903404.83 \\ 
  18 & PWM & Measure & beta=2 & sigma=3 & n=100 & 17.13 \\ 
  19 & MLE & Measure & beta=2.5 & sigma=3 & n=100 & 19359.22 \\ 
  20 & MLE.b & Measure & beta=2.5 & sigma=3 & n=100 & 19358.68 \\ 
  21 & LME & Measure & beta=2.5 & sigma=3 & n=100 & 30.22 \\ 
  22 & MDE.Phi.chisq & Measure & beta=2.5 & sigma=3 & n=100 & 1329.05 \\ 
  23 & MDE.Phi.tv & Measure & beta=2.5 & sigma=3 & n=100 & 1530.94 \\ 
  24 & MDE.Phi.kl & Measure & beta=2.5 & sigma=3 & n=100 & 99.45 \\ 
  25 & MME & Measure & beta=2.5 & sigma=3 & n=100 & 503.97 \\ 
  26 & MME.b & Measure & beta=2.5 & sigma=3 & n=100 & 7987.96 \\ 
  27 & PWM & Measure & beta=2.5 & sigma=3 & n=100 & 30.22 \\ 
  28 & MLE & Measure & beta=3 & sigma=3 & n=100 & 108973.43 \\ 
  29 & MLE.b & Measure & beta=3 & sigma=3 & n=100 & 108973.89 \\ 
  30 & LME & Measure & beta=3 & sigma=3 & n=100 & 46.40 \\ 
  31 & MDE.Phi.chisq & Measure & beta=3 & sigma=3 & n=100 & 2039.61 \\ 
  32 & MDE.Phi.tv & Measure & beta=3 & sigma=3 & n=100 & 2418.80 \\ 
  33 & MDE.Phi.kl & Measure & beta=3 & sigma=3 & n=100 & 256.10 \\ 
  34 & MME & Measure & beta=3 & sigma=3 & n=100 & 720485.20 \\ 
  35 & MME.b & Measure & beta=3 & sigma=3 & n=100 & 6855117.81 \\ 
  36 & PWM & Measure & beta=3 & sigma=3 & n=100 & 46.40 \\ 
  37 & MLE & Measure & beta=4 & sigma=3 & n=100 & 137435.35 \\ 
  38 & MLE.b & Measure & beta=4 & sigma=3 & n=100 & 137437.01 \\ 
  39 & LME & Measure & beta=4 & sigma=3 & n=100 & 92.94 \\ 
  40 & MDE.Phi.chisq & Measure & beta=4 & sigma=3 & n=100 & 3153.14 \\ 
  41 & MDE.Phi.tv & Measure & beta=4 & sigma=3 & n=100 & 3568.39 \\ 
  42 & MDE.Phi.kl & Measure & beta=4 & sigma=3 & n=100 & 374.97 \\ 
  43 & MME & Measure & beta=4 & sigma=3 & n=100 & 21436.57 \\ 
  44 & MME.b & Measure & beta=4 & sigma=3 & n=100 & 4358456.67 \\ 
  45 & PWM & Measure & beta=4 & sigma=3 & n=100 & 92.94 \\ 
  46 & MLE & Measure & beta=5 & sigma=3 & n=100 & 218584.56 \\ 
  47 & MLE.b & Measure & beta=5 & sigma=3 & n=100 & 218586.67 \\ 
  48 & LME & Measure & beta=5 & sigma=3 & n=100 & 139.25 \\ 
  49 & MDE.Phi.chisq & Measure & beta=5 & sigma=3 & n=100 & 3710.03 \\ 
  50 & MDE.Phi.tv & Measure & beta=5 & sigma=3 & n=100 & 3984.13 \\ 
  51 & MDE.Phi.kl & Measure & beta=5 & sigma=3 & n=100 & 515.19 \\ 
  52 & MME & Measure & beta=5 & sigma=3 & n=100 & 28119.21 \\ 
  53 & MME.b & Measure & beta=5 & sigma=3 & n=100 & 399478.23 \\ 
  54 & PWM & Measure & beta=5 & sigma=3 & n=100 & 139.25 \\ 
  55 & MLE & Measure & beta=1.5 & sigma=3 & n=200 & 1.14 \\ 
  56 & MLE.b & Measure & beta=1.5 & sigma=3 & n=200 & 0.80 \\ 
  57 & LME & Measure & beta=1.5 & sigma=3 & n=200 & 1.64 \\ 
  58 & MDE.Phi.chisq & Measure & beta=1.5 & sigma=3 & n=200 & 85.18 \\ 
  59 & MDE.Phi.tv & Measure & beta=1.5 & sigma=3 & n=200 & 3.63 \\ 
  60 & MDE.Phi.kl & Measure & beta=1.5 & sigma=3 & n=200 & 1.14 \\ 
  61 & MME & Measure & beta=1.5 & sigma=3 & n=200 & 43.48 \\ 
  62 & MME.b & Measure & beta=1.5 & sigma=3 & n=200 & 35.88 \\ 
  63 & PWM & Measure & beta=1.5 & sigma=3 & n=200 & 1.64 \\ 
  64 & MLE & Measure & beta=2 & sigma=3 & n=200 & 1.72 \\ 
  65 & MLE.b & Measure & beta=2 & sigma=3 & n=200 & 1.04 \\ 
  66 & LME & Measure & beta=2 & sigma=3 & n=200 & 1.88 \\ 
  67 & MDE.Phi.chisq & Measure & beta=2 & sigma=3 & n=200 & 19.87 \\ 
  68 & MDE.Phi.tv & Measure & beta=2 & sigma=3 & n=200 & 21.68 \\ 
  69 & MDE.Phi.kl & Measure & beta=2 & sigma=3 & n=200 & 1.72 \\ 
  70 & MME & Measure & beta=2 & sigma=3 & n=200 & 11.08 \\ 
  71 & MME.b & Measure & beta=2 & sigma=3 & n=200 & 32.58 \\ 
  72 & PWM & Measure & beta=2 & sigma=3 & n=200 & 1.88 \\ 
  73 & MLE & Measure & beta=2.5 & sigma=3 & n=200 & 4.33 \\ 
  74 & MLE.b & Measure & beta=2.5 & sigma=3 & n=200 & 3.07 \\ 
  75 & LME & Measure & beta=2.5 & sigma=3 & n=200 & 4.53 \\ 
  76 & MDE.Phi.chisq & Measure & beta=2.5 & sigma=3 & n=200 & 89.92 \\ 
  77 & MDE.Phi.tv & Measure & beta=2.5 & sigma=3 & n=200 & 68.50 \\ 
  78 & MDE.Phi.kl & Measure & beta=2.5 & sigma=3 & n=200 & 4.33 \\ 
  79 & MME & Measure & beta=2.5 & sigma=3 & n=200 & 11.55 \\ 
  80 & MME.b & Measure & beta=2.5 & sigma=3 & n=200 & 157.58 \\ 
  81 & PWM & Measure & beta=2.5 & sigma=3 & n=200 & 4.53 \\ 
  82 & MLE & Measure & beta=3 & sigma=3 & n=200 & 157.99 \\ 
  83 & MLE.b & Measure & beta=3 & sigma=3 & n=200 & 156.47 \\ 
  84 & LME & Measure & beta=3 & sigma=3 & n=200 & 11.37 \\ 
  85 & MDE.Phi.chisq & Measure & beta=3 & sigma=3 & n=200 & 318.56 \\ 
  86 & MDE.Phi.tv & Measure & beta=3 & sigma=3 & n=200 & 147.13 \\ 
  87 & MDE.Phi.kl & Measure & beta=3 & sigma=3 & n=200 & 20.11 \\ 
  88 & MME & Measure & beta=3 & sigma=3 & n=200 & 185.51 \\ 
  89 & MME.b & Measure & beta=3 & sigma=3 & n=200 & 22498.94 \\ 
  90 & PWM & Measure & beta=3 & sigma=3 & n=200 & 11.37 \\ 
  91 & MLE & Measure & beta=4 & sigma=3 & n=200 & 664.49 \\ 
  92 & MLE.b & Measure & beta=4 & sigma=3 & n=200 & 664.14 \\ 
  93 & LME & Measure & beta=4 & sigma=3 & n=200 & 33.72 \\ 
  94 & MDE.Phi.chisq & Measure & beta=4 & sigma=3 & n=200 & 1049.56 \\ 
  95 & MDE.Phi.tv & Measure & beta=4 & sigma=3 & n=200 & 773.28 \\ 
  96 & MDE.Phi.kl & Measure & beta=4 & sigma=3 & n=200 & 74.39 \\ 
  97 & MME & Measure & beta=4 & sigma=3 & n=200 & 1031.75 \\ 
  98 & MME.b & Measure & beta=4 & sigma=3 & n=200 & 84864.92 \\ 
  99 & PWM & Measure & beta=4 & sigma=3 & n=200 & 33.72 \\ 
  100 & MLE & Measure & beta=5 & sigma=3 & n=200 & 61336.79 \\ 
  101 & MLE.b & Measure & beta=5 & sigma=3 & n=200 & 61338.05 \\ 
  102 & LME & Measure & beta=5 & sigma=3 & n=200 & 96.16 \\ 
  103 & MDE.Phi.chisq & Measure & beta=5 & sigma=3 & n=200 & 2003.69 \\ 
  104 & MDE.Phi.tv & Measure & beta=5 & sigma=3 & n=200 & 1297.33 \\ 
  105 & MDE.Phi.kl & Measure & beta=5 & sigma=3 & n=200 & 195.95 \\ 
  106 & MME & Measure & beta=5 & sigma=3 & n=200 & 4089.96 \\ 
  107 & MME.b & Measure & beta=5 & sigma=3 & n=200 & 46765.26 \\ 
  108 & PWM & Measure & beta=5 & sigma=3 & n=200 & 96.16 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220209/Output.accuracy2.LaTeX.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Wed Feb 09 03:24:10 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & Measure & beta=1.5 & sigma=3 & n=100 & 0.00 \\ 
  2 & MLE.b & Measure & beta=1.5 & sigma=3 & n=100 & 0.00 \\ 
  3 & LME & Measure & beta=1.5 & sigma=3 & n=100 & 0.00 \\ 
  4 & MDE.Phi.chisq & Measure & beta=1.5 & sigma=3 & n=100 & 29905720362168969996808464202462800682084228428422286624866604884622022480262860460682862862686226040624222482222048606602484402222646462462484864666660068682042200040840686000648880046024888628684680884420400648460404606406286026460640028240266822446048208046826248202606046862408260486282006042842840.00 \\ 
  5 & MDE.Phi.tv & Measure & beta=1.5 & sigma=3 & n=100 & 0.05 \\ 
  6 & MDE.Phi.kl & Measure & beta=1.5 & sigma=3 & n=100 & 0.00 \\ 
  7 & MME & Measure & beta=1.5 & sigma=3 & n=100 & 0.01 \\ 
  8 & MME.b & Measure & beta=1.5 & sigma=3 & n=100 & 7.11 \\ 
  9 & PWM & Measure & beta=1.5 & sigma=3 & n=100 & 0.00 \\ 
  10 & MLE & Measure & beta=2 & sigma=3 & n=100 & 0.00 \\ 
  11 & MLE.b & Measure & beta=2 & sigma=3 & n=100 & 0.00 \\ 
  12 & LME & Measure & beta=2 & sigma=3 & n=100 & 0.00 \\ 
  13 & MDE.Phi.chisq & Measure & beta=2 & sigma=3 & n=100 & 200401541349741565044622684624444464828280006842260482802402460840480462420442408484064028888884208868082024240488464422404022004826686464640022442426206826664828668088026884008426280242408868226824242822022244844842404026644404868866080088628264048220088826862228624862888066442022220866444444086022.00 \\ 
  14 & MDE.Phi.tv & Measure & beta=2 & sigma=3 & n=100 & 0.02 \\ 
  15 & MDE.Phi.kl & Measure & beta=2 & sigma=3 & n=100 & 0.00 \\ 
  16 & MME & Measure & beta=2 & sigma=3 & n=100 & 0.00 \\ 
  17 & MME.b & Measure & beta=2 & sigma=3 & n=100 & 0.01 \\ 
  18 & PWM & Measure & beta=2 & sigma=3 & n=100 & 0.00 \\ 
  19 & MLE & Measure & beta=2.5 & sigma=3 & n=100 & 0.00 \\ 
  20 & MLE.b & Measure & beta=2.5 & sigma=3 & n=100 & 0.00 \\ 
  21 & LME & Measure & beta=2.5 & sigma=3 & n=100 & 0.00 \\ 
  22 & MDE.Phi.chisq & Measure & beta=2.5 & sigma=3 & n=100 & 0.02 \\ 
  23 & MDE.Phi.tv & Measure & beta=2.5 & sigma=3 & n=100 & 0.02 \\ 
  24 & MDE.Phi.kl & Measure & beta=2.5 & sigma=3 & n=100 & 0.00 \\ 
  25 & MME & Measure & beta=2.5 & sigma=3 & n=100 & 0.00 \\ 
  26 & MME.b & Measure & beta=2.5 & sigma=3 & n=100 & 8.08 \\ 
  27 & PWM & Measure & beta=2.5 & sigma=3 & n=100 & 0.00 \\ 
  28 & MLE & Measure & beta=3 & sigma=3 & n=100 & 0.00 \\ 
  29 & MLE.b & Measure & beta=3 & sigma=3 & n=100 & 0.00 \\ 
  30 & LME & Measure & beta=3 & sigma=3 & n=100 & 0.00 \\ 
  31 & MDE.Phi.chisq & Measure & beta=3 & sigma=3 & n=100 & 0.02 \\ 
  32 & MDE.Phi.tv & Measure & beta=3 & sigma=3 & n=100 & 0.02 \\ 
  33 & MDE.Phi.kl & Measure & beta=3 & sigma=3 & n=100 & 0.00 \\ 
  34 & MME & Measure & beta=3 & sigma=3 & n=100 & 0.00 \\ 
  35 & MME.b & Measure & beta=3 & sigma=3 & n=100 & 0.01 \\ 
  36 & PWM & Measure & beta=3 & sigma=3 & n=100 & 0.00 \\ 
  37 & MLE & Measure & beta=4 & sigma=3 & n=100 & 0.00 \\ 
  38 & MLE.b & Measure & beta=4 & sigma=3 & n=100 & 0.00 \\ 
  39 & LME & Measure & beta=4 & sigma=3 & n=100 & 0.00 \\ 
  40 & MDE.Phi.chisq & Measure & beta=4 & sigma=3 & n=100 & 0.02 \\ 
  41 & MDE.Phi.tv & Measure & beta=4 & sigma=3 & n=100 & 0.01 \\ 
  42 & MDE.Phi.kl & Measure & beta=4 & sigma=3 & n=100 & 0.00 \\ 
  43 & MME & Measure & beta=4 & sigma=3 & n=100 & 0.00 \\ 
  44 & MME.b & Measure & beta=4 & sigma=3 & n=100 & 4041.95 \\ 
  45 & PWM & Measure & beta=4 & sigma=3 & n=100 & 0.00 \\ 
  46 & MLE & Measure & beta=5 & sigma=3 & n=100 & 0.00 \\ 
  47 & MLE.b & Measure & beta=5 & sigma=3 & n=100 & 0.00 \\ 
  48 & LME & Measure & beta=5 & sigma=3 & n=100 & 0.00 \\ 
  49 & MDE.Phi.chisq & Measure & beta=5 & sigma=3 & n=100 & 0.01 \\ 
  50 & MDE.Phi.tv & Measure & beta=5 & sigma=3 & n=100 & 0.01 \\ 
  51 & MDE.Phi.kl & Measure & beta=5 & sigma=3 & n=100 & 0.00 \\ 
  52 & MME & Measure & beta=5 & sigma=3 & n=100 & 0.00 \\ 
  53 & MME.b & Measure & beta=5 & sigma=3 & n=100 & 515620813105830396128066264404.00 \\ 
  54 & PWM & Measure & beta=5 & sigma=3 & n=100 & 0.00 \\ 
  55 & MLE & Measure & beta=1.5 & sigma=3 & n=200 & 0.00 \\ 
  56 & MLE.b & Measure & beta=1.5 & sigma=3 & n=200 & 0.00 \\ 
  57 & LME & Measure & beta=1.5 & sigma=3 & n=200 & 0.00 \\ 
  58 & MDE.Phi.chisq & Measure & beta=1.5 & sigma=3 & n=200 & 9837907289457943076080860424686002862804084088868622806442288428220800848484046804640642828004806408848424602226224084064024022806886482060404828246848420044624888240228486882868422448202288484888486048048064060080266048086240822008882402206646624846664426442640206820402646048266080424848440048866046.00 \\ 
  59 & MDE.Phi.tv & Measure & beta=1.5 & sigma=3 & n=200 & 0.03 \\ 
  60 & MDE.Phi.kl & Measure & beta=1.5 & sigma=3 & n=200 & 0.00 \\ 
  61 & MME & Measure & beta=1.5 & sigma=3 & n=200 & 0.01 \\ 
  62 & MME.b & Measure & beta=1.5 & sigma=3 & n=200 & 0.01 \\ 
  63 & PWM & Measure & beta=1.5 & sigma=3 & n=200 & 0.00 \\ 
  64 & MLE & Measure & beta=2 & sigma=3 & n=200 & 0.00 \\ 
  65 & MLE.b & Measure & beta=2 & sigma=3 & n=200 & 0.00 \\ 
  66 & LME & Measure & beta=2 & sigma=3 & n=200 & 0.00 \\ 
  67 & MDE.Phi.chisq & Measure & beta=2 & sigma=3 & n=200 & 32276043278331587168486406646400660846806662666882604688464600480080426200002426084864284604086888482064664462866022264662644460466200220466224048842804640228082260680666222026220280482886440280228488686208846202006202806206086068882000024880682008846244444802282084408880600888628866268624424440842.00 \\ 
  68 & MDE.Phi.tv & Measure & beta=2 & sigma=3 & n=200 & 0.02 \\ 
  69 & MDE.Phi.kl & Measure & beta=2 & sigma=3 & n=200 & 0.00 \\ 
  70 & MME & Measure & beta=2 & sigma=3 & n=200 & 0.00 \\ 
  71 & MME.b & Measure & beta=2 & sigma=3 & n=200 & 0.00 \\ 
  72 & PWM & Measure & beta=2 & sigma=3 & n=200 & 0.00 \\ 
  73 & MLE & Measure & beta=2.5 & sigma=3 & n=200 & 0.00 \\ 
  74 & MLE.b & Measure & beta=2.5 & sigma=3 & n=200 & 0.00 \\ 
  75 & LME & Measure & beta=2.5 & sigma=3 & n=200 & 0.00 \\ 
  76 & MDE.Phi.chisq & Measure & beta=2.5 & sigma=3 & n=200 & 0.02 \\ 
  77 & MDE.Phi.tv & Measure & beta=2.5 & sigma=3 & n=200 & 0.01 \\ 
  78 & MDE.Phi.kl & Measure & beta=2.5 & sigma=3 & n=200 & 0.00 \\ 
  79 & MME & Measure & beta=2.5 & sigma=3 & n=200 & 0.00 \\ 
  80 & MME.b & Measure & beta=2.5 & sigma=3 & n=200 & 0.00 \\ 
  81 & PWM & Measure & beta=2.5 & sigma=3 & n=200 & 0.00 \\ 
  82 & MLE & Measure & beta=3 & sigma=3 & n=200 & 0.00 \\ 
  83 & MLE.b & Measure & beta=3 & sigma=3 & n=200 & 0.00 \\ 
  84 & LME & Measure & beta=3 & sigma=3 & n=200 & 0.00 \\ 
  85 & MDE.Phi.chisq & Measure & beta=3 & sigma=3 & n=200 & 0.01 \\ 
  86 & MDE.Phi.tv & Measure & beta=3 & sigma=3 & n=200 & 0.01 \\ 
  87 & MDE.Phi.kl & Measure & beta=3 & sigma=3 & n=200 & 0.00 \\ 
  88 & MME & Measure & beta=3 & sigma=3 & n=200 & 0.00 \\ 
  89 & MME.b & Measure & beta=3 & sigma=3 & n=200 & 0.00 \\ 
  90 & PWM & Measure & beta=3 & sigma=3 & n=200 & 0.00 \\ 
  91 & MLE & Measure & beta=4 & sigma=3 & n=200 & 0.00 \\ 
  92 & MLE.b & Measure & beta=4 & sigma=3 & n=200 & 0.00 \\ 
  93 & LME & Measure & beta=4 & sigma=3 & n=200 & 0.00 \\ 
  94 & MDE.Phi.chisq & Measure & beta=4 & sigma=3 & n=200 & 0.01 \\ 
  95 & MDE.Phi.tv & Measure & beta=4 & sigma=3 & n=200 & 0.01 \\ 
  96 & MDE.Phi.kl & Measure & beta=4 & sigma=3 & n=200 & 0.00 \\ 
  97 & MME & Measure & beta=4 & sigma=3 & n=200 & 0.00 \\ 
  98 & MME.b & Measure & beta=4 & sigma=3 & n=200 & 0.00 \\ 
  99 & PWM & Measure & beta=4 & sigma=3 & n=200 & 0.00 \\ 
  100 & MLE & Measure & beta=5 & sigma=3 & n=200 & 0.00 \\ 
  101 & MLE.b & Measure & beta=5 & sigma=3 & n=200 & 0.00 \\ 
  102 & LME & Measure & beta=5 & sigma=3 & n=200 & 0.00 \\ 
  103 & MDE.Phi.chisq & Measure & beta=5 & sigma=3 & n=200 & 0.01 \\ 
  104 & MDE.Phi.tv & Measure & beta=5 & sigma=3 & n=200 & 0.01 \\ 
  105 & MDE.Phi.kl & Measure & beta=5 & sigma=3 & n=200 & 0.00 \\ 
  106 & MME & Measure & beta=5 & sigma=3 & n=200 & 0.00 \\ 
  107 & MME.b & Measure & beta=5 & sigma=3 & n=200 & 2.02 \\ 
  108 & PWM & Measure & beta=5 & sigma=3 & n=200 & 0.00 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220209/Output.bias.LaTeX.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Wed Feb 09 03:24:10 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=3 & n=100 & 0.17 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=3 & n=100 & -0.02 \\ 
  3 & LME & beta & beta=1.5 & sigma=3 & n=100 & 0.33 \\ 
  4 & MDE.Phi.chisq & beta & beta=1.5 & sigma=3 & n=100 & -3.37 \\ 
  5 & MDE.Phi.tv & beta & beta=1.5 & sigma=3 & n=100 & -0.27 \\ 
  6 & MDE.Phi.kl & beta & beta=1.5 & sigma=3 & n=100 & 0.17 \\ 
  7 & MME & beta & beta=1.5 & sigma=3 & n=100 & 1.29 \\ 
  8 & MME.b & beta & beta=1.5 & sigma=3 & n=100 & 4.81 \\ 
  9 & PWM & beta & beta=1.5 & sigma=3 & n=100 & 0.33 \\ 
  10 & MLE & sigma & beta=1.5 & sigma=3 & n=100 & 0.55 \\ 
  11 & MLE.b & sigma & beta=1.5 & sigma=3 & n=100 & -0.07 \\ 
  12 & LME & sigma & beta=1.5 & sigma=3 & n=100 & 0.98 \\ 
  13 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=3 & n=100 & 2.22 \\ 
  14 & MDE.Phi.tv & sigma & beta=1.5 & sigma=3 & n=100 & 2.49 \\ 
  15 & MDE.Phi.kl & sigma & beta=1.5 & sigma=3 & n=100 & 0.55 \\ 
  16 & MME & sigma & beta=1.5 & sigma=3 & n=100 & 6.46 \\ 
  17 & MME.b & sigma & beta=1.5 & sigma=3 & n=100 & 17.50 \\ 
  18 & PWM & sigma & beta=1.5 & sigma=3 & n=100 & 0.98 \\ 
  19 & MLE & beta & beta=2 & sigma=3 & n=100 & 0.99 \\ 
  20 & MLE.b & beta & beta=2 & sigma=3 & n=100 & 0.64 \\ 
  21 & LME & beta & beta=2 & sigma=3 & n=100 & 0.45 \\ 
  22 & MDE.Phi.chisq & beta & beta=2 & sigma=3 & n=100 & 0.01 \\ 
  23 & MDE.Phi.tv & beta & beta=2 & sigma=3 & n=100 & 0.66 \\ 
  24 & MDE.Phi.kl & beta & beta=2 & sigma=3 & n=100 & 0.45 \\ 
  25 & MME & beta & beta=2 & sigma=3 & n=100 & 1.68 \\ 
  26 & MME.b & beta & beta=2 & sigma=3 & n=100 & 7.48 \\ 
  27 & PWM & beta & beta=2 & sigma=3 & n=100 & 0.45 \\ 
  28 & MLE & sigma & beta=2 & sigma=3 & n=100 & 1.89 \\ 
  29 & MLE.b & sigma & beta=2 & sigma=3 & n=100 & 1.13 \\ 
  30 & LME & sigma & beta=2 & sigma=3 & n=100 & 0.90 \\ 
  31 & MDE.Phi.chisq & sigma & beta=2 & sigma=3 & n=100 & 3.23 \\ 
  32 & MDE.Phi.tv & sigma & beta=2 & sigma=3 & n=100 & 4.71 \\ 
  33 & MDE.Phi.kl & sigma & beta=2 & sigma=3 & n=100 & 0.96 \\ 
  34 & MME & sigma & beta=2 & sigma=3 & n=100 & 4.31 \\ 
  35 & MME.b & sigma & beta=2 & sigma=3 & n=100 & 16.76 \\ 
  36 & PWM & sigma & beta=2 & sigma=3 & n=100 & 0.90 \\ 
  37 & MLE & beta & beta=2.5 & sigma=3 & n=100 & 2.03 \\ 
  38 & MLE.b & beta & beta=2.5 & sigma=3 & n=100 & 1.57 \\ 
  39 & LME & beta & beta=2.5 & sigma=3 & n=100 & 0.70 \\ 
  40 & MDE.Phi.chisq & beta & beta=2.5 & sigma=3 & n=100 & 1.52 \\ 
  41 & MDE.Phi.tv & beta & beta=2.5 & sigma=3 & n=100 & 2.33 \\ 
  42 & MDE.Phi.kl & beta & beta=2.5 & sigma=3 & n=100 & 0.93 \\ 
  43 & MME & beta & beta=2.5 & sigma=3 & n=100 & 2.32 \\ 
  44 & MME.b & beta & beta=2.5 & sigma=3 & n=100 & 5.49 \\ 
  45 & PWM & beta & beta=2.5 & sigma=3 & n=100 & 0.70 \\ 
  46 & MLE & sigma & beta=2.5 & sigma=3 & n=100 & 3.28 \\ 
  47 & MLE.b & sigma & beta=2.5 & sigma=3 & n=100 & 2.53 \\ 
  48 & LME & sigma & beta=2.5 & sigma=3 & n=100 & 1.08 \\ 
  49 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=3 & n=100 & 6.02 \\ 
  50 & MDE.Phi.tv & sigma & beta=2.5 & sigma=3 & n=100 & 7.57 \\ 
  51 & MDE.Phi.kl & sigma & beta=2.5 & sigma=3 & n=100 & 1.50 \\ 
  52 & MME & sigma & beta=2.5 & sigma=3 & n=100 & 4.06 \\ 
  53 & MME.b & sigma & beta=2.5 & sigma=3 & n=100 & 9.06 \\ 
  54 & PWM & sigma & beta=2.5 & sigma=3 & n=100 & 1.08 \\ 
  55 & MLE & beta & beta=3 & sigma=3 & n=100 & 8.54 \\ 
  56 & MLE.b & beta & beta=3 & sigma=3 & n=100 & 8.05 \\ 
  57 & LME & beta & beta=3 & sigma=3 & n=100 & 1.02 \\ 
  58 & MDE.Phi.chisq & beta & beta=3 & sigma=3 & n=100 & 3.62 \\ 
  59 & MDE.Phi.tv & beta & beta=3 & sigma=3 & n=100 & 4.96 \\ 
  60 & MDE.Phi.kl & beta & beta=3 & sigma=3 & n=100 & 1.83 \\ 
  61 & MME & beta & beta=3 & sigma=3 & n=100 & 14.49 \\ 
  62 & MME.b & beta & beta=3 & sigma=3 & n=100 & 46.99 \\ 
  63 & PWM & beta & beta=3 & sigma=3 & n=100 & 1.02 \\ 
  64 & MLE & sigma & beta=3 & sigma=3 & n=100 & 11.08 \\ 
  65 & MLE.b & sigma & beta=3 & sigma=3 & n=100 & 10.44 \\ 
  66 & LME & sigma & beta=3 & sigma=3 & n=100 & 1.28 \\ 
  67 & MDE.Phi.chisq & sigma & beta=3 & sigma=3 & n=100 & 8.99 \\ 
  68 & MDE.Phi.tv & sigma & beta=3 & sigma=3 & n=100 & 11.05 \\ 
  69 & MDE.Phi.kl & sigma & beta=3 & sigma=3 & n=100 & 2.36 \\ 
  70 & MME & sigma & beta=3 & sigma=3 & n=100 & 17.23 \\ 
  71 & MME.b & sigma & beta=3 & sigma=3 & n=100 & 55.71 \\ 
  72 & PWM & sigma & beta=3 & sigma=3 & n=100 & 1.28 \\ 
  73 & MLE & beta & beta=4 & sigma=3 & n=100 & 13.36 \\ 
  74 & MLE.b & beta & beta=4 & sigma=3 & n=100 & 12.91 \\ 
  75 & LME & beta & beta=4 & sigma=3 & n=100 & 1.74 \\ 
  76 & MDE.Phi.chisq & beta & beta=4 & sigma=3 & n=100 & 9.17 \\ 
  77 & MDE.Phi.tv & beta & beta=4 & sigma=3 & n=100 & 11.26 \\ 
  78 & MDE.Phi.kl & beta & beta=4 & sigma=3 & n=100 & 3.37 \\ 
  79 & MME & beta & beta=4 & sigma=3 & n=100 & 7.35 \\ 
  80 & MME.b & beta & beta=4 & sigma=3 & n=100 & 36.91 \\ 
  81 & PWM & beta & beta=4 & sigma=3 & n=100 & 1.74 \\ 
  82 & MLE & sigma & beta=4 & sigma=3 & n=100 & 12.18 \\ 
  83 & MLE.b & sigma & beta=4 & sigma=3 & n=100 & 11.77 \\ 
  84 & LME & sigma & beta=4 & sigma=3 & n=100 & 1.59 \\ 
  85 & MDE.Phi.chisq & sigma & beta=4 & sigma=3 & n=100 & 13.97 \\ 
  86 & MDE.Phi.tv & sigma & beta=4 & sigma=3 & n=100 & 16.02 \\ 
  87 & MDE.Phi.kl & sigma & beta=4 & sigma=3 & n=100 & 3.14 \\ 
  88 & MME & sigma & beta=4 & sigma=3 & n=100 & 7.00 \\ 
  89 & MME.b & sigma & beta=4 & sigma=3 & n=100 & 37.30 \\ 
  90 & PWM & sigma & beta=4 & sigma=3 & n=100 & 1.59 \\ 
  91 & MLE & beta & beta=5 & sigma=3 & n=100 & 23.37 \\ 
  92 & MLE.b & beta & beta=5 & sigma=3 & n=100 & 23.00 \\ 
  93 & LME & beta & beta=5 & sigma=3 & n=100 & 2.30 \\ 
  94 & MDE.Phi.chisq & beta & beta=5 & sigma=3 & n=100 & 14.14 \\ 
  95 & MDE.Phi.tv & beta & beta=5 & sigma=3 & n=100 & 16.20 \\ 
  96 & MDE.Phi.kl & beta & beta=5 & sigma=3 & n=100 & 4.95 \\ 
  97 & MME & beta & beta=5 & sigma=3 & n=100 & 11.71 \\ 
  98 & MME.b & beta & beta=5 & sigma=3 & n=100 & 42.12 \\ 
  99 & PWM & beta & beta=5 & sigma=3 & n=100 & 2.30 \\ 
  100 & MLE & sigma & beta=5 & sigma=3 & n=100 & 16.59 \\ 
  101 & MLE.b & sigma & beta=5 & sigma=3 & n=100 & 16.33 \\ 
  102 & LME & sigma & beta=5 & sigma=3 & n=100 & 1.61 \\ 
  103 & MDE.Phi.chisq & sigma & beta=5 & sigma=3 & n=100 & 15.83 \\ 
  104 & MDE.Phi.tv & sigma & beta=5 & sigma=3 & n=100 & 17.22 \\ 
  105 & MDE.Phi.kl & sigma & beta=5 & sigma=3 & n=100 & 3.50 \\ 
  106 & MME & sigma & beta=5 & sigma=3 & n=100 & 8.23 \\ 
  107 & MME.b & sigma & beta=5 & sigma=3 & n=100 & 29.87 \\ 
  108 & PWM & sigma & beta=5 & sigma=3 & n=100 & 1.61 \\ 
  109 & MLE & beta & beta=1.5 & sigma=3 & n=200 & 0.08 \\ 
  110 & MLE.b & beta & beta=1.5 & sigma=3 & n=200 & -0.00 \\ 
  111 & LME & beta & beta=1.5 & sigma=3 & n=200 & 0.21 \\ 
  112 & MDE.Phi.chisq & beta & beta=1.5 & sigma=3 & n=200 & -1.32 \\ 
  113 & MDE.Phi.tv & beta & beta=1.5 & sigma=3 & n=200 & -0.50 \\ 
  114 & MDE.Phi.kl & beta & beta=1.5 & sigma=3 & n=200 & 0.08 \\ 
  115 & MME & beta & beta=1.5 & sigma=3 & n=200 & 1.00 \\ 
  116 & MME.b & beta & beta=1.5 & sigma=3 & n=200 & 0.80 \\ 
  117 & PWM & beta & beta=1.5 & sigma=3 & n=200 & 0.21 \\ 
  118 & MLE & sigma & beta=1.5 & sigma=3 & n=200 & 0.25 \\ 
  119 & MLE.b & sigma & beta=1.5 & sigma=3 & n=200 & -0.01 \\ 
  120 & LME & sigma & beta=1.5 & sigma=3 & n=200 & 0.61 \\ 
  121 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=3 & n=200 & 0.65 \\ 
  122 & MDE.Phi.tv & sigma & beta=1.5 & sigma=3 & n=200 & 0.78 \\ 
  123 & MDE.Phi.kl & sigma & beta=1.5 & sigma=3 & n=200 & 0.25 \\ 
  124 & MME & sigma & beta=1.5 & sigma=3 & n=200 & 5.36 \\ 
  125 & MME.b & sigma & beta=1.5 & sigma=3 & n=200 & 4.53 \\ 
  126 & PWM & sigma & beta=1.5 & sigma=3 & n=200 & 0.61 \\ 
  127 & MLE & beta & beta=2 & sigma=3 & n=200 & 0.14 \\ 
  128 & MLE.b & beta & beta=2 & sigma=3 & n=200 & -0.03 \\ 
  129 & LME & beta & beta=2 & sigma=3 & n=200 & 0.22 \\ 
  130 & MDE.Phi.chisq & beta & beta=2 & sigma=3 & n=200 & -0.68 \\ 
  131 & MDE.Phi.tv & beta & beta=2 & sigma=3 & n=200 & -0.44 \\ 
  132 & MDE.Phi.kl & beta & beta=2 & sigma=3 & n=200 & 0.14 \\ 
  133 & MME & beta & beta=2 & sigma=3 & n=200 & 0.97 \\ 
  134 & MME.b & beta & beta=2 & sigma=3 & n=200 & 0.69 \\ 
  135 & PWM & beta & beta=2 & sigma=3 & n=200 & 0.22 \\ 
  136 & MLE & sigma & beta=2 & sigma=3 & n=200 & 0.29 \\ 
  137 & MLE.b & sigma & beta=2 & sigma=3 & n=200 & -0.07 \\ 
  138 & LME & sigma & beta=2 & sigma=3 & n=200 & 0.43 \\ 
  139 & MDE.Phi.chisq & sigma & beta=2 & sigma=3 & n=200 & 0.52 \\ 
  140 & MDE.Phi.tv & sigma & beta=2 & sigma=3 & n=200 & 0.83 \\ 
  141 & MDE.Phi.kl & sigma & beta=2 & sigma=3 & n=200 & 0.29 \\ 
  142 & MME & sigma & beta=2 & sigma=3 & n=200 & 2.67 \\ 
  143 & MME.b & sigma & beta=2 & sigma=3 & n=200 & 1.94 \\ 
  144 & PWM & sigma & beta=2 & sigma=3 & n=200 & 0.43 \\ 
  145 & MLE & beta & beta=2.5 & sigma=3 & n=200 & 0.25 \\ 
  146 & MLE.b & beta & beta=2.5 & sigma=3 & n=200 & -0.05 \\ 
  147 & LME & beta & beta=2.5 & sigma=3 & n=200 & 0.28 \\ 
  148 & MDE.Phi.chisq & beta & beta=2.5 & sigma=3 & n=200 & -0.46 \\ 
  149 & MDE.Phi.tv & beta & beta=2.5 & sigma=3 & n=200 & -0.23 \\ 
  150 & MDE.Phi.kl & beta & beta=2.5 & sigma=3 & n=200 & 0.25 \\ 
  151 & MME & beta & beta=2.5 & sigma=3 & n=200 & 1.06 \\ 
  152 & MME.b & beta & beta=2.5 & sigma=3 & n=200 & 0.84 \\ 
  153 & PWM & beta & beta=2.5 & sigma=3 & n=200 & 0.28 \\ 
  154 & MLE & sigma & beta=2.5 & sigma=3 & n=200 & 0.41 \\ 
  155 & MLE.b & sigma & beta=2.5 & sigma=3 & n=200 & -0.09 \\ 
  156 & LME & sigma & beta=2.5 & sigma=3 & n=200 & 0.43 \\ 
  157 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=3 & n=200 & 1.04 \\ 
  158 & MDE.Phi.tv & sigma & beta=2.5 & sigma=3 & n=200 & 1.20 \\ 
  159 & MDE.Phi.kl & sigma & beta=2.5 & sigma=3 & n=200 & 0.41 \\ 
  160 & MME & sigma & beta=2.5 & sigma=3 & n=200 & 1.96 \\ 
  161 & MME.b & sigma & beta=2.5 & sigma=3 & n=200 & 1.52 \\ 
  162 & PWM & sigma & beta=2.5 & sigma=3 & n=200 & 0.43 \\ 
  163 & MLE & beta & beta=3 & sigma=3 & n=200 & 0.55 \\ 
  164 & MLE.b & beta & beta=3 & sigma=3 & n=200 & 0.09 \\ 
  165 & LME & beta & beta=3 & sigma=3 & n=200 & 0.45 \\ 
  166 & MDE.Phi.chisq & beta & beta=3 & sigma=3 & n=200 & 0.27 \\ 
  167 & MDE.Phi.tv & beta & beta=3 & sigma=3 & n=200 & 0.19 \\ 
  168 & MDE.Phi.kl & beta & beta=3 & sigma=3 & n=200 & 0.49 \\ 
  169 & MME & beta & beta=3 & sigma=3 & n=200 & 1.40 \\ 
  170 & MME.b & beta & beta=3 & sigma=3 & n=200 & 2.69 \\ 
  171 & PWM & beta & beta=3 & sigma=3 & n=200 & 0.45 \\ 
  172 & MLE & sigma & beta=3 & sigma=3 & n=200 & 0.71 \\ 
  173 & MLE.b & sigma & beta=3 & sigma=3 & n=200 & 0.11 \\ 
  174 & LME & sigma & beta=3 & sigma=3 & n=200 & 0.57 \\ 
  175 & MDE.Phi.chisq & sigma & beta=3 & sigma=3 & n=200 & 2.25 \\ 
  176 & MDE.Phi.tv & sigma & beta=3 & sigma=3 & n=200 & 1.76 \\ 
  177 & MDE.Phi.kl & sigma & beta=3 & sigma=3 & n=200 & 0.64 \\ 
  178 & MME & sigma & beta=3 & sigma=3 & n=200 & 1.94 \\ 
  179 & MME.b & sigma & beta=3 & sigma=3 & n=200 & 3.69 \\ 
  180 & PWM & sigma & beta=3 & sigma=3 & n=200 & 0.57 \\ 
  181 & MLE & beta & beta=4 & sigma=3 & n=200 & 1.54 \\ 
  182 & MLE.b & beta & beta=4 & sigma=3 & n=200 & 0.87 \\ 
  183 & LME & beta & beta=4 & sigma=3 & n=200 & 0.92 \\ 
  184 & MDE.Phi.chisq & beta & beta=4 & sigma=3 & n=200 & 3.48 \\ 
  185 & MDE.Phi.tv & beta & beta=4 & sigma=3 & n=200 & 2.80 \\ 
  186 & MDE.Phi.kl & beta & beta=4 & sigma=3 & n=200 & 1.25 \\ 
  187 & MME & beta & beta=4 & sigma=3 & n=200 & 2.64 \\ 
  188 & MME.b & beta & beta=4 & sigma=3 & n=200 & 9.69 \\ 
  189 & PWM & beta & beta=4 & sigma=3 & n=200 & 0.92 \\ 
  190 & MLE & sigma & beta=4 & sigma=3 & n=200 & 1.43 \\ 
  191 & MLE.b & sigma & beta=4 & sigma=3 & n=200 & 0.81 \\ 
  192 & LME & sigma & beta=4 & sigma=3 & n=200 & 0.83 \\ 
  193 & MDE.Phi.chisq & sigma & beta=4 & sigma=3 & n=200 & 5.73 \\ 
  194 & MDE.Phi.tv & sigma & beta=4 & sigma=3 & n=200 & 4.52 \\ 
  195 & MDE.Phi.kl & sigma & beta=4 & sigma=3 & n=200 & 1.15 \\ 
  196 & MME & sigma & beta=4 & sigma=3 & n=200 & 2.49 \\ 
  197 & MME.b & sigma & beta=4 & sigma=3 & n=200 & 9.38 \\ 
  198 & PWM & sigma & beta=4 & sigma=3 & n=200 & 0.83 \\ 
  199 & MLE & beta & beta=5 & sigma=3 & n=200 & 7.02 \\ 
  200 & MLE.b & beta & beta=5 & sigma=3 & n=200 & 6.32 \\ 
  201 & LME & beta & beta=5 & sigma=3 & n=200 & 1.77 \\ 
  202 & MDE.Phi.chisq & beta & beta=5 & sigma=3 & n=200 & 8.57 \\ 
  203 & MDE.Phi.tv & beta & beta=5 & sigma=3 & n=200 & 6.01 \\ 
  204 & MDE.Phi.kl & beta & beta=5 & sigma=3 & n=200 & 2.55 \\ 
  205 & MME & beta & beta=5 & sigma=3 & n=200 & 4.77 \\ 
  206 & MME.b & beta & beta=5 & sigma=3 & n=200 & 16.61 \\ 
  207 & PWM & beta & beta=5 & sigma=3 & n=200 & 1.77 \\ 
  208 & MLE & sigma & beta=5 & sigma=3 & n=200 & 4.94 \\ 
  209 & MLE.b & sigma & beta=5 & sigma=3 & n=200 & 4.44 \\ 
  210 & LME & sigma & beta=5 & sigma=3 & n=200 & 1.24 \\ 
  211 & MDE.Phi.chisq & sigma & beta=5 & sigma=3 & n=200 & 9.29 \\ 
  212 & MDE.Phi.tv & sigma & beta=5 & sigma=3 & n=200 & 6.45 \\ 
  213 & MDE.Phi.kl & sigma & beta=5 & sigma=3 & n=200 & 1.81 \\ 
  214 & MME & sigma & beta=5 & sigma=3 & n=200 & 3.40 \\ 
  215 & MME.b & sigma & beta=5 & sigma=3 & n=200 & 11.83 \\ 
  216 & PWM & sigma & beta=5 & sigma=3 & n=200 & 1.24 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220209/Output.mean.LaTeX.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Wed Feb 09 03:24:10 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=3 & n=100 & 1.67 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=3 & n=100 & 1.48 \\ 
  3 & LME & beta & beta=1.5 & sigma=3 & n=100 & 1.83 \\ 
  4 & MDE.Phi.chisq & beta & beta=1.5 & sigma=3 & n=100 & -1.87 \\ 
  5 & MDE.Phi.tv & beta & beta=1.5 & sigma=3 & n=100 & 1.23 \\ 
  6 & MDE.Phi.kl & beta & beta=1.5 & sigma=3 & n=100 & 1.67 \\ 
  7 & MME & beta & beta=1.5 & sigma=3 & n=100 & 2.79 \\ 
  8 & MME.b & beta & beta=1.5 & sigma=3 & n=100 & 6.31 \\ 
  9 & PWM & beta & beta=1.5 & sigma=3 & n=100 & 1.83 \\ 
  10 & MLE & sigma & beta=1.5 & sigma=3 & n=100 & 3.55 \\ 
  11 & MLE.b & sigma & beta=1.5 & sigma=3 & n=100 & 2.93 \\ 
  12 & LME & sigma & beta=1.5 & sigma=3 & n=100 & 3.98 \\ 
  13 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=3 & n=100 & 5.22 \\ 
  14 & MDE.Phi.tv & sigma & beta=1.5 & sigma=3 & n=100 & 5.49 \\ 
  15 & MDE.Phi.kl & sigma & beta=1.5 & sigma=3 & n=100 & 3.55 \\ 
  16 & MME & sigma & beta=1.5 & sigma=3 & n=100 & 9.46 \\ 
  17 & MME.b & sigma & beta=1.5 & sigma=3 & n=100 & 20.50 \\ 
  18 & PWM & sigma & beta=1.5 & sigma=3 & n=100 & 3.98 \\ 
  19 & MLE & beta & beta=2 & sigma=3 & n=100 & 2.99 \\ 
  20 & MLE.b & beta & beta=2 & sigma=3 & n=100 & 2.64 \\ 
  21 & LME & beta & beta=2 & sigma=3 & n=100 & 2.45 \\ 
  22 & MDE.Phi.chisq & beta & beta=2 & sigma=3 & n=100 & 2.01 \\ 
  23 & MDE.Phi.tv & beta & beta=2 & sigma=3 & n=100 & 2.66 \\ 
  24 & MDE.Phi.kl & beta & beta=2 & sigma=3 & n=100 & 2.45 \\ 
  25 & MME & beta & beta=2 & sigma=3 & n=100 & 3.68 \\ 
  26 & MME.b & beta & beta=2 & sigma=3 & n=100 & 9.48 \\ 
  27 & PWM & beta & beta=2 & sigma=3 & n=100 & 2.45 \\ 
  28 & MLE & sigma & beta=2 & sigma=3 & n=100 & 4.89 \\ 
  29 & MLE.b & sigma & beta=2 & sigma=3 & n=100 & 4.13 \\ 
  30 & LME & sigma & beta=2 & sigma=3 & n=100 & 3.90 \\ 
  31 & MDE.Phi.chisq & sigma & beta=2 & sigma=3 & n=100 & 6.23 \\ 
  32 & MDE.Phi.tv & sigma & beta=2 & sigma=3 & n=100 & 7.71 \\ 
  33 & MDE.Phi.kl & sigma & beta=2 & sigma=3 & n=100 & 3.96 \\ 
  34 & MME & sigma & beta=2 & sigma=3 & n=100 & 7.31 \\ 
  35 & MME.b & sigma & beta=2 & sigma=3 & n=100 & 19.76 \\ 
  36 & PWM & sigma & beta=2 & sigma=3 & n=100 & 3.90 \\ 
  37 & MLE & beta & beta=2.5 & sigma=3 & n=100 & 4.53 \\ 
  38 & MLE.b & beta & beta=2.5 & sigma=3 & n=100 & 4.07 \\ 
  39 & LME & beta & beta=2.5 & sigma=3 & n=100 & 3.20 \\ 
  40 & MDE.Phi.chisq & beta & beta=2.5 & sigma=3 & n=100 & 4.02 \\ 
  41 & MDE.Phi.tv & beta & beta=2.5 & sigma=3 & n=100 & 4.83 \\ 
  42 & MDE.Phi.kl & beta & beta=2.5 & sigma=3 & n=100 & 3.43 \\ 
  43 & MME & beta & beta=2.5 & sigma=3 & n=100 & 4.82 \\ 
  44 & MME.b & beta & beta=2.5 & sigma=3 & n=100 & 7.99 \\ 
  45 & PWM & beta & beta=2.5 & sigma=3 & n=100 & 3.20 \\ 
  46 & MLE & sigma & beta=2.5 & sigma=3 & n=100 & 6.28 \\ 
  47 & MLE.b & sigma & beta=2.5 & sigma=3 & n=100 & 5.53 \\ 
  48 & LME & sigma & beta=2.5 & sigma=3 & n=100 & 4.08 \\ 
  49 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=3 & n=100 & 9.02 \\ 
  50 & MDE.Phi.tv & sigma & beta=2.5 & sigma=3 & n=100 & 10.57 \\ 
  51 & MDE.Phi.kl & sigma & beta=2.5 & sigma=3 & n=100 & 4.50 \\ 
  52 & MME & sigma & beta=2.5 & sigma=3 & n=100 & 7.06 \\ 
  53 & MME.b & sigma & beta=2.5 & sigma=3 & n=100 & 12.06 \\ 
  54 & PWM & sigma & beta=2.5 & sigma=3 & n=100 & 4.08 \\ 
  55 & MLE & beta & beta=3 & sigma=3 & n=100 & 11.54 \\ 
  56 & MLE.b & beta & beta=3 & sigma=3 & n=100 & 11.05 \\ 
  57 & LME & beta & beta=3 & sigma=3 & n=100 & 4.02 \\ 
  58 & MDE.Phi.chisq & beta & beta=3 & sigma=3 & n=100 & 6.62 \\ 
  59 & MDE.Phi.tv & beta & beta=3 & sigma=3 & n=100 & 7.96 \\ 
  60 & MDE.Phi.kl & beta & beta=3 & sigma=3 & n=100 & 4.83 \\ 
  61 & MME & beta & beta=3 & sigma=3 & n=100 & 17.49 \\ 
  62 & MME.b & beta & beta=3 & sigma=3 & n=100 & 49.99 \\ 
  63 & PWM & beta & beta=3 & sigma=3 & n=100 & 4.02 \\ 
  64 & MLE & sigma & beta=3 & sigma=3 & n=100 & 14.08 \\ 
  65 & MLE.b & sigma & beta=3 & sigma=3 & n=100 & 13.44 \\ 
  66 & LME & sigma & beta=3 & sigma=3 & n=100 & 4.28 \\ 
  67 & MDE.Phi.chisq & sigma & beta=3 & sigma=3 & n=100 & 11.99 \\ 
  68 & MDE.Phi.tv & sigma & beta=3 & sigma=3 & n=100 & 14.05 \\ 
  69 & MDE.Phi.kl & sigma & beta=3 & sigma=3 & n=100 & 5.36 \\ 
  70 & MME & sigma & beta=3 & sigma=3 & n=100 & 20.23 \\ 
  71 & MME.b & sigma & beta=3 & sigma=3 & n=100 & 58.71 \\ 
  72 & PWM & sigma & beta=3 & sigma=3 & n=100 & 4.28 \\ 
  73 & MLE & beta & beta=4 & sigma=3 & n=100 & 17.36 \\ 
  74 & MLE.b & beta & beta=4 & sigma=3 & n=100 & 16.91 \\ 
  75 & LME & beta & beta=4 & sigma=3 & n=100 & 5.74 \\ 
  76 & MDE.Phi.chisq & beta & beta=4 & sigma=3 & n=100 & 13.17 \\ 
  77 & MDE.Phi.tv & beta & beta=4 & sigma=3 & n=100 & 15.26 \\ 
  78 & MDE.Phi.kl & beta & beta=4 & sigma=3 & n=100 & 7.37 \\ 
  79 & MME & beta & beta=4 & sigma=3 & n=100 & 11.35 \\ 
  80 & MME.b & beta & beta=4 & sigma=3 & n=100 & 40.91 \\ 
  81 & PWM & beta & beta=4 & sigma=3 & n=100 & 5.74 \\ 
  82 & MLE & sigma & beta=4 & sigma=3 & n=100 & 15.18 \\ 
  83 & MLE.b & sigma & beta=4 & sigma=3 & n=100 & 14.77 \\ 
  84 & LME & sigma & beta=4 & sigma=3 & n=100 & 4.59 \\ 
  85 & MDE.Phi.chisq & sigma & beta=4 & sigma=3 & n=100 & 16.97 \\ 
  86 & MDE.Phi.tv & sigma & beta=4 & sigma=3 & n=100 & 19.02 \\ 
  87 & MDE.Phi.kl & sigma & beta=4 & sigma=3 & n=100 & 6.14 \\ 
  88 & MME & sigma & beta=4 & sigma=3 & n=100 & 10.00 \\ 
  89 & MME.b & sigma & beta=4 & sigma=3 & n=100 & 40.30 \\ 
  90 & PWM & sigma & beta=4 & sigma=3 & n=100 & 4.59 \\ 
  91 & MLE & beta & beta=5 & sigma=3 & n=100 & 28.37 \\ 
  92 & MLE.b & beta & beta=5 & sigma=3 & n=100 & 28.00 \\ 
  93 & LME & beta & beta=5 & sigma=3 & n=100 & 7.30 \\ 
  94 & MDE.Phi.chisq & beta & beta=5 & sigma=3 & n=100 & 19.14 \\ 
  95 & MDE.Phi.tv & beta & beta=5 & sigma=3 & n=100 & 21.20 \\ 
  96 & MDE.Phi.kl & beta & beta=5 & sigma=3 & n=100 & 9.95 \\ 
  97 & MME & beta & beta=5 & sigma=3 & n=100 & 16.71 \\ 
  98 & MME.b & beta & beta=5 & sigma=3 & n=100 & 47.12 \\ 
  99 & PWM & beta & beta=5 & sigma=3 & n=100 & 7.30 \\ 
  100 & MLE & sigma & beta=5 & sigma=3 & n=100 & 19.59 \\ 
  101 & MLE.b & sigma & beta=5 & sigma=3 & n=100 & 19.33 \\ 
  102 & LME & sigma & beta=5 & sigma=3 & n=100 & 4.61 \\ 
  103 & MDE.Phi.chisq & sigma & beta=5 & sigma=3 & n=100 & 18.83 \\ 
  104 & MDE.Phi.tv & sigma & beta=5 & sigma=3 & n=100 & 20.22 \\ 
  105 & MDE.Phi.kl & sigma & beta=5 & sigma=3 & n=100 & 6.50 \\ 
  106 & MME & sigma & beta=5 & sigma=3 & n=100 & 11.23 \\ 
  107 & MME.b & sigma & beta=5 & sigma=3 & n=100 & 32.87 \\ 
  108 & PWM & sigma & beta=5 & sigma=3 & n=100 & 4.61 \\ 
  109 & MLE & beta & beta=1.5 & sigma=3 & n=200 & 1.58 \\ 
  110 & MLE.b & beta & beta=1.5 & sigma=3 & n=200 & 1.50 \\ 
  111 & LME & beta & beta=1.5 & sigma=3 & n=200 & 1.71 \\ 
  112 & MDE.Phi.chisq & beta & beta=1.5 & sigma=3 & n=200 & 0.18 \\ 
  113 & MDE.Phi.tv & beta & beta=1.5 & sigma=3 & n=200 & 1.00 \\ 
  114 & MDE.Phi.kl & beta & beta=1.5 & sigma=3 & n=200 & 1.58 \\ 
  115 & MME & beta & beta=1.5 & sigma=3 & n=200 & 2.50 \\ 
  116 & MME.b & beta & beta=1.5 & sigma=3 & n=200 & 2.30 \\ 
  117 & PWM & beta & beta=1.5 & sigma=3 & n=200 & 1.71 \\ 
  118 & MLE & sigma & beta=1.5 & sigma=3 & n=200 & 3.25 \\ 
  119 & MLE.b & sigma & beta=1.5 & sigma=3 & n=200 & 2.99 \\ 
  120 & LME & sigma & beta=1.5 & sigma=3 & n=200 & 3.61 \\ 
  121 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=3 & n=200 & 3.65 \\ 
  122 & MDE.Phi.tv & sigma & beta=1.5 & sigma=3 & n=200 & 3.78 \\ 
  123 & MDE.Phi.kl & sigma & beta=1.5 & sigma=3 & n=200 & 3.25 \\ 
  124 & MME & sigma & beta=1.5 & sigma=3 & n=200 & 8.36 \\ 
  125 & MME.b & sigma & beta=1.5 & sigma=3 & n=200 & 7.53 \\ 
  126 & PWM & sigma & beta=1.5 & sigma=3 & n=200 & 3.61 \\ 
  127 & MLE & beta & beta=2 & sigma=3 & n=200 & 2.14 \\ 
  128 & MLE.b & beta & beta=2 & sigma=3 & n=200 & 1.97 \\ 
  129 & LME & beta & beta=2 & sigma=3 & n=200 & 2.22 \\ 
  130 & MDE.Phi.chisq & beta & beta=2 & sigma=3 & n=200 & 1.32 \\ 
  131 & MDE.Phi.tv & beta & beta=2 & sigma=3 & n=200 & 1.56 \\ 
  132 & MDE.Phi.kl & beta & beta=2 & sigma=3 & n=200 & 2.14 \\ 
  133 & MME & beta & beta=2 & sigma=3 & n=200 & 2.97 \\ 
  134 & MME.b & beta & beta=2 & sigma=3 & n=200 & 2.69 \\ 
  135 & PWM & beta & beta=2 & sigma=3 & n=200 & 2.22 \\ 
  136 & MLE & sigma & beta=2 & sigma=3 & n=200 & 3.29 \\ 
  137 & MLE.b & sigma & beta=2 & sigma=3 & n=200 & 2.93 \\ 
  138 & LME & sigma & beta=2 & sigma=3 & n=200 & 3.43 \\ 
  139 & MDE.Phi.chisq & sigma & beta=2 & sigma=3 & n=200 & 3.52 \\ 
  140 & MDE.Phi.tv & sigma & beta=2 & sigma=3 & n=200 & 3.83 \\ 
  141 & MDE.Phi.kl & sigma & beta=2 & sigma=3 & n=200 & 3.29 \\ 
  142 & MME & sigma & beta=2 & sigma=3 & n=200 & 5.67 \\ 
  143 & MME.b & sigma & beta=2 & sigma=3 & n=200 & 4.94 \\ 
  144 & PWM & sigma & beta=2 & sigma=3 & n=200 & 3.43 \\ 
  145 & MLE & beta & beta=2.5 & sigma=3 & n=200 & 2.75 \\ 
  146 & MLE.b & beta & beta=2.5 & sigma=3 & n=200 & 2.45 \\ 
  147 & LME & beta & beta=2.5 & sigma=3 & n=200 & 2.78 \\ 
  148 & MDE.Phi.chisq & beta & beta=2.5 & sigma=3 & n=200 & 2.04 \\ 
  149 & MDE.Phi.tv & beta & beta=2.5 & sigma=3 & n=200 & 2.27 \\ 
  150 & MDE.Phi.kl & beta & beta=2.5 & sigma=3 & n=200 & 2.75 \\ 
  151 & MME & beta & beta=2.5 & sigma=3 & n=200 & 3.56 \\ 
  152 & MME.b & beta & beta=2.5 & sigma=3 & n=200 & 3.34 \\ 
  153 & PWM & beta & beta=2.5 & sigma=3 & n=200 & 2.78 \\ 
  154 & MLE & sigma & beta=2.5 & sigma=3 & n=200 & 3.41 \\ 
  155 & MLE.b & sigma & beta=2.5 & sigma=3 & n=200 & 2.91 \\ 
  156 & LME & sigma & beta=2.5 & sigma=3 & n=200 & 3.43 \\ 
  157 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=3 & n=200 & 4.04 \\ 
  158 & MDE.Phi.tv & sigma & beta=2.5 & sigma=3 & n=200 & 4.20 \\ 
  159 & MDE.Phi.kl & sigma & beta=2.5 & sigma=3 & n=200 & 3.41 \\ 
  160 & MME & sigma & beta=2.5 & sigma=3 & n=200 & 4.96 \\ 
  161 & MME.b & sigma & beta=2.5 & sigma=3 & n=200 & 4.52 \\ 
  162 & PWM & sigma & beta=2.5 & sigma=3 & n=200 & 3.43 \\ 
  163 & MLE & beta & beta=3 & sigma=3 & n=200 & 3.55 \\ 
  164 & MLE.b & beta & beta=3 & sigma=3 & n=200 & 3.09 \\ 
  165 & LME & beta & beta=3 & sigma=3 & n=200 & 3.45 \\ 
  166 & MDE.Phi.chisq & beta & beta=3 & sigma=3 & n=200 & 3.27 \\ 
  167 & MDE.Phi.tv & beta & beta=3 & sigma=3 & n=200 & 3.19 \\ 
  168 & MDE.Phi.kl & beta & beta=3 & sigma=3 & n=200 & 3.49 \\ 
  169 & MME & beta & beta=3 & sigma=3 & n=200 & 4.40 \\ 
  170 & MME.b & beta & beta=3 & sigma=3 & n=200 & 5.69 \\ 
  171 & PWM & beta & beta=3 & sigma=3 & n=200 & 3.45 \\ 
  172 & MLE & sigma & beta=3 & sigma=3 & n=200 & 3.71 \\ 
  173 & MLE.b & sigma & beta=3 & sigma=3 & n=200 & 3.11 \\ 
  174 & LME & sigma & beta=3 & sigma=3 & n=200 & 3.57 \\ 
  175 & MDE.Phi.chisq & sigma & beta=3 & sigma=3 & n=200 & 5.25 \\ 
  176 & MDE.Phi.tv & sigma & beta=3 & sigma=3 & n=200 & 4.76 \\ 
  177 & MDE.Phi.kl & sigma & beta=3 & sigma=3 & n=200 & 3.64 \\ 
  178 & MME & sigma & beta=3 & sigma=3 & n=200 & 4.94 \\ 
  179 & MME.b & sigma & beta=3 & sigma=3 & n=200 & 6.69 \\ 
  180 & PWM & sigma & beta=3 & sigma=3 & n=200 & 3.57 \\ 
  181 & MLE & beta & beta=4 & sigma=3 & n=200 & 5.54 \\ 
  182 & MLE.b & beta & beta=4 & sigma=3 & n=200 & 4.87 \\ 
  183 & LME & beta & beta=4 & sigma=3 & n=200 & 4.92 \\ 
  184 & MDE.Phi.chisq & beta & beta=4 & sigma=3 & n=200 & 7.48 \\ 
  185 & MDE.Phi.tv & beta & beta=4 & sigma=3 & n=200 & 6.80 \\ 
  186 & MDE.Phi.kl & beta & beta=4 & sigma=3 & n=200 & 5.25 \\ 
  187 & MME & beta & beta=4 & sigma=3 & n=200 & 6.64 \\ 
  188 & MME.b & beta & beta=4 & sigma=3 & n=200 & 13.69 \\ 
  189 & PWM & beta & beta=4 & sigma=3 & n=200 & 4.92 \\ 
  190 & MLE & sigma & beta=4 & sigma=3 & n=200 & 4.43 \\ 
  191 & MLE.b & sigma & beta=4 & sigma=3 & n=200 & 3.81 \\ 
  192 & LME & sigma & beta=4 & sigma=3 & n=200 & 3.83 \\ 
  193 & MDE.Phi.chisq & sigma & beta=4 & sigma=3 & n=200 & 8.73 \\ 
  194 & MDE.Phi.tv & sigma & beta=4 & sigma=3 & n=200 & 7.52 \\ 
  195 & MDE.Phi.kl & sigma & beta=4 & sigma=3 & n=200 & 4.15 \\ 
  196 & MME & sigma & beta=4 & sigma=3 & n=200 & 5.49 \\ 
  197 & MME.b & sigma & beta=4 & sigma=3 & n=200 & 12.38 \\ 
  198 & PWM & sigma & beta=4 & sigma=3 & n=200 & 3.83 \\ 
  199 & MLE & beta & beta=5 & sigma=3 & n=200 & 12.02 \\ 
  200 & MLE.b & beta & beta=5 & sigma=3 & n=200 & 11.32 \\ 
  201 & LME & beta & beta=5 & sigma=3 & n=200 & 6.77 \\ 
  202 & MDE.Phi.chisq & beta & beta=5 & sigma=3 & n=200 & 13.57 \\ 
  203 & MDE.Phi.tv & beta & beta=5 & sigma=3 & n=200 & 11.01 \\ 
  204 & MDE.Phi.kl & beta & beta=5 & sigma=3 & n=200 & 7.55 \\ 
  205 & MME & beta & beta=5 & sigma=3 & n=200 & 9.77 \\ 
  206 & MME.b & beta & beta=5 & sigma=3 & n=200 & 21.61 \\ 
  207 & PWM & beta & beta=5 & sigma=3 & n=200 & 6.77 \\ 
  208 & MLE & sigma & beta=5 & sigma=3 & n=200 & 7.94 \\ 
  209 & MLE.b & sigma & beta=5 & sigma=3 & n=200 & 7.44 \\ 
  210 & LME & sigma & beta=5 & sigma=3 & n=200 & 4.24 \\ 
  211 & MDE.Phi.chisq & sigma & beta=5 & sigma=3 & n=200 & 12.29 \\ 
  212 & MDE.Phi.tv & sigma & beta=5 & sigma=3 & n=200 & 9.45 \\ 
  213 & MDE.Phi.kl & sigma & beta=5 & sigma=3 & n=200 & 4.81 \\ 
  214 & MME & sigma & beta=5 & sigma=3 & n=200 & 6.40 \\ 
  215 & MME.b & sigma & beta=5 & sigma=3 & n=200 & 14.83 \\ 
  216 & PWM & sigma & beta=5 & sigma=3 & n=200 & 4.24 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220209/Output.mse.LaTeX.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Wed Feb 09 03:24:10 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=3 & n=100 & 0.46 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=3 & n=100 & 0.32 \\ 
  3 & LME & beta & beta=1.5 & sigma=3 & n=100 & 0.40 \\ 
  4 & MDE.Phi.chisq & beta & beta=1.5 & sigma=3 & n=100 & 359.08 \\ 
  5 & MDE.Phi.tv & beta & beta=1.5 & sigma=3 & n=100 & 6.29 \\ 
  6 & MDE.Phi.kl & beta & beta=1.5 & sigma=3 & n=100 & 0.46 \\ 
  7 & MME & beta & beta=1.5 & sigma=3 & n=100 & 2.57 \\ 
  8 & MME.b & beta & beta=1.5 & sigma=3 & n=100 & 130057.24 \\ 
  9 & PWM & beta & beta=1.5 & sigma=3 & n=100 & 0.40 \\ 
  10 & MLE & sigma & beta=1.5 & sigma=3 & n=100 & 4.71 \\ 
  11 & MLE.b & sigma & beta=1.5 & sigma=3 & n=100 & 3.26 \\ 
  12 & LME & sigma & beta=1.5 & sigma=3 & n=100 & 3.94 \\ 
  13 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=3 & n=100 & 178.30 \\ 
  14 & MDE.Phi.tv & sigma & beta=1.5 & sigma=3 & n=100 & 150.85 \\ 
  15 & MDE.Phi.kl & sigma & beta=1.5 & sigma=3 & n=100 & 4.71 \\ 
  16 & MME & sigma & beta=1.5 & sigma=3 & n=100 & 59.63 \\ 
  17 & MME.b & sigma & beta=1.5 & sigma=3 & n=100 & 1340192.06 \\ 
  18 & PWM & sigma & beta=1.5 & sigma=3 & n=100 & 3.94 \\ 
  19 & MLE & beta & beta=2 & sigma=3 & n=100 & 2429.04 \\ 
  20 & MLE.b & beta & beta=2 & sigma=3 & n=100 & 2428.79 \\ 
  21 & LME & beta & beta=2 & sigma=3 & n=100 & 3.31 \\ 
  22 & MDE.Phi.chisq & beta & beta=2 & sigma=3 & n=100 & 65.32 \\ 
  23 & MDE.Phi.tv & beta & beta=2 & sigma=3 & n=100 & 78.89 \\ 
  24 & MDE.Phi.kl & beta & beta=2 & sigma=3 & n=100 & 11.53 \\ 
  25 & MME & beta & beta=2 & sigma=3 & n=100 & 55.69 \\ 
  26 & MME.b & beta & beta=2 & sigma=3 & n=100 & 151259.47 \\ 
  27 & PWM & beta & beta=2 & sigma=3 & n=100 & 3.31 \\ 
  28 & MLE & sigma & beta=2 & sigma=3 & n=100 & 6899.81 \\ 
  29 & MLE.b & sigma & beta=2 & sigma=3 & n=100 & 6898.56 \\ 
  30 & LME & sigma & beta=2 & sigma=3 & n=100 & 13.82 \\ 
  31 & MDE.Phi.chisq & sigma & beta=2 & sigma=3 & n=100 & 614.56 \\ 
  32 & MDE.Phi.tv & sigma & beta=2 & sigma=3 & n=100 & 789.09 \\ 
  33 & MDE.Phi.kl & sigma & beta=2 & sigma=3 & n=100 & 43.70 \\ 
  34 & MME & sigma & beta=2 & sigma=3 & n=100 & 224.26 \\ 
  35 & MME.b & sigma & beta=2 & sigma=3 & n=100 & 752145.36 \\ 
  36 & PWM & sigma & beta=2 & sigma=3 & n=100 & 13.82 \\ 
  37 & MLE & beta & beta=2.5 & sigma=3 & n=100 & 5315.03 \\ 
  38 & MLE.b & beta & beta=2.5 & sigma=3 & n=100 & 5314.90 \\ 
  39 & LME & beta & beta=2.5 & sigma=3 & n=100 & 8.83 \\ 
  40 & MDE.Phi.chisq & beta & beta=2.5 & sigma=3 & n=100 & 203.79 \\ 
  41 & MDE.Phi.tv & beta & beta=2.5 & sigma=3 & n=100 & 236.10 \\ 
  42 & MDE.Phi.kl & beta & beta=2.5 & sigma=3 & n=100 & 28.69 \\ 
  43 & MME & beta & beta=2.5 & sigma=3 & n=100 & 149.68 \\ 
  44 & MME.b & beta & beta=2.5 & sigma=3 & n=100 & 2235.69 \\ 
  45 & PWM & beta & beta=2.5 & sigma=3 & n=100 & 8.83 \\ 
  46 & MLE & sigma & beta=2.5 & sigma=3 & n=100 & 14044.19 \\ 
  47 & MLE.b & sigma & beta=2.5 & sigma=3 & n=100 & 14043.78 \\ 
  48 & LME & sigma & beta=2.5 & sigma=3 & n=100 & 21.39 \\ 
  49 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=3 & n=100 & 1125.26 \\ 
  50 & MDE.Phi.tv & sigma & beta=2.5 & sigma=3 & n=100 & 1294.84 \\ 
  51 & MDE.Phi.kl & sigma & beta=2.5 & sigma=3 & n=100 & 70.76 \\ 
  52 & MME & sigma & beta=2.5 & sigma=3 & n=100 & 354.29 \\ 
  53 & MME.b & sigma & beta=2.5 & sigma=3 & n=100 & 5752.28 \\ 
  54 & PWM & sigma & beta=2.5 & sigma=3 & n=100 & 21.39 \\ 
  55 & MLE & beta & beta=3 & sigma=3 & n=100 & 39586.86 \\ 
  56 & MLE.b & beta & beta=3 & sigma=3 & n=100 & 39587.06 \\ 
  57 & LME & beta & beta=3 & sigma=3 & n=100 & 17.02 \\ 
  58 & MDE.Phi.chisq & beta & beta=3 & sigma=3 & n=100 & 441.41 \\ 
  59 & MDE.Phi.tv & beta & beta=3 & sigma=3 & n=100 & 533.17 \\ 
  60 & MDE.Phi.kl & beta & beta=3 & sigma=3 & n=100 & 95.53 \\ 
  61 & MME & beta & beta=3 & sigma=3 & n=100 & 313324.91 \\ 
  62 & MME.b & beta & beta=3 & sigma=3 & n=100 & 2979285.90 \\ 
  63 & PWM & beta & beta=3 & sigma=3 & n=100 & 17.02 \\ 
  64 & MLE & sigma & beta=3 & sigma=3 & n=100 & 69386.57 \\ 
  65 & MLE.b & sigma & beta=3 & sigma=3 & n=100 & 69386.83 \\ 
  66 & LME & sigma & beta=3 & sigma=3 & n=100 & 29.38 \\ 
  67 & MDE.Phi.chisq & sigma & beta=3 & sigma=3 & n=100 & 1598.20 \\ 
  68 & MDE.Phi.tv & sigma & beta=3 & sigma=3 & n=100 & 1885.63 \\ 
  69 & MDE.Phi.kl & sigma & beta=3 & sigma=3 & n=100 & 160.57 \\ 
  70 & MME & sigma & beta=3 & sigma=3 & n=100 & 407160.29 \\ 
  71 & MME.b & sigma & beta=3 & sigma=3 & n=100 & 3875831.90 \\ 
  72 & PWM & sigma & beta=3 & sigma=3 & n=100 & 29.38 \\ 
  73 & MLE & beta & beta=4 & sigma=3 & n=100 & 75794.29 \\ 
  74 & MLE.b & beta & beta=4 & sigma=3 & n=100 & 75795.22 \\ 
  75 & LME & beta & beta=4 & sigma=3 & n=100 & 49.52 \\ 
  76 & MDE.Phi.chisq & beta & beta=4 & sigma=3 & n=100 & 1131.14 \\ 
  77 & MDE.Phi.tv & beta & beta=4 & sigma=3 & n=100 & 1324.20 \\ 
  78 & MDE.Phi.kl & beta & beta=4 & sigma=3 & n=100 & 198.72 \\ 
  79 & MME & beta & beta=4 & sigma=3 & n=100 & 11609.73 \\ 
  80 & MME.b & beta & beta=4 & sigma=3 & n=100 & 1922332.01 \\ 
  81 & PWM & beta & beta=4 & sigma=3 & n=100 & 49.52 \\ 
  82 & MLE & sigma & beta=4 & sigma=3 & n=100 & 61641.06 \\ 
  83 & MLE.b & sigma & beta=4 & sigma=3 & n=100 & 61641.79 \\ 
  84 & LME & sigma & beta=4 & sigma=3 & n=100 & 43.43 \\ 
  85 & MDE.Phi.chisq & sigma & beta=4 & sigma=3 & n=100 & 2022.01 \\ 
  86 & MDE.Phi.tv & sigma & beta=4 & sigma=3 & n=100 & 2244.20 \\ 
  87 & MDE.Phi.kl & sigma & beta=4 & sigma=3 & n=100 & 176.25 \\ 
  88 & MME & sigma & beta=4 & sigma=3 & n=100 & 9826.84 \\ 
  89 & MME.b & sigma & beta=4 & sigma=3 & n=100 & 2436124.66 \\ 
  90 & PWM & sigma & beta=4 & sigma=3 & n=100 & 43.43 \\ 
  91 & MLE & beta & beta=5 & sigma=3 & n=100 & 144826.94 \\ 
  92 & MLE.b & beta & beta=5 & sigma=3 & n=100 & 144828.37 \\ 
  93 & LME & beta & beta=5 & sigma=3 & n=100 & 92.61 \\ 
  94 & MDE.Phi.chisq & beta & beta=5 & sigma=3 & n=100 & 1823.98 \\ 
  95 & MDE.Phi.tv & beta & beta=5 & sigma=3 & n=100 & 2004.27 \\ 
  96 & MDE.Phi.kl & beta & beta=5 & sigma=3 & n=100 & 343.50 \\ 
  97 & MME & beta & beta=5 & sigma=3 & n=100 & 18721.79 \\ 
  98 & MME.b & beta & beta=5 & sigma=3 & n=100 & 259583.10 \\ 
  99 & PWM & beta & beta=5 & sigma=3 & n=100 & 92.61 \\ 
  100 & MLE & sigma & beta=5 & sigma=3 & n=100 & 73757.62 \\ 
  101 & MLE.b & sigma & beta=5 & sigma=3 & n=100 & 73758.30 \\ 
  102 & LME & sigma & beta=5 & sigma=3 & n=100 & 46.63 \\ 
  103 & MDE.Phi.chisq & sigma & beta=5 & sigma=3 & n=100 & 1886.05 \\ 
  104 & MDE.Phi.tv & sigma & beta=5 & sigma=3 & n=100 & 1979.86 \\ 
  105 & MDE.Phi.kl & sigma & beta=5 & sigma=3 & n=100 & 171.69 \\ 
  106 & MME & sigma & beta=5 & sigma=3 & n=100 & 9397.41 \\ 
  107 & MME.b & sigma & beta=5 & sigma=3 & n=100 & 139895.14 \\ 
  108 & PWM & sigma & beta=5 & sigma=3 & n=100 & 46.63 \\ 
  109 & MLE & beta & beta=1.5 & sigma=3 & n=200 & 0.11 \\ 
  110 & MLE.b & beta & beta=1.5 & sigma=3 & n=200 & 0.08 \\ 
  111 & LME & beta & beta=1.5 & sigma=3 & n=200 & 0.15 \\ 
  112 & MDE.Phi.chisq & beta & beta=1.5 & sigma=3 & n=200 & 72.05 \\ 
  113 & MDE.Phi.tv & beta & beta=1.5 & sigma=3 & n=200 & 0.43 \\ 
  114 & MDE.Phi.kl & beta & beta=1.5 & sigma=3 & n=200 & 0.11 \\ 
  115 & MME & beta & beta=1.5 & sigma=3 & n=200 & 1.16 \\ 
  116 & MME.b & beta & beta=1.5 & sigma=3 & n=200 & 0.89 \\ 
  117 & PWM & beta & beta=1.5 & sigma=3 & n=200 & 0.15 \\ 
  118 & MLE & sigma & beta=1.5 & sigma=3 & n=200 & 1.03 \\ 
  119 & MLE.b & sigma & beta=1.5 & sigma=3 & n=200 & 0.72 \\ 
  120 & LME & sigma & beta=1.5 & sigma=3 & n=200 & 1.48 \\ 
  121 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=3 & n=200 & 13.13 \\ 
  122 & MDE.Phi.tv & sigma & beta=1.5 & sigma=3 & n=200 & 3.20 \\ 
  123 & MDE.Phi.kl & sigma & beta=1.5 & sigma=3 & n=200 & 1.03 \\ 
  124 & MME & sigma & beta=1.5 & sigma=3 & n=200 & 42.33 \\ 
  125 & MME.b & sigma & beta=1.5 & sigma=3 & n=200 & 34.99 \\ 
  126 & PWM & sigma & beta=1.5 & sigma=3 & n=200 & 1.48 \\ 
  127 & MLE & beta & beta=2 & sigma=3 & n=200 & 0.32 \\ 
  128 & MLE.b & beta & beta=2 & sigma=3 & n=200 & 0.19 \\ 
  129 & LME & beta & beta=2 & sigma=3 & n=200 & 0.35 \\ 
  130 & MDE.Phi.chisq & beta & beta=2 & sigma=3 & n=200 & 4.74 \\ 
  131 & MDE.Phi.tv & beta & beta=2 & sigma=3 & n=200 & 2.23 \\ 
  132 & MDE.Phi.kl & beta & beta=2 & sigma=3 & n=200 & 0.32 \\ 
  133 & MME & beta & beta=2 & sigma=3 & n=200 & 1.48 \\ 
  134 & MME.b & beta & beta=2 & sigma=3 & n=200 & 5.87 \\ 
  135 & PWM & beta & beta=2 & sigma=3 & n=200 & 0.35 \\ 
  136 & MLE & sigma & beta=2 & sigma=3 & n=200 & 1.41 \\ 
  137 & MLE.b & sigma & beta=2 & sigma=3 & n=200 & 0.85 \\ 
  138 & LME & sigma & beta=2 & sigma=3 & n=200 & 1.53 \\ 
  139 & MDE.Phi.chisq & sigma & beta=2 & sigma=3 & n=200 & 15.13 \\ 
  140 & MDE.Phi.tv & sigma & beta=2 & sigma=3 & n=200 & 19.45 \\ 
  141 & MDE.Phi.kl & sigma & beta=2 & sigma=3 & n=200 & 1.41 \\ 
  142 & MME & sigma & beta=2 & sigma=3 & n=200 & 9.60 \\ 
  143 & MME.b & sigma & beta=2 & sigma=3 & n=200 & 26.71 \\ 
  144 & PWM & sigma & beta=2 & sigma=3 & n=200 & 1.53 \\ 
  145 & MLE & beta & beta=2.5 & sigma=3 & n=200 & 1.18 \\ 
  146 & MLE.b & beta & beta=2.5 & sigma=3 & n=200 & 0.83 \\ 
  147 & LME & beta & beta=2.5 & sigma=3 & n=200 & 1.28 \\ 
  148 & MDE.Phi.chisq & beta & beta=2.5 & sigma=3 & n=200 & 16.19 \\ 
  149 & MDE.Phi.tv & beta & beta=2.5 & sigma=3 & n=200 & 12.59 \\ 
  150 & MDE.Phi.kl & beta & beta=2.5 & sigma=3 & n=200 & 1.18 \\ 
  151 & MME & beta & beta=2.5 & sigma=3 & n=200 & 2.90 \\ 
  152 & MME.b & beta & beta=2.5 & sigma=3 & n=200 & 44.44 \\ 
  153 & PWM & beta & beta=2.5 & sigma=3 & n=200 & 1.28 \\ 
  154 & MLE & sigma & beta=2.5 & sigma=3 & n=200 & 3.15 \\ 
  155 & MLE.b & sigma & beta=2.5 & sigma=3 & n=200 & 2.23 \\ 
  156 & LME & sigma & beta=2.5 & sigma=3 & n=200 & 3.26 \\ 
  157 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=3 & n=200 & 73.72 \\ 
  158 & MDE.Phi.tv & sigma & beta=2.5 & sigma=3 & n=200 & 55.91 \\ 
  159 & MDE.Phi.kl & sigma & beta=2.5 & sigma=3 & n=200 & 3.15 \\ 
  160 & MME & sigma & beta=2.5 & sigma=3 & n=200 & 8.65 \\ 
  161 & MME.b & sigma & beta=2.5 & sigma=3 & n=200 & 113.14 \\ 
  162 & PWM & sigma & beta=2.5 & sigma=3 & n=200 & 3.26 \\ 
  163 & MLE & beta & beta=3 & sigma=3 & n=200 & 64.43 \\ 
  164 & MLE.b & beta & beta=3 & sigma=3 & n=200 & 63.87 \\ 
  165 & LME & beta & beta=3 & sigma=3 & n=200 & 4.35 \\ 
  166 & MDE.Phi.chisq & beta & beta=3 & sigma=3 & n=200 & 79.20 \\ 
  167 & MDE.Phi.tv & beta & beta=3 & sigma=3 & n=200 & 38.54 \\ 
  168 & MDE.Phi.kl & beta & beta=3 & sigma=3 & n=200 & 7.71 \\ 
  169 & MME & beta & beta=3 & sigma=3 & n=200 & 74.99 \\ 
  170 & MME.b & beta & beta=3 & sigma=3 & n=200 & 7353.37 \\ 
  171 & PWM & beta & beta=3 & sigma=3 & n=200 & 4.35 \\ 
  172 & MLE & sigma & beta=3 & sigma=3 & n=200 & 93.57 \\ 
  173 & MLE.b & sigma & beta=3 & sigma=3 & n=200 & 92.61 \\ 
  174 & LME & sigma & beta=3 & sigma=3 & n=200 & 7.02 \\ 
  175 & MDE.Phi.chisq & sigma & beta=3 & sigma=3 & n=200 & 239.36 \\ 
  176 & MDE.Phi.tv & sigma & beta=3 & sigma=3 & n=200 & 108.60 \\ 
  177 & MDE.Phi.kl & sigma & beta=3 & sigma=3 & n=200 & 12.40 \\ 
  178 & MME & sigma & beta=3 & sigma=3 & n=200 & 110.52 \\ 
  179 & MME.b & sigma & beta=3 & sigma=3 & n=200 & 15145.57 \\ 
  180 & PWM & sigma & beta=3 & sigma=3 & n=200 & 7.02 \\ 
  181 & MLE & beta & beta=4 & sigma=3 & n=200 & 355.39 \\ 
  182 & MLE.b & beta & beta=4 & sigma=3 & n=200 & 355.22 \\ 
  183 & LME & beta & beta=4 & sigma=3 & n=200 & 18.29 \\ 
  184 & MDE.Phi.chisq & beta & beta=4 & sigma=3 & n=200 & 418.95 \\ 
  185 & MDE.Phi.tv & beta & beta=4 & sigma=3 & n=200 & 314.56 \\ 
  186 & MDE.Phi.kl & beta & beta=4 & sigma=3 & n=200 & 40.16 \\ 
  187 & MME & beta & beta=4 & sigma=3 & n=200 & 551.00 \\ 
  188 & MME.b & beta & beta=4 & sigma=3 & n=200 & 40296.91 \\ 
  189 & PWM & beta & beta=4 & sigma=3 & n=200 & 18.29 \\ 
  190 & MLE & sigma & beta=4 & sigma=3 & n=200 & 309.10 \\ 
  191 & MLE.b & sigma & beta=4 & sigma=3 & n=200 & 308.92 \\ 
  192 & LME & sigma & beta=4 & sigma=3 & n=200 & 15.43 \\ 
  193 & MDE.Phi.chisq & sigma & beta=4 & sigma=3 & n=200 & 630.61 \\ 
  194 & MDE.Phi.tv & sigma & beta=4 & sigma=3 & n=200 & 458.72 \\ 
  195 & MDE.Phi.kl & sigma & beta=4 & sigma=3 & n=200 & 34.24 \\ 
  196 & MME & sigma & beta=4 & sigma=3 & n=200 & 480.75 \\ 
  197 & MME.b & sigma & beta=4 & sigma=3 & n=200 & 44568.02 \\ 
  198 & PWM & sigma & beta=4 & sigma=3 & n=200 & 15.43 \\ 
  199 & MLE & beta & beta=5 & sigma=3 & n=200 & 41125.93 \\ 
  200 & MLE.b & beta & beta=5 & sigma=3 & n=200 & 41126.79 \\ 
  201 & LME & beta & beta=5 & sigma=3 & n=200 & 63.80 \\ 
  202 & MDE.Phi.chisq & beta & beta=5 & sigma=3 & n=200 & 1064.11 \\ 
  203 & MDE.Phi.tv & beta & beta=5 & sigma=3 & n=200 & 706.91 \\ 
  204 & MDE.Phi.kl & beta & beta=5 & sigma=3 & n=200 & 130.30 \\ 
  205 & MME & beta & beta=5 & sigma=3 & n=200 & 2746.12 \\ 
  206 & MME.b & beta & beta=5 & sigma=3 & n=200 & 30989.31 \\ 
  207 & PWM & beta & beta=5 & sigma=3 & n=200 & 63.80 \\ 
  208 & MLE & sigma & beta=5 & sigma=3 & n=200 & 20210.86 \\ 
  209 & MLE.b & sigma & beta=5 & sigma=3 & n=200 & 20211.26 \\ 
  210 & LME & sigma & beta=5 & sigma=3 & n=200 & 32.36 \\ 
  211 & MDE.Phi.chisq & sigma & beta=5 & sigma=3 & n=200 & 939.58 \\ 
  212 & MDE.Phi.tv & sigma & beta=5 & sigma=3 & n=200 & 590.42 \\ 
  213 & MDE.Phi.kl & sigma & beta=5 & sigma=3 & n=200 & 65.65 \\ 
  214 & MME & sigma & beta=5 & sigma=3 & n=200 & 1343.84 \\ 
  215 & MME.b & sigma & beta=5 & sigma=3 & n=200 & 15775.95 \\ 
  216 & PWM & sigma & beta=5 & sigma=3 & n=200 & 32.36 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220209/Output.var.LaTeX.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Wed Feb 09 03:24:10 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=3 & n=100 & 0.44 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=3 & n=100 & 0.32 \\ 
  3 & LME & beta & beta=1.5 & sigma=3 & n=100 & 0.30 \\ 
  4 & MDE.Phi.chisq & beta & beta=1.5 & sigma=3 & n=100 & 347.78 \\ 
  5 & MDE.Phi.tv & beta & beta=1.5 & sigma=3 & n=100 & 6.22 \\ 
  6 & MDE.Phi.kl & beta & beta=1.5 & sigma=3 & n=100 & 0.44 \\ 
  7 & MME & beta & beta=1.5 & sigma=3 & n=100 & 0.90 \\ 
  8 & MME.b & beta & beta=1.5 & sigma=3 & n=100 & 130047.07 \\ 
  9 & PWM & beta & beta=1.5 & sigma=3 & n=100 & 0.30 \\ 
  10 & MLE & sigma & beta=1.5 & sigma=3 & n=100 & 4.41 \\ 
  11 & MLE.b & sigma & beta=1.5 & sigma=3 & n=100 & 3.25 \\ 
  12 & LME & sigma & beta=1.5 & sigma=3 & n=100 & 2.99 \\ 
  13 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=3 & n=100 & 173.39 \\ 
  14 & MDE.Phi.tv & sigma & beta=1.5 & sigma=3 & n=100 & 144.67 \\ 
  15 & MDE.Phi.kl & sigma & beta=1.5 & sigma=3 & n=100 & 4.41 \\ 
  16 & MME & sigma & beta=1.5 & sigma=3 & n=100 & 17.93 \\ 
  17 & MME.b & sigma & beta=1.5 & sigma=3 & n=100 & 1340019.71 \\ 
  18 & PWM & sigma & beta=1.5 & sigma=3 & n=100 & 2.99 \\ 
  19 & MLE & beta & beta=2 & sigma=3 & n=100 & 2428.30 \\ 
  20 & MLE.b & beta & beta=2 & sigma=3 & n=100 & 2428.61 \\ 
  21 & LME & beta & beta=2 & sigma=3 & n=100 & 3.11 \\ 
  22 & MDE.Phi.chisq & beta & beta=2 & sigma=3 & n=100 & 65.32 \\ 
  23 & MDE.Phi.tv & beta & beta=2 & sigma=3 & n=100 & 78.47 \\ 
  24 & MDE.Phi.kl & beta & beta=2 & sigma=3 & n=100 & 11.32 \\ 
  25 & MME & beta & beta=2 & sigma=3 & n=100 & 52.88 \\ 
  26 & MME.b & beta & beta=2 & sigma=3 & n=100 & 151218.71 \\ 
  27 & PWM & beta & beta=2 & sigma=3 & n=100 & 3.11 \\ 
  28 & MLE & sigma & beta=2 & sigma=3 & n=100 & 6896.93 \\ 
  29 & MLE.b & sigma & beta=2 & sigma=3 & n=100 & 6897.96 \\ 
  30 & LME & sigma & beta=2 & sigma=3 & n=100 & 13.01 \\ 
  31 & MDE.Phi.chisq & sigma & beta=2 & sigma=3 & n=100 & 604.20 \\ 
  32 & MDE.Phi.tv & sigma & beta=2 & sigma=3 & n=100 & 766.97 \\ 
  33 & MDE.Phi.kl & sigma & beta=2 & sigma=3 & n=100 & 42.77 \\ 
  34 & MME & sigma & beta=2 & sigma=3 & n=100 & 205.69 \\ 
  35 & MME.b & sigma & beta=2 & sigma=3 & n=100 & 751939.67 \\ 
  36 & PWM & sigma & beta=2 & sigma=3 & n=100 & 13.01 \\ 
  37 & MLE & beta & beta=2.5 & sigma=3 & n=100 & 5311.45 \\ 
  38 & MLE.b & beta & beta=2.5 & sigma=3 & n=100 & 5312.97 \\ 
  39 & LME & beta & beta=2.5 & sigma=3 & n=100 & 8.34 \\ 
  40 & MDE.Phi.chisq & beta & beta=2.5 & sigma=3 & n=100 & 201.51 \\ 
  41 & MDE.Phi.tv & beta & beta=2.5 & sigma=3 & n=100 & 230.70 \\ 
  42 & MDE.Phi.kl & beta & beta=2.5 & sigma=3 & n=100 & 27.83 \\ 
  43 & MME & beta & beta=2.5 & sigma=3 & n=100 & 144.30 \\ 
  44 & MME.b & beta & beta=2.5 & sigma=3 & n=100 & 2205.73 \\ 
  45 & PWM & beta & beta=2.5 & sigma=3 & n=100 & 8.34 \\ 
  46 & MLE & sigma & beta=2.5 & sigma=3 & n=100 & 14034.86 \\ 
  47 & MLE.b & sigma & beta=2.5 & sigma=3 & n=100 & 14038.77 \\ 
  48 & LME & sigma & beta=2.5 & sigma=3 & n=100 & 20.24 \\ 
  49 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=3 & n=100 & 1089.17 \\ 
  50 & MDE.Phi.tv & sigma & beta=2.5 & sigma=3 & n=100 & 1237.72 \\ 
  51 & MDE.Phi.kl & sigma & beta=2.5 & sigma=3 & n=100 & 68.52 \\ 
  52 & MME & sigma & beta=2.5 & sigma=3 & n=100 & 337.82 \\ 
  53 & MME.b & sigma & beta=2.5 & sigma=3 & n=100 & 5670.67 \\ 
  54 & PWM & sigma & beta=2.5 & sigma=3 & n=100 & 20.24 \\ 
  55 & MLE & beta & beta=3 & sigma=3 & n=100 & 39517.87 \\ 
  56 & MLE.b & beta & beta=3 & sigma=3 & n=100 & 39526.27 \\ 
  57 & LME & beta & beta=3 & sigma=3 & n=100 & 15.99 \\ 
  58 & MDE.Phi.chisq & beta & beta=3 & sigma=3 & n=100 & 428.37 \\ 
  59 & MDE.Phi.tv & beta & beta=3 & sigma=3 & n=100 & 508.61 \\ 
  60 & MDE.Phi.kl & beta & beta=3 & sigma=3 & n=100 & 92.20 \\ 
  61 & MME & beta & beta=3 & sigma=3 & n=100 & 313146.34 \\ 
  62 & MME.b & beta & beta=3 & sigma=3 & n=100 & 2977375.61 \\ 
  63 & PWM & beta & beta=3 & sigma=3 & n=100 & 15.99 \\ 
  64 & MLE & sigma & beta=3 & sigma=3 & n=100 & 69270.67 \\ 
  65 & MLE.b & sigma & beta=3 & sigma=3 & n=100 & 69284.72 \\ 
  66 & LME & sigma & beta=3 & sigma=3 & n=100 & 27.75 \\ 
  67 & MDE.Phi.chisq & sigma & beta=3 & sigma=3 & n=100 & 1517.48 \\ 
  68 & MDE.Phi.tv & sigma & beta=3 & sigma=3 & n=100 & 1763.67 \\ 
  69 & MDE.Phi.kl & sigma & beta=3 & sigma=3 & n=100 & 154.99 \\ 
  70 & MME & sigma & beta=3 & sigma=3 & n=100 & 406904.26 \\ 
  71 & MME.b & sigma & beta=3 & sigma=3 & n=100 & 3873116.01 \\ 
  72 & PWM & sigma & beta=3 & sigma=3 & n=100 & 27.75 \\ 
  73 & MLE & beta & beta=4 & sigma=3 & n=100 & 75623.37 \\ 
  74 & MLE.b & beta & beta=4 & sigma=3 & n=100 & 75636.10 \\ 
  75 & LME & beta & beta=4 & sigma=3 & n=100 & 46.48 \\ 
  76 & MDE.Phi.chisq & beta & beta=4 & sigma=3 & n=100 & 1047.10 \\ 
  77 & MDE.Phi.tv & beta & beta=4 & sigma=3 & n=100 & 1197.43 \\ 
  78 & MDE.Phi.kl & beta & beta=4 & sigma=3 & n=100 & 187.37 \\ 
  79 & MME & beta & beta=4 & sigma=3 & n=100 & 11556.83 \\ 
  80 & MME.b & beta & beta=4 & sigma=3 & n=100 & 1921162.10 \\ 
  81 & PWM & beta & beta=4 & sigma=3 & n=100 & 46.48 \\ 
  82 & MLE & sigma & beta=4 & sigma=3 & n=100 & 61498.81 \\ 
  83 & MLE.b & sigma & beta=4 & sigma=3 & n=100 & 61509.34 \\ 
  84 & LME & sigma & beta=4 & sigma=3 & n=100 & 40.89 \\ 
  85 & MDE.Phi.chisq & sigma & beta=4 & sigma=3 & n=100 & 1826.95 \\ 
  86 & MDE.Phi.tv & sigma & beta=4 & sigma=3 & n=100 & 1987.70 \\ 
  87 & MDE.Phi.kl & sigma & beta=4 & sigma=3 & n=100 & 166.42 \\ 
  88 & MME & sigma & beta=4 & sigma=3 & n=100 & 9778.87 \\ 
  89 & MME.b & sigma & beta=4 & sigma=3 & n=100 & 2434977.11 \\ 
  90 & PWM & sigma & beta=4 & sigma=3 & n=100 & 40.89 \\ 
  91 & MLE & beta & beta=5 & sigma=3 & n=100 & 144295.10 \\ 
  92 & MLE.b & beta & beta=5 & sigma=3 & n=100 & 144313.62 \\ 
  93 & LME & beta & beta=5 & sigma=3 & n=100 & 87.33 \\ 
  94 & MDE.Phi.chisq & beta & beta=5 & sigma=3 & n=100 & 1624.25 \\ 
  95 & MDE.Phi.tv & beta & beta=5 & sigma=3 & n=100 & 1742.16 \\ 
  96 & MDE.Phi.kl & beta & beta=5 & sigma=3 & n=100 & 319.00 \\ 
  97 & MME & beta & beta=5 & sigma=3 & n=100 & 18586.56 \\ 
  98 & MME.b & beta & beta=5 & sigma=3 & n=100 & 257834.84 \\ 
  99 & PWM & beta & beta=5 & sigma=3 & n=100 & 87.33 \\ 
  100 & MLE & sigma & beta=5 & sigma=3 & n=100 & 73489.84 \\ 
  101 & MLE.b & sigma & beta=5 & sigma=3 & n=100 & 73498.98 \\ 
  102 & LME & sigma & beta=5 & sigma=3 & n=100 & 44.04 \\ 
  103 & MDE.Phi.chisq & sigma & beta=5 & sigma=3 & n=100 & 1635.55 \\ 
  104 & MDE.Phi.tv & sigma & beta=5 & sigma=3 & n=100 & 1683.51 \\ 
  105 & MDE.Phi.kl & sigma & beta=5 & sigma=3 & n=100 & 159.47 \\ 
  106 & MME & sigma & beta=5 & sigma=3 & n=100 & 9330.58 \\ 
  107 & MME.b & sigma & beta=5 & sigma=3 & n=100 & 139016.87 \\ 
  108 & PWM & sigma & beta=5 & sigma=3 & n=100 & 44.04 \\ 
  109 & MLE & beta & beta=1.5 & sigma=3 & n=200 & 0.10 \\ 
  110 & MLE.b & beta & beta=1.5 & sigma=3 & n=200 & 0.08 \\ 
  111 & LME & beta & beta=1.5 & sigma=3 & n=200 & 0.11 \\ 
  112 & MDE.Phi.chisq & beta & beta=1.5 & sigma=3 & n=200 & 70.32 \\ 
  113 & MDE.Phi.tv & beta & beta=1.5 & sigma=3 & n=200 & 0.18 \\ 
  114 & MDE.Phi.kl & beta & beta=1.5 & sigma=3 & n=200 & 0.10 \\ 
  115 & MME & beta & beta=1.5 & sigma=3 & n=200 & 0.16 \\ 
  116 & MME.b & beta & beta=1.5 & sigma=3 & n=200 & 0.26 \\ 
  117 & PWM & beta & beta=1.5 & sigma=3 & n=200 & 0.11 \\ 
  118 & MLE & sigma & beta=1.5 & sigma=3 & n=200 & 0.97 \\ 
  119 & MLE.b & sigma & beta=1.5 & sigma=3 & n=200 & 0.72 \\ 
  120 & LME & sigma & beta=1.5 & sigma=3 & n=200 & 1.11 \\ 
  121 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=3 & n=200 & 12.71 \\ 
  122 & MDE.Phi.tv & sigma & beta=1.5 & sigma=3 & n=200 & 2.60 \\ 
  123 & MDE.Phi.kl & sigma & beta=1.5 & sigma=3 & n=200 & 0.97 \\ 
  124 & MME & sigma & beta=1.5 & sigma=3 & n=200 & 13.64 \\ 
  125 & MME.b & sigma & beta=1.5 & sigma=3 & n=200 & 14.48 \\ 
  126 & PWM & sigma & beta=1.5 & sigma=3 & n=200 & 1.11 \\ 
  127 & MLE & beta & beta=2 & sigma=3 & n=200 & 0.30 \\ 
  128 & MLE.b & beta & beta=2 & sigma=3 & n=200 & 0.19 \\ 
  129 & LME & beta & beta=2 & sigma=3 & n=200 & 0.30 \\ 
  130 & MDE.Phi.chisq & beta & beta=2 & sigma=3 & n=200 & 4.29 \\ 
  131 & MDE.Phi.tv & beta & beta=2 & sigma=3 & n=200 & 2.03 \\ 
  132 & MDE.Phi.kl & beta & beta=2 & sigma=3 & n=200 & 0.30 \\ 
  133 & MME & beta & beta=2 & sigma=3 & n=200 & 0.53 \\ 
  134 & MME.b & beta & beta=2 & sigma=3 & n=200 & 5.40 \\ 
  135 & PWM & beta & beta=2 & sigma=3 & n=200 & 0.30 \\ 
  136 & MLE & sigma & beta=2 & sigma=3 & n=200 & 1.32 \\ 
  137 & MLE.b & sigma & beta=2 & sigma=3 & n=200 & 0.84 \\ 
  138 & LME & sigma & beta=2 & sigma=3 & n=200 & 1.35 \\ 
  139 & MDE.Phi.chisq & sigma & beta=2 & sigma=3 & n=200 & 14.86 \\ 
  140 & MDE.Phi.tv & sigma & beta=2 & sigma=3 & n=200 & 18.76 \\ 
  141 & MDE.Phi.kl & sigma & beta=2 & sigma=3 & n=200 & 1.32 \\ 
  142 & MME & sigma & beta=2 & sigma=3 & n=200 & 2.50 \\ 
  143 & MME.b & sigma & beta=2 & sigma=3 & n=200 & 22.95 \\ 
  144 & PWM & sigma & beta=2 & sigma=3 & n=200 & 1.35 \\ 
  145 & MLE & beta & beta=2.5 & sigma=3 & n=200 & 1.12 \\ 
  146 & MLE.b & beta & beta=2.5 & sigma=3 & n=200 & 0.83 \\ 
  147 & LME & beta & beta=2.5 & sigma=3 & n=200 & 1.20 \\ 
  148 & MDE.Phi.chisq & beta & beta=2.5 & sigma=3 & n=200 & 15.99 \\ 
  149 & MDE.Phi.tv & beta & beta=2.5 & sigma=3 & n=200 & 12.54 \\ 
  150 & MDE.Phi.kl & beta & beta=2.5 & sigma=3 & n=200 & 1.12 \\ 
  151 & MME & beta & beta=2.5 & sigma=3 & n=200 & 1.77 \\ 
  152 & MME.b & beta & beta=2.5 & sigma=3 & n=200 & 43.75 \\ 
  153 & PWM & beta & beta=2.5 & sigma=3 & n=200 & 1.20 \\ 
  154 & MLE & sigma & beta=2.5 & sigma=3 & n=200 & 2.99 \\ 
  155 & MLE.b & sigma & beta=2.5 & sigma=3 & n=200 & 2.23 \\ 
  156 & LME & sigma & beta=2.5 & sigma=3 & n=200 & 3.07 \\ 
  157 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=3 & n=200 & 72.66 \\ 
  158 & MDE.Phi.tv & sigma & beta=2.5 & sigma=3 & n=200 & 54.46 \\ 
  159 & MDE.Phi.kl & sigma & beta=2.5 & sigma=3 & n=200 & 2.98 \\ 
  160 & MME & sigma & beta=2.5 & sigma=3 & n=200 & 4.79 \\ 
  161 & MME.b & sigma & beta=2.5 & sigma=3 & n=200 & 110.84 \\ 
  162 & PWM & sigma & beta=2.5 & sigma=3 & n=200 & 3.07 \\ 
  163 & MLE & beta & beta=3 & sigma=3 & n=200 & 64.12 \\ 
  164 & MLE.b & beta & beta=3 & sigma=3 & n=200 & 63.87 \\ 
  165 & LME & beta & beta=3 & sigma=3 & n=200 & 4.14 \\ 
  166 & MDE.Phi.chisq & beta & beta=3 & sigma=3 & n=200 & 79.14 \\ 
  167 & MDE.Phi.tv & beta & beta=3 & sigma=3 & n=200 & 38.50 \\ 
  168 & MDE.Phi.kl & beta & beta=3 & sigma=3 & n=200 & 7.46 \\ 
  169 & MME & beta & beta=3 & sigma=3 & n=200 & 73.03 \\ 
  170 & MME.b & beta & beta=3 & sigma=3 & n=200 & 7346.85 \\ 
  171 & PWM & beta & beta=3 & sigma=3 & n=200 & 4.14 \\ 
  172 & MLE & sigma & beta=3 & sigma=3 & n=200 & 93.07 \\ 
  173 & MLE.b & sigma & beta=3 & sigma=3 & n=200 & 92.60 \\ 
  174 & LME & sigma & beta=3 & sigma=3 & n=200 & 6.70 \\ 
  175 & MDE.Phi.chisq & sigma & beta=3 & sigma=3 & n=200 & 234.32 \\ 
  176 & MDE.Phi.tv & sigma & beta=3 & sigma=3 & n=200 & 105.50 \\ 
  177 & MDE.Phi.kl & sigma & beta=3 & sigma=3 & n=200 & 12.00 \\ 
  178 & MME & sigma & beta=3 & sigma=3 & n=200 & 106.77 \\ 
  179 & MME.b & sigma & beta=3 & sigma=3 & n=200 & 15133.43 \\ 
  180 & PWM & sigma & beta=3 & sigma=3 & n=200 & 6.70 \\ 
  181 & MLE & beta & beta=4 & sigma=3 & n=200 & 353.05 \\ 
  182 & MLE.b & beta & beta=4 & sigma=3 & n=200 & 354.49 \\ 
  183 & LME & beta & beta=4 & sigma=3 & n=200 & 17.45 \\ 
  184 & MDE.Phi.chisq & beta & beta=4 & sigma=3 & n=200 & 406.85 \\ 
  185 & MDE.Phi.tv & beta & beta=4 & sigma=3 & n=200 & 306.74 \\ 
  186 & MDE.Phi.kl & beta & beta=4 & sigma=3 & n=200 & 38.60 \\ 
  187 & MME & beta & beta=4 & sigma=3 & n=200 & 544.10 \\ 
  188 & MME.b & beta & beta=4 & sigma=3 & n=200 & 40207.11 \\ 
  189 & PWM & beta & beta=4 & sigma=3 & n=200 & 17.45 \\ 
  190 & MLE & sigma & beta=4 & sigma=3 & n=200 & 307.09 \\ 
  191 & MLE.b & sigma & beta=4 & sigma=3 & n=200 & 308.29 \\ 
  192 & LME & sigma & beta=4 & sigma=3 & n=200 & 14.74 \\ 
  193 & MDE.Phi.chisq & sigma & beta=4 & sigma=3 & n=200 & 597.79 \\ 
  194 & MDE.Phi.tv & sigma & beta=4 & sigma=3 & n=200 & 438.33 \\ 
  195 & MDE.Phi.kl & sigma & beta=4 & sigma=3 & n=200 & 32.91 \\ 
  196 & MME & sigma & beta=4 & sigma=3 & n=200 & 474.58 \\ 
  197 & MME.b & sigma & beta=4 & sigma=3 & n=200 & 44484.42 \\ 
  198 & PWM & sigma & beta=4 & sigma=3 & n=200 & 14.74 \\ 
  199 & MLE & beta & beta=5 & sigma=3 & n=200 & 41080.71 \\ 
  200 & MLE.b & beta & beta=5 & sigma=3 & n=200 & 41091.01 \\ 
  201 & LME & beta & beta=5 & sigma=3 & n=200 & 60.69 \\ 
  202 & MDE.Phi.chisq & beta & beta=5 & sigma=3 & n=200 & 990.75 \\ 
  203 & MDE.Phi.tv & beta & beta=5 & sigma=3 & n=200 & 670.90 \\ 
  204 & MDE.Phi.kl & beta & beta=5 & sigma=3 & n=200 & 123.78 \\ 
  205 & MME & beta & beta=5 & sigma=3 & n=200 & 2723.68 \\ 
  206 & MME.b & beta & beta=5 & sigma=3 & n=200 & 30716.43 \\ 
  207 & PWM & beta & beta=5 & sigma=3 & n=200 & 60.69 \\ 
  208 & MLE & sigma & beta=5 & sigma=3 & n=200 & 20188.50 \\ 
  209 & MLE.b & sigma & beta=5 & sigma=3 & n=200 & 20193.59 \\ 
  210 & LME & sigma & beta=5 & sigma=3 & n=200 & 30.83 \\ 
  211 & MDE.Phi.chisq & sigma & beta=5 & sigma=3 & n=200 & 853.36 \\ 
  212 & MDE.Phi.tv & sigma & beta=5 & sigma=3 & n=200 & 548.91 \\ 
  213 & MDE.Phi.kl & sigma & beta=5 & sigma=3 & n=200 & 62.38 \\ 
  214 & MME & sigma & beta=5 & sigma=3 & n=200 & 1332.40 \\ 
  215 & MME.b & sigma & beta=5 & sigma=3 & n=200 & 15637.60 \\ 
  216 & PWM & sigma & beta=5 & sigma=3 & n=200 & 30.83 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220214/20220213-13h27-Full.beta=1.5.sig=1.n=200.LaTeX.tex <==
% START DATE AND TIME=20220213-13h27
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=1.5,  \sigma=1$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.5737&1.4914&1.7059&0.8484&1.0038&1.5737&2.4961&2.2948&1.7059
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
1.0766&0.9904&1.2019&1.1205&1.2518&1.0766&2.7979&2.5193&1.2019
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1006&0.0759&0.1096&0.1218&0.1619&0.1006&0.1638&0.1915&0.1096
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.1062&0.0788&0.1188&0.2199&0.2749&0.1062&4.4084&4.1585&0.1188
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.0737&-0.0086&0.2059&-0.6516&-0.4962&0.0737&0.9961&0.7948&0.2059
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.0766&-0.0096&0.2019&0.1205&0.2518&0.0766&1.7979&1.5193&0.2019
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.106&0.076&0.152&0.5463&0.408&0.106&1.1561&0.8232&0.152
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.1121&0.0789&0.1595&0.2344&0.3383&0.1121&7.6403&6.4663&0.1595
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 0.218&0.1549&0.3115&0.7807&0.7463&0.218&8.7963&7.2895&0.3115\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 6e-04&6e-04&6e-04&0.0343&0.027&6e-04&0.0088&0.0087&6e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220214/20220213-13h27-Full.beta=2.5.sig=1.n=200.LaTeX.tex <==
% START DATE AND TIME=20220213-13h27
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2.5,  \sigma=1$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.7638&2.4525&2.793&2.113&2.3076&2.7639&3.598&3.703&2.793
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
1.1423&0.9738&1.1494&1.3938&1.4264&1.1423&1.6745&1.7171&1.1494
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.0591&0.7475&0.8951&24.1133&17.2888&1.0594&1.7388&977.7111&0.8951
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.3008&0.2095&0.2573&11.8722&8.7277&0.3009&0.5014&315.8387&0.2573
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.2638&-0.0475&0.293&-0.387&-0.1924&0.2639&1.098&1.203&0.293
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.1423&-0.0262&0.1494&0.3938&0.4264&0.1423&0.6745&0.7171&0.1494
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.1286&0.7497&0.9809&24.2607&17.3241&1.1289&2.9444&979.0605&0.9809
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.321&0.2101&0.2795&12.026&8.9086&0.3211&0.9562&316.3213&0.2795
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 1.4496&0.9598&1.2604&36.2868&26.2327&1.4501&3.9006&1295.3818&1.2604\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&6e-04&5e-04&0.0174&0.0121&5e-04&0.0011&0.0017&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220214/20220213-13h27-Full.beta=2.sig=1.n=200.LaTeX.tex <==
% START DATE AND TIME=20220213-13h27
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2,  \sigma=1$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.1509&1.9786&2.2244&1.3674&1.5611&2.1509&2.9788&2.6734&2.2244
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
1.1082&0.9846&1.1505&1.1958&1.2774&1.1082&1.8984&1.6444&1.1505
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.3276&0.2132&0.3063&4.3954&0.8038&0.3276&0.5666&3.8997&0.3063
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.166&0.1074&0.1545&4.5215&0.714&0.166&0.3108&2.0015&0.1545
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1509&-0.0214&0.2244&-0.6326&-0.4389&0.1509&0.9788&0.6734&0.2244
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.1082&-0.0154&0.1505&0.1958&0.2774&0.1082&0.8984&0.6444&0.1505
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.3503&0.2136&0.3566&4.7951&0.9964&0.3503&1.5245&4.3529&0.3566
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.1777&0.1076&0.1771&4.5594&0.7909&0.1777&1.1178&2.4166&0.1771
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 0.528&0.3212&0.5337&9.3545&1.7873&0.528&2.6424&6.7694&0.5337\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&5e-04&5e-04&0.0227&0.0165&5e-04&0.0024&0.0027&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220214/20220213-13h27-Full.beta=3.sig=1.n=200.LaTeX.tex <==
% START DATE AND TIME=20220213-13h27
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=3,  \sigma=1$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 3.4361&2.9785&3.3721&3.3784&3.3403&3.4362&4.3093&6.586&3.3721
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
1.1895&0.9917&1.1544&1.8159&1.6806&1.1895&1.6108&2.5792&1.1544
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 5.864&5.5311&1.8476&112.9598&73.0599&5.8793&9.8172&13779.7265&1.8476
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
1.1678&1.1045&0.3505&36.9241&23.854&1.1711&1.9654&2554.2536&0.3505
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.4361&-0.0215&0.3721&0.3784&0.3403&0.4362&1.3093&3.586&0.3721
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.1895&-0.0083&0.1544&0.8159&0.6806&0.1895&0.6108&1.5792&0.1544
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 6.0537&5.531&1.9859&113.0917&73.1684&6.069&11.5306&13791.2077&1.9859
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
1.2035&1.1045&0.3743&37.586&24.3148&1.2069&2.3382&2556.492&0.3743
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 7.2572&6.6354&2.3602&150.6777&97.4832&7.2759&13.8688&16347.6997&2.3602\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&5e-04&5e-04&0.0143&0.0097&5e-04&7e-04&0.0021&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220214/20220213-13h27-Full.beta=4.sig=1.n=200.LaTeX.tex <==
% START DATE AND TIME=20220213-13h27
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=4,  \sigma=1$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 8.6079&7.9346&4.961&8.2367&7.0632&5.3613&6.6323&36.3872&4.961
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
2.3951&2.1887&1.2877&3.1939&2.5845&1.4128&1.8154&11.1715&1.2877
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 49022.6279&49028.1905&22.9957&614.8822&410.6626&57.7964&366.3062&6124612.719&22.9957
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
4458.5038&4459.0152&2.1439&97.8237&62.0232&5.2062&31.4531&606258.129&2.1439
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 4.6079&3.9346&0.961&4.2367&3.0632&1.3613&2.6323&32.3872&0.961
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
1.3951&1.1887&0.2877&2.1939&1.5845&0.4128&0.8154&10.1715&0.2877
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 49038.9586&49038.7688&23.9168&632.7707&420.0045&59.6438&373.1988&6125049.1898&23.9168
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
4460.0043&4459.9824&2.2265&102.627&64.5276&5.3761&32.1148&606300.9616&2.2265
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 53498.9629&53498.7512&26.1433&735.3977&484.5322&65.0198&405.3136&6731350.1514&26.1433\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&6e-04&5e-04&0.0112&0.0074&5e-04&6e-04&0.0041&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220214/20220213-13h27-Full.beta=5.sig=1.n=200.LaTeX.tex <==
% START DATE AND TIME=20220213-13h27
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=5,  \sigma=1$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 20.5963&19.8909&6.8637&16.0318&12.7153&7.8735&9.9968&21.6294&6.8637
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
4.5957&4.4297&1.4351&4.8519&3.6499&1.6767&2.1886&4.944&1.4351
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 248940.586&248962.9434&74.3458&1568.2084&1070.0281&168.673&1452.5431&17707.6163&74.3458
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
13206.7933&13208.0048&4.2397&149.499&95.7624&9.4045&79.7093&956.6406&4.2397
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 15.5963&14.8909&1.8637&11.0318&7.7153&2.8735&4.9968&16.6294&1.8637
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
3.5957&3.4297&0.4351&3.8519&2.6499&0.6767&1.1886&3.944&0.4351
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 249158.9371&249159.7863&77.8116&1689.7513&1129.4465&176.9134&1477.3657&17982.384&77.8116
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
13218.402&13218.4466&4.4286&164.3214&102.7749&9.8615&81.1142&972.1005&4.4286
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 262377.3391&262378.2329&82.2402&1854.0727&1232.2214&186.7749&1558.4799&18954.4845&82.2402\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&6e-04&5e-04&0.0096&0.0062&5e-04&5e-04&0.0255&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220214/20220213-13h27-Output.accuracy.LaTeX.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Mon Feb 14 08:19:22 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & Measure & beta=1.5 & sigma=1 & n=200 & 0.22 \\ 
  2 & MLE.b & Measure & beta=1.5 & sigma=1 & n=200 & 0.15 \\ 
  3 & LME & Measure & beta=1.5 & sigma=1 & n=200 & 0.31 \\ 
  4 & MDE.Phi.chisq & Measure & beta=1.5 & sigma=1 & n=200 & 0.78 \\ 
  5 & MDE.Phi.tv & Measure & beta=1.5 & sigma=1 & n=200 & 0.75 \\ 
  6 & MDE.Phi.kl & Measure & beta=1.5 & sigma=1 & n=200 & 0.22 \\ 
  7 & MME & Measure & beta=1.5 & sigma=1 & n=200 & 8.80 \\ 
  8 & MME.b & Measure & beta=1.5 & sigma=1 & n=200 & 7.29 \\ 
  9 & PWM & Measure & beta=1.5 & sigma=1 & n=200 & 0.31 \\ 
  10 & MLE & Measure & beta=2 & sigma=1 & n=200 & 0.53 \\ 
  11 & MLE.b & Measure & beta=2 & sigma=1 & n=200 & 0.32 \\ 
  12 & LME & Measure & beta=2 & sigma=1 & n=200 & 0.53 \\ 
  13 & MDE.Phi.chisq & Measure & beta=2 & sigma=1 & n=200 & 9.35 \\ 
  14 & MDE.Phi.tv & Measure & beta=2 & sigma=1 & n=200 & 1.79 \\ 
  15 & MDE.Phi.kl & Measure & beta=2 & sigma=1 & n=200 & 0.53 \\ 
  16 & MME & Measure & beta=2 & sigma=1 & n=200 & 2.64 \\ 
  17 & MME.b & Measure & beta=2 & sigma=1 & n=200 & 6.77 \\ 
  18 & PWM & Measure & beta=2 & sigma=1 & n=200 & 0.53 \\ 
  19 & MLE & Measure & beta=2.5 & sigma=1 & n=200 & 1.45 \\ 
  20 & MLE.b & Measure & beta=2.5 & sigma=1 & n=200 & 0.96 \\ 
  21 & LME & Measure & beta=2.5 & sigma=1 & n=200 & 1.26 \\ 
  22 & MDE.Phi.chisq & Measure & beta=2.5 & sigma=1 & n=200 & 36.29 \\ 
  23 & MDE.Phi.tv & Measure & beta=2.5 & sigma=1 & n=200 & 26.23 \\ 
  24 & MDE.Phi.kl & Measure & beta=2.5 & sigma=1 & n=200 & 1.45 \\ 
  25 & MME & Measure & beta=2.5 & sigma=1 & n=200 & 3.90 \\ 
  26 & MME.b & Measure & beta=2.5 & sigma=1 & n=200 & 1295.38 \\ 
  27 & PWM & Measure & beta=2.5 & sigma=1 & n=200 & 1.26 \\ 
  28 & MLE & Measure & beta=3 & sigma=1 & n=200 & 7.26 \\ 
  29 & MLE.b & Measure & beta=3 & sigma=1 & n=200 & 6.64 \\ 
  30 & LME & Measure & beta=3 & sigma=1 & n=200 & 2.36 \\ 
  31 & MDE.Phi.chisq & Measure & beta=3 & sigma=1 & n=200 & 150.68 \\ 
  32 & MDE.Phi.tv & Measure & beta=3 & sigma=1 & n=200 & 97.48 \\ 
  33 & MDE.Phi.kl & Measure & beta=3 & sigma=1 & n=200 & 7.28 \\ 
  34 & MME & Measure & beta=3 & sigma=1 & n=200 & 13.87 \\ 
  35 & MME.b & Measure & beta=3 & sigma=1 & n=200 & 16347.70 \\ 
  36 & PWM & Measure & beta=3 & sigma=1 & n=200 & 2.36 \\ 
  37 & MLE & Measure & beta=4 & sigma=1 & n=200 & 53498.96 \\ 
  38 & MLE.b & Measure & beta=4 & sigma=1 & n=200 & 53498.75 \\ 
  39 & LME & Measure & beta=4 & sigma=1 & n=200 & 26.14 \\ 
  40 & MDE.Phi.chisq & Measure & beta=4 & sigma=1 & n=200 & 735.40 \\ 
  41 & MDE.Phi.tv & Measure & beta=4 & sigma=1 & n=200 & 484.53 \\ 
  42 & MDE.Phi.kl & Measure & beta=4 & sigma=1 & n=200 & 65.02 \\ 
  43 & MME & Measure & beta=4 & sigma=1 & n=200 & 405.31 \\ 
  44 & MME.b & Measure & beta=4 & sigma=1 & n=200 & 6731350.15 \\ 
  45 & PWM & Measure & beta=4 & sigma=1 & n=200 & 26.14 \\ 
  46 & MLE & Measure & beta=5 & sigma=1 & n=200 & 262377.34 \\ 
  47 & MLE.b & Measure & beta=5 & sigma=1 & n=200 & 262378.23 \\ 
  48 & LME & Measure & beta=5 & sigma=1 & n=200 & 82.24 \\ 
  49 & MDE.Phi.chisq & Measure & beta=5 & sigma=1 & n=200 & 1854.07 \\ 
  50 & MDE.Phi.tv & Measure & beta=5 & sigma=1 & n=200 & 1232.22 \\ 
  51 & MDE.Phi.kl & Measure & beta=5 & sigma=1 & n=200 & 186.77 \\ 
  52 & MME & Measure & beta=5 & sigma=1 & n=200 & 1558.48 \\ 
  53 & MME.b & Measure & beta=5 & sigma=1 & n=200 & 18954.48 \\ 
  54 & PWM & Measure & beta=5 & sigma=1 & n=200 & 82.24 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220214/20220213-13h27-Output.accuracy2.LaTeX.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Mon Feb 14 08:19:22 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & Measure & beta=1.5 & sigma=1 & n=200 & 0.00 \\ 
  2 & MLE.b & Measure & beta=1.5 & sigma=1 & n=200 & 0.00 \\ 
  3 & LME & Measure & beta=1.5 & sigma=1 & n=200 & 0.00 \\ 
  4 & MDE.Phi.chisq & Measure & beta=1.5 & sigma=1 & n=200 & 0.03 \\ 
  5 & MDE.Phi.tv & Measure & beta=1.5 & sigma=1 & n=200 & 0.03 \\ 
  6 & MDE.Phi.kl & Measure & beta=1.5 & sigma=1 & n=200 & 0.00 \\ 
  7 & MME & Measure & beta=1.5 & sigma=1 & n=200 & 0.01 \\ 
  8 & MME.b & Measure & beta=1.5 & sigma=1 & n=200 & 0.01 \\ 
  9 & PWM & Measure & beta=1.5 & sigma=1 & n=200 & 0.00 \\ 
  10 & MLE & Measure & beta=2 & sigma=1 & n=200 & 0.00 \\ 
  11 & MLE.b & Measure & beta=2 & sigma=1 & n=200 & 0.00 \\ 
  12 & LME & Measure & beta=2 & sigma=1 & n=200 & 0.00 \\ 
  13 & MDE.Phi.chisq & Measure & beta=2 & sigma=1 & n=200 & 0.02 \\ 
  14 & MDE.Phi.tv & Measure & beta=2 & sigma=1 & n=200 & 0.02 \\ 
  15 & MDE.Phi.kl & Measure & beta=2 & sigma=1 & n=200 & 0.00 \\ 
  16 & MME & Measure & beta=2 & sigma=1 & n=200 & 0.00 \\ 
  17 & MME.b & Measure & beta=2 & sigma=1 & n=200 & 0.00 \\ 
  18 & PWM & Measure & beta=2 & sigma=1 & n=200 & 0.00 \\ 
  19 & MLE & Measure & beta=2.5 & sigma=1 & n=200 & 0.00 \\ 
  20 & MLE.b & Measure & beta=2.5 & sigma=1 & n=200 & 0.00 \\ 
  21 & LME & Measure & beta=2.5 & sigma=1 & n=200 & 0.00 \\ 
  22 & MDE.Phi.chisq & Measure & beta=2.5 & sigma=1 & n=200 & 0.02 \\ 
  23 & MDE.Phi.tv & Measure & beta=2.5 & sigma=1 & n=200 & 0.01 \\ 
  24 & MDE.Phi.kl & Measure & beta=2.5 & sigma=1 & n=200 & 0.00 \\ 
  25 & MME & Measure & beta=2.5 & sigma=1 & n=200 & 0.00 \\ 
  26 & MME.b & Measure & beta=2.5 & sigma=1 & n=200 & 0.00 \\ 
  27 & PWM & Measure & beta=2.5 & sigma=1 & n=200 & 0.00 \\ 
  28 & MLE & Measure & beta=3 & sigma=1 & n=200 & 0.00 \\ 
  29 & MLE.b & Measure & beta=3 & sigma=1 & n=200 & 0.00 \\ 
  30 & LME & Measure & beta=3 & sigma=1 & n=200 & 0.00 \\ 
  31 & MDE.Phi.chisq & Measure & beta=3 & sigma=1 & n=200 & 0.01 \\ 
  32 & MDE.Phi.tv & Measure & beta=3 & sigma=1 & n=200 & 0.01 \\ 
  33 & MDE.Phi.kl & Measure & beta=3 & sigma=1 & n=200 & 0.00 \\ 
  34 & MME & Measure & beta=3 & sigma=1 & n=200 & 0.00 \\ 
  35 & MME.b & Measure & beta=3 & sigma=1 & n=200 & 0.00 \\ 
  36 & PWM & Measure & beta=3 & sigma=1 & n=200 & 0.00 \\ 
  37 & MLE & Measure & beta=4 & sigma=1 & n=200 & 0.00 \\ 
  38 & MLE.b & Measure & beta=4 & sigma=1 & n=200 & 0.00 \\ 
  39 & LME & Measure & beta=4 & sigma=1 & n=200 & 0.00 \\ 
  40 & MDE.Phi.chisq & Measure & beta=4 & sigma=1 & n=200 & 0.01 \\ 
  41 & MDE.Phi.tv & Measure & beta=4 & sigma=1 & n=200 & 0.01 \\ 
  42 & MDE.Phi.kl & Measure & beta=4 & sigma=1 & n=200 & 0.00 \\ 
  43 & MME & Measure & beta=4 & sigma=1 & n=200 & 0.00 \\ 
  44 & MME.b & Measure & beta=4 & sigma=1 & n=200 & 0.00 \\ 
  45 & PWM & Measure & beta=4 & sigma=1 & n=200 & 0.00 \\ 
  46 & MLE & Measure & beta=5 & sigma=1 & n=200 & 0.00 \\ 
  47 & MLE.b & Measure & beta=5 & sigma=1 & n=200 & 0.00 \\ 
  48 & LME & Measure & beta=5 & sigma=1 & n=200 & 0.00 \\ 
  49 & MDE.Phi.chisq & Measure & beta=5 & sigma=1 & n=200 & 0.01 \\ 
  50 & MDE.Phi.tv & Measure & beta=5 & sigma=1 & n=200 & 0.01 \\ 
  51 & MDE.Phi.kl & Measure & beta=5 & sigma=1 & n=200 & 0.00 \\ 
  52 & MME & Measure & beta=5 & sigma=1 & n=200 & 0.00 \\ 
  53 & MME.b & Measure & beta=5 & sigma=1 & n=200 & 0.03 \\ 
  54 & PWM & Measure & beta=5 & sigma=1 & n=200 & 0.00 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220214/20220213-13h27-Output.bias.LaTeX.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Mon Feb 14 08:19:22 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=1 & n=200 & 0.07 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=1 & n=200 & -0.01 \\ 
  3 & LME & beta & beta=1.5 & sigma=1 & n=200 & 0.21 \\ 
  4 & MDE.Phi.chisq & beta & beta=1.5 & sigma=1 & n=200 & -0.65 \\ 
  5 & MDE.Phi.tv & beta & beta=1.5 & sigma=1 & n=200 & -0.50 \\ 
  6 & MDE.Phi.kl & beta & beta=1.5 & sigma=1 & n=200 & 0.07 \\ 
  7 & MME & beta & beta=1.5 & sigma=1 & n=200 & 1.00 \\ 
  8 & MME.b & beta & beta=1.5 & sigma=1 & n=200 & 0.79 \\ 
  9 & PWM & beta & beta=1.5 & sigma=1 & n=200 & 0.21 \\ 
  10 & MLE & sigma & beta=1.5 & sigma=1 & n=200 & 0.08 \\ 
  11 & MLE.b & sigma & beta=1.5 & sigma=1 & n=200 & -0.01 \\ 
  12 & LME & sigma & beta=1.5 & sigma=1 & n=200 & 0.20 \\ 
  13 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=1 & n=200 & 0.12 \\ 
  14 & MDE.Phi.tv & sigma & beta=1.5 & sigma=1 & n=200 & 0.25 \\ 
  15 & MDE.Phi.kl & sigma & beta=1.5 & sigma=1 & n=200 & 0.08 \\ 
  16 & MME & sigma & beta=1.5 & sigma=1 & n=200 & 1.80 \\ 
  17 & MME.b & sigma & beta=1.5 & sigma=1 & n=200 & 1.52 \\ 
  18 & PWM & sigma & beta=1.5 & sigma=1 & n=200 & 0.20 \\ 
  19 & MLE & beta & beta=2 & sigma=1 & n=200 & 0.15 \\ 
  20 & MLE.b & beta & beta=2 & sigma=1 & n=200 & -0.02 \\ 
  21 & LME & beta & beta=2 & sigma=1 & n=200 & 0.22 \\ 
  22 & MDE.Phi.chisq & beta & beta=2 & sigma=1 & n=200 & -0.63 \\ 
  23 & MDE.Phi.tv & beta & beta=2 & sigma=1 & n=200 & -0.44 \\ 
  24 & MDE.Phi.kl & beta & beta=2 & sigma=1 & n=200 & 0.15 \\ 
  25 & MME & beta & beta=2 & sigma=1 & n=200 & 0.98 \\ 
  26 & MME.b & beta & beta=2 & sigma=1 & n=200 & 0.67 \\ 
  27 & PWM & beta & beta=2 & sigma=1 & n=200 & 0.22 \\ 
  28 & MLE & sigma & beta=2 & sigma=1 & n=200 & 0.11 \\ 
  29 & MLE.b & sigma & beta=2 & sigma=1 & n=200 & -0.02 \\ 
  30 & LME & sigma & beta=2 & sigma=1 & n=200 & 0.15 \\ 
  31 & MDE.Phi.chisq & sigma & beta=2 & sigma=1 & n=200 & 0.20 \\ 
  32 & MDE.Phi.tv & sigma & beta=2 & sigma=1 & n=200 & 0.28 \\ 
  33 & MDE.Phi.kl & sigma & beta=2 & sigma=1 & n=200 & 0.11 \\ 
  34 & MME & sigma & beta=2 & sigma=1 & n=200 & 0.90 \\ 
  35 & MME.b & sigma & beta=2 & sigma=1 & n=200 & 0.64 \\ 
  36 & PWM & sigma & beta=2 & sigma=1 & n=200 & 0.15 \\ 
  37 & MLE & beta & beta=2.5 & sigma=1 & n=200 & 0.26 \\ 
  38 & MLE.b & beta & beta=2.5 & sigma=1 & n=200 & -0.05 \\ 
  39 & LME & beta & beta=2.5 & sigma=1 & n=200 & 0.29 \\ 
  40 & MDE.Phi.chisq & beta & beta=2.5 & sigma=1 & n=200 & -0.39 \\ 
  41 & MDE.Phi.tv & beta & beta=2.5 & sigma=1 & n=200 & -0.19 \\ 
  42 & MDE.Phi.kl & beta & beta=2.5 & sigma=1 & n=200 & 0.26 \\ 
  43 & MME & beta & beta=2.5 & sigma=1 & n=200 & 1.10 \\ 
  44 & MME.b & beta & beta=2.5 & sigma=1 & n=200 & 1.20 \\ 
  45 & PWM & beta & beta=2.5 & sigma=1 & n=200 & 0.29 \\ 
  46 & MLE & sigma & beta=2.5 & sigma=1 & n=200 & 0.14 \\ 
  47 & MLE.b & sigma & beta=2.5 & sigma=1 & n=200 & -0.03 \\ 
  48 & LME & sigma & beta=2.5 & sigma=1 & n=200 & 0.15 \\ 
  49 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=1 & n=200 & 0.39 \\ 
  50 & MDE.Phi.tv & sigma & beta=2.5 & sigma=1 & n=200 & 0.43 \\ 
  51 & MDE.Phi.kl & sigma & beta=2.5 & sigma=1 & n=200 & 0.14 \\ 
  52 & MME & sigma & beta=2.5 & sigma=1 & n=200 & 0.67 \\ 
  53 & MME.b & sigma & beta=2.5 & sigma=1 & n=200 & 0.72 \\ 
  54 & PWM & sigma & beta=2.5 & sigma=1 & n=200 & 0.15 \\ 
  55 & MLE & beta & beta=3 & sigma=1 & n=200 & 0.44 \\ 
  56 & MLE.b & beta & beta=3 & sigma=1 & n=200 & -0.02 \\ 
  57 & LME & beta & beta=3 & sigma=1 & n=200 & 0.37 \\ 
  58 & MDE.Phi.chisq & beta & beta=3 & sigma=1 & n=200 & 0.38 \\ 
  59 & MDE.Phi.tv & beta & beta=3 & sigma=1 & n=200 & 0.34 \\ 
  60 & MDE.Phi.kl & beta & beta=3 & sigma=1 & n=200 & 0.44 \\ 
  61 & MME & beta & beta=3 & sigma=1 & n=200 & 1.31 \\ 
  62 & MME.b & beta & beta=3 & sigma=1 & n=200 & 3.59 \\ 
  63 & PWM & beta & beta=3 & sigma=1 & n=200 & 0.37 \\ 
  64 & MLE & sigma & beta=3 & sigma=1 & n=200 & 0.19 \\ 
  65 & MLE.b & sigma & beta=3 & sigma=1 & n=200 & -0.01 \\ 
  66 & LME & sigma & beta=3 & sigma=1 & n=200 & 0.15 \\ 
  67 & MDE.Phi.chisq & sigma & beta=3 & sigma=1 & n=200 & 0.82 \\ 
  68 & MDE.Phi.tv & sigma & beta=3 & sigma=1 & n=200 & 0.68 \\ 
  69 & MDE.Phi.kl & sigma & beta=3 & sigma=1 & n=200 & 0.19 \\ 
  70 & MME & sigma & beta=3 & sigma=1 & n=200 & 0.61 \\ 
  71 & MME.b & sigma & beta=3 & sigma=1 & n=200 & 1.58 \\ 
  72 & PWM & sigma & beta=3 & sigma=1 & n=200 & 0.15 \\ 
  73 & MLE & beta & beta=4 & sigma=1 & n=200 & 4.61 \\ 
  74 & MLE.b & beta & beta=4 & sigma=1 & n=200 & 3.93 \\ 
  75 & LME & beta & beta=4 & sigma=1 & n=200 & 0.96 \\ 
  76 & MDE.Phi.chisq & beta & beta=4 & sigma=1 & n=200 & 4.24 \\ 
  77 & MDE.Phi.tv & beta & beta=4 & sigma=1 & n=200 & 3.06 \\ 
  78 & MDE.Phi.kl & beta & beta=4 & sigma=1 & n=200 & 1.36 \\ 
  79 & MME & beta & beta=4 & sigma=1 & n=200 & 2.63 \\ 
  80 & MME.b & beta & beta=4 & sigma=1 & n=200 & 32.39 \\ 
  81 & PWM & beta & beta=4 & sigma=1 & n=200 & 0.96 \\ 
  82 & MLE & sigma & beta=4 & sigma=1 & n=200 & 1.40 \\ 
  83 & MLE.b & sigma & beta=4 & sigma=1 & n=200 & 1.19 \\ 
  84 & LME & sigma & beta=4 & sigma=1 & n=200 & 0.29 \\ 
  85 & MDE.Phi.chisq & sigma & beta=4 & sigma=1 & n=200 & 2.19 \\ 
  86 & MDE.Phi.tv & sigma & beta=4 & sigma=1 & n=200 & 1.58 \\ 
  87 & MDE.Phi.kl & sigma & beta=4 & sigma=1 & n=200 & 0.41 \\ 
  88 & MME & sigma & beta=4 & sigma=1 & n=200 & 0.82 \\ 
  89 & MME.b & sigma & beta=4 & sigma=1 & n=200 & 10.17 \\ 
  90 & PWM & sigma & beta=4 & sigma=1 & n=200 & 0.29 \\ 
  91 & MLE & beta & beta=5 & sigma=1 & n=200 & 15.60 \\ 
  92 & MLE.b & beta & beta=5 & sigma=1 & n=200 & 14.89 \\ 
  93 & LME & beta & beta=5 & sigma=1 & n=200 & 1.86 \\ 
  94 & MDE.Phi.chisq & beta & beta=5 & sigma=1 & n=200 & 11.03 \\ 
  95 & MDE.Phi.tv & beta & beta=5 & sigma=1 & n=200 & 7.72 \\ 
  96 & MDE.Phi.kl & beta & beta=5 & sigma=1 & n=200 & 2.87 \\ 
  97 & MME & beta & beta=5 & sigma=1 & n=200 & 5.00 \\ 
  98 & MME.b & beta & beta=5 & sigma=1 & n=200 & 16.63 \\ 
  99 & PWM & beta & beta=5 & sigma=1 & n=200 & 1.86 \\ 
  100 & MLE & sigma & beta=5 & sigma=1 & n=200 & 3.60 \\ 
  101 & MLE.b & sigma & beta=5 & sigma=1 & n=200 & 3.43 \\ 
  102 & LME & sigma & beta=5 & sigma=1 & n=200 & 0.44 \\ 
  103 & MDE.Phi.chisq & sigma & beta=5 & sigma=1 & n=200 & 3.85 \\ 
  104 & MDE.Phi.tv & sigma & beta=5 & sigma=1 & n=200 & 2.65 \\ 
  105 & MDE.Phi.kl & sigma & beta=5 & sigma=1 & n=200 & 0.68 \\ 
  106 & MME & sigma & beta=5 & sigma=1 & n=200 & 1.19 \\ 
  107 & MME.b & sigma & beta=5 & sigma=1 & n=200 & 3.94 \\ 
  108 & PWM & sigma & beta=5 & sigma=1 & n=200 & 0.44 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220214/20220213-13h27-Output.mean.LaTeX.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Mon Feb 14 08:19:22 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=1 & n=200 & 1.57 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=1 & n=200 & 1.49 \\ 
  3 & LME & beta & beta=1.5 & sigma=1 & n=200 & 1.71 \\ 
  4 & MDE.Phi.chisq & beta & beta=1.5 & sigma=1 & n=200 & 0.85 \\ 
  5 & MDE.Phi.tv & beta & beta=1.5 & sigma=1 & n=200 & 1.00 \\ 
  6 & MDE.Phi.kl & beta & beta=1.5 & sigma=1 & n=200 & 1.57 \\ 
  7 & MME & beta & beta=1.5 & sigma=1 & n=200 & 2.50 \\ 
  8 & MME.b & beta & beta=1.5 & sigma=1 & n=200 & 2.29 \\ 
  9 & PWM & beta & beta=1.5 & sigma=1 & n=200 & 1.71 \\ 
  10 & MLE & sigma & beta=1.5 & sigma=1 & n=200 & 1.08 \\ 
  11 & MLE.b & sigma & beta=1.5 & sigma=1 & n=200 & 0.99 \\ 
  12 & LME & sigma & beta=1.5 & sigma=1 & n=200 & 1.20 \\ 
  13 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=1 & n=200 & 1.12 \\ 
  14 & MDE.Phi.tv & sigma & beta=1.5 & sigma=1 & n=200 & 1.25 \\ 
  15 & MDE.Phi.kl & sigma & beta=1.5 & sigma=1 & n=200 & 1.08 \\ 
  16 & MME & sigma & beta=1.5 & sigma=1 & n=200 & 2.80 \\ 
  17 & MME.b & sigma & beta=1.5 & sigma=1 & n=200 & 2.52 \\ 
  18 & PWM & sigma & beta=1.5 & sigma=1 & n=200 & 1.20 \\ 
  19 & MLE & beta & beta=2 & sigma=1 & n=200 & 2.15 \\ 
  20 & MLE.b & beta & beta=2 & sigma=1 & n=200 & 1.98 \\ 
  21 & LME & beta & beta=2 & sigma=1 & n=200 & 2.22 \\ 
  22 & MDE.Phi.chisq & beta & beta=2 & sigma=1 & n=200 & 1.37 \\ 
  23 & MDE.Phi.tv & beta & beta=2 & sigma=1 & n=200 & 1.56 \\ 
  24 & MDE.Phi.kl & beta & beta=2 & sigma=1 & n=200 & 2.15 \\ 
  25 & MME & beta & beta=2 & sigma=1 & n=200 & 2.98 \\ 
  26 & MME.b & beta & beta=2 & sigma=1 & n=200 & 2.67 \\ 
  27 & PWM & beta & beta=2 & sigma=1 & n=200 & 2.22 \\ 
  28 & MLE & sigma & beta=2 & sigma=1 & n=200 & 1.11 \\ 
  29 & MLE.b & sigma & beta=2 & sigma=1 & n=200 & 0.98 \\ 
  30 & LME & sigma & beta=2 & sigma=1 & n=200 & 1.15 \\ 
  31 & MDE.Phi.chisq & sigma & beta=2 & sigma=1 & n=200 & 1.20 \\ 
  32 & MDE.Phi.tv & sigma & beta=2 & sigma=1 & n=200 & 1.28 \\ 
  33 & MDE.Phi.kl & sigma & beta=2 & sigma=1 & n=200 & 1.11 \\ 
  34 & MME & sigma & beta=2 & sigma=1 & n=200 & 1.90 \\ 
  35 & MME.b & sigma & beta=2 & sigma=1 & n=200 & 1.64 \\ 
  36 & PWM & sigma & beta=2 & sigma=1 & n=200 & 1.15 \\ 
  37 & MLE & beta & beta=2.5 & sigma=1 & n=200 & 2.76 \\ 
  38 & MLE.b & beta & beta=2.5 & sigma=1 & n=200 & 2.45 \\ 
  39 & LME & beta & beta=2.5 & sigma=1 & n=200 & 2.79 \\ 
  40 & MDE.Phi.chisq & beta & beta=2.5 & sigma=1 & n=200 & 2.11 \\ 
  41 & MDE.Phi.tv & beta & beta=2.5 & sigma=1 & n=200 & 2.31 \\ 
  42 & MDE.Phi.kl & beta & beta=2.5 & sigma=1 & n=200 & 2.76 \\ 
  43 & MME & beta & beta=2.5 & sigma=1 & n=200 & 3.60 \\ 
  44 & MME.b & beta & beta=2.5 & sigma=1 & n=200 & 3.70 \\ 
  45 & PWM & beta & beta=2.5 & sigma=1 & n=200 & 2.79 \\ 
  46 & MLE & sigma & beta=2.5 & sigma=1 & n=200 & 1.14 \\ 
  47 & MLE.b & sigma & beta=2.5 & sigma=1 & n=200 & 0.97 \\ 
  48 & LME & sigma & beta=2.5 & sigma=1 & n=200 & 1.15 \\ 
  49 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=1 & n=200 & 1.39 \\ 
  50 & MDE.Phi.tv & sigma & beta=2.5 & sigma=1 & n=200 & 1.43 \\ 
  51 & MDE.Phi.kl & sigma & beta=2.5 & sigma=1 & n=200 & 1.14 \\ 
  52 & MME & sigma & beta=2.5 & sigma=1 & n=200 & 1.67 \\ 
  53 & MME.b & sigma & beta=2.5 & sigma=1 & n=200 & 1.72 \\ 
  54 & PWM & sigma & beta=2.5 & sigma=1 & n=200 & 1.15 \\ 
  55 & MLE & beta & beta=3 & sigma=1 & n=200 & 3.44 \\ 
  56 & MLE.b & beta & beta=3 & sigma=1 & n=200 & 2.98 \\ 
  57 & LME & beta & beta=3 & sigma=1 & n=200 & 3.37 \\ 
  58 & MDE.Phi.chisq & beta & beta=3 & sigma=1 & n=200 & 3.38 \\ 
  59 & MDE.Phi.tv & beta & beta=3 & sigma=1 & n=200 & 3.34 \\ 
  60 & MDE.Phi.kl & beta & beta=3 & sigma=1 & n=200 & 3.44 \\ 
  61 & MME & beta & beta=3 & sigma=1 & n=200 & 4.31 \\ 
  62 & MME.b & beta & beta=3 & sigma=1 & n=200 & 6.59 \\ 
  63 & PWM & beta & beta=3 & sigma=1 & n=200 & 3.37 \\ 
  64 & MLE & sigma & beta=3 & sigma=1 & n=200 & 1.19 \\ 
  65 & MLE.b & sigma & beta=3 & sigma=1 & n=200 & 0.99 \\ 
  66 & LME & sigma & beta=3 & sigma=1 & n=200 & 1.15 \\ 
  67 & MDE.Phi.chisq & sigma & beta=3 & sigma=1 & n=200 & 1.82 \\ 
  68 & MDE.Phi.tv & sigma & beta=3 & sigma=1 & n=200 & 1.68 \\ 
  69 & MDE.Phi.kl & sigma & beta=3 & sigma=1 & n=200 & 1.19 \\ 
  70 & MME & sigma & beta=3 & sigma=1 & n=200 & 1.61 \\ 
  71 & MME.b & sigma & beta=3 & sigma=1 & n=200 & 2.58 \\ 
  72 & PWM & sigma & beta=3 & sigma=1 & n=200 & 1.15 \\ 
  73 & MLE & beta & beta=4 & sigma=1 & n=200 & 8.61 \\ 
  74 & MLE.b & beta & beta=4 & sigma=1 & n=200 & 7.93 \\ 
  75 & LME & beta & beta=4 & sigma=1 & n=200 & 4.96 \\ 
  76 & MDE.Phi.chisq & beta & beta=4 & sigma=1 & n=200 & 8.24 \\ 
  77 & MDE.Phi.tv & beta & beta=4 & sigma=1 & n=200 & 7.06 \\ 
  78 & MDE.Phi.kl & beta & beta=4 & sigma=1 & n=200 & 5.36 \\ 
  79 & MME & beta & beta=4 & sigma=1 & n=200 & 6.63 \\ 
  80 & MME.b & beta & beta=4 & sigma=1 & n=200 & 36.39 \\ 
  81 & PWM & beta & beta=4 & sigma=1 & n=200 & 4.96 \\ 
  82 & MLE & sigma & beta=4 & sigma=1 & n=200 & 2.40 \\ 
  83 & MLE.b & sigma & beta=4 & sigma=1 & n=200 & 2.19 \\ 
  84 & LME & sigma & beta=4 & sigma=1 & n=200 & 1.29 \\ 
  85 & MDE.Phi.chisq & sigma & beta=4 & sigma=1 & n=200 & 3.19 \\ 
  86 & MDE.Phi.tv & sigma & beta=4 & sigma=1 & n=200 & 2.58 \\ 
  87 & MDE.Phi.kl & sigma & beta=4 & sigma=1 & n=200 & 1.41 \\ 
  88 & MME & sigma & beta=4 & sigma=1 & n=200 & 1.82 \\ 
  89 & MME.b & sigma & beta=4 & sigma=1 & n=200 & 11.17 \\ 
  90 & PWM & sigma & beta=4 & sigma=1 & n=200 & 1.29 \\ 
  91 & MLE & beta & beta=5 & sigma=1 & n=200 & 20.60 \\ 
  92 & MLE.b & beta & beta=5 & sigma=1 & n=200 & 19.89 \\ 
  93 & LME & beta & beta=5 & sigma=1 & n=200 & 6.86 \\ 
  94 & MDE.Phi.chisq & beta & beta=5 & sigma=1 & n=200 & 16.03 \\ 
  95 & MDE.Phi.tv & beta & beta=5 & sigma=1 & n=200 & 12.72 \\ 
  96 & MDE.Phi.kl & beta & beta=5 & sigma=1 & n=200 & 7.87 \\ 
  97 & MME & beta & beta=5 & sigma=1 & n=200 & 10.00 \\ 
  98 & MME.b & beta & beta=5 & sigma=1 & n=200 & 21.63 \\ 
  99 & PWM & beta & beta=5 & sigma=1 & n=200 & 6.86 \\ 
  100 & MLE & sigma & beta=5 & sigma=1 & n=200 & 4.60 \\ 
  101 & MLE.b & sigma & beta=5 & sigma=1 & n=200 & 4.43 \\ 
  102 & LME & sigma & beta=5 & sigma=1 & n=200 & 1.44 \\ 
  103 & MDE.Phi.chisq & sigma & beta=5 & sigma=1 & n=200 & 4.85 \\ 
  104 & MDE.Phi.tv & sigma & beta=5 & sigma=1 & n=200 & 3.65 \\ 
  105 & MDE.Phi.kl & sigma & beta=5 & sigma=1 & n=200 & 1.68 \\ 
  106 & MME & sigma & beta=5 & sigma=1 & n=200 & 2.19 \\ 
  107 & MME.b & sigma & beta=5 & sigma=1 & n=200 & 4.94 \\ 
  108 & PWM & sigma & beta=5 & sigma=1 & n=200 & 1.44 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220214/20220213-13h27-Output.mse.LaTeX.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Mon Feb 14 08:19:22 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=1 & n=200 & 0.11 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=1 & n=200 & 0.08 \\ 
  3 & LME & beta & beta=1.5 & sigma=1 & n=200 & 0.15 \\ 
  4 & MDE.Phi.chisq & beta & beta=1.5 & sigma=1 & n=200 & 0.55 \\ 
  5 & MDE.Phi.tv & beta & beta=1.5 & sigma=1 & n=200 & 0.41 \\ 
  6 & MDE.Phi.kl & beta & beta=1.5 & sigma=1 & n=200 & 0.11 \\ 
  7 & MME & beta & beta=1.5 & sigma=1 & n=200 & 1.16 \\ 
  8 & MME.b & beta & beta=1.5 & sigma=1 & n=200 & 0.82 \\ 
  9 & PWM & beta & beta=1.5 & sigma=1 & n=200 & 0.15 \\ 
  10 & MLE & sigma & beta=1.5 & sigma=1 & n=200 & 0.11 \\ 
  11 & MLE.b & sigma & beta=1.5 & sigma=1 & n=200 & 0.08 \\ 
  12 & LME & sigma & beta=1.5 & sigma=1 & n=200 & 0.16 \\ 
  13 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=1 & n=200 & 0.23 \\ 
  14 & MDE.Phi.tv & sigma & beta=1.5 & sigma=1 & n=200 & 0.34 \\ 
  15 & MDE.Phi.kl & sigma & beta=1.5 & sigma=1 & n=200 & 0.11 \\ 
  16 & MME & sigma & beta=1.5 & sigma=1 & n=200 & 7.64 \\ 
  17 & MME.b & sigma & beta=1.5 & sigma=1 & n=200 & 6.47 \\ 
  18 & PWM & sigma & beta=1.5 & sigma=1 & n=200 & 0.16 \\ 
  19 & MLE & beta & beta=2 & sigma=1 & n=200 & 0.35 \\ 
  20 & MLE.b & beta & beta=2 & sigma=1 & n=200 & 0.21 \\ 
  21 & LME & beta & beta=2 & sigma=1 & n=200 & 0.36 \\ 
  22 & MDE.Phi.chisq & beta & beta=2 & sigma=1 & n=200 & 4.80 \\ 
  23 & MDE.Phi.tv & beta & beta=2 & sigma=1 & n=200 & 1.00 \\ 
  24 & MDE.Phi.kl & beta & beta=2 & sigma=1 & n=200 & 0.35 \\ 
  25 & MME & beta & beta=2 & sigma=1 & n=200 & 1.52 \\ 
  26 & MME.b & beta & beta=2 & sigma=1 & n=200 & 4.35 \\ 
  27 & PWM & beta & beta=2 & sigma=1 & n=200 & 0.36 \\ 
  28 & MLE & sigma & beta=2 & sigma=1 & n=200 & 0.18 \\ 
  29 & MLE.b & sigma & beta=2 & sigma=1 & n=200 & 0.11 \\ 
  30 & LME & sigma & beta=2 & sigma=1 & n=200 & 0.18 \\ 
  31 & MDE.Phi.chisq & sigma & beta=2 & sigma=1 & n=200 & 4.56 \\ 
  32 & MDE.Phi.tv & sigma & beta=2 & sigma=1 & n=200 & 0.79 \\ 
  33 & MDE.Phi.kl & sigma & beta=2 & sigma=1 & n=200 & 0.18 \\ 
  34 & MME & sigma & beta=2 & sigma=1 & n=200 & 1.12 \\ 
  35 & MME.b & sigma & beta=2 & sigma=1 & n=200 & 2.42 \\ 
  36 & PWM & sigma & beta=2 & sigma=1 & n=200 & 0.18 \\ 
  37 & MLE & beta & beta=2.5 & sigma=1 & n=200 & 1.13 \\ 
  38 & MLE.b & beta & beta=2.5 & sigma=1 & n=200 & 0.75 \\ 
  39 & LME & beta & beta=2.5 & sigma=1 & n=200 & 0.98 \\ 
  40 & MDE.Phi.chisq & beta & beta=2.5 & sigma=1 & n=200 & 24.26 \\ 
  41 & MDE.Phi.tv & beta & beta=2.5 & sigma=1 & n=200 & 17.32 \\ 
  42 & MDE.Phi.kl & beta & beta=2.5 & sigma=1 & n=200 & 1.13 \\ 
  43 & MME & beta & beta=2.5 & sigma=1 & n=200 & 2.94 \\ 
  44 & MME.b & beta & beta=2.5 & sigma=1 & n=200 & 979.06 \\ 
  45 & PWM & beta & beta=2.5 & sigma=1 & n=200 & 0.98 \\ 
  46 & MLE & sigma & beta=2.5 & sigma=1 & n=200 & 0.32 \\ 
  47 & MLE.b & sigma & beta=2.5 & sigma=1 & n=200 & 0.21 \\ 
  48 & LME & sigma & beta=2.5 & sigma=1 & n=200 & 0.28 \\ 
  49 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=1 & n=200 & 12.03 \\ 
  50 & MDE.Phi.tv & sigma & beta=2.5 & sigma=1 & n=200 & 8.91 \\ 
  51 & MDE.Phi.kl & sigma & beta=2.5 & sigma=1 & n=200 & 0.32 \\ 
  52 & MME & sigma & beta=2.5 & sigma=1 & n=200 & 0.96 \\ 
  53 & MME.b & sigma & beta=2.5 & sigma=1 & n=200 & 316.32 \\ 
  54 & PWM & sigma & beta=2.5 & sigma=1 & n=200 & 0.28 \\ 
  55 & MLE & beta & beta=3 & sigma=1 & n=200 & 6.05 \\ 
  56 & MLE.b & beta & beta=3 & sigma=1 & n=200 & 5.53 \\ 
  57 & LME & beta & beta=3 & sigma=1 & n=200 & 1.99 \\ 
  58 & MDE.Phi.chisq & beta & beta=3 & sigma=1 & n=200 & 113.09 \\ 
  59 & MDE.Phi.tv & beta & beta=3 & sigma=1 & n=200 & 73.17 \\ 
  60 & MDE.Phi.kl & beta & beta=3 & sigma=1 & n=200 & 6.07 \\ 
  61 & MME & beta & beta=3 & sigma=1 & n=200 & 11.53 \\ 
  62 & MME.b & beta & beta=3 & sigma=1 & n=200 & 13791.21 \\ 
  63 & PWM & beta & beta=3 & sigma=1 & n=200 & 1.99 \\ 
  64 & MLE & sigma & beta=3 & sigma=1 & n=200 & 1.20 \\ 
  65 & MLE.b & sigma & beta=3 & sigma=1 & n=200 & 1.10 \\ 
  66 & LME & sigma & beta=3 & sigma=1 & n=200 & 0.37 \\ 
  67 & MDE.Phi.chisq & sigma & beta=3 & sigma=1 & n=200 & 37.59 \\ 
  68 & MDE.Phi.tv & sigma & beta=3 & sigma=1 & n=200 & 24.31 \\ 
  69 & MDE.Phi.kl & sigma & beta=3 & sigma=1 & n=200 & 1.21 \\ 
  70 & MME & sigma & beta=3 & sigma=1 & n=200 & 2.34 \\ 
  71 & MME.b & sigma & beta=3 & sigma=1 & n=200 & 2556.49 \\ 
  72 & PWM & sigma & beta=3 & sigma=1 & n=200 & 0.37 \\ 
  73 & MLE & beta & beta=4 & sigma=1 & n=200 & 49038.96 \\ 
  74 & MLE.b & beta & beta=4 & sigma=1 & n=200 & 49038.77 \\ 
  75 & LME & beta & beta=4 & sigma=1 & n=200 & 23.92 \\ 
  76 & MDE.Phi.chisq & beta & beta=4 & sigma=1 & n=200 & 632.77 \\ 
  77 & MDE.Phi.tv & beta & beta=4 & sigma=1 & n=200 & 420.00 \\ 
  78 & MDE.Phi.kl & beta & beta=4 & sigma=1 & n=200 & 59.64 \\ 
  79 & MME & beta & beta=4 & sigma=1 & n=200 & 373.20 \\ 
  80 & MME.b & beta & beta=4 & sigma=1 & n=200 & 6125049.19 \\ 
  81 & PWM & beta & beta=4 & sigma=1 & n=200 & 23.92 \\ 
  82 & MLE & sigma & beta=4 & sigma=1 & n=200 & 4460.00 \\ 
  83 & MLE.b & sigma & beta=4 & sigma=1 & n=200 & 4459.98 \\ 
  84 & LME & sigma & beta=4 & sigma=1 & n=200 & 2.23 \\ 
  85 & MDE.Phi.chisq & sigma & beta=4 & sigma=1 & n=200 & 102.63 \\ 
  86 & MDE.Phi.tv & sigma & beta=4 & sigma=1 & n=200 & 64.53 \\ 
  87 & MDE.Phi.kl & sigma & beta=4 & sigma=1 & n=200 & 5.38 \\ 
  88 & MME & sigma & beta=4 & sigma=1 & n=200 & 32.11 \\ 
  89 & MME.b & sigma & beta=4 & sigma=1 & n=200 & 606300.96 \\ 
  90 & PWM & sigma & beta=4 & sigma=1 & n=200 & 2.23 \\ 
  91 & MLE & beta & beta=5 & sigma=1 & n=200 & 249158.94 \\ 
  92 & MLE.b & beta & beta=5 & sigma=1 & n=200 & 249159.79 \\ 
  93 & LME & beta & beta=5 & sigma=1 & n=200 & 77.81 \\ 
  94 & MDE.Phi.chisq & beta & beta=5 & sigma=1 & n=200 & 1689.75 \\ 
  95 & MDE.Phi.tv & beta & beta=5 & sigma=1 & n=200 & 1129.45 \\ 
  96 & MDE.Phi.kl & beta & beta=5 & sigma=1 & n=200 & 176.91 \\ 
  97 & MME & beta & beta=5 & sigma=1 & n=200 & 1477.37 \\ 
  98 & MME.b & beta & beta=5 & sigma=1 & n=200 & 17982.38 \\ 
  99 & PWM & beta & beta=5 & sigma=1 & n=200 & 77.81 \\ 
  100 & MLE & sigma & beta=5 & sigma=1 & n=200 & 13218.40 \\ 
  101 & MLE.b & sigma & beta=5 & sigma=1 & n=200 & 13218.45 \\ 
  102 & LME & sigma & beta=5 & sigma=1 & n=200 & 4.43 \\ 
  103 & MDE.Phi.chisq & sigma & beta=5 & sigma=1 & n=200 & 164.32 \\ 
  104 & MDE.Phi.tv & sigma & beta=5 & sigma=1 & n=200 & 102.77 \\ 
  105 & MDE.Phi.kl & sigma & beta=5 & sigma=1 & n=200 & 9.86 \\ 
  106 & MME & sigma & beta=5 & sigma=1 & n=200 & 81.11 \\ 
  107 & MME.b & sigma & beta=5 & sigma=1 & n=200 & 972.10 \\ 
  108 & PWM & sigma & beta=5 & sigma=1 & n=200 & 4.43 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220214/20220213-13h27-Output.var.LaTeX.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Mon Feb 14 08:19:22 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=1 & n=200 & 0.10 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=1 & n=200 & 0.08 \\ 
  3 & LME & beta & beta=1.5 & sigma=1 & n=200 & 0.11 \\ 
  4 & MDE.Phi.chisq & beta & beta=1.5 & sigma=1 & n=200 & 0.12 \\ 
  5 & MDE.Phi.tv & beta & beta=1.5 & sigma=1 & n=200 & 0.16 \\ 
  6 & MDE.Phi.kl & beta & beta=1.5 & sigma=1 & n=200 & 0.10 \\ 
  7 & MME & beta & beta=1.5 & sigma=1 & n=200 & 0.16 \\ 
  8 & MME.b & beta & beta=1.5 & sigma=1 & n=200 & 0.19 \\ 
  9 & PWM & beta & beta=1.5 & sigma=1 & n=200 & 0.11 \\ 
  10 & MLE & sigma & beta=1.5 & sigma=1 & n=200 & 0.11 \\ 
  11 & MLE.b & sigma & beta=1.5 & sigma=1 & n=200 & 0.08 \\ 
  12 & LME & sigma & beta=1.5 & sigma=1 & n=200 & 0.12 \\ 
  13 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=1 & n=200 & 0.22 \\ 
  14 & MDE.Phi.tv & sigma & beta=1.5 & sigma=1 & n=200 & 0.27 \\ 
  15 & MDE.Phi.kl & sigma & beta=1.5 & sigma=1 & n=200 & 0.11 \\ 
  16 & MME & sigma & beta=1.5 & sigma=1 & n=200 & 4.41 \\ 
  17 & MME.b & sigma & beta=1.5 & sigma=1 & n=200 & 4.16 \\ 
  18 & PWM & sigma & beta=1.5 & sigma=1 & n=200 & 0.12 \\ 
  19 & MLE & beta & beta=2 & sigma=1 & n=200 & 0.33 \\ 
  20 & MLE.b & beta & beta=2 & sigma=1 & n=200 & 0.21 \\ 
  21 & LME & beta & beta=2 & sigma=1 & n=200 & 0.31 \\ 
  22 & MDE.Phi.chisq & beta & beta=2 & sigma=1 & n=200 & 4.40 \\ 
  23 & MDE.Phi.tv & beta & beta=2 & sigma=1 & n=200 & 0.80 \\ 
  24 & MDE.Phi.kl & beta & beta=2 & sigma=1 & n=200 & 0.33 \\ 
  25 & MME & beta & beta=2 & sigma=1 & n=200 & 0.57 \\ 
  26 & MME.b & beta & beta=2 & sigma=1 & n=200 & 3.90 \\ 
  27 & PWM & beta & beta=2 & sigma=1 & n=200 & 0.31 \\ 
  28 & MLE & sigma & beta=2 & sigma=1 & n=200 & 0.17 \\ 
  29 & MLE.b & sigma & beta=2 & sigma=1 & n=200 & 0.11 \\ 
  30 & LME & sigma & beta=2 & sigma=1 & n=200 & 0.15 \\ 
  31 & MDE.Phi.chisq & sigma & beta=2 & sigma=1 & n=200 & 4.52 \\ 
  32 & MDE.Phi.tv & sigma & beta=2 & sigma=1 & n=200 & 0.71 \\ 
  33 & MDE.Phi.kl & sigma & beta=2 & sigma=1 & n=200 & 0.17 \\ 
  34 & MME & sigma & beta=2 & sigma=1 & n=200 & 0.31 \\ 
  35 & MME.b & sigma & beta=2 & sigma=1 & n=200 & 2.00 \\ 
  36 & PWM & sigma & beta=2 & sigma=1 & n=200 & 0.15 \\ 
  37 & MLE & beta & beta=2.5 & sigma=1 & n=200 & 1.06 \\ 
  38 & MLE.b & beta & beta=2.5 & sigma=1 & n=200 & 0.75 \\ 
  39 & LME & beta & beta=2.5 & sigma=1 & n=200 & 0.90 \\ 
  40 & MDE.Phi.chisq & beta & beta=2.5 & sigma=1 & n=200 & 24.11 \\ 
  41 & MDE.Phi.tv & beta & beta=2.5 & sigma=1 & n=200 & 17.29 \\ 
  42 & MDE.Phi.kl & beta & beta=2.5 & sigma=1 & n=200 & 1.06 \\ 
  43 & MME & beta & beta=2.5 & sigma=1 & n=200 & 1.74 \\ 
  44 & MME.b & beta & beta=2.5 & sigma=1 & n=200 & 977.71 \\ 
  45 & PWM & beta & beta=2.5 & sigma=1 & n=200 & 0.90 \\ 
  46 & MLE & sigma & beta=2.5 & sigma=1 & n=200 & 0.30 \\ 
  47 & MLE.b & sigma & beta=2.5 & sigma=1 & n=200 & 0.21 \\ 
  48 & LME & sigma & beta=2.5 & sigma=1 & n=200 & 0.26 \\ 
  49 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=1 & n=200 & 11.87 \\ 
  50 & MDE.Phi.tv & sigma & beta=2.5 & sigma=1 & n=200 & 8.73 \\ 
  51 & MDE.Phi.kl & sigma & beta=2.5 & sigma=1 & n=200 & 0.30 \\ 
  52 & MME & sigma & beta=2.5 & sigma=1 & n=200 & 0.50 \\ 
  53 & MME.b & sigma & beta=2.5 & sigma=1 & n=200 & 315.84 \\ 
  54 & PWM & sigma & beta=2.5 & sigma=1 & n=200 & 0.26 \\ 
  55 & MLE & beta & beta=3 & sigma=1 & n=200 & 5.86 \\ 
  56 & MLE.b & beta & beta=3 & sigma=1 & n=200 & 5.53 \\ 
  57 & LME & beta & beta=3 & sigma=1 & n=200 & 1.85 \\ 
  58 & MDE.Phi.chisq & beta & beta=3 & sigma=1 & n=200 & 112.96 \\ 
  59 & MDE.Phi.tv & beta & beta=3 & sigma=1 & n=200 & 73.06 \\ 
  60 & MDE.Phi.kl & beta & beta=3 & sigma=1 & n=200 & 5.88 \\ 
  61 & MME & beta & beta=3 & sigma=1 & n=200 & 9.82 \\ 
  62 & MME.b & beta & beta=3 & sigma=1 & n=200 & 13779.73 \\ 
  63 & PWM & beta & beta=3 & sigma=1 & n=200 & 1.85 \\ 
  64 & MLE & sigma & beta=3 & sigma=1 & n=200 & 1.17 \\ 
  65 & MLE.b & sigma & beta=3 & sigma=1 & n=200 & 1.10 \\ 
  66 & LME & sigma & beta=3 & sigma=1 & n=200 & 0.35 \\ 
  67 & MDE.Phi.chisq & sigma & beta=3 & sigma=1 & n=200 & 36.92 \\ 
  68 & MDE.Phi.tv & sigma & beta=3 & sigma=1 & n=200 & 23.85 \\ 
  69 & MDE.Phi.kl & sigma & beta=3 & sigma=1 & n=200 & 1.17 \\ 
  70 & MME & sigma & beta=3 & sigma=1 & n=200 & 1.97 \\ 
  71 & MME.b & sigma & beta=3 & sigma=1 & n=200 & 2554.25 \\ 
  72 & PWM & sigma & beta=3 & sigma=1 & n=200 & 0.35 \\ 
  73 & MLE & beta & beta=4 & sigma=1 & n=200 & 49022.63 \\ 
  74 & MLE.b & beta & beta=4 & sigma=1 & n=200 & 49028.19 \\ 
  75 & LME & beta & beta=4 & sigma=1 & n=200 & 23.00 \\ 
  76 & MDE.Phi.chisq & beta & beta=4 & sigma=1 & n=200 & 614.88 \\ 
  77 & MDE.Phi.tv & beta & beta=4 & sigma=1 & n=200 & 410.66 \\ 
  78 & MDE.Phi.kl & beta & beta=4 & sigma=1 & n=200 & 57.80 \\ 
  79 & MME & beta & beta=4 & sigma=1 & n=200 & 366.31 \\ 
  80 & MME.b & beta & beta=4 & sigma=1 & n=200 & 6124612.72 \\ 
  81 & PWM & beta & beta=4 & sigma=1 & n=200 & 23.00 \\ 
  82 & MLE & sigma & beta=4 & sigma=1 & n=200 & 4458.50 \\ 
  83 & MLE.b & sigma & beta=4 & sigma=1 & n=200 & 4459.02 \\ 
  84 & LME & sigma & beta=4 & sigma=1 & n=200 & 2.14 \\ 
  85 & MDE.Phi.chisq & sigma & beta=4 & sigma=1 & n=200 & 97.82 \\ 
  86 & MDE.Phi.tv & sigma & beta=4 & sigma=1 & n=200 & 62.02 \\ 
  87 & MDE.Phi.kl & sigma & beta=4 & sigma=1 & n=200 & 5.21 \\ 
  88 & MME & sigma & beta=4 & sigma=1 & n=200 & 31.45 \\ 
  89 & MME.b & sigma & beta=4 & sigma=1 & n=200 & 606258.13 \\ 
  90 & PWM & sigma & beta=4 & sigma=1 & n=200 & 2.14 \\ 
  91 & MLE & beta & beta=5 & sigma=1 & n=200 & 248940.59 \\ 
  92 & MLE.b & beta & beta=5 & sigma=1 & n=200 & 248962.94 \\ 
  93 & LME & beta & beta=5 & sigma=1 & n=200 & 74.35 \\ 
  94 & MDE.Phi.chisq & beta & beta=5 & sigma=1 & n=200 & 1568.21 \\ 
  95 & MDE.Phi.tv & beta & beta=5 & sigma=1 & n=200 & 1070.03 \\ 
  96 & MDE.Phi.kl & beta & beta=5 & sigma=1 & n=200 & 168.67 \\ 
  97 & MME & beta & beta=5 & sigma=1 & n=200 & 1452.54 \\ 
  98 & MME.b & beta & beta=5 & sigma=1 & n=200 & 17707.62 \\ 
  99 & PWM & beta & beta=5 & sigma=1 & n=200 & 74.35 \\ 
  100 & MLE & sigma & beta=5 & sigma=1 & n=200 & 13206.79 \\ 
  101 & MLE.b & sigma & beta=5 & sigma=1 & n=200 & 13208.00 \\ 
  102 & LME & sigma & beta=5 & sigma=1 & n=200 & 4.24 \\ 
  103 & MDE.Phi.chisq & sigma & beta=5 & sigma=1 & n=200 & 149.50 \\ 
  104 & MDE.Phi.tv & sigma & beta=5 & sigma=1 & n=200 & 95.76 \\ 
  105 & MDE.Phi.kl & sigma & beta=5 & sigma=1 & n=200 & 9.40 \\ 
  106 & MME & sigma & beta=5 & sigma=1 & n=200 & 79.71 \\ 
  107 & MME.b & sigma & beta=5 & sigma=1 & n=200 & 956.64 \\ 
  108 & PWM & sigma & beta=5 & sigma=1 & n=200 & 4.24 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220214/20220213-13h28-Full.beta=1.5.sig=2.n=200.LaTeX.tex <==
% START DATE AND TIME=20220213-13h28
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=1.5,  \sigma=2$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.5737&1.4914&1.7059&0.7226&1.0026&1.5737&2.4961&2.2948&1.7059
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
2.1531&1.9808&2.4038&2.2869&2.504&2.1531&5.5957&5.0386&2.4038
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1006&0.0759&0.1096&14.0831&0.1638&0.1006&0.1638&0.1915&0.1096
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.4248&0.3152&0.475&2.5951&1.0978&0.4248&17.6337&16.6339&0.475
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.0737&-0.0086&0.2059&-0.7774&-0.4974&0.0737&0.9961&0.7948&0.2059
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.1531&-0.0192&0.4038&0.2869&0.504&0.1531&3.5957&3.0386&0.4038
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.106&0.076&0.152&14.6861&0.4111&0.106&1.1561&0.8232&0.152
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.4482&0.3156&0.638&2.6771&1.3517&0.4482&30.5612&25.8654&0.638
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 0.5542&0.3916&0.79&17.3632&1.7629&0.5542&31.7172&26.6886&0.79\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 6e-04&6e-04&6e-04&1.98995366779715e+299&0.0277&6e-04&0.0088&0.0087&6e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220214/20220213-13h28-Full.beta=2.5.sig=2.n=200.LaTeX.tex <==
% START DATE AND TIME=20220213-13h28
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2.5,  \sigma=2$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.7638&2.4525&2.793&2.0876&2.2976&2.7638&3.598&3.703&2.793
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
2.2846&1.9477&2.2987&2.7523&2.8386&2.2846&3.3489&3.4341&2.2987
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.0591&0.7475&0.8951&18.717&14.4954&1.0592&1.7388&977.7111&0.8951
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
1.2032&0.8379&1.0291&36.9481&29.2117&1.2034&2.0056&1263.3548&1.0291
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.2638&-0.0475&0.293&-0.4124&-0.2024&0.2638&1.098&1.203&0.293
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.2846&-0.0523&0.2987&0.7523&0.8386&0.2846&1.3489&1.4341&0.2987
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.1286&0.7497&0.9809&18.8852&14.5349&1.1287&2.9444&979.0605&0.9809
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
1.2841&0.8406&1.1182&37.5105&29.912&1.2843&3.825&1265.2851&1.1182
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 2.4127&1.5902&2.0991&56.3957&44.4468&2.413&6.7693&2244.3456&2.0991\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&6e-04&5e-04&0.0174&0.0121&5e-04&0.0011&0.0017&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220214/20220213-13h28-Full.beta=2.sig=2.n=200.LaTeX.tex <==
% START DATE AND TIME=20220213-13h28
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2,  \sigma=2$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.1509&1.9786&2.2244&1.3644&1.5611&2.1509&2.9788&2.6734&2.2244
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
2.2164&1.9692&2.3009&2.3856&2.5547&2.2164&3.7968&3.2888&2.3009
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.3276&0.2132&0.3063&3.6096&0.8049&0.3276&0.5666&3.8997&0.3063
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.664&0.4296&0.6179&14.7825&2.8592&0.664&1.2431&8.0061&0.6179
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1509&-0.0214&0.2244&-0.6356&-0.4389&0.1509&0.9788&0.6734&0.2244
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.2164&-0.0308&0.3009&0.3856&0.5547&0.2164&1.7968&1.2888&0.3009
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.3503&0.2136&0.3566&4.0133&0.9975&0.3503&1.5245&4.3529&0.3566
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.7108&0.4305&0.7084&14.9298&3.1666&0.7108&4.4714&9.6663&0.7084
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 1.0611&0.6441&1.065&18.943&4.1641&1.0611&5.9959&14.0191&1.065\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&5e-04&5e-04&0.0228&0.0165&5e-04&0.0024&0.0027&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220214/20220213-13h28-Full.beta=3.sig=2.n=200.LaTeX.tex <==
% START DATE AND TIME=20220213-13h28
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=3,  \sigma=2$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 3.4361&2.9785&3.3721&3.3021&3.2926&3.4347&4.3093&6.586&3.3721
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
2.379&1.9834&2.3088&3.5448&3.3062&2.3776&3.2215&5.1584&2.3088
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 5.864&5.5311&1.8476&90.9164&59.2641&5.4364&9.8172&13779.7265&1.8476
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
4.671&4.418&1.4019&118.9813&77.1925&4.2949&7.8614&10217.0144&1.4019
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.4361&-0.0215&0.3721&0.3021&0.2926&0.4347&1.3093&3.586&0.3721
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.379&-0.0166&0.3088&1.5448&1.3062&0.3776&1.2215&3.1584&0.3088
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 6.0537&5.531&1.9859&90.9986&59.3439&5.6247&11.5306&13791.2077&1.9859
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
4.8142&4.4179&1.4972&121.3557&78.8909&4.437&9.3528&10225.9681&1.4972
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 10.8678&9.9488&3.483&212.3543&138.2348&10.0618&20.8833&24017.1758&3.483\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&5e-04&5e-04&0.0143&0.0097&5e-04&7e-04&0.0021&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220214/20220213-13h28-Full.beta=4.sig=2.n=200.LaTeX.tex <==
% START DATE AND TIME=20220213-13h28
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=4,  \sigma=2$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 8.4458&7.7725&4.961&7.8&6.7847&5.3433&6.6323&36.3872&4.961
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
4.6932&4.2804&2.5755&6.0419&4.9532&2.8148&3.6307&22.3429&2.5755
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 43712.5764&43717.9207&22.9957&485.3556&326.6392&52.0529&366.3062&6124612.719&22.9957
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
15945.1551&15947.1203&8.5757&309.4471&197.4258&18.7736&125.8124&2425032.5159&8.5757
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 4.4458&3.7725&0.961&3.8&2.7847&1.3433&2.6323&32.3872&0.961
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
2.6932&2.2804&0.5755&4.0419&2.9532&0.8148&1.6307&20.3429&0.5755
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 43727.9707&43727.7809&23.9168&499.747&334.3609&53.8521&373.1988&6125049.1898&23.9168
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
15950.8137&15950.726&8.906&325.7533&206.1275&19.4356&128.4591&2425203.8463&8.906
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 59678.7844&59678.5069&32.8229&825.5003&540.4884&73.2877&501.6579&8550253.0361&32.8229\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&6e-04&5e-04&0.0112&0.0074&5e-04&6e-04&0.0041&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220214/20220213-13h28-Full.beta=5.sig=2.n=200.LaTeX.tex <==
% START DATE AND TIME=20220213-13h28
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=5,  \sigma=2$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 20.2364&19.5303&6.7832&14.8065&11.9395&7.7772&9.8718&21.3582&6.7832
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
9.0186&8.6861&2.8284&8.943&6.8354&3.3061&4.3123&9.7484&2.8284
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 239227.549&239249.418&61.7482&1212.7667&834.8687&145.1961&1335.9594&17260.1659&61.7482
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
50728.702&50733.4374&13.5459&461.3557&298.7014&32.1985&287.4741&3706.8924&13.5459
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 15.2364&14.5303&1.7832&9.8065&6.9395&2.7772&4.8718&16.3582&1.7832
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
7.0186&6.6861&0.8284&6.943&4.8354&1.3061&2.3123&7.7484&0.8284
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 239435.774&239436.6236&64.9219&1308.813&882.9423&152.8942&1359.5606&17526.0308&64.9219
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
50772.8899&50773.0682&14.2309&509.5148&322.0529&33.9011&292.7921&3766.5588&14.2309
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 290208.6638&290209.6918&79.1527&1818.3278&1204.9953&186.7953&1652.3527&21292.5896&79.1527\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&6e-04&5e-04&0.0095&0.0062&5e-04&5e-04&0.0255&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220214/20220213-13h28-Output.accuracy.LaTeX.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Mon Feb 14 11:20:06 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & Measure & beta=1.5 & sigma=2 & n=200 & 0.55 \\ 
  2 & MLE.b & Measure & beta=1.5 & sigma=2 & n=200 & 0.39 \\ 
  3 & LME & Measure & beta=1.5 & sigma=2 & n=200 & 0.79 \\ 
  4 & MDE.Phi.chisq & Measure & beta=1.5 & sigma=2 & n=200 & 17.36 \\ 
  5 & MDE.Phi.tv & Measure & beta=1.5 & sigma=2 & n=200 & 1.76 \\ 
  6 & MDE.Phi.kl & Measure & beta=1.5 & sigma=2 & n=200 & 0.55 \\ 
  7 & MME & Measure & beta=1.5 & sigma=2 & n=200 & 31.72 \\ 
  8 & MME.b & Measure & beta=1.5 & sigma=2 & n=200 & 26.69 \\ 
  9 & PWM & Measure & beta=1.5 & sigma=2 & n=200 & 0.79 \\ 
  10 & MLE & Measure & beta=2 & sigma=2 & n=200 & 1.06 \\ 
  11 & MLE.b & Measure & beta=2 & sigma=2 & n=200 & 0.64 \\ 
  12 & LME & Measure & beta=2 & sigma=2 & n=200 & 1.06 \\ 
  13 & MDE.Phi.chisq & Measure & beta=2 & sigma=2 & n=200 & 18.94 \\ 
  14 & MDE.Phi.tv & Measure & beta=2 & sigma=2 & n=200 & 4.16 \\ 
  15 & MDE.Phi.kl & Measure & beta=2 & sigma=2 & n=200 & 1.06 \\ 
  16 & MME & Measure & beta=2 & sigma=2 & n=200 & 6.00 \\ 
  17 & MME.b & Measure & beta=2 & sigma=2 & n=200 & 14.02 \\ 
  18 & PWM & Measure & beta=2 & sigma=2 & n=200 & 1.06 \\ 
  19 & MLE & Measure & beta=2.5 & sigma=2 & n=200 & 2.41 \\ 
  20 & MLE.b & Measure & beta=2.5 & sigma=2 & n=200 & 1.59 \\ 
  21 & LME & Measure & beta=2.5 & sigma=2 & n=200 & 2.10 \\ 
  22 & MDE.Phi.chisq & Measure & beta=2.5 & sigma=2 & n=200 & 56.40 \\ 
  23 & MDE.Phi.tv & Measure & beta=2.5 & sigma=2 & n=200 & 44.45 \\ 
  24 & MDE.Phi.kl & Measure & beta=2.5 & sigma=2 & n=200 & 2.41 \\ 
  25 & MME & Measure & beta=2.5 & sigma=2 & n=200 & 6.77 \\ 
  26 & MME.b & Measure & beta=2.5 & sigma=2 & n=200 & 2244.35 \\ 
  27 & PWM & Measure & beta=2.5 & sigma=2 & n=200 & 2.10 \\ 
  28 & MLE & Measure & beta=3 & sigma=2 & n=200 & 10.87 \\ 
  29 & MLE.b & Measure & beta=3 & sigma=2 & n=200 & 9.95 \\ 
  30 & LME & Measure & beta=3 & sigma=2 & n=200 & 3.48 \\ 
  31 & MDE.Phi.chisq & Measure & beta=3 & sigma=2 & n=200 & 212.35 \\ 
  32 & MDE.Phi.tv & Measure & beta=3 & sigma=2 & n=200 & 138.23 \\ 
  33 & MDE.Phi.kl & Measure & beta=3 & sigma=2 & n=200 & 10.06 \\ 
  34 & MME & Measure & beta=3 & sigma=2 & n=200 & 20.88 \\ 
  35 & MME.b & Measure & beta=3 & sigma=2 & n=200 & 24017.18 \\ 
  36 & PWM & Measure & beta=3 & sigma=2 & n=200 & 3.48 \\ 
  37 & MLE & Measure & beta=4 & sigma=2 & n=200 & 59678.78 \\ 
  38 & MLE.b & Measure & beta=4 & sigma=2 & n=200 & 59678.51 \\ 
  39 & LME & Measure & beta=4 & sigma=2 & n=200 & 32.82 \\ 
  40 & MDE.Phi.chisq & Measure & beta=4 & sigma=2 & n=200 & 825.50 \\ 
  41 & MDE.Phi.tv & Measure & beta=4 & sigma=2 & n=200 & 540.49 \\ 
  42 & MDE.Phi.kl & Measure & beta=4 & sigma=2 & n=200 & 73.29 \\ 
  43 & MME & Measure & beta=4 & sigma=2 & n=200 & 501.66 \\ 
  44 & MME.b & Measure & beta=4 & sigma=2 & n=200 & 8550253.04 \\ 
  45 & PWM & Measure & beta=4 & sigma=2 & n=200 & 32.82 \\ 
  46 & MLE & Measure & beta=5 & sigma=2 & n=200 & 290208.66 \\ 
  47 & MLE.b & Measure & beta=5 & sigma=2 & n=200 & 290209.69 \\ 
  48 & LME & Measure & beta=5 & sigma=2 & n=200 & 79.15 \\ 
  49 & MDE.Phi.chisq & Measure & beta=5 & sigma=2 & n=200 & 1818.33 \\ 
  50 & MDE.Phi.tv & Measure & beta=5 & sigma=2 & n=200 & 1205.00 \\ 
  51 & MDE.Phi.kl & Measure & beta=5 & sigma=2 & n=200 & 186.80 \\ 
  52 & MME & Measure & beta=5 & sigma=2 & n=200 & 1652.35 \\ 
  53 & MME.b & Measure & beta=5 & sigma=2 & n=200 & 21292.59 \\ 
  54 & PWM & Measure & beta=5 & sigma=2 & n=200 & 79.15 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220214/20220213-13h28-Output.accuracy2.LaTeX.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Mon Feb 14 11:20:06 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & Measure & beta=1.5 & sigma=2 & n=200 & 0.00 \\ 
  2 & MLE.b & Measure & beta=1.5 & sigma=2 & n=200 & 0.00 \\ 
  3 & LME & Measure & beta=1.5 & sigma=2 & n=200 & 0.00 \\ 
  4 & MDE.Phi.chisq & Measure & beta=1.5 & sigma=2 & n=200 & 198995366779715153280044842808400880828400882464846224026842404600006426606440840062208644240222440826624048068048842026288080622666444028206480226426066880688222244266624244046804224840668624482404444244822068424222464486824444468240460262086640008280860460004228046662662008286848646022880664240688.00 \\ 
  5 & MDE.Phi.tv & Measure & beta=1.5 & sigma=2 & n=200 & 0.03 \\ 
  6 & MDE.Phi.kl & Measure & beta=1.5 & sigma=2 & n=200 & 0.00 \\ 
  7 & MME & Measure & beta=1.5 & sigma=2 & n=200 & 0.01 \\ 
  8 & MME.b & Measure & beta=1.5 & sigma=2 & n=200 & 0.01 \\ 
  9 & PWM & Measure & beta=1.5 & sigma=2 & n=200 & 0.00 \\ 
  10 & MLE & Measure & beta=2 & sigma=2 & n=200 & 0.00 \\ 
  11 & MLE.b & Measure & beta=2 & sigma=2 & n=200 & 0.00 \\ 
  12 & LME & Measure & beta=2 & sigma=2 & n=200 & 0.00 \\ 
  13 & MDE.Phi.chisq & Measure & beta=2 & sigma=2 & n=200 & 0.02 \\ 
  14 & MDE.Phi.tv & Measure & beta=2 & sigma=2 & n=200 & 0.02 \\ 
  15 & MDE.Phi.kl & Measure & beta=2 & sigma=2 & n=200 & 0.00 \\ 
  16 & MME & Measure & beta=2 & sigma=2 & n=200 & 0.00 \\ 
  17 & MME.b & Measure & beta=2 & sigma=2 & n=200 & 0.00 \\ 
  18 & PWM & Measure & beta=2 & sigma=2 & n=200 & 0.00 \\ 
  19 & MLE & Measure & beta=2.5 & sigma=2 & n=200 & 0.00 \\ 
  20 & MLE.b & Measure & beta=2.5 & sigma=2 & n=200 & 0.00 \\ 
  21 & LME & Measure & beta=2.5 & sigma=2 & n=200 & 0.00 \\ 
  22 & MDE.Phi.chisq & Measure & beta=2.5 & sigma=2 & n=200 & 0.02 \\ 
  23 & MDE.Phi.tv & Measure & beta=2.5 & sigma=2 & n=200 & 0.01 \\ 
  24 & MDE.Phi.kl & Measure & beta=2.5 & sigma=2 & n=200 & 0.00 \\ 
  25 & MME & Measure & beta=2.5 & sigma=2 & n=200 & 0.00 \\ 
  26 & MME.b & Measure & beta=2.5 & sigma=2 & n=200 & 0.00 \\ 
  27 & PWM & Measure & beta=2.5 & sigma=2 & n=200 & 0.00 \\ 
  28 & MLE & Measure & beta=3 & sigma=2 & n=200 & 0.00 \\ 
  29 & MLE.b & Measure & beta=3 & sigma=2 & n=200 & 0.00 \\ 
  30 & LME & Measure & beta=3 & sigma=2 & n=200 & 0.00 \\ 
  31 & MDE.Phi.chisq & Measure & beta=3 & sigma=2 & n=200 & 0.01 \\ 
  32 & MDE.Phi.tv & Measure & beta=3 & sigma=2 & n=200 & 0.01 \\ 
  33 & MDE.Phi.kl & Measure & beta=3 & sigma=2 & n=200 & 0.00 \\ 
  34 & MME & Measure & beta=3 & sigma=2 & n=200 & 0.00 \\ 
  35 & MME.b & Measure & beta=3 & sigma=2 & n=200 & 0.00 \\ 
  36 & PWM & Measure & beta=3 & sigma=2 & n=200 & 0.00 \\ 
  37 & MLE & Measure & beta=4 & sigma=2 & n=200 & 0.00 \\ 
  38 & MLE.b & Measure & beta=4 & sigma=2 & n=200 & 0.00 \\ 
  39 & LME & Measure & beta=4 & sigma=2 & n=200 & 0.00 \\ 
  40 & MDE.Phi.chisq & Measure & beta=4 & sigma=2 & n=200 & 0.01 \\ 
  41 & MDE.Phi.tv & Measure & beta=4 & sigma=2 & n=200 & 0.01 \\ 
  42 & MDE.Phi.kl & Measure & beta=4 & sigma=2 & n=200 & 0.00 \\ 
  43 & MME & Measure & beta=4 & sigma=2 & n=200 & 0.00 \\ 
  44 & MME.b & Measure & beta=4 & sigma=2 & n=200 & 0.00 \\ 
  45 & PWM & Measure & beta=4 & sigma=2 & n=200 & 0.00 \\ 
  46 & MLE & Measure & beta=5 & sigma=2 & n=200 & 0.00 \\ 
  47 & MLE.b & Measure & beta=5 & sigma=2 & n=200 & 0.00 \\ 
  48 & LME & Measure & beta=5 & sigma=2 & n=200 & 0.00 \\ 
  49 & MDE.Phi.chisq & Measure & beta=5 & sigma=2 & n=200 & 0.01 \\ 
  50 & MDE.Phi.tv & Measure & beta=5 & sigma=2 & n=200 & 0.01 \\ 
  51 & MDE.Phi.kl & Measure & beta=5 & sigma=2 & n=200 & 0.00 \\ 
  52 & MME & Measure & beta=5 & sigma=2 & n=200 & 0.00 \\ 
  53 & MME.b & Measure & beta=5 & sigma=2 & n=200 & 0.03 \\ 
  54 & PWM & Measure & beta=5 & sigma=2 & n=200 & 0.00 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220214/20220213-13h28-Output.bias.LaTeX.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Mon Feb 14 11:20:06 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=2 & n=200 & 0.07 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=2 & n=200 & -0.01 \\ 
  3 & LME & beta & beta=1.5 & sigma=2 & n=200 & 0.21 \\ 
  4 & MDE.Phi.chisq & beta & beta=1.5 & sigma=2 & n=200 & -0.78 \\ 
  5 & MDE.Phi.tv & beta & beta=1.5 & sigma=2 & n=200 & -0.50 \\ 
  6 & MDE.Phi.kl & beta & beta=1.5 & sigma=2 & n=200 & 0.07 \\ 
  7 & MME & beta & beta=1.5 & sigma=2 & n=200 & 1.00 \\ 
  8 & MME.b & beta & beta=1.5 & sigma=2 & n=200 & 0.79 \\ 
  9 & PWM & beta & beta=1.5 & sigma=2 & n=200 & 0.21 \\ 
  10 & MLE & sigma & beta=1.5 & sigma=2 & n=200 & 0.15 \\ 
  11 & MLE.b & sigma & beta=1.5 & sigma=2 & n=200 & -0.02 \\ 
  12 & LME & sigma & beta=1.5 & sigma=2 & n=200 & 0.40 \\ 
  13 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=2 & n=200 & 0.29 \\ 
  14 & MDE.Phi.tv & sigma & beta=1.5 & sigma=2 & n=200 & 0.50 \\ 
  15 & MDE.Phi.kl & sigma & beta=1.5 & sigma=2 & n=200 & 0.15 \\ 
  16 & MME & sigma & beta=1.5 & sigma=2 & n=200 & 3.60 \\ 
  17 & MME.b & sigma & beta=1.5 & sigma=2 & n=200 & 3.04 \\ 
  18 & PWM & sigma & beta=1.5 & sigma=2 & n=200 & 0.40 \\ 
  19 & MLE & beta & beta=2 & sigma=2 & n=200 & 0.15 \\ 
  20 & MLE.b & beta & beta=2 & sigma=2 & n=200 & -0.02 \\ 
  21 & LME & beta & beta=2 & sigma=2 & n=200 & 0.22 \\ 
  22 & MDE.Phi.chisq & beta & beta=2 & sigma=2 & n=200 & -0.64 \\ 
  23 & MDE.Phi.tv & beta & beta=2 & sigma=2 & n=200 & -0.44 \\ 
  24 & MDE.Phi.kl & beta & beta=2 & sigma=2 & n=200 & 0.15 \\ 
  25 & MME & beta & beta=2 & sigma=2 & n=200 & 0.98 \\ 
  26 & MME.b & beta & beta=2 & sigma=2 & n=200 & 0.67 \\ 
  27 & PWM & beta & beta=2 & sigma=2 & n=200 & 0.22 \\ 
  28 & MLE & sigma & beta=2 & sigma=2 & n=200 & 0.22 \\ 
  29 & MLE.b & sigma & beta=2 & sigma=2 & n=200 & -0.03 \\ 
  30 & LME & sigma & beta=2 & sigma=2 & n=200 & 0.30 \\ 
  31 & MDE.Phi.chisq & sigma & beta=2 & sigma=2 & n=200 & 0.39 \\ 
  32 & MDE.Phi.tv & sigma & beta=2 & sigma=2 & n=200 & 0.55 \\ 
  33 & MDE.Phi.kl & sigma & beta=2 & sigma=2 & n=200 & 0.22 \\ 
  34 & MME & sigma & beta=2 & sigma=2 & n=200 & 1.80 \\ 
  35 & MME.b & sigma & beta=2 & sigma=2 & n=200 & 1.29 \\ 
  36 & PWM & sigma & beta=2 & sigma=2 & n=200 & 0.30 \\ 
  37 & MLE & beta & beta=2.5 & sigma=2 & n=200 & 0.26 \\ 
  38 & MLE.b & beta & beta=2.5 & sigma=2 & n=200 & -0.05 \\ 
  39 & LME & beta & beta=2.5 & sigma=2 & n=200 & 0.29 \\ 
  40 & MDE.Phi.chisq & beta & beta=2.5 & sigma=2 & n=200 & -0.41 \\ 
  41 & MDE.Phi.tv & beta & beta=2.5 & sigma=2 & n=200 & -0.20 \\ 
  42 & MDE.Phi.kl & beta & beta=2.5 & sigma=2 & n=200 & 0.26 \\ 
  43 & MME & beta & beta=2.5 & sigma=2 & n=200 & 1.10 \\ 
  44 & MME.b & beta & beta=2.5 & sigma=2 & n=200 & 1.20 \\ 
  45 & PWM & beta & beta=2.5 & sigma=2 & n=200 & 0.29 \\ 
  46 & MLE & sigma & beta=2.5 & sigma=2 & n=200 & 0.28 \\ 
  47 & MLE.b & sigma & beta=2.5 & sigma=2 & n=200 & -0.05 \\ 
  48 & LME & sigma & beta=2.5 & sigma=2 & n=200 & 0.30 \\ 
  49 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=2 & n=200 & 0.75 \\ 
  50 & MDE.Phi.tv & sigma & beta=2.5 & sigma=2 & n=200 & 0.84 \\ 
  51 & MDE.Phi.kl & sigma & beta=2.5 & sigma=2 & n=200 & 0.28 \\ 
  52 & MME & sigma & beta=2.5 & sigma=2 & n=200 & 1.35 \\ 
  53 & MME.b & sigma & beta=2.5 & sigma=2 & n=200 & 1.43 \\ 
  54 & PWM & sigma & beta=2.5 & sigma=2 & n=200 & 0.30 \\ 
  55 & MLE & beta & beta=3 & sigma=2 & n=200 & 0.44 \\ 
  56 & MLE.b & beta & beta=3 & sigma=2 & n=200 & -0.02 \\ 
  57 & LME & beta & beta=3 & sigma=2 & n=200 & 0.37 \\ 
  58 & MDE.Phi.chisq & beta & beta=3 & sigma=2 & n=200 & 0.30 \\ 
  59 & MDE.Phi.tv & beta & beta=3 & sigma=2 & n=200 & 0.29 \\ 
  60 & MDE.Phi.kl & beta & beta=3 & sigma=2 & n=200 & 0.43 \\ 
  61 & MME & beta & beta=3 & sigma=2 & n=200 & 1.31 \\ 
  62 & MME.b & beta & beta=3 & sigma=2 & n=200 & 3.59 \\ 
  63 & PWM & beta & beta=3 & sigma=2 & n=200 & 0.37 \\ 
  64 & MLE & sigma & beta=3 & sigma=2 & n=200 & 0.38 \\ 
  65 & MLE.b & sigma & beta=3 & sigma=2 & n=200 & -0.02 \\ 
  66 & LME & sigma & beta=3 & sigma=2 & n=200 & 0.31 \\ 
  67 & MDE.Phi.chisq & sigma & beta=3 & sigma=2 & n=200 & 1.54 \\ 
  68 & MDE.Phi.tv & sigma & beta=3 & sigma=2 & n=200 & 1.31 \\ 
  69 & MDE.Phi.kl & sigma & beta=3 & sigma=2 & n=200 & 0.38 \\ 
  70 & MME & sigma & beta=3 & sigma=2 & n=200 & 1.22 \\ 
  71 & MME.b & sigma & beta=3 & sigma=2 & n=200 & 3.16 \\ 
  72 & PWM & sigma & beta=3 & sigma=2 & n=200 & 0.31 \\ 
  73 & MLE & beta & beta=4 & sigma=2 & n=200 & 4.45 \\ 
  74 & MLE.b & beta & beta=4 & sigma=2 & n=200 & 3.77 \\ 
  75 & LME & beta & beta=4 & sigma=2 & n=200 & 0.96 \\ 
  76 & MDE.Phi.chisq & beta & beta=4 & sigma=2 & n=200 & 3.80 \\ 
  77 & MDE.Phi.tv & beta & beta=4 & sigma=2 & n=200 & 2.78 \\ 
  78 & MDE.Phi.kl & beta & beta=4 & sigma=2 & n=200 & 1.34 \\ 
  79 & MME & beta & beta=4 & sigma=2 & n=200 & 2.63 \\ 
  80 & MME.b & beta & beta=4 & sigma=2 & n=200 & 32.39 \\ 
  81 & PWM & beta & beta=4 & sigma=2 & n=200 & 0.96 \\ 
  82 & MLE & sigma & beta=4 & sigma=2 & n=200 & 2.69 \\ 
  83 & MLE.b & sigma & beta=4 & sigma=2 & n=200 & 2.28 \\ 
  84 & LME & sigma & beta=4 & sigma=2 & n=200 & 0.58 \\ 
  85 & MDE.Phi.chisq & sigma & beta=4 & sigma=2 & n=200 & 4.04 \\ 
  86 & MDE.Phi.tv & sigma & beta=4 & sigma=2 & n=200 & 2.95 \\ 
  87 & MDE.Phi.kl & sigma & beta=4 & sigma=2 & n=200 & 0.81 \\ 
  88 & MME & sigma & beta=4 & sigma=2 & n=200 & 1.63 \\ 
  89 & MME.b & sigma & beta=4 & sigma=2 & n=200 & 20.34 \\ 
  90 & PWM & sigma & beta=4 & sigma=2 & n=200 & 0.58 \\ 
  91 & MLE & beta & beta=5 & sigma=2 & n=200 & 15.24 \\ 
  92 & MLE.b & beta & beta=5 & sigma=2 & n=200 & 14.53 \\ 
  93 & LME & beta & beta=5 & sigma=2 & n=200 & 1.78 \\ 
  94 & MDE.Phi.chisq & beta & beta=5 & sigma=2 & n=200 & 9.81 \\ 
  95 & MDE.Phi.tv & beta & beta=5 & sigma=2 & n=200 & 6.94 \\ 
  96 & MDE.Phi.kl & beta & beta=5 & sigma=2 & n=200 & 2.78 \\ 
  97 & MME & beta & beta=5 & sigma=2 & n=200 & 4.87 \\ 
  98 & MME.b & beta & beta=5 & sigma=2 & n=200 & 16.36 \\ 
  99 & PWM & beta & beta=5 & sigma=2 & n=200 & 1.78 \\ 
  100 & MLE & sigma & beta=5 & sigma=2 & n=200 & 7.02 \\ 
  101 & MLE.b & sigma & beta=5 & sigma=2 & n=200 & 6.69 \\ 
  102 & LME & sigma & beta=5 & sigma=2 & n=200 & 0.83 \\ 
  103 & MDE.Phi.chisq & sigma & beta=5 & sigma=2 & n=200 & 6.94 \\ 
  104 & MDE.Phi.tv & sigma & beta=5 & sigma=2 & n=200 & 4.84 \\ 
  105 & MDE.Phi.kl & sigma & beta=5 & sigma=2 & n=200 & 1.31 \\ 
  106 & MME & sigma & beta=5 & sigma=2 & n=200 & 2.31 \\ 
  107 & MME.b & sigma & beta=5 & sigma=2 & n=200 & 7.75 \\ 
  108 & PWM & sigma & beta=5 & sigma=2 & n=200 & 0.83 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220214/20220213-13h28-Output.mean.LaTeX.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Mon Feb 14 11:20:06 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=2 & n=200 & 1.57 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=2 & n=200 & 1.49 \\ 
  3 & LME & beta & beta=1.5 & sigma=2 & n=200 & 1.71 \\ 
  4 & MDE.Phi.chisq & beta & beta=1.5 & sigma=2 & n=200 & 0.72 \\ 
  5 & MDE.Phi.tv & beta & beta=1.5 & sigma=2 & n=200 & 1.00 \\ 
  6 & MDE.Phi.kl & beta & beta=1.5 & sigma=2 & n=200 & 1.57 \\ 
  7 & MME & beta & beta=1.5 & sigma=2 & n=200 & 2.50 \\ 
  8 & MME.b & beta & beta=1.5 & sigma=2 & n=200 & 2.29 \\ 
  9 & PWM & beta & beta=1.5 & sigma=2 & n=200 & 1.71 \\ 
  10 & MLE & sigma & beta=1.5 & sigma=2 & n=200 & 2.15 \\ 
  11 & MLE.b & sigma & beta=1.5 & sigma=2 & n=200 & 1.98 \\ 
  12 & LME & sigma & beta=1.5 & sigma=2 & n=200 & 2.40 \\ 
  13 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=2 & n=200 & 2.29 \\ 
  14 & MDE.Phi.tv & sigma & beta=1.5 & sigma=2 & n=200 & 2.50 \\ 
  15 & MDE.Phi.kl & sigma & beta=1.5 & sigma=2 & n=200 & 2.15 \\ 
  16 & MME & sigma & beta=1.5 & sigma=2 & n=200 & 5.60 \\ 
  17 & MME.b & sigma & beta=1.5 & sigma=2 & n=200 & 5.04 \\ 
  18 & PWM & sigma & beta=1.5 & sigma=2 & n=200 & 2.40 \\ 
  19 & MLE & beta & beta=2 & sigma=2 & n=200 & 2.15 \\ 
  20 & MLE.b & beta & beta=2 & sigma=2 & n=200 & 1.98 \\ 
  21 & LME & beta & beta=2 & sigma=2 & n=200 & 2.22 \\ 
  22 & MDE.Phi.chisq & beta & beta=2 & sigma=2 & n=200 & 1.36 \\ 
  23 & MDE.Phi.tv & beta & beta=2 & sigma=2 & n=200 & 1.56 \\ 
  24 & MDE.Phi.kl & beta & beta=2 & sigma=2 & n=200 & 2.15 \\ 
  25 & MME & beta & beta=2 & sigma=2 & n=200 & 2.98 \\ 
  26 & MME.b & beta & beta=2 & sigma=2 & n=200 & 2.67 \\ 
  27 & PWM & beta & beta=2 & sigma=2 & n=200 & 2.22 \\ 
  28 & MLE & sigma & beta=2 & sigma=2 & n=200 & 2.22 \\ 
  29 & MLE.b & sigma & beta=2 & sigma=2 & n=200 & 1.97 \\ 
  30 & LME & sigma & beta=2 & sigma=2 & n=200 & 2.30 \\ 
  31 & MDE.Phi.chisq & sigma & beta=2 & sigma=2 & n=200 & 2.39 \\ 
  32 & MDE.Phi.tv & sigma & beta=2 & sigma=2 & n=200 & 2.55 \\ 
  33 & MDE.Phi.kl & sigma & beta=2 & sigma=2 & n=200 & 2.22 \\ 
  34 & MME & sigma & beta=2 & sigma=2 & n=200 & 3.80 \\ 
  35 & MME.b & sigma & beta=2 & sigma=2 & n=200 & 3.29 \\ 
  36 & PWM & sigma & beta=2 & sigma=2 & n=200 & 2.30 \\ 
  37 & MLE & beta & beta=2.5 & sigma=2 & n=200 & 2.76 \\ 
  38 & MLE.b & beta & beta=2.5 & sigma=2 & n=200 & 2.45 \\ 
  39 & LME & beta & beta=2.5 & sigma=2 & n=200 & 2.79 \\ 
  40 & MDE.Phi.chisq & beta & beta=2.5 & sigma=2 & n=200 & 2.09 \\ 
  41 & MDE.Phi.tv & beta & beta=2.5 & sigma=2 & n=200 & 2.30 \\ 
  42 & MDE.Phi.kl & beta & beta=2.5 & sigma=2 & n=200 & 2.76 \\ 
  43 & MME & beta & beta=2.5 & sigma=2 & n=200 & 3.60 \\ 
  44 & MME.b & beta & beta=2.5 & sigma=2 & n=200 & 3.70 \\ 
  45 & PWM & beta & beta=2.5 & sigma=2 & n=200 & 2.79 \\ 
  46 & MLE & sigma & beta=2.5 & sigma=2 & n=200 & 2.28 \\ 
  47 & MLE.b & sigma & beta=2.5 & sigma=2 & n=200 & 1.95 \\ 
  48 & LME & sigma & beta=2.5 & sigma=2 & n=200 & 2.30 \\ 
  49 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=2 & n=200 & 2.75 \\ 
  50 & MDE.Phi.tv & sigma & beta=2.5 & sigma=2 & n=200 & 2.84 \\ 
  51 & MDE.Phi.kl & sigma & beta=2.5 & sigma=2 & n=200 & 2.28 \\ 
  52 & MME & sigma & beta=2.5 & sigma=2 & n=200 & 3.35 \\ 
  53 & MME.b & sigma & beta=2.5 & sigma=2 & n=200 & 3.43 \\ 
  54 & PWM & sigma & beta=2.5 & sigma=2 & n=200 & 2.30 \\ 
  55 & MLE & beta & beta=3 & sigma=2 & n=200 & 3.44 \\ 
  56 & MLE.b & beta & beta=3 & sigma=2 & n=200 & 2.98 \\ 
  57 & LME & beta & beta=3 & sigma=2 & n=200 & 3.37 \\ 
  58 & MDE.Phi.chisq & beta & beta=3 & sigma=2 & n=200 & 3.30 \\ 
  59 & MDE.Phi.tv & beta & beta=3 & sigma=2 & n=200 & 3.29 \\ 
  60 & MDE.Phi.kl & beta & beta=3 & sigma=2 & n=200 & 3.43 \\ 
  61 & MME & beta & beta=3 & sigma=2 & n=200 & 4.31 \\ 
  62 & MME.b & beta & beta=3 & sigma=2 & n=200 & 6.59 \\ 
  63 & PWM & beta & beta=3 & sigma=2 & n=200 & 3.37 \\ 
  64 & MLE & sigma & beta=3 & sigma=2 & n=200 & 2.38 \\ 
  65 & MLE.b & sigma & beta=3 & sigma=2 & n=200 & 1.98 \\ 
  66 & LME & sigma & beta=3 & sigma=2 & n=200 & 2.31 \\ 
  67 & MDE.Phi.chisq & sigma & beta=3 & sigma=2 & n=200 & 3.54 \\ 
  68 & MDE.Phi.tv & sigma & beta=3 & sigma=2 & n=200 & 3.31 \\ 
  69 & MDE.Phi.kl & sigma & beta=3 & sigma=2 & n=200 & 2.38 \\ 
  70 & MME & sigma & beta=3 & sigma=2 & n=200 & 3.22 \\ 
  71 & MME.b & sigma & beta=3 & sigma=2 & n=200 & 5.16 \\ 
  72 & PWM & sigma & beta=3 & sigma=2 & n=200 & 2.31 \\ 
  73 & MLE & beta & beta=4 & sigma=2 & n=200 & 8.45 \\ 
  74 & MLE.b & beta & beta=4 & sigma=2 & n=200 & 7.77 \\ 
  75 & LME & beta & beta=4 & sigma=2 & n=200 & 4.96 \\ 
  76 & MDE.Phi.chisq & beta & beta=4 & sigma=2 & n=200 & 7.80 \\ 
  77 & MDE.Phi.tv & beta & beta=4 & sigma=2 & n=200 & 6.78 \\ 
  78 & MDE.Phi.kl & beta & beta=4 & sigma=2 & n=200 & 5.34 \\ 
  79 & MME & beta & beta=4 & sigma=2 & n=200 & 6.63 \\ 
  80 & MME.b & beta & beta=4 & sigma=2 & n=200 & 36.39 \\ 
  81 & PWM & beta & beta=4 & sigma=2 & n=200 & 4.96 \\ 
  82 & MLE & sigma & beta=4 & sigma=2 & n=200 & 4.69 \\ 
  83 & MLE.b & sigma & beta=4 & sigma=2 & n=200 & 4.28 \\ 
  84 & LME & sigma & beta=4 & sigma=2 & n=200 & 2.58 \\ 
  85 & MDE.Phi.chisq & sigma & beta=4 & sigma=2 & n=200 & 6.04 \\ 
  86 & MDE.Phi.tv & sigma & beta=4 & sigma=2 & n=200 & 4.95 \\ 
  87 & MDE.Phi.kl & sigma & beta=4 & sigma=2 & n=200 & 2.81 \\ 
  88 & MME & sigma & beta=4 & sigma=2 & n=200 & 3.63 \\ 
  89 & MME.b & sigma & beta=4 & sigma=2 & n=200 & 22.34 \\ 
  90 & PWM & sigma & beta=4 & sigma=2 & n=200 & 2.58 \\ 
  91 & MLE & beta & beta=5 & sigma=2 & n=200 & 20.24 \\ 
  92 & MLE.b & beta & beta=5 & sigma=2 & n=200 & 19.53 \\ 
  93 & LME & beta & beta=5 & sigma=2 & n=200 & 6.78 \\ 
  94 & MDE.Phi.chisq & beta & beta=5 & sigma=2 & n=200 & 14.81 \\ 
  95 & MDE.Phi.tv & beta & beta=5 & sigma=2 & n=200 & 11.94 \\ 
  96 & MDE.Phi.kl & beta & beta=5 & sigma=2 & n=200 & 7.78 \\ 
  97 & MME & beta & beta=5 & sigma=2 & n=200 & 9.87 \\ 
  98 & MME.b & beta & beta=5 & sigma=2 & n=200 & 21.36 \\ 
  99 & PWM & beta & beta=5 & sigma=2 & n=200 & 6.78 \\ 
  100 & MLE & sigma & beta=5 & sigma=2 & n=200 & 9.02 \\ 
  101 & MLE.b & sigma & beta=5 & sigma=2 & n=200 & 8.69 \\ 
  102 & LME & sigma & beta=5 & sigma=2 & n=200 & 2.83 \\ 
  103 & MDE.Phi.chisq & sigma & beta=5 & sigma=2 & n=200 & 8.94 \\ 
  104 & MDE.Phi.tv & sigma & beta=5 & sigma=2 & n=200 & 6.84 \\ 
  105 & MDE.Phi.kl & sigma & beta=5 & sigma=2 & n=200 & 3.31 \\ 
  106 & MME & sigma & beta=5 & sigma=2 & n=200 & 4.31 \\ 
  107 & MME.b & sigma & beta=5 & sigma=2 & n=200 & 9.75 \\ 
  108 & PWM & sigma & beta=5 & sigma=2 & n=200 & 2.83 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220214/20220213-13h28-Output.mse.LaTeX.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Mon Feb 14 11:20:06 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=2 & n=200 & 0.11 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=2 & n=200 & 0.08 \\ 
  3 & LME & beta & beta=1.5 & sigma=2 & n=200 & 0.15 \\ 
  4 & MDE.Phi.chisq & beta & beta=1.5 & sigma=2 & n=200 & 14.69 \\ 
  5 & MDE.Phi.tv & beta & beta=1.5 & sigma=2 & n=200 & 0.41 \\ 
  6 & MDE.Phi.kl & beta & beta=1.5 & sigma=2 & n=200 & 0.11 \\ 
  7 & MME & beta & beta=1.5 & sigma=2 & n=200 & 1.16 \\ 
  8 & MME.b & beta & beta=1.5 & sigma=2 & n=200 & 0.82 \\ 
  9 & PWM & beta & beta=1.5 & sigma=2 & n=200 & 0.15 \\ 
  10 & MLE & sigma & beta=1.5 & sigma=2 & n=200 & 0.45 \\ 
  11 & MLE.b & sigma & beta=1.5 & sigma=2 & n=200 & 0.32 \\ 
  12 & LME & sigma & beta=1.5 & sigma=2 & n=200 & 0.64 \\ 
  13 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=2 & n=200 & 2.68 \\ 
  14 & MDE.Phi.tv & sigma & beta=1.5 & sigma=2 & n=200 & 1.35 \\ 
  15 & MDE.Phi.kl & sigma & beta=1.5 & sigma=2 & n=200 & 0.45 \\ 
  16 & MME & sigma & beta=1.5 & sigma=2 & n=200 & 30.56 \\ 
  17 & MME.b & sigma & beta=1.5 & sigma=2 & n=200 & 25.87 \\ 
  18 & PWM & sigma & beta=1.5 & sigma=2 & n=200 & 0.64 \\ 
  19 & MLE & beta & beta=2 & sigma=2 & n=200 & 0.35 \\ 
  20 & MLE.b & beta & beta=2 & sigma=2 & n=200 & 0.21 \\ 
  21 & LME & beta & beta=2 & sigma=2 & n=200 & 0.36 \\ 
  22 & MDE.Phi.chisq & beta & beta=2 & sigma=2 & n=200 & 4.01 \\ 
  23 & MDE.Phi.tv & beta & beta=2 & sigma=2 & n=200 & 1.00 \\ 
  24 & MDE.Phi.kl & beta & beta=2 & sigma=2 & n=200 & 0.35 \\ 
  25 & MME & beta & beta=2 & sigma=2 & n=200 & 1.52 \\ 
  26 & MME.b & beta & beta=2 & sigma=2 & n=200 & 4.35 \\ 
  27 & PWM & beta & beta=2 & sigma=2 & n=200 & 0.36 \\ 
  28 & MLE & sigma & beta=2 & sigma=2 & n=200 & 0.71 \\ 
  29 & MLE.b & sigma & beta=2 & sigma=2 & n=200 & 0.43 \\ 
  30 & LME & sigma & beta=2 & sigma=2 & n=200 & 0.71 \\ 
  31 & MDE.Phi.chisq & sigma & beta=2 & sigma=2 & n=200 & 14.93 \\ 
  32 & MDE.Phi.tv & sigma & beta=2 & sigma=2 & n=200 & 3.17 \\ 
  33 & MDE.Phi.kl & sigma & beta=2 & sigma=2 & n=200 & 0.71 \\ 
  34 & MME & sigma & beta=2 & sigma=2 & n=200 & 4.47 \\ 
  35 & MME.b & sigma & beta=2 & sigma=2 & n=200 & 9.67 \\ 
  36 & PWM & sigma & beta=2 & sigma=2 & n=200 & 0.71 \\ 
  37 & MLE & beta & beta=2.5 & sigma=2 & n=200 & 1.13 \\ 
  38 & MLE.b & beta & beta=2.5 & sigma=2 & n=200 & 0.75 \\ 
  39 & LME & beta & beta=2.5 & sigma=2 & n=200 & 0.98 \\ 
  40 & MDE.Phi.chisq & beta & beta=2.5 & sigma=2 & n=200 & 18.89 \\ 
  41 & MDE.Phi.tv & beta & beta=2.5 & sigma=2 & n=200 & 14.53 \\ 
  42 & MDE.Phi.kl & beta & beta=2.5 & sigma=2 & n=200 & 1.13 \\ 
  43 & MME & beta & beta=2.5 & sigma=2 & n=200 & 2.94 \\ 
  44 & MME.b & beta & beta=2.5 & sigma=2 & n=200 & 979.06 \\ 
  45 & PWM & beta & beta=2.5 & sigma=2 & n=200 & 0.98 \\ 
  46 & MLE & sigma & beta=2.5 & sigma=2 & n=200 & 1.28 \\ 
  47 & MLE.b & sigma & beta=2.5 & sigma=2 & n=200 & 0.84 \\ 
  48 & LME & sigma & beta=2.5 & sigma=2 & n=200 & 1.12 \\ 
  49 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=2 & n=200 & 37.51 \\ 
  50 & MDE.Phi.tv & sigma & beta=2.5 & sigma=2 & n=200 & 29.91 \\ 
  51 & MDE.Phi.kl & sigma & beta=2.5 & sigma=2 & n=200 & 1.28 \\ 
  52 & MME & sigma & beta=2.5 & sigma=2 & n=200 & 3.82 \\ 
  53 & MME.b & sigma & beta=2.5 & sigma=2 & n=200 & 1265.29 \\ 
  54 & PWM & sigma & beta=2.5 & sigma=2 & n=200 & 1.12 \\ 
  55 & MLE & beta & beta=3 & sigma=2 & n=200 & 6.05 \\ 
  56 & MLE.b & beta & beta=3 & sigma=2 & n=200 & 5.53 \\ 
  57 & LME & beta & beta=3 & sigma=2 & n=200 & 1.99 \\ 
  58 & MDE.Phi.chisq & beta & beta=3 & sigma=2 & n=200 & 91.00 \\ 
  59 & MDE.Phi.tv & beta & beta=3 & sigma=2 & n=200 & 59.34 \\ 
  60 & MDE.Phi.kl & beta & beta=3 & sigma=2 & n=200 & 5.62 \\ 
  61 & MME & beta & beta=3 & sigma=2 & n=200 & 11.53 \\ 
  62 & MME.b & beta & beta=3 & sigma=2 & n=200 & 13791.21 \\ 
  63 & PWM & beta & beta=3 & sigma=2 & n=200 & 1.99 \\ 
  64 & MLE & sigma & beta=3 & sigma=2 & n=200 & 4.81 \\ 
  65 & MLE.b & sigma & beta=3 & sigma=2 & n=200 & 4.42 \\ 
  66 & LME & sigma & beta=3 & sigma=2 & n=200 & 1.50 \\ 
  67 & MDE.Phi.chisq & sigma & beta=3 & sigma=2 & n=200 & 121.36 \\ 
  68 & MDE.Phi.tv & sigma & beta=3 & sigma=2 & n=200 & 78.89 \\ 
  69 & MDE.Phi.kl & sigma & beta=3 & sigma=2 & n=200 & 4.44 \\ 
  70 & MME & sigma & beta=3 & sigma=2 & n=200 & 9.35 \\ 
  71 & MME.b & sigma & beta=3 & sigma=2 & n=200 & 10225.97 \\ 
  72 & PWM & sigma & beta=3 & sigma=2 & n=200 & 1.50 \\ 
  73 & MLE & beta & beta=4 & sigma=2 & n=200 & 43727.97 \\ 
  74 & MLE.b & beta & beta=4 & sigma=2 & n=200 & 43727.78 \\ 
  75 & LME & beta & beta=4 & sigma=2 & n=200 & 23.92 \\ 
  76 & MDE.Phi.chisq & beta & beta=4 & sigma=2 & n=200 & 499.75 \\ 
  77 & MDE.Phi.tv & beta & beta=4 & sigma=2 & n=200 & 334.36 \\ 
  78 & MDE.Phi.kl & beta & beta=4 & sigma=2 & n=200 & 53.85 \\ 
  79 & MME & beta & beta=4 & sigma=2 & n=200 & 373.20 \\ 
  80 & MME.b & beta & beta=4 & sigma=2 & n=200 & 6125049.19 \\ 
  81 & PWM & beta & beta=4 & sigma=2 & n=200 & 23.92 \\ 
  82 & MLE & sigma & beta=4 & sigma=2 & n=200 & 15950.81 \\ 
  83 & MLE.b & sigma & beta=4 & sigma=2 & n=200 & 15950.73 \\ 
  84 & LME & sigma & beta=4 & sigma=2 & n=200 & 8.91 \\ 
  85 & MDE.Phi.chisq & sigma & beta=4 & sigma=2 & n=200 & 325.75 \\ 
  86 & MDE.Phi.tv & sigma & beta=4 & sigma=2 & n=200 & 206.13 \\ 
  87 & MDE.Phi.kl & sigma & beta=4 & sigma=2 & n=200 & 19.44 \\ 
  88 & MME & sigma & beta=4 & sigma=2 & n=200 & 128.46 \\ 
  89 & MME.b & sigma & beta=4 & sigma=2 & n=200 & 2425203.85 \\ 
  90 & PWM & sigma & beta=4 & sigma=2 & n=200 & 8.91 \\ 
  91 & MLE & beta & beta=5 & sigma=2 & n=200 & 239435.77 \\ 
  92 & MLE.b & beta & beta=5 & sigma=2 & n=200 & 239436.62 \\ 
  93 & LME & beta & beta=5 & sigma=2 & n=200 & 64.92 \\ 
  94 & MDE.Phi.chisq & beta & beta=5 & sigma=2 & n=200 & 1308.81 \\ 
  95 & MDE.Phi.tv & beta & beta=5 & sigma=2 & n=200 & 882.94 \\ 
  96 & MDE.Phi.kl & beta & beta=5 & sigma=2 & n=200 & 152.89 \\ 
  97 & MME & beta & beta=5 & sigma=2 & n=200 & 1359.56 \\ 
  98 & MME.b & beta & beta=5 & sigma=2 & n=200 & 17526.03 \\ 
  99 & PWM & beta & beta=5 & sigma=2 & n=200 & 64.92 \\ 
  100 & MLE & sigma & beta=5 & sigma=2 & n=200 & 50772.89 \\ 
  101 & MLE.b & sigma & beta=5 & sigma=2 & n=200 & 50773.07 \\ 
  102 & LME & sigma & beta=5 & sigma=2 & n=200 & 14.23 \\ 
  103 & MDE.Phi.chisq & sigma & beta=5 & sigma=2 & n=200 & 509.51 \\ 
  104 & MDE.Phi.tv & sigma & beta=5 & sigma=2 & n=200 & 322.05 \\ 
  105 & MDE.Phi.kl & sigma & beta=5 & sigma=2 & n=200 & 33.90 \\ 
  106 & MME & sigma & beta=5 & sigma=2 & n=200 & 292.79 \\ 
  107 & MME.b & sigma & beta=5 & sigma=2 & n=200 & 3766.56 \\ 
  108 & PWM & sigma & beta=5 & sigma=2 & n=200 & 14.23 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220215/20220213-13h28-Full.beta=1.5.sig=3.n=200.LaTeX.tex <==
% START DATE AND TIME=20220213-13h28
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=1.5,  \sigma=3$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.5737&1.4914&1.7059&0.1403&0.9979&1.5737&2.4961&2.2948&1.7059
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
3.2297&2.9712&3.6057&3.6506&3.7689&3.2297&8.3936&7.5579&3.6057
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1006&0.0759&0.1096&76.8946&0.1708&0.1006&0.1638&0.1915&0.1096
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.9558&0.7093&1.0689&15.2329&2.4628&0.9558&39.6758&37.4263&1.0689
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.0737&-0.0086&0.2059&-1.3597&-0.5021&0.0737&0.9961&0.7948&0.2059
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.2297&-0.0288&0.6057&0.6506&0.7689&0.2297&5.3936&4.5579&0.6057
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.106&0.076&0.152&78.7358&0.4229&0.106&1.1561&0.8232&0.152
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
1.0085&0.7101&1.4356&15.6547&3.0538&1.0085&68.7626&58.1971&1.4356
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 1.1144&0.7861&1.5876&94.3905&3.4768&1.1145&69.9187&59.0203&1.5876\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 6e-04&6e-04&6e-04&1.07212035094377e+300&0.0304&6e-04&0.0088&0.0087&6e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220215/20220213-13h28-Full.beta=2.5.sig=3.n=200.LaTeX.tex <==
% START DATE AND TIME=20220213-13h28
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2.5,  \sigma=3$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.7638&2.4525&2.793&2.0907&2.2926&2.7638&3.598&3.703&2.793
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
3.4269&2.9215&3.4481&4.1343&4.2472&3.4269&5.0234&5.1512&3.4481
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.0591&0.7475&0.8951&18.0554&13.2403&1.0589&1.7388&977.7111&0.8951
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
2.7073&1.8853&2.3154&79.7506&59.9366&2.7068&4.5127&2842.5483&2.3154
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.2638&-0.0475&0.293&-0.4093&-0.2074&0.2638&1.098&1.203&0.293
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.4269&-0.0785&0.4481&1.1343&1.2472&0.4269&2.0234&2.1512&0.4481
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.1286&0.7497&0.9809&18.2211&13.282&1.1284&2.9444&979.0605&0.9809
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
2.8893&1.8912&2.5159&81.0293&61.4861&2.8887&8.6062&2846.8915&2.5159
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 4.0179&2.6409&3.4968&99.2504&74.7681&4.0171&11.5506&3825.952&3.4968\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&6e-04&5e-04&0.0174&0.0121&5e-04&0.0011&0.0017&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220215/20220213-13h28-Full.beta=2.sig=3.n=200.LaTeX.tex <==
% START DATE AND TIME=20220213-13h28
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=2,  \sigma=3$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.1509&1.9786&2.2244&1.3425&1.5611&2.1509&2.9788&2.6734&2.2244
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
3.3247&2.9539&3.4514&3.5795&3.8324&3.3247&5.6952&4.9332&3.4514
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.3276&0.2132&0.3063&5.3254&0.8051&0.3276&0.5666&3.8997&0.3063
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
1.494&0.9665&1.3903&29.9829&6.4335&1.4941&2.7971&18.0138&1.3903
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1509&-0.0214&0.2244&-0.6575&-0.4389&0.1509&0.9788&0.6734&0.2244
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.3247&-0.0461&0.4514&0.5795&0.8324&0.3247&2.6952&1.9332&0.4514
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.3503&0.2136&0.3566&5.7571&0.9976&0.3503&1.5245&4.3529&0.3566
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
1.5993&0.9685&1.5939&30.3157&7.1257&1.5994&10.0606&21.7491&1.5939
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 1.9496&1.1821&1.9505&36.0728&8.1234&1.9497&11.5851&26.102&1.9505\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&5e-04&5e-04&3.97147385408803e+298&0.0166&5e-04&0.0024&0.0027&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220215/20220213-13h28-Full.beta=3.sig=3.n=200.LaTeX.tex <==
% START DATE AND TIME=20220213-13h28
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=3,  \sigma=3$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 3.4361&2.9785&3.3721&3.2638&3.2683&3.4338&4.3093&6.586&3.3721
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
3.5685&2.9751&3.4633&5.2519&4.9187&3.5651&4.8323&7.7376&3.4633
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 5.864&5.531&1.8476&80.9396&52.9284&5.1886&9.8172&13779.7265&1.8476
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
10.5097&9.9405&3.1543&238.5195&155.3912&9.1733&17.6882&22988.2823&3.1543
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.4361&-0.0215&0.3721&0.2638&0.2683&0.4338&1.3093&3.586&0.3721
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.5685&-0.0249&0.4633&2.2519&1.9187&0.5651&1.8323&4.7376&0.4633
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 6.0536&5.5309&1.9859&81.0011&52.9951&5.3762&11.5306&13791.2077&1.9859
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
10.8318&9.9401&3.3686&243.5666&159.057&9.4917&21.0437&23008.4282&3.3686
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 16.8854&15.471&5.3545&324.5677&212.0522&14.868&32.5743&36799.6358&5.3545\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&5e-04&5e-04&0.0143&0.0097&5e-04&7e-04&0.0021&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220215/20220213-13h28-Full.beta=4.sig=3.n=200.LaTeX.tex <==
% START DATE AND TIME=20220213-13h28
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=4,  \sigma=3$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 8.2545&7.5812&4.961&7.5825&6.6423&5.3335&6.6323&36.3872&4.961
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
6.8662&6.2471&3.8632&8.7988&7.2652&4.2133&5.4461&33.5144&3.8632
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 38088.8056&38093.8922&22.9957&427.6843&287.9375&49.1879&366.3062&6124612.3417&22.9957
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
31294.8459&31299.0529&19.2954&611.9313&392.0447&39.9102&283.078&5456322.8246&19.2954
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 4.2545&3.5812&0.961&3.5825&2.6423&1.3335&2.6323&32.3872&0.961
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
3.8662&3.2471&0.8632&5.7988&4.2652&1.2133&2.4461&30.5144&0.8632
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 38103.0974&38102.9076&23.9168&440.476&294.8902&50.9612&373.1988&6125048.8125&23.9168
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
31306.664&31306.4666&20.0386&645.4962&410.1972&41.3784&289.0329&5456708.3182&20.0386
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 69409.7614&69409.3743&43.9554&1085.9722&705.0874&92.3396&662.2317&11581757.1307&43.9554\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&6e-04&5e-04&0.0112&0.0074&5e-04&6e-04&0.0041&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220215/20220213-13h28-Full.beta=5.sig=3.n=200.LaTeX.tex <==
% START DATE AND TIME=20220213-13h28
      \begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
      \cline{2-11}    \multicolumn{1}{r|}{} &       & \multicolumn{9}{c|}{$\beta=5,  \sigma=3$ $n=200$} \\
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.chisq}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 19.6806&18.9744&6.7416&14.2282&11.5266&7.7247&9.7827&21.1825&6.7416
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
13.1458&12.647&4.2124&12.8847&9.8849&4.9223&6.4081&14.5035&4.2124
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 220471.2518&220492.3394&55.4473&1059.8893&726.9847&133.1513&1266.8233&16995.4416&55.4473
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
105148.3979&105158.6732&27.1389&908.7044&585.6139&66.5237&615.5281&8220.8766&27.1389
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 14.6806&13.9744&1.7416&9.2282&6.5266&2.7247&4.7827&16.1825&1.7416
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
10.1458&9.647&1.2124&9.8847&6.8849&1.9223&3.4081&11.5035&1.2124
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 220664.7252&220665.575&58.475&1144.9431&769.5088&140.562&1289.5711&17255.6149&58.475
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
105240.8199&105241.2213&28.606&1006.3201&632.9573&70.2122&627.0815&8352.3845&28.606
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 325905.5452&325906.7963&87.0811&2151.2632&1402.4661&210.7743&1916.6526&25607.9994&87.0811\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&6e-04&5e-04&0.0095&0.0062&5e-04&5e-04&0.0255&5e-04\\
\hline
\end{tabular}
\end{table}

==> Tables20220525/output/output20220215/20220213-13h28-Output.accuracy.LaTeX.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Mon Feb 14 15:15:09 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & Measure & beta=1.5 & sigma=3 & n=200 & 1.11 \\ 
  2 & MLE.b & Measure & beta=1.5 & sigma=3 & n=200 & 0.79 \\ 
  3 & LME & Measure & beta=1.5 & sigma=3 & n=200 & 1.59 \\ 
  4 & MDE.Phi.chisq & Measure & beta=1.5 & sigma=3 & n=200 & 94.39 \\ 
  5 & MDE.Phi.tv & Measure & beta=1.5 & sigma=3 & n=200 & 3.48 \\ 
  6 & MDE.Phi.kl & Measure & beta=1.5 & sigma=3 & n=200 & 1.11 \\ 
  7 & MME & Measure & beta=1.5 & sigma=3 & n=200 & 69.92 \\ 
  8 & MME.b & Measure & beta=1.5 & sigma=3 & n=200 & 59.02 \\ 
  9 & PWM & Measure & beta=1.5 & sigma=3 & n=200 & 1.59 \\ 
  10 & MLE & Measure & beta=2 & sigma=3 & n=200 & 1.95 \\ 
  11 & MLE.b & Measure & beta=2 & sigma=3 & n=200 & 1.18 \\ 
  12 & LME & Measure & beta=2 & sigma=3 & n=200 & 1.95 \\ 
  13 & MDE.Phi.chisq & Measure & beta=2 & sigma=3 & n=200 & 36.07 \\ 
  14 & MDE.Phi.tv & Measure & beta=2 & sigma=3 & n=200 & 8.12 \\ 
  15 & MDE.Phi.kl & Measure & beta=2 & sigma=3 & n=200 & 1.95 \\ 
  16 & MME & Measure & beta=2 & sigma=3 & n=200 & 11.59 \\ 
  17 & MME.b & Measure & beta=2 & sigma=3 & n=200 & 26.10 \\ 
  18 & PWM & Measure & beta=2 & sigma=3 & n=200 & 1.95 \\ 
  19 & MLE & Measure & beta=2.5 & sigma=3 & n=200 & 4.02 \\ 
  20 & MLE.b & Measure & beta=2.5 & sigma=3 & n=200 & 2.64 \\ 
  21 & LME & Measure & beta=2.5 & sigma=3 & n=200 & 3.50 \\ 
  22 & MDE.Phi.chisq & Measure & beta=2.5 & sigma=3 & n=200 & 99.25 \\ 
  23 & MDE.Phi.tv & Measure & beta=2.5 & sigma=3 & n=200 & 74.77 \\ 
  24 & MDE.Phi.kl & Measure & beta=2.5 & sigma=3 & n=200 & 4.02 \\ 
  25 & MME & Measure & beta=2.5 & sigma=3 & n=200 & 11.55 \\ 
  26 & MME.b & Measure & beta=2.5 & sigma=3 & n=200 & 3825.95 \\ 
  27 & PWM & Measure & beta=2.5 & sigma=3 & n=200 & 3.50 \\ 
  28 & MLE & Measure & beta=3 & sigma=3 & n=200 & 16.89 \\ 
  29 & MLE.b & Measure & beta=3 & sigma=3 & n=200 & 15.47 \\ 
  30 & LME & Measure & beta=3 & sigma=3 & n=200 & 5.35 \\ 
  31 & MDE.Phi.chisq & Measure & beta=3 & sigma=3 & n=200 & 324.57 \\ 
  32 & MDE.Phi.tv & Measure & beta=3 & sigma=3 & n=200 & 212.05 \\ 
  33 & MDE.Phi.kl & Measure & beta=3 & sigma=3 & n=200 & 14.87 \\ 
  34 & MME & Measure & beta=3 & sigma=3 & n=200 & 32.57 \\ 
  35 & MME.b & Measure & beta=3 & sigma=3 & n=200 & 36799.64 \\ 
  36 & PWM & Measure & beta=3 & sigma=3 & n=200 & 5.35 \\ 
  37 & MLE & Measure & beta=4 & sigma=3 & n=200 & 69409.76 \\ 
  38 & MLE.b & Measure & beta=4 & sigma=3 & n=200 & 69409.37 \\ 
  39 & LME & Measure & beta=4 & sigma=3 & n=200 & 43.96 \\ 
  40 & MDE.Phi.chisq & Measure & beta=4 & sigma=3 & n=200 & 1085.97 \\ 
  41 & MDE.Phi.tv & Measure & beta=4 & sigma=3 & n=200 & 705.09 \\ 
  42 & MDE.Phi.kl & Measure & beta=4 & sigma=3 & n=200 & 92.34 \\ 
  43 & MME & Measure & beta=4 & sigma=3 & n=200 & 662.23 \\ 
  44 & MME.b & Measure & beta=4 & sigma=3 & n=200 & 11581757.13 \\ 
  45 & PWM & Measure & beta=4 & sigma=3 & n=200 & 43.96 \\ 
  46 & MLE & Measure & beta=5 & sigma=3 & n=200 & 325905.55 \\ 
  47 & MLE.b & Measure & beta=5 & sigma=3 & n=200 & 325906.80 \\ 
  48 & LME & Measure & beta=5 & sigma=3 & n=200 & 87.08 \\ 
  49 & MDE.Phi.chisq & Measure & beta=5 & sigma=3 & n=200 & 2151.26 \\ 
  50 & MDE.Phi.tv & Measure & beta=5 & sigma=3 & n=200 & 1402.47 \\ 
  51 & MDE.Phi.kl & Measure & beta=5 & sigma=3 & n=200 & 210.77 \\ 
  52 & MME & Measure & beta=5 & sigma=3 & n=200 & 1916.65 \\ 
  53 & MME.b & Measure & beta=5 & sigma=3 & n=200 & 25608.00 \\ 
  54 & PWM & Measure & beta=5 & sigma=3 & n=200 & 87.08 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220215/20220213-13h28-Output.accuracy2.LaTeX.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Mon Feb 14 15:15:09 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & Measure & beta=1.5 & sigma=3 & n=200 & 0.00 \\ 
  2 & MLE.b & Measure & beta=1.5 & sigma=3 & n=200 & 0.00 \\ 
  3 & LME & Measure & beta=1.5 & sigma=3 & n=200 & 0.00 \\ 
  4 & MDE.Phi.chisq & Measure & beta=1.5 & sigma=3 & n=200 & 1072120350943766605288668820268666400026828066468426088602280260684664282682042422400626624220844464886488668884840048482846624268606608666688240040428688880262804422608644288204008882282264804046486606222262620242240286268240260008420806662404266280688844822604066084004244220024068046226048206446886.00 \\ 
  5 & MDE.Phi.tv & Measure & beta=1.5 & sigma=3 & n=200 & 0.03 \\ 
  6 & MDE.Phi.kl & Measure & beta=1.5 & sigma=3 & n=200 & 0.00 \\ 
  7 & MME & Measure & beta=1.5 & sigma=3 & n=200 & 0.01 \\ 
  8 & MME.b & Measure & beta=1.5 & sigma=3 & n=200 & 0.01 \\ 
  9 & PWM & Measure & beta=1.5 & sigma=3 & n=200 & 0.00 \\ 
  10 & MLE & Measure & beta=2 & sigma=3 & n=200 & 0.00 \\ 
  11 & MLE.b & Measure & beta=2 & sigma=3 & n=200 & 0.00 \\ 
  12 & LME & Measure & beta=2 & sigma=3 & n=200 & 0.00 \\ 
  13 & MDE.Phi.chisq & Measure & beta=2 & sigma=3 & n=200 & 39714738540880314608828444668240686266286288864482882206084406466266042608864886046042668266840604000688864688424080002466222248606624260882442668280028082486206646846408222420200884446244828484666088402466224026062282842644260640002608822280862602846664280402028488446624606086408022846202222460682.00 \\ 
  14 & MDE.Phi.tv & Measure & beta=2 & sigma=3 & n=200 & 0.02 \\ 
  15 & MDE.Phi.kl & Measure & beta=2 & sigma=3 & n=200 & 0.00 \\ 
  16 & MME & Measure & beta=2 & sigma=3 & n=200 & 0.00 \\ 
  17 & MME.b & Measure & beta=2 & sigma=3 & n=200 & 0.00 \\ 
  18 & PWM & Measure & beta=2 & sigma=3 & n=200 & 0.00 \\ 
  19 & MLE & Measure & beta=2.5 & sigma=3 & n=200 & 0.00 \\ 
  20 & MLE.b & Measure & beta=2.5 & sigma=3 & n=200 & 0.00 \\ 
  21 & LME & Measure & beta=2.5 & sigma=3 & n=200 & 0.00 \\ 
  22 & MDE.Phi.chisq & Measure & beta=2.5 & sigma=3 & n=200 & 0.02 \\ 
  23 & MDE.Phi.tv & Measure & beta=2.5 & sigma=3 & n=200 & 0.01 \\ 
  24 & MDE.Phi.kl & Measure & beta=2.5 & sigma=3 & n=200 & 0.00 \\ 
  25 & MME & Measure & beta=2.5 & sigma=3 & n=200 & 0.00 \\ 
  26 & MME.b & Measure & beta=2.5 & sigma=3 & n=200 & 0.00 \\ 
  27 & PWM & Measure & beta=2.5 & sigma=3 & n=200 & 0.00 \\ 
  28 & MLE & Measure & beta=3 & sigma=3 & n=200 & 0.00 \\ 
  29 & MLE.b & Measure & beta=3 & sigma=3 & n=200 & 0.00 \\ 
  30 & LME & Measure & beta=3 & sigma=3 & n=200 & 0.00 \\ 
  31 & MDE.Phi.chisq & Measure & beta=3 & sigma=3 & n=200 & 0.01 \\ 
  32 & MDE.Phi.tv & Measure & beta=3 & sigma=3 & n=200 & 0.01 \\ 
  33 & MDE.Phi.kl & Measure & beta=3 & sigma=3 & n=200 & 0.00 \\ 
  34 & MME & Measure & beta=3 & sigma=3 & n=200 & 0.00 \\ 
  35 & MME.b & Measure & beta=3 & sigma=3 & n=200 & 0.00 \\ 
  36 & PWM & Measure & beta=3 & sigma=3 & n=200 & 0.00 \\ 
  37 & MLE & Measure & beta=4 & sigma=3 & n=200 & 0.00 \\ 
  38 & MLE.b & Measure & beta=4 & sigma=3 & n=200 & 0.00 \\ 
  39 & LME & Measure & beta=4 & sigma=3 & n=200 & 0.00 \\ 
  40 & MDE.Phi.chisq & Measure & beta=4 & sigma=3 & n=200 & 0.01 \\ 
  41 & MDE.Phi.tv & Measure & beta=4 & sigma=3 & n=200 & 0.01 \\ 
  42 & MDE.Phi.kl & Measure & beta=4 & sigma=3 & n=200 & 0.00 \\ 
  43 & MME & Measure & beta=4 & sigma=3 & n=200 & 0.00 \\ 
  44 & MME.b & Measure & beta=4 & sigma=3 & n=200 & 0.00 \\ 
  45 & PWM & Measure & beta=4 & sigma=3 & n=200 & 0.00 \\ 
  46 & MLE & Measure & beta=5 & sigma=3 & n=200 & 0.00 \\ 
  47 & MLE.b & Measure & beta=5 & sigma=3 & n=200 & 0.00 \\ 
  48 & LME & Measure & beta=5 & sigma=3 & n=200 & 0.00 \\ 
  49 & MDE.Phi.chisq & Measure & beta=5 & sigma=3 & n=200 & 0.01 \\ 
  50 & MDE.Phi.tv & Measure & beta=5 & sigma=3 & n=200 & 0.01 \\ 
  51 & MDE.Phi.kl & Measure & beta=5 & sigma=3 & n=200 & 0.00 \\ 
  52 & MME & Measure & beta=5 & sigma=3 & n=200 & 0.00 \\ 
  53 & MME.b & Measure & beta=5 & sigma=3 & n=200 & 0.03 \\ 
  54 & PWM & Measure & beta=5 & sigma=3 & n=200 & 0.00 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220215/20220213-13h28-Output.bias.LaTeX.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Mon Feb 14 15:15:09 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=3 & n=200 & 0.07 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=3 & n=200 & -0.01 \\ 
  3 & LME & beta & beta=1.5 & sigma=3 & n=200 & 0.21 \\ 
  4 & MDE.Phi.chisq & beta & beta=1.5 & sigma=3 & n=200 & -1.36 \\ 
  5 & MDE.Phi.tv & beta & beta=1.5 & sigma=3 & n=200 & -0.50 \\ 
  6 & MDE.Phi.kl & beta & beta=1.5 & sigma=3 & n=200 & 0.07 \\ 
  7 & MME & beta & beta=1.5 & sigma=3 & n=200 & 1.00 \\ 
  8 & MME.b & beta & beta=1.5 & sigma=3 & n=200 & 0.79 \\ 
  9 & PWM & beta & beta=1.5 & sigma=3 & n=200 & 0.21 \\ 
  10 & MLE & sigma & beta=1.5 & sigma=3 & n=200 & 0.23 \\ 
  11 & MLE.b & sigma & beta=1.5 & sigma=3 & n=200 & -0.03 \\ 
  12 & LME & sigma & beta=1.5 & sigma=3 & n=200 & 0.61 \\ 
  13 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=3 & n=200 & 0.65 \\ 
  14 & MDE.Phi.tv & sigma & beta=1.5 & sigma=3 & n=200 & 0.77 \\ 
  15 & MDE.Phi.kl & sigma & beta=1.5 & sigma=3 & n=200 & 0.23 \\ 
  16 & MME & sigma & beta=1.5 & sigma=3 & n=200 & 5.39 \\ 
  17 & MME.b & sigma & beta=1.5 & sigma=3 & n=200 & 4.56 \\ 
  18 & PWM & sigma & beta=1.5 & sigma=3 & n=200 & 0.61 \\ 
  19 & MLE & beta & beta=2 & sigma=3 & n=200 & 0.15 \\ 
  20 & MLE.b & beta & beta=2 & sigma=3 & n=200 & -0.02 \\ 
  21 & LME & beta & beta=2 & sigma=3 & n=200 & 0.22 \\ 
  22 & MDE.Phi.chisq & beta & beta=2 & sigma=3 & n=200 & -0.66 \\ 
  23 & MDE.Phi.tv & beta & beta=2 & sigma=3 & n=200 & -0.44 \\ 
  24 & MDE.Phi.kl & beta & beta=2 & sigma=3 & n=200 & 0.15 \\ 
  25 & MME & beta & beta=2 & sigma=3 & n=200 & 0.98 \\ 
  26 & MME.b & beta & beta=2 & sigma=3 & n=200 & 0.67 \\ 
  27 & PWM & beta & beta=2 & sigma=3 & n=200 & 0.22 \\ 
  28 & MLE & sigma & beta=2 & sigma=3 & n=200 & 0.32 \\ 
  29 & MLE.b & sigma & beta=2 & sigma=3 & n=200 & -0.05 \\ 
  30 & LME & sigma & beta=2 & sigma=3 & n=200 & 0.45 \\ 
  31 & MDE.Phi.chisq & sigma & beta=2 & sigma=3 & n=200 & 0.58 \\ 
  32 & MDE.Phi.tv & sigma & beta=2 & sigma=3 & n=200 & 0.83 \\ 
  33 & MDE.Phi.kl & sigma & beta=2 & sigma=3 & n=200 & 0.32 \\ 
  34 & MME & sigma & beta=2 & sigma=3 & n=200 & 2.70 \\ 
  35 & MME.b & sigma & beta=2 & sigma=3 & n=200 & 1.93 \\ 
  36 & PWM & sigma & beta=2 & sigma=3 & n=200 & 0.45 \\ 
  37 & MLE & beta & beta=2.5 & sigma=3 & n=200 & 0.26 \\ 
  38 & MLE.b & beta & beta=2.5 & sigma=3 & n=200 & -0.05 \\ 
  39 & LME & beta & beta=2.5 & sigma=3 & n=200 & 0.29 \\ 
  40 & MDE.Phi.chisq & beta & beta=2.5 & sigma=3 & n=200 & -0.41 \\ 
  41 & MDE.Phi.tv & beta & beta=2.5 & sigma=3 & n=200 & -0.21 \\ 
  42 & MDE.Phi.kl & beta & beta=2.5 & sigma=3 & n=200 & 0.26 \\ 
  43 & MME & beta & beta=2.5 & sigma=3 & n=200 & 1.10 \\ 
  44 & MME.b & beta & beta=2.5 & sigma=3 & n=200 & 1.20 \\ 
  45 & PWM & beta & beta=2.5 & sigma=3 & n=200 & 0.29 \\ 
  46 & MLE & sigma & beta=2.5 & sigma=3 & n=200 & 0.43 \\ 
  47 & MLE.b & sigma & beta=2.5 & sigma=3 & n=200 & -0.08 \\ 
  48 & LME & sigma & beta=2.5 & sigma=3 & n=200 & 0.45 \\ 
  49 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=3 & n=200 & 1.13 \\ 
  50 & MDE.Phi.tv & sigma & beta=2.5 & sigma=3 & n=200 & 1.25 \\ 
  51 & MDE.Phi.kl & sigma & beta=2.5 & sigma=3 & n=200 & 0.43 \\ 
  52 & MME & sigma & beta=2.5 & sigma=3 & n=200 & 2.02 \\ 
  53 & MME.b & sigma & beta=2.5 & sigma=3 & n=200 & 2.15 \\ 
  54 & PWM & sigma & beta=2.5 & sigma=3 & n=200 & 0.45 \\ 
  55 & MLE & beta & beta=3 & sigma=3 & n=200 & 0.44 \\ 
  56 & MLE.b & beta & beta=3 & sigma=3 & n=200 & -0.02 \\ 
  57 & LME & beta & beta=3 & sigma=3 & n=200 & 0.37 \\ 
  58 & MDE.Phi.chisq & beta & beta=3 & sigma=3 & n=200 & 0.26 \\ 
  59 & MDE.Phi.tv & beta & beta=3 & sigma=3 & n=200 & 0.27 \\ 
  60 & MDE.Phi.kl & beta & beta=3 & sigma=3 & n=200 & 0.43 \\ 
  61 & MME & beta & beta=3 & sigma=3 & n=200 & 1.31 \\ 
  62 & MME.b & beta & beta=3 & sigma=3 & n=200 & 3.59 \\ 
  63 & PWM & beta & beta=3 & sigma=3 & n=200 & 0.37 \\ 
  64 & MLE & sigma & beta=3 & sigma=3 & n=200 & 0.57 \\ 
  65 & MLE.b & sigma & beta=3 & sigma=3 & n=200 & -0.02 \\ 
  66 & LME & sigma & beta=3 & sigma=3 & n=200 & 0.46 \\ 
  67 & MDE.Phi.chisq & sigma & beta=3 & sigma=3 & n=200 & 2.25 \\ 
  68 & MDE.Phi.tv & sigma & beta=3 & sigma=3 & n=200 & 1.92 \\ 
  69 & MDE.Phi.kl & sigma & beta=3 & sigma=3 & n=200 & 0.57 \\ 
  70 & MME & sigma & beta=3 & sigma=3 & n=200 & 1.83 \\ 
  71 & MME.b & sigma & beta=3 & sigma=3 & n=200 & 4.74 \\ 
  72 & PWM & sigma & beta=3 & sigma=3 & n=200 & 0.46 \\ 
  73 & MLE & beta & beta=4 & sigma=3 & n=200 & 4.25 \\ 
  74 & MLE.b & beta & beta=4 & sigma=3 & n=200 & 3.58 \\ 
  75 & LME & beta & beta=4 & sigma=3 & n=200 & 0.96 \\ 
  76 & MDE.Phi.chisq & beta & beta=4 & sigma=3 & n=200 & 3.58 \\ 
  77 & MDE.Phi.tv & beta & beta=4 & sigma=3 & n=200 & 2.64 \\ 
  78 & MDE.Phi.kl & beta & beta=4 & sigma=3 & n=200 & 1.33 \\ 
  79 & MME & beta & beta=4 & sigma=3 & n=200 & 2.63 \\ 
  80 & MME.b & beta & beta=4 & sigma=3 & n=200 & 32.39 \\ 
  81 & PWM & beta & beta=4 & sigma=3 & n=200 & 0.96 \\ 
  82 & MLE & sigma & beta=4 & sigma=3 & n=200 & 3.87 \\ 
  83 & MLE.b & sigma & beta=4 & sigma=3 & n=200 & 3.25 \\ 
  84 & LME & sigma & beta=4 & sigma=3 & n=200 & 0.86 \\ 
  85 & MDE.Phi.chisq & sigma & beta=4 & sigma=3 & n=200 & 5.80 \\ 
  86 & MDE.Phi.tv & sigma & beta=4 & sigma=3 & n=200 & 4.27 \\ 
  87 & MDE.Phi.kl & sigma & beta=4 & sigma=3 & n=200 & 1.21 \\ 
  88 & MME & sigma & beta=4 & sigma=3 & n=200 & 2.45 \\ 
  89 & MME.b & sigma & beta=4 & sigma=3 & n=200 & 30.51 \\ 
  90 & PWM & sigma & beta=4 & sigma=3 & n=200 & 0.86 \\ 
  91 & MLE & beta & beta=5 & sigma=3 & n=200 & 14.68 \\ 
  92 & MLE.b & beta & beta=5 & sigma=3 & n=200 & 13.97 \\ 
  93 & LME & beta & beta=5 & sigma=3 & n=200 & 1.74 \\ 
  94 & MDE.Phi.chisq & beta & beta=5 & sigma=3 & n=200 & 9.23 \\ 
  95 & MDE.Phi.tv & beta & beta=5 & sigma=3 & n=200 & 6.53 \\ 
  96 & MDE.Phi.kl & beta & beta=5 & sigma=3 & n=200 & 2.72 \\ 
  97 & MME & beta & beta=5 & sigma=3 & n=200 & 4.78 \\ 
  98 & MME.b & beta & beta=5 & sigma=3 & n=200 & 16.18 \\ 
  99 & PWM & beta & beta=5 & sigma=3 & n=200 & 1.74 \\ 
  100 & MLE & sigma & beta=5 & sigma=3 & n=200 & 10.15 \\ 
  101 & MLE.b & sigma & beta=5 & sigma=3 & n=200 & 9.65 \\ 
  102 & LME & sigma & beta=5 & sigma=3 & n=200 & 1.21 \\ 
  103 & MDE.Phi.chisq & sigma & beta=5 & sigma=3 & n=200 & 9.88 \\ 
  104 & MDE.Phi.tv & sigma & beta=5 & sigma=3 & n=200 & 6.88 \\ 
  105 & MDE.Phi.kl & sigma & beta=5 & sigma=3 & n=200 & 1.92 \\ 
  106 & MME & sigma & beta=5 & sigma=3 & n=200 & 3.41 \\ 
  107 & MME.b & sigma & beta=5 & sigma=3 & n=200 & 11.50 \\ 
  108 & PWM & sigma & beta=5 & sigma=3 & n=200 & 1.21 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220215/20220213-13h28-Output.mse.LaTeX.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Mon Feb 14 15:15:09 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=3 & n=200 & 0.11 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=3 & n=200 & 0.08 \\ 
  3 & LME & beta & beta=1.5 & sigma=3 & n=200 & 0.15 \\ 
  4 & MDE.Phi.chisq & beta & beta=1.5 & sigma=3 & n=200 & 78.74 \\ 
  5 & MDE.Phi.tv & beta & beta=1.5 & sigma=3 & n=200 & 0.42 \\ 
  6 & MDE.Phi.kl & beta & beta=1.5 & sigma=3 & n=200 & 0.11 \\ 
  7 & MME & beta & beta=1.5 & sigma=3 & n=200 & 1.16 \\ 
  8 & MME.b & beta & beta=1.5 & sigma=3 & n=200 & 0.82 \\ 
  9 & PWM & beta & beta=1.5 & sigma=3 & n=200 & 0.15 \\ 
  10 & MLE & sigma & beta=1.5 & sigma=3 & n=200 & 1.01 \\ 
  11 & MLE.b & sigma & beta=1.5 & sigma=3 & n=200 & 0.71 \\ 
  12 & LME & sigma & beta=1.5 & sigma=3 & n=200 & 1.44 \\ 
  13 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=3 & n=200 & 15.65 \\ 
  14 & MDE.Phi.tv & sigma & beta=1.5 & sigma=3 & n=200 & 3.05 \\ 
  15 & MDE.Phi.kl & sigma & beta=1.5 & sigma=3 & n=200 & 1.01 \\ 
  16 & MME & sigma & beta=1.5 & sigma=3 & n=200 & 68.76 \\ 
  17 & MME.b & sigma & beta=1.5 & sigma=3 & n=200 & 58.20 \\ 
  18 & PWM & sigma & beta=1.5 & sigma=3 & n=200 & 1.44 \\ 
  19 & MLE & beta & beta=2 & sigma=3 & n=200 & 0.35 \\ 
  20 & MLE.b & beta & beta=2 & sigma=3 & n=200 & 0.21 \\ 
  21 & LME & beta & beta=2 & sigma=3 & n=200 & 0.36 \\ 
  22 & MDE.Phi.chisq & beta & beta=2 & sigma=3 & n=200 & 5.76 \\ 
  23 & MDE.Phi.tv & beta & beta=2 & sigma=3 & n=200 & 1.00 \\ 
  24 & MDE.Phi.kl & beta & beta=2 & sigma=3 & n=200 & 0.35 \\ 
  25 & MME & beta & beta=2 & sigma=3 & n=200 & 1.52 \\ 
  26 & MME.b & beta & beta=2 & sigma=3 & n=200 & 4.35 \\ 
  27 & PWM & beta & beta=2 & sigma=3 & n=200 & 0.36 \\ 
  28 & MLE & sigma & beta=2 & sigma=3 & n=200 & 1.60 \\ 
  29 & MLE.b & sigma & beta=2 & sigma=3 & n=200 & 0.97 \\ 
  30 & LME & sigma & beta=2 & sigma=3 & n=200 & 1.59 \\ 
  31 & MDE.Phi.chisq & sigma & beta=2 & sigma=3 & n=200 & 30.32 \\ 
  32 & MDE.Phi.tv & sigma & beta=2 & sigma=3 & n=200 & 7.13 \\ 
  33 & MDE.Phi.kl & sigma & beta=2 & sigma=3 & n=200 & 1.60 \\ 
  34 & MME & sigma & beta=2 & sigma=3 & n=200 & 10.06 \\ 
  35 & MME.b & sigma & beta=2 & sigma=3 & n=200 & 21.75 \\ 
  36 & PWM & sigma & beta=2 & sigma=3 & n=200 & 1.59 \\ 
  37 & MLE & beta & beta=2.5 & sigma=3 & n=200 & 1.13 \\ 
  38 & MLE.b & beta & beta=2.5 & sigma=3 & n=200 & 0.75 \\ 
  39 & LME & beta & beta=2.5 & sigma=3 & n=200 & 0.98 \\ 
  40 & MDE.Phi.chisq & beta & beta=2.5 & sigma=3 & n=200 & 18.22 \\ 
  41 & MDE.Phi.tv & beta & beta=2.5 & sigma=3 & n=200 & 13.28 \\ 
  42 & MDE.Phi.kl & beta & beta=2.5 & sigma=3 & n=200 & 1.13 \\ 
  43 & MME & beta & beta=2.5 & sigma=3 & n=200 & 2.94 \\ 
  44 & MME.b & beta & beta=2.5 & sigma=3 & n=200 & 979.06 \\ 
  45 & PWM & beta & beta=2.5 & sigma=3 & n=200 & 0.98 \\ 
  46 & MLE & sigma & beta=2.5 & sigma=3 & n=200 & 2.89 \\ 
  47 & MLE.b & sigma & beta=2.5 & sigma=3 & n=200 & 1.89 \\ 
  48 & LME & sigma & beta=2.5 & sigma=3 & n=200 & 2.52 \\ 
  49 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=3 & n=200 & 81.03 \\ 
  50 & MDE.Phi.tv & sigma & beta=2.5 & sigma=3 & n=200 & 61.49 \\ 
  51 & MDE.Phi.kl & sigma & beta=2.5 & sigma=3 & n=200 & 2.89 \\ 
  52 & MME & sigma & beta=2.5 & sigma=3 & n=200 & 8.61 \\ 
  53 & MME.b & sigma & beta=2.5 & sigma=3 & n=200 & 2846.89 \\ 
  54 & PWM & sigma & beta=2.5 & sigma=3 & n=200 & 2.52 \\ 
  55 & MLE & beta & beta=3 & sigma=3 & n=200 & 6.05 \\ 
  56 & MLE.b & beta & beta=3 & sigma=3 & n=200 & 5.53 \\ 
  57 & LME & beta & beta=3 & sigma=3 & n=200 & 1.99 \\ 
  58 & MDE.Phi.chisq & beta & beta=3 & sigma=3 & n=200 & 81.00 \\ 
  59 & MDE.Phi.tv & beta & beta=3 & sigma=3 & n=200 & 53.00 \\ 
  60 & MDE.Phi.kl & beta & beta=3 & sigma=3 & n=200 & 5.38 \\ 
  61 & MME & beta & beta=3 & sigma=3 & n=200 & 11.53 \\ 
  62 & MME.b & beta & beta=3 & sigma=3 & n=200 & 13791.21 \\ 
  63 & PWM & beta & beta=3 & sigma=3 & n=200 & 1.99 \\ 
  64 & MLE & sigma & beta=3 & sigma=3 & n=200 & 10.83 \\ 
  65 & MLE.b & sigma & beta=3 & sigma=3 & n=200 & 9.94 \\ 
  66 & LME & sigma & beta=3 & sigma=3 & n=200 & 3.37 \\ 
  67 & MDE.Phi.chisq & sigma & beta=3 & sigma=3 & n=200 & 243.57 \\ 
  68 & MDE.Phi.tv & sigma & beta=3 & sigma=3 & n=200 & 159.06 \\ 
  69 & MDE.Phi.kl & sigma & beta=3 & sigma=3 & n=200 & 9.49 \\ 
  70 & MME & sigma & beta=3 & sigma=3 & n=200 & 21.04 \\ 
  71 & MME.b & sigma & beta=3 & sigma=3 & n=200 & 23008.43 \\ 
  72 & PWM & sigma & beta=3 & sigma=3 & n=200 & 3.37 \\ 
  73 & MLE & beta & beta=4 & sigma=3 & n=200 & 38103.10 \\ 
  74 & MLE.b & beta & beta=4 & sigma=3 & n=200 & 38102.91 \\ 
  75 & LME & beta & beta=4 & sigma=3 & n=200 & 23.92 \\ 
  76 & MDE.Phi.chisq & beta & beta=4 & sigma=3 & n=200 & 440.48 \\ 
  77 & MDE.Phi.tv & beta & beta=4 & sigma=3 & n=200 & 294.89 \\ 
  78 & MDE.Phi.kl & beta & beta=4 & sigma=3 & n=200 & 50.96 \\ 
  79 & MME & beta & beta=4 & sigma=3 & n=200 & 373.20 \\ 
  80 & MME.b & beta & beta=4 & sigma=3 & n=200 & 6125048.81 \\ 
  81 & PWM & beta & beta=4 & sigma=3 & n=200 & 23.92 \\ 
  82 & MLE & sigma & beta=4 & sigma=3 & n=200 & 31306.66 \\ 
  83 & MLE.b & sigma & beta=4 & sigma=3 & n=200 & 31306.47 \\ 
  84 & LME & sigma & beta=4 & sigma=3 & n=200 & 20.04 \\ 
  85 & MDE.Phi.chisq & sigma & beta=4 & sigma=3 & n=200 & 645.50 \\ 
  86 & MDE.Phi.tv & sigma & beta=4 & sigma=3 & n=200 & 410.20 \\ 
  87 & MDE.Phi.kl & sigma & beta=4 & sigma=3 & n=200 & 41.38 \\ 
  88 & MME & sigma & beta=4 & sigma=3 & n=200 & 289.03 \\ 
  89 & MME.b & sigma & beta=4 & sigma=3 & n=200 & 5456708.32 \\ 
  90 & PWM & sigma & beta=4 & sigma=3 & n=200 & 20.04 \\ 
  91 & MLE & beta & beta=5 & sigma=3 & n=200 & 220664.73 \\ 
  92 & MLE.b & beta & beta=5 & sigma=3 & n=200 & 220665.57 \\ 
  93 & LME & beta & beta=5 & sigma=3 & n=200 & 58.48 \\ 
  94 & MDE.Phi.chisq & beta & beta=5 & sigma=3 & n=200 & 1144.94 \\ 
  95 & MDE.Phi.tv & beta & beta=5 & sigma=3 & n=200 & 769.51 \\ 
  96 & MDE.Phi.kl & beta & beta=5 & sigma=3 & n=200 & 140.56 \\ 
  97 & MME & beta & beta=5 & sigma=3 & n=200 & 1289.57 \\ 
  98 & MME.b & beta & beta=5 & sigma=3 & n=200 & 17255.61 \\ 
  99 & PWM & beta & beta=5 & sigma=3 & n=200 & 58.48 \\ 
  100 & MLE & sigma & beta=5 & sigma=3 & n=200 & 105240.82 \\ 
  101 & MLE.b & sigma & beta=5 & sigma=3 & n=200 & 105241.22 \\ 
  102 & LME & sigma & beta=5 & sigma=3 & n=200 & 28.61 \\ 
  103 & MDE.Phi.chisq & sigma & beta=5 & sigma=3 & n=200 & 1006.32 \\ 
  104 & MDE.Phi.tv & sigma & beta=5 & sigma=3 & n=200 & 632.96 \\ 
  105 & MDE.Phi.kl & sigma & beta=5 & sigma=3 & n=200 & 70.21 \\ 
  106 & MME & sigma & beta=5 & sigma=3 & n=200 & 627.08 \\ 
  107 & MME.b & sigma & beta=5 & sigma=3 & n=200 & 8352.38 \\ 
  108 & PWM & sigma & beta=5 & sigma=3 & n=200 & 28.61 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220215/20220213-13h28-Output.var.LaTeX.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Mon Feb 14 15:15:09 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=3 & n=200 & 0.10 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=3 & n=200 & 0.08 \\ 
  3 & LME & beta & beta=1.5 & sigma=3 & n=200 & 0.11 \\ 
  4 & MDE.Phi.chisq & beta & beta=1.5 & sigma=3 & n=200 & 76.89 \\ 
  5 & MDE.Phi.tv & beta & beta=1.5 & sigma=3 & n=200 & 0.17 \\ 
  6 & MDE.Phi.kl & beta & beta=1.5 & sigma=3 & n=200 & 0.10 \\ 
  7 & MME & beta & beta=1.5 & sigma=3 & n=200 & 0.16 \\ 
  8 & MME.b & beta & beta=1.5 & sigma=3 & n=200 & 0.19 \\ 
  9 & PWM & beta & beta=1.5 & sigma=3 & n=200 & 0.11 \\ 
  10 & MLE & sigma & beta=1.5 & sigma=3 & n=200 & 0.96 \\ 
  11 & MLE.b & sigma & beta=1.5 & sigma=3 & n=200 & 0.71 \\ 
  12 & LME & sigma & beta=1.5 & sigma=3 & n=200 & 1.07 \\ 
  13 & MDE.Phi.chisq & sigma & beta=1.5 & sigma=3 & n=200 & 15.23 \\ 
  14 & MDE.Phi.tv & sigma & beta=1.5 & sigma=3 & n=200 & 2.46 \\ 
  15 & MDE.Phi.kl & sigma & beta=1.5 & sigma=3 & n=200 & 0.96 \\ 
  16 & MME & sigma & beta=1.5 & sigma=3 & n=200 & 39.68 \\ 
  17 & MME.b & sigma & beta=1.5 & sigma=3 & n=200 & 37.43 \\ 
  18 & PWM & sigma & beta=1.5 & sigma=3 & n=200 & 1.07 \\ 
  19 & MLE & beta & beta=2 & sigma=3 & n=200 & 0.33 \\ 
  20 & MLE.b & beta & beta=2 & sigma=3 & n=200 & 0.21 \\ 
  21 & LME & beta & beta=2 & sigma=3 & n=200 & 0.31 \\ 
  22 & MDE.Phi.chisq & beta & beta=2 & sigma=3 & n=200 & 5.33 \\ 
  23 & MDE.Phi.tv & beta & beta=2 & sigma=3 & n=200 & 0.81 \\ 
  24 & MDE.Phi.kl & beta & beta=2 & sigma=3 & n=200 & 0.33 \\ 
  25 & MME & beta & beta=2 & sigma=3 & n=200 & 0.57 \\ 
  26 & MME.b & beta & beta=2 & sigma=3 & n=200 & 3.90 \\ 
  27 & PWM & beta & beta=2 & sigma=3 & n=200 & 0.31 \\ 
  28 & MLE & sigma & beta=2 & sigma=3 & n=200 & 1.49 \\ 
  29 & MLE.b & sigma & beta=2 & sigma=3 & n=200 & 0.97 \\ 
  30 & LME & sigma & beta=2 & sigma=3 & n=200 & 1.39 \\ 
  31 & MDE.Phi.chisq & sigma & beta=2 & sigma=3 & n=200 & 29.98 \\ 
  32 & MDE.Phi.tv & sigma & beta=2 & sigma=3 & n=200 & 6.43 \\ 
  33 & MDE.Phi.kl & sigma & beta=2 & sigma=3 & n=200 & 1.49 \\ 
  34 & MME & sigma & beta=2 & sigma=3 & n=200 & 2.80 \\ 
  35 & MME.b & sigma & beta=2 & sigma=3 & n=200 & 18.01 \\ 
  36 & PWM & sigma & beta=2 & sigma=3 & n=200 & 1.39 \\ 
  37 & MLE & beta & beta=2.5 & sigma=3 & n=200 & 1.06 \\ 
  38 & MLE.b & beta & beta=2.5 & sigma=3 & n=200 & 0.75 \\ 
  39 & LME & beta & beta=2.5 & sigma=3 & n=200 & 0.90 \\ 
  40 & MDE.Phi.chisq & beta & beta=2.5 & sigma=3 & n=200 & 18.06 \\ 
  41 & MDE.Phi.tv & beta & beta=2.5 & sigma=3 & n=200 & 13.24 \\ 
  42 & MDE.Phi.kl & beta & beta=2.5 & sigma=3 & n=200 & 1.06 \\ 
  43 & MME & beta & beta=2.5 & sigma=3 & n=200 & 1.74 \\ 
  44 & MME.b & beta & beta=2.5 & sigma=3 & n=200 & 977.71 \\ 
  45 & PWM & beta & beta=2.5 & sigma=3 & n=200 & 0.90 \\ 
  46 & MLE & sigma & beta=2.5 & sigma=3 & n=200 & 2.71 \\ 
  47 & MLE.b & sigma & beta=2.5 & sigma=3 & n=200 & 1.89 \\ 
  48 & LME & sigma & beta=2.5 & sigma=3 & n=200 & 2.32 \\ 
  49 & MDE.Phi.chisq & sigma & beta=2.5 & sigma=3 & n=200 & 79.75 \\ 
  50 & MDE.Phi.tv & sigma & beta=2.5 & sigma=3 & n=200 & 59.94 \\ 
  51 & MDE.Phi.kl & sigma & beta=2.5 & sigma=3 & n=200 & 2.71 \\ 
  52 & MME & sigma & beta=2.5 & sigma=3 & n=200 & 4.51 \\ 
  53 & MME.b & sigma & beta=2.5 & sigma=3 & n=200 & 2842.55 \\ 
  54 & PWM & sigma & beta=2.5 & sigma=3 & n=200 & 2.32 \\ 
  55 & MLE & beta & beta=3 & sigma=3 & n=200 & 5.86 \\ 
  56 & MLE.b & beta & beta=3 & sigma=3 & n=200 & 5.53 \\ 
  57 & LME & beta & beta=3 & sigma=3 & n=200 & 1.85 \\ 
  58 & MDE.Phi.chisq & beta & beta=3 & sigma=3 & n=200 & 80.94 \\ 
  59 & MDE.Phi.tv & beta & beta=3 & sigma=3 & n=200 & 52.93 \\ 
  60 & MDE.Phi.kl & beta & beta=3 & sigma=3 & n=200 & 5.19 \\ 
  61 & MME & beta & beta=3 & sigma=3 & n=200 & 9.82 \\ 
  62 & MME.b & beta & beta=3 & sigma=3 & n=200 & 13779.73 \\ 
  63 & PWM & beta & beta=3 & sigma=3 & n=200 & 1.85 \\ 
  64 & MLE & sigma & beta=3 & sigma=3 & n=200 & 10.51 \\ 
  65 & MLE.b & sigma & beta=3 & sigma=3 & n=200 & 9.94 \\ 
  66 & LME & sigma & beta=3 & sigma=3 & n=200 & 3.15 \\ 
  67 & MDE.Phi.chisq & sigma & beta=3 & sigma=3 & n=200 & 238.52 \\ 
  68 & MDE.Phi.tv & sigma & beta=3 & sigma=3 & n=200 & 155.39 \\ 
  69 & MDE.Phi.kl & sigma & beta=3 & sigma=3 & n=200 & 9.17 \\ 
  70 & MME & sigma & beta=3 & sigma=3 & n=200 & 17.69 \\ 
  71 & MME.b & sigma & beta=3 & sigma=3 & n=200 & 22988.28 \\ 
  72 & PWM & sigma & beta=3 & sigma=3 & n=200 & 3.15 \\ 
  73 & MLE & beta & beta=4 & sigma=3 & n=200 & 38088.81 \\ 
  74 & MLE.b & beta & beta=4 & sigma=3 & n=200 & 38093.89 \\ 
  75 & LME & beta & beta=4 & sigma=3 & n=200 & 23.00 \\ 
  76 & MDE.Phi.chisq & beta & beta=4 & sigma=3 & n=200 & 427.68 \\ 
  77 & MDE.Phi.tv & beta & beta=4 & sigma=3 & n=200 & 287.94 \\ 
  78 & MDE.Phi.kl & beta & beta=4 & sigma=3 & n=200 & 49.19 \\ 
  79 & MME & beta & beta=4 & sigma=3 & n=200 & 366.31 \\ 
  80 & MME.b & beta & beta=4 & sigma=3 & n=200 & 6124612.34 \\ 
  81 & PWM & beta & beta=4 & sigma=3 & n=200 & 23.00 \\ 
  82 & MLE & sigma & beta=4 & sigma=3 & n=200 & 31294.85 \\ 
  83 & MLE.b & sigma & beta=4 & sigma=3 & n=200 & 31299.05 \\ 
  84 & LME & sigma & beta=4 & sigma=3 & n=200 & 19.30 \\ 
  85 & MDE.Phi.chisq & sigma & beta=4 & sigma=3 & n=200 & 611.93 \\ 
  86 & MDE.Phi.tv & sigma & beta=4 & sigma=3 & n=200 & 392.04 \\ 
  87 & MDE.Phi.kl & sigma & beta=4 & sigma=3 & n=200 & 39.91 \\ 
  88 & MME & sigma & beta=4 & sigma=3 & n=200 & 283.08 \\ 
  89 & MME.b & sigma & beta=4 & sigma=3 & n=200 & 5456322.82 \\ 
  90 & PWM & sigma & beta=4 & sigma=3 & n=200 & 19.30 \\ 
  91 & MLE & beta & beta=5 & sigma=3 & n=200 & 220471.25 \\ 
  92 & MLE.b & beta & beta=5 & sigma=3 & n=200 & 220492.34 \\ 
  93 & LME & beta & beta=5 & sigma=3 & n=200 & 55.45 \\ 
  94 & MDE.Phi.chisq & beta & beta=5 & sigma=3 & n=200 & 1059.89 \\ 
  95 & MDE.Phi.tv & beta & beta=5 & sigma=3 & n=200 & 726.98 \\ 
  96 & MDE.Phi.kl & beta & beta=5 & sigma=3 & n=200 & 133.15 \\ 
  97 & MME & beta & beta=5 & sigma=3 & n=200 & 1266.82 \\ 
  98 & MME.b & beta & beta=5 & sigma=3 & n=200 & 16995.44 \\ 
  99 & PWM & beta & beta=5 & sigma=3 & n=200 & 55.45 \\ 
  100 & MLE & sigma & beta=5 & sigma=3 & n=200 & 105148.40 \\ 
  101 & MLE.b & sigma & beta=5 & sigma=3 & n=200 & 105158.67 \\ 
  102 & LME & sigma & beta=5 & sigma=3 & n=200 & 27.14 \\ 
  103 & MDE.Phi.chisq & sigma & beta=5 & sigma=3 & n=200 & 908.70 \\ 
  104 & MDE.Phi.tv & sigma & beta=5 & sigma=3 & n=200 & 585.61 \\ 
  105 & MDE.Phi.kl & sigma & beta=5 & sigma=3 & n=200 & 66.52 \\ 
  106 & MME & sigma & beta=5 & sigma=3 & n=200 & 615.53 \\ 
  107 & MME.b & sigma & beta=5 & sigma=3 & n=200 & 8220.88 \\ 
  108 & PWM & sigma & beta=5 & sigma=3 & n=200 & 27.14 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220223/20220223-11h07m58s-Full.beta=1.5.sig=1.n=100.LaTeX.tex <==
% START DATE AND TIME=20220223-11h07m58s
      \begin{table}[htbp]
  \centering
  \caption{$\beta=1.5,  \sigma=1$ $n=100$}
  \resizebox{\columnwidth}{!}{
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|r|r|}
      %\cline{2-13}    \multicolumn{1}{r|}{} &       & \multicolumn{11}{c|}{$\beta=1.5,  \sigma=1$ $n=100$} \\
\cline{2-13}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.CvM}} & \multicolumn{1}{l|}{\textbf{MDE.LS}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.X2}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.5681&1.4008&1.7528&1.576&1.4758&0.8702&1.084&1.5681&5.3002&8.1746&1.7528
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
1.0798&0.9036&1.2523&1.0855&0.9966&1.2953&1.5608&1.0798&6.535&10.4889&1.2523
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1414&0.0788&0.1263&0.2595&0.1993&0.1184&0.2456&0.1414&765.522&3059.4462&0.1263
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.1585&0.0861&0.1537&0.2574&0.1986&0.316&0.6869&0.1585&1320.0737&5283.477&0.1537
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.0681&-0.0992&0.2528&0.076&-0.0242&-0.6298&-0.416&0.0681&3.8002&6.6746&0.2528
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.0798&-0.0964&0.2523&0.0855&-0.0034&0.2953&0.5608&0.0798&5.535&9.4889&0.2523
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.146&0.0886&0.1902&0.2653&0.1999&0.515&0.4186&0.146&779.887&3103.6909&0.1902
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.1648&0.0954&0.2173&0.2647&0.1986&0.4032&1.0013&0.1648&1350.5779&5372.9875&0.2173
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 0.3109&0.184&0.4076&0.53&0.3985&0.9182&1.4199&0.3109&2130.465&8476.6784&0.4076\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0011&0.0011&0.0012&0.0012&0.0403&0.033&0.0011&0.0103&0.0117&0.0011\\
\hline
\end{tabular}
}
\end{table}

==> Tables20220525/output/output20220223/20220223-11h07m58s-Full.beta=2.5.sig=1.n=100.LaTeX.tex <==
% START DATE AND TIME=20220223-11h07m58s
      \begin{table}[htbp]
  \centering
  \caption{$\beta=2.5,  \sigma=1$ $n=100$}
  \resizebox{\columnwidth}{!}{
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|r|r|}
      %\cline{2-13}    \multicolumn{1}{r|}{} &       & \multicolumn{11}{c|}{$\beta=2.5,  \sigma=1$ $n=100$} \\
\cline{2-13}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.CvM}} & \multicolumn{1}{l|}{\textbf{MDE.LS}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.X2}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.2347&1.8686&2.2979&2.3103&2.1123&1.2966&1.6571&2.2347&16.9083&31.2559&2.2979
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.8763&0.6783&0.8977&0.9113&0.818&0.945&1.163&0.8763&10.547&19.9925&0.8977
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.2293&0.0876&0.1796&0.5969&0.4086&0.1526&0.361&0.2293&94221.9057&376880.4733&0.1796
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.0725&0.0282&0.0601&0.1578&0.1098&0.1134&0.2848&0.0725&46154.2735&184616.1735&0.0601
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & -0.2653&-0.6314&-0.2021&-0.1897&-0.3877&-1.2034&-0.8429&-0.2653&14.4083&28.7559&-0.2021
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
-0.1237&-0.3217&-0.1023&-0.0887&-0.182&-0.055&0.163&-0.1237&9.547&18.9925&-0.1023
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.2997&0.4863&0.2204&0.6328&0.5588&1.6007&1.0716&0.2997&94420.0825&377669.6848&0.2204
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.0878&0.1317&0.0706&0.1657&0.1429&0.1165&0.3113&0.0878&46240.8042&184958.4253&0.0706
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 0.3875&0.6179&0.291&0.7985&0.7017&1.7172&1.3829&0.3875&140660.8867&562628.1101&0.291\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 9e-04&0.0011&9e-04&0.001&0.001&0.0278&0.0213&9e-04&0.0038&0.0049&9e-04\\
\hline
\end{tabular}
}
\end{table}

==> Tables20220525/output/output20220223/20220223-11h07m58s-Full.beta=2.sig=1.n=100.LaTeX.tex <==
% START DATE AND TIME=20220223-11h07m58s
      \begin{table}[htbp]
  \centering
  \caption{$\beta=2,  \sigma=1$ $n=100$}
  \resizebox{\columnwidth}{!}{
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|r|r|}
      %\cline{2-13}    \multicolumn{1}{r|}{} &       & \multicolumn{11}{c|}{$\beta=2,  \sigma=1$ $n=100$} \\
\cline{2-13}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.CvM}} & \multicolumn{1}{l|}{\textbf{MDE.LS}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.X2}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.9446&1.6748&2.0675&1.9557&1.809&1.1273&1.4275&1.9446&70.9308&139.3487&2.0675
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.9732&0.7799&1.0435&0.9775&0.8873&1.1049&1.3489&0.9732&52.0352&102.5279&1.0435
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.2035&0.0911&0.1682&0.4167&0.3037&0.1507&0.3307&0.2035&28202779.5777&112811067.0066&0.1682
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.1094&0.0487&0.0959&0.1896&0.14&0.189&0.4325&0.1094&13767086.386&55068399.7816&0.0959
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & -0.0554&-0.3252&0.0675&-0.0443&-0.191&-0.8727&-0.5725&-0.0554&68.9308&137.3487&0.0675
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
-0.0268&-0.2201&0.0435&-0.0225&-0.1127&0.1049&0.3489&-0.0268&51.0352&101.5279&0.0435
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.2066&0.1968&0.1728&0.4186&0.3402&0.9122&0.6584&0.2066&28204710.7531&112818650.5739&0.1728
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.1101&0.0972&0.0978&0.1901&0.1527&0.2&0.5542&0.1101&13768314.2664&55073200.853&0.0978
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 0.3167&0.294&0.2705&0.6087&0.4929&1.1122&1.2126&0.3167&41973025.0195&167891851.4269&0.2705\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.001&0.0011&0.001&0.0011&0.0011&0.0318&0.025&0.001&0.0055&0.0068&0.001\\
\hline
\end{tabular}
}
\end{table}

==> Tables20220525/output/output20220223/20220223-11h07m58s-Full.beta=3.sig=1.n=100.LaTeX.tex <==
% START DATE AND TIME=20220223-11h07m58s
      \begin{table}[htbp]
  \centering
  \caption{$\beta=3,  \sigma=1$ $n=100$}
  \resizebox{\columnwidth}{!}{
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|r|r|}
      %\cline{2-13}    \multicolumn{1}{r|}{} &       & \multicolumn{11}{c|}{$\beta=3,  \sigma=1$ $n=100$} \\
\cline{2-13}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.CvM}} & \multicolumn{1}{l|}{\textbf{MDE.LS}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.X2}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.4746&2.0175&2.4971&2.603&2.3574&1.4284&1.8329&2.4746&20.5023&38.409&2.4971
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.7981&0.6003&0.7982&0.8483&0.7544&0.8295&1.0221&0.7981&9.947&19.0331&0.7982
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.2495&0.0935&0.1828&0.8067&0.5153&0.146&0.368&0.2495&30010.0267&120033.1831&0.1828
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.0495&0.0192&0.0386&0.1373&0.0894&0.0719&0.1927&0.0495&7636.737&30546.5727&0.0386
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & -0.5254&-0.9825&-0.5029&-0.397&-0.6426&-1.5716&-1.1671&-0.5254&17.5023&35.409&-0.5029
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
-0.2019&-0.3997&-0.2018&-0.1517&-0.2456&-0.1705&0.0221&-0.2019&8.947&18.0331&-0.2018
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.5256&1.0587&0.4357&0.9642&0.9282&2.6159&1.7301&0.5256&30313.3561&121274.9749&0.4357
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.0902&0.179&0.0794&0.1603&0.1497&0.1009&0.1932&0.0902&7716.0217&30868.7123&0.0794
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 0.6158&1.2377&0.5151&1.1245&1.0779&2.7168&1.9232&0.6158&38029.3778&152143.6873&0.5151\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 9e-04&0.0011&9e-04&0.001&0.001&0.0256&0.0193&9e-04&0.0032&0.0041&9e-04\\
\hline
\end{tabular}
}
\end{table}

==> Tables20220525/output/output20220223/20220223-11h07m58s-Output.accuracy.LaTeX.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Wed Feb 23 14:33:40 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & Measure & beta=1.5 & sigma=1 & n=100 & 0.31 \\ 
  2 & MLE.b & Measure & beta=1.5 & sigma=1 & n=100 & 0.18 \\ 
  3 & LME & Measure & beta=1.5 & sigma=1 & n=100 & 0.41 \\ 
  4 & MDE.CvM & Measure & beta=1.5 & sigma=1 & n=100 & 0.53 \\ 
  5 & MDE.LS & Measure & beta=1.5 & sigma=1 & n=100 & 0.40 \\ 
  6 & MDE.Phi.X2 & Measure & beta=1.5 & sigma=1 & n=100 & 0.92 \\ 
  7 & MDE.Phi.tv & Measure & beta=1.5 & sigma=1 & n=100 & 1.42 \\ 
  8 & MDE.Phi.kl & Measure & beta=1.5 & sigma=1 & n=100 & 0.31 \\ 
  9 & MME & Measure & beta=1.5 & sigma=1 & n=100 & 2130.46 \\ 
  10 & MME.b & Measure & beta=1.5 & sigma=1 & n=100 & 8476.68 \\ 
  11 & PWM & Measure & beta=1.5 & sigma=1 & n=100 & 0.41 \\ 
  12 & MLE & Measure & beta=2 & sigma=1 & n=100 & 0.32 \\ 
  13 & MLE.b & Measure & beta=2 & sigma=1 & n=100 & 0.29 \\ 
  14 & LME & Measure & beta=2 & sigma=1 & n=100 & 0.27 \\ 
  15 & MDE.CvM & Measure & beta=2 & sigma=1 & n=100 & 0.61 \\ 
  16 & MDE.LS & Measure & beta=2 & sigma=1 & n=100 & 0.49 \\ 
  17 & MDE.Phi.X2 & Measure & beta=2 & sigma=1 & n=100 & 1.11 \\ 
  18 & MDE.Phi.tv & Measure & beta=2 & sigma=1 & n=100 & 1.21 \\ 
  19 & MDE.Phi.kl & Measure & beta=2 & sigma=1 & n=100 & 0.32 \\ 
  20 & MME & Measure & beta=2 & sigma=1 & n=100 & 41973025.02 \\ 
  21 & MME.b & Measure & beta=2 & sigma=1 & n=100 & 167891851.43 \\ 
  22 & PWM & Measure & beta=2 & sigma=1 & n=100 & 0.27 \\ 
  23 & MLE & Measure & beta=2.5 & sigma=1 & n=100 & 0.39 \\ 
  24 & MLE.b & Measure & beta=2.5 & sigma=1 & n=100 & 0.62 \\ 
  25 & LME & Measure & beta=2.5 & sigma=1 & n=100 & 0.29 \\ 
  26 & MDE.CvM & Measure & beta=2.5 & sigma=1 & n=100 & 0.80 \\ 
  27 & MDE.LS & Measure & beta=2.5 & sigma=1 & n=100 & 0.70 \\ 
  28 & MDE.Phi.X2 & Measure & beta=2.5 & sigma=1 & n=100 & 1.72 \\ 
  29 & MDE.Phi.tv & Measure & beta=2.5 & sigma=1 & n=100 & 1.38 \\ 
  30 & MDE.Phi.kl & Measure & beta=2.5 & sigma=1 & n=100 & 0.39 \\ 
  31 & MME & Measure & beta=2.5 & sigma=1 & n=100 & 140660.89 \\ 
  32 & MME.b & Measure & beta=2.5 & sigma=1 & n=100 & 562628.11 \\ 
  33 & PWM & Measure & beta=2.5 & sigma=1 & n=100 & 0.29 \\ 
  34 & MLE & Measure & beta=3 & sigma=1 & n=100 & 0.62 \\ 
  35 & MLE.b & Measure & beta=3 & sigma=1 & n=100 & 1.24 \\ 
  36 & LME & Measure & beta=3 & sigma=1 & n=100 & 0.52 \\ 
  37 & MDE.CvM & Measure & beta=3 & sigma=1 & n=100 & 1.12 \\ 
  38 & MDE.LS & Measure & beta=3 & sigma=1 & n=100 & 1.08 \\ 
  39 & MDE.Phi.X2 & Measure & beta=3 & sigma=1 & n=100 & 2.72 \\ 
  40 & MDE.Phi.tv & Measure & beta=3 & sigma=1 & n=100 & 1.92 \\ 
  41 & MDE.Phi.kl & Measure & beta=3 & sigma=1 & n=100 & 0.62 \\ 
  42 & MME & Measure & beta=3 & sigma=1 & n=100 & 38029.38 \\ 
  43 & MME.b & Measure & beta=3 & sigma=1 & n=100 & 152143.69 \\ 
  44 & PWM & Measure & beta=3 & sigma=1 & n=100 & 0.52 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220223/20220223-11h07m58s-Output.accuracy2.LaTeX.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Wed Feb 23 14:33:40 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & Measure & beta=1.5 & sigma=1 & n=100 & 0.00 \\ 
  2 & MLE.b & Measure & beta=1.5 & sigma=1 & n=100 & 0.00 \\ 
  3 & LME & Measure & beta=1.5 & sigma=1 & n=100 & 0.00 \\ 
  4 & MDE.CvM & Measure & beta=1.5 & sigma=1 & n=100 & 0.00 \\ 
  5 & MDE.LS & Measure & beta=1.5 & sigma=1 & n=100 & 0.00 \\ 
  6 & MDE.Phi.X2 & Measure & beta=1.5 & sigma=1 & n=100 & 0.04 \\ 
  7 & MDE.Phi.tv & Measure & beta=1.5 & sigma=1 & n=100 & 0.03 \\ 
  8 & MDE.Phi.kl & Measure & beta=1.5 & sigma=1 & n=100 & 0.00 \\ 
  9 & MME & Measure & beta=1.5 & sigma=1 & n=100 & 0.01 \\ 
  10 & MME.b & Measure & beta=1.5 & sigma=1 & n=100 & 0.01 \\ 
  11 & PWM & Measure & beta=1.5 & sigma=1 & n=100 & 0.00 \\ 
  12 & MLE & Measure & beta=2 & sigma=1 & n=100 & 0.00 \\ 
  13 & MLE.b & Measure & beta=2 & sigma=1 & n=100 & 0.00 \\ 
  14 & LME & Measure & beta=2 & sigma=1 & n=100 & 0.00 \\ 
  15 & MDE.CvM & Measure & beta=2 & sigma=1 & n=100 & 0.00 \\ 
  16 & MDE.LS & Measure & beta=2 & sigma=1 & n=100 & 0.00 \\ 
  17 & MDE.Phi.X2 & Measure & beta=2 & sigma=1 & n=100 & 0.03 \\ 
  18 & MDE.Phi.tv & Measure & beta=2 & sigma=1 & n=100 & 0.03 \\ 
  19 & MDE.Phi.kl & Measure & beta=2 & sigma=1 & n=100 & 0.00 \\ 
  20 & MME & Measure & beta=2 & sigma=1 & n=100 & 0.01 \\ 
  21 & MME.b & Measure & beta=2 & sigma=1 & n=100 & 0.01 \\ 
  22 & PWM & Measure & beta=2 & sigma=1 & n=100 & 0.00 \\ 
  23 & MLE & Measure & beta=2.5 & sigma=1 & n=100 & 0.00 \\ 
  24 & MLE.b & Measure & beta=2.5 & sigma=1 & n=100 & 0.00 \\ 
  25 & LME & Measure & beta=2.5 & sigma=1 & n=100 & 0.00 \\ 
  26 & MDE.CvM & Measure & beta=2.5 & sigma=1 & n=100 & 0.00 \\ 
  27 & MDE.LS & Measure & beta=2.5 & sigma=1 & n=100 & 0.00 \\ 
  28 & MDE.Phi.X2 & Measure & beta=2.5 & sigma=1 & n=100 & 0.03 \\ 
  29 & MDE.Phi.tv & Measure & beta=2.5 & sigma=1 & n=100 & 0.02 \\ 
  30 & MDE.Phi.kl & Measure & beta=2.5 & sigma=1 & n=100 & 0.00 \\ 
  31 & MME & Measure & beta=2.5 & sigma=1 & n=100 & 0.00 \\ 
  32 & MME.b & Measure & beta=2.5 & sigma=1 & n=100 & 0.00 \\ 
  33 & PWM & Measure & beta=2.5 & sigma=1 & n=100 & 0.00 \\ 
  34 & MLE & Measure & beta=3 & sigma=1 & n=100 & 0.00 \\ 
  35 & MLE.b & Measure & beta=3 & sigma=1 & n=100 & 0.00 \\ 
  36 & LME & Measure & beta=3 & sigma=1 & n=100 & 0.00 \\ 
  37 & MDE.CvM & Measure & beta=3 & sigma=1 & n=100 & 0.00 \\ 
  38 & MDE.LS & Measure & beta=3 & sigma=1 & n=100 & 0.00 \\ 
  39 & MDE.Phi.X2 & Measure & beta=3 & sigma=1 & n=100 & 0.03 \\ 
  40 & MDE.Phi.tv & Measure & beta=3 & sigma=1 & n=100 & 0.02 \\ 
  41 & MDE.Phi.kl & Measure & beta=3 & sigma=1 & n=100 & 0.00 \\ 
  42 & MME & Measure & beta=3 & sigma=1 & n=100 & 0.00 \\ 
  43 & MME.b & Measure & beta=3 & sigma=1 & n=100 & 0.00 \\ 
  44 & PWM & Measure & beta=3 & sigma=1 & n=100 & 0.00 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220223/20220223-11h07m58s-Output.bias.LaTeX.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Wed Feb 23 14:33:40 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=1 & n=100 & 0.07 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=1 & n=100 & -0.10 \\ 
  3 & LME & beta & beta=1.5 & sigma=1 & n=100 & 0.25 \\ 
  4 & MDE.CvM & beta & beta=1.5 & sigma=1 & n=100 & 0.08 \\ 
  5 & MDE.LS & beta & beta=1.5 & sigma=1 & n=100 & -0.02 \\ 
  6 & MDE.Phi.X2 & beta & beta=1.5 & sigma=1 & n=100 & -0.63 \\ 
  7 & MDE.Phi.tv & beta & beta=1.5 & sigma=1 & n=100 & -0.42 \\ 
  8 & MDE.Phi.kl & beta & beta=1.5 & sigma=1 & n=100 & 0.07 \\ 
  9 & MME & beta & beta=1.5 & sigma=1 & n=100 & 3.80 \\ 
  10 & MME.b & beta & beta=1.5 & sigma=1 & n=100 & 6.67 \\ 
  11 & PWM & beta & beta=1.5 & sigma=1 & n=100 & 0.25 \\ 
  12 & MLE & sigma & beta=1.5 & sigma=1 & n=100 & 0.08 \\ 
  13 & MLE.b & sigma & beta=1.5 & sigma=1 & n=100 & -0.10 \\ 
  14 & LME & sigma & beta=1.5 & sigma=1 & n=100 & 0.25 \\ 
  15 & MDE.CvM & sigma & beta=1.5 & sigma=1 & n=100 & 0.09 \\ 
  16 & MDE.LS & sigma & beta=1.5 & sigma=1 & n=100 & -0.00 \\ 
  17 & MDE.Phi.X2 & sigma & beta=1.5 & sigma=1 & n=100 & 0.30 \\ 
  18 & MDE.Phi.tv & sigma & beta=1.5 & sigma=1 & n=100 & 0.56 \\ 
  19 & MDE.Phi.kl & sigma & beta=1.5 & sigma=1 & n=100 & 0.08 \\ 
  20 & MME & sigma & beta=1.5 & sigma=1 & n=100 & 5.53 \\ 
  21 & MME.b & sigma & beta=1.5 & sigma=1 & n=100 & 9.49 \\ 
  22 & PWM & sigma & beta=1.5 & sigma=1 & n=100 & 0.25 \\ 
  23 & MLE & beta & beta=2 & sigma=1 & n=100 & -0.06 \\ 
  24 & MLE.b & beta & beta=2 & sigma=1 & n=100 & -0.33 \\ 
  25 & LME & beta & beta=2 & sigma=1 & n=100 & 0.07 \\ 
  26 & MDE.CvM & beta & beta=2 & sigma=1 & n=100 & -0.04 \\ 
  27 & MDE.LS & beta & beta=2 & sigma=1 & n=100 & -0.19 \\ 
  28 & MDE.Phi.X2 & beta & beta=2 & sigma=1 & n=100 & -0.87 \\ 
  29 & MDE.Phi.tv & beta & beta=2 & sigma=1 & n=100 & -0.57 \\ 
  30 & MDE.Phi.kl & beta & beta=2 & sigma=1 & n=100 & -0.06 \\ 
  31 & MME & beta & beta=2 & sigma=1 & n=100 & 68.93 \\ 
  32 & MME.b & beta & beta=2 & sigma=1 & n=100 & 137.35 \\ 
  33 & PWM & beta & beta=2 & sigma=1 & n=100 & 0.07 \\ 
  34 & MLE & sigma & beta=2 & sigma=1 & n=100 & -0.03 \\ 
  35 & MLE.b & sigma & beta=2 & sigma=1 & n=100 & -0.22 \\ 
  36 & LME & sigma & beta=2 & sigma=1 & n=100 & 0.04 \\ 
  37 & MDE.CvM & sigma & beta=2 & sigma=1 & n=100 & -0.02 \\ 
  38 & MDE.LS & sigma & beta=2 & sigma=1 & n=100 & -0.11 \\ 
  39 & MDE.Phi.X2 & sigma & beta=2 & sigma=1 & n=100 & 0.10 \\ 
  40 & MDE.Phi.tv & sigma & beta=2 & sigma=1 & n=100 & 0.35 \\ 
  41 & MDE.Phi.kl & sigma & beta=2 & sigma=1 & n=100 & -0.03 \\ 
  42 & MME & sigma & beta=2 & sigma=1 & n=100 & 51.04 \\ 
  43 & MME.b & sigma & beta=2 & sigma=1 & n=100 & 101.53 \\ 
  44 & PWM & sigma & beta=2 & sigma=1 & n=100 & 0.04 \\ 
  45 & MLE & beta & beta=2.5 & sigma=1 & n=100 & -0.27 \\ 
  46 & MLE.b & beta & beta=2.5 & sigma=1 & n=100 & -0.63 \\ 
  47 & LME & beta & beta=2.5 & sigma=1 & n=100 & -0.20 \\ 
  48 & MDE.CvM & beta & beta=2.5 & sigma=1 & n=100 & -0.19 \\ 
  49 & MDE.LS & beta & beta=2.5 & sigma=1 & n=100 & -0.39 \\ 
  50 & MDE.Phi.X2 & beta & beta=2.5 & sigma=1 & n=100 & -1.20 \\ 
  51 & MDE.Phi.tv & beta & beta=2.5 & sigma=1 & n=100 & -0.84 \\ 
  52 & MDE.Phi.kl & beta & beta=2.5 & sigma=1 & n=100 & -0.27 \\ 
  53 & MME & beta & beta=2.5 & sigma=1 & n=100 & 14.41 \\ 
  54 & MME.b & beta & beta=2.5 & sigma=1 & n=100 & 28.76 \\ 
  55 & PWM & beta & beta=2.5 & sigma=1 & n=100 & -0.20 \\ 
  56 & MLE & sigma & beta=2.5 & sigma=1 & n=100 & -0.12 \\ 
  57 & MLE.b & sigma & beta=2.5 & sigma=1 & n=100 & -0.32 \\ 
  58 & LME & sigma & beta=2.5 & sigma=1 & n=100 & -0.10 \\ 
  59 & MDE.CvM & sigma & beta=2.5 & sigma=1 & n=100 & -0.09 \\ 
  60 & MDE.LS & sigma & beta=2.5 & sigma=1 & n=100 & -0.18 \\ 
  61 & MDE.Phi.X2 & sigma & beta=2.5 & sigma=1 & n=100 & -0.06 \\ 
  62 & MDE.Phi.tv & sigma & beta=2.5 & sigma=1 & n=100 & 0.16 \\ 
  63 & MDE.Phi.kl & sigma & beta=2.5 & sigma=1 & n=100 & -0.12 \\ 
  64 & MME & sigma & beta=2.5 & sigma=1 & n=100 & 9.55 \\ 
  65 & MME.b & sigma & beta=2.5 & sigma=1 & n=100 & 18.99 \\ 
  66 & PWM & sigma & beta=2.5 & sigma=1 & n=100 & -0.10 \\ 
  67 & MLE & beta & beta=3 & sigma=1 & n=100 & -0.53 \\ 
  68 & MLE.b & beta & beta=3 & sigma=1 & n=100 & -0.98 \\ 
  69 & LME & beta & beta=3 & sigma=1 & n=100 & -0.50 \\ 
  70 & MDE.CvM & beta & beta=3 & sigma=1 & n=100 & -0.40 \\ 
  71 & MDE.LS & beta & beta=3 & sigma=1 & n=100 & -0.64 \\ 
  72 & MDE.Phi.X2 & beta & beta=3 & sigma=1 & n=100 & -1.57 \\ 
  73 & MDE.Phi.tv & beta & beta=3 & sigma=1 & n=100 & -1.17 \\ 
  74 & MDE.Phi.kl & beta & beta=3 & sigma=1 & n=100 & -0.53 \\ 
  75 & MME & beta & beta=3 & sigma=1 & n=100 & 17.50 \\ 
  76 & MME.b & beta & beta=3 & sigma=1 & n=100 & 35.41 \\ 
  77 & PWM & beta & beta=3 & sigma=1 & n=100 & -0.50 \\ 
  78 & MLE & sigma & beta=3 & sigma=1 & n=100 & -0.20 \\ 
  79 & MLE.b & sigma & beta=3 & sigma=1 & n=100 & -0.40 \\ 
  80 & LME & sigma & beta=3 & sigma=1 & n=100 & -0.20 \\ 
  81 & MDE.CvM & sigma & beta=3 & sigma=1 & n=100 & -0.15 \\ 
  82 & MDE.LS & sigma & beta=3 & sigma=1 & n=100 & -0.25 \\ 
  83 & MDE.Phi.X2 & sigma & beta=3 & sigma=1 & n=100 & -0.17 \\ 
  84 & MDE.Phi.tv & sigma & beta=3 & sigma=1 & n=100 & 0.02 \\ 
  85 & MDE.Phi.kl & sigma & beta=3 & sigma=1 & n=100 & -0.20 \\ 
  86 & MME & sigma & beta=3 & sigma=1 & n=100 & 8.95 \\ 
  87 & MME.b & sigma & beta=3 & sigma=1 & n=100 & 18.03 \\ 
  88 & PWM & sigma & beta=3 & sigma=1 & n=100 & -0.20 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220223/20220223-11h07m58s-Output.mean.LaTeX.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Wed Feb 23 14:33:40 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=1 & n=100 & 1.57 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=1 & n=100 & 1.40 \\ 
  3 & LME & beta & beta=1.5 & sigma=1 & n=100 & 1.75 \\ 
  4 & MDE.CvM & beta & beta=1.5 & sigma=1 & n=100 & 1.58 \\ 
  5 & MDE.LS & beta & beta=1.5 & sigma=1 & n=100 & 1.48 \\ 
  6 & MDE.Phi.X2 & beta & beta=1.5 & sigma=1 & n=100 & 0.87 \\ 
  7 & MDE.Phi.tv & beta & beta=1.5 & sigma=1 & n=100 & 1.08 \\ 
  8 & MDE.Phi.kl & beta & beta=1.5 & sigma=1 & n=100 & 1.57 \\ 
  9 & MME & beta & beta=1.5 & sigma=1 & n=100 & 5.30 \\ 
  10 & MME.b & beta & beta=1.5 & sigma=1 & n=100 & 8.17 \\ 
  11 & PWM & beta & beta=1.5 & sigma=1 & n=100 & 1.75 \\ 
  12 & MLE & sigma & beta=1.5 & sigma=1 & n=100 & 1.08 \\ 
  13 & MLE.b & sigma & beta=1.5 & sigma=1 & n=100 & 0.90 \\ 
  14 & LME & sigma & beta=1.5 & sigma=1 & n=100 & 1.25 \\ 
  15 & MDE.CvM & sigma & beta=1.5 & sigma=1 & n=100 & 1.09 \\ 
  16 & MDE.LS & sigma & beta=1.5 & sigma=1 & n=100 & 1.00 \\ 
  17 & MDE.Phi.X2 & sigma & beta=1.5 & sigma=1 & n=100 & 1.30 \\ 
  18 & MDE.Phi.tv & sigma & beta=1.5 & sigma=1 & n=100 & 1.56 \\ 
  19 & MDE.Phi.kl & sigma & beta=1.5 & sigma=1 & n=100 & 1.08 \\ 
  20 & MME & sigma & beta=1.5 & sigma=1 & n=100 & 6.53 \\ 
  21 & MME.b & sigma & beta=1.5 & sigma=1 & n=100 & 10.49 \\ 
  22 & PWM & sigma & beta=1.5 & sigma=1 & n=100 & 1.25 \\ 
  23 & MLE & beta & beta=2 & sigma=1 & n=100 & 1.94 \\ 
  24 & MLE.b & beta & beta=2 & sigma=1 & n=100 & 1.67 \\ 
  25 & LME & beta & beta=2 & sigma=1 & n=100 & 2.07 \\ 
  26 & MDE.CvM & beta & beta=2 & sigma=1 & n=100 & 1.96 \\ 
  27 & MDE.LS & beta & beta=2 & sigma=1 & n=100 & 1.81 \\ 
  28 & MDE.Phi.X2 & beta & beta=2 & sigma=1 & n=100 & 1.13 \\ 
  29 & MDE.Phi.tv & beta & beta=2 & sigma=1 & n=100 & 1.43 \\ 
  30 & MDE.Phi.kl & beta & beta=2 & sigma=1 & n=100 & 1.94 \\ 
  31 & MME & beta & beta=2 & sigma=1 & n=100 & 70.93 \\ 
  32 & MME.b & beta & beta=2 & sigma=1 & n=100 & 139.35 \\ 
  33 & PWM & beta & beta=2 & sigma=1 & n=100 & 2.07 \\ 
  34 & MLE & sigma & beta=2 & sigma=1 & n=100 & 0.97 \\ 
  35 & MLE.b & sigma & beta=2 & sigma=1 & n=100 & 0.78 \\ 
  36 & LME & sigma & beta=2 & sigma=1 & n=100 & 1.04 \\ 
  37 & MDE.CvM & sigma & beta=2 & sigma=1 & n=100 & 0.98 \\ 
  38 & MDE.LS & sigma & beta=2 & sigma=1 & n=100 & 0.89 \\ 
  39 & MDE.Phi.X2 & sigma & beta=2 & sigma=1 & n=100 & 1.10 \\ 
  40 & MDE.Phi.tv & sigma & beta=2 & sigma=1 & n=100 & 1.35 \\ 
  41 & MDE.Phi.kl & sigma & beta=2 & sigma=1 & n=100 & 0.97 \\ 
  42 & MME & sigma & beta=2 & sigma=1 & n=100 & 52.04 \\ 
  43 & MME.b & sigma & beta=2 & sigma=1 & n=100 & 102.53 \\ 
  44 & PWM & sigma & beta=2 & sigma=1 & n=100 & 1.04 \\ 
  45 & MLE & beta & beta=2.5 & sigma=1 & n=100 & 2.23 \\ 
  46 & MLE.b & beta & beta=2.5 & sigma=1 & n=100 & 1.87 \\ 
  47 & LME & beta & beta=2.5 & sigma=1 & n=100 & 2.30 \\ 
  48 & MDE.CvM & beta & beta=2.5 & sigma=1 & n=100 & 2.31 \\ 
  49 & MDE.LS & beta & beta=2.5 & sigma=1 & n=100 & 2.11 \\ 
  50 & MDE.Phi.X2 & beta & beta=2.5 & sigma=1 & n=100 & 1.30 \\ 
  51 & MDE.Phi.tv & beta & beta=2.5 & sigma=1 & n=100 & 1.66 \\ 
  52 & MDE.Phi.kl & beta & beta=2.5 & sigma=1 & n=100 & 2.23 \\ 
  53 & MME & beta & beta=2.5 & sigma=1 & n=100 & 16.91 \\ 
  54 & MME.b & beta & beta=2.5 & sigma=1 & n=100 & 31.26 \\ 
  55 & PWM & beta & beta=2.5 & sigma=1 & n=100 & 2.30 \\ 
  56 & MLE & sigma & beta=2.5 & sigma=1 & n=100 & 0.88 \\ 
  57 & MLE.b & sigma & beta=2.5 & sigma=1 & n=100 & 0.68 \\ 
  58 & LME & sigma & beta=2.5 & sigma=1 & n=100 & 0.90 \\ 
  59 & MDE.CvM & sigma & beta=2.5 & sigma=1 & n=100 & 0.91 \\ 
  60 & MDE.LS & sigma & beta=2.5 & sigma=1 & n=100 & 0.82 \\ 
  61 & MDE.Phi.X2 & sigma & beta=2.5 & sigma=1 & n=100 & 0.94 \\ 
  62 & MDE.Phi.tv & sigma & beta=2.5 & sigma=1 & n=100 & 1.16 \\ 
  63 & MDE.Phi.kl & sigma & beta=2.5 & sigma=1 & n=100 & 0.88 \\ 
  64 & MME & sigma & beta=2.5 & sigma=1 & n=100 & 10.55 \\ 
  65 & MME.b & sigma & beta=2.5 & sigma=1 & n=100 & 19.99 \\ 
  66 & PWM & sigma & beta=2.5 & sigma=1 & n=100 & 0.90 \\ 
  67 & MLE & beta & beta=3 & sigma=1 & n=100 & 2.47 \\ 
  68 & MLE.b & beta & beta=3 & sigma=1 & n=100 & 2.02 \\ 
  69 & LME & beta & beta=3 & sigma=1 & n=100 & 2.50 \\ 
  70 & MDE.CvM & beta & beta=3 & sigma=1 & n=100 & 2.60 \\ 
  71 & MDE.LS & beta & beta=3 & sigma=1 & n=100 & 2.36 \\ 
  72 & MDE.Phi.X2 & beta & beta=3 & sigma=1 & n=100 & 1.43 \\ 
  73 & MDE.Phi.tv & beta & beta=3 & sigma=1 & n=100 & 1.83 \\ 
  74 & MDE.Phi.kl & beta & beta=3 & sigma=1 & n=100 & 2.47 \\ 
  75 & MME & beta & beta=3 & sigma=1 & n=100 & 20.50 \\ 
  76 & MME.b & beta & beta=3 & sigma=1 & n=100 & 38.41 \\ 
  77 & PWM & beta & beta=3 & sigma=1 & n=100 & 2.50 \\ 
  78 & MLE & sigma & beta=3 & sigma=1 & n=100 & 0.80 \\ 
  79 & MLE.b & sigma & beta=3 & sigma=1 & n=100 & 0.60 \\ 
  80 & LME & sigma & beta=3 & sigma=1 & n=100 & 0.80 \\ 
  81 & MDE.CvM & sigma & beta=3 & sigma=1 & n=100 & 0.85 \\ 
  82 & MDE.LS & sigma & beta=3 & sigma=1 & n=100 & 0.75 \\ 
  83 & MDE.Phi.X2 & sigma & beta=3 & sigma=1 & n=100 & 0.83 \\ 
  84 & MDE.Phi.tv & sigma & beta=3 & sigma=1 & n=100 & 1.02 \\ 
  85 & MDE.Phi.kl & sigma & beta=3 & sigma=1 & n=100 & 0.80 \\ 
  86 & MME & sigma & beta=3 & sigma=1 & n=100 & 9.95 \\ 
  87 & MME.b & sigma & beta=3 & sigma=1 & n=100 & 19.03 \\ 
  88 & PWM & sigma & beta=3 & sigma=1 & n=100 & 0.80 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220223/20220223-11h07m58s-Output.mse.LaTeX.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Wed Feb 23 14:33:40 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=1 & n=100 & 0.15 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=1 & n=100 & 0.09 \\ 
  3 & LME & beta & beta=1.5 & sigma=1 & n=100 & 0.19 \\ 
  4 & MDE.CvM & beta & beta=1.5 & sigma=1 & n=100 & 0.27 \\ 
  5 & MDE.LS & beta & beta=1.5 & sigma=1 & n=100 & 0.20 \\ 
  6 & MDE.Phi.X2 & beta & beta=1.5 & sigma=1 & n=100 & 0.52 \\ 
  7 & MDE.Phi.tv & beta & beta=1.5 & sigma=1 & n=100 & 0.42 \\ 
  8 & MDE.Phi.kl & beta & beta=1.5 & sigma=1 & n=100 & 0.15 \\ 
  9 & MME & beta & beta=1.5 & sigma=1 & n=100 & 779.89 \\ 
  10 & MME.b & beta & beta=1.5 & sigma=1 & n=100 & 3103.69 \\ 
  11 & PWM & beta & beta=1.5 & sigma=1 & n=100 & 0.19 \\ 
  12 & MLE & sigma & beta=1.5 & sigma=1 & n=100 & 0.16 \\ 
  13 & MLE.b & sigma & beta=1.5 & sigma=1 & n=100 & 0.10 \\ 
  14 & LME & sigma & beta=1.5 & sigma=1 & n=100 & 0.22 \\ 
  15 & MDE.CvM & sigma & beta=1.5 & sigma=1 & n=100 & 0.26 \\ 
  16 & MDE.LS & sigma & beta=1.5 & sigma=1 & n=100 & 0.20 \\ 
  17 & MDE.Phi.X2 & sigma & beta=1.5 & sigma=1 & n=100 & 0.40 \\ 
  18 & MDE.Phi.tv & sigma & beta=1.5 & sigma=1 & n=100 & 1.00 \\ 
  19 & MDE.Phi.kl & sigma & beta=1.5 & sigma=1 & n=100 & 0.16 \\ 
  20 & MME & sigma & beta=1.5 & sigma=1 & n=100 & 1350.58 \\ 
  21 & MME.b & sigma & beta=1.5 & sigma=1 & n=100 & 5372.99 \\ 
  22 & PWM & sigma & beta=1.5 & sigma=1 & n=100 & 0.22 \\ 
  23 & MLE & beta & beta=2 & sigma=1 & n=100 & 0.21 \\ 
  24 & MLE.b & beta & beta=2 & sigma=1 & n=100 & 0.20 \\ 
  25 & LME & beta & beta=2 & sigma=1 & n=100 & 0.17 \\ 
  26 & MDE.CvM & beta & beta=2 & sigma=1 & n=100 & 0.42 \\ 
  27 & MDE.LS & beta & beta=2 & sigma=1 & n=100 & 0.34 \\ 
  28 & MDE.Phi.X2 & beta & beta=2 & sigma=1 & n=100 & 0.91 \\ 
  29 & MDE.Phi.tv & beta & beta=2 & sigma=1 & n=100 & 0.66 \\ 
  30 & MDE.Phi.kl & beta & beta=2 & sigma=1 & n=100 & 0.21 \\ 
  31 & MME & beta & beta=2 & sigma=1 & n=100 & 28204710.75 \\ 
  32 & MME.b & beta & beta=2 & sigma=1 & n=100 & 112818650.57 \\ 
  33 & PWM & beta & beta=2 & sigma=1 & n=100 & 0.17 \\ 
  34 & MLE & sigma & beta=2 & sigma=1 & n=100 & 0.11 \\ 
  35 & MLE.b & sigma & beta=2 & sigma=1 & n=100 & 0.10 \\ 
  36 & LME & sigma & beta=2 & sigma=1 & n=100 & 0.10 \\ 
  37 & MDE.CvM & sigma & beta=2 & sigma=1 & n=100 & 0.19 \\ 
  38 & MDE.LS & sigma & beta=2 & sigma=1 & n=100 & 0.15 \\ 
  39 & MDE.Phi.X2 & sigma & beta=2 & sigma=1 & n=100 & 0.20 \\ 
  40 & MDE.Phi.tv & sigma & beta=2 & sigma=1 & n=100 & 0.55 \\ 
  41 & MDE.Phi.kl & sigma & beta=2 & sigma=1 & n=100 & 0.11 \\ 
  42 & MME & sigma & beta=2 & sigma=1 & n=100 & 13768314.27 \\ 
  43 & MME.b & sigma & beta=2 & sigma=1 & n=100 & 55073200.85 \\ 
  44 & PWM & sigma & beta=2 & sigma=1 & n=100 & 0.10 \\ 
  45 & MLE & beta & beta=2.5 & sigma=1 & n=100 & 0.30 \\ 
  46 & MLE.b & beta & beta=2.5 & sigma=1 & n=100 & 0.49 \\ 
  47 & LME & beta & beta=2.5 & sigma=1 & n=100 & 0.22 \\ 
  48 & MDE.CvM & beta & beta=2.5 & sigma=1 & n=100 & 0.63 \\ 
  49 & MDE.LS & beta & beta=2.5 & sigma=1 & n=100 & 0.56 \\ 
  50 & MDE.Phi.X2 & beta & beta=2.5 & sigma=1 & n=100 & 1.60 \\ 
  51 & MDE.Phi.tv & beta & beta=2.5 & sigma=1 & n=100 & 1.07 \\ 
  52 & MDE.Phi.kl & beta & beta=2.5 & sigma=1 & n=100 & 0.30 \\ 
  53 & MME & beta & beta=2.5 & sigma=1 & n=100 & 94420.08 \\ 
  54 & MME.b & beta & beta=2.5 & sigma=1 & n=100 & 377669.68 \\ 
  55 & PWM & beta & beta=2.5 & sigma=1 & n=100 & 0.22 \\ 
  56 & MLE & sigma & beta=2.5 & sigma=1 & n=100 & 0.09 \\ 
  57 & MLE.b & sigma & beta=2.5 & sigma=1 & n=100 & 0.13 \\ 
  58 & LME & sigma & beta=2.5 & sigma=1 & n=100 & 0.07 \\ 
  59 & MDE.CvM & sigma & beta=2.5 & sigma=1 & n=100 & 0.17 \\ 
  60 & MDE.LS & sigma & beta=2.5 & sigma=1 & n=100 & 0.14 \\ 
  61 & MDE.Phi.X2 & sigma & beta=2.5 & sigma=1 & n=100 & 0.12 \\ 
  62 & MDE.Phi.tv & sigma & beta=2.5 & sigma=1 & n=100 & 0.31 \\ 
  63 & MDE.Phi.kl & sigma & beta=2.5 & sigma=1 & n=100 & 0.09 \\ 
  64 & MME & sigma & beta=2.5 & sigma=1 & n=100 & 46240.80 \\ 
  65 & MME.b & sigma & beta=2.5 & sigma=1 & n=100 & 184958.43 \\ 
  66 & PWM & sigma & beta=2.5 & sigma=1 & n=100 & 0.07 \\ 
  67 & MLE & beta & beta=3 & sigma=1 & n=100 & 0.53 \\ 
  68 & MLE.b & beta & beta=3 & sigma=1 & n=100 & 1.06 \\ 
  69 & LME & beta & beta=3 & sigma=1 & n=100 & 0.44 \\ 
  70 & MDE.CvM & beta & beta=3 & sigma=1 & n=100 & 0.96 \\ 
  71 & MDE.LS & beta & beta=3 & sigma=1 & n=100 & 0.93 \\ 
  72 & MDE.Phi.X2 & beta & beta=3 & sigma=1 & n=100 & 2.62 \\ 
  73 & MDE.Phi.tv & beta & beta=3 & sigma=1 & n=100 & 1.73 \\ 
  74 & MDE.Phi.kl & beta & beta=3 & sigma=1 & n=100 & 0.53 \\ 
  75 & MME & beta & beta=3 & sigma=1 & n=100 & 30313.36 \\ 
  76 & MME.b & beta & beta=3 & sigma=1 & n=100 & 121274.97 \\ 
  77 & PWM & beta & beta=3 & sigma=1 & n=100 & 0.44 \\ 
  78 & MLE & sigma & beta=3 & sigma=1 & n=100 & 0.09 \\ 
  79 & MLE.b & sigma & beta=3 & sigma=1 & n=100 & 0.18 \\ 
  80 & LME & sigma & beta=3 & sigma=1 & n=100 & 0.08 \\ 
  81 & MDE.CvM & sigma & beta=3 & sigma=1 & n=100 & 0.16 \\ 
  82 & MDE.LS & sigma & beta=3 & sigma=1 & n=100 & 0.15 \\ 
  83 & MDE.Phi.X2 & sigma & beta=3 & sigma=1 & n=100 & 0.10 \\ 
  84 & MDE.Phi.tv & sigma & beta=3 & sigma=1 & n=100 & 0.19 \\ 
  85 & MDE.Phi.kl & sigma & beta=3 & sigma=1 & n=100 & 0.09 \\ 
  86 & MME & sigma & beta=3 & sigma=1 & n=100 & 7716.02 \\ 
  87 & MME.b & sigma & beta=3 & sigma=1 & n=100 & 30868.71 \\ 
  88 & PWM & sigma & beta=3 & sigma=1 & n=100 & 0.08 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220223/20220223-11h07m58s-Output.var.LaTeX.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Wed Feb 23 14:33:40 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=1 & n=100 & 0.14 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=1 & n=100 & 0.08 \\ 
  3 & LME & beta & beta=1.5 & sigma=1 & n=100 & 0.13 \\ 
  4 & MDE.CvM & beta & beta=1.5 & sigma=1 & n=100 & 0.26 \\ 
  5 & MDE.LS & beta & beta=1.5 & sigma=1 & n=100 & 0.20 \\ 
  6 & MDE.Phi.X2 & beta & beta=1.5 & sigma=1 & n=100 & 0.12 \\ 
  7 & MDE.Phi.tv & beta & beta=1.5 & sigma=1 & n=100 & 0.25 \\ 
  8 & MDE.Phi.kl & beta & beta=1.5 & sigma=1 & n=100 & 0.14 \\ 
  9 & MME & beta & beta=1.5 & sigma=1 & n=100 & 765.52 \\ 
  10 & MME.b & beta & beta=1.5 & sigma=1 & n=100 & 3059.45 \\ 
  11 & PWM & beta & beta=1.5 & sigma=1 & n=100 & 0.13 \\ 
  12 & MLE & sigma & beta=1.5 & sigma=1 & n=100 & 0.16 \\ 
  13 & MLE.b & sigma & beta=1.5 & sigma=1 & n=100 & 0.09 \\ 
  14 & LME & sigma & beta=1.5 & sigma=1 & n=100 & 0.15 \\ 
  15 & MDE.CvM & sigma & beta=1.5 & sigma=1 & n=100 & 0.26 \\ 
  16 & MDE.LS & sigma & beta=1.5 & sigma=1 & n=100 & 0.20 \\ 
  17 & MDE.Phi.X2 & sigma & beta=1.5 & sigma=1 & n=100 & 0.32 \\ 
  18 & MDE.Phi.tv & sigma & beta=1.5 & sigma=1 & n=100 & 0.69 \\ 
  19 & MDE.Phi.kl & sigma & beta=1.5 & sigma=1 & n=100 & 0.16 \\ 
  20 & MME & sigma & beta=1.5 & sigma=1 & n=100 & 1320.07 \\ 
  21 & MME.b & sigma & beta=1.5 & sigma=1 & n=100 & 5283.48 \\ 
  22 & PWM & sigma & beta=1.5 & sigma=1 & n=100 & 0.15 \\ 
  23 & MLE & beta & beta=2 & sigma=1 & n=100 & 0.20 \\ 
  24 & MLE.b & beta & beta=2 & sigma=1 & n=100 & 0.09 \\ 
  25 & LME & beta & beta=2 & sigma=1 & n=100 & 0.17 \\ 
  26 & MDE.CvM & beta & beta=2 & sigma=1 & n=100 & 0.42 \\ 
  27 & MDE.LS & beta & beta=2 & sigma=1 & n=100 & 0.30 \\ 
  28 & MDE.Phi.X2 & beta & beta=2 & sigma=1 & n=100 & 0.15 \\ 
  29 & MDE.Phi.tv & beta & beta=2 & sigma=1 & n=100 & 0.33 \\ 
  30 & MDE.Phi.kl & beta & beta=2 & sigma=1 & n=100 & 0.20 \\ 
  31 & MME & beta & beta=2 & sigma=1 & n=100 & 28202779.58 \\ 
  32 & MME.b & beta & beta=2 & sigma=1 & n=100 & 112811067.01 \\ 
  33 & PWM & beta & beta=2 & sigma=1 & n=100 & 0.17 \\ 
  34 & MLE & sigma & beta=2 & sigma=1 & n=100 & 0.11 \\ 
  35 & MLE.b & sigma & beta=2 & sigma=1 & n=100 & 0.05 \\ 
  36 & LME & sigma & beta=2 & sigma=1 & n=100 & 0.10 \\ 
  37 & MDE.CvM & sigma & beta=2 & sigma=1 & n=100 & 0.19 \\ 
  38 & MDE.LS & sigma & beta=2 & sigma=1 & n=100 & 0.14 \\ 
  39 & MDE.Phi.X2 & sigma & beta=2 & sigma=1 & n=100 & 0.19 \\ 
  40 & MDE.Phi.tv & sigma & beta=2 & sigma=1 & n=100 & 0.43 \\ 
  41 & MDE.Phi.kl & sigma & beta=2 & sigma=1 & n=100 & 0.11 \\ 
  42 & MME & sigma & beta=2 & sigma=1 & n=100 & 13767086.39 \\ 
  43 & MME.b & sigma & beta=2 & sigma=1 & n=100 & 55068399.78 \\ 
  44 & PWM & sigma & beta=2 & sigma=1 & n=100 & 0.10 \\ 
  45 & MLE & beta & beta=2.5 & sigma=1 & n=100 & 0.23 \\ 
  46 & MLE.b & beta & beta=2.5 & sigma=1 & n=100 & 0.09 \\ 
  47 & LME & beta & beta=2.5 & sigma=1 & n=100 & 0.18 \\ 
  48 & MDE.CvM & beta & beta=2.5 & sigma=1 & n=100 & 0.60 \\ 
  49 & MDE.LS & beta & beta=2.5 & sigma=1 & n=100 & 0.41 \\ 
  50 & MDE.Phi.X2 & beta & beta=2.5 & sigma=1 & n=100 & 0.15 \\ 
  51 & MDE.Phi.tv & beta & beta=2.5 & sigma=1 & n=100 & 0.36 \\ 
  52 & MDE.Phi.kl & beta & beta=2.5 & sigma=1 & n=100 & 0.23 \\ 
  53 & MME & beta & beta=2.5 & sigma=1 & n=100 & 94221.91 \\ 
  54 & MME.b & beta & beta=2.5 & sigma=1 & n=100 & 376880.47 \\ 
  55 & PWM & beta & beta=2.5 & sigma=1 & n=100 & 0.18 \\ 
  56 & MLE & sigma & beta=2.5 & sigma=1 & n=100 & 0.07 \\ 
  57 & MLE.b & sigma & beta=2.5 & sigma=1 & n=100 & 0.03 \\ 
  58 & LME & sigma & beta=2.5 & sigma=1 & n=100 & 0.06 \\ 
  59 & MDE.CvM & sigma & beta=2.5 & sigma=1 & n=100 & 0.16 \\ 
  60 & MDE.LS & sigma & beta=2.5 & sigma=1 & n=100 & 0.11 \\ 
  61 & MDE.Phi.X2 & sigma & beta=2.5 & sigma=1 & n=100 & 0.11 \\ 
  62 & MDE.Phi.tv & sigma & beta=2.5 & sigma=1 & n=100 & 0.28 \\ 
  63 & MDE.Phi.kl & sigma & beta=2.5 & sigma=1 & n=100 & 0.07 \\ 
  64 & MME & sigma & beta=2.5 & sigma=1 & n=100 & 46154.27 \\ 
  65 & MME.b & sigma & beta=2.5 & sigma=1 & n=100 & 184616.17 \\ 
  66 & PWM & sigma & beta=2.5 & sigma=1 & n=100 & 0.06 \\ 
  67 & MLE & beta & beta=3 & sigma=1 & n=100 & 0.25 \\ 
  68 & MLE.b & beta & beta=3 & sigma=1 & n=100 & 0.09 \\ 
  69 & LME & beta & beta=3 & sigma=1 & n=100 & 0.18 \\ 
  70 & MDE.CvM & beta & beta=3 & sigma=1 & n=100 & 0.81 \\ 
  71 & MDE.LS & beta & beta=3 & sigma=1 & n=100 & 0.52 \\ 
  72 & MDE.Phi.X2 & beta & beta=3 & sigma=1 & n=100 & 0.15 \\ 
  73 & MDE.Phi.tv & beta & beta=3 & sigma=1 & n=100 & 0.37 \\ 
  74 & MDE.Phi.kl & beta & beta=3 & sigma=1 & n=100 & 0.25 \\ 
  75 & MME & beta & beta=3 & sigma=1 & n=100 & 30010.03 \\ 
  76 & MME.b & beta & beta=3 & sigma=1 & n=100 & 120033.18 \\ 
  77 & PWM & beta & beta=3 & sigma=1 & n=100 & 0.18 \\ 
  78 & MLE & sigma & beta=3 & sigma=1 & n=100 & 0.05 \\ 
  79 & MLE.b & sigma & beta=3 & sigma=1 & n=100 & 0.02 \\ 
  80 & LME & sigma & beta=3 & sigma=1 & n=100 & 0.04 \\ 
  81 & MDE.CvM & sigma & beta=3 & sigma=1 & n=100 & 0.14 \\ 
  82 & MDE.LS & sigma & beta=3 & sigma=1 & n=100 & 0.09 \\ 
  83 & MDE.Phi.X2 & sigma & beta=3 & sigma=1 & n=100 & 0.07 \\ 
  84 & MDE.Phi.tv & sigma & beta=3 & sigma=1 & n=100 & 0.19 \\ 
  85 & MDE.Phi.kl & sigma & beta=3 & sigma=1 & n=100 & 0.05 \\ 
  86 & MME & sigma & beta=3 & sigma=1 & n=100 & 7636.74 \\ 
  87 & MME.b & sigma & beta=3 & sigma=1 & n=100 & 30546.57 \\ 
  88 & PWM & sigma & beta=3 & sigma=1 & n=100 & 0.04 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220223/20220223-11h09m48s-Full.beta=1.5.sig=1.n=200.LaTeX.tex <==
% START DATE AND TIME=20220223-11h09m48s
      \begin{table}[htbp]
  \centering
  \caption{$\beta=1.5,  \sigma=1$ $n=200$}
  \resizebox{\columnwidth}{!}{
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|r|r|}
      %\cline{2-13}    \multicolumn{1}{r|}{} &       & \multicolumn{11}{c|}{$\beta=1.5,  \sigma=1$ $n=200$} \\
\cline{2-13}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.CvM}} & \multicolumn{1}{l|}{\textbf{MDE.LS}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.X2}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.5552&1.4757&1.6981&1.5654&1.5161&0.8401&0.9976&1.5552&3.4668&4.5858&1.6981
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
1.0591&0.9759&1.1951&1.0674&1.0241&1.1066&1.2425&1.0591&4.0554&5.6065&1.1951
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.0854&0.0659&0.0946&0.1553&0.1365&0.0949&0.139&0.0854&480.1369&1919.3188&0.0946
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.0913&0.0694&0.104&0.1486&0.1309&0.1698&0.2428&0.0913&795.5482&3182.6464&0.104
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.0552&-0.0243&0.1981&0.0654&0.0161&-0.6599&-0.5024&0.0552&1.9668&3.0858&0.1981
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.0591&-0.0241&0.1951&0.0674&0.0241&0.1066&0.2425&0.0591&3.0554&4.6065&0.1951
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.0884&0.0664&0.1338&0.1596&0.1367&0.5304&0.3914&0.0884&483.9571&1928.6491&0.1338
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.0948&0.07&0.142&0.1531&0.1315&0.1811&0.3016&0.0948&804.8041&3203.5484&0.142
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 0.1832&0.1364&0.2758&0.3127&0.2682&0.7116&0.6931&0.1832&1288.7611&5132.1975&0.2758\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 6e-04&6e-04&6e-04&6e-04&6e-04&0.0335&0.0261&6e-04&0.0092&0.0104&6e-04\\
\hline
\end{tabular}
}
\end{table}

==> Tables20220525/output/output20220223/20220223-11h09m48s-Full.beta=2.5.sig=1.n=200.LaTeX.tex <==
% START DATE AND TIME=20220223-11h09m48s
      \begin{table}[htbp]
  \centering
  \caption{$\beta=2.5,  \sigma=1$ $n=200$}
  \resizebox{\columnwidth}{!}{
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|r|r|}
      %\cline{2-13}    \multicolumn{1}{r|}{} &       & \multicolumn{11}{c|}{$\beta=2.5,  \sigma=1$ $n=200$} \\
\cline{2-13}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.CvM}} & \multicolumn{1}{l|}{\textbf{MDE.LS}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.X2}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.3956&2.1835&2.4474&2.4764&2.3588&1.4604&1.7304&2.3956&27.632&52.7238&2.4474
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.9496&0.8356&0.9699&0.9881&0.9326&0.9459&1.0506&0.9496&15.6217&30.1973&0.9699
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.2011&0.1239&0.1729&0.5946&0.4779&0.1768&0.264&0.2011&1419789.1533&5679142.983&0.1729
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.0604&0.0372&0.053&0.1505&0.1222&0.0905&0.142&0.0604&396462.7351&1585854.388&0.053
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & -0.1044&-0.3165&-0.0526&-0.0236&-0.1412&-1.0396&-0.7696&-0.1044&25.132&50.2238&-0.0526
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
-0.0504&-0.1644&-0.0301&-0.0119&-0.0674&-0.0541&0.0506&-0.0504&14.6217&29.1973&-0.0301
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.212&0.224&0.1756&0.5951&0.4978&1.2575&0.8563&0.212&1420278.7943&5681097.5007&0.1756
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.0629&0.0643&0.0539&0.1506&0.1268&0.0934&0.1446&0.0629&396636.8828&1586548.2852&0.0539
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 0.2749&0.2883&0.2296&0.7457&0.6246&1.3509&1.0008&0.2749&1816915.677&7267645.7859&0.2296\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&5e-04&5e-04&6e-04&6e-04&0.0189&0.0131&5e-04&0.0026&0.0036&5e-04\\
\hline
\end{tabular}
}
\end{table}

==> Tables20220525/output/output20220223/20220223-11h09m48s-Full.beta=2.sig=1.n=200.LaTeX.tex <==
% START DATE AND TIME=20220223-11h09m48s
      \begin{table}[htbp]
  \centering
  \caption{$\beta=2,  \sigma=1$ $n=200$}
  \resizebox{\columnwidth}{!}{
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|r|r|}
      %\cline{2-13}    \multicolumn{1}{r|}{} &       & \multicolumn{11}{c|}{$\beta=2,  \sigma=1$ $n=200$} \\
\cline{2-13}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.CvM}} & \multicolumn{1}{l|}{\textbf{MDE.LS}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.X2}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.0267&1.8821&2.1252&2.0327&1.953&1.2146&1.4385&2.0267&8.3777&14.2819&2.1252
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
1.0215&0.9183&1.0811&1.0235&0.9745&1.0558&1.1745&1.0215&6.624&11.7889&1.0811
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.156&0.1073&0.1496&0.3196&0.2709&0.1656&0.2404&0.156&8103.5348&32409.7217&0.1496
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.0792&0.0539&0.0774&0.1405&0.1198&0.1449&0.2125&0.0792&6497.7762&25991.0262&0.0774
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.0267&-0.1179&0.1252&0.0327&-0.047&-0.7854&-0.5615&0.0267&6.3777&12.2819&0.1252
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.0215&-0.0817&0.0811&0.0235&-0.0255&0.0558&0.1745&0.0215&5.624&10.7889&0.0811
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1567&0.1212&0.1652&0.3207&0.2731&0.7825&0.5556&0.1567&8143.3989&32557.3267&0.1652
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.0796&0.0606&0.0839&0.141&0.1204&0.148&0.2429&0.0796&6528.7558&26104.8271&0.0839
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 0.2363&0.1817&0.2491&0.4617&0.3935&0.9305&0.7986&0.2363&14672.1548&58662.1538&0.2491\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&5e-04&5e-04&6e-04&6e-04&0.0231&0.0168&5e-04&0.0038&0.0049&5e-04\\
\hline
\end{tabular}
}
\end{table}

==> Tables20220525/output/output20220223/20220223-11h09m48s-Full.beta=3.sig=1.n=200.LaTeX.tex <==
% START DATE AND TIME=20220223-11h09m48s
      \begin{table}[htbp]
  \centering
  \caption{$\beta=3,  \sigma=1$ $n=200$}
  \resizebox{\columnwidth}{!}{
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|r|r|}
      %\cline{2-13}    \multicolumn{1}{r|}{} &       & \multicolumn{11}{c|}{$\beta=3,  \sigma=1$ $n=200$} \\
\cline{2-13}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.CvM}} & \multicolumn{1}{l|}{\textbf{MDE.LS}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.X2}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.7026&2.4222&2.7155&2.884&2.7253&1.6399&1.9543&2.7027&98.2417&193.9009&2.7155
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.881&0.7606&0.8818&0.9528&0.8921&0.8476&0.947&0.881&49.1174&97.4158&0.8818
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.2316&0.1284&0.185&0.8894&0.687&0.1661&0.268&0.2316&39861199.8782&159444757.2567&0.185
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.044&0.0246&0.0364&0.1463&0.1141&0.0563&0.0996&0.044&10110051.5753&40440199.8027&0.0364
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & -0.2974&-0.5778&-0.2845&-0.116&-0.2747&-1.3601&-1.0457&-0.2973&95.2417&190.9009&-0.2845
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
-0.119&-0.2394&-0.1182&-0.0472&-0.1079&-0.1524&-0.053&-0.119&48.1174&96.4158&-0.1182
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.32&0.4622&0.2659&0.9028&0.7624&2.0161&1.3615&0.32&39866284.7393&159465255.9203&0.2659
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.0581&0.0819&0.0504&0.1485&0.1257&0.0795&0.1024&0.0581&10111355.8567&40445451.7987&0.0504
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 0.3782&0.5441&0.3163&1.0513&0.8881&2.0956&1.4639&0.3781&49977640.596&199910707.719&0.3163\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&5e-04&5e-04&5e-04&5e-04&0.0168&0.0113&5e-04&0.0022&0.0029&5e-04\\
\hline
\end{tabular}
}
\end{table}

==> Tables20220525/output/output20220223/20220223-11h09m48s-Output.accuracy.LaTeX.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Wed Feb 23 13:42:56 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & Measure & beta=1.5 & sigma=1 & n=200 & 0.18 \\ 
  2 & MLE.b & Measure & beta=1.5 & sigma=1 & n=200 & 0.14 \\ 
  3 & LME & Measure & beta=1.5 & sigma=1 & n=200 & 0.28 \\ 
  4 & MDE.CvM & Measure & beta=1.5 & sigma=1 & n=200 & 0.31 \\ 
  5 & MDE.LS & Measure & beta=1.5 & sigma=1 & n=200 & 0.27 \\ 
  6 & MDE.Phi.X2 & Measure & beta=1.5 & sigma=1 & n=200 & 0.71 \\ 
  7 & MDE.Phi.tv & Measure & beta=1.5 & sigma=1 & n=200 & 0.69 \\ 
  8 & MDE.Phi.kl & Measure & beta=1.5 & sigma=1 & n=200 & 0.18 \\ 
  9 & MME & Measure & beta=1.5 & sigma=1 & n=200 & 1288.76 \\ 
  10 & MME.b & Measure & beta=1.5 & sigma=1 & n=200 & 5132.20 \\ 
  11 & PWM & Measure & beta=1.5 & sigma=1 & n=200 & 0.28 \\ 
  12 & MLE & Measure & beta=2 & sigma=1 & n=200 & 0.24 \\ 
  13 & MLE.b & Measure & beta=2 & sigma=1 & n=200 & 0.18 \\ 
  14 & LME & Measure & beta=2 & sigma=1 & n=200 & 0.25 \\ 
  15 & MDE.CvM & Measure & beta=2 & sigma=1 & n=200 & 0.46 \\ 
  16 & MDE.LS & Measure & beta=2 & sigma=1 & n=200 & 0.39 \\ 
  17 & MDE.Phi.X2 & Measure & beta=2 & sigma=1 & n=200 & 0.93 \\ 
  18 & MDE.Phi.tv & Measure & beta=2 & sigma=1 & n=200 & 0.80 \\ 
  19 & MDE.Phi.kl & Measure & beta=2 & sigma=1 & n=200 & 0.24 \\ 
  20 & MME & Measure & beta=2 & sigma=1 & n=200 & 14672.15 \\ 
  21 & MME.b & Measure & beta=2 & sigma=1 & n=200 & 58662.15 \\ 
  22 & PWM & Measure & beta=2 & sigma=1 & n=200 & 0.25 \\ 
  23 & MLE & Measure & beta=2.5 & sigma=1 & n=200 & 0.27 \\ 
  24 & MLE.b & Measure & beta=2.5 & sigma=1 & n=200 & 0.29 \\ 
  25 & LME & Measure & beta=2.5 & sigma=1 & n=200 & 0.23 \\ 
  26 & MDE.CvM & Measure & beta=2.5 & sigma=1 & n=200 & 0.75 \\ 
  27 & MDE.LS & Measure & beta=2.5 & sigma=1 & n=200 & 0.62 \\ 
  28 & MDE.Phi.X2 & Measure & beta=2.5 & sigma=1 & n=200 & 1.35 \\ 
  29 & MDE.Phi.tv & Measure & beta=2.5 & sigma=1 & n=200 & 1.00 \\ 
  30 & MDE.Phi.kl & Measure & beta=2.5 & sigma=1 & n=200 & 0.27 \\ 
  31 & MME & Measure & beta=2.5 & sigma=1 & n=200 & 1816915.68 \\ 
  32 & MME.b & Measure & beta=2.5 & sigma=1 & n=200 & 7267645.79 \\ 
  33 & PWM & Measure & beta=2.5 & sigma=1 & n=200 & 0.23 \\ 
  34 & MLE & Measure & beta=3 & sigma=1 & n=200 & 0.38 \\ 
  35 & MLE.b & Measure & beta=3 & sigma=1 & n=200 & 0.54 \\ 
  36 & LME & Measure & beta=3 & sigma=1 & n=200 & 0.32 \\ 
  37 & MDE.CvM & Measure & beta=3 & sigma=1 & n=200 & 1.05 \\ 
  38 & MDE.LS & Measure & beta=3 & sigma=1 & n=200 & 0.89 \\ 
  39 & MDE.Phi.X2 & Measure & beta=3 & sigma=1 & n=200 & 2.10 \\ 
  40 & MDE.Phi.tv & Measure & beta=3 & sigma=1 & n=200 & 1.46 \\ 
  41 & MDE.Phi.kl & Measure & beta=3 & sigma=1 & n=200 & 0.38 \\ 
  42 & MME & Measure & beta=3 & sigma=1 & n=200 & 49977640.60 \\ 
  43 & MME.b & Measure & beta=3 & sigma=1 & n=200 & 199910707.72 \\ 
  44 & PWM & Measure & beta=3 & sigma=1 & n=200 & 0.32 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220223/20220223-11h09m48s-Output.accuracy2.LaTeX.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Wed Feb 23 13:42:56 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & Measure & beta=1.5 & sigma=1 & n=200 & 0.00 \\ 
  2 & MLE.b & Measure & beta=1.5 & sigma=1 & n=200 & 0.00 \\ 
  3 & LME & Measure & beta=1.5 & sigma=1 & n=200 & 0.00 \\ 
  4 & MDE.CvM & Measure & beta=1.5 & sigma=1 & n=200 & 0.00 \\ 
  5 & MDE.LS & Measure & beta=1.5 & sigma=1 & n=200 & 0.00 \\ 
  6 & MDE.Phi.X2 & Measure & beta=1.5 & sigma=1 & n=200 & 0.03 \\ 
  7 & MDE.Phi.tv & Measure & beta=1.5 & sigma=1 & n=200 & 0.03 \\ 
  8 & MDE.Phi.kl & Measure & beta=1.5 & sigma=1 & n=200 & 0.00 \\ 
  9 & MME & Measure & beta=1.5 & sigma=1 & n=200 & 0.01 \\ 
  10 & MME.b & Measure & beta=1.5 & sigma=1 & n=200 & 0.01 \\ 
  11 & PWM & Measure & beta=1.5 & sigma=1 & n=200 & 0.00 \\ 
  12 & MLE & Measure & beta=2 & sigma=1 & n=200 & 0.00 \\ 
  13 & MLE.b & Measure & beta=2 & sigma=1 & n=200 & 0.00 \\ 
  14 & LME & Measure & beta=2 & sigma=1 & n=200 & 0.00 \\ 
  15 & MDE.CvM & Measure & beta=2 & sigma=1 & n=200 & 0.00 \\ 
  16 & MDE.LS & Measure & beta=2 & sigma=1 & n=200 & 0.00 \\ 
  17 & MDE.Phi.X2 & Measure & beta=2 & sigma=1 & n=200 & 0.02 \\ 
  18 & MDE.Phi.tv & Measure & beta=2 & sigma=1 & n=200 & 0.02 \\ 
  19 & MDE.Phi.kl & Measure & beta=2 & sigma=1 & n=200 & 0.00 \\ 
  20 & MME & Measure & beta=2 & sigma=1 & n=200 & 0.00 \\ 
  21 & MME.b & Measure & beta=2 & sigma=1 & n=200 & 0.00 \\ 
  22 & PWM & Measure & beta=2 & sigma=1 & n=200 & 0.00 \\ 
  23 & MLE & Measure & beta=2.5 & sigma=1 & n=200 & 0.00 \\ 
  24 & MLE.b & Measure & beta=2.5 & sigma=1 & n=200 & 0.00 \\ 
  25 & LME & Measure & beta=2.5 & sigma=1 & n=200 & 0.00 \\ 
  26 & MDE.CvM & Measure & beta=2.5 & sigma=1 & n=200 & 0.00 \\ 
  27 & MDE.LS & Measure & beta=2.5 & sigma=1 & n=200 & 0.00 \\ 
  28 & MDE.Phi.X2 & Measure & beta=2.5 & sigma=1 & n=200 & 0.02 \\ 
  29 & MDE.Phi.tv & Measure & beta=2.5 & sigma=1 & n=200 & 0.01 \\ 
  30 & MDE.Phi.kl & Measure & beta=2.5 & sigma=1 & n=200 & 0.00 \\ 
  31 & MME & Measure & beta=2.5 & sigma=1 & n=200 & 0.00 \\ 
  32 & MME.b & Measure & beta=2.5 & sigma=1 & n=200 & 0.00 \\ 
  33 & PWM & Measure & beta=2.5 & sigma=1 & n=200 & 0.00 \\ 
  34 & MLE & Measure & beta=3 & sigma=1 & n=200 & 0.00 \\ 
  35 & MLE.b & Measure & beta=3 & sigma=1 & n=200 & 0.00 \\ 
  36 & LME & Measure & beta=3 & sigma=1 & n=200 & 0.00 \\ 
  37 & MDE.CvM & Measure & beta=3 & sigma=1 & n=200 & 0.00 \\ 
  38 & MDE.LS & Measure & beta=3 & sigma=1 & n=200 & 0.00 \\ 
  39 & MDE.Phi.X2 & Measure & beta=3 & sigma=1 & n=200 & 0.02 \\ 
  40 & MDE.Phi.tv & Measure & beta=3 & sigma=1 & n=200 & 0.01 \\ 
  41 & MDE.Phi.kl & Measure & beta=3 & sigma=1 & n=200 & 0.00 \\ 
  42 & MME & Measure & beta=3 & sigma=1 & n=200 & 0.00 \\ 
  43 & MME.b & Measure & beta=3 & sigma=1 & n=200 & 0.00 \\ 
  44 & PWM & Measure & beta=3 & sigma=1 & n=200 & 0.00 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220223/20220223-11h09m48s-Output.bias.LaTeX.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Wed Feb 23 13:42:56 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=1 & n=200 & 0.06 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=1 & n=200 & -0.02 \\ 
  3 & LME & beta & beta=1.5 & sigma=1 & n=200 & 0.20 \\ 
  4 & MDE.CvM & beta & beta=1.5 & sigma=1 & n=200 & 0.07 \\ 
  5 & MDE.LS & beta & beta=1.5 & sigma=1 & n=200 & 0.02 \\ 
  6 & MDE.Phi.X2 & beta & beta=1.5 & sigma=1 & n=200 & -0.66 \\ 
  7 & MDE.Phi.tv & beta & beta=1.5 & sigma=1 & n=200 & -0.50 \\ 
  8 & MDE.Phi.kl & beta & beta=1.5 & sigma=1 & n=200 & 0.06 \\ 
  9 & MME & beta & beta=1.5 & sigma=1 & n=200 & 1.97 \\ 
  10 & MME.b & beta & beta=1.5 & sigma=1 & n=200 & 3.09 \\ 
  11 & PWM & beta & beta=1.5 & sigma=1 & n=200 & 0.20 \\ 
  12 & MLE & sigma & beta=1.5 & sigma=1 & n=200 & 0.06 \\ 
  13 & MLE.b & sigma & beta=1.5 & sigma=1 & n=200 & -0.02 \\ 
  14 & LME & sigma & beta=1.5 & sigma=1 & n=200 & 0.20 \\ 
  15 & MDE.CvM & sigma & beta=1.5 & sigma=1 & n=200 & 0.07 \\ 
  16 & MDE.LS & sigma & beta=1.5 & sigma=1 & n=200 & 0.02 \\ 
  17 & MDE.Phi.X2 & sigma & beta=1.5 & sigma=1 & n=200 & 0.11 \\ 
  18 & MDE.Phi.tv & sigma & beta=1.5 & sigma=1 & n=200 & 0.24 \\ 
  19 & MDE.Phi.kl & sigma & beta=1.5 & sigma=1 & n=200 & 0.06 \\ 
  20 & MME & sigma & beta=1.5 & sigma=1 & n=200 & 3.06 \\ 
  21 & MME.b & sigma & beta=1.5 & sigma=1 & n=200 & 4.61 \\ 
  22 & PWM & sigma & beta=1.5 & sigma=1 & n=200 & 0.20 \\ 
  23 & MLE & beta & beta=2 & sigma=1 & n=200 & 0.03 \\ 
  24 & MLE.b & beta & beta=2 & sigma=1 & n=200 & -0.12 \\ 
  25 & LME & beta & beta=2 & sigma=1 & n=200 & 0.13 \\ 
  26 & MDE.CvM & beta & beta=2 & sigma=1 & n=200 & 0.03 \\ 
  27 & MDE.LS & beta & beta=2 & sigma=1 & n=200 & -0.05 \\ 
  28 & MDE.Phi.X2 & beta & beta=2 & sigma=1 & n=200 & -0.79 \\ 
  29 & MDE.Phi.tv & beta & beta=2 & sigma=1 & n=200 & -0.56 \\ 
  30 & MDE.Phi.kl & beta & beta=2 & sigma=1 & n=200 & 0.03 \\ 
  31 & MME & beta & beta=2 & sigma=1 & n=200 & 6.38 \\ 
  32 & MME.b & beta & beta=2 & sigma=1 & n=200 & 12.28 \\ 
  33 & PWM & beta & beta=2 & sigma=1 & n=200 & 0.13 \\ 
  34 & MLE & sigma & beta=2 & sigma=1 & n=200 & 0.02 \\ 
  35 & MLE.b & sigma & beta=2 & sigma=1 & n=200 & -0.08 \\ 
  36 & LME & sigma & beta=2 & sigma=1 & n=200 & 0.08 \\ 
  37 & MDE.CvM & sigma & beta=2 & sigma=1 & n=200 & 0.02 \\ 
  38 & MDE.LS & sigma & beta=2 & sigma=1 & n=200 & -0.03 \\ 
  39 & MDE.Phi.X2 & sigma & beta=2 & sigma=1 & n=200 & 0.06 \\ 
  40 & MDE.Phi.tv & sigma & beta=2 & sigma=1 & n=200 & 0.17 \\ 
  41 & MDE.Phi.kl & sigma & beta=2 & sigma=1 & n=200 & 0.02 \\ 
  42 & MME & sigma & beta=2 & sigma=1 & n=200 & 5.62 \\ 
  43 & MME.b & sigma & beta=2 & sigma=1 & n=200 & 10.79 \\ 
  44 & PWM & sigma & beta=2 & sigma=1 & n=200 & 0.08 \\ 
  45 & MLE & beta & beta=2.5 & sigma=1 & n=200 & -0.10 \\ 
  46 & MLE.b & beta & beta=2.5 & sigma=1 & n=200 & -0.32 \\ 
  47 & LME & beta & beta=2.5 & sigma=1 & n=200 & -0.05 \\ 
  48 & MDE.CvM & beta & beta=2.5 & sigma=1 & n=200 & -0.02 \\ 
  49 & MDE.LS & beta & beta=2.5 & sigma=1 & n=200 & -0.14 \\ 
  50 & MDE.Phi.X2 & beta & beta=2.5 & sigma=1 & n=200 & -1.04 \\ 
  51 & MDE.Phi.tv & beta & beta=2.5 & sigma=1 & n=200 & -0.77 \\ 
  52 & MDE.Phi.kl & beta & beta=2.5 & sigma=1 & n=200 & -0.10 \\ 
  53 & MME & beta & beta=2.5 & sigma=1 & n=200 & 25.13 \\ 
  54 & MME.b & beta & beta=2.5 & sigma=1 & n=200 & 50.22 \\ 
  55 & PWM & beta & beta=2.5 & sigma=1 & n=200 & -0.05 \\ 
  56 & MLE & sigma & beta=2.5 & sigma=1 & n=200 & -0.05 \\ 
  57 & MLE.b & sigma & beta=2.5 & sigma=1 & n=200 & -0.16 \\ 
  58 & LME & sigma & beta=2.5 & sigma=1 & n=200 & -0.03 \\ 
  59 & MDE.CvM & sigma & beta=2.5 & sigma=1 & n=200 & -0.01 \\ 
  60 & MDE.LS & sigma & beta=2.5 & sigma=1 & n=200 & -0.07 \\ 
  61 & MDE.Phi.X2 & sigma & beta=2.5 & sigma=1 & n=200 & -0.05 \\ 
  62 & MDE.Phi.tv & sigma & beta=2.5 & sigma=1 & n=200 & 0.05 \\ 
  63 & MDE.Phi.kl & sigma & beta=2.5 & sigma=1 & n=200 & -0.05 \\ 
  64 & MME & sigma & beta=2.5 & sigma=1 & n=200 & 14.62 \\ 
  65 & MME.b & sigma & beta=2.5 & sigma=1 & n=200 & 29.20 \\ 
  66 & PWM & sigma & beta=2.5 & sigma=1 & n=200 & -0.03 \\ 
  67 & MLE & beta & beta=3 & sigma=1 & n=200 & -0.30 \\ 
  68 & MLE.b & beta & beta=3 & sigma=1 & n=200 & -0.58 \\ 
  69 & LME & beta & beta=3 & sigma=1 & n=200 & -0.28 \\ 
  70 & MDE.CvM & beta & beta=3 & sigma=1 & n=200 & -0.12 \\ 
  71 & MDE.LS & beta & beta=3 & sigma=1 & n=200 & -0.27 \\ 
  72 & MDE.Phi.X2 & beta & beta=3 & sigma=1 & n=200 & -1.36 \\ 
  73 & MDE.Phi.tv & beta & beta=3 & sigma=1 & n=200 & -1.05 \\ 
  74 & MDE.Phi.kl & beta & beta=3 & sigma=1 & n=200 & -0.30 \\ 
  75 & MME & beta & beta=3 & sigma=1 & n=200 & 95.24 \\ 
  76 & MME.b & beta & beta=3 & sigma=1 & n=200 & 190.90 \\ 
  77 & PWM & beta & beta=3 & sigma=1 & n=200 & -0.28 \\ 
  78 & MLE & sigma & beta=3 & sigma=1 & n=200 & -0.12 \\ 
  79 & MLE.b & sigma & beta=3 & sigma=1 & n=200 & -0.24 \\ 
  80 & LME & sigma & beta=3 & sigma=1 & n=200 & -0.12 \\ 
  81 & MDE.CvM & sigma & beta=3 & sigma=1 & n=200 & -0.05 \\ 
  82 & MDE.LS & sigma & beta=3 & sigma=1 & n=200 & -0.11 \\ 
  83 & MDE.Phi.X2 & sigma & beta=3 & sigma=1 & n=200 & -0.15 \\ 
  84 & MDE.Phi.tv & sigma & beta=3 & sigma=1 & n=200 & -0.05 \\ 
  85 & MDE.Phi.kl & sigma & beta=3 & sigma=1 & n=200 & -0.12 \\ 
  86 & MME & sigma & beta=3 & sigma=1 & n=200 & 48.12 \\ 
  87 & MME.b & sigma & beta=3 & sigma=1 & n=200 & 96.42 \\ 
  88 & PWM & sigma & beta=3 & sigma=1 & n=200 & -0.12 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220223/20220223-11h09m48s-Output.mean.LaTeX.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Wed Feb 23 13:42:56 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=1 & n=200 & 1.56 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=1 & n=200 & 1.48 \\ 
  3 & LME & beta & beta=1.5 & sigma=1 & n=200 & 1.70 \\ 
  4 & MDE.CvM & beta & beta=1.5 & sigma=1 & n=200 & 1.57 \\ 
  5 & MDE.LS & beta & beta=1.5 & sigma=1 & n=200 & 1.52 \\ 
  6 & MDE.Phi.X2 & beta & beta=1.5 & sigma=1 & n=200 & 0.84 \\ 
  7 & MDE.Phi.tv & beta & beta=1.5 & sigma=1 & n=200 & 1.00 \\ 
  8 & MDE.Phi.kl & beta & beta=1.5 & sigma=1 & n=200 & 1.56 \\ 
  9 & MME & beta & beta=1.5 & sigma=1 & n=200 & 3.47 \\ 
  10 & MME.b & beta & beta=1.5 & sigma=1 & n=200 & 4.59 \\ 
  11 & PWM & beta & beta=1.5 & sigma=1 & n=200 & 1.70 \\ 
  12 & MLE & sigma & beta=1.5 & sigma=1 & n=200 & 1.06 \\ 
  13 & MLE.b & sigma & beta=1.5 & sigma=1 & n=200 & 0.98 \\ 
  14 & LME & sigma & beta=1.5 & sigma=1 & n=200 & 1.20 \\ 
  15 & MDE.CvM & sigma & beta=1.5 & sigma=1 & n=200 & 1.07 \\ 
  16 & MDE.LS & sigma & beta=1.5 & sigma=1 & n=200 & 1.02 \\ 
  17 & MDE.Phi.X2 & sigma & beta=1.5 & sigma=1 & n=200 & 1.11 \\ 
  18 & MDE.Phi.tv & sigma & beta=1.5 & sigma=1 & n=200 & 1.24 \\ 
  19 & MDE.Phi.kl & sigma & beta=1.5 & sigma=1 & n=200 & 1.06 \\ 
  20 & MME & sigma & beta=1.5 & sigma=1 & n=200 & 4.06 \\ 
  21 & MME.b & sigma & beta=1.5 & sigma=1 & n=200 & 5.61 \\ 
  22 & PWM & sigma & beta=1.5 & sigma=1 & n=200 & 1.20 \\ 
  23 & MLE & beta & beta=2 & sigma=1 & n=200 & 2.03 \\ 
  24 & MLE.b & beta & beta=2 & sigma=1 & n=200 & 1.88 \\ 
  25 & LME & beta & beta=2 & sigma=1 & n=200 & 2.13 \\ 
  26 & MDE.CvM & beta & beta=2 & sigma=1 & n=200 & 2.03 \\ 
  27 & MDE.LS & beta & beta=2 & sigma=1 & n=200 & 1.95 \\ 
  28 & MDE.Phi.X2 & beta & beta=2 & sigma=1 & n=200 & 1.21 \\ 
  29 & MDE.Phi.tv & beta & beta=2 & sigma=1 & n=200 & 1.44 \\ 
  30 & MDE.Phi.kl & beta & beta=2 & sigma=1 & n=200 & 2.03 \\ 
  31 & MME & beta & beta=2 & sigma=1 & n=200 & 8.38 \\ 
  32 & MME.b & beta & beta=2 & sigma=1 & n=200 & 14.28 \\ 
  33 & PWM & beta & beta=2 & sigma=1 & n=200 & 2.13 \\ 
  34 & MLE & sigma & beta=2 & sigma=1 & n=200 & 1.02 \\ 
  35 & MLE.b & sigma & beta=2 & sigma=1 & n=200 & 0.92 \\ 
  36 & LME & sigma & beta=2 & sigma=1 & n=200 & 1.08 \\ 
  37 & MDE.CvM & sigma & beta=2 & sigma=1 & n=200 & 1.02 \\ 
  38 & MDE.LS & sigma & beta=2 & sigma=1 & n=200 & 0.97 \\ 
  39 & MDE.Phi.X2 & sigma & beta=2 & sigma=1 & n=200 & 1.06 \\ 
  40 & MDE.Phi.tv & sigma & beta=2 & sigma=1 & n=200 & 1.17 \\ 
  41 & MDE.Phi.kl & sigma & beta=2 & sigma=1 & n=200 & 1.02 \\ 
  42 & MME & sigma & beta=2 & sigma=1 & n=200 & 6.62 \\ 
  43 & MME.b & sigma & beta=2 & sigma=1 & n=200 & 11.79 \\ 
  44 & PWM & sigma & beta=2 & sigma=1 & n=200 & 1.08 \\ 
  45 & MLE & beta & beta=2.5 & sigma=1 & n=200 & 2.40 \\ 
  46 & MLE.b & beta & beta=2.5 & sigma=1 & n=200 & 2.18 \\ 
  47 & LME & beta & beta=2.5 & sigma=1 & n=200 & 2.45 \\ 
  48 & MDE.CvM & beta & beta=2.5 & sigma=1 & n=200 & 2.48 \\ 
  49 & MDE.LS & beta & beta=2.5 & sigma=1 & n=200 & 2.36 \\ 
  50 & MDE.Phi.X2 & beta & beta=2.5 & sigma=1 & n=200 & 1.46 \\ 
  51 & MDE.Phi.tv & beta & beta=2.5 & sigma=1 & n=200 & 1.73 \\ 
  52 & MDE.Phi.kl & beta & beta=2.5 & sigma=1 & n=200 & 2.40 \\ 
  53 & MME & beta & beta=2.5 & sigma=1 & n=200 & 27.63 \\ 
  54 & MME.b & beta & beta=2.5 & sigma=1 & n=200 & 52.72 \\ 
  55 & PWM & beta & beta=2.5 & sigma=1 & n=200 & 2.45 \\ 
  56 & MLE & sigma & beta=2.5 & sigma=1 & n=200 & 0.95 \\ 
  57 & MLE.b & sigma & beta=2.5 & sigma=1 & n=200 & 0.84 \\ 
  58 & LME & sigma & beta=2.5 & sigma=1 & n=200 & 0.97 \\ 
  59 & MDE.CvM & sigma & beta=2.5 & sigma=1 & n=200 & 0.99 \\ 
  60 & MDE.LS & sigma & beta=2.5 & sigma=1 & n=200 & 0.93 \\ 
  61 & MDE.Phi.X2 & sigma & beta=2.5 & sigma=1 & n=200 & 0.95 \\ 
  62 & MDE.Phi.tv & sigma & beta=2.5 & sigma=1 & n=200 & 1.05 \\ 
  63 & MDE.Phi.kl & sigma & beta=2.5 & sigma=1 & n=200 & 0.95 \\ 
  64 & MME & sigma & beta=2.5 & sigma=1 & n=200 & 15.62 \\ 
  65 & MME.b & sigma & beta=2.5 & sigma=1 & n=200 & 30.20 \\ 
  66 & PWM & sigma & beta=2.5 & sigma=1 & n=200 & 0.97 \\ 
  67 & MLE & beta & beta=3 & sigma=1 & n=200 & 2.70 \\ 
  68 & MLE.b & beta & beta=3 & sigma=1 & n=200 & 2.42 \\ 
  69 & LME & beta & beta=3 & sigma=1 & n=200 & 2.72 \\ 
  70 & MDE.CvM & beta & beta=3 & sigma=1 & n=200 & 2.88 \\ 
  71 & MDE.LS & beta & beta=3 & sigma=1 & n=200 & 2.73 \\ 
  72 & MDE.Phi.X2 & beta & beta=3 & sigma=1 & n=200 & 1.64 \\ 
  73 & MDE.Phi.tv & beta & beta=3 & sigma=1 & n=200 & 1.95 \\ 
  74 & MDE.Phi.kl & beta & beta=3 & sigma=1 & n=200 & 2.70 \\ 
  75 & MME & beta & beta=3 & sigma=1 & n=200 & 98.24 \\ 
  76 & MME.b & beta & beta=3 & sigma=1 & n=200 & 193.90 \\ 
  77 & PWM & beta & beta=3 & sigma=1 & n=200 & 2.72 \\ 
  78 & MLE & sigma & beta=3 & sigma=1 & n=200 & 0.88 \\ 
  79 & MLE.b & sigma & beta=3 & sigma=1 & n=200 & 0.76 \\ 
  80 & LME & sigma & beta=3 & sigma=1 & n=200 & 0.88 \\ 
  81 & MDE.CvM & sigma & beta=3 & sigma=1 & n=200 & 0.95 \\ 
  82 & MDE.LS & sigma & beta=3 & sigma=1 & n=200 & 0.89 \\ 
  83 & MDE.Phi.X2 & sigma & beta=3 & sigma=1 & n=200 & 0.85 \\ 
  84 & MDE.Phi.tv & sigma & beta=3 & sigma=1 & n=200 & 0.95 \\ 
  85 & MDE.Phi.kl & sigma & beta=3 & sigma=1 & n=200 & 0.88 \\ 
  86 & MME & sigma & beta=3 & sigma=1 & n=200 & 49.12 \\ 
  87 & MME.b & sigma & beta=3 & sigma=1 & n=200 & 97.42 \\ 
  88 & PWM & sigma & beta=3 & sigma=1 & n=200 & 0.88 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220223/20220223-11h09m48s-Output.mse.LaTeX.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Wed Feb 23 13:42:56 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=1 & n=200 & 0.09 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=1 & n=200 & 0.07 \\ 
  3 & LME & beta & beta=1.5 & sigma=1 & n=200 & 0.13 \\ 
  4 & MDE.CvM & beta & beta=1.5 & sigma=1 & n=200 & 0.16 \\ 
  5 & MDE.LS & beta & beta=1.5 & sigma=1 & n=200 & 0.14 \\ 
  6 & MDE.Phi.X2 & beta & beta=1.5 & sigma=1 & n=200 & 0.53 \\ 
  7 & MDE.Phi.tv & beta & beta=1.5 & sigma=1 & n=200 & 0.39 \\ 
  8 & MDE.Phi.kl & beta & beta=1.5 & sigma=1 & n=200 & 0.09 \\ 
  9 & MME & beta & beta=1.5 & sigma=1 & n=200 & 483.96 \\ 
  10 & MME.b & beta & beta=1.5 & sigma=1 & n=200 & 1928.65 \\ 
  11 & PWM & beta & beta=1.5 & sigma=1 & n=200 & 0.13 \\ 
  12 & MLE & sigma & beta=1.5 & sigma=1 & n=200 & 0.09 \\ 
  13 & MLE.b & sigma & beta=1.5 & sigma=1 & n=200 & 0.07 \\ 
  14 & LME & sigma & beta=1.5 & sigma=1 & n=200 & 0.14 \\ 
  15 & MDE.CvM & sigma & beta=1.5 & sigma=1 & n=200 & 0.15 \\ 
  16 & MDE.LS & sigma & beta=1.5 & sigma=1 & n=200 & 0.13 \\ 
  17 & MDE.Phi.X2 & sigma & beta=1.5 & sigma=1 & n=200 & 0.18 \\ 
  18 & MDE.Phi.tv & sigma & beta=1.5 & sigma=1 & n=200 & 0.30 \\ 
  19 & MDE.Phi.kl & sigma & beta=1.5 & sigma=1 & n=200 & 0.09 \\ 
  20 & MME & sigma & beta=1.5 & sigma=1 & n=200 & 804.80 \\ 
  21 & MME.b & sigma & beta=1.5 & sigma=1 & n=200 & 3203.55 \\ 
  22 & PWM & sigma & beta=1.5 & sigma=1 & n=200 & 0.14 \\ 
  23 & MLE & beta & beta=2 & sigma=1 & n=200 & 0.16 \\ 
  24 & MLE.b & beta & beta=2 & sigma=1 & n=200 & 0.12 \\ 
  25 & LME & beta & beta=2 & sigma=1 & n=200 & 0.17 \\ 
  26 & MDE.CvM & beta & beta=2 & sigma=1 & n=200 & 0.32 \\ 
  27 & MDE.LS & beta & beta=2 & sigma=1 & n=200 & 0.27 \\ 
  28 & MDE.Phi.X2 & beta & beta=2 & sigma=1 & n=200 & 0.78 \\ 
  29 & MDE.Phi.tv & beta & beta=2 & sigma=1 & n=200 & 0.56 \\ 
  30 & MDE.Phi.kl & beta & beta=2 & sigma=1 & n=200 & 0.16 \\ 
  31 & MME & beta & beta=2 & sigma=1 & n=200 & 8143.40 \\ 
  32 & MME.b & beta & beta=2 & sigma=1 & n=200 & 32557.33 \\ 
  33 & PWM & beta & beta=2 & sigma=1 & n=200 & 0.17 \\ 
  34 & MLE & sigma & beta=2 & sigma=1 & n=200 & 0.08 \\ 
  35 & MLE.b & sigma & beta=2 & sigma=1 & n=200 & 0.06 \\ 
  36 & LME & sigma & beta=2 & sigma=1 & n=200 & 0.08 \\ 
  37 & MDE.CvM & sigma & beta=2 & sigma=1 & n=200 & 0.14 \\ 
  38 & MDE.LS & sigma & beta=2 & sigma=1 & n=200 & 0.12 \\ 
  39 & MDE.Phi.X2 & sigma & beta=2 & sigma=1 & n=200 & 0.15 \\ 
  40 & MDE.Phi.tv & sigma & beta=2 & sigma=1 & n=200 & 0.24 \\ 
  41 & MDE.Phi.kl & sigma & beta=2 & sigma=1 & n=200 & 0.08 \\ 
  42 & MME & sigma & beta=2 & sigma=1 & n=200 & 6528.76 \\ 
  43 & MME.b & sigma & beta=2 & sigma=1 & n=200 & 26104.83 \\ 
  44 & PWM & sigma & beta=2 & sigma=1 & n=200 & 0.08 \\ 
  45 & MLE & beta & beta=2.5 & sigma=1 & n=200 & 0.21 \\ 
  46 & MLE.b & beta & beta=2.5 & sigma=1 & n=200 & 0.22 \\ 
  47 & LME & beta & beta=2.5 & sigma=1 & n=200 & 0.18 \\ 
  48 & MDE.CvM & beta & beta=2.5 & sigma=1 & n=200 & 0.60 \\ 
  49 & MDE.LS & beta & beta=2.5 & sigma=1 & n=200 & 0.50 \\ 
  50 & MDE.Phi.X2 & beta & beta=2.5 & sigma=1 & n=200 & 1.26 \\ 
  51 & MDE.Phi.tv & beta & beta=2.5 & sigma=1 & n=200 & 0.86 \\ 
  52 & MDE.Phi.kl & beta & beta=2.5 & sigma=1 & n=200 & 0.21 \\ 
  53 & MME & beta & beta=2.5 & sigma=1 & n=200 & 1420278.79 \\ 
  54 & MME.b & beta & beta=2.5 & sigma=1 & n=200 & 5681097.50 \\ 
  55 & PWM & beta & beta=2.5 & sigma=1 & n=200 & 0.18 \\ 
  56 & MLE & sigma & beta=2.5 & sigma=1 & n=200 & 0.06 \\ 
  57 & MLE.b & sigma & beta=2.5 & sigma=1 & n=200 & 0.06 \\ 
  58 & LME & sigma & beta=2.5 & sigma=1 & n=200 & 0.05 \\ 
  59 & MDE.CvM & sigma & beta=2.5 & sigma=1 & n=200 & 0.15 \\ 
  60 & MDE.LS & sigma & beta=2.5 & sigma=1 & n=200 & 0.13 \\ 
  61 & MDE.Phi.X2 & sigma & beta=2.5 & sigma=1 & n=200 & 0.09 \\ 
  62 & MDE.Phi.tv & sigma & beta=2.5 & sigma=1 & n=200 & 0.14 \\ 
  63 & MDE.Phi.kl & sigma & beta=2.5 & sigma=1 & n=200 & 0.06 \\ 
  64 & MME & sigma & beta=2.5 & sigma=1 & n=200 & 396636.88 \\ 
  65 & MME.b & sigma & beta=2.5 & sigma=1 & n=200 & 1586548.29 \\ 
  66 & PWM & sigma & beta=2.5 & sigma=1 & n=200 & 0.05 \\ 
  67 & MLE & beta & beta=3 & sigma=1 & n=200 & 0.32 \\ 
  68 & MLE.b & beta & beta=3 & sigma=1 & n=200 & 0.46 \\ 
  69 & LME & beta & beta=3 & sigma=1 & n=200 & 0.27 \\ 
  70 & MDE.CvM & beta & beta=3 & sigma=1 & n=200 & 0.90 \\ 
  71 & MDE.LS & beta & beta=3 & sigma=1 & n=200 & 0.76 \\ 
  72 & MDE.Phi.X2 & beta & beta=3 & sigma=1 & n=200 & 2.02 \\ 
  73 & MDE.Phi.tv & beta & beta=3 & sigma=1 & n=200 & 1.36 \\ 
  74 & MDE.Phi.kl & beta & beta=3 & sigma=1 & n=200 & 0.32 \\ 
  75 & MME & beta & beta=3 & sigma=1 & n=200 & 39866284.74 \\ 
  76 & MME.b & beta & beta=3 & sigma=1 & n=200 & 159465255.92 \\ 
  77 & PWM & beta & beta=3 & sigma=1 & n=200 & 0.27 \\ 
  78 & MLE & sigma & beta=3 & sigma=1 & n=200 & 0.06 \\ 
  79 & MLE.b & sigma & beta=3 & sigma=1 & n=200 & 0.08 \\ 
  80 & LME & sigma & beta=3 & sigma=1 & n=200 & 0.05 \\ 
  81 & MDE.CvM & sigma & beta=3 & sigma=1 & n=200 & 0.15 \\ 
  82 & MDE.LS & sigma & beta=3 & sigma=1 & n=200 & 0.13 \\ 
  83 & MDE.Phi.X2 & sigma & beta=3 & sigma=1 & n=200 & 0.08 \\ 
  84 & MDE.Phi.tv & sigma & beta=3 & sigma=1 & n=200 & 0.10 \\ 
  85 & MDE.Phi.kl & sigma & beta=3 & sigma=1 & n=200 & 0.06 \\ 
  86 & MME & sigma & beta=3 & sigma=1 & n=200 & 10111355.86 \\ 
  87 & MME.b & sigma & beta=3 & sigma=1 & n=200 & 40445451.80 \\ 
  88 & PWM & sigma & beta=3 & sigma=1 & n=200 & 0.05 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220223/20220223-11h09m48s-Output.var.LaTeX.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Wed Feb 23 13:42:56 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.5 & sigma=1 & n=200 & 0.09 \\ 
  2 & MLE.b & beta & beta=1.5 & sigma=1 & n=200 & 0.07 \\ 
  3 & LME & beta & beta=1.5 & sigma=1 & n=200 & 0.09 \\ 
  4 & MDE.CvM & beta & beta=1.5 & sigma=1 & n=200 & 0.16 \\ 
  5 & MDE.LS & beta & beta=1.5 & sigma=1 & n=200 & 0.14 \\ 
  6 & MDE.Phi.X2 & beta & beta=1.5 & sigma=1 & n=200 & 0.09 \\ 
  7 & MDE.Phi.tv & beta & beta=1.5 & sigma=1 & n=200 & 0.14 \\ 
  8 & MDE.Phi.kl & beta & beta=1.5 & sigma=1 & n=200 & 0.09 \\ 
  9 & MME & beta & beta=1.5 & sigma=1 & n=200 & 480.14 \\ 
  10 & MME.b & beta & beta=1.5 & sigma=1 & n=200 & 1919.32 \\ 
  11 & PWM & beta & beta=1.5 & sigma=1 & n=200 & 0.09 \\ 
  12 & MLE & sigma & beta=1.5 & sigma=1 & n=200 & 0.09 \\ 
  13 & MLE.b & sigma & beta=1.5 & sigma=1 & n=200 & 0.07 \\ 
  14 & LME & sigma & beta=1.5 & sigma=1 & n=200 & 0.10 \\ 
  15 & MDE.CvM & sigma & beta=1.5 & sigma=1 & n=200 & 0.15 \\ 
  16 & MDE.LS & sigma & beta=1.5 & sigma=1 & n=200 & 0.13 \\ 
  17 & MDE.Phi.X2 & sigma & beta=1.5 & sigma=1 & n=200 & 0.17 \\ 
  18 & MDE.Phi.tv & sigma & beta=1.5 & sigma=1 & n=200 & 0.24 \\ 
  19 & MDE.Phi.kl & sigma & beta=1.5 & sigma=1 & n=200 & 0.09 \\ 
  20 & MME & sigma & beta=1.5 & sigma=1 & n=200 & 795.55 \\ 
  21 & MME.b & sigma & beta=1.5 & sigma=1 & n=200 & 3182.65 \\ 
  22 & PWM & sigma & beta=1.5 & sigma=1 & n=200 & 0.10 \\ 
  23 & MLE & beta & beta=2 & sigma=1 & n=200 & 0.16 \\ 
  24 & MLE.b & beta & beta=2 & sigma=1 & n=200 & 0.11 \\ 
  25 & LME & beta & beta=2 & sigma=1 & n=200 & 0.15 \\ 
  26 & MDE.CvM & beta & beta=2 & sigma=1 & n=200 & 0.32 \\ 
  27 & MDE.LS & beta & beta=2 & sigma=1 & n=200 & 0.27 \\ 
  28 & MDE.Phi.X2 & beta & beta=2 & sigma=1 & n=200 & 0.17 \\ 
  29 & MDE.Phi.tv & beta & beta=2 & sigma=1 & n=200 & 0.24 \\ 
  30 & MDE.Phi.kl & beta & beta=2 & sigma=1 & n=200 & 0.16 \\ 
  31 & MME & beta & beta=2 & sigma=1 & n=200 & 8103.53 \\ 
  32 & MME.b & beta & beta=2 & sigma=1 & n=200 & 32409.72 \\ 
  33 & PWM & beta & beta=2 & sigma=1 & n=200 & 0.15 \\ 
  34 & MLE & sigma & beta=2 & sigma=1 & n=200 & 0.08 \\ 
  35 & MLE.b & sigma & beta=2 & sigma=1 & n=200 & 0.05 \\ 
  36 & LME & sigma & beta=2 & sigma=1 & n=200 & 0.08 \\ 
  37 & MDE.CvM & sigma & beta=2 & sigma=1 & n=200 & 0.14 \\ 
  38 & MDE.LS & sigma & beta=2 & sigma=1 & n=200 & 0.12 \\ 
  39 & MDE.Phi.X2 & sigma & beta=2 & sigma=1 & n=200 & 0.14 \\ 
  40 & MDE.Phi.tv & sigma & beta=2 & sigma=1 & n=200 & 0.21 \\ 
  41 & MDE.Phi.kl & sigma & beta=2 & sigma=1 & n=200 & 0.08 \\ 
  42 & MME & sigma & beta=2 & sigma=1 & n=200 & 6497.78 \\ 
  43 & MME.b & sigma & beta=2 & sigma=1 & n=200 & 25991.03 \\ 
  44 & PWM & sigma & beta=2 & sigma=1 & n=200 & 0.08 \\ 
  45 & MLE & beta & beta=2.5 & sigma=1 & n=200 & 0.20 \\ 
  46 & MLE.b & beta & beta=2.5 & sigma=1 & n=200 & 0.12 \\ 
  47 & LME & beta & beta=2.5 & sigma=1 & n=200 & 0.17 \\ 
  48 & MDE.CvM & beta & beta=2.5 & sigma=1 & n=200 & 0.59 \\ 
  49 & MDE.LS & beta & beta=2.5 & sigma=1 & n=200 & 0.48 \\ 
  50 & MDE.Phi.X2 & beta & beta=2.5 & sigma=1 & n=200 & 0.18 \\ 
  51 & MDE.Phi.tv & beta & beta=2.5 & sigma=1 & n=200 & 0.26 \\ 
  52 & MDE.Phi.kl & beta & beta=2.5 & sigma=1 & n=200 & 0.20 \\ 
  53 & MME & beta & beta=2.5 & sigma=1 & n=200 & 1419789.15 \\ 
  54 & MME.b & beta & beta=2.5 & sigma=1 & n=200 & 5679142.98 \\ 
  55 & PWM & beta & beta=2.5 & sigma=1 & n=200 & 0.17 \\ 
  56 & MLE & sigma & beta=2.5 & sigma=1 & n=200 & 0.06 \\ 
  57 & MLE.b & sigma & beta=2.5 & sigma=1 & n=200 & 0.04 \\ 
  58 & LME & sigma & beta=2.5 & sigma=1 & n=200 & 0.05 \\ 
  59 & MDE.CvM & sigma & beta=2.5 & sigma=1 & n=200 & 0.15 \\ 
  60 & MDE.LS & sigma & beta=2.5 & sigma=1 & n=200 & 0.12 \\ 
  61 & MDE.Phi.X2 & sigma & beta=2.5 & sigma=1 & n=200 & 0.09 \\ 
  62 & MDE.Phi.tv & sigma & beta=2.5 & sigma=1 & n=200 & 0.14 \\ 
  63 & MDE.Phi.kl & sigma & beta=2.5 & sigma=1 & n=200 & 0.06 \\ 
  64 & MME & sigma & beta=2.5 & sigma=1 & n=200 & 396462.74 \\ 
  65 & MME.b & sigma & beta=2.5 & sigma=1 & n=200 & 1585854.39 \\ 
  66 & PWM & sigma & beta=2.5 & sigma=1 & n=200 & 0.05 \\ 
  67 & MLE & beta & beta=3 & sigma=1 & n=200 & 0.23 \\ 
  68 & MLE.b & beta & beta=3 & sigma=1 & n=200 & 0.13 \\ 
  69 & LME & beta & beta=3 & sigma=1 & n=200 & 0.18 \\ 
  70 & MDE.CvM & beta & beta=3 & sigma=1 & n=200 & 0.89 \\ 
  71 & MDE.LS & beta & beta=3 & sigma=1 & n=200 & 0.69 \\ 
  72 & MDE.Phi.X2 & beta & beta=3 & sigma=1 & n=200 & 0.17 \\ 
  73 & MDE.Phi.tv & beta & beta=3 & sigma=1 & n=200 & 0.27 \\ 
  74 & MDE.Phi.kl & beta & beta=3 & sigma=1 & n=200 & 0.23 \\ 
  75 & MME & beta & beta=3 & sigma=1 & n=200 & 39861199.88 \\ 
  76 & MME.b & beta & beta=3 & sigma=1 & n=200 & 159444757.26 \\ 
  77 & PWM & beta & beta=3 & sigma=1 & n=200 & 0.18 \\ 
  78 & MLE & sigma & beta=3 & sigma=1 & n=200 & 0.04 \\ 
  79 & MLE.b & sigma & beta=3 & sigma=1 & n=200 & 0.02 \\ 
  80 & LME & sigma & beta=3 & sigma=1 & n=200 & 0.04 \\ 
  81 & MDE.CvM & sigma & beta=3 & sigma=1 & n=200 & 0.15 \\ 
  82 & MDE.LS & sigma & beta=3 & sigma=1 & n=200 & 0.11 \\ 
  83 & MDE.Phi.X2 & sigma & beta=3 & sigma=1 & n=200 & 0.06 \\ 
  84 & MDE.Phi.tv & sigma & beta=3 & sigma=1 & n=200 & 0.10 \\ 
  85 & MDE.Phi.kl & sigma & beta=3 & sigma=1 & n=200 & 0.04 \\ 
  86 & MME & sigma & beta=3 & sigma=1 & n=200 & 10110051.58 \\ 
  87 & MME.b & sigma & beta=3 & sigma=1 & n=200 & 40440199.80 \\ 
  88 & PWM & sigma & beta=3 & sigma=1 & n=200 & 0.04 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220520/20220519-10h55m12s-Full.beta=1.1.sig=2.n=30.LaTeX.tex <==
% START DATE AND TIME=20220519-10h55m12s
      \begin{table}[htbp]
  \centering
  \caption{$\beta=1.1,  \sigma=2$ $n=30$}
  \resizebox{\columnwidth}{!}{
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|r|r|}
      %\cline{2-13}    \multicolumn{1}{r|}{} &       & \multicolumn{11}{c|}{$\beta=1.1,  \sigma=2$ $n=30$} \\
\cline{2-13}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.CvM}} & \multicolumn{1}{l|}{\textbf{MDE.LS}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.X2}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.7987&1.512&1.7401&1.3427&1.1135&-1.6633&3.0483&1.6001&3.636&-1.3929&1.7401
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
3.8588&3.0454&3.3854&2.466&1.9066&9.1863&15.9833&3.1893&54.036&34.3719&3.3854
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 160.0243&160.3052&1.838&2.5208&1.7722&498.3215&172.4203&16.417&239.0424&807.0952&1.838
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
1765.3744&1767.7238&23.0907&31.9671&22.7828&1958.5497&5046.1827&174.1169&16777095.9217&14350843.71&23.0907
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.6987&0.412&0.6401&0.2427&0.0135&-2.7633&1.9483&0.5001&2.536&-2.4929&0.6401
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
1.8588&1.0454&1.3854&0.466&-0.0934&7.1863&13.9833&1.1893&52.036&32.3719&1.3854
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 160.4966&160.4589&2.2475&2.5795&1.7722&505.9077&176.1988&16.6654&245.4497&813.2289&2.2475
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
1768.6528&1768.6398&25.0076&32.1811&22.7893&2009.9973&5241.2101&175.5139&16778125.9621&14350456.5675&25.0076
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 1929.1494&1929.0987&27.2551&34.7606&24.5615&2515.905&5417.4089&192.1793&16778371.4118&14351269.7963&27.2551\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0034&0.0052&0.0033&0.0035&0.0036&Inf&14.8947&0.0034&0.0136&NaN&0.0033\\
\hline
\end{tabular}
}
\end{table}

==> Tables20220525/output/output20220520/20220519-10h55m12s-Full.beta=1.5.sig=2.n=30.LaTeX.tex <==
% START DATE AND TIME=20220519-10h55m12s
      \begin{table}[htbp]
  \centering
  \caption{$\beta=1.5,  \sigma=2$ $n=30$}
  \resizebox{\columnwidth}{!}{
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|r|r|}
      %\cline{2-13}    \multicolumn{1}{r|}{} &       & \multicolumn{11}{c|}{$\beta=1.5,  \sigma=2$ $n=30$} \\
\cline{2-13}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.CvM}} & \multicolumn{1}{l|}{\textbf{MDE.LS}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.X2}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.4901&2.1904&2.0696&1.6011&1.2928&2.5147&6.8422&2.1075&4.7683&-4.0642&2.0696
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
3.7605&3.1454&2.9696&2.1819&1.6477&10.8446&24.9727&3.1457&10.1186&-10.6768&2.9696
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 676.4235&677.077&4.3208&5.1165&4.1411&221.6163&508.585&24.9565&1262.0699&4183.0383&4.3208
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
1459.9615&1462.2551&16.5047&20.0532&15.751&2155.1416&7167.5418&99.245&2823.5225&25288.728&16.5047
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.9901&0.6904&0.5696&0.1011&-0.2072&1.0147&5.3422&0.6075&3.2683&-5.5642&0.5696
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
1.7605&1.1454&0.9696&0.1819&-0.3523&8.8446&22.9727&1.1457&8.1186&-12.6768&0.9696
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 677.3361&677.4859&4.6448&5.1262&4.1836&222.6237&537.0733&25.3231&1272.6254&4213.5804&4.6448
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
1462.9148&1463.4209&17.4432&20.0843&15.8735&2233.1523&7694.5721&100.5476&2889.1524&25446.901&17.4432
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 2140.2509&2140.9068&22.088&25.2105&20.0572&2455.776&8231.6454&125.8707&4161.7777&29660.4814&22.088\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0033&0.0045&0.0032&0.0034&0.0036&3.7320026081711e+300&0.0425&0.0033&0.0103&NaN&0.0032\\
\hline
\end{tabular}
}
\end{table}

==> Tables20220525/output/output20220520/20220519-10h55m12s-Full.beta=2.1.sig=2.n=30.LaTeX.tex <==
% START DATE AND TIME=20220519-10h55m12s
      \begin{table}[htbp]
  \centering
  \caption{$\beta=2.1,  \sigma=2$ $n=30$}
  \resizebox{\columnwidth}{!}{
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|r|r|}
      %\cline{2-13}    \multicolumn{1}{r|}{} &       & \multicolumn{11}{c|}{$\beta=2.1,  \sigma=2$ $n=30$} \\
\cline{2-13}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.CvM}} & \multicolumn{1}{l|}{\textbf{MDE.LS}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.X2}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 190.3827&190.1359&2.6848&2.1794&1.7069&6.2166&14.4035&3.3928&234.2205&207.4698&2.6848
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
307.25&306.9266&2.6748&2.1499&1.5989&14.4706&33.6177&3.6912&378.2798&343.2558&2.6748
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 347663582.8526&347663676.1193&11.6001&12.9381&11.3367&448.5575&1203.4724&71.6477&516949623.7701&517478254.8612&11.6001
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
917857063.1782&917857261.1597&21.6604&24.0655&21.2499&2545.5761&6995.7748&127.7713&1364784801.6468&1365233776.7568&21.6604
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 188.2827&188.0359&0.5848&0.0794&-0.3931&4.1166&12.3035&1.2928&232.1205&205.3698&0.5848
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
305.25&304.9266&0.6748&0.1499&-0.4011&12.4706&31.6177&1.6912&376.2798&341.2558&0.6748
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 347664266.8537&347664267.2401&11.941&12.9432&11.4901&465.4593&1354.7283&73.3117&516951808.7525&517468683.7706&11.941
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
917858455.0599&917858455.647&22.1136&24.0856&21.4086&2700.8372&7994.7561&130.6186&1364789909.6253&1365213708.8973&22.1136
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 1265522721.9136&1265522722.8871&34.0545&37.0287&32.8987&3166.2966&9349.4844&203.9303&1881741718.3778&1882682392.668&34.0545\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0033&0.0046&0.0033&0.0036&0.0038&0.0408&0.0349&0.0033&0.0058&NaN&0.0033\\
\hline
\end{tabular}
}
\end{table}

==> Tables20220525/output/output20220520/20220519-10h55m12s-Full.beta=2.sig=2.n=30.LaTeX.tex <==
% START DATE AND TIME=20220519-10h55m12s
      \begin{table}[htbp]
  \centering
  \caption{$\beta=2,  \sigma=2$ $n=30$}
  \resizebox{\columnwidth}{!}{
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|r|r|}
      %\cline{2-13}    \multicolumn{1}{r|}{} &       & \multicolumn{11}{c|}{$\beta=2,  \sigma=2$ $n=30$} \\
\cline{2-13}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.CvM}} & \multicolumn{1}{l|}{\textbf{MDE.LS}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.X2}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 3.5985&3.3375&2.5409&2.0315&1.5923&5.4862&12.9728&3.0757&6.5573&-11.3198&2.5409
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
4.2896&3.9212&2.6719&2.0958&1.5553&13.7122&32.4026&3.524&9.3146&-18.902&2.6719
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 582.0675&583.1951&9.484&10.7491&9.1678&376.4655&1074.9486&54.9588&1131.4863&64850.0259&9.484
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
1195.9372&1198.1041&22.9949&25.5117&22.4334&2377.2184&7185.6666&119.9379&2474.2323&125188.8812&22.9949
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.5985&1.3375&0.5409&0.0315&-0.4077&3.4862&10.9728&1.0757&4.5573&-13.3198&0.5409
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
2.2896&1.9212&0.6719&0.0958&-0.4447&11.7122&30.4026&1.524&7.3146&-20.902&0.6719
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 584.5646&584.9257&9.7756&10.749&9.3331&388.5811&1195.2431&56.1105&1152.1424&65020.9568&9.7756
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
1201.06&1201.6751&23.4441&25.5183&22.6289&2514.1573&8109.2662&122.2484&2527.4878&125613.2556&23.4441
\\
\hline
\multicolumn{2}{|c|}{Accuracy (Euclid Dist.)} & 1785.6246&1786.6008&33.2197&36.2673&31.962&2902.7384&9304.5093&178.3589&3679.6302&190634.2123&33.2197\\
\hline
\multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0033&0.0046&0.0032&0.0035&0.0037&1.72772079166811e+299&0.0369&0.0033&0.0066&NaN&0.0032\\
\hline
\end{tabular}
}
\end{table}

==> Tables20220525/output/output20220520/20220519-10h55m12s-Output.accuracy.LaTeX.tex <==
% latex table generated in R 4.0.5 by xtable 1.8-4 package
% Thu May 19 23:31:51 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & Measure & beta=1.1 & sigma=2 & n=30 & 1929.15 \\ 
  2 & MLE.b & Measure & beta=1.1 & sigma=2 & n=30 & 1929.10 \\ 
  3 & LME & Measure & beta=1.1 & sigma=2 & n=30 & 27.26 \\ 
  4 & MDE.CvM & Measure & beta=1.1 & sigma=2 & n=30 & 34.76 \\ 
  5 & MDE.LS & Measure & beta=1.1 & sigma=2 & n=30 & 24.56 \\ 
  6 & MDE.Phi.X2 & Measure & beta=1.1 & sigma=2 & n=30 & 2515.90 \\ 
  7 & MDE.Phi.tv & Measure & beta=1.1 & sigma=2 & n=30 & 5417.41 \\ 
  8 & MDE.Phi.kl & Measure & beta=1.1 & sigma=2 & n=30 & 192.18 \\ 
  9 & MME & Measure & beta=1.1 & sigma=2 & n=30 & 16778371.41 \\ 
  10 & MME.b & Measure & beta=1.1 & sigma=2 & n=30 & 14351269.80 \\ 
  11 & PWM & Measure & beta=1.1 & sigma=2 & n=30 & 27.26 \\ 
  12 & MLE & Measure & beta=1.5 & sigma=2 & n=30 & 2140.25 \\ 
  13 & MLE.b & Measure & beta=1.5 & sigma=2 & n=30 & 2140.91 \\ 
  14 & LME & Measure & beta=1.5 & sigma=2 & n=30 & 22.09 \\ 
  15 & MDE.CvM & Measure & beta=1.5 & sigma=2 & n=30 & 25.21 \\ 
  16 & MDE.LS & Measure & beta=1.5 & sigma=2 & n=30 & 20.06 \\ 
  17 & MDE.Phi.X2 & Measure & beta=1.5 & sigma=2 & n=30 & 2455.78 \\ 
  18 & MDE.Phi.tv & Measure & beta=1.5 & sigma=2 & n=30 & 8231.65 \\ 
  19 & MDE.Phi.kl & Measure & beta=1.5 & sigma=2 & n=30 & 125.87 \\ 
  20 & MME & Measure & beta=1.5 & sigma=2 & n=30 & 4161.78 \\ 
  21 & MME.b & Measure & beta=1.5 & sigma=2 & n=30 & 29660.48 \\ 
  22 & PWM & Measure & beta=1.5 & sigma=2 & n=30 & 22.09 \\ 
  23 & MLE & Measure & beta=2 & sigma=2 & n=30 & 1785.62 \\ 
  24 & MLE.b & Measure & beta=2 & sigma=2 & n=30 & 1786.60 \\ 
  25 & LME & Measure & beta=2 & sigma=2 & n=30 & 33.22 \\ 
  26 & MDE.CvM & Measure & beta=2 & sigma=2 & n=30 & 36.27 \\ 
  27 & MDE.LS & Measure & beta=2 & sigma=2 & n=30 & 31.96 \\ 
  28 & MDE.Phi.X2 & Measure & beta=2 & sigma=2 & n=30 & 2902.74 \\ 
  29 & MDE.Phi.tv & Measure & beta=2 & sigma=2 & n=30 & 9304.51 \\ 
  30 & MDE.Phi.kl & Measure & beta=2 & sigma=2 & n=30 & 178.36 \\ 
  31 & MME & Measure & beta=2 & sigma=2 & n=30 & 3679.63 \\ 
  32 & MME.b & Measure & beta=2 & sigma=2 & n=30 & 190634.21 \\ 
  33 & PWM & Measure & beta=2 & sigma=2 & n=30 & 33.22 \\ 
  34 & MLE & Measure & beta=2.1 & sigma=2 & n=30 & 1265522721.91 \\ 
  35 & MLE.b & Measure & beta=2.1 & sigma=2 & n=30 & 1265522722.89 \\ 
  36 & LME & Measure & beta=2.1 & sigma=2 & n=30 & 34.05 \\ 
  37 & MDE.CvM & Measure & beta=2.1 & sigma=2 & n=30 & 37.03 \\ 
  38 & MDE.LS & Measure & beta=2.1 & sigma=2 & n=30 & 32.90 \\ 
  39 & MDE.Phi.X2 & Measure & beta=2.1 & sigma=2 & n=30 & 3166.30 \\ 
  40 & MDE.Phi.tv & Measure & beta=2.1 & sigma=2 & n=30 & 9349.48 \\ 
  41 & MDE.Phi.kl & Measure & beta=2.1 & sigma=2 & n=30 & 203.93 \\ 
  42 & MME & Measure & beta=2.1 & sigma=2 & n=30 & 1881741718.38 \\ 
  43 & MME.b & Measure & beta=2.1 & sigma=2 & n=30 & 1882682392.67 \\ 
  44 & PWM & Measure & beta=2.1 & sigma=2 & n=30 & 34.05 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220520/20220519-10h55m12s-Output.accuracy2.LaTeX.tex <==
% latex table generated in R 4.0.5 by xtable 1.8-4 package
% Thu May 19 23:31:51 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & Measure & beta=1.1 & sigma=2 & n=30 & 0.00 \\ 
  2 & MLE.b & Measure & beta=1.1 & sigma=2 & n=30 & 0.01 \\ 
  3 & LME & Measure & beta=1.1 & sigma=2 & n=30 & 0.00 \\ 
  4 & MDE.CvM & Measure & beta=1.1 & sigma=2 & n=30 & 0.00 \\ 
  5 & MDE.LS & Measure & beta=1.1 & sigma=2 & n=30 & 0.00 \\ 
  6 & MDE.Phi.X2 & Measure & beta=1.1 & sigma=2 & n=30 & Inf \\ 
  7 & MDE.Phi.tv & Measure & beta=1.1 & sigma=2 & n=30 & 14.89 \\ 
  8 & MDE.Phi.kl & Measure & beta=1.1 & sigma=2 & n=30 & 0.00 \\ 
  9 & MME & Measure & beta=1.1 & sigma=2 & n=30 & 0.01 \\ 
  10 & MME.b & Measure & beta=1.1 & sigma=2 & n=30 &  \\ 
  11 & PWM & Measure & beta=1.1 & sigma=2 & n=30 & 0.00 \\ 
  12 & MLE & Measure & beta=1.5 & sigma=2 & n=30 & 0.00 \\ 
  13 & MLE.b & Measure & beta=1.5 & sigma=2 & n=30 & 0.00 \\ 
  14 & LME & Measure & beta=1.5 & sigma=2 & n=30 & 0.00 \\ 
  15 & MDE.CvM & Measure & beta=1.5 & sigma=2 & n=30 & 0.00 \\ 
  16 & MDE.LS & Measure & beta=1.5 & sigma=2 & n=30 & 0.00 \\ 
  17 & MDE.Phi.X2 & Measure & beta=1.5 & sigma=2 & n=30 & 3732002608171100715224820280888602262666228460008200604826020884600600866644640882868848600480882820804000882028064080000864660004886880268620022004220464888682606848408686868088262044620880664884828028848462822286268064260286220024460644448848206006248202886000824460042226484462068066460488004262266.00 \\ 
  18 & MDE.Phi.tv & Measure & beta=1.5 & sigma=2 & n=30 & 0.04 \\ 
  19 & MDE.Phi.kl & Measure & beta=1.5 & sigma=2 & n=30 & 0.00 \\ 
  20 & MME & Measure & beta=1.5 & sigma=2 & n=30 & 0.01 \\ 
  21 & MME.b & Measure & beta=1.5 & sigma=2 & n=30 &  \\ 
  22 & PWM & Measure & beta=1.5 & sigma=2 & n=30 & 0.00 \\ 
  23 & MLE & Measure & beta=2 & sigma=2 & n=30 & 0.00 \\ 
  24 & MLE.b & Measure & beta=2 & sigma=2 & n=30 & 0.00 \\ 
  25 & LME & Measure & beta=2 & sigma=2 & n=30 & 0.00 \\ 
  26 & MDE.CvM & Measure & beta=2 & sigma=2 & n=30 & 0.00 \\ 
  27 & MDE.LS & Measure & beta=2 & sigma=2 & n=30 & 0.00 \\ 
  28 & MDE.Phi.X2 & Measure & beta=2 & sigma=2 & n=30 & 172772079166811130272600628462262886608886808800220660820422686602028444606026666668426620422822620620286802688066802022082888088602462626064244602604260208600046240624804628668262644268826646402242884008080462824622844244442844462264684428420622462640682400802246246822408800440406206424064680686044.00 \\ 
  29 & MDE.Phi.tv & Measure & beta=2 & sigma=2 & n=30 & 0.04 \\ 
  30 & MDE.Phi.kl & Measure & beta=2 & sigma=2 & n=30 & 0.00 \\ 
  31 & MME & Measure & beta=2 & sigma=2 & n=30 & 0.01 \\ 
  32 & MME.b & Measure & beta=2 & sigma=2 & n=30 &  \\ 
  33 & PWM & Measure & beta=2 & sigma=2 & n=30 & 0.00 \\ 
  34 & MLE & Measure & beta=2.1 & sigma=2 & n=30 & 0.00 \\ 
  35 & MLE.b & Measure & beta=2.1 & sigma=2 & n=30 & 0.00 \\ 
  36 & LME & Measure & beta=2.1 & sigma=2 & n=30 & 0.00 \\ 
  37 & MDE.CvM & Measure & beta=2.1 & sigma=2 & n=30 & 0.00 \\ 
  38 & MDE.LS & Measure & beta=2.1 & sigma=2 & n=30 & 0.00 \\ 
  39 & MDE.Phi.X2 & Measure & beta=2.1 & sigma=2 & n=30 & 0.04 \\ 
  40 & MDE.Phi.tv & Measure & beta=2.1 & sigma=2 & n=30 & 0.03 \\ 
  41 & MDE.Phi.kl & Measure & beta=2.1 & sigma=2 & n=30 & 0.00 \\ 
  42 & MME & Measure & beta=2.1 & sigma=2 & n=30 & 0.01 \\ 
  43 & MME.b & Measure & beta=2.1 & sigma=2 & n=30 &  \\ 
  44 & PWM & Measure & beta=2.1 & sigma=2 & n=30 & 0.00 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220520/20220519-10h55m12s-Output.bias.LaTeX.tex <==
% latex table generated in R 4.0.5 by xtable 1.8-4 package
% Thu May 19 23:31:51 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.1 & sigma=2 & n=30 & 0.70 \\ 
  2 & MLE.b & beta & beta=1.1 & sigma=2 & n=30 & 0.41 \\ 
  3 & LME & beta & beta=1.1 & sigma=2 & n=30 & 0.64 \\ 
  4 & MDE.CvM & beta & beta=1.1 & sigma=2 & n=30 & 0.24 \\ 
  5 & MDE.LS & beta & beta=1.1 & sigma=2 & n=30 & 0.01 \\ 
  6 & MDE.Phi.X2 & beta & beta=1.1 & sigma=2 & n=30 & -2.76 \\ 
  7 & MDE.Phi.tv & beta & beta=1.1 & sigma=2 & n=30 & 1.95 \\ 
  8 & MDE.Phi.kl & beta & beta=1.1 & sigma=2 & n=30 & 0.50 \\ 
  9 & MME & beta & beta=1.1 & sigma=2 & n=30 & 2.54 \\ 
  10 & MME.b & beta & beta=1.1 & sigma=2 & n=30 & -2.49 \\ 
  11 & PWM & beta & beta=1.1 & sigma=2 & n=30 & 0.64 \\ 
  12 & MLE & sigma & beta=1.1 & sigma=2 & n=30 & 1.86 \\ 
  13 & MLE.b & sigma & beta=1.1 & sigma=2 & n=30 & 1.05 \\ 
  14 & LME & sigma & beta=1.1 & sigma=2 & n=30 & 1.39 \\ 
  15 & MDE.CvM & sigma & beta=1.1 & sigma=2 & n=30 & 0.47 \\ 
  16 & MDE.LS & sigma & beta=1.1 & sigma=2 & n=30 & -0.09 \\ 
  17 & MDE.Phi.X2 & sigma & beta=1.1 & sigma=2 & n=30 & 7.19 \\ 
  18 & MDE.Phi.tv & sigma & beta=1.1 & sigma=2 & n=30 & 13.98 \\ 
  19 & MDE.Phi.kl & sigma & beta=1.1 & sigma=2 & n=30 & 1.19 \\ 
  20 & MME & sigma & beta=1.1 & sigma=2 & n=30 & 52.04 \\ 
  21 & MME.b & sigma & beta=1.1 & sigma=2 & n=30 & 32.37 \\ 
  22 & PWM & sigma & beta=1.1 & sigma=2 & n=30 & 1.39 \\ 
  23 & MLE & beta & beta=1.5 & sigma=2 & n=30 & 0.99 \\ 
  24 & MLE.b & beta & beta=1.5 & sigma=2 & n=30 & 0.69 \\ 
  25 & LME & beta & beta=1.5 & sigma=2 & n=30 & 0.57 \\ 
  26 & MDE.CvM & beta & beta=1.5 & sigma=2 & n=30 & 0.10 \\ 
  27 & MDE.LS & beta & beta=1.5 & sigma=2 & n=30 & -0.21 \\ 
  28 & MDE.Phi.X2 & beta & beta=1.5 & sigma=2 & n=30 & 1.01 \\ 
  29 & MDE.Phi.tv & beta & beta=1.5 & sigma=2 & n=30 & 5.34 \\ 
  30 & MDE.Phi.kl & beta & beta=1.5 & sigma=2 & n=30 & 0.61 \\ 
  31 & MME & beta & beta=1.5 & sigma=2 & n=30 & 3.27 \\ 
  32 & MME.b & beta & beta=1.5 & sigma=2 & n=30 & -5.56 \\ 
  33 & PWM & beta & beta=1.5 & sigma=2 & n=30 & 0.57 \\ 
  34 & MLE & sigma & beta=1.5 & sigma=2 & n=30 & 1.76 \\ 
  35 & MLE.b & sigma & beta=1.5 & sigma=2 & n=30 & 1.15 \\ 
  36 & LME & sigma & beta=1.5 & sigma=2 & n=30 & 0.97 \\ 
  37 & MDE.CvM & sigma & beta=1.5 & sigma=2 & n=30 & 0.18 \\ 
  38 & MDE.LS & sigma & beta=1.5 & sigma=2 & n=30 & -0.35 \\ 
  39 & MDE.Phi.X2 & sigma & beta=1.5 & sigma=2 & n=30 & 8.84 \\ 
  40 & MDE.Phi.tv & sigma & beta=1.5 & sigma=2 & n=30 & 22.97 \\ 
  41 & MDE.Phi.kl & sigma & beta=1.5 & sigma=2 & n=30 & 1.15 \\ 
  42 & MME & sigma & beta=1.5 & sigma=2 & n=30 & 8.12 \\ 
  43 & MME.b & sigma & beta=1.5 & sigma=2 & n=30 & -12.68 \\ 
  44 & PWM & sigma & beta=1.5 & sigma=2 & n=30 & 0.97 \\ 
  45 & MLE & beta & beta=2 & sigma=2 & n=30 & 1.60 \\ 
  46 & MLE.b & beta & beta=2 & sigma=2 & n=30 & 1.34 \\ 
  47 & LME & beta & beta=2 & sigma=2 & n=30 & 0.54 \\ 
  48 & MDE.CvM & beta & beta=2 & sigma=2 & n=30 & 0.03 \\ 
  49 & MDE.LS & beta & beta=2 & sigma=2 & n=30 & -0.41 \\ 
  50 & MDE.Phi.X2 & beta & beta=2 & sigma=2 & n=30 & 3.49 \\ 
  51 & MDE.Phi.tv & beta & beta=2 & sigma=2 & n=30 & 10.97 \\ 
  52 & MDE.Phi.kl & beta & beta=2 & sigma=2 & n=30 & 1.08 \\ 
  53 & MME & beta & beta=2 & sigma=2 & n=30 & 4.56 \\ 
  54 & MME.b & beta & beta=2 & sigma=2 & n=30 & -13.32 \\ 
  55 & PWM & beta & beta=2 & sigma=2 & n=30 & 0.54 \\ 
  56 & MLE & sigma & beta=2 & sigma=2 & n=30 & 2.29 \\ 
  57 & MLE.b & sigma & beta=2 & sigma=2 & n=30 & 1.92 \\ 
  58 & LME & sigma & beta=2 & sigma=2 & n=30 & 0.67 \\ 
  59 & MDE.CvM & sigma & beta=2 & sigma=2 & n=30 & 0.10 \\ 
  60 & MDE.LS & sigma & beta=2 & sigma=2 & n=30 & -0.44 \\ 
  61 & MDE.Phi.X2 & sigma & beta=2 & sigma=2 & n=30 & 11.71 \\ 
  62 & MDE.Phi.tv & sigma & beta=2 & sigma=2 & n=30 & 30.40 \\ 
  63 & MDE.Phi.kl & sigma & beta=2 & sigma=2 & n=30 & 1.52 \\ 
  64 & MME & sigma & beta=2 & sigma=2 & n=30 & 7.31 \\ 
  65 & MME.b & sigma & beta=2 & sigma=2 & n=30 & -20.90 \\ 
  66 & PWM & sigma & beta=2 & sigma=2 & n=30 & 0.67 \\ 
  67 & MLE & beta & beta=2.1 & sigma=2 & n=30 & 188.28 \\ 
  68 & MLE.b & beta & beta=2.1 & sigma=2 & n=30 & 188.04 \\ 
  69 & LME & beta & beta=2.1 & sigma=2 & n=30 & 0.58 \\ 
  70 & MDE.CvM & beta & beta=2.1 & sigma=2 & n=30 & 0.08 \\ 
  71 & MDE.LS & beta & beta=2.1 & sigma=2 & n=30 & -0.39 \\ 
  72 & MDE.Phi.X2 & beta & beta=2.1 & sigma=2 & n=30 & 4.12 \\ 
  73 & MDE.Phi.tv & beta & beta=2.1 & sigma=2 & n=30 & 12.30 \\ 
  74 & MDE.Phi.kl & beta & beta=2.1 & sigma=2 & n=30 & 1.29 \\ 
  75 & MME & beta & beta=2.1 & sigma=2 & n=30 & 232.12 \\ 
  76 & MME.b & beta & beta=2.1 & sigma=2 & n=30 & 205.37 \\ 
  77 & PWM & beta & beta=2.1 & sigma=2 & n=30 & 0.58 \\ 
  78 & MLE & sigma & beta=2.1 & sigma=2 & n=30 & 305.25 \\ 
  79 & MLE.b & sigma & beta=2.1 & sigma=2 & n=30 & 304.93 \\ 
  80 & LME & sigma & beta=2.1 & sigma=2 & n=30 & 0.67 \\ 
  81 & MDE.CvM & sigma & beta=2.1 & sigma=2 & n=30 & 0.15 \\ 
  82 & MDE.LS & sigma & beta=2.1 & sigma=2 & n=30 & -0.40 \\ 
  83 & MDE.Phi.X2 & sigma & beta=2.1 & sigma=2 & n=30 & 12.47 \\ 
  84 & MDE.Phi.tv & sigma & beta=2.1 & sigma=2 & n=30 & 31.62 \\ 
  85 & MDE.Phi.kl & sigma & beta=2.1 & sigma=2 & n=30 & 1.69 \\ 
  86 & MME & sigma & beta=2.1 & sigma=2 & n=30 & 376.28 \\ 
  87 & MME.b & sigma & beta=2.1 & sigma=2 & n=30 & 341.26 \\ 
  88 & PWM & sigma & beta=2.1 & sigma=2 & n=30 & 0.67 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220520/20220519-10h55m12s-Output.mean.LaTeX.tex <==
% latex table generated in R 4.0.5 by xtable 1.8-4 package
% Thu May 19 23:31:51 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.1 & sigma=2 & n=30 & 1.80 \\ 
  2 & MLE.b & beta & beta=1.1 & sigma=2 & n=30 & 1.51 \\ 
  3 & LME & beta & beta=1.1 & sigma=2 & n=30 & 1.74 \\ 
  4 & MDE.CvM & beta & beta=1.1 & sigma=2 & n=30 & 1.34 \\ 
  5 & MDE.LS & beta & beta=1.1 & sigma=2 & n=30 & 1.11 \\ 
  6 & MDE.Phi.X2 & beta & beta=1.1 & sigma=2 & n=30 & -1.66 \\ 
  7 & MDE.Phi.tv & beta & beta=1.1 & sigma=2 & n=30 & 3.05 \\ 
  8 & MDE.Phi.kl & beta & beta=1.1 & sigma=2 & n=30 & 1.60 \\ 
  9 & MME & beta & beta=1.1 & sigma=2 & n=30 & 3.64 \\ 
  10 & MME.b & beta & beta=1.1 & sigma=2 & n=30 & -1.39 \\ 
  11 & PWM & beta & beta=1.1 & sigma=2 & n=30 & 1.74 \\ 
  12 & MLE & sigma & beta=1.1 & sigma=2 & n=30 & 3.86 \\ 
  13 & MLE.b & sigma & beta=1.1 & sigma=2 & n=30 & 3.05 \\ 
  14 & LME & sigma & beta=1.1 & sigma=2 & n=30 & 3.39 \\ 
  15 & MDE.CvM & sigma & beta=1.1 & sigma=2 & n=30 & 2.47 \\ 
  16 & MDE.LS & sigma & beta=1.1 & sigma=2 & n=30 & 1.91 \\ 
  17 & MDE.Phi.X2 & sigma & beta=1.1 & sigma=2 & n=30 & 9.19 \\ 
  18 & MDE.Phi.tv & sigma & beta=1.1 & sigma=2 & n=30 & 15.98 \\ 
  19 & MDE.Phi.kl & sigma & beta=1.1 & sigma=2 & n=30 & 3.19 \\ 
  20 & MME & sigma & beta=1.1 & sigma=2 & n=30 & 54.04 \\ 
  21 & MME.b & sigma & beta=1.1 & sigma=2 & n=30 & 34.37 \\ 
  22 & PWM & sigma & beta=1.1 & sigma=2 & n=30 & 3.39 \\ 
  23 & MLE & beta & beta=1.5 & sigma=2 & n=30 & 2.49 \\ 
  24 & MLE.b & beta & beta=1.5 & sigma=2 & n=30 & 2.19 \\ 
  25 & LME & beta & beta=1.5 & sigma=2 & n=30 & 2.07 \\ 
  26 & MDE.CvM & beta & beta=1.5 & sigma=2 & n=30 & 1.60 \\ 
  27 & MDE.LS & beta & beta=1.5 & sigma=2 & n=30 & 1.29 \\ 
  28 & MDE.Phi.X2 & beta & beta=1.5 & sigma=2 & n=30 & 2.51 \\ 
  29 & MDE.Phi.tv & beta & beta=1.5 & sigma=2 & n=30 & 6.84 \\ 
  30 & MDE.Phi.kl & beta & beta=1.5 & sigma=2 & n=30 & 2.11 \\ 
  31 & MME & beta & beta=1.5 & sigma=2 & n=30 & 4.77 \\ 
  32 & MME.b & beta & beta=1.5 & sigma=2 & n=30 & -4.06 \\ 
  33 & PWM & beta & beta=1.5 & sigma=2 & n=30 & 2.07 \\ 
  34 & MLE & sigma & beta=1.5 & sigma=2 & n=30 & 3.76 \\ 
  35 & MLE.b & sigma & beta=1.5 & sigma=2 & n=30 & 3.15 \\ 
  36 & LME & sigma & beta=1.5 & sigma=2 & n=30 & 2.97 \\ 
  37 & MDE.CvM & sigma & beta=1.5 & sigma=2 & n=30 & 2.18 \\ 
  38 & MDE.LS & sigma & beta=1.5 & sigma=2 & n=30 & 1.65 \\ 
  39 & MDE.Phi.X2 & sigma & beta=1.5 & sigma=2 & n=30 & 10.84 \\ 
  40 & MDE.Phi.tv & sigma & beta=1.5 & sigma=2 & n=30 & 24.97 \\ 
  41 & MDE.Phi.kl & sigma & beta=1.5 & sigma=2 & n=30 & 3.15 \\ 
  42 & MME & sigma & beta=1.5 & sigma=2 & n=30 & 10.12 \\ 
  43 & MME.b & sigma & beta=1.5 & sigma=2 & n=30 & -10.68 \\ 
  44 & PWM & sigma & beta=1.5 & sigma=2 & n=30 & 2.97 \\ 
  45 & MLE & beta & beta=2 & sigma=2 & n=30 & 3.60 \\ 
  46 & MLE.b & beta & beta=2 & sigma=2 & n=30 & 3.34 \\ 
  47 & LME & beta & beta=2 & sigma=2 & n=30 & 2.54 \\ 
  48 & MDE.CvM & beta & beta=2 & sigma=2 & n=30 & 2.03 \\ 
  49 & MDE.LS & beta & beta=2 & sigma=2 & n=30 & 1.59 \\ 
  50 & MDE.Phi.X2 & beta & beta=2 & sigma=2 & n=30 & 5.49 \\ 
  51 & MDE.Phi.tv & beta & beta=2 & sigma=2 & n=30 & 12.97 \\ 
  52 & MDE.Phi.kl & beta & beta=2 & sigma=2 & n=30 & 3.08 \\ 
  53 & MME & beta & beta=2 & sigma=2 & n=30 & 6.56 \\ 
  54 & MME.b & beta & beta=2 & sigma=2 & n=30 & -11.32 \\ 
  55 & PWM & beta & beta=2 & sigma=2 & n=30 & 2.54 \\ 
  56 & MLE & sigma & beta=2 & sigma=2 & n=30 & 4.29 \\ 
  57 & MLE.b & sigma & beta=2 & sigma=2 & n=30 & 3.92 \\ 
  58 & LME & sigma & beta=2 & sigma=2 & n=30 & 2.67 \\ 
  59 & MDE.CvM & sigma & beta=2 & sigma=2 & n=30 & 2.10 \\ 
  60 & MDE.LS & sigma & beta=2 & sigma=2 & n=30 & 1.56 \\ 
  61 & MDE.Phi.X2 & sigma & beta=2 & sigma=2 & n=30 & 13.71 \\ 
  62 & MDE.Phi.tv & sigma & beta=2 & sigma=2 & n=30 & 32.40 \\ 
  63 & MDE.Phi.kl & sigma & beta=2 & sigma=2 & n=30 & 3.52 \\ 
  64 & MME & sigma & beta=2 & sigma=2 & n=30 & 9.31 \\ 
  65 & MME.b & sigma & beta=2 & sigma=2 & n=30 & -18.90 \\ 
  66 & PWM & sigma & beta=2 & sigma=2 & n=30 & 2.67 \\ 
  67 & MLE & beta & beta=2.1 & sigma=2 & n=30 & 190.38 \\ 
  68 & MLE.b & beta & beta=2.1 & sigma=2 & n=30 & 190.14 \\ 
  69 & LME & beta & beta=2.1 & sigma=2 & n=30 & 2.68 \\ 
  70 & MDE.CvM & beta & beta=2.1 & sigma=2 & n=30 & 2.18 \\ 
  71 & MDE.LS & beta & beta=2.1 & sigma=2 & n=30 & 1.71 \\ 
  72 & MDE.Phi.X2 & beta & beta=2.1 & sigma=2 & n=30 & 6.22 \\ 
  73 & MDE.Phi.tv & beta & beta=2.1 & sigma=2 & n=30 & 14.40 \\ 
  74 & MDE.Phi.kl & beta & beta=2.1 & sigma=2 & n=30 & 3.39 \\ 
  75 & MME & beta & beta=2.1 & sigma=2 & n=30 & 234.22 \\ 
  76 & MME.b & beta & beta=2.1 & sigma=2 & n=30 & 207.47 \\ 
  77 & PWM & beta & beta=2.1 & sigma=2 & n=30 & 2.68 \\ 
  78 & MLE & sigma & beta=2.1 & sigma=2 & n=30 & 307.25 \\ 
  79 & MLE.b & sigma & beta=2.1 & sigma=2 & n=30 & 306.93 \\ 
  80 & LME & sigma & beta=2.1 & sigma=2 & n=30 & 2.67 \\ 
  81 & MDE.CvM & sigma & beta=2.1 & sigma=2 & n=30 & 2.15 \\ 
  82 & MDE.LS & sigma & beta=2.1 & sigma=2 & n=30 & 1.60 \\ 
  83 & MDE.Phi.X2 & sigma & beta=2.1 & sigma=2 & n=30 & 14.47 \\ 
  84 & MDE.Phi.tv & sigma & beta=2.1 & sigma=2 & n=30 & 33.62 \\ 
  85 & MDE.Phi.kl & sigma & beta=2.1 & sigma=2 & n=30 & 3.69 \\ 
  86 & MME & sigma & beta=2.1 & sigma=2 & n=30 & 378.28 \\ 
  87 & MME.b & sigma & beta=2.1 & sigma=2 & n=30 & 343.26 \\ 
  88 & PWM & sigma & beta=2.1 & sigma=2 & n=30 & 2.67 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220520/20220519-10h55m12s-Output.mse.LaTeX.tex <==
% latex table generated in R 4.0.5 by xtable 1.8-4 package
% Thu May 19 23:31:51 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.1 & sigma=2 & n=30 & 160.50 \\ 
  2 & MLE.b & beta & beta=1.1 & sigma=2 & n=30 & 160.46 \\ 
  3 & LME & beta & beta=1.1 & sigma=2 & n=30 & 2.25 \\ 
  4 & MDE.CvM & beta & beta=1.1 & sigma=2 & n=30 & 2.58 \\ 
  5 & MDE.LS & beta & beta=1.1 & sigma=2 & n=30 & 1.77 \\ 
  6 & MDE.Phi.X2 & beta & beta=1.1 & sigma=2 & n=30 & 505.91 \\ 
  7 & MDE.Phi.tv & beta & beta=1.1 & sigma=2 & n=30 & 176.20 \\ 
  8 & MDE.Phi.kl & beta & beta=1.1 & sigma=2 & n=30 & 16.67 \\ 
  9 & MME & beta & beta=1.1 & sigma=2 & n=30 & 245.45 \\ 
  10 & MME.b & beta & beta=1.1 & sigma=2 & n=30 & 813.23 \\ 
  11 & PWM & beta & beta=1.1 & sigma=2 & n=30 & 2.25 \\ 
  12 & MLE & sigma & beta=1.1 & sigma=2 & n=30 & 1768.65 \\ 
  13 & MLE.b & sigma & beta=1.1 & sigma=2 & n=30 & 1768.64 \\ 
  14 & LME & sigma & beta=1.1 & sigma=2 & n=30 & 25.01 \\ 
  15 & MDE.CvM & sigma & beta=1.1 & sigma=2 & n=30 & 32.18 \\ 
  16 & MDE.LS & sigma & beta=1.1 & sigma=2 & n=30 & 22.79 \\ 
  17 & MDE.Phi.X2 & sigma & beta=1.1 & sigma=2 & n=30 & 2010.00 \\ 
  18 & MDE.Phi.tv & sigma & beta=1.1 & sigma=2 & n=30 & 5241.21 \\ 
  19 & MDE.Phi.kl & sigma & beta=1.1 & sigma=2 & n=30 & 175.51 \\ 
  20 & MME & sigma & beta=1.1 & sigma=2 & n=30 & 16778125.96 \\ 
  21 & MME.b & sigma & beta=1.1 & sigma=2 & n=30 & 14350456.57 \\ 
  22 & PWM & sigma & beta=1.1 & sigma=2 & n=30 & 25.01 \\ 
  23 & MLE & beta & beta=1.5 & sigma=2 & n=30 & 677.34 \\ 
  24 & MLE.b & beta & beta=1.5 & sigma=2 & n=30 & 677.49 \\ 
  25 & LME & beta & beta=1.5 & sigma=2 & n=30 & 4.64 \\ 
  26 & MDE.CvM & beta & beta=1.5 & sigma=2 & n=30 & 5.13 \\ 
  27 & MDE.LS & beta & beta=1.5 & sigma=2 & n=30 & 4.18 \\ 
  28 & MDE.Phi.X2 & beta & beta=1.5 & sigma=2 & n=30 & 222.62 \\ 
  29 & MDE.Phi.tv & beta & beta=1.5 & sigma=2 & n=30 & 537.07 \\ 
  30 & MDE.Phi.kl & beta & beta=1.5 & sigma=2 & n=30 & 25.32 \\ 
  31 & MME & beta & beta=1.5 & sigma=2 & n=30 & 1272.63 \\ 
  32 & MME.b & beta & beta=1.5 & sigma=2 & n=30 & 4213.58 \\ 
  33 & PWM & beta & beta=1.5 & sigma=2 & n=30 & 4.64 \\ 
  34 & MLE & sigma & beta=1.5 & sigma=2 & n=30 & 1462.91 \\ 
  35 & MLE.b & sigma & beta=1.5 & sigma=2 & n=30 & 1463.42 \\ 
  36 & LME & sigma & beta=1.5 & sigma=2 & n=30 & 17.44 \\ 
  37 & MDE.CvM & sigma & beta=1.5 & sigma=2 & n=30 & 20.08 \\ 
  38 & MDE.LS & sigma & beta=1.5 & sigma=2 & n=30 & 15.87 \\ 
  39 & MDE.Phi.X2 & sigma & beta=1.5 & sigma=2 & n=30 & 2233.15 \\ 
  40 & MDE.Phi.tv & sigma & beta=1.5 & sigma=2 & n=30 & 7694.57 \\ 
  41 & MDE.Phi.kl & sigma & beta=1.5 & sigma=2 & n=30 & 100.55 \\ 
  42 & MME & sigma & beta=1.5 & sigma=2 & n=30 & 2889.15 \\ 
  43 & MME.b & sigma & beta=1.5 & sigma=2 & n=30 & 25446.90 \\ 
  44 & PWM & sigma & beta=1.5 & sigma=2 & n=30 & 17.44 \\ 
  45 & MLE & beta & beta=2 & sigma=2 & n=30 & 584.56 \\ 
  46 & MLE.b & beta & beta=2 & sigma=2 & n=30 & 584.93 \\ 
  47 & LME & beta & beta=2 & sigma=2 & n=30 & 9.78 \\ 
  48 & MDE.CvM & beta & beta=2 & sigma=2 & n=30 & 10.75 \\ 
  49 & MDE.LS & beta & beta=2 & sigma=2 & n=30 & 9.33 \\ 
  50 & MDE.Phi.X2 & beta & beta=2 & sigma=2 & n=30 & 388.58 \\ 
  51 & MDE.Phi.tv & beta & beta=2 & sigma=2 & n=30 & 1195.24 \\ 
  52 & MDE.Phi.kl & beta & beta=2 & sigma=2 & n=30 & 56.11 \\ 
  53 & MME & beta & beta=2 & sigma=2 & n=30 & 1152.14 \\ 
  54 & MME.b & beta & beta=2 & sigma=2 & n=30 & 65020.96 \\ 
  55 & PWM & beta & beta=2 & sigma=2 & n=30 & 9.78 \\ 
  56 & MLE & sigma & beta=2 & sigma=2 & n=30 & 1201.06 \\ 
  57 & MLE.b & sigma & beta=2 & sigma=2 & n=30 & 1201.68 \\ 
  58 & LME & sigma & beta=2 & sigma=2 & n=30 & 23.44 \\ 
  59 & MDE.CvM & sigma & beta=2 & sigma=2 & n=30 & 25.52 \\ 
  60 & MDE.LS & sigma & beta=2 & sigma=2 & n=30 & 22.63 \\ 
  61 & MDE.Phi.X2 & sigma & beta=2 & sigma=2 & n=30 & 2514.16 \\ 
  62 & MDE.Phi.tv & sigma & beta=2 & sigma=2 & n=30 & 8109.27 \\ 
  63 & MDE.Phi.kl & sigma & beta=2 & sigma=2 & n=30 & 122.25 \\ 
  64 & MME & sigma & beta=2 & sigma=2 & n=30 & 2527.49 \\ 
  65 & MME.b & sigma & beta=2 & sigma=2 & n=30 & 125613.26 \\ 
  66 & PWM & sigma & beta=2 & sigma=2 & n=30 & 23.44 \\ 
  67 & MLE & beta & beta=2.1 & sigma=2 & n=30 & 347664266.85 \\ 
  68 & MLE.b & beta & beta=2.1 & sigma=2 & n=30 & 347664267.24 \\ 
  69 & LME & beta & beta=2.1 & sigma=2 & n=30 & 11.94 \\ 
  70 & MDE.CvM & beta & beta=2.1 & sigma=2 & n=30 & 12.94 \\ 
  71 & MDE.LS & beta & beta=2.1 & sigma=2 & n=30 & 11.49 \\ 
  72 & MDE.Phi.X2 & beta & beta=2.1 & sigma=2 & n=30 & 465.46 \\ 
  73 & MDE.Phi.tv & beta & beta=2.1 & sigma=2 & n=30 & 1354.73 \\ 
  74 & MDE.Phi.kl & beta & beta=2.1 & sigma=2 & n=30 & 73.31 \\ 
  75 & MME & beta & beta=2.1 & sigma=2 & n=30 & 516951808.75 \\ 
  76 & MME.b & beta & beta=2.1 & sigma=2 & n=30 & 517468683.77 \\ 
  77 & PWM & beta & beta=2.1 & sigma=2 & n=30 & 11.94 \\ 
  78 & MLE & sigma & beta=2.1 & sigma=2 & n=30 & 917858455.06 \\ 
  79 & MLE.b & sigma & beta=2.1 & sigma=2 & n=30 & 917858455.65 \\ 
  80 & LME & sigma & beta=2.1 & sigma=2 & n=30 & 22.11 \\ 
  81 & MDE.CvM & sigma & beta=2.1 & sigma=2 & n=30 & 24.09 \\ 
  82 & MDE.LS & sigma & beta=2.1 & sigma=2 & n=30 & 21.41 \\ 
  83 & MDE.Phi.X2 & sigma & beta=2.1 & sigma=2 & n=30 & 2700.84 \\ 
  84 & MDE.Phi.tv & sigma & beta=2.1 & sigma=2 & n=30 & 7994.76 \\ 
  85 & MDE.Phi.kl & sigma & beta=2.1 & sigma=2 & n=30 & 130.62 \\ 
  86 & MME & sigma & beta=2.1 & sigma=2 & n=30 & 1364789909.63 \\ 
  87 & MME.b & sigma & beta=2.1 & sigma=2 & n=30 & 1365213708.90 \\ 
  88 & PWM & sigma & beta=2.1 & sigma=2 & n=30 & 22.11 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220520/20220519-10h55m12s-Output.var.LaTeX.tex <==
% latex table generated in R 4.0.5 by xtable 1.8-4 package
% Thu May 19 23:31:51 2022
\begin{table}[ht]
\centering
\begin{tabular}{rlllllr}
  \hline
 & Var1 & Var2 & Var3 & Var4 & Var5 & Freq \\ 
  \hline
1 & MLE & beta & beta=1.1 & sigma=2 & n=30 & 160.02 \\ 
  2 & MLE.b & beta & beta=1.1 & sigma=2 & n=30 & 160.31 \\ 
  3 & LME & beta & beta=1.1 & sigma=2 & n=30 & 1.84 \\ 
  4 & MDE.CvM & beta & beta=1.1 & sigma=2 & n=30 & 2.52 \\ 
  5 & MDE.LS & beta & beta=1.1 & sigma=2 & n=30 & 1.77 \\ 
  6 & MDE.Phi.X2 & beta & beta=1.1 & sigma=2 & n=30 & 498.32 \\ 
  7 & MDE.Phi.tv & beta & beta=1.1 & sigma=2 & n=30 & 172.42 \\ 
  8 & MDE.Phi.kl & beta & beta=1.1 & sigma=2 & n=30 & 16.42 \\ 
  9 & MME & beta & beta=1.1 & sigma=2 & n=30 & 239.04 \\ 
  10 & MME.b & beta & beta=1.1 & sigma=2 & n=30 & 807.10 \\ 
  11 & PWM & beta & beta=1.1 & sigma=2 & n=30 & 1.84 \\ 
  12 & MLE & sigma & beta=1.1 & sigma=2 & n=30 & 1765.37 \\ 
  13 & MLE.b & sigma & beta=1.1 & sigma=2 & n=30 & 1767.72 \\ 
  14 & LME & sigma & beta=1.1 & sigma=2 & n=30 & 23.09 \\ 
  15 & MDE.CvM & sigma & beta=1.1 & sigma=2 & n=30 & 31.97 \\ 
  16 & MDE.LS & sigma & beta=1.1 & sigma=2 & n=30 & 22.78 \\ 
  17 & MDE.Phi.X2 & sigma & beta=1.1 & sigma=2 & n=30 & 1958.55 \\ 
  18 & MDE.Phi.tv & sigma & beta=1.1 & sigma=2 & n=30 & 5046.18 \\ 
  19 & MDE.Phi.kl & sigma & beta=1.1 & sigma=2 & n=30 & 174.12 \\ 
  20 & MME & sigma & beta=1.1 & sigma=2 & n=30 & 16777095.92 \\ 
  21 & MME.b & sigma & beta=1.1 & sigma=2 & n=30 & 14350843.71 \\ 
  22 & PWM & sigma & beta=1.1 & sigma=2 & n=30 & 23.09 \\ 
  23 & MLE & beta & beta=1.5 & sigma=2 & n=30 & 676.42 \\ 
  24 & MLE.b & beta & beta=1.5 & sigma=2 & n=30 & 677.08 \\ 
  25 & LME & beta & beta=1.5 & sigma=2 & n=30 & 4.32 \\ 
  26 & MDE.CvM & beta & beta=1.5 & sigma=2 & n=30 & 5.12 \\ 
  27 & MDE.LS & beta & beta=1.5 & sigma=2 & n=30 & 4.14 \\ 
  28 & MDE.Phi.X2 & beta & beta=1.5 & sigma=2 & n=30 & 221.62 \\ 
  29 & MDE.Phi.tv & beta & beta=1.5 & sigma=2 & n=30 & 508.59 \\ 
  30 & MDE.Phi.kl & beta & beta=1.5 & sigma=2 & n=30 & 24.96 \\ 
  31 & MME & beta & beta=1.5 & sigma=2 & n=30 & 1262.07 \\ 
  32 & MME.b & beta & beta=1.5 & sigma=2 & n=30 & 4183.04 \\ 
  33 & PWM & beta & beta=1.5 & sigma=2 & n=30 & 4.32 \\ 
  34 & MLE & sigma & beta=1.5 & sigma=2 & n=30 & 1459.96 \\ 
  35 & MLE.b & sigma & beta=1.5 & sigma=2 & n=30 & 1462.26 \\ 
  36 & LME & sigma & beta=1.5 & sigma=2 & n=30 & 16.50 \\ 
  37 & MDE.CvM & sigma & beta=1.5 & sigma=2 & n=30 & 20.05 \\ 
  38 & MDE.LS & sigma & beta=1.5 & sigma=2 & n=30 & 15.75 \\ 
  39 & MDE.Phi.X2 & sigma & beta=1.5 & sigma=2 & n=30 & 2155.14 \\ 
  40 & MDE.Phi.tv & sigma & beta=1.5 & sigma=2 & n=30 & 7167.54 \\ 
  41 & MDE.Phi.kl & sigma & beta=1.5 & sigma=2 & n=30 & 99.24 \\ 
  42 & MME & sigma & beta=1.5 & sigma=2 & n=30 & 2823.52 \\ 
  43 & MME.b & sigma & beta=1.5 & sigma=2 & n=30 & 25288.73 \\ 
  44 & PWM & sigma & beta=1.5 & sigma=2 & n=30 & 16.50 \\ 
  45 & MLE & beta & beta=2 & sigma=2 & n=30 & 582.07 \\ 
  46 & MLE.b & beta & beta=2 & sigma=2 & n=30 & 583.20 \\ 
  47 & LME & beta & beta=2 & sigma=2 & n=30 & 9.48 \\ 
  48 & MDE.CvM & beta & beta=2 & sigma=2 & n=30 & 10.75 \\ 
  49 & MDE.LS & beta & beta=2 & sigma=2 & n=30 & 9.17 \\ 
  50 & MDE.Phi.X2 & beta & beta=2 & sigma=2 & n=30 & 376.47 \\ 
  51 & MDE.Phi.tv & beta & beta=2 & sigma=2 & n=30 & 1074.95 \\ 
  52 & MDE.Phi.kl & beta & beta=2 & sigma=2 & n=30 & 54.96 \\ 
  53 & MME & beta & beta=2 & sigma=2 & n=30 & 1131.49 \\ 
  54 & MME.b & beta & beta=2 & sigma=2 & n=30 & 64850.03 \\ 
  55 & PWM & beta & beta=2 & sigma=2 & n=30 & 9.48 \\ 
  56 & MLE & sigma & beta=2 & sigma=2 & n=30 & 1195.94 \\ 
  57 & MLE.b & sigma & beta=2 & sigma=2 & n=30 & 1198.10 \\ 
  58 & LME & sigma & beta=2 & sigma=2 & n=30 & 22.99 \\ 
  59 & MDE.CvM & sigma & beta=2 & sigma=2 & n=30 & 25.51 \\ 
  60 & MDE.LS & sigma & beta=2 & sigma=2 & n=30 & 22.43 \\ 
  61 & MDE.Phi.X2 & sigma & beta=2 & sigma=2 & n=30 & 2377.22 \\ 
  62 & MDE.Phi.tv & sigma & beta=2 & sigma=2 & n=30 & 7185.67 \\ 
  63 & MDE.Phi.kl & sigma & beta=2 & sigma=2 & n=30 & 119.94 \\ 
  64 & MME & sigma & beta=2 & sigma=2 & n=30 & 2474.23 \\ 
  65 & MME.b & sigma & beta=2 & sigma=2 & n=30 & 125188.88 \\ 
  66 & PWM & sigma & beta=2 & sigma=2 & n=30 & 22.99 \\ 
  67 & MLE & beta & beta=2.1 & sigma=2 & n=30 & 347663582.85 \\ 
  68 & MLE.b & beta & beta=2.1 & sigma=2 & n=30 & 347663676.12 \\ 
  69 & LME & beta & beta=2.1 & sigma=2 & n=30 & 11.60 \\ 
  70 & MDE.CvM & beta & beta=2.1 & sigma=2 & n=30 & 12.94 \\ 
  71 & MDE.LS & beta & beta=2.1 & sigma=2 & n=30 & 11.34 \\ 
  72 & MDE.Phi.X2 & beta & beta=2.1 & sigma=2 & n=30 & 448.56 \\ 
  73 & MDE.Phi.tv & beta & beta=2.1 & sigma=2 & n=30 & 1203.47 \\ 
  74 & MDE.Phi.kl & beta & beta=2.1 & sigma=2 & n=30 & 71.65 \\ 
  75 & MME & beta & beta=2.1 & sigma=2 & n=30 & 516949623.77 \\ 
  76 & MME.b & beta & beta=2.1 & sigma=2 & n=30 & 517478254.86 \\ 
  77 & PWM & beta & beta=2.1 & sigma=2 & n=30 & 11.60 \\ 
  78 & MLE & sigma & beta=2.1 & sigma=2 & n=30 & 917857063.18 \\ 
  79 & MLE.b & sigma & beta=2.1 & sigma=2 & n=30 & 917857261.16 \\ 
  80 & LME & sigma & beta=2.1 & sigma=2 & n=30 & 21.66 \\ 
  81 & MDE.CvM & sigma & beta=2.1 & sigma=2 & n=30 & 24.07 \\ 
  82 & MDE.LS & sigma & beta=2.1 & sigma=2 & n=30 & 21.25 \\ 
  83 & MDE.Phi.X2 & sigma & beta=2.1 & sigma=2 & n=30 & 2545.58 \\ 
  84 & MDE.Phi.tv & sigma & beta=2.1 & sigma=2 & n=30 & 6995.77 \\ 
  85 & MDE.Phi.kl & sigma & beta=2.1 & sigma=2 & n=30 & 127.77 \\ 
  86 & MME & sigma & beta=2.1 & sigma=2 & n=30 & 1364784801.65 \\ 
  87 & MME.b & sigma & beta=2.1 & sigma=2 & n=30 & 1365233776.76 \\ 
  88 & PWM & sigma & beta=2.1 & sigma=2 & n=30 & 21.66 \\ 
   \hline
\end{tabular}
\end{table}


==> Tables20220525/output/output20220520/n100sig05.tex <==
% START DATE AND TIME=20220517-11h19m32s
      \begin{table}[htbp]
  \centering
%   \caption{$\beta=1.1,  \sigma=0.5$ $n=100$}
\caption{Comparison of different estimation methods for different values of $\beta$ ($\sigma=0.5$ and $n=100$). \label{tbl:n100sig05}}
%   \resizebox{\columnwidth}{!}{
%     \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|r|r|}
%       %\cline{2-13}    \multicolumn{1}{r|}{} &       & \multicolumn{11}{c|}{$\beta=1.1,  \sigma=0.5$ $n=100$} \\
% \cline{2-13}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.CvM}} & \multicolumn{1}{l|}{\textbf{MDE.LS}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.X2}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
%     \hline
\resizebox{1.3\textwidth}{!}{
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.CvM}} & \multicolumn{1}{l|}{\textbf{MDE.SD}} & \multicolumn{1}{l|}{\textbf{MDE.$\chi^2$}} & \multicolumn{1}{l|}{\textbf{MDE.TV}} &\multicolumn{1}{l|}{\textbf{MDE.KL}} & \multicolumn{1}{l|}{\textbf{MME}} \\
\cline{2-11}
  \multicolumn{11}{c}{$\beta=1.1,  \sigma=0.5$ $n=100$}\\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.2104&1.1144&1.4644&1.2224&1.1583&0.6222&0.764&1.2104&2.4114%&2.1242&1.4644
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.5882&0.51&0.7944&0.5937&0.5512&0.7796&0.9259&0.5882&2.7967%&2.4538&0.7944
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.0937&0.0621&0.0849&0.1495&0.1203&0.101&0.9553&0.0938&0.1611%&0.5555&0.0849
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.0569&0.036&0.0631&0.0791&0.0636&0.1476&1.0126&0.0569&0.807%&1.293&0.0631
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1104&0.0144&0.3644&0.1224&0.0583&-0.4778&-0.336&0.1104&1.3114%&1.0242&0.3644
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.0882&0.01&0.2944&0.0937&0.0512&0.2796&0.4259&0.0882&2.2967%&1.9538&0.2944
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1059&0.0623&0.2176&0.1645&0.1237&0.3293&1.0681&0.1059&1.881%&1.6044&0.2176
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.0647&0.0361&0.1498&0.0878&0.0662&0.2257&1.1939&0.0647&6.0818%&5.1102&0.1498
\\
\hline
\multicolumn{2}{|c|}{Accuracy } & 0.1706&0.0984&0.3674&0.2523&0.1899&0.555&2.262&0.1706&7.9628%&6.7146&0.3674
\\
\hline
% \multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.0011&0.0014&0.0012&0.0012&0.0546&0.0469&0.0011&0.0225&NaN&0.0014\\
% \hline
% \end{tabular}
% }
% \end{table}
% % START DATE AND TIME=20220517-11h19m32s
%       \begin{table}[htbp]
%   \centering
%   \caption{$\beta=1.5,  \sigma=0.5$ $n=100$}
%   \resizebox{\columnwidth}{!}{
%     \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|r|r|}
%       %\cline{2-13}    \multicolumn{1}{r|}{} &       & \multicolumn{11}{c|}{$\beta=1.5,  \sigma=0.5$ $n=100$} \\
% \cline{2-13}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.CvM}} & \multicolumn{1}{l|}{\textbf{MDE.LS}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.X2}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
%     \hline
  \multicolumn{11}{c}{$\beta=1.5,  \sigma=0.5$ $n=100$}\\
\hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.7252&1.518&1.8665&1.7245&1.6062&1.0512&1.3026&1.7251&2.832%&1.7864&1.8665
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.6284&0.5171&0.6927&0.6234&0.5696&0.7898&0.95&0.6284&1.575%&0.9581&0.6927
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.8391&2.7204&0.4115&0.5383&0.4377&9.325&9.1924&2.7971&4.2551%&39.7078&0.4115
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.7682&0.7355&0.1109&0.1296&0.1068&5.5659&6.5195&0.7568&1.2238%&11.2554&0.1109
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.2252&0.018&0.3665&0.2245&0.1062&-0.4488&-0.1974&0.2251&1.332%&0.2864&0.3665
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.1284&0.0171&0.1927&0.1234&0.0696&0.2898&0.45&0.1284&1.075%&0.4581&0.1927
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.8895&2.7205&0.5459&0.5887&0.4489&9.5255&9.2305&2.8475&6.0288%&39.7859&0.5459
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.7846&0.7357&0.148&0.1448&0.1117&5.6494&6.7213&0.7732&2.3794%&11.4641&0.148
\\
\hline
\multicolumn{2}{|c|}{Accuracy } & 3.6742&3.4562&0.6938&0.7335&0.5605&15.1748&15.9518&3.6208&8.4082%&51.25&0.6938
\\
\hline
% \multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0011&0.001&0.0011&0.0012&0.0011&0.0405&0.0332&0.0011&0.0092&NaN&0.0011\\
% \hline
% \end{tabular}
% }
% \end{table}
% % START DATE AND TIME=20220517-11h19m32s
%       \begin{table}[htbp]
%   \centering
%   \caption{$\beta=2,  \sigma=0.5$ $n=100$}
%   \resizebox{\columnwidth}{!}{
%     \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|r|r|}
%       %\cline{2-13}    \multicolumn{1}{r|}{} &       & \multicolumn{11}{c|}{$\beta=2,  \sigma=0.5$ $n=100$} \\
% \cline{2-13}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.CvM}} & \multicolumn{1}{l|}{\textbf{MDE.LS}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.X2}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
  \multicolumn{11}{c}{$\beta=2,  \sigma=0.5$ $n=100$}\\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.4522&2.0398&2.531&2.3562&2.1546&1.8227&2.6369&2.4522&3.5801%&-0.4069&2.531
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.6818&0.5276&0.6998&0.6474&0.5815&0.9232&1.3149&0.6818&1.2076%&-0.3344&0.6998
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.1598&1.9502&4.3536&4.6029&4.3387&23.4131&78.1332&2.1602&3.2804%&1082.6082&4.3536
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.2564&0.2263&0.5957&0.6271&0.5972&7.3001&24.9992&0.2566&0.3962%&170.9233&0.5957
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.4522&0.0398&0.531&0.3562&0.1546&-0.1773&0.6369&0.4522&1.5801%&-2.4069&0.531
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.1818&0.0276&0.1998&0.1474&0.0815&0.4232&0.8149&0.1818&0.7076%&-0.8344&0.1998
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.3641&1.9516&4.6352&4.7293&4.3622&23.4422&78.531&2.3644&5.7769%&1088.293&4.6352
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.2894&0.227&0.6355&0.6488&0.6038&7.4784&25.6607&0.2896&0.8969%&171.6024&0.6355
\\
\hline
\multicolumn{2}{|c|}{Accuracy } & 2.6535&2.1786&5.2707&5.378&4.966&30.9206&104.1918&2.654&6.6738%&1259.8955&5.2707
\\
\hline
% \multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0012&0.0011&0.0011&0.0012&0.0012&0.03&0.0236&0.0012&0.0036&NaN&0.0011\\
% \hline
% \end{tabular}
% }
% \end{table}
% % START DATE AND TIME=20220517-11h19m32s
%       \begin{table}[htbp]
%   \centering
%   \caption{$\beta=2.1,  \sigma=0.5$ $n=100$}
%   \resizebox{\columnwidth}{!}{
%     \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|r|r|}
%       %\cline{2-13}    \multicolumn{1}{r|}{} &       & \multicolumn{11}{c|}{$\beta=2.1,  \sigma=0.5$ $n=100$} \\
% \cline{2-13}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.CvM}} & \multicolumn{1}{l|}{\textbf{MDE.LS}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.X2}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
  \multicolumn{11}{c}{$\beta=2.1,  \sigma=0.5$ $n=100$}\\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.673&2.2248&2.6774&2.5137&2.2725&2.0937&2.9983&2.6478&3.8262%&-2.5887&2.6774
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.7199&0.5615&0.7084&0.6627&0.5875&0.9908&1.3874&0.7095&1.216%&-1.1034&0.7084
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 22.5683&22.4489&4.0274&7.3758&4.0219&42.4843&106.5311&7.9549&29.9248%&28264.571&4.0274
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
3.4961&3.4804&0.4541&0.8276&0.4542&9.3422&25.1345&1.0319&4.5985%&3881.4089&0.4541
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.573&0.1248&0.5774&0.4137&0.1725&-0.0063&0.8983&0.5478&1.7262%&-4.6887&0.5774
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.2199&0.0615&0.2084&0.1627&0.0875&0.4908&0.8874&0.2095&0.716%&-1.6034&0.2084
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 22.8944&22.4622&4.3604&7.5462&4.0513&42.4801&107.3274&8.2543&32.9016%&28283.7284&4.3604
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
3.5441&3.4838&0.4975&0.854&0.4618&9.5821&25.9195&1.0757&5.1107%&3883.5917&0.4975
\\
\hline
\multicolumn{2}{|c|}{Accuracy } & 26.4385&25.946&4.8578&8.4002&4.5131&52.0622&133.2468&9.33&38.0123%&32167.3202&4.8578
\\
\hline
% \multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0012&0.0011&0.0011&0.0012&0.0012&0.0289&0.0227&0.0012&0.0033&NaN&0.0011\\
% \hline
\end{tabular}
}
\end{table}

==> Tables20220525/output/output20220520/n200sig05.tex <==
% START DATE AND TIME=20220517-11h19m42s
      \begin{table}[htbp]
  \centering
%   \caption{$\beta=1.1,  \sigma=0.5$ $n=200$}
\caption{Comparison of different estimation methods for different values of $\beta$ ($\sigma=0.5$ and $n=200$). \label{tbl:n200sig05}}
%   \resizebox{\columnwidth}{!}{
%     \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|r|r|}
%       %\cline{2-13}    \multicolumn{1}{r|}{} &       & \multicolumn{11}{c|}{$\beta=1.1,  \sigma=0.5$ $n=200$} \\
% \cline{2-13}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.CvM}} & \multicolumn{1}{l|}{\textbf{MDE.LS}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.X2}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
%     \hline
\resizebox{1.3\textwidth}{!}{
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.CvM}} & \multicolumn{1}{l|}{\textbf{MDE.SD}} & \multicolumn{1}{l|}{\textbf{MDE.$\chi^2$}} & \multicolumn{1}{l|}{\textbf{MDE.TV}} &\multicolumn{1}{l|}{\textbf{MDE.KL}} & \multicolumn{1}{l|}{\textbf{MME}} \\
\cline{2-11}
  \multicolumn{11}{c}{$\beta=1.1,  \sigma=0.5$ $n=200$}\\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.1492&1.1081&1.361&1.1646&1.1357&0.5474&0.6441&1.1492&2.2303%&2.1242&1.361
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.5403&0.5071&0.7147&0.5498&0.5308&0.626&0.7052&0.5403&2.9018%&2.7444&0.7147
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.0341&0.0289&0.0371&0.0676&0.0611&0.0307&0.0509&0.0341&0.0416%&0.0505&0.0371
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.0204&0.017&0.0282&0.0344&0.0312&0.0325&0.0545&0.0204&1.4283%&1.4141&0.0282
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.0492&0.0081&0.261&0.0646&0.0357&-0.5526&-0.4559&0.0492&1.1303%&1.0242&0.261
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.0403&0.0071&0.2147&0.0498&0.0308&0.126&0.2052&0.0403&2.4018%&2.2444&0.2147
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.0365&0.0289&0.1052&0.0717&0.0624&0.3361&0.2587&0.0365&1.3192%&1.0994&0.1052
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.0221&0.017&0.0743&0.0369&0.0321&0.0484&0.0966&0.0221&7.1968%&6.4512&0.0743
\\
\hline
\multicolumn{2}{|c|}{Accuracy } & 0.0586&0.0459&0.1796&0.1087&0.0945&0.3845&0.3553&0.0586&8.516%&7.5506&0.1796
\\
 \hline
% \multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 6e-04&6e-04&8e-04&6e-04&6e-04&0.0514&0.0435&6e-04&0.028&NaN&8e-04\\
% \hline
% \end{tabular}
% }
% \end{table}
% % START DATE AND TIME=20220517-11h19m42s
%       \begin{table}[htbp]
%   \centering
%   \caption{$\beta=1.5,  \sigma=0.5$ $n=200$}
%   \resizebox{\columnwidth}{!}{
%     \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|r|r|}
%       %\cline{2-13}    \multicolumn{1}{r|}{} &       & \multicolumn{11}{c|}{$\beta=1.5,  \sigma=0.5$ $n=200$} \\
% \cline{2-13}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.CvM}} & \multicolumn{1}{l|}{\textbf{MDE.LS}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.X2}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
%     \hline
  \multicolumn{11}{c}{$\beta=1.5,  \sigma=0.5$ $n=200$}\\
  \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.6251&1.5367&1.741&1.675&1.6192&0.8826&1.0444&1.6251&2.5184%&2.3039&1.741
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.5721&0.5251&0.6273&0.5932&0.5682&0.5861&0.6536&0.5721&1.3828%&1.2359&0.6273
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1068&0.0797&0.1199&0.1818&0.1571&0.1382&0.187&0.1068&0.1773%&0.228&0.1199
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.0275&0.0201&0.0323&0.0421&0.0365&0.0652&0.0819&0.0275&0.144%&0.1662&0.0323
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1251&0.0367&0.241&0.175&0.1192&-0.6174&-0.4556&0.1251&1.0184%&0.8039&0.241
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.0721&0.0251&0.1273&0.0932&0.0682&0.0861&0.1536&0.0721&0.8828%&0.7359&0.1273
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1224&0.0811&0.178&0.2124&0.1713&0.5194&0.3946&0.1224&1.2144%&0.8743&0.178
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.0326&0.0207&0.0485&0.0508&0.0411&0.0726&0.1055&0.0326&0.9233%&0.7078&0.0485
\\
\hline
\multicolumn{2}{|c|}{Accuracy } & 0.1551&0.1017&0.2265&0.2633&0.2124&0.5919&0.5001&0.1551&2.1377%&1.5821&0.2265
\\
% \hline
% \multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 5e-04&5e-04&6e-04&6e-04&6e-04&0.0337&0.0262&5e-04&0.0085&NaN&6e-04\\
% \hline
% \end{tabular}
% }
% \end{table}
% % START DATE AND TIME=20220517-11h19m42s
%       \begin{table}[htbp]
%   \centering
%   \caption{$\beta=2,  \sigma=0.5$ $n=200$}
%   \resizebox{\columnwidth}{!}{
%     \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|r|r|}
%       %\cline{2-13}    \multicolumn{1}{r|}{} &       & \multicolumn{11}{c|}{$\beta=2,  \sigma=0.5$ $n=200$} \\
% \cline{2-13}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.CvM}} & \multicolumn{1}{l|}{\textbf{MDE.LS}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.X2}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
     \hline
  \multicolumn{11}{c}{$\beta=2,  \sigma=0.5$ $n=200$}\\
  \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.3414&2.1301&2.4109&2.3392&2.2355&1.5339&1.7854&2.3414&3.163%&2.5375&2.4109
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.6346&0.5567&0.6539&0.6319&0.5984&0.6833&0.7453&0.6346&1.0155%&0.7683&0.6539
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.3817&0.2262&0.3354&0.5006&0.4038&1.371&3.1955&0.3817&0.6528%&2.8809&0.3354
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.0481&0.0277&0.042&0.0597&0.0484&0.3548&0.8499&0.0481&0.0869%&0.4015&0.042
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.3414&0.1301&0.4109&0.3392&0.2355&-0.4661&-0.2146&0.3414&1.163%&0.5375&0.4109
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.1346&0.0567&0.1539&0.1319&0.0984&0.1833&0.2453&0.1346&0.5155%&0.2683&0.1539
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.4982&0.2431&0.5043&0.6157&0.4592&1.5881&3.2412&0.4982&2.0053%&3.1695&0.5043
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.0662&0.0309&0.0657&0.0771&0.0581&0.3884&0.91&0.0662&0.3527%&0.4735&0.0657
\\
\hline
\multicolumn{2}{|c|}{Accuracy } & 0.5644&0.274&0.57&0.6927&0.5173&1.9765&4.1512&0.5644&2.3579%&3.643&0.57
\\
\hline
% \multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 6e-04&5e-04&6e-04&6e-04&6e-04&0.0218&0.0157&6e-04&0.0022&NaN&6e-04\\
% \hline
% \end{tabular}
% }
% \end{table}
% % START DATE AND TIME=20220517-11h19m42s
%       \begin{table}[htbp]
%   \centering
%   \caption{$\beta=2.1,  \sigma=0.5$ $n=200$}
%   \resizebox{\columnwidth}{!}{
%     \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|r|r|}
%       %\cline{2-13}    \multicolumn{1}{r|}{} &       & \multicolumn{11}{c|}{$\beta=2.1,  \sigma=0.5$ $n=200$} \\
% \cline{2-13}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.CvM}} & \multicolumn{1}{l|}{\textbf{MDE.LS}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.X2}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
%     \hline
  \multicolumn{11}{c}{$\beta=2.1,  \sigma=0.5$ $n=200$}\\
  \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.4926&2.2446&2.5527&2.484&2.3676&1.6739&1.9476&2.4926&3.3137%&2.4699&2.5527
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.6455&0.5596&0.6604&0.6409&0.6054&0.7002&0.7648&0.6456&0.994%&0.6865&0.6604
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.4556&0.2483&0.3928&0.6001&0.4757&0.8421&3.199&0.4556&0.7531%&35.6634&0.3928
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.0511&0.0273&0.0437&0.0645&0.0514&0.1763&1.054&0.0511&0.0871%&4.1686&0.0437
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.3926&0.1446&0.4527&0.384&0.2676&-0.4261&-0.1524&0.3926&1.2137%&0.3699&0.4527
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.1455&0.0596&0.1604&0.1409&0.1054&0.2002&0.2648&0.1456&0.494%&0.1865&0.1604
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.6097&0.2692&0.5977&0.7475&0.5473&1.0236&3.2219&0.6097&2.226%&35.7967&0.5977
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.0723&0.0309&0.0694&0.0844&0.0626&0.2164&1.124&0.0723&0.3312%&4.203&0.0694
\\
\hline
\multicolumn{2}{|c|}{Accuracy } & 0.682&0.3001&0.6672&0.8318&0.6098&1.24&4.3459&0.682&2.5571%&39.9997&0.6672
\\
% \hline
% \multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 6e-04&5e-04&6e-04&6e-04&6e-04&0.0205&0.0146&6e-04&0.0019&NaN&6e-04\\
\hline
\end{tabular}
}
\end{table}

==> Tables20220525/output/output20220520/n30sig1.tex <==
% START DATE AND TIME=20220517-11h18m15s
      \begin{table}[htbp]
  \centering
%   \caption{$\beta=1.1,  \sigma=1$ $n=30$}
\caption{Comparison of different estimation methods for different values of $\beta$ ($\sigma=1$ and $n=30$). \label{tbl:n30sig1}}
%   \resizebox{\columnwidth}{!}{
%     \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|r|r|}
%       %\cline{2-13}    \multicolumn{1}{r|}{} &       & \multicolumn{11}{c|}{$\beta=1.1,  \sigma=1$ $n=30$} \\
% \cline{2-13}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.CvM}} & \multicolumn{1}{l|}{\textbf{MDE.LS}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.X2}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
\resizebox{1.3\textwidth}{!}{
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.CvM}} & \multicolumn{1}{l|}{\textbf{MDE.SD}} & \multicolumn{1}{l|}{\textbf{MDE.$\chi^2$}} & \multicolumn{1}{l|}{\textbf{MDE.TV}} &\multicolumn{1}{l|}{\textbf{MDE.KL}} & \multicolumn{1}{l|}{\textbf{MME}} \\
\cline{2-11}
  \multicolumn{11}{c}{$\beta=1.1,  \sigma=1$ $n=30$}\\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.5476&1.2726&1.7559&1.2913&1.0669&1.5509&4.1037&1.533&3.4594%&-5.9574&1.7559
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
1.6955&1.2439&1.9754&1.2957&0.9948&5.9319&12.7978&1.6637&7.0156%&-15.0766&1.9754
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 11.3504&11.4836&1.1517&1.3721&0.9943&123.0776&284.9745&5.5924&31.4146%&72560.1429&1.1517
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
43.4201&43.6817&3.5183&3.9974&2.9891&795.4071&2994.4695&16.2858&113.5301%&669734.8812&3.5183
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.4476&0.1726&0.6559&0.1913&-0.0331&0.4509&3.0037&0.433&2.3594%&-7.0574&0.6559
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.6955&0.2439&0.9754&0.2957&-0.0052&4.9319&11.7978&0.6637&6.0156%&-16.0766&0.9754
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 11.5496&11.5122&1.5817&1.4086&0.9953&123.2687&293.9685&5.7793&36.9783%&72602.6931&1.5817
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
43.8995&43.7368&4.4693&4.0845&2.9888&819.6511&3133.3572&16.7247&149.706%&669926.3641&4.4693
\\
\hline
\multicolumn{2}{|c|}{Accuracy} & 55.449&55.249&6.051&5.493&3.984&942.9198&3427.3257&22.504&186.6843%&742529.0573&6.051
\\
% \hline
% \multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0035&0.0042&0.0038&0.0036&0.0036&6.82246116457383e+300&0.0526&0.0035&0.0178%&NaN&0.0038
% \\
\hline
% \end{tabular}
% }
% \end{table}
% % START DATE AND TIME=20220517-11h18m15s
%       \begin{table}[htbp]
%   \centering
%   \caption{$\beta=1.5,  \sigma=1$ $n=30$}
%   \resizebox{\columnwidth}{!}{
%     \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|r|r|}
%       %\cline{2-13}    \multicolumn{1}{r|}{} &       & \multicolumn{11}{c|}{$\beta=1.5,  \sigma=1$ $n=30$} \\
% \cline{2-13}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.CvM}} & \multicolumn{1}{l|}{\textbf{MDE.LS}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.X2}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
 \multicolumn{11}{c}{$\beta=1.5,  \sigma=1$ $n=30$}\\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.8331&2.5506&2.1876&1.7125&1.3796&4.1668&9.1831&2.4101&5.2836%&-14.9536&2.1876
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
2.4327&2.13&1.6816&1.2511&0.9471&8.0571&18.0677&1.9777&5.9445%&-19.1697&1.6816
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 537.7961&538.6079&8.8244&9.2019&8.4143&309.924&796.1032&44.5747&767.6051%&459310.533&8.8244
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
738.8522&739.722&9.1242&9.6195&8.8048&1114.0289&3334.0138&51.3856&943.0195%&813088.4194&9.1242
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.3331&1.0506&0.6876&0.2125&-0.1204&2.6668&7.6831&0.9101&3.7836%&-16.4536&0.6876
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
1.4327&1.13&0.6816&0.2511&-0.0529&7.0571&17.0677&0.9777&4.9445%&-20.1697&0.6816
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 539.5195&539.6578&9.2963&9.2461&8.4279&317.0051&855.053&45.3985&781.8436%&459535.3235&9.2963
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
740.8309&740.9249&9.588&9.6816&8.8067&1163.7205&3624.9879&52.3363&967.3733%&813413.9272&9.588
\\
\hline
\multicolumn{2}{|c|}{Accuracy} & 1280.3504&1280.5828&18.8843&18.9277&17.2346&1480.7256&4480.0409&97.7348&1749.217%&1272949.2507&18.8843
\\
% \hline
% \multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0034&0.0043&0.0034&0.0035&0.0036&2.28475770806158e+299&0.0454&0.0034&0.0109%&NaN&0.0034
% \\
\hline
% \end{tabular}
% }
% \end{table}
% % START DATE AND TIME=20220517-11h18m15s
%       \begin{table}[htbp]
%   \centering
%   \caption{$\beta=2,  \sigma=1$ $n=30$}
%   \resizebox{\columnwidth}{!}{
%     \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|r|r|}
%       %\cline{2-13}    \multicolumn{1}{r|}{} &       & \multicolumn{11}{c|}{$\beta=2,  \sigma=1$ $n=30$} \\
% \cline{2-13}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.CvM}} & \multicolumn{1}{l|}{\textbf{MDE.LS}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.X2}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
%     \hline
 \multicolumn{11}{c}{$\beta=2,  \sigma=1$ $n=30$}\\
\hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 3.4344&3.1834&2.6276&2.1444&1.7162&5.8848&13.8046&3.1405&6.3004%&-11.5785&2.6276
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
2.1379&1.9548&1.456&1.1598&0.8834&8.2224&19.0806&1.9323&4.7337%&-10.1073&1.456
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 276.7184&277.7227&22.2422&23.5306&22.1061&458.0391&1270.0878&66.7231&576.623%&40259.0504&22.2422
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
141.0373&141.5665&11.0524&11.4991&10.8802&979.6179&2633.8056&39.3883&338.1092%&23157.567&11.0524
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.4344&1.1834&0.6276&0.1444&-0.2838&3.8848&11.8046&1.1405&4.3004%&-13.5785&0.6276
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
1.1379&0.9548&0.456&0.1598&-0.1166&7.2224&18.0806&0.9323&3.7337%&-11.1073&0.456
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 278.7483&279.0954&22.6338&23.5491&22.1845&473.0849&1409.3091&68.0171&595.0591%&40439.4013&22.6338
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
142.318&142.464&11.2592&11.5235&10.8927&1031.683&2960.4518&40.2535&352.016%&23278.6232&11.2592
\\
\hline
\multicolumn{2}{|c|}{Accuracy} & 421.0663&421.5594&33.893&35.0727&33.0772&1504.768&4369.7609&108.2706&947.0751%&63718.0245&33.893
\\
\hline
% \multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0032&0.0043&0.003&0.0034&0.0036&0.0464&0.04&0.0032&0.0073&NaN&0.003\\
% \hline
% \end{tabular}
% }
% \end{table}
% % START DATE AND TIME=20220517-11h18m15s
%       \begin{table}[htbp]
%   \centering
%   \caption{$\beta=2.1,  \sigma=1$ $n=30$}
%   \resizebox{\columnwidth}{!}{
%     \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|r|r|}
%       %\cline{2-13}    \multicolumn{1}{r|}{} &       & \multicolumn{11}{c|}{$\beta=2.1,  \sigma=1$ $n=30$} \\
% \cline{2-13}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.CvM}} & \multicolumn{1}{l|}{\textbf{MDE.LS}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.X2}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
 \multicolumn{11}{c}{$\beta=2.1,  \sigma=1$ $n=30$}\\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 9.6554&9.4144&2.6477&2.1479&1.6945&6.2325&15.4106&3.3185&15.4483%&-2.8909&2.6477
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
6.3885&6.2219&1.3824&1.0907&0.8145&8.0983&20.1261&1.9497&10.8971%&-4.0719&1.3824
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 365388.6874&365392.647&13.8781&15.9321&13.6836&488.1136&1437.3828&70.9096&742413.8126%&767434.0704&13.8781
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
177005.1682&177007.0778&5.9903&6.4848&5.7064&885.1725&2682.0175&37.7575&359896.2062%&382117.3051&5.9903
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 7.5554&7.3144&0.5477&0.0479&-0.4055&4.1325&13.3106&1.2185&13.3483%&-4.9909&0.5477
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
5.3885&5.2219&0.3824&0.0907&-0.1855&7.0983&19.1261&0.9497&9.8971%&-5.0719&0.3824
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 365409.2329&365409.6079&14.1767&15.9328&13.8467&505.1421&1614.4118&72.3873&742517.7483%&767382.2363&14.1767
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
177016.504&177016.6452&6.1359&6.4924&5.7402&935.4699&3047.5561&38.6556&359958.1691%&382104.8175&6.1359
\\
\hline
\multicolumn{2}{|c|}{Accuracy } & 542425.737&542426.2531&20.3126&22.4252&19.5869&1440.6121&4661.9679&111.0429&1102475.9173%&1149487.0538&20.3126
\\
% \hline
% \multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0032&0.0042&0.0029&0.0033&0.0036&0.046&0.0397&0.0032&0.0069%&NaN&0.0029\\
\hline
\end{tabular}
}
\end{table}

==> Tables20220525/output/output20220520/n30sig2.tex <==
% START DATE AND TIME=20220519-10h55m12s
\begin{table}[htbp]
  \centering
  \caption{Comparison of different estimation methods for different values of $\beta$ ($\sigma=2$ and $n=30$). \label{tbl:n30sig2}}
\resizebox{1.3\textwidth}{!}{
%     \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|r|r|}
%       %\cline{2-13}    \multicolumn{1}{r|}{} &       & \multicolumn{11}{c|}{$\beta=1.1,  \sigma=2$ $n=30$} \\
% \cline{2-13}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.CvM}} & \multicolumn{1}{l|}{\textbf{MDE.LS}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.X2}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
%     \hline
      \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.CvM}} & \multicolumn{1}{l|}{\textbf{MDE.SD}} & \multicolumn{1}{l|}{\textbf{MDE.$\chi^2$}} & \multicolumn{1}{l|}{\textbf{MDE.TV}} &\multicolumn{1}{l|}{\textbf{MDE.KL}} & \multicolumn{1}{l|}{\textbf{MME}} \\
\cline{2-11}
  \multicolumn{11}{c}{$\beta=2.1,  \sigma=2$ $n=30$}\\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.7987&1.512&1.7401&1.3427&1.1135&-1.6633&3.0483&1.6001&3.636%&-1.3929&1.7401
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
3.8588&3.0454&3.3854&2.466&1.9066&9.1863&15.9833&3.1893&54.036%&34.3719&3.3854
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 160.0243&160.3052&1.838&2.5208&1.7722&498.3215&172.4203&16.417&239.0424%&807.0952&1.838
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
1765.3744&1767.7238&23.0907&31.9671&22.7828&1958.5497&5046.1827&174.1169&16777095.9217%&14350843.71&23.0907
\\
\hline
%\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.6987&0.412&0.6401&0.2427&0.0135&-2.7633&1.9483&0.5001&2.536%&-2.4929&0.6401
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 63.5182&37.4545&58.1909&22.0636&1.2273&-251.2091&177.1182&45.4636&230.5455%&-2.4929&0.6401
\\
%\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
%1.8588&1.0454&1.3854&0.466&-0.0934&7.1863&13.9833&1.1893&52.036%&32.3719&1.3854
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
92.94&52.27&69.27&23.3&-4.67&359.315&699.165&59.465&2601.8%&32.3719&1.3854
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 160.4966&160.4589&2.2475&2.5795&1.7722&505.9077&176.1988&16.6654&245.4497%&813.2289&2.2475
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
1768.6528&1768.6398&25.0076&32.1811&22.7893&2009.9973&5241.2101&175.5139&16778125.9621%&14350456.5675&25.0076
\\
\hline
\multicolumn{2}{|c|}{Accuracy} & 1929.1494&1929.0987&27.2551&34.7606&24.5615&2515.905&5417.4089&192.1793&16778371.4118%&14351269.7963&27.2551\\
\\
\hline
  \multicolumn{11}{c}{$\beta=1.5,  \sigma=2$ $n=30$}\\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.4901&2.1904&2.0696&1.6011&1.2928&2.5147&6.8422&2.1075%&4.7683&-4.0642&2.0696
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
3.7605&3.1454&2.9696&2.1819&1.6477&10.8446&24.9727&3.1457&10.1186%&-10.6768&2.9696
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 676.4235&677.077&4.3208&5.1165&4.1411&221.6163&508.585&24.9565&1262.0699%&4183.0383&4.3208
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
1459.9615&1462.2551&16.5047&20.0532&15.751&2155.1416&7167.5418&99.245&2823.5225%&25288.728&16.5047
\\
\hline
%\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.9901&0.6904&0.5696&0.1011&-0.2072&1.0147&5.3422&0.6075&3.2683%&-5.5642&0.5696
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 66.0067&46.0267&37.97336&6.74&-13.8133&67.6467&356.1467&40.5&217.8867%&-5.5642&0.5696
\\
%\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
%1.7605&1.1454&0.9696&0.1819&-0.3523&8.8446&22.9727&1.1457&8.1186%&-12.6768&0.9696
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
88.025&57.27&48.48&9.095&-17.615&442.23&1148.635&57.285&405.93%&-12.6768&0.9696
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 677.3361&677.4859&4.6448&5.1262&4.1836&222.6237&537.0733&25.3231&1272.6254%&4213.5804&4.6448
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
1462.9148&1463.4209&17.4432&20.0843&15.8735&2233.1523&7694.5721&100.5476&2889.1524%&25446.901&17.4432
\\
\hline
\multicolumn{2}{|c|}{Accuracy} & 2140.2509&2140.9068&22.088&25.2105&20.0572&2455.776&8231.6454&125.8707&4161.7777%&29660.4814&22.088\\
\\
\hline
  \multicolumn{11}{c}{$\beta=2,  \sigma=2$ $n=30$}\\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 3.5985&3.3375&2.5409&2.0315&1.5923&5.4862&12.9728&3.0757&6.5573%&-11.3198&2.5409
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
4.2896&3.9212&2.6719&2.0958&1.5553&13.7122&32.4026&3.524&9.3146%&-18.902&2.6719
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 582.0675&583.1951&9.484&10.7491&9.1678&376.4655&1074.9486&54.9588&1131.4863%&64850.0259&9.484
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
1195.9372&1198.1041&22.9949&25.5117&22.4334&2377.2184&7185.6666&119.9379&2474.2323%&125188.8812&22.9949
\\
\hline
%\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.5985&1.3375&0.5409&0.0315&-0.4077&3.4862&10.9728&1.0757&4.5573%&-13.3198&0.5409
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 79.925&66.875&27.045&1.575&-20.385&174.31&548.64&53.785&227.865%&-13.3198&0.5409
\\
%\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
%2.2896&1.9212&0.6719&0.0958&-0.4447&11.7122&30.4026&1.524&7.3146%&-20.902&0.6719
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
114.48&96.06&33.595&4.79&-22.235&585.61&1520.13&76.2&365.73%&-20.902&0.6719
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 584.5646&584.9257&9.7756&10.749&9.3331&388.5811&1195.2431&56.1105&1152.1424%&65020.9568&9.7756
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
1201.06&1201.6751&23.4441&25.5183&22.6289&2514.1573&8109.2662&122.2484&2527.4878%&125613.2556&23.4441
\\
\hline
\multicolumn{2}{|c|}{Accuracy} & 1785.6246&1786.6008&33.2197&36.2673&31.962&2902.7384&9304.5093&178.3589&3679.6302%&190634.2123&33.2197
\\
\hline
  \multicolumn{11}{c}{$\beta=2.1,  \sigma=2$ $n=30$}\\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 190.3827&190.1359&2.6848&2.1794&1.7069&6.2166&14.4035&3.3928&234.2205%&207.4698&2.6848
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
307.25&306.9266&2.6748&2.1499&1.5989&14.4706&33.6177&3.6912&378.2798%&343.2558&2.6748
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 347663582.8526&347663676.1193&11.6001&12.9381&11.3367&448.5575&1203.4724&71.6477&516949623.7701%&517478254.8612&11.6001
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
917857063.1782&917857261.1597&21.6604&24.0655&21.2499&2545.5761&6995.7748&127.7713&1364784801.6468%&1365233776.7568&21.6604
\\
\hline
%\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 188.2827&188.0359&0.5848&0.0794&-0.3931&4.1166&12.3035&1.2928&232.1205%&205.3698&0.5848
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 8965.8429&8954.0905&27.8476&3.7810&-18.7190&196.0286&585.8810&61.5619&11053.3571%&205.3698&0.5848
\\
%\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
%305.25&304.9266&0.6748&0.1499&-0.4011&12.4706&31.6177&1.6912&376.2798%&341.2558&0.6748
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
15262.5&15246.33&33.74&7.495&-20.055&623.53&1580.885&84.56&18813.99%&341.2558&0.6748
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 347664266.8537&347664267.2401&11.941&12.9432&11.4901&465.4593&1354.7283&73.3117&516951808.7525%&517468683.7706&11.941
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
917858455.0599&917858455.647&22.1136&24.0856&21.4086&2700.8372&7994.7561&130.6186&1364789909.6253%&1365213708.8973&22.1136
\\
\hline
\multicolumn{2}{|c|}{Accuracy} & 1265522721.9136&1265522722.8871&34.0545&37.0287&32.8987&3166.2966&9349.4844&203.9303&1881741718.3778%&1882682392.668&34.0545
\\
\hline
\end{tabular}
}
\end{table}


==> Tables20220525/output/output20220520/n500sig05.tex <==
% START DATE AND TIME=20220518-13h04m11s
      \begin{table}[htbp]
  \centering
%   \caption{$\beta=1.1,  \sigma=0.5$ $n=500$}
\caption{Comparison of different estimation methods for different values of $\beta$ ($\sigma=0.5$ and $n=500$). \label{tbl:n500sig05}}
%   \resizebox{\columnwidth}{!}{
%     \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|r|r|}
%       %\cline{2-13}    \multicolumn{1}{r|}{} &       & \multicolumn{11}{c|}{$\beta=1.1,  \sigma=0.5$ $n=500$} \\
% \cline{2-13}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.CvM}} & \multicolumn{1}{l|}{\textbf{MDE.LS}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.X2}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
%     \hline
\resizebox{1.3\textwidth}{!}{
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.CvM}} & \multicolumn{1}{l|}{\textbf{MDE.SD}} & \multicolumn{1}{l|}{\textbf{MDE.$\chi^2$}} & \multicolumn{1}{l|}{\textbf{MDE.TV}} &\multicolumn{1}{l|}{\textbf{MDE.KL}} & \multicolumn{1}{l|}{\textbf{MME}} \\
\cline{2-11}
  \multicolumn{11}{c}{$\beta=1.1,  \sigma=0.5$ $n=500$}\\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.1164&1.1012&1.2852&1.1225&1.1119&0.5774&0.6496&1.1164&2.1181%&2.0699&1.2852
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.5135&0.5013&0.6531&0.5173&0.5104&0.6374&0.676&0.5134&3.0482%&2.965&0.6531
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.0116&0.011&0.0168&0.0215&0.0207&0.0099&0.0165&0.0116&0.0107%&0.0132&0.0168
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.0068&0.0064&0.0121&0.0109&0.0106&0.0094&0.0139&0.0068&2.0185%&1.9965&0.0121
\\
\hline
%\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.0164&0.0012&0.1852&0.0225&0.0119&-0.5226&-0.4504&0.0164&1.0181&0.9699&0.1852
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.4909&0.1091&16.8364&2.0455&1.0818&-47.5091&-40.9455&1.4909&92.5545
\\
%\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
%0.0135&0.0013&0.1531&0.0173&0.0104&0.1374&0.176&0.0134&2.5482&2.465&0.1531
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
2.7&0.26&30.62&3.46&2.08&27.48&35.2&2.68&509.64
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.0119&0.011&0.0511&0.022&0.0209&0.283&0.2193&0.0119&1.0472%&0.9539&0.0511
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.007&0.0064&0.0355&0.0112&0.0107&0.0282&0.0448&0.007&8.5117%&8.0725&0.0355
\\
\hline
\multicolumn{2}{|c|}{Accuracy } & 0.0189&0.0173&0.0866&0.0332&0.0315&0.3112&0.2641&0.0189&9.5589%&9.0264&0.0866
\\
\hline
% \multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 2e-04&2e-04&4e-04&2e-04&2e-04&0.0446&0.0378&2e-04&0.0332&0.033&4e-04\\
% \hline
% \end{tabular}
% }
% \end{table}
% % START DATE AND TIME=20220518-13h04m11s
%       \begin{table}[htbp]
%   \centering
%   \caption{$\beta=1.5,  \sigma=0.5$ $n=500$}
%   \resizebox{\columnwidth}{!}{
%     \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|r|r|}
%       %\cline{2-13}    \multicolumn{1}{r|}{} &       & \multicolumn{11}{c|}{$\beta=1.5,  \sigma=0.5$ $n=500$} \\
% \cline{2-13}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.CvM}} & \multicolumn{1}{l|}{\textbf{MDE.LS}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.X2}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
  \multicolumn{11}{c}{$\beta=1.5,  \sigma=0.5$ $n=500$}\\
     \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.5517&1.5211&1.6311&1.5796&1.56&0.8658&0.9797&1.5517&2.3106%&2.2152&1.6311
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.5287&0.5127&0.5673&0.5407&0.5321&0.5161&0.5365&0.5287&1.2428%&1.1714&0.5673
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.03&0.0274&0.0468&0.056&0.0532&0.0541&0.062&0.03&0.051%&0.0634&0.0468
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.0076&0.0069&0.0124&0.0127&0.0121&0.0153&0.0153&0.0076&0.0977%&0.1003&0.0124
\\
\hline
%\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.0517&0.0211&0.1311&0.0796&0.06&-0.6342&-0.5203&0.0517&0.8106&0.7152&0.1311
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 
3.4467&1.4067&8.74&5.3067&4&-42.28&-34.6867&3.4467&54.04
\\
%\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
%0.0287&0.0127&0.0673&0.0407&0.0321&0.0161&0.0365&0.0287&0.7428&0.6714&0.0673
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
5.74&2.54&13.46&8.14&6.42&3.22&7.3&5.74&148.56
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.0327&0.0278&0.064&0.0624&0.0568&0.4562&0.3326&0.0327&0.708%&0.5748&0.064
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.0084&0.0071&0.0169&0.0143&0.0131&0.0156&0.0167&0.0084&0.6494%&0.551&0.0169
\\
\hline
\multicolumn{2}{|c|}{Accuracy } & 0.0411&0.0349&0.0809&0.0767&0.0699&0.4718&0.3493&0.0411&1.3574%&1.1258&0.0809
\\
\hline
% \multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 2e-04&2e-04&2e-04&2e-04&2e-04&0.026&0.019&2e-04&0.0074&0.0071&2e-04\\
% \hline
% \end{tabular}
% }
% \end{table}
% % START DATE AND TIME=20220518-13h04m11s
%       \begin{table}[htbp]
%   \centering
%   \caption{$\beta=2,  \sigma=0.5$ $n=500$}
%   \resizebox{\columnwidth}{!}{
%     \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|r|r|}
%       %\cline{2-13}    \multicolumn{1}{r|}{} &       & \multicolumn{11}{c|}{$\beta=2,  \sigma=0.5$ $n=500$} \\
% \cline{2-13}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.CvM}} & \multicolumn{1}{l|}{\textbf{MDE.LS}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.X2}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
  \multicolumn{11}{c}{$\beta=2,  \sigma=0.5$ $n=500$}\\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.148&2.084&2.2049&2.1705&2.1354&1.4127&1.5514&2.148&2.7557%&2.5973&2.2049
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.5575&0.5343&0.5752&0.564&0.553&0.5519&0.5491&0.5575&0.8431%&0.7759&0.5752
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.083&0.0713&0.0941&0.1212&0.1126&0.1733&0.156&0.083&0.16%&0.1891&0.0941
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.0099&0.0084&0.0112&0.0138&0.0128&0.0287&0.0233&0.0099&0.0214%&0.0278&0.0112
\\
\hline
%\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.148&0.084&0.2049&0.1705&0.1354&-0.5873&-0.4486&0.148&0.7557&0.5973&0.2049
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 
7.4&4.2&10.245&8.525&6.77&-29.365&-22.43&7.4&37.785
\\
%\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
%0.0575&0.0343&0.0752&0.064&0.053&0.0519&0.0491&0.0575&0.3431&0.2759&0.0752
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
11.5&6.86&15.04&12.8&10.6&10.38&9.82&11.5&68.62
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1049&0.0783&0.1361&0.1503&0.1309&0.5182&0.3573&0.1049&0.7311%&0.5459&0.1361
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.0132&0.0096&0.0169&0.0179&0.0157&0.0314&0.0257&0.0132&0.1391%&0.1039&0.0169
\\
\hline
\multicolumn{2}{|c|}{Accuracy } & 0.1181&0.0879&0.1529&0.1682&0.1465&0.5496&0.383&0.1181&0.8702%&0.6499&0.1529
\\
\hline
% \multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 2e-04&2e-04&2e-04&2e-04&2e-04&0.0146&0.009&2e-04&0.0013&0.0011&2e-04\\
% \hline
% \end{tabular}
% }
% \end{table}
% % START DATE AND TIME=20220518-13h04m11s
%       \begin{table}[htbp]
%   \centering
%   \caption{$\beta=2.1,  \sigma=0.5$ $n=500$}
%   \resizebox{\columnwidth}{!}{
%     \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|r|r|}
%       %\cline{2-13}    \multicolumn{1}{r|}{} &       & \multicolumn{11}{c|}{$\beta=2.1,  \sigma=0.5$ $n=500$} \\
% \cline{2-13}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.CvM}} & \multicolumn{1}{l|}{\textbf{MDE.LS}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.X2}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
%     \hline
  \multicolumn{11}{c}{$\beta=2,  \sigma=0.5$ $n=500$}\\
\hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.281&2.2073&2.335&2.2986&2.2597&1.5479&1.6853&2.281&2.8742%&2.6998&2.335
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.5664&0.5413&0.5821&0.5708&0.5593&0.5691&0.5604&0.5664&0.8206%&0.7523&0.5821
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1002&0.0846&0.1096&0.1389&0.1283&0.2164&0.1907&0.1002&0.1948%&0.2283&0.1096
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.0107&0.009&0.0117&0.0142&0.0131&0.0326&0.0262&0.0107&0.0237%&0.03&0.0117
\\
\hline
%\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.181&0.1073&0.235&0.1986&0.1597&-0.5521&-0.4147&0.181&0.7742&0.5998&0.235
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 
8.6190&5.1095&11.1905&9.4571&7.6048&-26.2905&-19.7476&8.6190&36.8667
\\
%\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
%0.0664&0.0413&0.0821&0.0708&0.0593&0.0691&0.0604&0.0664&0.3206&0.2523&0.0821
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
13.28&8.26&16.42&14.16&11.86&13.82&12.08&13.28&64.12
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1329&0.0961&0.1648&0.1784&0.1538&0.5213&0.3627&0.1329&0.7942%&0.5881&0.1648
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.0151&0.0107&0.0184&0.0192&0.0166&0.0373&0.0298&0.0151&0.1264%&0.0937&0.0184
\\
\hline
\multicolumn{2}{|c|}{Accuracy } & 0.1481&0.1068&0.1832&0.1976&0.1705&0.5586&0.3925&0.1481&0.9206%&0.6817&0.1832
\\
\hline
% \multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 2e-04&2e-04&2e-04&2e-04&2e-04&0.0134&0.0081&2e-04&0.0011&9e-04&2e-04\\
% \hline
\end{tabular}
}
\end{table}

==> Tables20220525/output/output20220520/n500sig1.tex <==
% START DATE AND TIME=20220518-13h02m59s
      \begin{table}[htbp]
  \centering
%   \caption{$\beta=1.1,  \sigma=1$ $n=500$}
\caption{Comparison of different estimation methods for different values of $\beta$ ($\sigma=1$ and $n=500$). \label{tbl:n500sig1}}
%   \resizebox{\columnwidth}{!}{
%     \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|r|r|}
%       %\cline{2-13}    \multicolumn{1}{r|}{} &       & \multicolumn{11}{c|}{$\beta=1.1,  \sigma=1$ $n=500$} \\
% \cline{2-13}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.CvM}} & \multicolumn{1}{l|}{\textbf{MDE.LS}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.X2}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
\resizebox{1.3\textwidth}{!}{
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.CvM}} & \multicolumn{1}{l|}{\textbf{MDE.SD}} & \multicolumn{1}{l|}{\textbf{MDE.$\chi^2$}} & \multicolumn{1}{l|}{\textbf{MDE.TV}} &\multicolumn{1}{l|}{\textbf{MDE.KL}} & \multicolumn{1}{l|}{\textbf{MME}} \\
\cline{2-11}
  \multicolumn{11}{c}{$\beta=1.1,  \sigma=1$ $n=500$}\\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.1154&1.1002&1.2872&1.1199&1.1093&0.5791&0.652&1.1154&2.1193%&2.0713&1.2872
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
1.0245&1.0002&1.3086&1.0304&1.0166&1.2738&1.3525&1.0245&5.9558%&5.7909&1.3086
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.0117&0.0111&0.0163&0.0217&0.021&0.0095&0.0157&0.0117&0.0106%&0.0132&0.0163
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.0278&0.0261&0.0472&0.0448&0.0432&0.0377&0.055&0.0278&6.0378%&5.9782&0.0472
\\
\hline
%\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.0154&2e-04&0.1872&0.0199&0.0093&-0.5209&-0.448&0.0154&1.0193&0.9713&0.1872
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 
1.4&0.0182&17.0182&1.8091&0.8455&-47.3545&-40.7273&1.4&92.6636
\\
%\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
%0.0245&2e-04&0.3086&0.0304&0.0166&0.2738&0.3525&0.0245&4.9558&4.7909&0.3086
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
2.45&0.02&30.86&3.04&1.66&27.38&35.25&2.45&495.58
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.012&0.0111&0.0514&0.0221&0.0211&0.2808&0.2164&0.012&1.0495%&0.9565&0.0514
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.0284&0.0261&0.1424&0.0458&0.0435&0.1126&0.1793&0.0284&30.5975%&28.9308&0.1424
\\
\hline
\multicolumn{2}{|c|}{Accuracy} & 0.0404&0.0371&0.1937&0.0679&0.0646&0.3935&0.3958&0.0404&31.647%&29.8873&0.1937
\\
% \hline
% \multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 2e-04&2e-04&4e-04&2e-04&2e-04&0.0441&0.0373&2e-04&0.0321&0.032&4e-04\\
% \hline
% \end{tabular}
% }
% \end{table}
% % START DATE AND TIME=20220518-13h02m59s
%       \begin{table}[htbp]
%   \centering
%   \caption{$\beta=1.5,  \sigma=1$ $n=500$}
%   \resizebox{\columnwidth}{!}{
%     \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|r|r|}
%       %\cline{2-13}    \multicolumn{1}{r|}{} &       & \multicolumn{11}{c|}{$\beta=1.5,  \sigma=1$ $n=500$} \\
% \cline{2-13}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.CvM}} & \multicolumn{1}{l|}{\textbf{MDE.LS}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.X2}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
  \multicolumn{11}{c}{$\beta=1.5,  \sigma=1$ $n=500$}\\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.5278&1.4982&1.6201&1.5399&1.5211&0.8576&0.9685&1.5278&2.3089%&2.2147&1.6201
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
1.0294&0.9985&1.1192&1.04&1.0235&1.0218&1.0596&1.0294&2.4912%&2.3498&1.1192
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.0317&0.029&0.0459&0.0638&0.0607&0.0525&0.0597&0.0317&0.0504%&0.063&0.0459
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.0335&0.0304&0.0493&0.0594&0.0566&0.0598&0.0594&0.0335&0.3038%&0.3159&0.0493
\\
\hline
%\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.0278&-0.0018&0.1201&0.0399&0.0211&-0.6424&-0.5315&0.0278&0.8089&0.7147&0.1201
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.8533&-0.12&8.0067&2.66&1.4067&-42.8267&-35.4333&1.8533&53.9267
\\
%\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
%0.0294&-0.0015&0.1192&0.04&0.0235&0.0218&0.0596&0.0294&1.4912&1.3498&0.1192
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
2.94&-0.15&11.92&4&2.35&2.18&5.96&2.94&149.12
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.0325&0.029&0.0603&0.0654&0.0612&0.4652&0.3422&0.0325&0.7047%&0.5737&0.0603
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.0343&0.0304&0.0635&0.061&0.0572&0.0603&0.063&0.0343&2.5276%&2.1377&0.0635
\\
\hline
\multicolumn{2}{|c|}{Accuracy } & 0.0668&0.0594&0.1238&0.1264&0.1183&0.5254&0.4052&0.0668&3.2323%&2.7114&0.1238
\\
\hline
% \multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 2e-04&2e-04&3e-04&2e-04&2e-04&0.026&0.0191&2e-04&0.0075&0.0072&3e-04\\
% \hline
% \end{tabular}
% }
% \end{table}
% % START DATE AND TIME=20220518-13h02m59s
%       \begin{table}[htbp]
%   \centering
%   \caption{$\beta=2,  \sigma=1$ $n=500$}
%   \resizebox{\columnwidth}{!}{
%     \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|r|r|}
%       %\cline{2-13}    \multicolumn{1}{r|}{} &       & \multicolumn{11}{c|}{$\beta=2,  \sigma=1$ $n=500$} \\
% \cline{2-13}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.CvM}} & \multicolumn{1}{l|}{\textbf{MDE.LS}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.X2}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
  \multicolumn{11}{c}{$\beta=2,  \sigma=1$ $n=500$}\\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.0492&1.9914&2.1127&2.0492&2.017&1.3236&1.4499&2.0492&2.6872%&2.5319&2.1127
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
1.0347&0.9935&1.0744&1.034&1.0142&1.0279&1.02&1.0347&1.6444%&1.5115&1.0744
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.0867&0.0752&0.1008&0.1682&0.1569&0.1752&0.1574&0.0867&0.1649%&0.1969&0.1008
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.0428&0.037&0.0491&0.0744&0.0696&0.1123&0.0878&0.0428&0.0893%&0.1153&0.0491
\\
\hline
%\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.0492&-0.0086&0.1127&0.0492&0.017&-0.6764&-0.5501&0.0492&0.6872&0.5319&0.1127
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 
2.46&-0.43&5.635&2.46&0.85&-33.82&-27.505&2.46&34.36
\\
%\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
%0.0347&-0.0065&0.0744&0.034&0.0142&0.0279&0.02&0.0347&0.6444&0.5115&0.0744
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
3.47&-0.65&7.44&3.4&1.42&2.79&2&3.47&64.44
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.0892&0.0753&0.1135&0.1706&0.1572&0.6328&0.46&0.0892&0.6371%&0.4798&0.1135
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.044&0.037&0.0546&0.0755&0.0698&0.1131&0.0882&0.044&0.5046%&0.3769&0.0546
\\
\hline
\multicolumn{2}{|c|}{Accuracy } & 0.1332&0.1123&0.1681&0.2461&0.227&0.7458&0.5482&0.1332&1.1417%&0.8567&0.1681
\\
\hline
% \multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 2e-04&2e-04&2e-04&2e-04&2e-04&0.0155&0.0098&2e-04&0.0014&0.0013&2e-04\\
% \hline
% \end{tabular}
% }
% \end{table}
% % START DATE AND TIME=20220518-13h02m59s
%       \begin{table}[htbp]
%   \centering
%   \caption{$\beta=2.1,  \sigma=1$ $n=500$}
%   \resizebox{\columnwidth}{!}{
%     \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|r|r|}
%       %\cline{2-13}    \multicolumn{1}{r|}{} &       & \multicolumn{11}{c|}{$\beta=2.1,  \sigma=1$ $n=500$} \\
% \cline{2-13}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.CvM}} & \multicolumn{1}{l|}{\textbf{MDE.LS}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.X2}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
  \multicolumn{11}{c}{$\beta=2.1,  \sigma=1$ $n=500$}\\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.1524&2.0876&2.2114&2.1581&2.1225&1.4255&1.5539&2.1524&2.774%&2.6089&2.2114
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
1.0349&0.9915&1.0692&1.0376&1.0169&1.0382&1.0259&1.0349&1.576%&1.4463&1.0692
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1012&0.0867&0.1129&0.2021&0.1876&0.2052&0.1823&0.1012&0.1915%&0.232&0.1129
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.0443&0.0378&0.0491&0.0792&0.0737&0.1209&0.0965&0.0443&0.0894%&0.1178&0.0491
\\
\hline
%\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.0524&-0.0124&0.1114&0.0581&0.0225&-0.6745&-0.5461&0.0524&0.674&0.5089&0.1114
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.4952&-0.5905&5.3048&2.7667&1.0714&-32.1190&-26.0048&2.4952&32.0952
\\
%\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
%0.0349&-0.0085&0.0692&0.0376&0.0169&0.0382&0.0259&0.0349&0.576&0.4463&0.0692
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
3.49&-0.85&6.92&3.76&1.69&3.82&2.59&3.49&5.76
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1039&0.0869&0.1253&0.2055&0.1881&0.6602&0.4805&0.1039&0.6457%&0.4909&0.1253
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.0455&0.0378&0.0539&0.0806&0.0739&0.1223&0.0971&0.0455&0.4212%&0.317&0.0539
\\
\hline
\multicolumn{2}{|c|}{Accuracy } & 0.1494&0.1247&0.1792&0.2861&0.2621&0.7825&0.5776&0.1494&1.0669%&0.8079&0.1792
\\
\hline
% \multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 2e-04&2e-04&2e-04&2e-04&2e-04&0.0142&0.0088&2e-04&0.0011&NaN&2e-04\\
% \hline
\end{tabular}
}
\end{table}


==> Tables20220525/output/output20220520/n500sig2.tex <==
% START DATE AND TIME=20220518-13h03m03s
      \begin{table}[htbp]
  \centering
%   \caption{$\beta=1.1,  \sigma=2$ $n=500$}
\caption{Comparison of different estimation methods for different values of $\beta$ ($\sigma=2$ and $n=500$). \label{tbl:n500sig2}}
%   \resizebox{\columnwidth}{!}{
%     \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|r|r|}
%       %\cline{2-13}    \multicolumn{1}{r|}{} &       & \multicolumn{11}{c|}{$\beta=1.1,  \sigma=2$ $n=500$} \\
% \cline{2-13}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.CvM}} & \multicolumn{1}{l|}{\textbf{MDE.LS}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.X2}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
\resizebox{1.3\textwidth}{!}{
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.CvM}} & \multicolumn{1}{l|}{\textbf{MDE.SD}} & \multicolumn{1}{l|}{\textbf{MDE.$\chi^2$}} & \multicolumn{1}{l|}{\textbf{MDE.TV}} &\multicolumn{1}{l|}{\textbf{MDE.KL}} & \multicolumn{1}{l|}{\textbf{MME}} \\
\cline{2-11}
  \multicolumn{11}{c}{$\beta=1.1,  \sigma=2$ $n=500$}\\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.118&1.1028&1.2901&1.1228&1.1121&0.4762&0.6528&1.118&2.122%&2.074&1.2901
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
2.0498&2.0011&2.6161&2.0618&2.0344&2.5698&2.6795&2.0498&12.3378%&12.0083&2.6161
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.0115&0.0108&0.0168&0.021&0.0202&10.6342&0.017&0.0115&0.0108%&0.0134&0.0168
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.11&0.103&0.1959&0.1743&0.168&2.2753&0.2117&0.11&72.915%&72.145&0.1959
\\
\hline
%\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.018&0.0028&0.1901&0.0228&0.0121&-0.6238&-0.4472&0.018&1.022&0.974&0.1901
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 
1.6364&0.2545&17.2818&2.0727&1.1&-56.7091&-40.6545&1.6364&92.9091
\\
%\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
%0.0498&0.0011&0.6161&0.0618&0.0344&0.5698&0.6795&0.0498&10.3378&10.0083&0.6161
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
2.49&0.055&30.805&3.09&1.72&28.49&33.975&2.49&516.89
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.0118&0.0108&0.0529&0.0215&0.0204&11.0223&0.2169&0.0118&1.0553%&0.9621&0.0529
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.1125&0.103&0.5755&0.1781&0.1692&2.5998&0.6734&0.1125&179.777%&172.3033&0.5755
\\
\hline
\multicolumn{2}{|c|}{Accuracy } & 0.1243&0.1138&0.6284&0.1996&0.1896&13.6221&0.8903&0.1243&180.8323%&173.2654&0.6284
\\
\hline
% \multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 2e-04&2e-04&4e-04&2e-04&2e-04&2.22455819348699e+298&0.037&2e-04&0.0326&0.0324&4e-04\\
% \hline
% \end{tabular}
% }
% \end{table}
% % START DATE AND TIME=20220518-13h03m03s
%       \begin{table}[htbp]
%   \centering
%   \caption{$\beta=1.5,  \sigma=2$ $n=500$}
%   \resizebox{\columnwidth}{!}{
%     \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|r|r|}
%       %\cline{2-13}    \multicolumn{1}{r|}{} &       & \multicolumn{11}{c|}{$\beta=1.5,  \sigma=2$ $n=500$} \\
% \cline{2-13}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.CvM}} & \multicolumn{1}{l|}{\textbf{MDE.LS}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.X2}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
\multicolumn{11}{c}{$\beta=1.5,  \sigma=2$ $n=500$}\\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.5243&1.4948&1.6233&1.5271&1.5085&0.8602&0.9719&1.5243&2.3125%&2.2191&1.6233
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
2.0507&1.9892&2.2438&2.0543&2.0219&2.0467&2.1227&2.0507&4.9648%&4.6844&2.2438
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.0314&0.0287&0.0452&0.057&0.0542&0.0524&0.0593&0.0314&0.0504%&0.0624&0.0452
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.1323&0.1203&0.1945&0.2106&0.2005&0.2391&0.2375&0.1323&1.0955%&1.1541&0.1945
\\
\hline
%\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.0243&-0.0052&0.1233&0.0271&0.0085&-0.6398&-0.5281&0.0243&0.8125&0.7191&0.1233
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 
1.62&-0.3467&8.22&1.8067&0.5667&-42.6533&-35.2067&1.62&54.1667
\\
%\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
%0.0507&-0.0108&0.2438&0.0543&0.0219&0.0467&0.1227&0.0507&2.9648&2.6844&0.2438
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
2.535&-0.54&12.19&2.715&1.095&2.335&6.135&2.535&148.24
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.032&0.0288&0.0604&0.0578&0.0543&0.4617&0.3382&0.032&0.7106%&0.5796&0.0604
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.1349&0.1204&0.254&0.2135&0.201&0.2413&0.2526&0.1349&9.8855%&8.3601&0.254
\\
\hline
\multicolumn{2}{|c|}{Accuracy } & 0.1669&0.1491&0.3144&0.2713&0.2553&0.703&0.5907&0.1669&10.5961%&8.9397&0.3144
\\
\hline
% \multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 2e-04&2e-04&3e-04&2e-04&2e-04&0.0258&0.0188&2e-04&0.0073&0.007&3e-04\\
% \hline
% \end{tabular}
% }
% \end{table}
% % START DATE AND TIME=20220518-13h03m03s
%       \begin{table}[htbp]
%   \centering
%   \caption{$\beta=2,  \sigma=2$ $n=500$}
%   \resizebox{\columnwidth}{!}{
%     \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|r|r|}
%       %\cline{2-13}    \multicolumn{1}{r|}{} &       & \multicolumn{11}{c|}{$\beta=2,  \sigma=2$ $n=500$} \\
% \cline{2-13}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.CvM}} & \multicolumn{1}{l|}{\textbf{MDE.LS}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.X2}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
 \multicolumn{11}{c}{$\beta=2,  \sigma=2$ $n=500$}\\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.0422&1.985&2.1075&2.0265&1.995&1.321&1.4472&2.0422&2.6861%&2.531&2.1075
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
2.0602&1.9786&2.1419&2.0388&2.0001&2.0539&2.0391&2.0602&3.2895%&3.0238&2.1419
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.0833&0.0724&0.0989&0.1405&0.1314&0.1751&0.1569&0.0833&0.1656%&0.1984&0.0989
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.1639&0.1417&0.1921&0.2505&0.2348&0.449&0.3485&0.1639&0.3398%&0.4464&0.1921
\\
\hline
%\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.0422&-0.015&0.1075&0.0265&-0.005&-0.679&-0.5528&0.0422&0.6861&0.531&0.1075
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} &
2.11&-0.75&5.375&1.325&-0.25&-33.95&-27.64&2.11&34.305
\\
%\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
%0.0602&-0.0214&0.1419&0.0388&1e-04&0.0539&0.0391&0.0602&1.2895&1.0238&0.1419
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
3.01&-1.07&7.095&1.94&0.005&2.695&1.955&3.01&64.475
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.0851&0.0726&0.1105&0.1412&0.1314&0.6362&0.4625&0.0851&0.6363%&0.4804&0.1105
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.1675&0.1421&0.2122&0.2519&0.2348&0.4519&0.35&0.1675&2.0025%&1.4945&0.2122
\\
\hline
\multicolumn{2}{|c|}{Accuracy } & 0.2526&0.2147&0.3227&0.3931&0.3662&1.0881&0.8125&0.2526&2.6388%&1.9749&0.3227
\\
\hline
% \multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 2e-04&2e-04&2e-04&2e-04&2e-04&0.0156&0.0099&2e-04&0.0014&0.0013&2e-04\\
% \hline
% \end{tabular}
% }
% \end{table}
% % START DATE AND TIME=20220518-13h03m03s
%       \begin{table}[htbp]
%   \centering
%   \caption{$\beta=2.1,  \sigma=2$ $n=500$}
%   \resizebox{\columnwidth}{!}{
%     \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|r|r|}
%       %\cline{2-13}    \multicolumn{1}{r|}{} &       & \multicolumn{11}{c|}{$\beta=2.1,  \sigma=2$ $n=500$} \\
% \cline{2-13}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.CvM}} & \multicolumn{1}{l|}{\textbf{MDE.LS}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.X2}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
\multicolumn{11}{c}{$\beta=2.1,  \sigma=2$ $n=500$}\\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.1444&2.0802&2.2041&2.1286&2.0941&1.4203&1.5468&2.1444&2.7706%&2.6049&2.2041
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
2.0599&1.9739&2.1292&2.0394&1.9992&2.0719&2.0449&2.0599&3.1525%&2.8917&2.1292
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.0992&0.0851&0.1136&0.1636&0.1524&0.2076&0.184&0.0992&0.1941%&0.2356&0.1136
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.1749&0.1493&0.1979&0.2614&0.2442&0.4882&0.3875&0.1749&0.3666%&0.4819&0.1979
\\
\hline
%\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.0444&-0.0198&0.1041&0.0286&-0.0059&-0.6797&-0.5532&0.0444&0.6706&0.5049&0.1041
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.1143&-0.9429&4.9571&1.3619&-0.2810&-32.3667&-26.3429&2.1143&31.9333
\\
%\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
%0.0599&-0.0261&0.1292&0.0394&-8e-04&0.0719&0.0449&0.0599&1.1525&0.8917&0.1292
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
2.995&-1.305&6.46&1.97&-0.04&3.595&2.245&2.995&57.625
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.1011&0.0854&0.1245&0.1644&0.1524&0.6695&0.4899&0.1011&0.6438%&0.4905&0.1245
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.1785&0.15&0.2145&0.2629&0.2441&0.4933&0.3895&0.1785&1.6949%&1.2771&0.2145
\\
\hline
\multicolumn{2}{|c|}{Accuracy } & 0.2796&0.2354&0.339&0.4273&0.3966&1.1629&0.8794&0.2796&2.3386%&1.7676&0.339
\\
\hline
% \multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 2e-04&2e-04&2e-04&2e-04&2e-04&0.0143&0.0089&2e-04&0.0011&NaN&2e-04\\
% \hline
\end{tabular}
}
\end{table}

==> Tables20220525/output/output20220520/n50sig05.tex <==
% START DATE AND TIME=20220517-11h19m22s
      \begin{table}[htbp]
  \centering
%   \caption{$\beta=1.1,  \sigma=0.5$ $n=50$}
\caption{Comparison of different estimation methods for different values of $\beta$ ($\sigma=0.5$ and $n=50$). \label{tbl:n50sig05}}
%   \resizebox{\columnwidth}{!}{
%     \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|r|r|}
%       %\cline{2-13}    \multicolumn{1}{r|}{} &       & \multicolumn{11}{c|}{$\beta=1.1,  \sigma=0.5$ $n=50$} \\
% \cline{2-13}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.CvM}} & \multicolumn{1}{l|}{\textbf{MDE.LS}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.X2}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
%     \hline
\resizebox{1.3\textwidth}{!}{
    \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|}
\cline{2-11}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.CvM}} & \multicolumn{1}{l|}{\textbf{MDE.SD}} & \multicolumn{1}{l|}{\textbf{MDE.$\chi^2$}} & \multicolumn{1}{l|}{\textbf{MDE.TV}} &\multicolumn{1}{l|}{\textbf{MDE.KL}} & \multicolumn{1}{l|}{\textbf{MME}} \\
\cline{2-11}
  \multicolumn{11}{c}{$\beta=1.1,  \sigma=0.5$ $n=50$}\\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 1.3505&1.1325&1.6196&1.2905&1.1478&0.8498&1.5689&1.3505&2.8314%&0.4477&1.6196
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.7021&0.5219&0.9134&0.6496&0.5534&1.343&2.3115&0.7022&3.0522%&0.7792&0.9134
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.1236&2.058&0.2486&0.3516&0.2095&15.3211&56.3549&2.131&7.4458%&326.2685&0.2486
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
1.293&1.2445&0.1798&0.1872&0.1138&19.7277&146.2716&1.2975&5.1888%&245.6358&0.1798
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.2505&0.0325&0.5196&0.1905&0.0478&-0.2502&0.4689&0.2505&1.7314%&-0.6523&0.5196
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.2021&0.0219&0.4134&0.1496&0.0534&0.843&1.8115&0.2022&2.5522%&0.2792&0.4134
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.1861&2.0588&0.5186&0.3878&0.2118&15.3822&56.5691&2.1936&10.4427%&326.6613&0.5186
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
1.3337&1.2448&0.3507&0.2096&0.1166&20.4364&149.5386&1.3383&11.702%&245.6892&0.3507
\\
\hline
\multicolumn{2}{|c|}{Accuracy } & 3.5199&3.3037&0.8692&0.5974&0.3284&35.8186&206.1077&3.5319&22.1447%&572.3505&0.8692
\\
\hline
% \multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0022&0.0022&0.0025&0.0023&0.0023&1.42350934291955e+299&0.0515&0.0022&0.0197&NaN&0.0025\\
% \hline
% \end{tabular}
% }
% \end{table}
% % START DATE AND TIME=20220517-11h19m22s
%       \begin{table}[htbp]
%   \centering
%   \caption{$\beta=1.5,  \sigma=0.5$ $n=50$}
%   \resizebox{\columnwidth}{!}{
%     \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|r|r|}
%       %\cline{2-13}    \multicolumn{1}{r|}{} &       & \multicolumn{11}{c|}{$\beta=1.5,  \sigma=0.5$ $n=50$} \\
% \cline{2-13}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.CvM}} & \multicolumn{1}{l|}{\textbf{MDE.LS}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.X2}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
  \multicolumn{11}{c}{$\beta=1.5,  \sigma=0.5$ $n=50$}\\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.1256&1.8074&2.0032&1.7383&1.4936&1.7147&3.1381&1.8863&3.6846%&-7.8269&2.0032
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.8612&0.6853&0.7742&0.6472&0.5337&1.5713&2.893&0.7327&2.1393%&-4.3409&0.7742
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 595.2731&595.4835&1.6249&3.5241&1.5645&66.0963&198.1615&9.9703&783.02%&359505.886&1.6249
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
172.6361&172.6916&0.3901&0.7099&0.3473&63.1345&193.3304&2.5872&226.8672%&100522.7452&0.3901
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.6256&0.3074&0.5032&0.2383&-0.0064&0.2147&1.6381&0.3863&2.1846%&-9.3269&0.5032
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.3612&0.1853&0.2742&0.1472&0.0337&1.0713&2.393&0.2327&1.6393%&-4.8409&0.2742
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 595.6049&595.5185&1.878&3.5805&1.5644&66.1358&200.8249&10.1185&787.7142%&359556.927&1.878
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
172.7493&172.7086&0.4653&0.7315&0.3484&64.2759&199.0377&2.6411&229.5318%&100536.1272&0.4653
\\
\hline
\multicolumn{2}{|c|}{Accuracy } & 768.3542&768.2271&2.3433&4.312&1.9128&130.4117&399.8627&12.7596&1017.246%&460093.0542&2.3433
\\
\hline
% \multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0022&0.0023&0.0021&0.0023&0.0024&0.05&0.0429&0.0022&0.0113&NaN&0.0021\\
% \hline
% \end{tabular}
% }
% START DATE AND TIME=20220517-11h19m22s
%       \begin{table}[htbp]
%   \centering
%   \caption{$\beta=2,  \sigma=0.5$ $n=50$}
%   \resizebox{\columnwidth}{!}{
%     \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|r|r|}
%       %\cline{2-13}    \multicolumn{1}{r|}{} &       & \multicolumn{11}{c|}{$\beta=2,  \sigma=0.5$ $n=50$} \\
% \cline{2-13}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.CvM}} & \multicolumn{1}{l|}{\textbf{MDE.LS}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.X2}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
%     \hline
  \multicolumn{11}{c}{$\beta=2,  \sigma=0.5$ $n=50$}\\
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 2.5936&2.2447&2.5912&2.3667&1.9728&2.6719&5.4332&2.5481&4.2315%&-3.6556&2.5912
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.7568&0.623&0.733&0.6688&0.5374&1.6134&3.3078&0.7398&1.5532%&-1.6979&0.733
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 55.4376&55.9003&19.9251&29.0259&20.0825&145.0452&446.9227&32.0439&78.0783%&2334.4605&19.9251
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
7.5856&7.6434&2.4641&3.4602&2.4737&57.5669&181.2889&4.2284&11.1352%&484.4018&2.4641
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 0.5936&0.2447&0.5912&0.3667&-0.0272&0.6719&3.4332&0.5481&2.2315%&-5.6556&0.5912
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
0.2568&0.123&0.233&0.1688&0.0374&1.1134&2.8078&0.2398&1.0532%&-2.1979&0.233
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 55.7843&55.9546&20.2726&29.1575&20.0813&145.4821&458.6648&32.3411&83.0499%&2366.2126&20.2726
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
7.6508&7.6578&2.5181&3.4883&2.4748&58.8008&189.1548&4.2855&12.2433%&489.1843&2.5181
\\
\hline
\multicolumn{2}{|c|}{Accuracy } & 63.4351&63.6124&22.7907&32.6458&22.5561&204.2829&647.8195&36.6265&95.2932%&2855.397&22.7907
\\
\hline
% \multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0023&0.0025&0.0021&0.0025&0.0026&0.0421&0.0355&0.0023&0.0063&NaN&0.0021\\
% \hline
% \end{tabular}
% }
% \end{table}
% \end{table}
% % START DATE AND TIME=20220517-11h19m22s
%       \begin{table}[htbp]
%   \centering
%   \caption{$\beta=2.1,  \sigma=0.5$ $n=50$}
%   \resizebox{\columnwidth}{!}{
%     \begin{tabular}{|cc|r|r|r|r|r|r|r|r|r|r|r|}
%       %\cline{2-13}    \multicolumn{1}{r|}{} &       & \multicolumn{11}{c|}{$\beta=2.1,  \sigma=0.5$ $n=50$} \\
% \cline{2-13}    \multicolumn{1}{r|}{} & \textbf{METHODS} & \multicolumn{1}{l|}{\textbf{MLE}} & \multicolumn{1}{l|}{\textbf{MLE.b}} & \multicolumn{1}{l|}{\textbf{LME}} & \multicolumn{1}{l|}{\textbf{MDE.CvM}} & \multicolumn{1}{l|}{\textbf{MDE.LS}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.X2}} & \multicolumn{1}{l|}{\textbf{MDE.Phi.tv}} &\multicolumn{1}{l|}{\textbf{MDE.Phi.kl}} & \multicolumn{1}{l|}{\textbf{MME}} & \multicolumn{1}{l|}{\textbf{MME.b}} & \multicolumn{1}{l|}{\textbf{PWM}} \\
  \multicolumn{11}{c}{$\beta=2.1,  \sigma=0.5$ $n=50$}\\
    \hline
\multirow{2}[4]{*}{Mean} & \multicolumn{1}{|c|}{$\widehat\beta$} & 5.4872&5.1504&2.8263&2.6476&2.1967&3.0372&5.8801&2.8915&7.73%&-6.0869&2.8263
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
1.5554&1.4333&0.7672&0.7256&0.5805&1.7091&3.2875&0.8178&2.4879%&-2.7979&0.7672
\\
\hline
\multirow{2}[4]{*}{Var} & \multicolumn{1}{|c|}{$\widehat\beta$} & 22917.9041&22920.2999&31.9911&43.1895&32.2829&185.326&491.6256&56.3596&34127.8431%&87992.3932&31.9911
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
1665.5491&1665.8037&3.3274&4.6126&3.3872&61.7311&162.781&7.0081&2700.7557%&11608.1913&3.3274
\\
\hline
\multirow{2}[4]{*}{Bias} & \multicolumn{1}{|c|}{$\widehat\beta$} & 3.3872&3.0504&0.7263&0.5476&0.0967&0.9372&3.7801&0.7915&5.63%&-8.1869&0.7263
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
1.0554&0.9333&0.2672&0.2256&0.0805&1.2091&2.7875&0.3178&1.9879%&-3.2979&0.2672
\\
\hline
\multirow{2}[4]{*}{MSE} & \multicolumn{1}{|c|}{$\widehat\beta$} & 22927.0854&22927.3131&32.5154&43.4851&32.289&186.1858&505.8659&56.9805&34156.1274%&88050.6198&32.5154
\\
\cline{2-11}          & \multicolumn{1}{|c|}{$\widehat\sigma$} &
1666.4965&1666.5081&3.3984&4.663&3.3934&63.1869&170.5348&7.1084&2704.4376%&11617.9064&3.3984
\\
\hline
\multicolumn{2}{|c|}{Accuracy } & 24593.5819&24593.8212&35.9138&48.148&35.6823&249.3727&676.4007&64.0889&36860.5649%&99668.5261&35.9138
\\
% \hline
% \multicolumn{2}{|c|}{Accuracy (DF sq.diff.)} & 0.0024&0.0026&0.0021&0.0026&0.0027&0.0415&0.0348&0.0024&0.0059&NaN&0.0021\\
\hline
\end{tabular}
}
\end{table}




